On Guillotine Separable Packings for the Two-dimensional Geometric Knapsack Problem

In two-dimensional geometric knapsack problem, we are given a set of n axis-aligned rectangular items and an axis-aligned square-shaped knapsack. Each item has integral width, integral height and an associated integral profit. The goal is to find a (non-overlapping axis-aligned) packing of a maximum profit subset of rectangles into the knapsack. A well-studied and frequently used constraint in practice is to allow only packings that are guillotine separable, i.e., every rectangle in the packing can be obtained by recursively applying a sequence of edge-to-edge axis-parallel cuts that do not intersect any item of the solution. In this paper we study approximation algorithms for the geometric knapsack problem under guillotine cut constraints. We present polynomial time (1 + {\epsilon})-approximation algorithms for the cases with and without allowing rotations by 90 degrees, assuming that all input numeric data are polynomially bounded in n. In comparison, the best-known approximation factor for this setting is 3 + {\epsilon} [Jansen-Zhang, SODA 2004], even in the cardinality case where all items have the same profit. Our main technical contribution is a structural lemma which shows that any guillotine packing can be converted into another structured guillotine packing with almost the same profit. In this packing, each item is completely contained in one of a constant number of boxes and L-shaped regions, inside which the items are placed by a simple greedy routine. In particular, we provide a clean sufficient condition when such a packing obeys the guillotine cut constraints which might be useful for other settings where these constraints are imposed.

==> 2_Preliminaries.tex <==
\section{Preliminaries}
\label{sec:prelim}
Let $\mathbb{N}$ (resp.~$\mathbb{N}_0$) be the set of positive (resp.~non-negative) integers. 
Let  $[n]:=\{1, 2, \dots, n\}$. 
A  {\em piece} is  an axis-aligned rectangular region with non-overlapping axis-aligned rectangles $\mathcal{R}:=[n]$ embedded on it. 
A {\em guillotine cut} for a piece $P$ is an end-to-end axis-parallel cut along a straight line $\ell$ dividing the piece into two nonempty {\em subpieces} $P_1$, $P_2$. 

\begin{obs} \label{endtoend}
Given a piece containing a set of guillotine separable rectangles, there must exist an end-to-end guillotine cut in the piece. 
%In other words, the first level of guillotine cuts in the piece is end-to-end.
\end{obs}

A {\em pseudorectangle} (or pseudoitem) is a guillotine-separable rectangular region with embedded items inside it. Sometimes we will treat this whole region as a single item.
A horizontal cut $l_{h}$ is said to be {\em intercepted} by a vertical cut $l_{v}$ if $l_{v}$ occurs before $l_{h}$ in the guillotine cutting sequence and $l_{h}$ touches $l_{v}$ at point $p$ but does not cross it. If an edge $e$ of a pseudorectangle (resp. rectangle) coincides with $l_{v}$ and point $p$ is part of edge $e$, then we say that the pseudorectangle (resp. rectangle)  {\em intercepts} the cut $l_{h}$.
%\arir{Arnab, added this definition of pseudoitem. modify it if needed.}

%%%%%%%%%%%
\subsection{Classification of rectangles}
We classify the input items according to their heights and widths, as done in \cite{GalvezGHI0W17}. 
For two given constants  $1 \geq \epsl > \epss >  0$, we classify an item $i$ as: 
		\begin{itemize}
		\item {\em Large}: $\width_{i} \ > \epsl N$ and $\height_{i} \ > \epsl N$;
		\item {\em Small}: $\width_{i} \leq \epss N$ and $\height_{i} \leq \epss N$;
		\item {\em Horizontal}: $\width_{i} \ > \epsl N$ and $\height_{i} \leq \epss N$;
		\item {\em Vertical}: $\height_{i} \ > \epsl N$ and $\width_{i} \leq \epss N$;
		\item {\em Intermediate:} Either $\epsl N \geq \height_{i} \ > \epss N$ or  $\epsl N \geq \width_{i} \ >  \epss N$.	
		\end{itemize}
Using standard shifting arguments, one can show that we can ignore intermediate items.

\begin{lem}  \label{class}
\cite{GalvezGHI0W17}
Let $\eps>0$ and $f(.)$ be any positive increasing function such that $f(x)<x$ $\forall x \in (0,1]$. Then we can efficiently find $\epsl, \epss \in \Omega_\eps(1)$, with $\eps \ge f(\eps) \ge \epsl \ge f(\epsl) \ge \epss$ so that the total profit of intermediate rectangles is at most $\eps \profit(\opt)$. 
\end{lem}		
		
\noindent We define {\em skewed} items to be items that are horizontal or vertical.  
%We define orientation of a skewed item to be  horizontal (resp., vertical) if the item is horizontal (resp., horizontal).  
An item is {\em wide}  if  $\width_{i} > \frac{N}{2}$ and {\em tall}  if  $\height_{i}  > \frac{N}{2}$.
{\em Long} items are either tall or wide. Items that are not long are called {\em short}. 
Long and skewed items  play a special role in our algorithms. 
%, i.e., for short items $\width_{i} \leq \frac{N}{2}$ and $\height_{i} \leq \frac{N}{2}$.
Let $\Rla$, $\Rsm$, $\Rho, \Rve, \Rsk, \Rwi, \Rta, \Rln, \Rsht$ be the set of large, small, horizontal, vertical, intermediate, skewed, wide, tall, long and short rectangles, respectively. The corresponding intersections with $\opt$ (the optimal guillotine packing) defines the sets $\optla$, $\optsm$, $\optho,$ $\optve, \optsk,$ $\optwi, \optta, \optln, \optsh$, respectively. 
%Now onwards, whenever we mention $\opt$ or related terms, we intend to mention the optimal guillotine packing.

\subsection{Corridor decomposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Figs::begin

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.25\textwidth}
		\centering
		\resizebox{!}{2cm}{
		\begin{tikzpicture}
			
			\draw[thick] (0,3)--(3,3)--(3,1)--(5,1)--(5,3)--(6,3)--(6,0)--(2,0)--(2,2)--(0,2)--(0,3);
			%bends
			\draw[dotted] (2,0)--(3,1);
			\draw[dotted] (2,2)--(3,3);
			\draw[dotted] (6,0)--(5,1);
			%cuts
			\draw[dashed] (1,2)--(1,3);
			\draw (1.2,2.5) node {\large \textbf{$l_{1}$}};
			\draw[dashed] (2,1.5)--(3,1.5);
			\draw (2.5,1.7) node {\large \textbf{$l_{2}$}};
			\draw[dashed] (5,2)--(6,2);
			\draw (5.5,2.3) node {\large \textbf{$l_{4}$}};
			\draw[dashed] (4,0)--(4,1);
			\draw (4.3,.5) node {\large \textbf{$l_{3}$}};
			%edges
			\draw (-.3,2.5) node {\large \textbf{$e_{0}$}};
			\draw (1,1.7) node {\large \textbf{$e_{1}$}};
			\draw (1.7,1) node {\large \textbf{$e_{2}$}};
			\draw (4,-.5) node {\large \textbf{$e_{3}$}};
			\draw (6.3,1.5) node {\large \textbf{$e_{4}$}};
			\draw (5.5,3.2) node {\large \textbf{$e_{5}$}};
			\draw (4.7,2) node {\large \textbf{$e_{6}$}};
			\draw (4,1.2) node {\large \textbf{$e_{7}$}};
			\draw (3.2,2) node {\large \textbf{$e_{8}$}};
			\draw (1.5,3.2) node {\large \textbf{$e_{9}$}};
		\node[below,scale=2] at (2,0) {(a)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c11}
	\end{subfigure}
	\begin{subfigure}[b]{.22\textwidth}
		\centering
		\resizebox{!}{2.05cm}{
		\begin{tikzpicture}		
			\draw[thick](0,0)--(0,4)--(2,4)--(2,6)--(6,6)--(6,0)--(0,0);
			\draw[thick](1,1)--(1,3)--(3,3)--(3,5)--(5,5)--(5,1)--(1,1);
			% boundary curves
			\draw[dotted](0,0)--(1,1);
			\draw[dotted](6,0)--(5,1);
			\draw[dotted](5,5)--(6,6);
			\draw[dotted](0,4)--(1,3);
			\draw[dotted](2,4)--(3,3);
			\draw[dotted](2,6)--(3,5);
			% edges
			\draw (-.3,2) node {\large \textbf{$e_{0}$}};
			\draw (3,-.3) node {\large \textbf{$e_{1}$}};
			\draw (6.3,3) node {\large \textbf{$e_{2}$}};
			\draw (4,6.3) node {\large \textbf{$e_{3}$}};
			\draw (1.7,5) node {\large \textbf{$e_{4}$}};
			\draw (1,4.3) node {\large \textbf{$e_{5}$}};
			\draw (1.3,2) node {\large \textbf{$e_{0}'$}};
			\draw (3,1.3) node {\large \textbf{$e_{1}'$}};
			\draw (4.7,3) node {\large \textbf{$e_{2}'$}};
			\draw (4,4.7) node {\large \textbf{$e_{3}'$}};
			\draw (3.3,4) node {\large \textbf{$e_{4}'$}};
			\draw (2,2.7) node {\large \textbf{$e_{5}'$}};

		\node[below,scale=2] at (2,0) {(b)};				
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c12}
	\end{subfigure}
	\begin{subfigure}[b]{.22\textwidth}
		\centering
		\resizebox{!}{2.1cm}{
		\begin{tikzpicture}		
			\draw[thick](0,0) rectangle (6,6);
			%items
			\draw[fill=lightgray] (0,0)--(6,0)--(6,2.8)--(1.5,2.8)--(1.5,6)--(0,6)--(0,0);
			\draw[solid, fill=gray] (6,0) rectangle (.7,.7);
			\draw[solid, fill=gray] (6,0.7) rectangle (1.5,1.4);
			\draw[solid, fill=gray] (6,1.4) rectangle (2,2.1);
			\draw[solid, fill=gray] (6,2.1) rectangle (2.5,2.8);

			\draw[solid, fill=gray] (0,6) rectangle (.5,.3);
			\draw[solid, fill=gray] (.5,6) rectangle (1,1.7);
			\draw[solid, fill=gray] (1,6) rectangle (1.5,2);
		
			\draw (6.5,1.4) node {\large \textbf{$K_{1}$}};
			\draw (.7,6.5) node {\large \textbf{$K_{2}$}};
			\draw (5.6,6.3) node {\large \textbf{$K\times K$}};

			
			\draw [thick,decorate,decoration={brace,amplitude=8pt}] (0,6) -- (1.5,6); 

			\draw [thick,decorate,decoration={brace,amplitude=8pt}] (6,2.8) -- (6,0); 
		\node[below,scale=2] at (2,0) {(c)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c13}
	\end{subfigure}
	\begin{subfigure}[b]{.22\textwidth}
		\centering
		\resizebox{!}{1.89cm}{
		\begin{tikzpicture}		
			\draw[thick](0,0) rectangle (6,6);
						
			\draw[fill=lightgray] (0,0)--(6,0)--(6,1.8)--(1.5,1.8)--(1.5,6)--(0,6)--(0,0);
			\draw[solid, fill=gray] (6,0) rectangle (.7,.7);
			\draw[solid, fill=gray] (6,0.7) rectangle (1.5,1.1);
			\draw[solid, fill=gray] (6,1.1) rectangle (2,1.4);
			\draw[solid, fill=gray] (6,1.4) rectangle (2.5,1.8);

			\draw[solid, fill=gray] (0,6) rectangle (.5,.3);
			\draw[solid, fill=gray] (.5,6) rectangle (1,1.7);
			\draw[solid, fill=gray] (1,6) rectangle (1.5,2);

			% small item container and rectangles
			\draw[fill=lightgray](1.5,1.8) rectangle (3.8,3);
			\draw[solid, fill=gray] (1.55,1.805) rectangle (2.05,2.5);
			\draw[solid, fill=gray] (2.05,1.805) rectangle (2.55,2.4);
			\draw[solid, fill=gray] (2.55,1.805) rectangle (2.95,2.3);
			\draw[solid, fill=gray] (2.95,1.805) rectangle (3.35,2.1);
			\draw[solid, fill=gray] (3.35,1.805) rectangle (3.65,2);

			\draw[solid, fill=gray] (1.55,2.5) rectangle (1.85,3);
			\draw[solid, fill=gray] (1.85,2.5) rectangle (2.35,2.9);
			\draw[solid, fill=gray] (2.35,2.5) rectangle (2.65,2.8);
			\draw[solid, fill=gray] (2.65,2.5) rectangle (2.95,2.7);
			\draw[solid, fill=gray] (2.95,2.5) rectangle (3.35,2.6);
			
			% horizontal containers and rectangles
			\draw[fill=lightgray](1.5, 3.8) rectangle (3.3,6);

			\draw[solid, fill=gray] (1.55,3.8)rectangle(3.25,4.1);
			\draw[solid, fill=gray] (1.55,4.1)rectangle(3.2,4.4);
			\draw[solid, fill=gray] (1.55,4.4)rectangle(3.1,4.7);			
			\draw[solid, fill=gray] (1.55,4.7)rectangle(3,5);
			\draw[solid, fill=gray] (1.55,5)rectangle(2.9,5.2);
			\draw[solid, fill=gray] (1.55,5.2)rectangle(2.8,5.4);
			\draw[solid, fill=gray] (1.55,5.4)rectangle(2.7,5.6);
			\draw[solid, fill=gray] (1.55,5.6)rectangle(2.6,5.8);
			\draw[solid, fill=gray] (1.55,5.8)rectangle(2.5,5.9);


			
			% vertical container and rectangles
			\draw[fill=lightgray](3.6,3.5) rectangle (5.5,6);
			
			\draw[solid, fill=gray] (3.65,5.96)rectangle(3.78,3.55);
			\draw[solid, fill=gray] (3.78,5.96)rectangle(4,3.68);
			\draw[solid, fill=gray] (4,5.96)rectangle(4.28,3.9);
			\draw[solid, fill=gray] (4.28,5.96)rectangle(4.5,4);
			\draw[solid, fill=gray] (4.5,5.96)rectangle(4.85,4.15);
			\draw[solid, fill=gray] (4.85,5.96)rectangle(5.1,4.26);
			\draw[solid, fill=gray] (5.1,5.96)rectangle(5.45,4.36);

			\draw [solid, fill=gray] (4.5,1.9) rectangle (5.7,3.4);

			
		\node[below,scale=2] at (2,0) {(d)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c14}
	\end{subfigure}
	\caption{(a) Open corridor ($b=5$), (b) Closed corridor ($b=6$), (c) Boundary-$\Lc$ (height $K_{1}$, width $K_{2}$), (d) $L\&C$-packing: long \& short items packed in boundary-$\Lc$ \&  containers (4 types), resp.}
	\label{fig:c1}
\end{figure}

\vspace{-4mm}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.02\textwidth}
		\centering
		\resizebox{!}{1cm}{
		\begin{tikzpicture}			
			\draw[solid, fill=lightgray] (0,0) rectangle (1,4);
		\node[below,scale=2] at (2,0) {(a)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c21}
	\end{subfigure}
	\begin{subfigure}[b]{.11\textwidth}
		\centering
		\resizebox{!}{1cm}{
		\begin{tikzpicture}		
			\draw[solid, fill=lightgray](0,0)--(0,4)--(1,4)--(1,1)--(4,1)--(4,0)--(0,0);		
			\draw[dotted] (0,0)--(1,1);	
		\node[below,scale=2] at (2,0) {(c)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c22}
	\end{subfigure}
	\begin{subfigure}[b]{.13\textwidth}
		\centering
		\resizebox{!}{1.2cm}{
		\begin{tikzpicture}		
			\draw[solid, fill=lightgray](0,0)--(3,0)--(3,2)--(2.3,2)--(2.3,.5)--(.7,.5)--(.7,2)--(0,2)--(0,0);
			\draw[dotted](0,0)--(.7,.5);
			\draw[dotted](3,0)--(2.3,.5);
		\node[below,scale=2] at (2,0) {(c)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c23}
	\end{subfigure}
	\begin{subfigure}[b]{.15\textwidth}
		\centering
		\resizebox{!}{1.2cm}{
		\begin{tikzpicture}		
			\draw[solid, fill=lightgray](0,0)--(5,0)--(5,3)--(3,3)--(3,2)--(4,2)--(4,1)--(1,1)--(1,2)--(0,2)--(0,0);
			\draw[dotted](0,0)--(1,1);
			\draw[dotted](5,0)--(4,1);
			\draw[dotted](4,2)--(5,3);			
		\node[below,scale=2] at (2,0) {(d)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c24}
	\end{subfigure}
	\begin{subfigure}[b]{.15\textwidth}
		\centering
		\resizebox{!}{1.2cm}{
		\begin{tikzpicture}		
			\draw[solid, fill=lightgray] (0,3)--(3,3)--(3,1)--(5,1)--(5,0)--(2,0)--(2,2)--(0,2)--(0,3);
			\draw[dotted] (2,2)--(3,3);
			\draw[dotted] (2,0)--(3,1);
			
			\draw (1,2.5) node {\large \textbf{$S_{i}$}};
			\draw (2.5,1.5) node {\large \textbf{$S_{i'}$}};
			\draw (4,.5) node {\large \textbf{$S_{i''}$}};
		\node[below,scale=2] at (2,0) {(e)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c25}
	\end{subfigure}
	\begin{subfigure}[b]{.15\textwidth}
		\centering
		\resizebox{!}{1.7cm}{
		\begin{tikzpicture}		
\draw[solid, fill=lightgray](0,0)--(6,0)--(6,6)--(0,6)--(0,0)--(.1,0)--(.1,.1)--(.2,.1)--(.2,.2)--(.3,.2)--(.3,.3)--(.4,.3)--(.4,.4)--(.5,.4)--(.5,.5)--(.5,5.5)--(5.5,5.5)--(5.5,.5)--(.5,.5);
			
			\draw[dotted](0,6)--(0.5,5.5);
			\draw[dotted](6,6)--(5.5,5.5);
			\draw[dotted](6,0)--(5.5,0.5);
			
			\draw[solid, fill=gray] (3,.7)--(.7,.7)--(.7,5.1)--(5.1,5.1)--(5.1,1.5)--(1.5,1.5)--(1.5,4.3)--(4.3,4.3)--(4.3,2.2)--(2.2,2.2)--(2.2,3.5)--(2.5,3.5)--(2.5,2.6)--(3.9,2.6)--(3.9,3.9)--(1.9,3.9)--(1.9,1.9)--(4.7,1.9)--(4.7,4.7)--(1.1,4.7)--(1.1,1.1)--(3,1.1)--(3,.7);
		\node[below,scale=2] at (2,0) {(f)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c26}
	\end{subfigure}
	\begin{subfigure}[b]{.15\textwidth}
		\centering
		\resizebox{!}{1.5cm}{
		\begin{tikzpicture}		
			\draw[solid, fill=lightgray] (0,3)--(3,3)--(3,1)--(5,1)--(5,3)--(6,3)--(6,0)--(2,0)--(2,2)--(0,2)--(0,3);
			%bends
			\fill[pattern=north west lines] (2,0)rectangle(3,1);
			\fill[pattern=north west lines] (2,2)rectangle(3,3);
			\fill[pattern=north west lines] (6,0)rectangle(5,1);
			%\fill[pattern=north west lines] (0,3)--(3,3)--(3,1)--(5,1)--(5,0)--(2,0)--(2,2)--(0,2)--(0,3);
			%\fill[pattern=north east lines] (5,0)--(5,3)--(6,3)--(6,0)--(5,0);
			\draw (1,2.5) node {\large \textbf{$S_{1}$}};
			\draw (2.5,1.5) node {\large \textbf{$S_{2}$}};
			\draw (4,.5) node {\large \textbf{$S_{3}$}};
			\draw (5.5,2) node {\large \textbf{$S_{4}$}};

			\draw (3.2,3.2) node {\large \textbf{$S_{12}$}};			
			\draw (1.8,-.2) node {\large \textbf{$S_{23}$}};
			\draw (6.2,-.2) node {\large \textbf{$S_{34}$}};		
		\node[below,scale=2] at (2,0) {(g)};	
		\end{tikzpicture}}
		%\caption{}
		\label{fig:c27}
	\end{subfigure}
	\caption{Types of corridors: (a):$\Bc$, (b):$\Lc$, (c):$\Uc$, (d):$\Gc$, (e):$\Zc$, (f): {\em spiral} (darkgray), {\em ring} (gray), (g): $S_{1}, S_{2}, S_{3}$ form $\Zc$-bend, $S_{4}$ is a spiral subcorridor. Shaded region $S_{i,i+1}=S_i \cap S_{i+1}$ for $i \in [3]$.} 
	\label{fig:c2}
\end{figure}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Figs::end

%Most of the geometric packing algorithms works as follows. Start with an optimal packing, and {\em rearrange} the items to show the existence of a {\em structured} packing with high profit and then show a constructive efficient algorithm which can approximately  find such a structured packing.
\noindent Adamaszek et al. \cite{adamaszek2015knapsack} introduced corridor decomposition to decompose the optimal solution into simpler substructures, called {\em corridors}, without losing much profit. Corridors are then {\em processed} to obtain {\em containers}, which can be found efficiently. 
G{\'a}lvez et al.~\cite{GalvezGHI0W17} build on this idea and we will also follow similar notations and definitions (see Figure \ref{fig:c1} and \ref{fig:c2}).

\begin{definition}[Open corridor]
An open corridor is a subregion of knapsack bounded by simple rectilinear polygon with $2b$ edges $e_0, e_1, \dots, e_{2b-1}$ for $b \ge 2, b \in \mathbb{N}$, so that for each pair of horizontal (resp. vertical) edges $e_i, e_{2b-i}, i \in [b-1]$ there exists a vertical (resp. horizontal) line segment $\ell_i$ such that both $e_i$ and $e_{2b-i}$ intersect $\ell_i$ but no other edges intersect $\ell_i$. 
\end{definition}

\begin{definition}[Closed corridor]
A closed corridor (or {\em cycle}) is a subregion of knapsack bounded by two simple rectilinear polygon 
defined by edges  $e_0, e_1, \dots, e_{b-1}$ and $e'_0, e'_1, \dots, e'_{b-1}$ for $b \ge 2, b \in \mathbb{N}$, so that 
the second polygon is contained within the first polygon and 
for each pair of horizontal (resp.~vertical) edges $e_i, e'_{i}, i \in [b-1]$, there exists a vertical (resp.~horizontal) line segment $\ell_i$ such that  $e_i$ and $e'_{i}$ intersect $\ell_i$ but no other edges intersect $\ell_i$. \end{definition}

The {\em width} of a corridor is the maximum length of any such $\ell_i$ for $i \in [b-1]$.
An open (resp.~closed) corridor of the above kind has $b-2$ (resp.~$b$) {\em bends}.
%A corridor partition partitions the knapsack into $O_{\eps, \epsl}(1)$ number of corridors with $O_{\eps}(1)$ bends.

\begin{lem}[Corridor Packing Lemma \cite{adamaszek2015knapsack}]\label{lem:corridorPack}
There exists a corridor partition \footnote{In \cite{adamaszek2015knapsack},  $\opt$ was optimal \tgk~packing. However, it also works when $\opt$ is optimal \tggk~packing.} and $\optco \subseteq \optsk$ such that:
\begin{enumerate}\itemsep0pt
\item there is a subset $\optco^{cross} \subseteq \optco$ with  $|\optco^{cross}| \le O_\eps(1)$ such that  each $i\in \optco \setminus \optco^{cross}$ is fully contained in some corridor,
\item $\profit(\optco) \ge (1-O(\eps))\profit(\optsk)$,
\item the number of corridors is $O_{\eps,\epsl}(1)$ and each corridor has width at most $\epsl N$ and has at most $1/\eps$ bends.
\end{enumerate}
\end{lem}
%\arir{can we remove  $|\optco^{cross}|$ }

\noindent A {\em subcorridor} $S_i$ of an open (resp.~closed) corridor is the maximally large rectangle contained in the corridor, containing edges $e_i,e_{2b-i}$ (resp.~$e_i,e_{i'}$) on its boundary. 
An open (resp.~closed) corridor is the union of $b-1$ (resp.~$b$) such rectangular regions.
%The length of $S_i$ is the \emph{length} of the shortest such edge. 
%\arir{do we use long and short subcorridor in our paper? where?}
%We say that a subcorridor is \emph{long} if its length is more than $N/2$, and \emph{short} otherwise.  
%We call a subcorridor \emph{horizontal} (resp., \emph{vertical}) if 
%its width (resp. height) is more than its height (resp. width).
%Note that each rectangle in $\optco$ is distinctly associated with the only subcorridor that fully contains it.  Let  $S_1,\ldots,S_{k'}$ be a sequence of consecutive subcorridors of an open (or closed) corridor. 
%Consider two consecutive corridors $S_i$ and $S_{j}$ with $j=i+1$ in the case of an open corridor and $j=(i+1)$(mod $k'$) otherwise.
Region $S_{i,j}$ is the shared rectangular region between two consecutive subcorridors $S_i$ and $S_j$. 
{\em Unshared region} of $S_i$ is the region not shared with any other subcorridors.
%There is a natural subdivision of each corridor into regions that 
 The boundary between the regions containing  only vertical or only horizontal items  in two consecutive subcorridors $S_i$ and $S_j$, is a  monotone axis-parallel curve in $S_{i,j}$, which we call {boundary curve} (see Figure \ref{fig:lproc}).
%\arir{defined boundary curve}
%
We define $S_{j}$ to be the right (resp.~left, top, bottom) of $S_i$ if there exists a point in $S_i$ to the left (resp.~right, bottom, top) of every point in $S_{j}\setminus S_{i,j}$.
A pair $(S_i,S_{j})$ forms a {\em clockwise}  bend if $S_i$ is horizontal and $S_{j}$ is to either bottom-right or top-left of $S_i$, and the complementary cases if $S_i$ is vertical. Otherwise, they form a counter-clockwise bend. 
A corridor with no bends (resp.~one bend), is called a $Box$($\Bc$)-corridor (resp.~$\Lc$-corridor). 
%A corridor with only one bend, is called an $\Lc$-corridor. 
An open corridor whose bends are all clockwise (resp.~counter-clockwise) is a \emph{spiral}. 
Spirals with $2,3$ bends  are called $\Uc, \Gc$-corridors, respectively. A closed corridor with $b=4$ is a \emph{ring}. %Note that in a ring all bends are either clockwise or counter-clockwise, thus intuitively it is the closed analogue of a spiral.
We call a triple $(S_{i},S_{i'},S_{i''})$ of consecutive subcorridors to be a $\Zc$-bend if $S_{i},S_{i'}$ form clockwise (resp.~counterclockwise) bend and $S_{i'},S_{i''}$ form counterclockwise (resp.~clockwise) bend, and the subcorridors $S_{i},S_{i'},S_{i''}$ are called $\Zc$-subcorridors.
We call $S_{i'}$ to be the \emph{center-sc} of the bend, and $S_{i},S_{i''}$ its \emph{side-sc}.  
A spiral corridor can not have $\Zc$ bends.
A subcorridor that is not a $\Zc$-subcorridor is called a {\em spiral subcorridor}.
A $\Zc$-corridor is a corridor formed by union of 3 $\Zc$-subcorridors. 	
In \cite{adamaszek2015knapsack, GalvezGHI0W17} the subcorridors are processed (see Section \ref{prosec} for proof of Lemma \ref{lem:subcpr}) so that by rearranging and removing some items, the rest can be packed into constant number of boxes. However, these rearrangements may violate guillotine separability. 

\begin{lem}[\cite{GalvezGHI0W17}]
\label{lem:subcpr}
For appropriate constant $\epsb, \eps>0$, given a spiral  subcorridor $S$, we can remove two sets of rectangles {\em kill} and {\em thin} and rearrange the remaining rectangles (we call them {\em fat}) such that all fat rectangles are completely packed into $O_{\epsb}(1)$ boxes, $|kill|=O_{\eps, \epsl, \epsb}(1)$ and the total area of thin rectangles $\le \epsb N^2$.
\end{lem}
%\arir{check if it is better to mention the width of thin etc. shift this proof to appendix.}

\begin{definition}[Container]
Containers are axis-aligned rectangular regions labeled as {\em large, horizontal, vertical,} or {\em area}. In a {\em container packing}, all items are packed inside containers:
(a) next to each other if items are vertical (vertical container), (b) above each other if  items are horizontal (horizontal container), (c) single item if the item is large (large container), (d) each item packed in a container of size $a \times b$ must have $w_i \le \eps a, h_i \le \eps b$ (area container).
\end{definition}

\begin{definition}
\label{orien}
If all  {\em skewed} items completely contained in a subcorridor (or container) $S_{1}$ are horizontal (resp.~vertical) then $S_1$ (or its orientation) is called horizontal (resp.~vertical).
\end{definition} 

\begin{definition}[Boundary corridors]
A {\em boundary-$\Lc$} of height $N_1$ and width $N_2$ in a  $[l,r] \times [b, t]$ box,  is the region $\big(([l,r]\times[b,b+N_1]) \cup ([l,l+N_2] \times[b, t])\big)$. Similarly, a {\em boundary-$\Uc$} (resp.~{\em boundary-$\Gc$}) occupies the region 
$\big(([l,r]\times[b,b+N_1]) \cup ([l,l+N_2] \times[t, b]) \cup ([r-N_3,r] \times[b, t]) \big)$  (resp.~
$\big(([l,r]\times[b,b+N_1]) \cup ([l,l+N_2] \times[t, b]) \cup ([r-N_3,r] \times[b, t]) \cup ([l,r]\times[t-N_4,t]) \big)$).  Ring, {\em boundary-$\Lc$, boundary-$\Uc$, boundary-$\Gc$} are termed as {\em boundary} corridors.
\end{definition}
%\arir{merged all boundary corridors to save space.}

%\arir{added bounding box definition here.}
The number of bends in a corridor $C$ is denoted by $b(C)$.  
A box $\mathcal{B}$ is said to be a {\em bounding box } of $C$ or {\em bounding} $C$, if  $b(C)\ge1$ and the outermost corners at the bends of the corridor coincides with the corners of the box. Also, $\mathcal{B}$ should be guillotine separable when considered as a pseudoitem. 
Note that a corridor $C'$ inside $\mathcal{B}$ may not be a boundary corridor of $\mathcal{B}$. 

In $\lpack$, the goal is to pack maximum profit subset of long items into  a {\em boundary-$\Lc$}.
%$\lpack$ will play a crucial role in our paper. 

\begin{lem}
\label{lem:lpack} \cite{GalvezGHI0W17}
There is a PTAS for the $\lpack$ problem.
\end{lem}

\begin{definition}[$L\&C$ Packing]
In $L\&C$ packing, we have a  boundary-$\Lc$ with width $N_1$ and height $N_2$ in $[0, N] \times [0, N]$-box and $O_{\eps,\epsl}(1)$  number of non-overlapping containers contained in the space not occupied by the  boundary-$\Lc$. Only {\em long} rectangles are packed  in the boundary-$\Lc$.
%, and only {\em short} items are packed in the containers. 
In this paper, we have an additional constraint that the containers (and the items therein) in  $L\&C$ packing are guillotine separable.
\end{definition}

%\arir{changed definition of  $L\&C$ PACKING. check if this is fine.}

\subsection{One Sided Resource Augmentation}
In resource augmentation we  allow slightly larger sized knapsack. 
%This  has been a useful technique for geometric packing. 
The resource augmentation algorithm of \cite{GalvezGHI0W17} can easily be adapted to satisfy the property of guillotine separability.
\begin{lem}\cite{GalvezGHI0W17}
	\label{lemma1}
	Let $\R'$ be packed in a box of size $a\times b$, and $\epsau>0$. Then there exists a container packing of $\R''\subseteq \R'$ inside a box of size $a\times(1+\epsau)b$ (resp.~$(1+\epsau)a\times b$) with:
	\begin{enumerate}
	\item $\profit(\R'')\geq (1-O(\epsau))\profit(\R')$,
	\item The number of containers is $O_{\epsau}(1)$ and their sizes belong to a set of cardinality $n^{O_{\epsau}(1)}$,
	\item The total area of the containers is at most $\area(\R')+\epsau ab$; 
         \item If the initial packing of $\R'$ in the $a\times b$ box is guillotine separable then the container packing of $\R''$ inside the $a\times(1+\epsau)b$ box (resp.~$(1+\epsau)a\times b$) remains guillotine separable.
	\end{enumerate}
	\end{lem}		
%\begin{proof}
%We give the proof of Lemma \ref{lemma1} in the Section \ref{resource_aug} of Appendix.
%\end{proof}		


==> 3_L_Packing.tex <==
\section{Guillotine $\lpack$}
\label{glp}
G{\'a}lvez et al.~\cite{GalvezGHI0W17}  showed that one could pack $\frac34 \optln$ profit using $\lpack$.
Now  we show an $\lpack$ of {\em all} long rectangles in $\opt$. Using simple induction, we can prove that every $\lpack$ arrangement is guillotine separable.
 %For the proof we use some basic rearrangements maintaining  the guillotine separability of packing: 
	%\item {\em Compression:} Consider a piece with only wide (resp. tall) items. Compression piles  the wide (resp. tall) items on top (resp. side) of each other, staring from the bottom (resp. left) boundary such that they share a common vertical right (resp. horizontal top) boundary.
	%\item {\em Sorting:} Given a set of compressed items, sorting reorders the items such that the wide (resp. tall) items are packed according to a nonincreasing width (resp. height) from bottom to top (resp. left to right) with every item touching the same vertical right (resp. horizontal top) boundary.
We define a rearrangement operation {\em mirroring} that preserves guillotine separability. 
Given a piece $P:= [l_i, r_i]\times [b_i, t_i]$ with embedded rectangles, mirroring of $P$ creates a packing  that is a mirror image. $Mirror(P, y)$ (resp. $Mirror(P,x)$)  is mirroring of $P$  w.r.t. $y$-axis (resp. $x$-axis) that maps rectangle $R(i):=(\leftc_i, \rightc_i) \times (\bottomc_i, \topc_i)$ to the position $(l_i+r_i-\rightc_i, l_i+r_i-\leftc_i)\times (\bottomc_i, \topc_i)$ (resp. $(\leftc_i, \rightc_i) \times (b_i+t_i-\topc_i, b_i+t_i-\bottomc_i)$).

	
\begin{lem}\label{lpackinglem}
There exists an $\lpack$ of rectangles in $\optln$ into an $\Lp$-region:   ([0,N] $\times$ [0,$\height_{wide}$]) $\cup$ ([0,$\width_{tall}$] $\times$ [0,N]), where $\height_{wide}$ is the total height of all wide items in $\optln$ and $\width_{tall}$ is the total width of all tall items in $\optln$.
\end{lem}	
\begin{proof} 
We will prove it by induction on the number of items. The base case is trivial. 
For the induction step, consider the guillotine cut sequence of  $\optln$. 
W.l.o.g.~assume the first cut is a horizontal cut $y=h_1$ that divides the $N\times N$ knapsack piece $P$  into two subpieces $P_1:=[0,N]\times[0,h_1]$ and $P_2:=[0,N]\times[h_1, N]$. 
W.l.o.g. let us assume that both $P_1$ and $P_2$ contains long rectangles (otherwise, we can take the first guillotine cut that separates two long rectangles).
Then, either $h_1 \le N/2$ or $(N-h_1)\le N/2$. W.l.o.g. assume the latter case. We will discuss the rearrangement steps for this case. The other cases are symmetric. 

Let $\height_{wide}(P_1)$ (resp. $\height_{wide}(P_2)$ ) and $\width_{tall}(P_1)$ (resp. $\width_{tall}(P_2)$) be the total height of tall rectangles in $P_1$ (resp. $P_2$) and the total width of wide rectangles in $P_1$ (resp. $P_2$).
Now, using induction on $P_1$, we obtain a packing of all long rectangles in $P_1$ in a region 
$L_1:= ([0,N] \times [0, \height_{wide}(P_1)]) \cup  ([0,\width_{tall}(P_1)] \times [0,h_1])$.
Note that $P_2$ can not have tall rectangles, and can only consist wide rectangles. So, $\width_{tall}(P_2)=0$. Thus using induction on $P_2$, we obtain a packing in a region 
$L_2:=([0,N] \times [h_1, h_1+\height_{wide}(P_2)])$. 
Now use $Mirror(P_2, x)$ to shift the long rectangles in $P_2$ to the region $([0,N] \times [N -\height_{wide}(P_2),N])$.
Clearly, $y=N -\height_{wide}(P_2)$ does not intersect any items. 
Now define $P_1':=[0,N]\times[0, N -\height_{wide}(P_2)]$ and use $Mirror(P_1',x)$.
This gives a packing of $\optln$ in $\big([0, N]\times [0,N]\big) \setminus \big([\width_{tall}(P_1),N]$$\times$$[0, $$N-\height_{wide}(P_1)-\height_{wide}(P_2)]\big)$.
Finally, the desired $\lpack$ is obtained using $Mirror(P,x)$ (see Figure \ref{fig:lstages} for the procedure). 
\end{proof}
	


	%\begin{figure}[!htb]
	%\centering
	%\includegraphics[scale=.75]{lpack}
	%\caption{An illustration of $\lpack$. Here we are doing compression after every stage. Flipping the red and yellow pieces to bring smaller %piece to the horizontal leg of $\Lp$}
	%\label{$\lpack$}
	%\end{figure}
	
	
	%%%%%%%%%%%%%%%%%%%
	%%%.   Deletion of figure starts
	%%%%%%%%%%%%%%%%%%%
%	\begin{comment}
%	
%	\begin{figure}[!tbh]
%		%\centering
%		\captionsetup[subfigure]{justification=centering}
%		\hspace{-10pt}
%		\begin{subfigure}[t]{.25\textwidth}
%			\centering
%			\resizebox{!}{3.5cm}{
%			\begin{tikzpicture}\node[rotate = 90, yscale  =-1] at (0,0){\begin{tikzpicture}
%				%box			
%				\draw[thick] (0,0) rectangle (70,70);
%				% items
%				\draw[solid, fill = lightgray] (2.4,4.2) rectangle (5.5,55.7);
%				\draw[solid, fill = lightgray] (7.4,15) rectangle (8.2,61.7);
%				\draw[solid, fill = lightgray] (12.4,5) rectangle (14.5,24.5);
%				\draw[solid, fill = lightgray] (18.3,15.8) rectangle (26.6,44.1);
%				\draw[solid, fill = lightgray] (28.3, .2) rectangle (28.31,70);
%				\draw[dashed] (28.3,0) -- ( 28.3, 70);
%				\draw[solid, fill = lightgray] (31.6,2.7) rectangle (33.3,40.2);
%				\draw[solid, fill = lightgray] (35.8,6.9) rectangle (37.88,24.4);
%				\draw[solid, fill = lightgray] (40.8,5.2) rectangle (69.2,6.9);
%				\draw[solid, fill = lightgray] (39.9,14.4) rectangle (66.6,16.9);
%				\draw[solid, fill = lightgray] (58.5,18.7) rectangle (61.4,32.7);
%				\draw[solid, fill = lightgray] (39.5,35.8) rectangle (68.7,38.3);
%				\draw[solid, fill = lightgray] (31.6,44.4) rectangle (69.1,46.9);
%				\draw[solid, fill = lightgray] (38,49.4) rectangle (66.3,51.1);
%				\draw[solid, fill = lightgray] (28.4,53.5) rectangle (55.9,58.1);
%				\draw[solid, fill = lightgray] (33.3,60.2) rectangle (50,61.9);
%	
%				%\draw (50, 72) node {\large \textbf{$1$}};
%			\end{tikzpicture}};\end{tikzpicture}}
%		\caption{Horizontal cut separating horizontal only items on bottom sub-piece.}
%		\label{fig a}
%		\end{subfigure}
%		\begin{subfigure}[t]{.25\textwidth}
%			\centering
%			\resizebox{!}{3.5cm}{
%			\begin{tikzpicture}\node[rotate = 90, yscale  =-1] at (0,0){\begin{tikzpicture}
%				%box			
%				\draw[thick] (0,0) rectangle (70,70);
%				% items
%				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
%				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
%				\draw[solid, fill = lightgray] (4.1,50) rectangle (6.6,70);
%				\draw[solid, fill = lightgray] (6.6,41.7) rectangle (14.9,70);
%				\draw[dotted] (15,0) -- (15,70);
%				%first guillotine cut
%				\draw[solid, fill = lightgray] (31.6,2.7) rectangle (33.3,40.2);
%				\draw[solid, fill = lightgray] (35.8,6.9) rectangle (37.88,24.4);
%				\draw[solid, fill = lightgray] (40.8,5.2) rectangle (69.2,6.9);
%				\draw[solid, fill = lightgray] (39.9,14.4) rectangle (66.6,16.9);
%				\draw[solid, fill = lightgray] (58.5,18.7) rectangle (61.4,32.7);
%				\draw[solid, fill = lightgray] (39.5,35.8) rectangle (68.7,38.3);
%				\draw[dotted] (15, 42) -- ( 70, 42);
%				\draw[solid, fill = lightgray] (31.6,44.4) rectangle (69.1,46.9);
%				\draw[solid, fill = lightgray] (38,49.4) rectangle (66.3,51.1);
%				\draw[solid, fill = lightgray] (28.4,53.5) rectangle (55.9,58.1);
%				\draw[solid, fill = lightgray] (33.3,60.2) rectangle (50,61.9);
%			\end{tikzpicture}};\end{tikzpicture}}
%			\caption{Compression of items on bottom subpiece}
%			\label{fig b}
%		\end{subfigure}
%		\begin{subfigure}[t]{.25\textwidth}
%			\centering
%			\resizebox{!}{3.5cm}{
%			\begin{tikzpicture}\node[rotate = 90, yscale = -1] at (0,0){\begin{tikzpicture}
%				%box			
%				\draw[thick] (0,0) rectangle (70,70);
%				% items
%				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
%				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
%				\draw[solid, fill = lightgray] (4.1,41.7) rectangle (12.4,70);
%				\draw[solid, fill = lightgray] (12.4,50) rectangle (14.9,70);
%				\draw[solid, fill = lightgray] (14.9,0) rectangle (15,70);
%				%first guillotine cut
%				\draw[solid, fill = lightgray] (31.6,2.7) rectangle (33.3,40.2);
%				\draw[solid, fill = lightgray] (35.8,6.9) rectangle (37.88,24.4);
%				\draw[solid, fill = lightgray] (40.8,5.2) rectangle (69.2,6.9);
%				\draw[solid, fill = lightgray] (39.9,14.4) rectangle (66.6,16.9);
%				\draw[solid, fill = lightgray] (58.5,18.7) rectangle (61.4,32.7);
%				\draw[solid, fill = lightgray] (39.5,35.8) rectangle (68.7,38.3);
%				% second cut
%				\draw[solid, fill = lightgray] (22.5,67.5) rectangle (70,70);
%				\draw[solid, fill = lightgray] (41.7,65.8) rectangle (70,67.5);
%				\draw[solid, fill = lightgray] (42.5,61.4) rectangle (70,65.8);
%				\draw[solid, fill = lightgray] (43.3,59.5) rectangle (70,61.4);
%				\draw[solid, fill = lightgray] (15,59.4) rectangle (70,59.5);
%			\end{tikzpicture}};\end{tikzpicture}}
%			\caption{Vertical cut compressing and sorting rectangles in left subpiece}
%			\label{fig c}
%		\end{subfigure}
%		\begin{subfigure}[t]{.25\textwidth}
%			\centering
%			\resizebox{!}{3.5cm}{
%			\begin{tikzpicture}\node[rotate = 90, yscale  =-1] at (0,0){\begin{tikzpicture}
%				%box			
%				\draw[thick] (0,0) rectangle (70,70);
%				% items
%				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
%				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
%				\draw[solid, fill = lightgray] (4.1,41.7) rectangle (12.4,70);
%				\draw[solid, fill = lightgray] (12.4,50) rectangle (14.9,70);
%				\draw[solid, fill = lightgray] (14.9,0) rectangle (15,70);
%				%first guillotine cut
%				\draw[solid, fill = lightgray] (31.6,13.3) rectangle (33.3,50.8);
%				\draw[solid, fill = lightgray] (35.8,17.5) rectangle (37.88,35);
%				
%				\draw[dashed] (39,10.6) -- (39,70);
%				\draw[solid, fill = lightgray] (40.8,15.8) rectangle (69.2,17.5);
%				\draw[solid, fill = lightgray] (39.9,25) rectangle (66.6,27.5);
%				\draw[solid, fill = lightgray] (58.5,29.3) rectangle (61.4,43.3);
%				\draw[solid, fill = lightgray] (39.5,46.4) rectangle (68.7,48.9);
%				% second cut
%				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
%				\draw[solid, fill = lightgray] (41.7,2.5) rectangle (70,4.2);
%				\draw[solid, fill = lightgray] (42.5,4.2) rectangle (70,8.8);
%				\draw[solid, fill = lightgray] (43.3,8.8) rectangle (70,10.5);
%				\draw[solid, fill = lightgray] (15,10.5) rectangle ( 70, 10.6);
%			\end{tikzpicture}};\end{tikzpicture}}
%			\caption{Flipping to form vertical leg of L, followed by compression and sorting to form Horizontal leg of L-structure}
%			\label{fig d}
%		\end{subfigure} 
%		%\hspace{-20pt}
%		\begin{subfigure}[t]{.25\textwidth}
%			\centering
%			\resizebox{!}{3.5cm}{
%			\begin{tikzpicture}\node[rotate = 90 ,yscale = -1] at (0,0){\begin{tikzpicture}
%				%box			
%				\draw[thick] (0,0) rectangle (70,70);
%				% items
%				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
%				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
%				\draw[solid, fill = lightgray] (4.1,32.5) rectangle (5.8,70);
%				\draw[solid, fill = lightgray] (5.8,41.7) rectangle (14.1,70);
%				\draw[solid, fill = lightgray] (14.1,50) rectangle (16.6,70);
%				\draw[solid, fill = lightgray] (16.6,52.5) rectangle (19.4,70);
%				\draw[dotted] (19.5,0) -- (19.5,70);
%				
%				%first guillotine cut
%				
%				
%				%third cut
%				
%				\draw[solid, fill = lightgray] (40.8,15.8) rectangle (69.2,17.5);
%				\draw[solid, fill = lightgray] (39.9,25) rectangle (66.6,27.5);
%				\draw[dashed] (19.5, 28) -- ( 70, 28);
%				\draw[solid, fill = lightgray] (58.5,29.3) rectangle (61.4,43.3);
%				\draw[solid, fill = lightgray] (39.5,46.4) rectangle (68.7,48.9);
%				% second cut
%				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
%				\draw[solid, fill = lightgray] (41.7,2.5) rectangle (70,4.2);
%				\draw[solid, fill = lightgray] (42.5,4.2) rectangle (70,8.8);
%				\draw[solid, fill = lightgray] (43.3,8.8) rectangle (70,10.5);
%				\draw[solid, fill = lightgray] (19.5,10.5) rectangle ( 70, 10.6);
%			\end{tikzpicture}};\end{tikzpicture}}
%			\caption{Compression of items obtained by horizontal cut and sorting all items of horizontal leg of L-structure}
%		\end{subfigure}	
%		\begin{subfigure}[t]{.25\textwidth}
%			\centering
%			\resizebox{!}{3.5cm}{
%			\begin{tikzpicture}\node[rotate = 90, yscale = -1] at (0,0){\begin{tikzpicture}
%				%box
%				
%				\draw[thick] (0,0) rectangle (70,70);
%				% items
%				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
%				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
%				\draw[solid, fill = lightgray] (4.1,32.5) rectangle (5.8,70);
%				\draw[solid, fill = lightgray] (5.8,41.7) rectangle (14.1,70);
%				\draw[solid, fill = lightgray] (14.1,50) rectangle (16.6,70);
%				\draw[solid, fill = lightgray] (16.6,52.5) rectangle (19.4,70);
%				\draw[dotted] (19.5,0) -- (19.5,70);
%				
%				%first guillotine cut
%				
%				
%				%third cut
%				\draw[solid, fill = lightgray] (58.5,29.3) rectangle (61.4,43.3);
%				\draw[dotted] (19.5,45) -- (70,45);
%				\draw[solid, fill = lightgray] (39.5,46.4) rectangle (68.7,48.9);
%				% second cut
%				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
%				\draw[solid, fill = lightgray] (40.8,2.5) rectangle (70,4.2);
%				\draw[solid, fill = lightgray] (41.7,4.2) rectangle (70,5.9);
%				\draw[solid, fill = lightgray] (42.5,5.9) rectangle (70,10.5);
%				\draw[solid, fill = lightgray] (43.3,10.5) rectangle (70,12.2);
%				\draw[solid, fill = lightgray] (43.3,12.2) rectangle (70,14.7);
%				\draw[dotted] (19.5,14.7) -- ( 70, 14.7);
%			\end{tikzpicture}};\end{tikzpicture}}
%			\caption{Compression of items obtained by vertical cut followed by sorting all items of vertical leg of L-structure}
%			\label{fig f}
%		\end{subfigure}
%		%\hspace{5cm}
%		\begin{subfigure}[t]{.25\textwidth}
%			\centering
%			\resizebox{!}{3.5cm}{
%			\begin{tikzpicture}\node[rotate = 90, yscale = -1] at (0,0){\begin{tikzpicture}
%				%box
%				
%				\draw[thick] (0,0) rectangle (70,70);
%				% items
%				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
%				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
%				\draw[solid, fill = lightgray] (4.1,32.5) rectangle (5.8,70);
%				\draw[solid, fill = lightgray] (5.8,41.7) rectangle (14.1,70);
%				\draw[solid, fill = lightgray] (14.1,50) rectangle (16.6,70);
%				\draw[solid, fill = lightgray] (16.6,52.5) rectangle (19.4,70);
%				\draw[dotted] (19.5,0) -- (19.5,70);
%				
%				%first guillotine cut
%				
%				
%				%third cut
%				\draw[solid, fill = lightgray] (58.5,29.3) rectangle (61.4,43.3);
%				\draw[dotted] (19.5,45) -- (70,45);
%				
%				% second cut
%				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
%				\draw[solid, fill = lightgray] (40.8,2.5) rectangle (70,5);
%				\draw[solid, fill = lightgray] (40.8,5) rectangle (70,6.7);
%				\draw[solid, fill = lightgray] (41.7,6.7) rectangle (70,8.4);
%				\draw[solid, fill = lightgray] (42.5,8.4) rectangle (70,12.7);
%				\draw[solid, fill = lightgray] (43.3,12.7) rectangle (70,14.7);
%				\draw[solid, fill = lightgray] (43.3,14.7) rectangle (70,17.2);
%				\draw[dotted] (19.5,17.2) -- ( 70, 17.2);
%			\end{tikzpicture}};\end{tikzpicture}}
%			\caption{Compression of items obtained by vertical cut followed by sorting all items of vertical leg of L-structure}
%			\label{fig g}
%		\end{subfigure}
%		\begin{subfigure}[t]{.23\textwidth}
%			\centering
%			\resizebox{!}{3.5cm}{
%			\begin{tikzpicture}\node[rotate = 90, yscale = -1] at (0,0){\begin{tikzpicture}
%				%box
%				
%				\draw[thick] (0,0) rectangle (70,70);
%				% items
%				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
%				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
%				\draw[solid, fill = lightgray] (4.1,32.5) rectangle (5.8,70);
%				\draw[solid, fill = lightgray] (5.8,41.7) rectangle (14.1,70);
%				\draw[solid, fill = lightgray] (14.1,50) rectangle (16.6,70);
%				\draw[solid, fill = lightgray] (16.6,52.5) rectangle (19.4,70);
%				\draw[solid, fill = lightgray] (19.4,56) rectangle (22.3,70);
%				\draw[dotted] (22.3,0) -- (22.3,70);
%				
%				%first guillotine cut
%				
%				
%				%third cut
%				
%				
%				% second cut
%				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
%				\draw[solid, fill = lightgray] (40.8,2.5) rectangle (70,5);
%				\draw[solid, fill = lightgray] (40.8,5) rectangle (70,6.7);
%				\draw[solid, fill = lightgray] (41.7,6.7) rectangle (70,8.4);
%				\draw[solid, fill = lightgray] (42.5,8.4) rectangle (70,12.7);
%				\draw[solid, fill = lightgray] (43.3,12.7) rectangle (70,14.7);
%				\draw[solid, fill = lightgray] (43.3,14.7) rectangle (70,17.2);
%				\draw[dotted] (22.3,17.2) -- ( 70, 17.2);
%			\end{tikzpicture}};\end{tikzpicture}}
%			\caption{Compression of item obtained by horizontal cut followed by sorting all items of horizontal leg of L-structure}
%			\label{fig h}
%		\end{subfigure}
%		\caption{Step wise construction of L from guillotine separable optimal packing. }
%%(a) Compression of item obtained by horizontal cut followed by sorting all items of horizontal leg of L-structure. (b)Compression of items obtained by vertical cut followed by sorting all items of vertical leg of L-structure. (c) Compression of items obtained by vertical cut followed by sorting all items of vertical leg of L-structure. (d) Compression of items obtained by horizontal cut and sorting all items of horizontal leg of L-structure. (e) Flipping to form vertical leg of L, followed by compression and sorting to form Horizontal leg of L-structure. (f) Vertical cut compressing and sorting rectangles in left subpiece. (g) Compression of items on bottom subpiece. (h) Horizontal cut separating horizontal only items on bottom sub-piece.}
%		\label{$\lpack$}
%	\end{figure}
%	
%\end{comment}	
%%%%%%%%%%%%
%%%%%%Deletion of figure ends
%%%%%%%%%%%%	
	
	\begin{lem}
	\label{lem:PTASL}
	In polynomial time, we can find an $\lpack$ with profit $(1-O(\eps))\profit(\optln)$.	\end{lem}
\begin{proof}
Follows from Lemma \ref{lpackinglem} and PTAS for $\lpack$ (Lemma \ref{lem:lpack}) on $\R_{long}$.
\end{proof}

\begin{figure}[!tbh]
		\captionsetup[subfigure]{justification=centering}
		\hspace{20pt}
		\begin{subfigure}[t]{.21\textwidth}
			\centering
			\resizebox{!}{2.4 cm}{
			\begin{tikzpicture}
				\draw[thick] (0,0) rectangle (6.0,6.0);
				\draw[dashed] (0,4.5) -- ( 6, 4.5);	

				%p2
				\draw[solid, fill = lightgray] (.4,5.1) rectangle (4.3,5.3);
				\draw[solid, fill = lightgray] (.5,5.5) rectangle (5.9,5.8);
				\draw[solid, fill = lightgray] (.2,4.6) rectangle (5.3,4.9);

				%p1
				\draw[solid, fill = lightgray] (.2,.6) rectangle (.9,4.1);
				\draw[solid, fill = lightgray] (1.3,.3) rectangle (1.6,3.7);
				\draw[solid, fill = lightgray] (5.2,.1) rectangle (5.6,4.4);

				\draw[solid, fill = lightgray] (1.8,2.6) rectangle (4.9,3.1);
				\draw[solid, fill = lightgray] (1.7,3.6) rectangle (4.7,3.9);
				\draw[solid, fill = lightgray] (1.65,.55) rectangle (5.1,1.1);
			\node[below,scale=2] at (2,0) {(a)};
			\end{tikzpicture}}
		%\caption{}
		%\label{fig a}
		\end{subfigure}
		\begin{subfigure}[t]{.21\textwidth}
			\centering
			\resizebox{!}{2.4cm}{
			\begin{tikzpicture}

				\draw[thick](0,0) rectangle (6,6);
				\draw[dashed] (0,4.5) -- ( 6, 4.5);	

				%p2
				\draw[solid, fill = lightgray] (2.1,5.1) rectangle (6,5.3);
				\draw[solid, fill = lightgray] (.6,4.5) rectangle (6,4.8);
				\draw[solid, fill = lightgray] (0.9,4.8) rectangle (6,5.1);

				%p1
				\draw[solid, fill = lightgray] (0.9,1) rectangle (1.6,4.5);
				\draw[solid, fill = lightgray] (.4,1.1) rectangle (.9,4.5);
				\draw[solid, fill = lightgray] (0,.2) rectangle (.4,4.5);

				\draw[solid, fill = lightgray] (2.55,0) rectangle (6,.55);
				\draw[solid, fill = lightgray] (2.9,0.55) rectangle (6,1.05);
				\draw[solid, fill = lightgray] (3,1.05) rectangle (6,1.35);
			\node[below,scale=2] at (2,0) {(b)};
			\end{tikzpicture}}
			%\caption{}
			%\label{fig b}
		\end{subfigure}
		\begin{subfigure}[t]{.21\textwidth}
			\centering
			\resizebox{!}{2.4cm}{
			\begin{tikzpicture}
				\draw[thick](0,0) rectangle (6,6);

				\draw[solid, color = red] (0,0) rectangle (6,5.2);	

				%p2
				\draw[solid, fill = lightgray] (2.1,5.2) rectangle (6,5.4);
				\draw[solid, fill = lightgray] (.6,5.7) rectangle (6,6);
				\draw[solid, fill = lightgray] (0.9,5.4) rectangle (6,5.7);

				%p1
				\draw[solid, fill = lightgray] (0.9,1) rectangle (1.6,4.5);
				\draw[solid, fill = lightgray] (.4,1.1) rectangle (.9,4.5);
				\draw[solid, fill = lightgray] (0,.2) rectangle (.4,4.5);

				\draw[solid, fill = lightgray] (2.55,0) rectangle (6,.55);
				\draw[solid, fill = lightgray] (2.9,0.55) rectangle (6,1.05);
				\draw[solid, fill = lightgray] (3,1.05) rectangle (6,1.35);
				\node[below,scale=2] at (2,0) {(c)};	
				\end{tikzpicture}}
			%\caption{}
			%\label{fig c}
		\end{subfigure}
		\begin{subfigure}[t]{.21\textwidth}
			\centering
			\resizebox{!}{2.4cm}{
			\begin{tikzpicture}
				\draw[thick] (0,0) rectangle (6.0,6.0);
				\draw[solid, color = red] (0,0) rectangle (6,5.2);

				%p2
				\draw[solid, fill = lightgray] (2.1,5.2) rectangle (6,5.4);
				\draw[solid, fill = lightgray] (.6,5.7) rectangle (6,6);
				\draw[solid, fill = lightgray] (0.9,5.4) rectangle (6,5.7);

				%p1
				\draw[solid, fill = lightgray] (0.9,0) rectangle (1.6,3.5);
				\draw[solid, fill = lightgray] (.4,0) rectangle (.9,3.4);
				\draw[solid, fill = lightgray] (0,0) rectangle (.4,4.3);

				\draw[solid, fill = lightgray] (2.55,5.2) rectangle (6,4.65);
				\draw[solid, fill = lightgray] (2.9,4.65) rectangle (6,4.15);
				\draw[solid, fill = lightgray] (3,4.15) rectangle (6,3.85);
			\node[below,scale=2] at (2,0) {(d)};
			\end{tikzpicture}}
			%\caption{}
			%\label{fig d}
		\end{subfigure} 
	
		\caption{Stages of obtaining guillotine $\lpack$ (a)Horizontal Cut (b)Applying induction (c)$Mirror(P_2, x)$ (d)$Mirror(P_1', x)$. Final stage following (d) is $Mirror(P, x)$.}
		\label{fig:lstages}			
	\end{figure}

	

==> 4A_Structural_Property.tex <==
\subsection{Obtaining corridors of type B,L,U,G}
\label{subsec43}
\begin{lem}
\label{ringlem}
Every ring $R$ obtained after the previous corridor decomposition, can be converted into $O_{\eps,\epsl}(1)$ number of open corridors with at most 3 bends and possibly a box which is guillotine separable and the box contains a smaller ring. All items in this decomposition remain guillotine separable. 
\end{lem}
\begin{proof}
We call a function Algo-Box-Creation($R$) (see Algorithm \ref{boxalgo} and its explaination ). This function now takes the ring and bounds a certain portion of it with a box which is guillotine separable. The function also ensures that only $O_{\eps,\epsl}(1)$ additional spiral corridors with at most 3 bends are created during this entire process. 		
\end{proof}







		\begin{thm}
		\label{3max}
		Any  corridor $C$ can be converted into $O_{\eps,\epsl}(1)$ corridors of type $\Bc, \Lc, \Uc, \Gc$, maintaining guillotine separability.
		\end{thm}
		\begin{proof}W.l.o.g. assume $C$ has no $\Zc$-bends (else apply Lemma \ref{noz}) and more than 3 bends. There are 2 cases. 
		
\noindent {\em Case 1. } $C$ is an open corridor with more than 3 bends.  Call the function Algo-Spiral($C$)(see the Algorithm \ref{spialgo} and its explaination). The function Algo-Spiral($C$) takes corridor $C$ as input and converts it into $O_{\eps,\epsl}(1)$ spiral corridors with at most 3 bends. 
\\
\noindent {\em Case 2.} $C$ is a ring. Then consider the bounding box $\mathcal{B}$ (if any) which contains a smaller ring as shown in Lemma \ref{ringlem}. 
We now call the function Algo-Process($\mathcal{B},C$) (see Algorithm \ref{balgo} and its explaination). The function Algo-Process($\mathcal{B},C$) converts a portion of the ring $C$ into another ring $C'$ whose items can be separated out using the cuts of type $C_p$ and is bounded by the box $\mathcal{B}$.
We then call the function Algo-Boundary-L($\mathcal{B},C'$) (see the Algorithm \ref{Lalgo} and its explaination). The function Algo-Boundary-L($\mathcal{B},C'$) coverts the ring $C'$   into a the boundary-$\Lc$ (whose items can be separated out using the cuts of type $C_p$) by appropriately shifting the items of $C'$. 

The functions used in this subcase also have the property that only $O_{\eps,\epsl}(1)$ additional spiral corridors with at most 3 bends are created during this entire process. 	
\end{proof}

\subsection{Obtaining corridors with at most 2 bends}
\label{sub:bldec}
\begin{comment}
	\begin{lem} \label{structure}
	Given an optimal guillotine packing of  a set of skewed  rectangles $\R$, we can partition the knapsack into $O_{\eps,\epsl}(1)$  $\Lc$ and $\Bc$-corridors and place $\R' \subseteq \R$ rectangles in these corridors such that:
	\begin{enumerate}
	\item$\profit(\R') \geq (1-O(\eps))\profit(\R)$ and  $|\R \setminus \R'|=O_{\eps}(1)$.
	\item Each vertical (resp. horizontal) rectangle is completely contained in a  vertical (resp. horizontal) subcorridor. 
	\item Each rectangle is guillotine separable
	\item Each $\Lc$-corridor is a boundary-$\Lc$ for a rectangular box.
         \item $\Bc$-corridors  and rectangular boxes (which bound the items in $\Lc$ corridors ) when considered as a pseudo rectangle are guillotine separable.
     	\end{enumerate}
	\end{lem}
The remainder of the section is dedicated to the proof of Lemma \ref{structure}.
\end{comment}
\subsubsection{Creation of Bounding Boxes}\label{box_11}
Given an optimal guillotine packing of skewed rectangles $\R$, using lemma \ref{lem:corridorPack} and Theorem \ref{3max}, we partition the knapsack into $O_{\eps}(1)$ spiral corridors with at most three bends and obtain a guillotine  packing of $\R'$. By proper shifting argumentation as done in Subsection \ref{subsec:shifting}, we can ensure that $\profit(\R \setminus \R') \leq O(\eps)\profit(\R)$. We now  provide a construction of finding the rectangular box for each type of corridor with at least one bend such that the corridor is at the boundary of the box and the box is guillotine separable. For this we will be taking the help of Algo-Box-Creation(.) (see  Algorithm \ref{boxalgo}). Whenever we call Algo-Box-Creation(.) we consider only those guillotine cuts to find a bounding box which don't pass through the interior of the boxes which are created before we called Algo-Box-Creation(.). Let the set $S$ of corridors with  one or more bends which are not bounded by box be $\{ C_{1},...,C_{k'}\}$ where $k'$ is at most $O_{\eps,\epsl}(1)$. We now call the function Algo-Box-Creation($C_{1}$) to construct a bounding box for $C_1$. We then update the set $S$ if some other corridor also gets bounded by a box after the function Algo-Box-Creation($C_{1}$) completes its job. Run this function on the rest of the corridors in $S$ one by one. This process terminates as the size of $S$ decreases after each call to the function Algo-Box-Creation(.). The function Algo-Box-Creation(.) ensures that the entire process leads to the creation of  $O_{\eps,\epsl}(1)$ boxes and $O_{\eps,\epsl}(1)$ extra corridors in total.

\subsection{BL-arrangement}\label{ssss}

\subsubsection{Handling L,U,G corridors which are bounded by a box}\label{sssl}
Let a box $\mathcal{B}$ bound a corridor such that $b(C)>0$. We call the function Algo-Process($\mathcal{B},C$) (see the Algorithm \ref{balgo}). The function Algo-Process($\mathcal{B},C$) by appropriately shifting the items inside it creates a boundary corridor $C'$ (whose items can be separated out using the cuts of type $C_p$). We then call the function Algo-Boundary-L($\mathcal{B},C'$) (see the Algorithm \ref{Lalgo}). The function Algo-Boundary-L($\mathcal{B},C'$) by appropriately shifting the items of $C'$ coverts it to a boundary-$\Lc$ (whose items can be separated out using the cuts of type $C_p$). So now we have a box $\mathcal{B}$ such that it bounds a boundary-$\Lc$. So using the results of this subsubsection and subsubsection \ref{finalB} we satisfy the properties of Theorem \ref{thm:ldecom}.

%\begin{comment}
%	\subsubsection{$\Lc$ corridor}\label{L corridor}
%	%Consider a L corridor $S$ with vertical subcorridor placed top left with respect to the horizontal subcorridor.W.l.o.g let us assume that the corridor $S$ can't be divided into smaller corridors with cuts perpendicular to subcorridor. Let us denote the line along the rightmost edge of horizontal subcorridor by $\Lc$. Consider the 2 left most vertical guillotine cuts in the vertical subcorridor of $S$ during the actual guillotine cutting sequence. If leftmost cut is intercepted by a rectangle $R_{1}$ which is above $S$ and the other cut is not intercepted by any rectangle which isn't completely above $R_{1}$ then there should exist a guillotine either top or bottom of the rectangle $R_{1}$ which crosses the line $\Lc$. Suppose there is no such cut and w.l.o.g let us assume that rectangle $R_{2}$ above $R_{1}$ which intercepts the second leftmost cut has a guillotine cut above it which crosses $\Lc$. But this situation is not possible as the set of rectangles in L corridor, rectangles which intercept the guillotine cuts of $R_{1}$ and $R_{2}$ form a non-guillotine structure as there is no end to end cuts be it horizontal or vertical  which spans the entire length of the subcorridor of $S$. So W.l.o.g let us assume that the two left most guillotine are intercepted by a single rectangle or by a rectangle which next to each other and above $S$. Consider the rectangle with upper most interception among the two. Let it be $R_{3}$. Now there must exist a guillotine cut between $R_{3}$ and the top most edge $e_{1}$ of vertical subcorridor of $S$ which crosses the line $\Lc$ and the leftmost guillotine cut. Suppose not then all the rectangles intercepting the guillotine cuts between $R_{3}$ and $e_{1}$, $R_{3}$ and the set of rectangles in the L corridor form a non-guillotine structure  as there is no end to end cuts be it horizontal or vertical which spans the entire length of the subcorridor of $S$. Now consider the lower most such guillotine cut which crosses line $\Lc$.Let this be $l_{1}$. Then by similar analogy we must have a guillotine cut to the right of horizontal subcorridor of $S$ which crosses $l_{1}$ and is parallel to $\Lc$. Hence we have constructed a box which is guillotine separable and has $S$ as it's boundary L.\\
%
%Consider a $\Lc$ corridor $S$. W.l.o.g we can assume that vertical subcorridor $S_{1}$ of $S$ is placed to the top left w.r.t the horizontal subcorridor $S_{2}$. We consider the smallest subpiece $P$ containing $S$.
%% Three cases might exist. Case 1: If left boundary of vertical subcorridor of S coincides with the left boundary of P, we have found the left boundary of bounding box. We then consider the sequence  If bottom boundary of horizontal subcorridor of S coincides with the bottom boundary of P, we have found the bottom boundary of bounding box. %
%Next consider the first stage guillotine cuts in the $P$. W.l.o.g let the first stage cuts be vertical.
%Then we have the following cuts which can occur to a $\Lc$ corridor during the recursive procedure to bound the $\Lc$ corridor which we are going to describe later:
%\begin{itemize}
%\item Cut 1:Rightmost vertical Guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$
%\item Cut 2:Horizontal Guillotine cut passing through $S_{1}$ and not through the interior of $S_{12}$
%\item Cut 3: Horizontal Guillotine cut passing through $S_{2}$
%\item Cut 4:  Cut which doesn't pass through $\Lc$ corridor.
%\end{itemize}
%Now we describe the recursive procedure.According to our assumption we begin with Cut 1. If we have Cut 1 then make a $\Bc$-corridor out of the rectangles separated from $\Lc$ corridor in our subpiece and consider the right subpiece to be the new subpiece. Merge all the $\Bc$-corridors obtained due to Cut 1 provided that these cuts occured before the first cut 2.For the rest of cuts which are of type cut 1 make a corridor for rectangles separated by these cuts. If we have Cut 2 then make a $\Bc$-corridor out of the rectangles separated from $\Lc$ corridor in our subpiece and consider the bottom subpiece to be the new subpiece.
%We stop the recursive procedure if either $S_{1}$ has exhausted or we obtain cut 2. If we obtain a cut 2 then we clearly have a bounding box with the edges being cut 1,cut 2 and the top and the right edges of the smaller subpiece $P'$ we are in after the last step of the recursive procedure. In the whole procedure we obtain only $O(\frac{1}{\epsl})$ extra $\Bc$-corridors. 
%	\subsubsection{$\Uc$-corrdor}\label{twobends}
%	%Consider a corridor $S$ with 2 bends such that 2 vertical subcorridors $S_{1},S_{3}$ placed on the top of the horizontal subcorridor $S_{2}$.W.l.o.g let us assume that the corridor $S$ can't be divided into smaller corridors with cuts perpendicular to subcorridor.Consider the 2 left most vertical guillotine cuts in the leftmost vertical subcorridor $S_{1}$ of $S$ during the actual guillotine cutting sequence. W.l.o.g let us assume that the two left most are intercepted by a single rectangle or by a rectangle which next to each other and above $S$. Consider the rectangle with upper most interception among the two. Let it be $R_{3}$. We denote the line along the rightmost edge of rightmost vertical subcorridor $S_{3}$ by $\Lc$. Now there must exist a guillotine cut between $R_{3}$ and the top most edge $e_{1}$ of vertical subcorridor of $S$ which crosses the line $\Lc$ and the leftmost guillotine cut. Suppose not then all the rectangles intercepting the guillotine cuts between $R_{3}$ and $e_{1}$, $R_{3}$ and the set of rectangles in the corridor $S$ form a non-guillotine structure as there is no end to end cuts be it horizontal or vertical  which spans the entire length of the subcorridor of $S$. Now consider the lower most such guillotine cut which crosses line $\Lc$.Let this be $l_{1}$. There is no rectangle between $l_{1}$ and topmost edge of the rightmost vertical subcorridor such that it intercepts line $\Lc$ otherwise the set of rectangle below line $l_{1}$ form a non-guillotine structure. Hence we have a box which is guillotine separable such that the corridor is along the boundary of the box. Now consider the corridor with 2 bends. By appropriate shifting of vertical rectangles we can convert it into a L corridor without disturbing the guillotine property. Exact details are available in subsubsection \ref{sss2}.\\
%Let $S$ be a corridor with $2$ bends. Let the top left vertical, horizontal and top right vertical subcorridors of $S$ be $S_{1}$, $S_{2}$ and $S_{3}$ respectively as shown in Figure \ref{figtwobends}. Consider the smallest subpiece $P$ containing $S$. We define three types of end-to-end cuts possible in $P$ or in any of the subpieces formed by a sequence of cuts in $P$.The rightmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$ is termed as \textit{Type $1$}. The leftmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{3}$ is termed as \textit{Type $3$}. The topmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{2}$ is termed as \textit{Type $2$}. Figure \ref{figtwobends} shows all the three types of cuts defined. We then follow a recursive approach to define bounding box using the cuts in guillotine cutting sequence. Clearly obtaining all three type of cuts, i.e., type $1,2,3$ will result in a bounding box where the box is bounded by these cuts and upper boundary of subpiece $P'$ containing a subset of items of $S$. Subpiece $P'$ is that subpiece which contains smaller corridor with 2 bends after we obtain the last of the three type cut.  \\
%\\Basic idea follows dividing $S$ into  $O(\frac{1}{\epsl})$ corridors $\{L_{1},L_{2},...,L_{k}\}$ (with at most 1 bend) consisting of some items from $S_{1}$ ( w.l.og it can be $S_{3}$ but we assume for the remainder of the section that $S_{1}$ is the one contributing to $\Lc'$) and $S_{2}$,  $O(\frac{1}{\epsl})$ $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$ from a subset of items of $S_{3}$ and a corridor (with at most 2 bends) with the remaining set of items. Note that $C_{i+1}$ is left of $C_{i}$ and $C_{i+1}$ has height less than $C_{i}$. Similarly $L_{i+1}$ is place to the top right of $L_{i}$ and $L_{i+1}$ is smaller in size than $L_{i}$   \\
%\\We now formally define the algorithm for processing corridor $S$ with $2$ bends. From observation \ref{endtoend} we know that the first cut in any guillotine separable piece is end-to-end. In the remainder of the subsection by closing a corridor or $\Bc$-corridor we mean that no more items will be packed in that corridor or $\Bc$-corridor. And, by opening a corridor  or $\Bc$-corridor we mean that we are allowed to pack rectangles in this corridor or $\Bc$-corridor only. Initially corridor $L_{1}$ is open  and $\Bc$-corridor $C_{1}$ is open. Depending on the type of this cut we do the following processing :
%\begin{enumerate}
%\item Scenario $1$:Let's assume that corridor $L_{i}$ and $\Bc$-corridor $C_{j}$ is open right now. If we have a horizontal cut through $S_{1}$ or $S_{3}$ but not through $S_{2}$ then we pack the items of $S_{1}$ above the cut in one $\Bc$-corridor and pack the items of $S_{3}$ above the cut in another $\Bc$-corridor. Then we continue our recursive procedure for the smaller portion of our original corridor present in the subpiece below this cut. If the horizontal cut passes through $S_{1}$ then we close $L_{i}$ and open $L_{i+1}$. Similarly if the horizontal cut passes through $S_{3}$ then we close $C_{j}$ and open $C_{j+1}$.    Such kind of cuts can have $O(\frac{1}{\epsl})$ number of occurences as the larger dimension of any rectangle is at least $\epsl N$. So when the recursive procedure halts scenario 1 would be contributing at most $O(\frac{1}{\epsl})$ new $\Bc$-corridors. 
%\item Scenario $2$ : (Type $1$ cut) Add the items of $S_{1}$ which is left of cut 1 to the vertical subcorridor of $L'$. Consider the new-subpiece to be the subpiece which is right of cut 1. Run algorithm recursively on the new-subpiece.
%\item Scenario $3$ : (Type $2$ cut) Add the items of $S_{2}$ below the cut 2 to the horizontal subcorridor of $L'$. Consider the new-subpiece to be the top-subpiece. Run algorithm recursively on the new-subpiece.
%\item  Scenario $4$ : (Type $3$ cut) Pack the items of $S_{3}$ which is right of cut 3 in a new vertical $\Bc$-corridor $C$. Consider the new-subpiece to be the subpiece which is right of cut 3. Run algorithm recursively on the new-subpiece.
%
%\end{enumerate}
%%The algorithm when run on subpiece $P$, considers one of the above three cases depending on the type of end-to-end cut, augments some items from $S_{1}$ or $S_{2}$ to $L'$ and runs again on the new subpiece. We halt at the iteration when at least one of each type of cut is obtained. The boundaries of subpiece at this step along with the cut considered define the bouding box for remaing set of items of $S$. Thus we get a box surrounded by $L'$ on two edges (left and bottom) and a corridor on the third (right). The fourth (top) edge of box is trivially defined by top edge of $P$\\It is clear that number of new corridors is 2, i.e., one L-corridor and one $\Bc$-corridor. Since we follow the original sequence of guillotine cuts without moving any items, guillotine separability is not disturbed.
%
%We halt if one of the following three cases happens. First case occurs if at some iteration at least one cut from each type of cut is obtained. The boundaries of subpiece at this step along with the cut considered define the bounding box for remaing set of items of $S$. Thus we get a box surrounded by corridors $\{L_{1},L_{2},...,L_{k}\}$ and $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$ . Figure \ref{figtwobends} shows final bounding box $B$ formed after the algorithm alongwith $L_{1}$ formed after considering sequence of type $1$ and type $2$ cuts in subcorridors $S_{1}$, $S_{2}$ and the $\Bc$-corridor $C_{1}$ formed from type $3$ cuts in $S_{3}$. Second case occurs if one or more subcorridors in the piece exhausts i.e. all the items of these subcorridors are already packed in corridors $\{L_{1},L_{2},...,L_{k}\}$ or in $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$. In this case we are left with at most 2 corridors with at most 1 bend who rectangles are not part of the $\Bc$-corridors or corridors created during the recursive procedure. We can use the previous section results to bound this corridor with the a box (Except for a $\Bc$-corridor which will be dealt in the later subsections). Third Case occurs when the next guillotine cut in the sequence is vertical and passes through subcorridor $S_{2}$ only. This leaves us with 2 corridors of at most 1 bend. So, we can use the previous section results to bound the corridors with the boxes (Except for a $\Bc$-corridor which will be dealt in the later subsections).\\
%\\Now we observe that using the algorithm defined above we add only a $O(\frac{1}{\epsl})$ number of new corridors and $\Bc$-corridors. The proof follows from the fact that if it is the case that all algorithm halts when at least one of each type of cuts is obtained then in the end we have corridors  $\{L_{1},L_{2},...,L_{k}\}$ (with at most 1 bend) and $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$. This accounts to $O(\frac{1}{\epsl})$ new $\Bc$-corridors and corridors as new $\Bc$-corridor or corridor is created only when we have scenario 1 and as we have shown there the number of times this scenario occurs is $O(\frac{1}{\epsl})$. Else if it is the case that algorithm halts when one or more of subcorridors is exhausted, then also we have either corridors $\{L_{1},L_{2},...,L_{k}\}$ (with at most 1 bend) or we have $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$ and we have already shown that the number of such $\Bc$-corridors are $O(\frac{1}{\epsl})$. We then run the algorithm on remaining corridors which has lesser number of bends than $S$, i.e., at most 1 bend(if there is any such corridor). As it follows from section \ref{L corridor}, we get $O(\frac{1}{\epsl})$ corridors from processing in this case. For  the third type of halting due to vertical cuts which passes through $S_{2}$ only, we have already shown in the previous paragraph that we obtain only $O(\frac{1}{\epsl})$ new $\Bc$-corridors and corridors.
%\end{comment}

\begin{figure}[t]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.3cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,3) -- (0,0) -- (6,0) -- (6,4) -- ( 5,4) -- (5,1) -- (1,1) -- (1,3) -- (0,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,1.25) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};

			
		

			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,4) -- ( .5,0.5) ;
			\draw[dotted] (.25,4) -- ( .25,0.25) ;
			
			\draw[dotted] (0.25,.5) -- ( 6,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0.5) ;
			
				
		
		\end{tikzpicture}}
		\caption{Guillotine Cuts (dashed lines) through a corridor $S$}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.3cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,4) -- (1,1) -- (7,1) -- (7,5) -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick]  (1.5,6) -- (1.5,1.5) -- (7,1.5);% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[pattern=north east lines, pattern color=black] (6.5,1.5)--(6.5,5)--(7,5)--(7,1.5)--(6.5,1.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,4) -- (1.5,4) -- (1.5,1.5) -- (7,1.5) -- (7,1) --(1,1) -- (1,4);		

			\draw (1.25,1.25) node {\large \textbf{$L_{1}$}};
			\draw (6.75,2.5) node {\large \textbf{$C_{1}$}};
			\draw (4,4) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Final Bounding Box of $S$}
	\end{subfigure}
	\caption{Depiction of Algorithm \ref{boxalgo} for a 2-bend corridor}
	\label{figtwobends}
\end{figure}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.4cm}{
		\begin{tikzpicture}		
			\draw[thick] (0,0) rectangle (6,6);	
			\draw (0,4)--(1,4)--(1,1)--(5,1)--(5,4)--(6,4)--(6,0)--(0,0)--(0,4);
			\draw [solid, fill=lightgray](2.5,2) rectangle (3.5,3);
			\draw [solid, fill=lightgray](2.5,3.5) rectangle (3.5,4.7);
			\draw (0,6) rectangle (3.4,5.5);
			\draw (6,6)--(6,4.5)--(5,4.5)--(5,5.3)--(4,5.3)--(4,6)--(6,6);
			\draw (0,4.5) rectangle (1.5,5);

			\draw[dashed] (0,5.5)--(6,5.5);
			\draw[dashed] (5.75,5.5)--(5.75,0);
			\draw[dashed] (5.25,5.5)--(5.25,0.25);
			\draw[dashed] (5.75,0.25)--(0.25,.25);
			\draw[dashed] (.25,0)--(.25,5.5);
			\draw[dashed] (.5,5.5)--(.5,.25);
			\draw[dashed] (.5,.5)--(5.25,.5);
			\draw[dashed] (0.5,3.25)--(5.25,3.25);
			\draw[dashed] (0.5,1.9)--(5.25,1.9);

		\end{tikzpicture}}
		\caption{}
		\label{fig:c41}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.4cm}{
		\begin{tikzpicture}		
			\draw[thick] (0,0) rectangle (6,6);	
			\draw (0.5,4.5)--(1,4.5)--(1,1.5)--(5,1.5)--(5,4.5)--(5.25,4.5)--(5.25,1)--(.5,1)--(.5,4.5);
			\draw [solid, fill=lightgray](2.5,2.5) rectangle (3.5,3.5);
			\draw [solid, fill=lightgray](2.5,4) rectangle (3.5,5.2);
			
			\draw (5.25,5)--(5,5)--(5,5.8)--(4,5.8)--(4,6)--(5.25,6)--(5.25,5);
			\draw (.5,5) rectangle (1.5,5.5);

%			\draw[dashed] (0,5.5)--(6,5.5);
%			\draw[dashed] (5.75,5.5)--(5.75,0);
			\draw (5.25,6)--(5.25,1);
%			\draw[dashed] (5.75,0.25)--(0.25,.25);
%			\draw[dashed] (.25,0)--(.25,5.5);
			\draw (.5,6)--(.5,1);
			\draw (.5,1)--(5.25,1);
			\draw (0.5,3.75)--(5.25,3.75);
			\draw (0.5,2.4)--(5.25,2.4);

		\end{tikzpicture}}
		\caption{}
		\label{fig:c42}
	\end{subfigure}
	\caption{Depiction of Algorithm \ref{balgo}. (a) Dashed lines denote guillotine cuts. (b) Creation of Boundary Corridor and additional boxes.}
	\label{fig:c43}
\end{figure}

%\begin{comment}
%	\subsubsection{$\Gc$ Corridor}\label{threebends}
%	%Consider a corridor $S$ with 3 bends.  W.l.o.g let us assume that the corridor $S$ can't be divided into smaller corridors with cuts perpendicular to subcorridor.Let us consider vertical subcorridors $S_{1}$ and $S_{3}$ which are on top of horizontal subcorridor $S_{2}$ and $S_{3}$ is right of $S_{1}$ and below horizontal subcorridor $S_{4}$. Now consider a corridor comprising of $S_{1},S_{2},S_{3}$ and assuming the w.l.o.g conditions of previous section we get a box for this triple. Similarly we get a box for the triple $S_{2},S_{3},S_{4}$ . Intersection of both the boxes gives us a box whose edges are the topmost,bottom most, leftmost and rightmost edges of the corridor $S$.  By appropriate shifting of vertical rectangles we can convert it into a L corridor without disturbing the guillotine property.Exact details are available in subsubsection \ref{sss3}.\\
%The approach is similar to section \ref{twobends}. Let $S$ be a corridor with $3$ bends. Let the top left vertical, bottom horizontal, top right vertical subcorridors and top horizontal subcorridors of $S$ be $S_{1}$, $S_{2}$, $S_{3}$ and $S_{4}$ respectively as shown in Figure \ref{figthreebends}. Consider the smallest subpiece $P$ containing $S$. We define four types of end-to-end cuts possible in $P$ or in any of the subpieces formed by a sequence of cuts in $P$. The rightmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$ is termed as Type $1$. The leftmost end-to-end guillotine cut passing during a single stage of guillotine cutting sequence through $S_{3}$ is termed as Type $3$. The topmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{2}$ is termed as Type $2$. The bottommost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{4}$ is termed as Type $4$. Figure \ref{figthreebends} shows all the four types of cuts defined.
%\\Basic idea follows divinding $S$ into a corridor $U'$ (with at most $2$ bends) consisting of some items from $S_{1}$, $S_{2}$, $S_{3}$ ( w.l.og it can be $S_{2}$, $S_{3}$, $S_{4}$ but for the rest of the proof we assume that it's the former case not the latter), a $\Bc$-corridor $C$ from a subset of items of $S_{4}$ and a corridor (with at most 3 bends) with the remaining set of items. We follow a recursive approach to define bounding box $B$. Clearly obtaining all four type of cuts will result in a box  bounded by these cuts. \\
%We now formally define the algorithm for processing corridor $S$ with $3$ bends. From observation \ref{endtoend} we know that the first cut in any guillotine separable piece is end-to-end. Depending on the type of this cut we do the following processing :
%\begin{enumerate}
%\item Scenario $1$ : (Type $1$ cut) Add the items of $S_{1}$ which is left of Cut 1 to the left-vertical subcorridor of the 3-bend corridor $U'$. Consider the new-subpiece to be the subpiece which is right of Cut 1. Run algorithm recursively on the new-subpiece.
%\item Scenario $2$ : (Type $2$ cut) Add the items of $S_{2}$ which is below Cut 2 to the horizontal subcorridor of $U'$. Consider the new-subpiece to be subpiece which is above Cut 2. Run algorithm recursively on the new-subpiece.
%\item Scenario $3$ : (Type $3$ cut) Add the items of $S_{3}$ which is right of Cut 3  to the right-vertical subcorridor of $U'$. Consider the new-subpiece to be the subpiece which is left of Cut 3. Run algorithm recursively on the new-subpiece.
%\item  Scenario $4$ : (Type $4$ cut) Pack the items of $S_{4}$ which is above Cut 4 in a new horizontal $\Bc$-corridor $C$. Consider the new-subpiece to be the subpiece which is below Cut 4. Run algorithm recursively on the new-subpiece.
%\end{enumerate}
% We halt if one of the following three cases happens. First case occurs if at some iteration at least one cut from each type of cut is obtained. The boundaries of subpiece at this step along with the cut considered define the bouding box for remaing set of items of $S$. Thus we get the box $B$ surrounded by $U'$ on three edges and a $\Bc$-corridor $C$ on the fourth. Figure \ref{figthreebends} shows final bounding box $B$ formed after the algorithm alongwith $U'$ formed after considering sequence of type $1$ ,type $2$ and type $3$ cuts in subcorridors $S_{1}$, $S_{2}$, $S_{3}$ and the $\Bc$-corridor formed from type $4$ cuts in $S_{4}$. Second case occurs if one or more of the subcorridors in the piece exhausts, i.e., all the items of subcorridor are already packed in $U'$ or in $C$. In this case we are left with at most 2 corridors with at most 2 bends whose items are not part of either $U'$ or $C$. Using the previous section we get that the corridor with at most two bends is bounded by a box (Except for a $\Bc$-corridor which will be dealt in the later subsections) . Third Case occurs when the next guillotine cut in the guillotine cutting sequence passes completely through any subcorridor perpendicular to its longer sides. This divides $S$ into at most three corridors with at most 2 bends each. Using the previous section results each corridor with at most two bends is bounded by a box (Except for a $\Bc$-corridor which will be dealt in the later subsections) .\\
%\\Now we observe that using the algorithm defined above we add only a $O(\frac{1}{\epsl})$ number of new corridors and $\Bc$-corridors. The proof follows from the fact that if it the case that all algorithm halts when at least one cut from each type of cuts is obtained then in the end we have a corridor ( with at most 3 bends) , a $\Bc$-corridor and a bounding box. This accounts to $O(1)$ new $\Bc$-corridors and corridors. Else if it is the case that algorithm halts when one or more of subcorridors is exhausted, i.e., packed in either $U'$ or $C$, then we have a new corridor (with at most 2 bends) or one new $\Bc$-corridor $C$. We then run the algorithm on remaining corridors which has lesser number of bends than $S$ i.e. at most 2 bends (Except for a $\Bc$-corridor which will be dealt in the later subsections) . As it follows from subsections \ref{twobends} and \ref{L corridor}, we get $O(\frac{1}{\epsl})$ corridors from processing in both the cases. In the third case of halting, $O(\frac{1}{\epsl})$ extra $\Bc$-corridors follows from the results of subsections \ref{twobends} and \ref{L corridor}.
%\end{comment}
%
%\begin{figure}[h]
%	%\centering
%	\captionsetup[subfigure]{justification=centering}
%	\hspace{-10pt}
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{3.5cm}{
%		\begin{tikzpicture}
%				
%			%box
%
%			\draw[thick] (0,3) -- (0,0) -- (6,0) -- (6,4) --( 2,4)--(2,3)--(5,3) -- (5,1) -- (1,1) -- (1,3) -- (0,3); 
%
%			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
%			\draw (3,0.75) node {\large \textbf{$S_{2}$}};
%			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};
%                           \draw (3,3.5) node {\large \textbf{$S_{4}$}};
%
%			\draw (1,3.7) node {\large \textbf{Type 1}};
%			\draw (6.9,.45) node {\large \textbf{Type 2}};
%			\draw (6,4.7) node {\large \textbf{Type 3}};
%			\draw (6.9,3.2) node {\large \textbf{Type 4}};
%
%			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
%			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
%			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
%			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);
%
%			\draw[dotted] (.5,3.5) -- ( .5,0) ;
%			\draw[dotted] (.25,3) -- ( .25,0) ;
%			
%			\draw[dotted] (0,.5) -- ( 6.5,0.5) ;
%			\draw[dotted] (0,.25) -- ( 6,0.25) ;
%			
%			
%			\draw[dotted] (5.5,4.5) -- ( 5.5,0) ;
%			\draw[dotted] (5.25,4) -- ( 5.25,0) ;
%
%			\draw[dotted] (2,3.5) -- ( 6,3.5) ;
%			\draw[dotted] (2,3.25) -- ( 6.5,3.25) ;
%				
%		
%		\end{tikzpicture}}
%		\caption{Types of cuts}
%	\end{subfigure}
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{3.5cm}{
%		\begin{tikzpicture}
%				%box	
%			\draw  (0,0) rectangle (8,6);
%			\draw[thick] (1,4) -- (1,1) -- (7,1) -- (7,5) -- ( 6,5) --(3,5)--(3,4)--(6,4)-- (6,2) -- (2,2) -- (2,4) -- (1,4); 
%			\draw[thick]  (1.5,1.5) -- (1.5,6) ;% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
%			\draw[thick] (6.5,1.5)-- (6.5,6); 
%			\draw[thick] (6.5,4.5)--(1.5,4.5);
%			\draw[pattern=north east lines, pattern color=black] (6.5,4.5)--(6.5,5)--(3,5)--(3,4.5)--(6.5,4.5);
%	
%			\draw[pattern=north west lines, pattern color=gray] (1,4) -- (1.5,4) -- (1.5,1.5) -- (6.5,1.5) -- (6.5,5) --(7,5) -- (7,1)--(1,1)--(1,4);		
%
%			\draw (4,1.25) node {\large \textbf{$U'$}};
%			\draw (5,4.75) node {\large \textbf{$C$}};
%			\draw (4,3) node {\large \textbf{$B$}};
%			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
%			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
%			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
%							
%
%		\end{tikzpicture}}
%		\caption{Final Bounding Box of $S$}
%	\end{subfigure}
%	\caption{Processing 3-bend corridor}
%	\label{figthreebends}
%\end{figure}
%
%
%\begin{figure}[h]
%	%\centering
%	\captionsetup[subfigure]{justification=centering}
%	\hspace{-10pt}
%		\centering
%		\resizebox{!}{4cm}{
%		\begin{tikzpicture}		
%			\draw[thick] (0,0) rectangle (6,6);	
%			\draw (2.3,1.5) rectangle (3.7,4.5);
%			\draw [thick,pattern=north east lines,pattern color=gray] (1,2.5) rectangle (3,3.5);
%			\draw[dashed] (0,2.5)--(6,2.5);
%			\draw[dashed] (0,3.5)--(6,3.5);
%			\draw[dashed] (3,0)--(3,6);
%			
%
%		\end{tikzpicture}}
%	\caption{Box (Region which has north-east lines) divides the $\Bc$-corridor into 6 parts }
%	\label{fig:c4}
%\end{figure}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.35\textwidth}
		\centering
		\resizebox{!}{3.4cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,3) -- (0,0) -- (6,0) -- (6,4) --( 2,4)--(2,3)--(5,3) -- (5,1) -- (1,1) -- (1,3) -- (0,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,0.75) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};
                           \draw (3,3.5) node {\large \textbf{$S_{4}$}};

			
			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,4) -- ( .5,0.5) ;
			\draw[dotted] (.25,4) -- ( .25,0.25) ;
			
			\draw[dotted] (0.25,.5) -- ( 5.75,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0.5) ;
			\draw[dotted] (5.75,4.5) -- ( 5.75,0.25) ;

			\draw[dotted] (0.5,3.5) -- ( 5.5,3.5) ;
			
				
		
		\end{tikzpicture}}
		\caption{}
		\label{figthreebends}
	\end{subfigure}
	\begin{subfigure}[b]{.34\textwidth}
		\centering
		\resizebox{!}{3.1cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,4) -- (1,1) -- (7,1) -- (7,5) -- ( 6,5) --(3,5)--(3,4)--(6,4)-- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick]  (1.5,1.5) -- (1.5,6) ;% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[thick] (6.5,4.5)--(1.5,4.5);
			\draw[pattern=north east lines, pattern color=black] (6.5,4.5)--(6.5,5)--(3,5)--(3,4.5)--(6.5,4.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,4) -- (1.5,4) -- (1.5,1.5) -- (6.5,1.5) -- (6.5,5) --(7,5) -- (7,1)--(1,1)--(1,4);		

			\draw (4,1.25) node {\large \textbf{$U'$}};
			\draw (5,4.75) node {\large \textbf{$C$}};
			\draw (4,3) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{}\label{figthreebends1}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\resizebox{!}{3.1cm}{
		\begin{tikzpicture}		
			\draw[thick] (0,0) rectangle (6,6);	
			
			\draw [fill=white] (1,2.5) rectangle (3,3.5);
			\draw [thick,pattern=north east lines,pattern color=gray] (1,2.5) rectangle (3,3.5);
			\draw[dashed] (0,2.5)--(6,2.5);
			\draw[dashed] (0,3.5)--(6,3.5);
			\draw[dashed] (3,0)--(3,6);
			\draw (2.3,1.5) rectangle (3.7,4.5);

		\end{tikzpicture}}
	\caption{}
	\label{fig:c4}
	\end{subfigure}
	\caption{Figure(a)$\&$(b): Depiction of Algorithm \ref{boxalgo} for a 3-bend corridor. (a) Guillotine Cuts (dashed lines) through a corridor $S$. (b) Final Bounding Box of $S$. Figure(c): Box (Region which has north-east lines) divides the $\Bc$-corridor into 6 parts.}
\end{figure}

	\subsubsection{B-Corridor} \label{finalB}
	In this subsection we deal with the items inside a $\Bc$-corridor in 2 ways. In first way, the $\Bc$-corridors can be either divided into $O_{\eps,\epsl}(1)$ $\Bc$-corridors and the $\Bc$-corridors as a pseudo rectangle are guillotine separable. In second way, the items in $\Bc$-corridors are merged with a corridor and later become a part of boundary $\Lc$. Given a knapsack, first we construct the guillotine separable boxes as mentioned in the previous subsections. Note that one box may lie completely inside another box. Now consider the set of outermost boxes which are not part of any other box in the original knapsack. Note that the boundaries of outermost boxes may divide the $\Bc$-corridors into smaller parts. The number of such smaller parts is $O(\frac{1}{\epsl})$ as the guillotine cuts which are part of the boundary of a single box can divide a $\Bc$-corridor into at most 6 parts (as shown in Figure \ref{fig:c4}) and number of such boxes is $O(\frac{1}{\epsl})$. Now we have to deal with 2 cases.\\
\\ In the first case, a $\Bc$-corridor say $S$ lies inside a box $\mathcal{B}$. Algorithm \ref{balgo} merges a part of $S$ in boundary corridor $C$ that is being created. Then after this we convert $C$ to a boundary-$\Lc$. The region in the box $\mathcal{B}$ which doesn't contain the boundary-$\Lc$ can be thought of as a smaller knapsack and we repeat our case analysis depending whether the portion of $S$ which isn't merged in the boundary-$\Lc$  is part of any box in the new knapsack or not. We satisfy all the properties of Theorem \ref{thm:ldecom}. \\
\\Now in the second case the $\Bc$-corridors lie outside any box in the original knapsack. Now consider the set of guillotine cuts which separates out the boxes when considered as a pseudoitem and the rectangles in $\Bc$-corridors. Note that the way we have constructed the outermost boxes the guillotine cuts don't pass through the boxes except its edges.  Let the first stage cuts be horizontal. These cuts divide the knapsack into horizontal strips. Merge adjacent strips if they contain only horizontal rectangles. Make a horizontal strip a $\Bc$-corridor if it contains atleast one rectangle and all of them are horizontal. Now take the strip which contains vertical items and repeat above step by considering the vertical cuts and appropriately creating new $\Bc$-corridors in the similar fashion. Continue this process repeatedly until we are left with a subpiece containing only one type of rectangles or a pseudoitem. Make the subpiece containing one type of rectangles a $\Bc$-corridor. Now we claim that the number of $\Bc$-corridors created is at most $O_{\epsl,\eps}(1)$. Note that during the first stage of cutting, the number of strips containing vertical items is $O_{\epsl}(1)$. Therefore number of $\Bc$-corridors created during the first stage of cutting is  $O_{\epsl}(1)$. By similar logic we can show that during any stage of cutting, only $O_{\epsl}(1)$ $\Bc$-corridors were created. So to prove our claim it suffices to show that the number of the stages is $O_{\epsl,\eps}(1)$. Also number of stages where more than one horizontal strip contains vertical items is $O_{\epsl,\eps}(1)$. We can draw similar conclusions for vertical stage cuts. So let us assume that only one horizontal (resp. vertical) strip during any horizontal (resp. vertical) stage cutting contains vertical (resp. horizontal ) items. Since we had only $\Bc$-corridors and pseudo items before we started this process, no two consective stage cuts extracts rectangles from the same corridor (this wouldn't have been the case if there were $\Lc$-corridors) . Due to maximality conditions of the strips being created it easy to observe that for $2k$ stages of cuts, we have extracted rectangles from atleast $k$ corridors (see Figure \ref{bcorO1}).  Since there are atmost $O_{\epsl,\eps}(1)$ corridors, therefore the number is stages is also $O_{\epsl,\eps}(1)$.
%\begin{itemize}
%\item Subcase 3: Consider a set of horizontal cuts through $S_{1}$ which are intercepted by the rectangles which belonged to the same corridor $S_{2}$. Now assume 2 or more than 2 consecutive horizontal cuts do not have space more than $\epsl N$ between them (otherwise the cuts are intercepted by at most $O_{\epsl}(1)$ rectangles) . Then we take that cut $l$ among the consecutive cuts such that $|l \cap S_{2}|$ is maximum and shift vertically those rectangles which intercepted these consecutive cuts other than $l$ and make them touch $l$. Hence we consider $l$ as valid guillotine cut and deal with the rest of the consecutive cuts using the Subcase 1. Subcase 3 is depicted in Figure \ref{C02a} and Figure \ref{C02b}.  
%\item Subcase 1:  Now consider the horizontal cuts (which are not entirely inside the $\Bc$-corridor $S_{1}$) through $S_{1}$. If 3 or more horizontal cuts are intercepted by the same vertical cut in the guillotine cutting sequence then include the topmost and the bottom cut in the set $G$. This subcase is depicted in Figure \ref{C01b}.
%\item Subcase 2: Now consider the set of vertical cuts which intercept the horizontal cuts through $S_{1}$. If these vertical cuts are edges of an outermost box which we created then there can be at most $O(\frac{1}{\epsl})$ of them. Now if these vertical cuts are edges of vertical rectangle which belonged to different corridors then these can be at most $O_{\eps}(1)$ of them. Both of the scenarios are depicted together in Figure \ref{C01c}.

%\item Subcase 4: Using the same techniques of Subcase 1 and 3 (No need of Subcase 2 as the cuts there interact with different boxes or corridors)
%and applying it to the vertical cuts which pass through some vertical corridor $S_{3}$ with zero bends (repeat the same for other set of cuts which pass through the same vertical $\Bc$-corridor)  and are intercepted by the rectangles in $S_{2}$ we get that there can be at most $O(\frac{1}{\epsl})$ vertical cuts  (which are not entirely inside the $\Bc$-corridor $S_{1}$) passing through $S_{1}$ since width of each rectangle is at least $\epsl N$. This subcase is depicted in Figure \ref{C01a} (even depicted in the Figures \ref{C01b} and \ref{C02b} if we rotate them by 90 degrees).
%\end{itemize}
%Now we argue that at most $O(\frac{1}{\epsl})$ horizontal cuts (which are not entirely inside the $\Bc$-corridor $S_{1}$) pass through the $\Bc$-corridor $S_{1}$. Subcase 2 and Subcase 3 ensure that the number of vertical cuts which intercept the horizontal cuts passing through $S_{1}$ is $O_{\eps,\epsl}(1)$. And for each such vertical cut we end up keeping at most 2 horizontal cuts which pass through $S_{1}$ as explained in Subcase 1. Now these horizontal cuts along with the vertical cuts of Subcase 4 and vertical edges of $S_{1}$ results into partition of $S_{1}$ into $O_{\eps,\epsl}(1)$ $\Bc$-corridors and these corridors when considered as a pseudo rectangle is guillotine separable

 Now the procedure mentioned above is recursively applied to those portion of the outermost boxes which doesn't have items from its boundary-$\Lc$.  This process stops when there is no $\Bc$-corridor which when considered as a pseudoitem isn't guillotine separable. Number of such boxes bounding the $\Lc$-corridor or items of a $\Bc$-corridor is $O_{\eps,\epsl}(1)$. This follows from constructive procedures in subsection \ref{ssss} and the fact that we started the section with $O_{\eps,\epsl}(1)$ $\Bc$-corridors and corridors.

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[t]{.32\textwidth}
		\centering
		\resizebox{!}{3.4cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,8);
			\draw (4,6) rectangle (7,7.8);
			\draw (1,1) rectangle (3,5);
			\draw[dotted] (0,7.5) -- ( 8,7.5) ;
			\draw[dotted] (1.5,7.5) -- ( 1.5,0) ;
			\draw[dotted] (1.5,7.2) -- ( 8,7.2) ;
			\draw[dotted] (1.8,7.2) -- ( 1.8,0) ;
			\draw[dotted] (1.8,6.5) -- ( 8,6.5) ;
			\draw[dotted] (2.5,6.5) -- ( 2.5,0) ;
			\draw[dotted] (2.5,6) -- ( 8,6) ;
			\draw[dotted] (3,6) -- ( 3,0) ;
			\draw[solid,fill=lightgray] (3.1,0) rectangle (7.9,5.8);
			
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{}\label{C01a}
	\end{subfigure}
	\begin{subfigure}[t]{.32\textwidth}
		\centering
		\resizebox{!}{3.4cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,8);
			\draw (4,6) rectangle (7,7.8);
			\draw (1,1) rectangle (3,5);
			
			\draw[dotted] (0,6) -- ( 8,6) ;
			\draw[dotted] (3,0) -- ( 3,6) ;
				\draw[solid,fill=lightgray] (3.1,0) rectangle (7.9,5.8);			

		\end{tikzpicture}}
		\caption{ }\label{C01b}
	\end{subfigure}
	\begin{subfigure}[t]{.32\textwidth}
		\centering
		\resizebox{!}{3.4cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,8);
			\draw[dotted] (0,7.5) -- ( 8,7.5) ;
			\draw[dotted] (1.5,7.5) -- ( 1.5,0) ;
			\draw[dotted] (1.5,7.2) -- ( 8,7.2) ;
			\draw[dotted] (1.8,7.2) -- ( 1.8,0) ;
			\draw[dotted] (1.8,6.5) -- ( 8,6.5) ;
			\draw[dotted] (2.5,6.5) -- ( 2.5,0) ;
			\draw[dotted] (2.5,6) -- ( 8,6) ;
			\draw[dotted] (3,6) -- ( 3,0) ;
			\draw[thick] (3,5)--(8,5);
			\draw[thick] (4,0)--(4,5);
			\draw[solid, fill=lightgray]  (3.1,5.2) rectangle (7.9,5.4);					
			\draw[solid, fill=lightgray]  (3.2,0.1) rectangle (3.4,4.9);
			\draw[solid, fill=lightgray]  (3.1,5.2) rectangle (7.9,5.4);					
			\draw[solid, fill=lightgray]  (3.2,0.1) rectangle (3.4,4.9);
			\draw[solid, fill=lightgray]  (2.6,0.1) rectangle (2.8,5.9);
			
		\end{tikzpicture}}
		\caption{}\label{C01c}
	\end{subfigure}
	
	\caption{Creating guillotine separable $\Bc$-corridors. Figure \ref{C01a}: Assume that the rectangles are in the $\Bc$-corridors and the pseudoitem. Here we have 8 stages of cuts but we are extracting rectangles from 2 corridors. But the way these corridors are getting it can happen only when we dont consider all the first stage cuts. Hence we won't end up with such corridors and instead we will end up with corridors as shown in Figure \ref{C01b}  Figure \ref{C01c} : Here the dotted the lines denote the $2k$ stages of cuts and the 2 thick lines denote the $2k+1$ and $2k+2$ stage cuts. Now observe that a rectangle extracted from a new corridor in $2k+2$-th stage cut as the rectangle in the $2k$-th stage cut belonged to a different corridor. Instead if the belonged to the same corridor, the rectangle in  $2k$-th stage cut must be below the rectangle in $2k+1$-th stage and therefore we can merge $2k+1$ and $2k+2$ strips with their adjacent strips and can end up with $2k$ stage cuts. Similar idea works for the other arrangements too}
\label{bcorO1}
\end{figure}





%\begin{comment}
%	Consider a boundary $\Lc$ corridor $S$ with vertical subcorridor $S_{1}$ placed top left with respect to the horizontal subcorridor $S_{2}$. Now consider a sequence of guillotine cuts (cut is parallel to the orientation of the subcorridor and the rectangles which are being separated in that subcorridor) which separates the rectangles in the boundary $\Lc$. Continue this process till there doesn't exist any such cut. Either we have separated all the rectangles of a subcorridor of boundary $\Lc$ or still we have a portion of the boundary $\Lc$ left. In the former case we fix the rectangles which got separated due to guillotine cuts as the boundary $\Lc$ of the original box. In the later case w.l.o.g let the next stage of cuts be horizontal and these cuts passes though $S_{1}$ only . Now consider the lowermost cut among these horizontal cut. Let it be $l$. Let $l$ be at a distance of $h$ from the top of the box. If $h \leq \epsl N$,we remove the items in the strip above $l$, then we shift upwards the rectangles below the cut $l$ except those rectangles which got separated due to previous guillotine cuts by a distance of $h$ and then place the rectangles from the strip which we removed initially in the empty region created due to shifting. Otherwise if $h > \epsl N$ then we consider the items separated due to cuts before $l$ as the boundary $\Lc$ of the original box and we divide rest of region of the box into 2 smaller boxes with cut $l$ being the common edge between both the smaller boxes. Now that an original boundary $\Lc$ along with some $\Bc$-corridors gets divided into $O(\frac{1}{\epsl})$ smaller boundary $\Lc$. The reason being that a boundary $\Lc$ and some $\Bc$-corridors get divided into smaller boundary $\Lc$ only if the height of the new box which we are about to create is greater than $\epsl  N$ and therefore number of such boxes is $O(\frac{1}{\epsl})$. Similar processes can be done to corridors with 2 or 3 bends.
%
%	\subsubsection{Converting boundary corridor with $2$ bends to a single Boundary $\Lc$ in a box}\label{sss2}
%	Let us consider a boundary corridor with $2$ bends with two vertical subcorridors $S_{1}, S_{3}$ on top of the horizontal subcorridor $S_{2}$ with $S_{3}$ being placed to the right of $S_{1}$. W.l.o.g let us assume that the first stage cuts in the guillotine cutting sequence in the box is vertical. Now consider the cut $l$ through $S_{3}$. Let the distance between $l$ and edge of the boundary be $d$. Now remove the strip to the right of $l$ and shift the rest of items of box to the right by a distance of $d$. Now in the empty region created near the left edge of the box we place the strip which we removed. Now consider the rectangles in this strip, rectangles to the left of cut through $S_{1}$ before the shifting procedure and set of horizontal rectangles whose guillotine cut is intercepted by the former rectangles mentioned in this sentence. We now freeze these rectangles after shifting and consider the rest of the box as a new box and recursively apply the process to remaining part of the corridor till we don't have any vertical guillotine cuts left. If we have exhausted the corridor then we are done and we have a single boundary $\Lc$. Otherwise we must have horizontal cut through the remaining portion of the box to separate the rectangles because there no end to end vertical cut. We handle this in sub-subsection \ref{sssl}. The boundary $\Lc$ achieved due to the sequence of guillotine cuts forms the boundary $\Lc$ of the box. Also this boundary $\Lc$ can be converted into $O_{\epsl}$ smaller boundary $L$ with width at most $\epsl N$ by  dropping at most $O_{\eps,\epsl}(1)$ items as shown in Figure \ref{divL}. 
%	\subsubsection{Converting boundary corridor with 3 bends to a single Boundary $\Lc$}\label{sss3}
%	Consider a boundary corridor $S$ with 3 bends. Let us consider vertical subcorridors $S_{1}$ and $S_{3}$ which are on top of horizontal subcorridor $S_{2}$. $S_{3}$ is right of $S_{1}$ and below horizontal subcorridor $S_{4}$. Consider the horizontal guillotine cut through $S_{4}$ and remove the rectangles above this cut and place it  below corridor $S_{2}$ by shifting rectangles below the cut upwards. Now freeze this set of rectangles from $S_{4}$ which were moved down. Now in the remaining portion of the box take the vertical guillotine cut through $S_{3}$ and remove the rectangles to the right of this cut and place it to the left of $S_{1}$. Now freeze the rectangles in the similar fashion as done in the Sub-subsection \ref {sss2} and recursively repeat the process for the rectangles in subcorridors $S_{3}, S_{4}$ which aren't freezed yet till we exhaust these both the corridors. Note that we stop if there is no vertical cut through $S_{3}$ or a horizontal cut through $S_{4}$ then there must exist which divides the remaining portion of the box into 2 parts each containing corridors with at most 2 bends. If any one of them has a corridors of 2 bends then we can use the results of sub-subsection \ref{sss2} to get a box with boundary $\Lc$. Otherwise, we are done  and the rectangles which got freezed before this step form the boundary $\Lc$ of our original box with which we started initially. Also this boundary $\Lc$ can be converted into $O_{\epsl}$ smaller boundary $L$ with width at most $\epsl N$ by  dropping at most $O_{\eps,\epsl}(1)$ items  as shown in Figure \ref{divL}.
%
%\begin{figure}[h]
%	%\centering
%	\captionsetup[subfigure]{justification=centering}
%	\hspace{-10pt}
%
%		\centering
%		\resizebox{!}{3.5cm}{
%		\begin{tikzpicture}
%				%box	
%			\draw  (0,0) rectangle (10,10);
%			
%			\draw [solid,fill=lightgray] (0,0)--(0,10)--(3,10)--(3,3)--(10,3)--(10,0)--(0,0);
%			
%			\draw [dashed] (1,10)--(1,1)--(10,1);
%			\draw [dashed] (2,10)--(2,2)--(10,2);
%			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
%			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
%			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
%							
%
%		\end{tikzpicture}}
%
%
%
%	\caption{Dividing a boundary $L$ (shaded region) into smaller boundary using dashed lines as shown in this figure. Vertical and horizontal dashed lines meet at the boundary curve. Dashed lines also form the edges of the smaller boxes which bound the new $L$ corridors being created}\label{divL}
%
%\end{figure}
%	           \end{comment}
	%\subsubsection{Merging 2 boundary $\Lc$ into a single boundary $\Lc$}\label{sss2l}
	%Now consider that we have 2 boundary $\Lc$ for the same box. If there is any end to end cut possible in the box which doesn't pass through any of the 2 boundary $\Lc$ or it passes through one or more than one subcorridors of 2 boundary $\Lc$ but it is perpendicular to the orientation of these subcorridors, then we divide the box into 2 boxes. We repeat the same procedure on the smaller box which contains both the boundary $\Lc$. If at any stage we find a cut which places both the boundary $\Lc$ in 2 different smaller boxes then we are done. So we now assume that there is no such end to end cut in the box we are considering which has 2 boundary $\Lc$. If the 2 boundary $\Lc$  are placed diagonally opposite to each other then consider the 2 boundary $\Lc$ as a corridor with 3 bends and convert into a single boundary $\Lc$ as mentioned in the subsubsection  \ref{sss3}. If the process in subsection \ref{sss3} can't covert it into a single boundary $\Lc$ it means in the remaining portion of the box which hasn't formed a part of the boundary $\Lc$ we have an end to end cut which separates the 2 remaining portions of the 2 boundary $\Lc$. If the boundary $\Lc$ are placed at the adjacent corners of the box then consider the 2 boundary $\Lc$ as a corridor with 2 bends and convert it into a single boundary $\Lc$ as mentioned in the subsubsection \ref{sss2}. If the process in subsection \ref{sss2} can't covert it into a single boundary $\Lc$ it means in the remaining portion of the box which hasn't formed a part of the boundary $\Lc$ we have an end to end cut which separates the 2 remaining portions of the 2 boundary $\Lc$.
	%\subsubsection{Merging 3 boundary $\Lc$ into a single boundary $\Lc$}\label{sss3l}
	%Now consider that we have 3 boundary $\Lc$ for the same box. If there is any end to end cut possible in the box which doesn't pass through any of the 3 boundary $\Lc$ or it passes through one or more than one subcorridors of 3 boundary $\Lc$ but it is perpendicular to the orientation of these subcorridors, then we divide the box into 2 boxes. One of the box contains 2 boundary $\Lc$ and other box contains 1 boundary $\Lc$. Boxes with 2 boundary $\Lc$ is handled in subsubsection \ref{sss2l}. So we now assume that there is no such end to end cut in the box we are considering which has 3 boundary $\Lc$. Now consider the 3 boundary $\Lc$ as a corridor with 3 bends and convert into a single boundary $\Lc$ as mentioned in the subsubsection  \ref{sss3}. If the process in subsection \ref{sss3} can't covert it into a single boundary $\Lc$ it means in the remaining portion of the box which hasn't formed a part of the boundary $\Lc$ we have an end to end cut which separates the 3 remaining portions of the 3 boundary $\Lc$ into smaller boxes with one box containing 2 boundary $\Lc$ and other box containing 1 boundary $\Lc$. Boxes with 2 boundary $\Lc$ is handled in subsubsection \ref{sss2l}.
	 %\subsubsection{Merging 4 boundary $\Lc$ into a single boundary $\Lc$}\label{sss4l}
	%Now consider that we have 4 boundary $\Lc$ for the same box. If there is any end to end cut possible in the box which doesn't pass through any of the 4 boundary $\Lc$ or it passes through one or more than one subcorridors of 4 boundary $\Lc$ but it is perpendicular to the orientation of these subcorridors. Each box has now 2 boundary $\Lc$. Boxes with 2 boundary $\Lc$ is handled in subsubsection \ref{sss2l}. So we now assume that there is no end to end cut in the box we are considering which has 4 boundary $\Lc$. Let's combine these to form a ring. Now consider the sequence of gullotine cuts which separate the rectangles in the ring. If we are cutting (cut is parallel to the orientation of the subcorridor and the rectangles which are being separated in that subcorridor) through leftmost vertical subcorridor or bottom most horizontal subcorridors then we freeze these rectangles as we freezed rectangles in subsubsection \ref{sss2l} and \ref{sss3l}. Now in the remaining portion of the box if there is a cut $l_{1}$ (cut is parallel to the orientation of the subcorridor) through rightmost vertical subcorridor and the distance between $l_{1}$ and edge of the boundary to the right of it be $d$ then we remove the strip to the right of $l_{1}$ and shift the rest of items of box which are not freezed to the right by a distance of $d$. Now in the empty region created near the left edge of the box we place the strip which we removed. Now freeze the rectangles in the strip which we moved. Do the same process if there is a cut (cut is parallel to the orientation of the subcorridor the rectangles which are being separated in that subcorridor) through the upper most horizontal corridor and now instead of shifting the strip above the cut to the left we shift it down by appropriately shifting the remaining portion of the box upwards which isn't still freezed. Continue this process till we convert these in to single boundary $\Lc$. If at some we can no longer find any cut parallel to the orientation of the subcorridors in the remaing portion of the ring it implies that there should exist an end to end cut in the remaining portion of the box which divides the remaining portion of the box into 2 boxes each containing 2 boundary $\Lc$ at most and this case is dealt in subsubsection \ref{sss2l}. So now have a box with boundary $\Lc$ and possibly 2 smaller boxes each containing 2 boundary $\Lc$.

This completes the proof of $\Bc\Lc$-arrangement.

\subsection{Functions used in BL-arrangement}
\label{subsec42}
Now we describe functions used in the processing of spiral corridors to obtain $\Bc \Lc$-arrangement.
%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Explanation of Algorithms }

%%% Algo 1
\subsubsection{Algo-separate(C, {\em List}, {\em Halting conditions},{\em Type})}

\noindent Algo-separate(.) is one of the main subroutines in our decomposition. We explain it here briefly ( see Algorithm \ref{sepalgo} for the exact details).   
Algo-separate(.) takes as input a spiral corridor $C$ with $k$ subcorridors $\{ S_{1},S_{2},S_{3},...,S_{k}\}$ such that $\forall i \in [k-1]$, $S_{i}$ and $S_{i+1}$ share a region $S_{i,i+1}$ with each other. We are also given a {\em List}, a set of the subcorridors of $C$. Algo-separate(.) tries to extract a smaller corridor from the main corridor $C$ using the cuts of the type $C_p$ such that the items belong to the subcorridors mentioned in the {\em List}. 
The function also takes {\em Halting conditions} as input which denote the scenarios under which the Algo-separate(.) halts the process of extracting any item from a subcorridor. 
Depending on the cases, the halting conditions can be as follows: (i) presence of cut $l$ of Type $C_b$ or $C_{u}$ in $C$,  and (ii) at least one rectangle is obtained from each subcorridor of $C$. 
First Halting condition takes care of the situation where we separated out all the rectangles from one subcorridor say $S_{i'}$ as in this case we have cut which passes through the boundary of $S_{i'}$ which is also a cut of Type $C_b$ which passes through the subcorridor which shares region with $S_{i'}$. First Halting Condition also takes care of the situation where we no longer have any cuts left of Type $C_p$ or $C_b$ passing through the subcorridors in the {\em List} which implies that the next has to be a cut of Type $C_u$. 
There are two {\em types}:  {\em Boundary} and {\em Ordinary}, according to which we  
 separate out different types (either boundary-corridor or corridors that are not boundary-corridors) of smaller spiral corridor $C'$  
 with at most 3 bends from the corridor $C$ (e.g., we separate out a $\Gc'$ corridor in Figure \ref{bends}). 

We now give an intuitive idea how exactly the smaller corridors are extracted.
Consider a sequence of guillotine cuts through subcorridors $S_{i_1}, \dots, S_{i_{b(C')+1}}$ (these are part of the {\em List}) such that these cuts are of Type $C_p$ and $C_b$ and these occurred until one of the halting conditions in the parameter {\em Halting conditions} in Algo-separate(.) was satisfied.  Consider the set of cuts which occurred last in their respective subcorridors. These cuts clearly  extracts $C'$ from $C$. This process is clearly depicted in Figure \ref{sepi1} and Figure \ref{sepi2} where we want to extract an $\Lc$-corridor from the original corridor. 

 
 %%%% Algo 2
 
\begin{algorithm}
\caption{Algo-separate($C$, {\em List}, {\em Halting conditions},{\em Type})}\label{sepalgo}
\begin{algorithmic}[1]
\STATE Let $C'$ be the corridor which will be separated.
\STATE $k \gets 1$
\WHILE {(No {\em Halting condition} is satisfied)}
\STATE Do guillotine cuts of stage-$k$
\STATE $k \gets k+1$
\ENDWHILE
\STATE Let $\mathcal{C}$ be the set of cuts of Type $C_p $ and $C_b$ passing through the subcorridors\\ in {\em List} which occurred last in their respective subcorridors.\label{stepcut}
\IF {(`Type' is {\em Boundary})}
\STATE Use $\mathcal{C}$  to separate out a boundary spiral corridor $C'$ from Box $\mathcal{B}$, bounding $C$.
\ELSIF {(`Type' is {\em Ordinary})}
\STATE Use $\mathcal{C}$  to separate out the spiral corridor $C'$ (contains items from subcorridors \\in the {\em List}, some subcorridors in $C'$ can be degenerate too.  This  may lead to \\$O(1)$ spiral corridors) from $C$
\ENDIF
\STATE Return the Halting Condition which got satisfied in {\em while} loop along with the $C'$.
\end{algorithmic}
\end{algorithm}
 

\subsubsection {Algo-Spiral(C)}

\noindent Using the function Algo-Spiral($C$) we divide a spiral corridor $C$ with more than 3 bends into spiral corridors with at most 3 bends (see Algorithm \ref{spialgo} for more details). We extract the rectangles from the leftmost, bottom most, rightmost and topmost subcorridor in $C$ using the function Algo-separate(.). If we extract all the rectangles from any one of the four subcorridors, then we have a cut of type $C_b$ which divides the remaining portion of the corridor $C$ (whose rectangles are not extracted yet) into $O_\eps(1)$ corridors with lesser number of bends than $C$. Instead if we had some cut of type $C_u$ in $C$ then it would divide the remaining portion of $C$ (whose rectangles are not extracted yet) into  $O_\eps(1)$ corridors with lesser number of bends than $C$. We repeat the same procedure on the smaller corridors created and this procedure stops if there is no corridor with more than 3 bends.

{\em Technical Details of Algorithm:} The number of new spiral corridors created is $O_{\eps,\epsl}(1)$. The reason is that the number of cuts of type $C_u$ or $C_b$ is $O_{\eps,\epsl}(1)$ as $C$ has at most $O(\frac{1}{\eps})$ bends and  each rectangle is greater than $\epsl N$ in one dimension. Plus each cut of type $C_u$ or $C_b$ creates $O_\eps(1)$ extra corridors.The Algorithm terminates because after each such cut of type $C_b$ or $C_u$ we get corridors of lesser number of bends than the original spiral corridor. Algorithm \ref{spialgo} is depicted in Figure \ref{bends}.

\begin{algorithm}
\caption{Algo-Spiral($C$)}\label{spialgo}
\begin{algorithmic}[1]
\STATE Let {\em List} be the set of subcorridors containing the leftmost, bottom-most,\\ rightmost and topmost subcorridor.
\STATE Call Algo-separate($C$, {\em List}, {\em presence of cut $l$ of Type $C_u$ or $C_b$ in $C$}, {\em Ordinary})\label{spi2}
\STATE Partition the existing corridors after the previous step into smaller corridors \\using the cut $l$\label{spi1}.
\STATE Call Algo-Spiral($C''$) for all newly created corridor $C''$ with $b(C'')>3$.
\end {algorithmic}
\end{algorithm}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.3cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,4) -- (0,0) -- (6,0) -- (6,4) --( 0,4);
			\draw[thick] (1,3)--(5,3) -- (5,1) -- (1,1) -- (1,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,1) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};
			\draw (2.5,3.7) node {\large \textbf{$S_{4}$}};


			

			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,4.5) -- ( .5,0.5) ;
			\draw[dotted] (.25,4.5) -- ( .25,0.25) ;
			
			\draw[dotted] (0.25,.5) -- ( 6,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0.5) ;
			\draw[dotted] (5.75,4.5) -- ( 5.75,0.5) ;

			
			\draw[dotted] (0.5,3.25) -- (5.5,3.25) ;
				
		
		\end{tikzpicture}}
		\caption{Guillotine cuts parallel to the orientation of subcorridors}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.3cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,5) -- (1,1) -- (7,1) -- (7,5) --(1,5);
			\draw[thick] (2,4)--(6,4)-- (6,2) -- (2,2) -- (2,4) ;
			\draw[thick]  (1.5,1.5) -- (1.5,6) ;% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[thick] (6.5,4.5)--(1.5,4.5);
			\draw[pattern=north east lines, pattern color=black] (6.5,4.5)--(6.5,5)--(1.5,5)--(1.5,4.5)--(6.5,4.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,5) -- (1.5,5) -- (1.5,1.5) -- (6.5,1.5) -- (6.5,5) --(7,5) -- (7,1)--(1,1)--(1,5);		

			\draw (4,1.25) node {\large \textbf{$U'$}};
			\draw (5,4.75) node {\large \textbf{$C$}};
			\draw (4,3) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Separating out a ring corridor which is then partitioned into $U'$,$C'$}
	\end{subfigure}
	\caption{Creating Bounding Box of $S$}
	\label{ringproc}
\end{figure}

%%%% Algo 3
\subsubsection{Algo-Box-Creation(C)}

\noindent Using the function Algo-Box-Creation($C$), we bound a corridor $C$ ($b(C)>0$) using a bounding box which is guillotine separable (see Algorithm \ref{boxalgo} for more details). We use Algo-separate(.) to extract items from $C$. During this if we extracted at least one rectangle from each corridor in $C$ then we bound the remaining portion of corridor $C$ using the edges of the subpiece which contains it. Clearly the bounding box created is guillotine separable. If we are not able to bound $C$, it implies that we get a cut of type $C_b$ or $C_u$ in $C$. Then divide the corridor $C$ into corridors of smaller number of bends and then bound the corridors with smaller number of bends (should be non-zero)  using guillotine separable boxes by recursively calling the function Algo-Box-Creation(.).\\
\\
{\em Technical Details of Algorithm \ref{boxalgo}:}  If the function Algo-separate(.) halts due to the presence of cut $l$ of type $C_b$ or $C_u$ in $C$, then such cuts are $O_{\eps,\epsl}(1)$ in number and each such cut leads to the creation of  $O_{\eps,\epsl}(1)$ corridors. If the function Algo-separate(.) halts due to the fact that one rectangle is obtained from each subcorridor in $C$, then we are creating O(1) extra corridors of lesser number of bends than $C$ and bounding a part of $C$ with a box. See Algorithm \ref{boxalgo} for the exact procedure on how we are doing this. So the function Algo-Box-Creation(.) recursively calls itself at most $O_{\epsl,\eps}(1)$ times which leads to the creation of  $O_{\epsl,\eps}(1)$ boxes which bound the  $O_{\epsl,\eps}(1)$ corridors. Algorithm \ref{boxalgo} is depicted in Figures \ref{ringproc}, \ref{figtwobends}, \ref{figthreebends}, \ref{figthreebends1}.

%algo4
\begin{algorithm}
\caption{Algo-Box-Creation($C$)}\label{boxalgo}
\begin{algorithmic}[1]
\STATE Let $c$ be the number of subcorridors in $C$. 
\STATE Call Algo-separate($C$, {\em all subcorridors in $C$}, {\em \{ at least one rectangle obtained from \\each subcorridor in $C$, presence of cut $l$ of type $C_b$ or $C_u$ in $C$ \}}, {\em Ordinary}).\label {st1abc}
\STATE Let {\em halting condition} denotes the reason why Algo-separate(.) halted. %\\was halted in the previous step. 
 \IF {({\em halting condition} is {\em at least one rectangle obtained from each subcorridor in $C$})\\}
\STATE	Create a bounding box using the edges of the subpiece which contains the \\ portion of $C$ excluding $C'$ when at least one rectangle from each corridor \\ of $C$ was separated out into $C'$ in Step \ref{st1abc}.
\STATE Let $S_{i}$ be the last subcorridor from which a rectangle was separated in Step \ref{st1abc}.\\ Make $S_{i}'=S_{i}\cap C'$ as a $\Bc$-corridor.\\ Let the corridor formed due to $S_{1}', \dots, S_{i-1}'$ be $C_{1}$ if $i>1$.\\ Let the corridor formed due to $S_{i+1}', \dots, S_{c}'$ be $C_{2}$ if $i<c$.
\IF{$i >2$} 
\STATE Call Algo-Box-Creation($C_{1}$).
\ENDIF 
\IF{$i<c-1$}
\STATE Call Algo-Box-Creation($C_{2}$).
\ENDIF
\ENDIF
\IF{({\em halting condition} is  {\em  presence of cut $l$ of type $C_b$ or $C_u$ in $C$})}
\STATE Partition the existing corridors into smaller corridors using the cut $l$.
\STATE Call  Algo-Box-Creation($C''$) for all corridor $C''$ created from $C$ after \\cut $l$ except the $\Bc$-corridors, if any.   
\ENDIF		 
\end{algorithmic}
\end{algorithm}

\subsubsection{Algo-Process($\mathcal{B},C$)}


\noindent Using the function Algo-Process($\mathcal{B},C$), we create boundary corridor in the box $\mathcal{B}$ with an additional property that the rectangles in the boundary corridor that are being created can be separated out using cuts of type $C_p$ (See Algorithm \ref{balgo} for more details). The function Algo-Process($\mathcal{B},C$) takes a part of corridor $C$ and extends it by including rectangles from other corridors to create a boundary corridor (whose items can be separated by cuts of type $C_p$). The basic procedure involves extracting rectangles (including those rectangles which are part of other corridors) using the cuts in $C$ of  type $C_p$ by calling Algo-separate(.) . The extracted rectangles form a part of the boundary corridor. Now consider the region $R$ which doesn't contain the boundary corridor which we extracted using the function Algo-separate(.). Let the next stage of cuts in $R$ be horizontal. The horizontal strips (similarly vertical) which are separated using a cut which isn't of type $C_p$ (w.r.t $C$) by appropriately shifting are merged into our boundary corridor . Note that we merge these horizontal strips if the height of the strip is at most $\epsl N$ which would ensure that all the rectangles in it are horizontal. Merging of horizontal strip in this way ensures that other corridors which are bounded by $\mathcal{B}$ get  automatically incorporated in our boundary corridor. If we get 2 horizontal strips with heights more than $\epsl N$ then there is a chance that these strips can contain a vertical rectangle and hence we divide the region $R$ into at most 3 parts and repeat our procedure on each such part. See Algorithm \ref{balgo} for the exact process.\\
\\
{\em Technical Details of Algorithm \ref{balgo}:} If the box $\mathcal{B}$ bounds more than one corridor of type either $\Lc,\Uc$ or $\Gc$, then by arbitrarily choosing one corridor and calling the function Algo-Process($\mathcal{B},C$) would merge some rectangles from other corridors (including some rectangles from $\Bc$-corridors) into boundary corridor that is being created (which happens when the condition $d_1\leq\epsl N$ or $d_2\leq\epsl N$ holds true)  and  the merging is stopped, if both the conditions $d_1>\epsl N$ and $d_2 >\epsl N$ holds true. At most 3 new boundary corridors are created each time both the conditions $d_1>\epsl N$ and $d_2 >\epsl N$ holds true, which can happen at most $O_{\epsl}(1)$ times in a given knapsack as the at least one of the dimension of in the new boxes decreases by at least $\epsl N$. Algorithm \ref{balgo} is depicted in Figure \ref{fig:c43}.

\begin{algorithm}
\caption{Algo-Process($\mathcal{B},C$)}\label{balgo}
\begin{algorithmic}[1]

\STATE Box $\mathcal{B}$ bounds  corridor $C$.
\STATE Consider other smaller boxes inside the $\mathcal{B}$ as  pseudoitems so that the \\guillotine cuts do not pass through it.
\STATE Algo-separate($C$, {\em every subcorridor of $C$}, \{{\em presence of cut $l$ of type $C_b$ or $C_u$ in $C$\\ or does not pass through $C$} \}, {\em Boundary}).\label{stepcreate}
\STATE Let $R$ be the rectangular region in $\mathcal{B}$ which does not contain the boundary \\corridor obtained from Step \ref{stepcreate}.
\STATE Let us assume that there is a horizontal subcorridor in the boundary corridor \\created in the Step \ref{stepcreate} which is below $R$.
\STATE Let us assume that the next stage cuts in $R$ be horizontal (similar steps if it was vertical). Let cut $l_{1}$ (resp., $l_2$) be topmost (resp., bottommost) horizontal cut in $R$ .\\ Let $l_1$ be at a distance of $d_1$ (resp., $d_2$) from the top (resp., bottom) edge in $R$.
\STATE Divide $R$ into three boxes $\mathcal{B}_{1},\mathcal{B}_{2},\mathcal{B}_{3}$ using the cuts $l_1,l_2$ where $\mathcal{B}_{2}$ is below $\mathcal{B}_{1}$\\ and $\mathcal{B}_{3}$ is below $\mathcal{B}_{2}$.
\IF{($d_2 \le \epsl N$)}
\STATE Let $\mathcal{B}_{5}$ be a box such that $\mathcal{B}_{5}=\mathcal{B}_{1}\cup \mathcal{B}_{2}$.
\STATE Merge $\mathcal{B}_{3}$ with the boundary corridor created in Step \ref{stepcreate}. \label{stpc11}
\STATE Call Algo-Process($\mathcal{B}_{5},C'$), if $\mathcal{B}_{5}$ bounds a corridor $C'$ and $b(C')>0$. \label{stpb5}
\STATE Merge the boundary corridor of $\mathcal{B}_{5}$ created in the Step \ref{stpb5} with the boundary \\corridor of $\mathcal{B}$ created in Step \ref{stpc11}.
\ELSIF{($d_1 \le \epsl N$)}
\STATE Let $\mathcal{B}_{4}$ be a box such that $\mathcal{B}_{4}=\mathcal{B}_{2}\cup \mathcal{B}_{3}$.
\STATE Remove $\mathcal{B}_{1}$ and push the box $\mathcal{B}_{4}$ upwards by a distance $d_1$.
\STATE Place $\mathcal{B}_{1}$ in the empty space created in $R$ due to movement of $\mathcal{B}_{4}$.
\STATE Merge $\mathcal{B}_{1}$ with the boundary corridor created in Step \ref{stepcreate}. \label{stpc1}
\STATE Call Algo-Process($\mathcal{B}_{4},C'$), if $\mathcal{B}_{4}$ bounds a corridor $C'$ and $b(C')>0$.\label{stpb4}
\STATE Merge the boundary corridor of $\mathcal{B}_{4}$ created in the Step \ref{stpb4} with the boundary \\corridor of $\mathcal{B}$ created in Step \ref{stpc1}.
\ELSIF {($d_1> \epsl N$ and $d_2> \epsl N$)}
\STATE Call Algo-Process($\mathcal{B}_{i},C'$), if $\mathcal{B}_{i}$ bounds a corridor $C'$ and $b(C')>0$ for $i \in [3]$. 
%\STATE  Call Algo-Process($\mathcal{B}_{2},C'$), if $\mathcal{B}_{2}$ bounds a corridor $C'$ and $b(C')>0$.
%\STATE  Call Algo-Process($\mathcal{B}_{3},C'$), if $\mathcal{B}_{3}$ bounds a corridor $C'$ and $b(C')>0$.
\ENDIF
\STATE Return Boundary Corridor of $\mathcal{B}$.
\end{algorithmic}
\end{algorithm}


%%%%%%%%%%%

\subsubsection{Algo-Boundary-L($\mathcal{B},C$)}
\noindent Using the function Algo-Boundary-L($\mathcal{B},C$), in the box $\mathcal{B}$, we convert a boundary corridor $C$ (whose items can be separated out using the cuts of type $C_p$) into boundary-$\Lc$ (whose items can be separated out using the cuts of type $C_p$). See Algorithm \ref{Lalgo} for the exact procedure.
%%%%%%%%%
\begin{algorithm}
\caption{Algo-Boundary-L($\mathcal{B},C$)}\label{Lalgo}
\begin{algorithmic}[1]
\STATE Consider the rectangular region $R$ in the box $\mathcal{B}$ which does not contain the \\boundary corridor $C$. Consider $R$ as a pseudoitem and remove it from $\mathcal{B}$.
\STATE Consider the first stage of guillotine cuts passing through some corridors of $C$ \\and having the same orientation as the subcorridor.
\IF {(First stage cuts  are vertical)}
\IF {(there is a vertical subcorridor $S_{i}$ of $C$ which touches the left edge of $\mathcal{B}$ \\such that there is a first-stage vertical cut $l$ through $S_{i}$)}
\STATE Let $l$ divide $\mathcal{B}$ into 2 regions $\mathcal{B}_{1}$ and $\mathcal{B}_{2}$ such that $\mathcal{B}_{1}$ is left of $\mathcal{B}_{2}$. 
\STATE Call Algo-Boundary-L($\mathcal{B}_{2},C'$) where $C'$ is that portion of corridor $C$ which \\doesn't contain items from $\mathcal{B}_{1}$, and $\mathcal{B}_{2}$ has at least one rectangle in it.\label{stp12}
\STATE Merge the boundary-$\Lc$ from Step \ref{stp12} with $\mathcal{B}_{1}$ to create the boundary-$\Lc$ of $\mathcal{B}$. 
\ELSIF {(there is vertical subcorridor $S_{i}$ of $C$ which touches the right edge of \\$\mathcal{B}$ such that there is a first-stage vertical cut $l$ through $S_{i}$)}
\STATE Let $l$ divide $\mathcal{B}$ into 2 regions $\mathcal{B}_{1}$ and $\mathcal{B}_{2}$ such that $\mathcal{B}_{1}$ is left of $\mathcal{B}_{2}$.
\STATE Remove $\mathcal{B}_{2}$ and push $\mathcal{B}_{1}$ to the right until it touches the right edge of $\mathcal{B}$.
\STATE Place $\mathcal{B}_{2}$ to the left of $\mathcal{B}_{1}$. 
\STATE Call Algo-Boundary-L($\mathcal{B}_{1},C'$) where $C'$ is that portion of corridor $C$ which \\doesn't contain items from $\mathcal{B}_{2}$ and $\mathcal{B}_{1}$ has at least one  rectangle in it. \label{stp13}
\STATE Merge the boundary-$\Lc$ from Step \ref{stp13} with $\mathcal{B}_{2}$ to create the boundary-$\Lc$ of $\mathcal{B}$.
\ENDIF
\ELSIF{(First stage cuts  are horizontal)}
\STATE Do analogous procedure to obtain a boundary-$\Lc$ with its horizontal subcorridor \\touching the bottom edge of $\mathcal{B}$.
\ENDIF
\STATE Place $R$ in the empty region left in $\mathcal{B}$.   
\end{algorithmic}
\end{algorithm}


	\subsection{Guillotine property}
	\label{subs:guilp}
	The construction of boxes and shifting of rectangle does not disturb the guillotine property. Now we show that the processing which we do in Subsection \ref{prosec} doesn't disturb the guillotine property if it is done to boundary-$\Lc$ which we obtain in the previous section. W.l.o.g.~assume that we are processing (as done in Subsection \ref{prosec}) a vertical subcorridor of the boundary-$\Lc$ which is placed top-left with respect to horizontal subcorridor. Note that this processing does not create any conflict in terms of guillotine separability with elements in boxes and $\Bc$-corridors outside the box bounding this boundary-$\Lc$ since by construction the boxes and $\Bc$-corridors are guillotine separable when considered as a pseudorectangle. Also the way in which we have constructed the boundary-$\Lc$, we always have a sequence of vertical (resp., horizontal) cuts through the vertical (resp., horizontal) subcorridor of boundary-$\Lc$ which separates the rectangles in the vertical (resp., horizontal) subcorridor. This ensures that as long we can separate out the items in the boundary-$\Lc$ from the rest of box using cuts which do not pass through the rest of the box, then the items in the rest of box can be separated as we have not changed their orientation. Now we need to focus on the boundary curve of the $\Lc$-corridor. Consider the strip containing the thin items. Let the length of the shorter vertical edge be $l$. Now the vertical strip which replaces this strip has rectangles of length at most $l$. So the horizontal rectangles which interacted with the thin items can be directly separated as there is no vertical rectangle intercepting the cut. Similar analogy for other strips shows that there is no conflict with horizontal rectangles. So we can conclude that the processing in Subsection \ref{prosec} does not disturb guillotine property.
	


==> 4A_Structural_Property_backup.tex <==
\subsection{Obtaining corridors with at most 2 bends}
\label{sub:bldec}

	\begin{lem} \label{structure}
	Given an optimal guillotine packing of $\R$ rectangles and the rectangles are either horizontal or vertical, we can partition the knapsack into $O_{\eps}(1)$  L corridors and $O_{\eps}(1)$ $\Bc$-corridors and place $\R' \subseteq \R$ rectangles in these corridors and $\Bc$-corridors such that:
	\begin{enumerate}
	\item$\profit(\R') \geq (1-O(\eps))\profit(\R)$ provided we can drop $O_{\eps}(1)$ rectangles without loosing any profit
	\item Each $\Bc$-corridor or subcorridor contains only one type of rectangle(i.e, either horizontal or vertical)
	\item Each rectangle is guillotine separable
	\item Each L corridor is a boundary $\Lc$ for a rectangular box.
         \item Rectangular boxes (which bound the items in $\Lc$ corridors ) when considered as a pseudorectangle are guillotine separable and number of such boxes is $O_{\eps,\epsl}(1)$
         \item Each $\Bc$-corridor when considered as a pseudorectangle are guillotine separable and the number of such corridors is $O_{\eps,\epsl}(1)$.
     	\end{enumerate}
	\end{lem}
\begin{proof}
	Given an optimal guillotine packing $\R$ (these rectangles are skewed) and using lemma \ref{lem:corridorPack} and Theorem \ref{3max} we  partition the knapsack into $O_{\eps}(1)$ corridors with no Z bends and the number of bends is at most 3. Also the packing $\R'$ is guillotine separable and $\profit(\R') \geq (1-O(\eps))\profit(\R)$. We now provide a construction of finding the rectangular box for each type of corridor with at least one bend such that the corridor is at the boundary of the box and the box is guillotine separable. For the remainder of the section we assume that a given corridor $S$  can't be divided into smaller corridors with cuts perpendicular to the orientation of any subcorridor. If there were such corridors then we can divide our corridor into smaller corridor and $O(\frac{1}{\epsl})$ $\Bc$-corridors which are obtained by these perpendicular cuts \end{proof}. In the following subsections we show a construction of boxes
\begin{obs} \label{endtoend}
Given a piece containing a set of guillotine separable rectangles, there must exist an end-to-end guillotine cut in the piece. In other words, the first level of guillotine cuts in the piece is end-to-end.
\end{obs}
We follow some terminologies in the remainder of the section. We define subpiece $P$ completely containing corridor $C$ as \textit{smallest} iff the piece $P$ which is obtained from the sequence of guillotine cuts has no previous cut that passed through the corridor $C$ and the next end to end cut in $P$ passes through $C$. We also define \textit{box $B$ bounding} a set of rectangles as a subpiece which is guillotine separable from the rest of the piece. In other ways $B$ if considered as a pseudorectangle, forms a guillotine separable arrangement with the rest of the items of knapsack. In the rest of the section, by freezing a rectangle, we mean that the rectangle is not moved while shifting other rectangles. A subcorridor $S_{1}$ is said to be exhausted if there is no rectangle from $S_{1}$ in the smaller subpiece on which we would running our recursive procedure in the following section. A box $B$ is said to be bounding a corridor with at least one bend if the outermost corners at the bends of the corridor coincides with the corners of the box. Now in the following section we provide a construction of boxes and $\Bc$-corridors which satisfy Lemma \ref{structure}.
	\subsubsection{$\Lc$ corridor}\label{L corridor}
	%Consider a L corridor $S$ with vertical subcorridor placed top left with respect to the horizontal subcorridor.W.l.o.g let us assume that the corridor $S$ can't be divided into smaller corridors with cuts perpendicular to subcorridor. Let us denote the line along the rightmost edge of horizontal subcorridor by $\Lc$. Consider the 2 left most vertical guillotine cuts in the vertical subcorridor of $S$ during the actual guillotine cutting sequence. If leftmost cut is intercepted by a rectangle $R_{1}$ which is above $S$ and the other cut is not intercepted by any rectangle which isn't completely above $R_{1}$ then there should exist a guillotine either top or bottom of the rectangle $R_{1}$ which crosses the line $\Lc$. Suppose there is no such cut and w.l.o.g let us assume that rectangle $R_{2}$ above $R_{1}$ which intercepts the second leftmost cut has a guillotine cut above it which crosses $\Lc$. But this situation is not possible as the set of rectangles in L corridor, rectangles which intercept the guillotine cuts of $R_{1}$ and $R_{2}$ form a non-guillotine structure as there is no end to end cuts be it horizontal or vertical  which spans the entire length of the subcorridor of $S$. So W.l.o.g let us assume that the two left most guillotine are intercepted by a single rectangle or by a rectangle which next to each other and above $S$. Consider the rectangle with upper most interception among the two. Let it be $R_{3}$. Now there must exist a guillotine cut between $R_{3}$ and the top most edge $e_{1}$ of vertical subcorridor of $S$ which crosses the line $\Lc$ and the leftmost guillotine cut. Suppose not then all the rectangles intercepting the guillotine cuts between $R_{3}$ and $e_{1}$, $R_{3}$ and the set of rectangles in the L corridor form a non-guillotine structure  as there is no end to end cuts be it horizontal or vertical which spans the entire length of the subcorridor of $S$. Now consider the lower most such guillotine cut which crosses line $\Lc$.Let this be $l_{1}$. Then by similar analogy we must have a guillotine cut to the right of horizontal subcorridor of $S$ which crosses $l_{1}$ and is parallel to $\Lc$. Hence we have constructed a box which is guillotine separable and has $S$ as it's boundary L.\\

Consider a $\Lc$ corridor $S$. W.l.o.g.~we can assume that vertical subcorridor $S_{1}$ of $S$ is placed to the top left w.r.t the horizontal subcorridor $S_{2}$. We consider the smallest subpiece $P$ containing $S$.
% Three cases might exist. Case 1: If left boundary of vertical subcorridor of S coincides with the left boundary of P, we have found the left boundary of bounding box. We then consider the sequence  If bottom boundary of horizontal subcorridor of S coincides with the bottom boundary of P, we have found the bottom boundary of bounding box. %
Next consider the first stage guillotine cuts in the $P$. W.l.o.g.~let the first stage cuts be vertical.
Then we have the following cuts which can occur to a $\Lc$ corridor during the recursive procedure to bound the $\Lc$ corridor which we are going to describe later:
\begin{itemize}
\item Cut 1:Rightmost vertical Guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$
\item Cut 2:Horizontal Guillotine cut passing through $S_{1}$ and not through the interior of $S_{12}$
\item Cut 3: Horizontal Guillotine cut passing through $S_{2}$
\item Cut 4:  Cut which doesn't pass through $\Lc$ corridor.
\end{itemize}
Now we describe the recursive procedure. According to our assumption we begin with Cut 1. If we have Cut 1 then make a $\Bc$-corridor out of the rectangles separated from $\Lc$ corridor in our subpiece and consider the right subpiece to be the new subpiece. Merge all the $\Bc$-corridors obtained due to Cut 1 provided that these cuts occurred before the first cut 2. For the rest of cuts which are of type cut 1 make a corridor for rectangles separated by these cuts. If we have Cut 2 then make a $\Bc$-corridor out of the rectangles separated from $\Lc$ corridor in our subpiece and consider the bottom subpiece to be the new subpiece.
We stop the recursive procedure if either $S_{1}$ has exhausted or we obtain cut 2. If we obtain a cut 2 then we clearly have a bounding box with the edges being cut 1,cut 2 and the top and the right edges of the smaller subpiece $P'$ we are in after the last step of the recursive procedure. In the whole procedure we obtain only $O(\frac{1}{\epsl})$ extra $\Bc$-corridors. 
	\subsubsection{$\Uc$-corrdor}\label{twobends}
	%Consider a corridor $S$ with 2 bends such that 2 vertical subcorridors $S_{1},S_{3}$ placed on the top of the horizontal subcorridor $S_{2}$.W.l.o.g let us assume that the corridor $S$ can't be divided into smaller corridors with cuts perpendicular to subcorridor.Consider the 2 left most vertical guillotine cuts in the leftmost vertical subcorridor $S_{1}$ of $S$ during the actual guillotine cutting sequence. W.l.o.g let us assume that the two left most are intercepted by a single rectangle or by a rectangle which next to each other and above $S$. Consider the rectangle with upper most interception among the two. Let it be $R_{3}$. We denote the line along the rightmost edge of rightmost vertical subcorridor $S_{3}$ by $\Lc$. Now there must exist a guillotine cut between $R_{3}$ and the top most edge $e_{1}$ of vertical subcorridor of $S$ which crosses the line $\Lc$ and the leftmost guillotine cut. Suppose not then all the rectangles intercepting the guillotine cuts between $R_{3}$ and $e_{1}$, $R_{3}$ and the set of rectangles in the corridor $S$ form a non-guillotine structure as there is no end to end cuts be it horizontal or vertical  which spans the entire length of the subcorridor of $S$. Now consider the lower most such guillotine cut which crosses line $\Lc$.Let this be $l_{1}$. There is no rectangle between $l_{1}$ and topmost edge of the rightmost vertical subcorridor such that it intercepts line $\Lc$ otherwise the set of rectangle below line $l_{1}$ form a non-guillotine structure. Hence we have a box which is guillotine separable such that the corridor is along the boundary of the box. Now consider the corridor with 2 bends. By appropriate shifting of vertical rectangles we can convert it into a L corridor without disturbing the guillotine property. Exact details are available in subsubsection \ref{sss2}.\\
Let $S$ be a corridor with $2$ bends. Let the top left vertical, horizontal and top right vertical subcorridors of $S$ be $S_{1}$, $S_{2}$ and $S_{3}$ respectively as shown in Figure \ref{figtwobends}. Consider the smallest subpiece $P$ containing $S$. We define three types of end-to-end cuts possible in $P$ or in any of the subpieces formed by a sequence of cuts in $P$.The rightmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$ is termed as \textit{Type $1$}. The leftmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{3}$ is termed as \textit{Type $3$}. The topmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{2}$ is termed as \textit{Type $2$}. Figure \ref{figtwobends} shows all the three types of cuts defined. We then follow a recursive approach to define bounding box using the cuts in guillotine cutting sequence. Clearly, obtaining all three type of cuts, i.e., type $1,2,3$ will result in a bounding box where the box is bounded by these cuts and upper boundary of subpiece $P'$ containing a subset of items of $S$. Subpiece $P'$ is that subpiece which contains smaller corridor with 2 bends after we obtain the last of the three type cut.  \\
\\Basic idea follows dividing $S$ into  $O(\frac{1}{\epsl})$ corridors $\{L_{1},L_{2},...,L_{k}\}$ (with at most 1 bend) consisting of some items from $S_{1}$ ( w.l.og it can be $S_{3}$ but we assume for the remainder of the section that $S_{1}$ is the one contributing to $\Lc'$) and $S_{2}$,  $O(\frac{1}{\epsl})$ $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$ from a subset of items of $S_{3}$ and a corridor (with at most 2 bends) with the remaining set of items. Note that $C_{i+1}$ is left of $C_{i}$ and $C_{i+1}$ has height less than $C_{i}$. Similarly $L_{i+1}$ is place to the top right of $L_{i}$ and $L_{i+1}$ is smaller in size than $L_{i}$   \\
\\We now formally define the algorithm for processing corridor $S$ with $2$ bends. From observation \ref{endtoend} we know that the first cut in any guillotine separable piece is end-to-end. In the remainder of the subsection by closing a corridor or $\Bc$-corridor we mean that no more items will be packed in that corridor or $\Bc$-corridor. And, by opening a corridor  or $\Bc$-corridor we mean that we are allowed to pack rectangles in this corridor or $\Bc$-corridor only. Initially corridor $L_{1}$ is open  and $\Bc$-corridor $C_{1}$ is open. Depending on the type of this cut we do the following processing :
\begin{enumerate}
\item Scenario $1$:Let's assume that corridor $L_{i}$ and $\Bc$-corridor $C_{j}$ is open right now. If we have a horizontal cut through $S_{1}$ or $S_{3}$ but not through $S_{2}$ then we pack the items of $S_{1}$ above the cut in one $\Bc$-corridor and pack the items of $S_{3}$ above the cut in another $\Bc$-corridor. Then we continue our recursive procedure for the smaller portion of our original corridor present in the subpiece below this cut. If the horizontal cut passes through $S_{1}$ then we close $L_{i}$ and open $L_{i+1}$. Similarly if the horizontal cut passes through $S_{3}$ then we close $C_{j}$ and open $C_{j+1}$.    Such kind of cuts can have $O(\frac{1}{\epsl})$ number of occurrences as the larger dimension of any rectangle is at least $\epsl N$. So when the recursive procedure halts scenario 1 would be contributing at most $O(\frac{1}{\epsl})$ new $\Bc$-corridors. 
\item Scenario $2$ : (Type $1$ cut) Add the items of $S_{1}$ which is left of cut 1 to the vertical subcorridor of $L'$. Consider the new-subpiece to be the subpiece which is right of cut 1. Run algorithm recursively on the new-subpiece.
\item Scenario $3$ : (Type $2$ cut) Add the items of $S_{2}$ below the cut 2 to the horizontal subcorridor of $L'$. Consider the new-subpiece to be the top-subpiece. Run algorithm recursively on the new-subpiece.
\item  Scenario $4$ : (Type $3$ cut) Pack the items of $S_{3}$ which is right of cut 3 in a new vertical $\Bc$-corridor $C$. Consider the new-subpiece to be the subpiece which is right of cut 3. Run algorithm recursively on the new-subpiece.

\end{enumerate}
%The algorithm when run on subpiece $P$, considers one of the above three cases depending on the type of end-to-end cut, augments some items from $S_{1}$ or $S_{2}$ to $L'$ and runs again on the new subpiece. We halt at the iteration when at least one of each type of cut is obtained. The boundaries of subpiece at this step along with the cut considered define the bouding box for remaing set of items of $S$. Thus we get a box surrounded by $L'$ on two edges (left and bottom) and a corridor on the third (right). The fourth (top) edge of box is trivially defined by top edge of $P$\\It is clear that number of new corridors is 2, i.e., one L-corridor and one $\Bc$-corridor. Since we follow the original sequence of guillotine cuts without moving any items, guillotine separability is not disturbed.

We halt if one of the following three cases happens. First case occurs if at some iteration at least one cut from each type of cut is obtained. The boundaries of subpiece at this step along with the cut considered define the bounding box for remaining set of items of $S$. Thus we get a box surrounded by corridors $\{L_{1},L_{2},...,L_{k}\}$ and $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$ . Figure \ref{figtwobends} shows final bounding box $B$ formed after the algorithm alongwith $L_{1}$ formed after considering sequence of type $1$ and type $2$ cuts in subcorridors $S_{1}$, $S_{2}$ and the $\Bc$-corridor $C_{1}$ formed from type $3$ cuts in $S_{3}$. Second case occurs if one or more subcorridors in the piece exhausts i.e. all the items of these subcorridors are already packed in corridors $\{L_{1},L_{2},...,L_{k}\}$ or in $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$. In this case we are left with at most 2 corridors with at most 1 bend who rectangles are not part of the $\Bc$-corridors or corridors created during the recursive procedure. We can use the previous section results to bound this corridor with the a box (Except for a $\Bc$-corridor which will be dealt in the later subsections). Third Case occurs when the next guillotine cut in the sequence is vertical and passes through subcorridor $S_{2}$ only. This leaves us with 2 corridors of at most 1 bend. So, we can use the previous section results to bound the corridors with the boxes (Except for a $\Bc$-corridor which will be dealt in the later subsections).\\
\\Now we observe that using the algorithm defined above we add only a $O(\frac{1}{\epsl})$ number of new corridors and $\Bc$-corridors. The proof follows from the fact that if it is the case that all algorithm halts when at least one of each type of cuts is obtained then in the end we have corridors  $\{L_{1},L_{2},...,L_{k}\}$ (with at most 1 bend) and $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$. This accounts to $O(\frac{1}{\epsl})$ new $\Bc$-corridors and corridors as new $\Bc$-corridor or corridor is created only when we have scenario 1 and as we have shown there the number of times this scenario occurs is $O(\frac{1}{\epsl})$. Else if it is the case that algorithm halts when one or more of subcorridors is exhausted, then also we have either corridors $\{L_{1},L_{2},...,L_{k}\}$ (with at most 1 bend) or we have $\Bc$-corridors $\{C_{1},C_{2},...,C_{l}\}$ and we have already shown that the number of such $\Bc$-corridors are $O(\frac{1}{\epsl})$. We then run the algorithm on remaining corridors which has lesser number of bends than $S$, i.e., at most 1 bend(if there is any such corridor). As it follows from section \ref{L corridor}, we get $O(\frac{1}{\epsl})$ corridors from processing in this case. For  the third type of halting due to vertical cuts which passes through $S_{2}$ only, we have already shown in the previous paragraph that we obtain only $O(\frac{1}{\epsl})$ new $\Bc$-corridors and corridors.


\begin{figure}[t]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,3) -- (0,0) -- (6,0) -- (6,4) -- ( 5,4) -- (5,1) -- (1,1) -- (1,3) -- (0,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,1.25) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};

			\draw (1,3.7) node {\large \textbf{Type 1}};
			\draw (6.7,.6) node {\large \textbf{Type 2}};
			\draw (6,4.7) node {\large \textbf{Type 3}};
		

			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,3.5) -- ( .5,0) ;
			\draw[dotted] (.25,3) -- ( .25,0) ;
			
			\draw[dotted] (0,.5) -- ( 6.2,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0) ;
			\draw[dotted] (5.25,4) -- ( 5.25,0) ;
				
		
		\end{tikzpicture}}
		\caption{Types of cuts}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,4) -- (1,1) -- (7,1) -- (7,5) -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick]  (1.5,6) -- (1.5,1.5) -- (7,1.5);% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[pattern=north east lines, pattern color=black] (6.5,1.5)--(6.5,5)--(7,5)--(7,1.5)--(6.5,1.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,4) -- (1.5,4) -- (1.5,1.5) -- (7,1.5) -- (7,1) --(1,1) -- (1,4);		

			\draw (1.25,1.25) node {\large \textbf{$L_{1}$}};
			\draw (6.75,2.5) node {\large \textbf{$C_{1}$}};
			\draw (4,4) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Final Bounding Box of $S$}
	\end{subfigure}
	\caption{Processing 2-bend corridor}
	\label{figtwobends}
\end{figure}
	\subsubsection{$\Gc$ Corridor}\label{threebends}
	%Consider a corridor $S$ with 3 bends.  W.l.o.g let us assume that the corridor $S$ can't be divided into smaller corridors with cuts perpendicular to subcorridor.Let us consider vertical subcorridors $S_{1}$ and $S_{3}$ which are on top of horizontal subcorridor $S_{2}$ and $S_{3}$ is right of $S_{1}$ and below horizontal subcorridor $S_{4}$. Now consider a corridor comprising of $S_{1},S_{2},S_{3}$ and assuming the w.l.o.g conditions of previous section we get a box for this triple. Similarly we get a box for the triple $S_{2},S_{3},S_{4}$ . Intersection of both the boxes gives us a box whose edges are the topmost,bottom most, leftmost and rightmost edges of the corridor $S$.  By appropriate shifting of vertical rectangles we can convert it into a L corridor without disturbing the guillotine property.Exact details are available in subsubsection \ref{sss3}.\\
The approach is similar to section \ref{twobends}. Let $S$ be a corridor with $3$ bends. Let the top left vertical, bottom horizontal, top right vertical subcorridors and top horizontal subcorridors of $S$ be $S_{1}$, $S_{2}$, $S_{3}$ and $S_{4}$ respectively as shown in Figure \ref{figthreebends}. Consider the smallest subpiece $P$ containing $S$. We define four types of end-to-end cuts possible in $P$ or in any of the subpieces formed by a sequence of cuts in $P$. The rightmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$ is termed as Type $1$. The leftmost end-to-end guillotine cut passing during a single stage of guillotine cutting sequence through $S_{3}$ is termed as Type $3$. The topmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{2}$ is termed as Type $2$. The bottommost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{4}$ is termed as Type $4$. Figure \ref{figthreebends} shows all the four types of cuts defined.
\\Basic idea follows divinding $S$ into a corridor $U'$ (with at most $2$ bends) consisting of some items from $S_{1}$, $S_{2}$, $S_{3}$ ( w.l.og it can be $S_{2}$, $S_{3}$, $S_{4}$ but for the rest of the proof we assume that it's the former case not the latter), a $\Bc$-corridor $C$ from a subset of items of $S_{4}$ and a corridor (with at most 3 bends) with the remaining set of items. We follow a recursive approach to define bounding box $B$. Clearly,  obtaining all four type of cuts will result in a box  bounded by these cuts. \\
We now formally define the algorithm for processing corridor $S$ with $3$ bends. From observation \ref{endtoend} we know that the first cut in any guillotine separable piece is end-to-end. Depending on the type of this cut we do the following processing :
\begin{enumerate}
\item Scenario $1$ : (Type $1$ cut) Add the items of $S_{1}$ which is left of Cut 1 to the left-vertical subcorridor of the 3-bend corridor $U'$. Consider the new-subpiece to be the subpiece which is right of Cut 1. Run algorithm recursively on the new-subpiece.
\item Scenario $2$ : (Type $2$ cut) Add the items of $S_{2}$ which is below Cut 2 to the horizontal subcorridor of $U'$. Consider the new-subpiece to be subpiece which is above Cut 2. Run algorithm recursively on the new-subpiece.
\item Scenario $3$ : (Type $3$ cut) Add the items of $S_{3}$ which is right of Cut 3  to the right-vertical subcorridor of $U'$. Consider the new-subpiece to be the subpiece which is left of Cut 3. Run algorithm recursively on the new-subpiece.
\item  Scenario $4$ : (Type $4$ cut) Pack the items of $S_{4}$ which is above Cut 4 in a new horizontal $\Bc$-corridor $C$. Consider the new-subpiece to be the subpiece which is below Cut 4. Run algorithm recursively on the new-subpiece.
\end{enumerate}
 We halt if one of the following three cases happens. First case occurs if at some iteration at least one cut from each type of cut is obtained. The boundaries of subpiece at this step along with the cut considered define the bounding box for remaining set of items of $S$. Thus we get the box $B$ surrounded by $U'$ on three edges and a $\Bc$-corridor $C$ on the fourth. Figure \ref{figthreebends} shows final bounding box $B$ formed after the algorithm alongwith $U'$ formed after considering sequence of type $1$ ,type $2$ and type $3$ cuts in subcorridors $S_{1}$, $S_{2}$, $S_{3}$ and the $\Bc$-corridor formed from type $4$ cuts in $S_{4}$. Second case occurs if one or more of the subcorridors in the piece exhausts, i.e., all the items of subcorridor are already packed in $U'$ or in $C$. In this case we are left with at most 2 corridors with at most 2 bends whose items are not part of either $U'$ or $C$. Using the previous section we get that the corridor with at most two bends is bounded by a box (Except for a $\Bc$-corridor which will be dealt in the later subsections) . Third Case occurs when the next guillotine cut in the guillotine cutting sequence passes completely through any subcorridor perpendicular to its longer sides. This divides $S$ into at most three corridors with at most 2 bends each. Using the previous section results each corridor with at most two bends is bounded by a box (Except for a $\Bc$-corridor which will be dealt in the later subsections) .\\
\\Now we observe that using the algorithm defined above we add only a $O(\frac{1}{\epsl})$ number of new corridors and $\Bc$-corridors. The proof follows from the fact that if it the case that all algorithm halts when at least one cut from each type of cuts is obtained then in the end we have a corridor ( with at most 3 bends) , a $\Bc$-corridor and a bounding box. This accounts to $O(1)$ new $\Bc$-corridors and corridors. Else if it is the case that algorithm halts when one or more of subcorridors is exhausted, i.e., packed in either $U'$ or $C$, then we have a new corridor (with at most 2 bends) or one new $\Bc$-corridor $C$. We then run the algorithm on remaining corridors which has lesser number of bends than $S$ i.e. at most 2 bends (Except for a $\Bc$-corridor which will be dealt in the later subsections) . As it follows from subsections \ref{twobends} and \ref{L corridor}, we get $O(\frac{1}{\epsl})$ corridors from processing in both the cases. In the third case of halting, $O(\frac{1}{\epsl})$ extra $\Bc$-corridors follows from the results of subsections \ref{twobends} and \ref{L corridor}.


\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,3) -- (0,0) -- (6,0) -- (6,4) --( 2,4)--(2,3)--(5,3) -- (5,1) -- (1,1) -- (1,3) -- (0,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,0.75) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};
                           \draw (3,3.5) node {\large \textbf{$S_{4}$}};

			\draw (1,3.7) node {\large \textbf{Type 1}};
			\draw (6.9,.45) node {\large \textbf{Type 2}};
			\draw (6,4.7) node {\large \textbf{Type 3}};
			\draw (6.9,3.2) node {\large \textbf{Type 4}};

			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,3.5) -- ( .5,0) ;
			\draw[dotted] (.25,3) -- ( .25,0) ;
			
			\draw[dotted] (0,.5) -- ( 6.5,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0) ;
			\draw[dotted] (5.25,4) -- ( 5.25,0) ;

			\draw[dotted] (2,3.5) -- ( 6,3.5) ;
			\draw[dotted] (2,3.25) -- ( 6.5,3.25) ;
				
		
		\end{tikzpicture}}
		\caption{Types of cuts}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,4) -- (1,1) -- (7,1) -- (7,5) -- ( 6,5) --(3,5)--(3,4)--(6,4)-- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick]  (1.5,1.5) -- (1.5,6) ;% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[thick] (6.5,4.5)--(1.5,4.5);
			\draw[pattern=north east lines, pattern color=black] (6.5,4.5)--(6.5,5)--(3,5)--(3,4.5)--(6.5,4.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,4) -- (1.5,4) -- (1.5,1.5) -- (6.5,1.5) -- (6.5,5) --(7,5) -- (7,1)--(1,1)--(1,4);		

			\draw (4,1.25) node {\large \textbf{$U'$}};
			\draw (5,4.75) node {\large \textbf{$C$}};
			\draw (4,3) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Final Bounding Box of $S$}
	\end{subfigure}
	\caption{Processing 3-bend corridor}
	\label{figthreebends}
\end{figure}
	\subsubsection{$\Bc$-Corridor}
	In this subsection we deal with the items inside a $\Bc$-corridor in 2 ways. In first way, the $\Bc$-corridors can be either divided into $O_{\eps,\epsl}(1)$ $\Bc$-corridors and the $\Bc$-corridors as a pseudo rectangle are guillotine separable. In second way, the items in $\Bc$-corridors is merged with a corridor and later become a part of boundary $\Lc$ . Given a knapsack, first we construct the boxes as mentioned in the previous subsections. Note that one box may lie completely inside another box. Now consider the set of outermost boxes which are not part of any other box in the original Knapsack. Note that the boundaries of outermost boxes may divide the corridors with zero bends into smaller parts. The number of such smaller parts is $O(\frac{1}{\epsl})$ as the guillotine cuts which are part of the boundary of a single box can divide a $\Bc$-corridor into at most 6 parts and number of such boxes is $O(\frac{1}{\epsl})$. Now we have to deal with 2 cases.\\
\\ In the first case, a $\Bc$-corridor say $S$ lies inside a box and if a part or the complete $\Bc$-corridor $S$ lies between the lines along the two longer edges of a subcorridor say $S_{1}$ of a boundary $\Lc$ and the orientation of the corridor is same as that of the subcorridor $S_{1}$. This case is appropriately handled in the subsubsection \ref{sssl} and we satisfy all the properties of the lemma \ref{structure}. Suppose instead that the longer edges of the rectangles in the $\Bc$-corridor $S$ was perpendicular to the longer edges of subcorridor $S_{1}$ of boundary $\Lc$ then this case is approriately handled in the subsubsection \ref{sssl} and we satisfy all the properties of the lemma \ref{structure}. Similar argument holds for corridors with 2 or 3 bends instead of $\Lc$ corridor and after all the similar processing as done in subsubsection \ref{sssl}  we convert them into a $\Lc$ corridor by appropriate shifting as mentioned in the subsubsections \ref{sss2} and \ref{sss3}.\\
\\Now in the second case the $\Bc$-corridors lie outside any box in the original knapsack. Now consider the set of guillotine cuts that separates the $\Bc$-corridors and the boxes. Note that the way we have constructed the outermost boxes the guillotine cuts don't pass through the boxes except its edges. Consider one $\Bc$-corridor $S_{1}$ and let its orientation be horizontal. Then we can divide into the following subcases based on the type of cut through $S_{1}$ and the interaction of the cuts with other cuts or rectangles:
\begin{itemize}
\item Subcase 1:  Now consider the horizontal cuts (which are not entirely inside the $\Bc$-corridor $S_{1}$) through $S_{1}$. If 3 or more horizontal cuts are intercepted by the same vertical cut in the guillotine cutting sequence then consider the topmost and the bottom cut as the cuts and ignore the rest. This subcase is depicted in Figure \ref{C01b}.
\item Subcase 2: Now consider set of vertical cuts which intercept the horizontal cuts through $S_{1}$. If these vertical cuts are edges of an outermost box which we created then there can be at most $O(\frac{1}{\epsl})$ of them. Now if these vertical cuts are edges of vertical rectangle which belonged to different corridors then these can be at most $O_{\eps}(1)$ of them. Both of the scenarios are depicted together in Figure \ref{C01c}.
\item Subcase 3:Supposed the rectangles which intercept the horizontal cuts through $S_{1}$ belonged to the same corridor $S_{2}$. Now assume 2 or more than 2 consecutive horizontal cuts dont have space more than $\epsl N$ between them (otherwise, the cuts are intercepted by at most $O_{\epsl}(1)$ rectangles) . Then we take that cut $l$ among the consecutive cuts such that $|l\bigcap S_{2}|$ is maximum and shift vertically those rectangles which intercepted these consecutive cuts other than $l$ and make them touch $l$. Hence we consider $l$ as valid guillotine cut and deal with the rest of the consecutive cuts using the Subcase 1. Subcase 3 is depicted in Figure \ref{C02a} and Figure \ref{C02b}.  
\item Subcase 4: Using the same techniques of Subcase 1 and 3 and applying it to the vertical cuts which pass through some vertical corridor $S_{3}$ with zero bends (repeat the same for other set of cuts which pass through the same vertical $\Bc$-corridor)  and are intercepted by the rectangles in $S_{2}$ we get that there can be at most $O(\frac{1}{\epsl})$ vertical cuts  (which are not entirely inside the $\Bc$-corridor $S_{1}$) passing through $S_{1}$ since width of each rectangle is at least $\epsl N$. This subcase is depicted in Figure \ref{C01a}.
\end{itemize}
Now we argue that at most $O(\frac{1}{\epsl})$ horizontal cuts (which are not entirely inside the $\Bc$-corridor $S_{1}$) pass through the $\Bc$-corridor $S_{1}$. Subcase 2 and Subcase 3 ensure that the number of vertical cuts which intercept the horizontal cuts passing through $S_{1}$ is $O_{\eps,\epsl}(1)$. And for each such vertical cut we end up keeping at most 2 horizontal cuts which pass through $S_{1}$ as explained in Subcase 1. Now these horizontal cuts along with the vertical cuts of Subcase 4 and vertical edges of $S_{1}$ results into partition of $S_{1}$ into $O_{\eps,\epsl}$ $\Bc$-corridors and these corridors when considered as a pseudo rectangle is guillotine separable
\\
\\ Now the procedure mentioned above is recursively applied to those portion of the outermost boxes which doesn't have items from its boundary $L$.  This process stops when there is no corridor with at least one bend which is not bounded by any box or there is no $\Bc$-corridor which when considered as a pseudo item isn't guillotine separable. Number of such boxes bounding the $\Lc$ corridor or items of a $\Bc$-corridor is $O_{\eps,\epsl}(1)$. This follows from constructive procedures in subsection \ref{ssss} and the fact that we started the section with $O_{\eps,\epsl}(1)$ $\Bc$-corridors and corridors.

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[t]{.3\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,8);
			\draw (1,4) rectangle (5,5);
			\draw[dotted] (0,4.3) -- ( 8,4.3) ;
			\draw[dotted] (0,4.6)--(8,4.6);
			\draw [dotted] (3,4.6)--(3,8);
			\draw [dotted] (2.3,4.3)--(2.3,0);
			\draw [dotted] (2,4)--(2,0);
			\draw[dotted] (2.5,4)--(2.5,0);
			\draw[dotted] (2.6,4)--(2.6,0);
			\draw[dotted] (2.7,4)--(2.7,0);			
			\draw[dotted](3.6,4.3)--(3.6,0);	
			\draw [dotted] (1,0)--(1,8);
			\draw [dotted] (5,0)--(5,8);
			
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{}\label{C01a}
	\end{subfigure}
	\begin{subfigure}[t]{.3\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			
			\draw (1,4) rectangle (5,6);
			\draw[solid,fill=lightgray] (7,3) rectangle (10,7);	
			\draw[dashed] (0,4.3) -- ( 7,4.3) ;
			\draw[dotted] (0,4.6)--(7,4.6);
			\draw[dotted] (0,4.9)--(7,4.9);
			\draw[dotted] (0,5.2)--(7,5.2);
			\draw[dotted] (0,5.5)--(7,5.5);
			\draw[dashed] (0,5.8)--(7,5.8);
			\draw[dotted](7,0)--(7,10);
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			\draw (8,5) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{ }\label{C01b}
	\end{subfigure}
	\begin{subfigure}[t]{.3\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			\draw (1,4) rectangle (5,6);
			\draw[solid,fill=lightgray] (6,5) rectangle (8,7);
			\draw[solid,fill=lightgray] (8.3,1) rectangle (9,5);	
			\draw[dotted] (0,4.6)--(8.3,4.6);
			\draw[dotted] (0,5.8)--(6,5.8);
			
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			\draw (8.6,3) node {\large \textbf{$C_{1}$}};
			\draw (7,6) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{}\label{C01c}
	\end{subfigure}
	
	\caption{Handling Corridors with 0 bends Part-1. Figure \ref{C01a} : Constant number of vertical cuts through a corridor $C$ which has horizontal orientation. Figure \ref{C01b} : We choose the topmost and bottommost horizontal cuts(shown as dashed lines in this figure ) if more than 3 horizontal cuts are intercepted by the same vertical cut as shown in this figure. Then these chosen cuts along with the portion of the boundary vertical edges of $C$ form the edges of a $\Bc$-corridor which is guillotine separable. Rest of the cuts which were not chosen is divided into 2 parts and pass through rectangles which are outside $C$. Figure \ref{C01c} : Horizontal cuts intercepted by different boxes or $\Bc$-corridors. }

\end{figure}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			
			\draw (1,4) rectangle (5,6);
			\draw[solid] (7,3) rectangle (10,7);	
			\draw[dotted] (0,4.3) -- ( 7.3,4.3) ;
			\draw[dotted] (0,4.6)--(7.6,4.6);
			
			\draw[dashed] (0,5.2)--(7.9,5.2);
			\draw[dotted] (0,5.5)--(7.6,5.5);
			\draw[dotted] (0,5.8)--(7.3,5.8);
			\draw[solid,fill=lightgray] (7.3,5.7) rectangle (7.5,6.8);
			\draw[solid,fill=lightgray] (7.6,5.4) rectangle (7.8,6.5);
			\draw[solid,fill=lightgray] (7.9,4) rectangle (8.1,6.2);
			\draw[solid,fill=lightgray] (7.5,4.8) rectangle (7.7,3.7);
			\draw[solid,fill=lightgray] (7.2,4.5) rectangle (7.4,3.4);
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			\draw (9,5) node {\large \textbf{$C_{1}$}};
			\draw (6,5) node {\large \textbf{$l$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{ }\label{C02a}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			
			\draw (1,4) rectangle (5,6);
			\draw[solid] (7,3) rectangle (10,7);	
			\draw[dotted] (0,4.3) -- ( 7.3,4.3) ;
			\draw[dotted] (0,4.6)--(7.3,4.6);
			
			\draw[dashed] (0,5.2)--(7.9,5.2);
			\draw[dotted] (0,5.5)--(7.3,5.5);
			\draw[dotted] (0,5.8)--(7.3,5.8);
			\draw[solid,fill=lightgray] (7.3,5.2) rectangle (7.5,6.3);
			\draw[solid,fill=lightgray] (7.6,5.2) rectangle (7.8,6.3);
			\draw[solid,fill=lightgray] (7.9,4) rectangle (8.1,6.2);
			\draw[solid,fill=lightgray] (7.5,5.2) rectangle (7.7,4.1);
			\draw[solid,fill=lightgray] (7.2,5.2) rectangle (7.4,4.1);
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			\draw (9,5) node {\large \textbf{$C_{1}$}};
			\draw (6,5) node {\large \textbf{$l$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{}\label{C02b}
	\end{subfigure}

	\caption{Handling Corridors with 0 bends Part-2. Figure \ref{C02a} : Horizontal cuts are intercepted by vertical rectangles belonging to same $\Bc$-corridor. Identify the horizontal cut $l$ (dashed line in this figure)which has maximum intrusion into corridor $C_{1}$. Figure \ref{C02b} : Then shift all the rectangles which are intercepting other cuts which are under consideration so that it touches cut $l$. Cuts other than $l$ are bow divided into 2 group and are now dealt in the same way as we dealt the cuts intercepted by same vertical cut.}

\end{figure}

	\subsection{Shifting Procedure}\label{ssss}
	In this subsection by boundary corridor we mean that the corridor is bounded by a box which is obtained by the recursive procedure in the subsection  \ref{L corridor}, \ref{twobends}, \ref{threebends}. Also we assume that the cuts which we are considering in a box $B$ don't pass through the smaller boxes inside $B$ except through its edges.
\subsubsection{Handling rectangles or $\Bc$-corridors interacting with a boundary $\Lc$ corridor}\label{sssl}
	Consider a boundary $\Lc$ corridor $S$ with vertical subcorridor $S_{1}$ placed top left with respect to the horizontal subcorridor $S_{2}$. Now consider a sequence of guillotine cuts (cut is parallel to the orientation of the subcorridor and the rectangles which are being separated in that subcorridor) which separates the rectangles in the boundary $\Lc$. Continue this process till there doesn't exist any such cut. Either we have separated all the rectangles of a subcorridor of boundary $\Lc$ or still we have a portion of the boundary $\Lc$ left. In the former case we fix the rectangles which got separated due to guillotine cuts as the boundary $\Lc$ of the original box. In the later case w.l.o.g.~let the next stage of cuts be horizontal and these cuts passes though $S_{1}$ only . Now consider the lowermost cut among these horizontal cut. Let it be $l$. Let $l$ be at a distance of $h$ from the top of the box. If $h \leq \epsl N$,we remove the items in the strip above $l$, then we shift upwards the rectangles below the cut $l$ except those rectangles which got separated due to previous guillotine cuts by a distance of $h$ and then place the rectangles from the strip which we removed initially in the empty region created due to shifting. Otherwise, if $h > \epsl N$, then we consider the items separated due to cuts before $l$ as the boundary $\Lc$ of the original box and we divide the rest of region of the box into 2 smaller boxes with cut $l$ being the common edge between both the smaller boxes. Now that an original boundary $\Lc$ along with some $\Bc$-corridors gets divided into $O(\frac{1}{\epsl})$ smaller boundary $\Lc$. The reason being that a boundary $\Lc$ and some $\Bc$-corridors get divided into smaller boundary $\Lc$ only if the height of the new box which we are about to create is greater than $\epsl  N$ and therefore number of such boxes is $O(\frac{1}{\epsl})$. Similar processes can be done to corridors with 2 or 3 bends.
	\subsubsection{Converting boundary corridor with $2$ bends to a single Boundary $\Lc$ in a box}\label{sss2}
	Let us consider a boundary corridor with $2$ bends with two vertical subcorridors $S_{1}, S_{3}$ on top of the horizontal subcorridor $S_{2}$ with $S_{3}$ being placed to the right of $S_{1}$. W.l.o.g.~ let us assume that the first stage cuts in the guillotine cutting sequence in the box is vertical. Now consider the cut $l$ through $S_{3}$. Let the distance between $l$ and edge of the boundary be $d$. Now remove the strip to the right of $l$ and shift the rest of items of box to the right by a distance of $d$. Now in the empty region created near the left edge of the box we place the strip which we removed. Now consider the rectangles in this strip, rectangles to the left of cut through $S_{1}$ before the shifting procedure and set of horizontal rectangles whose guillotine cut is intercepted by the former rectangles mentioned in this sentence. We now freeze these rectangles after shifting and consider the rest of the box as a new box and recursively apply the process to the remaining part of the corridor till we don't have any vertical guillotine cuts left. If we have exhausted the corridor then we are done and we have a single boundary $\Lc$. Otherwise, we must have horizontal cut through the remaining portion of the box to separate the rectangles because there no end to end vertical cut. We handle this in sub-subsection \ref{sssl}. The boundary $\Lc$ achieved due to the sequence of guillotine cuts forms the boundary $\Lc$ of the box. Also this boundary $\Lc$ can be converted into $O_{\epsl}$ smaller boundary $L$ with width at most $\epsl N$ by  dropping at most $O_{\eps,\epsl}(1)$ items as shown in Figure \ref{divL}. 
	\subsubsection{Converting boundary corridor with 3 bends to a single Boundary $\Lc$}\label{sss3}
	Consider a boundary corridor $S$ with 3 bends. Let us consider vertical subcorridors $S_{1}$ and $S_{3}$ which are on top of horizontal subcorridor $S_{2}$. $S_{3}$ is right of $S_{1}$ and below horizontal subcorridor $S_{4}$. Consider the horizontal guillotine cut through $S_{4}$ and remove the rectangles above this cut and place it  below corridor $S_{2}$ by shifting rectangles below the cut upwards. Now freeze this set of rectangles from $S_{4}$ which were moved down. Now in the remaining portion of the box take the vertical guillotine cut through $S_{3}$ and remove the rectangles to the right of this cut and place it to the left of $S_{1}$. Now freeze the rectangles in the similar fashion as done in the Sub-subsection \ref {sss2} and recursively repeat the process for the rectangles in subcorridors $S_{3}, S_{4}$ which aren't freezed yet till we exhaust these both the corridors. Note that we stop if there is no vertical cut through $S_{3}$ or a horizontal cut through $S_{4}$ then there must exist which divides the remaining portion of the box into 2 parts each containing corridors with at most 2 bends. If any one of them has a corridors of 2 bends then we can use the results of sub-subsection \ref{sss2} to get a box with boundary $\Lc$. Otherwise, we are done  and the rectangles which got freezed before this step form the boundary $\Lc$ of our original box with which we started initially. Also this boundary $\Lc$ can be converted into $O_{\epsl}$ smaller boundary $L$ with width at most $\epsl N$ by  dropping at most $O_{\eps,\epsl}(1)$ items  as shown in Figure \ref{divL}.

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}

		\centering
		\resizebox{!}{3.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			
			\draw [solid,fill=lightgray] (0,0)--(0,10)--(3,10)--(3,3)--(10,3)--(10,0)--(0,0);
			
			\draw [dashed] (1,10)--(1,1)--(10,1);
			\draw [dashed] (2,10)--(2,2)--(10,2);
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}



	\caption{Dividing a boundary $L$ (shaded region) into smaller boundary using dashed lines as shown in this figure. Vertical and horizontal dashed lines meet at the boundary curve. Dashed lines also form the edges of the smaller boxes which bound the new $L$ corridors being created}\label{divL}

\end{figure}
	           
	%\subsubsection{Merging 2 boundary $\Lc$ into a single boundary $\Lc$}\label{sss2l}
	%Now consider that we have 2 boundary $\Lc$ for the same box. If there is any end to end cut possible in the box which doesn't pass through any of the 2 boundary $\Lc$ or it passes through one or more than one subcorridors of 2 boundary $\Lc$ but it is perpendicular to the orientation of these subcorridors, then we divide the box into 2 boxes. We repeat the same procedure on the smaller box which contains both the boundary $\Lc$. If at any stage we find a cut which places both the boundary $\Lc$ in 2 different smaller boxes then we are done. So we now assume that there is no such end to end cut in the box we are considering which has 2 boundary $\Lc$. If the 2 boundary $\Lc$  are placed diagonally opposite to each other then consider the 2 boundary $\Lc$ as a corridor with 3 bends and convert into a single boundary $\Lc$ as mentioned in the subsubsection  \ref{sss3}. If the process in subsection \ref{sss3} can't covert it into a single boundary $\Lc$ it means in the remaining portion of the box which hasn't formed a part of the boundary $\Lc$ we have an end to end cut which separates the 2 remaining portions of the 2 boundary $\Lc$. If the boundary $\Lc$ are placed at the adjacent corners of the box then consider the 2 boundary $\Lc$ as a corridor with 2 bends and convert it into a single boundary $\Lc$ as mentioned in the subsubsection \ref{sss2}. If the process in subsection \ref{sss2} can't covert it into a single boundary $\Lc$ it means in the remaining portion of the box which hasn't formed a part of the boundary $\Lc$ we have an end to end cut which separates the 2 remaining portions of the 2 boundary $\Lc$.
	%\subsubsection{Merging 3 boundary $\Lc$ into a single boundary $\Lc$}\label{sss3l}
	%Now consider that we have 3 boundary $\Lc$ for the same box. If there is any end to end cut possible in the box which doesn't pass through any of the 3 boundary $\Lc$ or it passes through one or more than one subcorridors of 3 boundary $\Lc$ but it is perpendicular to the orientation of these subcorridors, then we divide the box into 2 boxes. One of the box contains 2 boundary $\Lc$ and other box contains 1 boundary $\Lc$. Boxes with 2 boundary $\Lc$ is handled in subsubsection \ref{sss2l}. So we now assume that there is no such end to end cut in the box we are considering which has 3 boundary $\Lc$. Now consider the 3 boundary $\Lc$ as a corridor with 3 bends and convert into a single boundary $\Lc$ as mentioned in the subsubsection  \ref{sss3}. If the process in subsection \ref{sss3} can't covert it into a single boundary $\Lc$ it means in the remaining portion of the box which hasn't formed a part of the boundary $\Lc$ we have an end to end cut which separates the 3 remaining portions of the 3 boundary $\Lc$ into smaller boxes with one box containing 2 boundary $\Lc$ and other box containing 1 boundary $\Lc$. Boxes with 2 boundary $\Lc$ is handled in subsubsection \ref{sss2l}.
	 %\subsubsection{Merging 4 boundary $\Lc$ into a single boundary $\Lc$}\label{sss4l}
	%Now consider that we have 4 boundary $\Lc$ for the same box. If there is any end to end cut possible in the box which doesn't pass through any of the 4 boundary $\Lc$ or it passes through one or more than one subcorridors of 4 boundary $\Lc$ but it is perpendicular to the orientation of these subcorridors. Each box has now 2 boundary $\Lc$. Boxes with 2 boundary $\Lc$ is handled in subsubsection \ref{sss2l}. So we now assume that there is no end to end cut in the box we are considering which has 4 boundary $\Lc$. Let's combine these to form a ring. Now consider the sequence of gullotine cuts which separate the rectangles in the ring. If we are cutting (cut is parallel to the orientation of the subcorridor and the rectangles which are being separated in that subcorridor) through leftmost vertical subcorridor or bottom most horizontal subcorridors then we freeze these rectangles as we freezed rectangles in subsubsection \ref{sss2l} and \ref{sss3l}. Now in the remaining portion of the box if there is a cut $l_{1}$ (cut is parallel to the orientation of the subcorridor) through rightmost vertical subcorridor and the distance between $l_{1}$ and edge of the boundary to the right of it be $d$ then we remove the strip to the right of $l_{1}$ and shift the rest of items of box which are not freezed to the right by a distance of $d$. Now in the empty region created near the left edge of the box we place the strip which we removed. Now freeze the rectangles in the strip which we moved. Do the same process if there is a cut (cut is parallel to the orientation of the subcorridor the rectangles which are being separated in that subcorridor) through the upper most horizontal corridor and now instead of shifting the strip above the cut to the left we shift it down by appropriately shifting the remaining portion of the box upwards which isn't still freezed. Continue this process till we convert these in to single boundary $\Lc$. If at some we can no longer find any cut parallel to the orientation of the subcorridors in the remaing portion of the ring it implies that there should exist an end to end cut in the remaining portion of the box which divides the remaining portion of the box into 2 boxes each containing 2 boundary $\Lc$ at most and this case is dealt in subsubsection \ref{sss2l}. So now have a box with boundary $\Lc$ and possibly 2 smaller boxes each containing 2 boundary $\Lc$.

	\subsection{Guillotine property}
	The construction of boxes and shifting of rectangle doesn't disturb the guillotine property. Now we show that the processing which we do in Subsection \ref{prosec} doesn't disturb the guillotine property if it is done to the boundary $\Lc$ which we obtain in the previous section. Now consider w.l.o.g.~that we are processing (as done in Subsection \ref{prosec}) a vertical subcorridor of the boundary $\Lc$ which is placed top-left with respect to horizontal subcorridor. Note that this processing does not create any conflict in terms of guillotine separability with elements in boxes and $\Bc$-corridors outside the box bounding this boundary $\Lc$ since by construction the boxes and $\Bc$-corridors are guillotine separable when considered as a pseudorectangle. Also the way in which we have constructed the boundary $\Lc$, we always have a sequence of vertical (resp.~horizontal) cuts through the vertical (resp.~horizontal) subcorridor of boundary $\Lc$ which separates the rectangles in the vertical (resp.~horizontal) subcorridor. This ensures that as long we can separate out the items in the boundary $\Lc$ from the rest of box using cuts which do not pass through the rest of the box, then the items in the rest of box can be separated as we have not changed their orientation. Now we need to focus on the boundary curve of the $\Lc$ corridor. Consider the strip containing the thin items. Let the length of the shorter vertical edge be $l$. Now the vertical strip which replaces this strip has rectangles of length at most $l$. So the horizontal rectangles which interacted with the thin items can be directly separated as there is no vertical rectangle intercepting the cut. Similar analogy for other strips shows that there is no conflict with horizontal rectangles. So we can conclude that the processing in Subsection \ref{prosec} doesn't disturb guillotine property.
	


==> 4_Corridor_Decomposition.tex <==
\section{BL-arrangement for guillotine packing} \label{sec:bl}
In this section, we prove our main structural result.
\begin{thm}[$\Bc \Lc$-arrangement (restatement of Theorem \ref{thm:ldecom})]
Given an optimal guillotine packing, there is a rearrangement of items into another guillotine packing and $\optco \subseteq \optsk$ such that:
\begin{enumerate}\itemsep0pt
\item there is a subset $\optco^{cross} \subseteq \optco$ with  $|\optco^{cross}| \le O_\eps(1)$ such that  each $i\in \optco \setminus \optco^{cross}$ is fully contained in some corridor,
\item $\profit(\optco) \ge (1-O(\eps))\profit(\optsk)$,
\item the number of corridors is $O_{\eps,\epsl}(1)$ and each horizontal (resp. vertical ) subcorridor has only horizontal (resp. vertical) items.
\item Every $\Lc$-corridor is a boundary-$\Lc$ for some guillotine separable bounding box and every $\Bc$-corridor is guillotine separable as a box. 
\end{enumerate}
\end{thm}			
	
	
To prove the theorem, first we will start with the corridor decomposition from Lemma \ref{lem:corridorPack} (see Figure \ref{fig:3a}). 
Then we apply Lemma \ref{noz}, remove all  $\Zc$-bends and  obtain only spiral corridors (see Figure \ref{fig:3b}).  
%In Section \ref{subsec41}, we have the omitted figures from proof of Lemma \ref{noz}. 
In Section \ref{subsec42}, we describe some subroutines that we use in the rest of the proof. 
Thereafter, in Section \ref{subsec43} we will further process to obtain spiral corridors with bends at most 4 (see Figure \ref{fig:3c}). 
In Section \ref{sub:bldec} we obtain bounding boxes for these corridors (see Figure \ref{fig:3e}). 
Finally, in Section \ref{ssss} we obtain boundary corridors and then the final $\Bc\Lc$-arrangement (see Figure \ref{fig:3f}). 
Section \ref{subs:guilp} finished the proof with a discussion on why the guillotine property was preserved in the rearrangement. 
For the remainder of the section we divide the cuts passing through the interior region of the subcorridors in a corridor $C$ into 3 types which are $C_p,C_b,C_u$. $C_p$ is a type of cut that passes through the interior region of a subcorridor $S_{i}$ and is parallel to the orientation of a $S_{i}$. $C_b$ is a type of cut that passes through a subcorridor $S_i$, is perpendicular to the orientation of a $S_i$ and passes through the boundary between one of the shared regions and the unshared region of $S_i$. $C_u$ is a type of cut which passes through a subcorridor $S_i$, is perpendicular to the orientation of a $S_i$ and passes through the unshared region of $S_i$.

%In this subsection, we provide the omitted figures from proof of Lemma \ref{noz}. 
%
%\begin{figure}[h]
%	%\centering
%	\captionsetup[subfigure]{justification=centering}
%	\hspace{-10pt}
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{3.5cm}{
%		\begin{tikzpicture}
%						\draw[thick] (0,6)--(2,6)--(2,5.5)--(4,5.5)--(4,6)--(6,6)--(6,4)--(5,4)--(5,3)--(4.5,3)--(4.5,4.5)--(5.5,4.5)--(5.5,5.5)--(4.5,5.5)--(4.5,5)--(1.5,5)--(1.5,5.5)--(.5,5.5)--(.5,4)--(2,4)--(2,3)--(4,3)--(4,2.5)--(1.5,2.5)--(1.5,3.5)--(0,3.5)--(0,6);		
%						
%						\draw[dotted] (6,4)--(5.5,4.5);
%						\draw[dotted] (5,4)--(4.5,4.5);
%						\draw[dotted] (6,6)--(5.5,5.5);
%						\draw[dotted] (4,6)--(4.5,5.5);
%						\draw[dotted] (2,6)--(1.5,5.5);
%						\draw[dotted] (0,6)--(.5,5.5);
%						\draw[dotted] (0.25,3.6)--(.5,4);
%						\draw[dotted] (1.5,2.5)--(2,3);
%						\draw[dotted] (1.5, 3.5)--(2,4);
%						\draw[dotted] (1.5, 5)--(2,5.5);
%						\draw[dotted] (4.5 , 5)--(4,5.5);
%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.4,3.5);	\draw (-.75,3.5) node {\textbf{$l_{i'+2}$}};
%						\draw[->] (1,5.75) edge[out=90,in=0,->] (.8,6.5);	\draw (.5,6.5) node {\textbf{$l_{i'+1}$}};
%						%\draw (1.75,5.25) node {\textbf{$l_{1}$}};
%						%\draw (4.25, 5.25) node {\textbf{$l_{2}$}{spialgo}};
%						%\draw[->] (5,5.75) edge[out=180,in=0,->] (4.75,6.5);	\draw (4.5,6.5) node {\textbf{$l$}};%
%%						\draw[->] (5.75,5) edge[out=180,in=0,->] (6.5,5);	\draw (6.5,5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%						\fill [lightgray] (0,3.5) rectangle (0.5,4);
%						\draw[->] (.2,3.75) edge[out=180,in=0,->] (-.4,2.5);	\draw (-.75,2.5) node {\textbf{$S_{i'+2,i'+3}$}};
%						\draw[dashed] (4.75,3) -- ( 4.75 ,4.25) -- ( 5.75, 4.25) -- ( 5.75, 5.75) -- ( 4.25, 5.75) -- ( 4.25, 5.25) -- ( 1.75, 5.25) -- ( 1.75, 5.75) -- (.25, 5.75) -- (.25, 3.5) ;	
%						%\draw (4,1.25) node {\large \textbf{$U'$}};
%						%\draw (5,4.75) node {\large \textbf{$C$}};
%						%\draw (4,3) node {\large \textbf{$B$}};
%		
%		\end{tikzpicture}}
%		\caption{k-bend Corridor Processing}
%		\label{fig:kbend}
%	\end{subfigure}
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{3.5cm}{
%		\begin{tikzpicture}
%						\draw[thick] (0,7)--(2,7)--(2,4)--(7,4)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
%						\draw  (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7) --(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
%						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
%						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
%					
%						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
%						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
%						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
%						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};
%
%
%						\draw[dashed] (5.6,.5)--(5.6,4);
%	
%		\end{tikzpicture}}
%		\caption{}
%		\label{fig:zbend}
%	\end{subfigure}
%	\caption{}
%\end{figure}


%\arir{ Fig. k-bend Corridor Processing. mention point P and show boundary curve.}



%\begin{figure}
%			\captionsetup[subfigure]{justification=centering}
%			\hspace{-15pt}
%			
%				\centering
%				\resizebox{!}{6cm}{
%					\begin{tikzpicture}					
%						\draw[thick] (0,6)--(2,6)--(2,5.5)--(4,5.5)--(4,6)--(6,6)--(6,4)--(5,4)--(5,3)--(4.5,3)--(4.5,4.5)--(5.5,4.5)--(5.5,5.5)--(4.5,5.5)--(4.5,5)--(1.5,5)--(1.5,5.5)--(.5,5.5)--(.5,4)--(2,4)--(2,3)--(4,3)--(4,2.5)--(1.5,2.5)--(1.5,3.5)--(0,3.5)--(0,6);		
%						
%						\draw[dotted] (6,4)--(5.5,4.5);
%						\draw[dotted] (5,4)--(4.5,4.5);
%						\draw[dotted] (6,6)--(5.5,5.5);
%						\draw[dotted] (4,6)--(4.5,5.5);
%						\draw[dotted] (2,6)--(1.5,5.5);
%						\draw[dotted] (0,6)--(.5,5.5);
%						\draw[dotted] (0.25,3.6)--(.5,4);
%						\draw[dotted] (1.5,2.5)--(2,3);
%						\draw[dotted] (1.5, 3.5)--(2,4);
%						\draw[dotted] (1.5, 5)--(2,5.5);
%						\draw[dotted] (4.5 , 5)--(4,5.5);
%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.4,3.5);	\draw (-.75,3.5) node {\textbf{$l_{i'+1}$}};
%						\draw[->] (1,5.75) edge[out=90,in=0,->] (.8,6.5);	\draw (.5,6.5) node {\textbf{$l_{i'+2}$}};
%						%\draw (1.75,5.25) node {\textbf{$l_{1}$}};
%						%\draw (4.25, 5.25) node {\textbf{$l_{2}$}};
%						%\draw[->] (5,5.75) edge[out=180,in=0,->] (4.75,6.5);	\draw (4.5,6.5) node {\textbf{$l$}};%
%%						\draw[->] (5.75,5) edge[out=180,in=0,->] (6.5,5);	\draw (6.5,5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%						\fill [lightgray] (0,3.5) rectangle (0.5,4);
%						\draw[->] (.2,3.75) edge[out=180,in=0,->] (-.4,2.5);	\draw (-.75,2.5) node {\textbf{$S_{i'+2,i'+3}$}};
%						\draw[dashed] (4.75,3) -- ( 4.75 ,4.25) -- ( 5.75, 4.25) -- ( 5.75, 5.75) -- ( 4.25, 5.75) -- ( 4.25, 5.25) -- ( 1.75, 5.25) -- ( 1.75, 5.75) -- (.25, 5.75) -- (.25, 3.5) ;	
%						%\draw (4,1.25) node {\large \textbf{$U'$}};
%						%\draw (5,4.75) node {\large \textbf{$C$}};
%						%\draw (4,3) node {\large \textbf{$B$}};
%					\end{tikzpicture}}
%				\caption{k-bend Corridor Processing}
%				\label{fig:kbend}
%		\end{figure}

%\begin{figure}[h]
%	%\centering
%	\captionsetup[subfigure]{justification=centering}
%	\hspace{-10pt}
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{3.5cm}{
%		\begin{tikzpicture}
%						\draw[thick] (0,7)--(7,7)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
%						\draw  (.75,6.25)--(6.25,6.25)--(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
%						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,0.5)--(5,0.5)--(5,0)--(7,0)--(7,7)--(0,7)--(0,3);
%						
%					
%						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
%						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
%						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
%						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};
%
%						
%	
%		\end{tikzpicture}}
%		\caption{}
%		\label{fig:zbend1}
%	\end{subfigure}
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{3.5cm}{
%		\begin{tikzpicture}
%						\draw[thick] (0,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
%						\draw  (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
%						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
%						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
%						\draw[pattern=north west lines, pattern color=gray] (5,.75)--(6.25,.75)--(6.25,0)--(5,0)--(5,.75);
%						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
%						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
%						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
%						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};
%						
%
%						
%	
%		\end{tikzpicture}}
%		\caption{}
%		\label{fig:zbend2}
%	\end{subfigure}
%	
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{3.5cm}{
%		\begin{tikzpicture}
%						\draw[thick] (0,7)--(7,7)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
%						\draw  (.75,6.25)--(6.25,6.25)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
%						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,2)--(7,2)--(7,7)--(0,7)--(0,3);
%						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
%					
%						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
%						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
%						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
%						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};
%
%						
%	
%		\end{tikzpicture}}
%		\caption{}
%		\label{fig:zbend3}
%	\end{subfigure}
%\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{3.5cm}{
%		\begin{tikzpicture}
%						\draw[thick] (0,5)--(0.75,5)--(0.75,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,5);
%						\draw  (.75,4.5)--(1.25,4.5)--(1.25,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,4.5); 	
%						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,5)--(0,5)--(0,3);
%						\draw[pattern=north west lines, pattern color=gray] (0.75,6.5)--(2,6.5)--(2,7)--(0.75,7)--(0.75,6.5);
%						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
%						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
%						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
%						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
%						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
%						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};
%						
%
%						
%	
%		\end{tikzpicture}}
%		\caption{}
%		\label{fig:zbend4}
%	\end{subfigure} 
%	\caption{}\label{closedcor2}	
%\end{figure}



\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{2cm}{
			\begin{tikzpicture}
		
					\draw[thick] (0,6) -- (0,0) -- (12,0) -- (12,10) -- (4,10) -- (4,4) -- (6,4) -- (6,8) -- ( 10,8) -- (10,2) -- (2,2) -- (2,6) -- (0,6); 
					\draw[thick,pattern=north west lines, pattern color=gray] (0,6) -- (0,0) -- (12,0) -- (12,10) -- (4,10)--(4,9)--(11,9)--(11,1)--(1,1)--(1,6)--(0,6);	
					\draw (1.5,3) node {\large \textbf{$S_{1}$}};
					\draw (6,1.5) node {\large \textbf{$S_{2}$}};
					\draw (10.5,5) node {\large \textbf{$S_{3}$}};
					\draw (8,8.5) node {\large \textbf{$S_{4}$}};
					\draw (4.5,7) node {\large \textbf{$S_{5}$}};
					\draw [dashed] (5,9)--(5,1);
					\end{tikzpicture}}
				\caption{}
				\label{bends}

	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{2cm}{
		\begin{tikzpicture}
					\draw (0,0)--(6,0)--(6,2)--(2,2)--(2,6)--(0,6)--(0,0);	
						
					\draw (1.5,3) node { \large \textbf{$S_{1}$}};
					\draw (3,1.5) node { \large \textbf{$S_{2}$}};
					\draw [dashed] (0.5,6)--(0.5,0);
					\draw [dashed] (1,6)--(1,0);
					\draw [dashed] (1,0.5)--(6,0.5);
					\end{tikzpicture}}
				\caption{}
				\label{sepi1}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{2cm}{
		\begin{tikzpicture}
					\draw (0,0)--(6,0)--(6,2)--(2,2)--(2,6)--(0,6)--(0,0);	
					\draw[pattern=north west lines, pattern color=gray] (0,0)--(6,0)--(6,0.5)--(1,0.5)--(1,6)--(0,6)--(0,0);	
					\draw (1.5,3) node { \large \textbf{$S_{1}$}};
					\draw (3,1.5) node { \large \textbf{$S_{2}$}};
					\draw [dashed] (0.5,6)--(0.5,0);
					\draw [dashed] (1,6)--(1,0);
					\draw [dashed] (1,0.5)--(6,0.5);
					\end{tikzpicture}}
				\caption{}
				\label{sepi2}
	\end{subfigure}
	\caption{(a) Cut of type $C_u$ (dashed lines) and with the corridor separated out (region having north-west lines) partition the original corridor with 4 bends into $O_{\eps,\epsl}$ corridors with less than 4 corridors. (b) Consider the last cuts through each corridor to separate out an $\Lc$-corridor. (c) $\Lc$-corridor separated out (region with north west lines)}
\end{figure}

%\begin{figure}[h]
%	%\centering
%	\captionsetup[subfigure]{justification=centering}
%	\hspace{-10pt}
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{2cm}{
%			\begin{tikzpicture}
%		
%					\draw[thick] (0,6) -- (0,0) -- (12,0) -- (12,10) -- (4,10) -- (4,4) -- (6,4) -- (6,8) -- ( 10,8) -- (10,2) -- (2,2) -- (2,6) -- (0,6); 
%					\draw[thick,pattern=north west lines, pattern color=gray] (0,6) -- (0,0) -- (12,0) -- (12,10) -- (4,10)--(4,9)--(11,9)--(11,1)--(1,1)--(1,6)--(0,6);	
%					\draw (1.5,3) node {\large \textbf{$S_{1}$}};
%					\draw (6,1.5) node {\large \textbf{$S_{2}$}};
%					\draw (10.5,5) node {\large \textbf{$S_{3}$}};
%					\draw (8,8.5) node {\large \textbf{$S_{4}$}};
%					\draw (4.5,7) node {\large \textbf{$S_{5}$}};
%					\draw [dashed] (5,9)--(5,1);
%					\end{tikzpicture}}
%				\caption{Cut perpendicular to the orientation of corridor (dashed lines) and with the corridor separated out (region having north-west lines) partition the original corridor with 4 bends into $O_{\eps,\epsl}$ corridors with less than 4 corridors}
%				\label{bends}
%
%	\end{subfigure}
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{2cm}{
%		\begin{tikzpicture}
%					\draw (0,0)--(6,0)--(6,2)--(2,2)--(2,6)--(0,6)--(0,0);	
%						
%					\draw (1.5,3) node { \large \textbf{$S_{1}$}};
%					\draw (3,1.5) node { \large \textbf{$S_{2}$}};
%					\draw [dashed] (0.5,6)--(0.5,0);
%					\draw [dashed] (1,6)--(1,0);
%					\draw [dashed] (1,0.5)--(6,0.5);
%					\end{tikzpicture}}
%				\caption{Consider the last cuts through each corridor to separate out an $\Lc$-corridor}
%				\label{sepi1}
%	\end{subfigure}
%	\begin{subfigure}[b]{.5\textwidth}
%		\centering
%		\resizebox{!}{2cm}{
%		\begin{tikzpicture}
%					\draw (0,0)--(6,0)--(6,2)--(2,2)--(2,6)--(0,6)--(0,0);	
%					\draw[pattern=north west lines, pattern color=gray] (0,0)--(6,0)--(6,1)--(1,1)--(1,6)--(0,6)--(0,0);	
%					\draw (1.5,3) node { \large \textbf{$S_{1}$}};
%					\draw (3,1.5) node { \large \textbf{$S_{2}$}};
%					\draw [dashed] (0.5,6)--(0.5,0);
%					\draw [dashed] (1,6)--(1,0);
%					\draw [dashed] (1,0.5)--(6,0.5);
%					\end{tikzpicture}}
%				\caption{$\Lc$-corridor separated out (region with north west lines)}
%				\label{sepi2}
%	\end{subfigure}
%	\caption{}
%\end{figure}

%%%%%%%%%%%%%%%%%


==> 4_Corridor_Decomposition_backup.tex <==
\section{$\Bc \Lc$-decomposition for guillotine packing} \label{sec:bl}
In this section we will show that we can have a better decomposition of the optimal guillotine packing.
We will show the existence of a corridor-decomposition where all corridors are either $\Bc$ or $\Lc$s.	
We will prove the main strcutural result as follows:	
\begin{thm}
\label{thm:ldecom}
There exists a corridor partition (we call it $\Bc \Lc$-decomposition) and $\optco \subseteq \optsk$ such that:
\begin{enumerate}\itemsep0pt
\item there is a subset $\optco^{cross} \subseteq \optco$ with  $|\optco^{cross}| \le O_\eps(1)$ such that  each $i\in \optco \setminus \optco^{cross}$ is fully contained in some corridor,
\item $\profit(\optco) \ge (1-O(\eps))\profit(\optsk)$,
\item the number of corridors is $O_{\eps,\epsl}(1)$ and each corridor is either $\Bc$ or $\Lc$ corridor with width at most $\epsl N$.
\end{enumerate}
\end{thm}		
	
To prove the theorem, first we will start with the corridor decomposition from Lemma \ref{lem:corridorPack}. Then process the $\Zc$-bends in the corridors to obtain only spiral corridors. Thereafter, we will further process to obtain spiral corridors with bends at most 4. Finally we will process $\Uc$ and $\Gc$ corridors to obtain only $\Lc$ or $\Bc$ corridors. 
	
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Obtaining corridors of types $\Bc, \Lc, \Uc, \Gc$} 
\label{subsec:blug}


		\begin{figure}
			\captionsetup[subfigure]{justification=centering}
			\hspace{-15pt}
				\centering
				\resizebox{!}{4cm}{
					\begin{tikzpicture}					
					\draw[solid] (0,6) rectangle (2,10);
					\draw[solid, fill=lightgray] (0,4) rectangle (2,6);
					\draw[solid] (2,4) rectangle (8,6);
					\draw[solid, fill=lightgray] (8,4) rectangle (10,6);
					\draw[solid] (8,0) rectangle (10,4);
		
					\draw (1,8) node {\large \textbf{$S_{1}$}};
					\draw (1,5) node {\large \textbf{$S_{12}$}};
					\draw (6,5) node {\large \textbf{$S_{2}$}};
					\draw (9,5) node {\large \textbf{$S_{23}$}};
					\draw (9,2) node {\large \textbf{$S_{3}$}};
		
					\end{tikzpicture}}
				\caption{Corridor C consisting of subcorridors $S_{1},S_{2},S_{3}$ and overlapping regions of the subcorridors $S_{12}$  and  $S_{23}$.}
				\label{zstructure}
		\end{figure}
		
	
	
\subsubsection{Obtaining spiral corridors}
First, we show how to process $\Zc$-bends. 

\begin{lem}
\label{theorem1}
Any $\Zc$-corridor $C$ can be decomposed into $O(\frac{1}{\epsl})$. corridors of type $\Bc$ or $\Lc$. 
\end{lem}
\begin{proof}
W.l.o.g.~assume the center-sc of $C$ to be horizontal (See Figure \ref{zstructure}). 
%Region $S_{12}$ is shared by subcorridors $S_{1}$ and $S_{2}$ and similar convention holds for $S_{23}$. 
Consider the guillotine cutting sequence of all rectangles in the knapsack. 
Let $P$ be the smallest piece containing $C$, i.e., the next guillotine cut in $P$ passes through $C$. 
Now we will consider the guillotine cutting  sequence of rectangles in $P$ to iteratively decompose the $\Zc$-corridor into one of the three subcases: ($i$) into two $\Lc$-corridors, or ($ii$) a $\Bc$-corridor and an  $\Lc$-corridor, or ($iii$) a $\Bc$-corridor and a smaller $\Zc$-corridor.  
We stop when we reach subcases ($i$) or ($ii$). Otherwise in subcase ($iii$), we continue iteratively. 
This sequence can have five types of cuts:
\begin{itemize}
\item {\em HS}: horizontal guillotine cut which passes through a side-sc but doesn't pass through center-sc,
%\item Cut 2: horizontal guillotine cut which passes through $S_{3}$ and doesn't pass through $S_{23}$,
\item {\em VS}: vertical guillotine cut which passes through a side-sc,
%\item Cut 4: vertical guillotine cut which passes through $S_{3}$,
\item  {\em VC}: vertical guillotine cut which passes through center-sc but doesn't pass through any side-sc,
\item {\em HC}: horizontal guillotine cut which passes through center-sc,
\item {\em NC}: cut which doesn't pass through $\Zc$-corridor.
\end{itemize}
Now, if we get cuts of type  {\em VC} (or {\em HC}) at any subpiece, we are in case $(i)$ as we obtain 2 $\Lc$-corridors. 
On the other hand, if we get {\em NC}-type cut we just focus on the subpiece containing the  $\Zc$-corridor of the present iteration.
If we have either cuts of type {\em VS} (or {\em HS}) passing through a side-sc then we are dividing the $\Zc$-bend into a rectangular region and a smaller $\Zc$-corridor. 
If there are no rectangle left in one of the side-sc of the smaller $\Zc$-corridor, we call the subcorridor to be {\em exhausted}. In case of exhaustion of a subcorridor, we reach case $(ii)$ as the smaller $\Zc$-corridor can be considered as an $\Lc$-corridor by ignoring the exhausted side-sc.
Otherwise, we are in case $(iii)$. 
The rectangles in side-sc have height $\ge \epsl N$, so the consecutive cuts of {\em HS} creating $\Bc$-corridor have to be at a distance of atleast $\epsl N$. This ensures that the number of such corridors is $O(\frac{1}{\epsl})$. 
Note that we can merge all the adjacent rectangular regions obtained due to successive cuts of {\em VS} into a $\Bc$-corridor of same height till we arrive at a cut of different type (excluding {\em NC}). And since the number of cuts excluding {\em VS} and {\em NC} is $O(\frac{1}{\epsl})$, therefore number of such $\Bc$-corridors created due to successive cuts of {\em VS} is $O(\frac{1}{\epsl})$. 
\end{proof}

\arir{need to add a figure. }


\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,6)--(2,6)--(2,5.5)--(4,5.5)--(4,6)--(6,6)--(6,4)--(5,4)--(5,3)--(4.5,3)--(4.5,4.5)--(5.5,4.5)--(5.5,5.5)--(4.5,5.5)--(4.5,5)--(1.5,5)--(1.5,5.5)--(.5,5.5)--(.5,4)--(2,4)--(2,3)--(4,3)--(4,2.5)--(1.5,2.5)--(1.5,3.5)--(0,3.5)--(0,6);		
						
						\draw[dotted] (6,4)--(5.5,4.5);
						\draw[dotted] (5,4)--(4.5,4.5);
						\draw[dotted] (6,6)--(5.5,5.5);
						\draw[dotted] (4,6)--(4.5,5.5);
						\draw[dotted] (2,6)--(1.5,5.5);
						\draw[dotted] (0,6)--(.5,5.5);
						\draw[dotted] (0.25,3.6)--(.5,4);
						\draw[dotted] (1.5,2.5)--(2,3);
						\draw[dotted] (1.5, 3.5)--(2,4);
						\draw[dotted] (1.5, 5)--(2,5.5);
						\draw[dotted] (4.5 , 5)--(4,5.5);

						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.4,3.5);	\draw (-.75,3.5) node {\textbf{$l_{i'+2}$}};
						\draw[->] (1,5.75) edge[out=90,in=0,->] (.8,6.5);	\draw (.5,6.5) node {\textbf{$l_{i'+1}$}};
						%\draw (1.75,5.25) node {\textbf{$l_{1}$}};
						%\draw (4.25, 5.25) node {\textbf{$l_{2}$}};
						%\draw[->] (5,5.75) edge[out=180,in=0,->] (4.75,6.5);	\draw (4.5,6.5) node {\textbf{$l$}};%
%						\draw[->] (5.75,5) edge[out=180,in=0,->] (6.5,5);	\draw (6.5,5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
						\fill [lightgray] (0,3.5) rectangle (0.5,4);
						\draw[->] (.2,3.75) edge[out=180,in=0,->] (-.4,2.5);	\draw (-.75,2.5) node {\textbf{$S_{i'+2,i'+3}$}};
						\draw[dashed] (4.75,3) -- ( 4.75 ,4.25) -- ( 5.75, 4.25) -- ( 5.75, 5.75) -- ( 4.25, 5.75) -- ( 4.25, 5.25) -- ( 1.75, 5.25) -- ( 1.75, 5.75) -- (.25, 5.75) -- (.25, 3.5) ;	
						%\draw (4,1.25) node {\large \textbf{$U'$}};
						%\draw (5,4.75) node {\large \textbf{$C$}};
						%\draw (4,3) node {\large \textbf{$B$}};
		
		\end{tikzpicture}}
		\caption{k-bend Corridor Processing}
		\label{fig:kbend}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,7)--(2,7)--(2,4)--(7,4)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw  (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7) --(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
					
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};


						\draw[dashed] (5.6,.5)--(5.6,4);
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend}
	\end{subfigure}
	\caption{}
\end{figure}



%\begin{figure}
%			\captionsetup[subfigure]{justification=centering}
%			\hspace{-15pt}
%			
%				\centering
%				\resizebox{!}{6cm}{
%					\begin{tikzpicture}					
%						\draw[thick] (0,6)--(2,6)--(2,5.5)--(4,5.5)--(4,6)--(6,6)--(6,4)--(5,4)--(5,3)--(4.5,3)--(4.5,4.5)--(5.5,4.5)--(5.5,5.5)--(4.5,5.5)--(4.5,5)--(1.5,5)--(1.5,5.5)--(.5,5.5)--(.5,4)--(2,4)--(2,3)--(4,3)--(4,2.5)--(1.5,2.5)--(1.5,3.5)--(0,3.5)--(0,6);		
%						
%						\draw[dotted] (6,4)--(5.5,4.5);
%						\draw[dotted] (5,4)--(4.5,4.5);
%						\draw[dotted] (6,6)--(5.5,5.5);
%						\draw[dotted] (4,6)--(4.5,5.5);
%						\draw[dotted] (2,6)--(1.5,5.5);
%						\draw[dotted] (0,6)--(.5,5.5);
%						\draw[dotted] (0.25,3.6)--(.5,4);
%						\draw[dotted] (1.5,2.5)--(2,3);
%						\draw[dotted] (1.5, 3.5)--(2,4);
%						\draw[dotted] (1.5, 5)--(2,5.5);
%						\draw[dotted] (4.5 , 5)--(4,5.5);
%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.4,3.5);	\draw (-.75,3.5) node {\textbf{$l_{i'+1}$}};
%						\draw[->] (1,5.75) edge[out=90,in=0,->] (.8,6.5);	\draw (.5,6.5) node {\textbf{$l_{i'+2}$}};
%						%\draw (1.75,5.25) node {\textbf{$l_{1}$}};
%						%\draw (4.25, 5.25) node {\textbf{$l_{2}$}};
%						%\draw[->] (5,5.75) edge[out=180,in=0,->] (4.75,6.5);	\draw (4.5,6.5) node {\textbf{$l$}};%
%%						\draw[->] (5.75,5) edge[out=180,in=0,->] (6.5,5);	\draw (6.5,5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%						\fill [lightgray] (0,3.5) rectangle (0.5,4);
%						\draw[->] (.2,3.75) edge[out=180,in=0,->] (-.4,2.5);	\draw (-.75,2.5) node {\textbf{$S_{i'+2,i'+3}$}};
%						\draw[dashed] (4.75,3) -- ( 4.75 ,4.25) -- ( 5.75, 4.25) -- ( 5.75, 5.75) -- ( 4.25, 5.75) -- ( 4.25, 5.25) -- ( 1.75, 5.25) -- ( 1.75, 5.75) -- (.25, 5.75) -- (.25, 3.5) ;	
%						%\draw (4,1.25) node {\large \textbf{$U'$}};
%						%\draw (5,4.75) node {\large \textbf{$C$}};
%						%\draw (4,3) node {\large \textbf{$B$}};
%					\end{tikzpicture}}
%				\caption{k-bend Corridor Processing}
%				\label{fig:kbend}
%		\end{figure}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,7)--(7,7)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw  (.75,6.25)--(6.25,6.25)--(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,0.5)--(5,0.5)--(5,0)--(7,0)--(7,7)--(0,7)--(0,3);
						
					
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};

						
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend1}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw  (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[pattern=north west lines, pattern color=gray] (5,.75)--(6.25,.75)--(6.25,0)--(5,0)--(5,.75);
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};
						

						
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend2}
	\end{subfigure}
	
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,7)--(7,7)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw  (.75,6.25)--(6.25,6.25)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,2)--(7,2)--(7,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
					
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};

						
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend3}
	\end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,5)--(0.75,5)--(0.75,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,5);
						\draw  (.75,4.5)--(1.25,4.5)--(1.25,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,4.5); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,5)--(0,5)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (0.75,6.5)--(2,6.5)--(2,7)--(0.75,7)--(0.75,6.5);
						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};
						

						
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend4}
	\end{subfigure} 
	\caption{}\label{closedcor2}	
\end{figure}

\begin{lem}\label{noz}
%A non-spiral corridor $C$ can be decomposed  into $O_{\eps}(1)$ spiral corridors and $O_{\eps}(1)$ $\Zc$-corridors by dropping atmost $O_{\eps,\epsl}(1)$ rectangles. 
A corridor with one or more $\Zc$ bends can be partitioned into $O_{\eps}(1)$ spiral corridors  by removing $O_{\eps,\epsl}(1)$ items, maintaining guillotine separability.
\end{lem}
\arir{write this proof and figure appropriately.}
\begin{proof}
There are two cases. 

\noindent \textit{Case 1: $C$ is open corridor with at least one $\Zc$-bend.} Let $C$ have $k$ subcorridors $\{ S_{1},S_{2},S_{3},...,S_{k}\}$ such that $\forall i \in [k-1]$, $S_{i}$ and $S_{i+1}$ share a region $S_{i,i+1}$ with each other. Assume there are 5 subcorridors (If there are less than 5 subcorridors the following proof would still hold) $S_{i'+1}, S_{i'+2}, S_{i'+3}, S_{i'+4} $ and $S_{i'+5}$ such that $\{S_{i'+2},S_{i'+3},S_{i'+4}\}$ form a $\Zc$ bend. Let $S_{i'+3}$ be a horizontal subcorridor and $S_{i'+2}$ be situated to the top left of $S_{i'+3}$. Let us consider a sequence of guillotine cuts through the five subcorridors  $S_{i'+1}, S_{i'+2}, S_{i'+3}, S_{i'+4} $ and $S_{i'+5}$.\\

After a sequence of guillotine cuts through corridor $C$ (including those which is coincident with the edges of $C$) , we get our first cut $l'$ which passes through the unshared region of $S_{i'+3}$. Now consider the guillotine cuts which occured before the cut $l'$. Let $l_{i'+2}$ be the rightmost vertical cut (including those which pass through the boundary of $S_{i'+2,i'+3}$ if any) through $S_{i'+2,i'+3}$. Extend the cut $l_{i'+2}$ so that it touches the boundary curve between $S_{i'+1}$ and $S_{i'+2}$ at point $P$. Now draw a line $l_{i'+1}$ from point $P$ parallel to the orientation of $S_{i'+1}$ till it touches the boundary curve between $S_{i'+1}$ and $S_{i'}$. Continue the same process by drawing lines $l_{j}$ through corridors $S_{j}$ where $1 \leq j \leq i'$ in similar fashion. Stop drawing these lines when we draw a line $l_{1}$ through $S_{1}$ parallel to the orientation of $S_{1}$ and reach its boundary edge.   Lines $\{l_{1},l_{2},..,l_{i'+2}\}$ partitions the corridor $C$ into atmost 2 smaller corridors $C_{1},C_{2}$ as shown in Figure \ref{fig:kbend}. $C_{1}$ contains rectangles from the subcorridors $S_{1},..,S_{i'+2}$ only. $C_{2}$ contains rectangles from the subcorridors $S_{1},...,S_{k}$ (maynot contain rectangles from every subcorridor). In a similar way we can partition $C_{2}$ into atmost 2 corridors $C_{3}$ and $C_{4}$ where $C_{3}$ contains rectangles from the subcorridors $S_{i'+4},..,S_{k}$ only and $C_{4}$ contains rectangles from the subcorridors $S_{1},...,S_{k}$ (maynot contain rectangles from every subcorridor). During this process of partitioning we drop atmost $O_{\eps,\epsl}(1)$ rectangles. Now suppose that the first cut through $S_{3}$ only is a horizontal cut. This divides the $C_{4}$ into 2 corridors containing atleast one lesser $\Zc$ bend when compared to $C$. Note that the reason for choosing $l_{i'+2}$ and extending it to partition the corridor $C$ is that $l_{i'+2}$ is the cut which intercepts the horizontal cut $l'$ in the shared region $S_{i'+2,i'+3}$ and hence it enables us to partition $C_{4}$ into 2 corridors using $l'$. Similarly if the first cut through $S_{3}$ only was vertical, then we can partition $C_{4}$ using the vertical cut into 2 corridors, each containing atleast one lesser $\Zc$ bend when compared to $C$.\\

Doing the above procedure for all $\Zc$ bends concludes the proof for case 1.

%Now let us consider the second subcase where we dont have any cut in the guillotine cutting sequence which passes through the region of $S_{3}$ which is not part of any other subcorridor and neither $S_{i'+2}$ nor $S_{i'+4}$ has a horizontal cut passing through the unshared regions of these subcorridors. If $S_{i'+2}$ gets exhausted during the guillotine cutting sequence then we simply divide the corridor $C$ into 2 corridors $C_{1'}$ and $C_{2'}$ such that $C_{1'}$ contains rectangles from  the subcorridors $S_{1},..,S_{i'+2}$ only and $C_{2'}$ contains rectangles from the subcorridors $S_{i'+3},...,S_{k}$ only. Similar partitioning can be done if $S_{i'+4}$ gets exhausted. Otherwise eventually due to the sequence of guillotine cuts $S_{i'+1}$ and $S_{i'+5}$ will be exhausted. Then we can partition $C$ into 3 corridors $C_{1''}$,$C_{2''}$ and $C_{3''}$ in similar fashion as we did in the previous subcase (which was done previously using the lines $\{l_{1},l_{2},..,l_{i'+2}\}$). $C_{1''}$ contains rectangles from the subcorridors $S_{1},..,S_{i'+2}$, $C_{2''}$ contains rectangles from the subcorridors $S_{i'+4},..,S_{k}$, $C_{3''}$ contains rectangles from the subcorridors $S_{i'+2},S_{i'+3},S_{i'+4}$.\\

%Now let us consider the last case where we dont have any cut in the guillotine cutting sequence which passes through the region of $S_{3}$ which is not part of any other subcorridor and either $S_{i'+2}$ or $S_{i'+4}$ has a horizontal cut passing through the unshared regions of these subcorridors.Let us assume that we have a horizontal cut through the unshared region of $S_{i'+2}$. Let $l_{v'}$ be the last vertical cut through $S_{i'+2,i'+3}$ before the first horizontal cut $l_{h}$ through $S_{i'+2}$ only. Let $l_{h'}$ be the part of $l_{h}$ which is inside $S_{i'+2}$. Extend $l_{v'}$ to meet the boundary curve between $S_{i'+2}$ and $S_{i'+1}$. Then continue making lines parallel to the orientation to the subcorridors $S_{i'+1},S_{i'},...,S_{1}$ as done in the previous subcase. Then using the lines created and $l_{h'}$ we can divide $C$ into 3 corridors $C_{1'''},C_{2'''},C_{3'''}$. $C_{1'''}$ and $C_{2'''}$ contains rectangles from the subcorridors $S_{1},..,S_{i'+2}$ only. $C_{3'''}$ contains rectangles from the subcorridor $S_{i'+2},...,S_{k}$. If there is a horizontal cut through the unshared region of $S_{i'+4}$ then we can partition $C_{3'''}$ into $C_{4'''}, C_{5'''},C_{6'''}$ where $C_{4'''}$ and $C_{5'''}$ contains rectangles from the subcorridors $S_{i'+4},..,S_{k}$,  $C_{6'''}$ contains rectangles from the subcorridors $S_{i'+2},S_{i'+3},S_{i'+4}$. Otherwise $C_{3'''}$ is handled appropriately in subcase 2.\\


\noindent \textit{Case 2: $C$ is a closed corridor with at least one $\Zc$-bend.}  Let $S_{1}$ be the leftmost vertical subcorridor in $C$, $S_{2}$ be the bottommost horizontal subcorridor in $C$, $S_{3}$ be the rightmost vertical subcorridor in $C$, $S_{4}$ be the topmost subcorridor in $C$.  Depending on the arrangement of these four subcorridors $\{S_{1},S_{2},S_{3},S_{4}\}$ we separate out the rectangles from these 4 subcorridors during guillotine cutting sequence into atmost 4 spiral corridors with atmost 4 bends as shown in Figure \ref{fig:zbend} and Figure  \ref{closedcor2}. Items are packed into $\Gc$ corridor if the 4 subcorridors  $\{S_{1},S_{2},S_{3},S_{4}\}$ form a $\Gc$ corridor among themselves. Similarly items are packed into a $\Uc$ corridor or $\Lc$ corridors or $\Bc$-corridors depending upon the arrangement of corridors among themselves. During the sequence of guillotine cuts if there cut which passes through the unshared region of subcorridor perpendicular to it's orientation then it clearly divides the subcorridor into $O_{\eps}(1)$ open corridors with atmost $O_{\eps}(1)$ which is handled in Case 1 as shown in Figure \ref{fig:zbend}. Otherwise if we don't have such cut then eventually one of the subcorridors  $\{S_{1},S_{2},S_{3},S_{4}\}$ is exhausted as the items are being added continuously to the $O(1)$ spiral corridors with atmost 4 bends. So, we are left with $O(1)$ open corridors as shown in Figure \ref{fig:zbend2} which is again dealt in Case 1. This concludes our proof.    
\end{proof}


\begin{lem}\label{no_z}
A corridor with one or more $\Zc$ bends can be partitioned into $O_{\eps}(1)$ spiral corridors  by removing $O_{\eps,\epsl}(1)$ items, maintaining guillotine separability. 
\end{lem}
\begin{proof}
Follows from Lemma \ref{noz} and Theorem \ref{thm:ldecom}.  
\end{proof}

		
%		
%\begin{figure}[t]
%			\captionsetup[subfigure]{justification=centering}
%			\hspace{-15pt}
%
%				\centering
%				\resizebox{!}{5cm}{
%					\begin{tikzpicture}
%		
%					\draw[thick] (0,6) -- (0,0) -- (12,0) -- (12,10) -- (4,10) -- (4,4) -- (6,4) -- (6,8) -- ( 10,8) -- (10,2) -- (2,2) -- (2,6) -- (0,6); 
%		
%					\draw (1,3) node {\large \textbf{$S_{1}$}};
%					\draw (6,1) node {\large \textbf{$S_{2}$}};
%					\draw (11,5) node {\large \textbf{$S_{3}$}};
%					\draw (8,9) node {\large \textbf{$S_{4}$}};
%					\draw (5,7) node {\large \textbf{$S_{5}$}};
%		
%					\end{tikzpicture}}
%				\caption{Corridors with more than 3 bends is not possible}
%				\label{bends}
%
%		\end{figure}
%\begin{figure}[t]
%			\captionsetup[subfigure]{justification=centering}
%			\hspace{-15pt}
%
%				\centering
%				\resizebox{!}{5cm}{
%					\begin{tikzpicture}
%		
%					\draw[thick](0,0) rectangle (12,12);
%					\draw[thick](2,2) rectangle (10,10);
%					\draw (1,6) node { \large \textbf{$S_{1}$}};
%					\draw (11,6) node { \large \textbf{$S_{3}$}};
%					\draw (6,1) node { \large \textbf{$S_{2}$}};	
%					\draw (6,11) node { \large \textbf{$S_{4}$}};
%					\end{tikzpicture}}
%				\caption{Ring can be converted into corridors without any $\Zc$ bend and consisting of atmost 3 bends.}
%				\label{rings}
%		\end{figure}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.5cm}{
			\begin{tikzpicture}
		
					\draw[thick] (0,6) -- (0,0) -- (12,0) -- (12,10) -- (4,10) -- (4,4) -- (6,4) -- (6,8) -- ( 10,8) -- (10,2) -- (2,2) -- (2,6) -- (0,6); 
		
					\draw (1,3) node {\large \textbf{$S_{1}$}};
					\draw (6,1) node {\large \textbf{$S_{2}$}};
					\draw (11,5) node {\large \textbf{$S_{3}$}};
					\draw (8,9) node {\large \textbf{$S_{4}$}};
					\draw (5,7) node {\large \textbf{$S_{5}$}};
		
					\end{tikzpicture}}
				\caption{Corridors with more than 3 bends is not possible}
				\label{bends}

	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.5cm}{
		\begin{tikzpicture}		
					\draw[thick](0,0) rectangle (12,12);
					\draw[thick](2,2) rectangle (10,10);
					\draw (1,6) node { \large \textbf{$S_{1}$}};
					\draw (11,6) node { \large \textbf{$S_{3}$}};
					\draw (6,1) node { \large \textbf{$S_{1}$}};	
					\draw (6,11) node { \large \textbf{$S_{1}$}};
					\end{tikzpicture}}
				\caption{Ring can be converted into corridors without any z bend and consisting of atmost 3 bends.}
				\label{rings}
	\end{subfigure}
	\caption{}
\end{figure}


\begin{cor}
Every closed corridor $C$ in corridor decomposition of guillotine separable set of items, obtained after the processing done in Theorem \ref{theorem1} and Lemma \ref{noz}, is a ring.
\end{cor}
%\begin{proof} It follows from Corollary \ref{no_z} as there exists no corridor with $\Zc$ bend.
%\end{proof}


%%%%%%%%%%%%%%%%%
\subsubsection{Obtaining corridors with at most three bends}

\begin{lem}
\label{ringlem}
Every ring $R$ obtained after the previous corridor decomposition, can be converted into $O(1)$ number of open corridors with at most 3 bends and possibly a box which is guillotine separable and the box contains a smaller ring. All items in this decomposition remain guillotine separable. 
\end{lem}
\begin{proof} Consider the guillotine cuts sequence on the knapsack. Let $P$ be the smallest subpiece such that ring $R$ lies completely inside $P$ and the next guillotine cut in $P$ is the first cut which passes through $R$.  As in Figure \ref{rings}, we call the left vertical, bottom horizontal, right vertical, top horizontal subcorridors of $R$ as $S_{1}$, $S_{2}$, $S_{3}$ and $S_{4}$ respectively. 
If any cut in $P$ cuts the smaller vertical (resp. horizontal) edges of $S_{1}$ and $S_{3}$ (resp. $S_{2}$ and $S_{4}$), then  we are done as $R$ gets divided into 2 $\Uc$-corridors.  Thus we can assume that first cut passes through a subcorridor and is parallel to its longer edges. 
We now define four types of end-to-end cuts possible in $P$ or in any of the subpieces formed by a sequence of cuts in $P$. The rightmost (resp. leftmost) end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$ ($S_{3}$) is termed as Type $1$ (resp. Type $3$). The topmost (resp. bottommost) end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{2}$ ($S_{4}$) is termed as Type $2$ (resp. Type $4$).  These  cuts may pass through the edges of the ring too.

The basic idea is to bound all the items of a ring to a bounding box $B$ and $O(1)$ number of open corridors with at most 3 bends such that the box is itself guillotine separable from the rest of the knapsack with guillotine cuts along the edges of $B$. We follow an iterative approach to define bounding box $B$. Clearly obtaining all four type of cuts will result in a box  bounded by these cuts which contains a smaller boundary ring. Thus our iterative algorithms halts when either ($i$) all four type of cuts are obtained, or ($ii$) when one of the subcorridors $S_{1}$, $S_{2}$, $S_{3}$, $S_{4}$ is exhausted (as previously, by exhausted we mean that there is no rectangle left in that subcorridor after a step of our iterative procedure in the new smaller subpiece),  or ($iii$) the corridor is divided into smaller open corridors by different type of cut other than the four types defined above.\\
We now formally define the iterative approach to find the bounding box. During the iterative procedure we will be adding rectangles to a 3 bend corridor $U'$(can be degenerate too) which we assume w.l.o.g.~to be coming from $S_{1},S_{2},S_{3}$, as in Figure \ref{ringproc}. That is w.l.o.g.~we assume that Type 4 cut doesn't come before other type of cuts. Considering the type of end-to-end guillotine cut in the subpiece do the following processing:
\begin{enumerate}
\item Case $1$: (Type $1$ cut) Add the items on left subpiece that are part of the ring, to the left-vertical subcorridor of the 3-bend corridor $U'$. Consider the new-subpiece to be the right-subpiece. Stop the iterative procedure if $S_{1}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new-subpiece. 
\item Case $2$: (Type $2$ cut) Add the items on bottom subpiece that are part of the ring,  to the horizontal subcorridor of $U'$. Consider the new-subpiece to be the top-subpiece. Stop the iterative procedure if $S_{2}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new-subpiece.
\item Case $3$: (Type $3$ cut) Add the items on the right subpiece that are part of the ring, to the right-vertical subcorridor of $U'$. Consider the new-subpiece to be the left-subpiece. Stop the iterative procedure if $S_{3}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new-subpiece.
\item  Case $4$: (Type $4$ cut) Pack the items of top subpiece in a new horizontal container $C$. Stop the iterative procedure. In this case we have $O(1)$ corridors and a box bounding the smaller ring whose edges are formed due to type cuts.
\item Case $5$: (Cuts perpendicular to the orientation of the subcorridors) Ring in the current subpiece is divided into 2 $\Uc$-corridors. Stop the iterative procedure.
\item Case $6$: (Cuts which don't pass through the ring) Continue only on the newly created subpiece that contains the ring,  ignore the other subpiece.
\end{enumerate}
The iterative algorithm stops in Case 5 or Case 4 or when one of the subcorridors get eventually exhausted by a type of cut. 
Each of the halting conditions results into $O(1)$ number of open corridors and possibly a box bounding a ring. 

\arir{I guess, in case 5 we get 2-$\Uc$, case 4 we get 1 $\Uc$, 1 $\Bc$ and a Box, Other cases 1 $\Uc$, 1 $\Bc$ but no box.}
%Hence we prove Lemma \ref{ringlem}.		
\end{proof}




\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,4) -- (0,0) -- (6,0) -- (6,4) --( 0,4);
			\draw[thick] (1,3)--(5,3) -- (5,1) -- (1,1) -- (1,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,1.25) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};
			\draw (2.5,3.7) node {\large \textbf{$S_{4}$}};


			\draw (1,4.7) node {\large \textbf{Type 1}};
			\draw (6.9,.45) node {\large \textbf{Type 2}};
			\draw (6,4.7) node {\large \textbf{Type 3}};
			\draw (6.9,3.2) node {\large \textbf{Type 4}};

			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,4.5) -- ( .5,0) ;
			\draw[dotted] (.25,4.5) -- ( .25,0) ;
			
			\draw[dotted] (0,.5) -- ( 6.5,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0) ;
			\draw[dotted] (5.25,4) -- ( 5.25,0) ;

			\draw[dotted] (0,3.5) -- ( 6,3.5) ;
			\draw[dotted] (0,3.25) -- ( 6.5,3.25) ;
				
		
		\end{tikzpicture}}
		\caption{Types of cuts}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,5) -- (1,1) -- (7,1) -- (7,5) --(1,5);
			\draw[thick] (2,4)--(6,4)-- (6,2) -- (2,2) -- (2,4) ;
			\draw[thick]  (1.5,1.5) -- (1.5,6) ;% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[thick] (6.5,4.5)--(1.5,4.5);
			\draw[pattern=north east lines, pattern color=black] (6.5,4.5)--(6.5,5)--(1.5,5)--(1.5,4.5)--(6.5,4.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,5) -- (1.5,5) -- (1.5,1.5) -- (6.5,1.5) -- (6.5,5) --(7,5) -- (7,1)--(1,1)--(1,5);		

			\draw (4,1.25) node {\large \textbf{$U'$}};
			\draw (5,4.75) node {\large \textbf{$C$}};
			\draw (4,3) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Final Bounding Box of $S$}
	\end{subfigure}
	\caption{Processing 3-bend corridor}
	\label{ringproc}
\end{figure}



		\begin{thm}
		\label{3max}
		Any  corridor $C$ can be converted into $O_{\eps}(1)$ corridors of type $\Bc, \Lc, \Uc, \Gc$, maintaining guillotine separability.
		\end{thm}
		\begin{proof}W.l.o.g. assume $C$ has no $\Zc$-bends (else apply Lemma \ref{}) and more than 3 bends. There are 2 cases. 
		
\noindent {\em Case 1. } $C$ is an open corridor.  W.l.o.g~assume $C$ has 4 bends.  \ari{Similar argument holds for other corridors with greater than 4 bends.} We also assume $S_{1}$ to be longer in length than $S_{3}$ (see Figure \ref{bends}).  We follow an iterative approach to partition the corridor $C$  into $O_{\epsl}(1)$ open corridors with at most 3 bends. During the iterative procedure we will be adding rectangles to a $\Gc$-corridor $G'$ (can be degenerate too) which we assume to be coming from $S_{1},S_{2},S_{3},S_{4}$. Considering the type of end-to-end guillotine cut through the corridor $C$ do the following processing:
\begin{enumerate}
\item Case $1$: Cut passes through a subcorridor perpendicular to the orientation of that subcorridor. 
We get two corridors with smaller number of bends. If they have at most 3 bends, we stop. Otherwise, we continue iteratively with the smaller corridors.
%Portion of the corridor $C$ which isn't part of corridor $G'$ gets divided into at most 4 open corridors with at most 3 bends. Stop the iterative procedure.
\item Case $2$ : $V_{S_1}$ cut (Vertical guillotine cut through $S_{1}$). Add the items left of $V_{S_1}$ cut which are part of the corridor $C$ to the leftmost-vertical subcorridor of the 4-bend corridor $G'$.  Stop the iterative procedure if $S_{1}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise continue the iterative procedure on the remaining portion of the corridor $C$ which is not part of $G'$.
\item Case $3$ : $H_{S_2}$ cut (Horizontal guillotine cut through $S_{2}$). Add the items below $H_{S_2}$ cut to the bottommost-horizontal subcorridor of $G'$. Stop the iterative procedure if $S_{2}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise continue the iterative procedure on the remaining portion of the corridor $C$ which is not part of $G'$.
\item Case $4$ : $V_{S_3}$ cut (Vertical guillotine cut through $S_{3}$). Add the items right of $V_{S_3}$ cut  to the rightmost-vertical subcorridor of $G'$.  Stop the iterative procedure if $S_{3}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new subpieces.
\item  Case $5$ : $H_{S_4}$ cut (Horizontal guillotine cut through $S_{4}$). Add the items above $H_{S_4}$ cut  to the topmost-horizontal subcorridor of $G'$. Stop the iterative procedure if $S_{4}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise continue the iterative procedure on the remaining portion of the corridor $C$ which is not part of $G'$.
\end{enumerate}
Thus our iterative algorithms halts when one of the subcorridors $S_{1}$, $S_{2}$, $S_{3}$, $S_{4}$ is exhausted (by exhausted we mean that there is all rectangles of that subcorridor is packed in $G'$ after a step of our iterative procedure)  or when the portion of corridor $C$ which isn't part of $G'$ is divided into at most 4 open corridors with at most 3 bends as in Case 1. This iterative algorithm halts otherwise one of the type cuts will eventually exhaust a subcorridor as the number of cuts in the guillotine cutting sequence is finite. Each of the halting conditions results into $O(1)$ open corridors. 

\noindent {\em Case 2.} $C$ is a ring (see Figure \ref{rings}). Then consider the bounding box $\mathcal{B}$ (if any) which contains a smaller ring as shown in Lemma \ref{ringlem}. For the remainder of the proof by {\em freezing} a rectangle we mean that the rectangle is not moved while rearranging other rectangles. 
If there is any end to end cut which passes through only two subcorridors of same orientation then we can divide the corridor into 2 corridors each having 3 bends. So we now assume that there is no such end to end cut in $\mathcal{B}$. 
Now consider the sequence of guillotine cuts which separate the rectangles in the ring. If we are cutting through leftmost vertical subcorridor or bottom most horizontal subcorridors then we freeze these rectangles. Now in the remaining portion of the box if there is a cut $l_{1}$ through rightmost vertical subcorridor and the distance between $l_{1}$ and edge of the boundary to the right of it be $d$ then we remove the strip $S$ to the right of $l_{1}$. Then we shift the rest of items of box to the right which isn't frozen by a distance of $d$. Now in the empty region created near the left edge of the box we place the strip $S$ which we removed. Now freeze the rectangles in the strip $S$. Do the same process if there is a cut through the upper most horizontal corridor and now instead of shifting  the strip situated above the cut to the left we shift it down by appropriating shifting the remaining portion of the box upwards which isn't still frozen. Note that guillotine separability remains preserved by this rearrangement.
Continue this process till we convert these into single boundary-$\Lc$. We stop when we exhaust all rectangles or we find a cut that divides the ring into two corridors with 3 bends at most. Then we have a box with boundary-$\Lc$ and possibly 2 smaller boxes each containing corridors with at most 3 bends. This completes our proof.
\end{proof}


==> 4_Corridor_Decomposition_comments.tex <==
\section{$\Bc \Lc$-decomposition for guillotine packing} \label{sec:bl}
In this section we will show that we can have a better decomposition of the optimal guillotine packing.
We will show the existence of a corridor-decomposition where all corridors are either $\Bc$ or $\Lc$s.	
We will prove the main strcutural result as follows:	
\begin{thm}
\label{thm:ldecom}
There exists a corridor partition (we call it $\Bc \Lc$-decomposition) and $\optco \subseteq \optsk$ such that:
\begin{enumerate}\itemsep0pt
\item there is a subset $\optco^{cross} \subseteq \optco$ with  $|\optco^{cross}| \le O_\eps(1)$ such that  each $i\in \optco \setminus \optco^{cross}$ is fully contained in some corridor,
\item $\profit(\optco) \ge (1-O(\eps))\profit(\optsk)$,
\item the number of corridors is $O_{\eps,\epsl}(1)$ and each corridor is either $\Bc$ or $\Lc$ corridor with width at most $\epsl N$.
\end{enumerate}
\end{thm}		
	
To prove the theorem, first we will start with the corridor decomposition from Lemma \ref{lem:corridorPack}. Then process the $\Zc$-bends in the corridors to obtain only spiral corridors. Thereafter, we will further process to obtain spiral corridors with bends at most 4. Finally we will process $\Uc$ and $\Gc$ corridors to obtain only $\Lc$ or $\Bc$ corridors. 

\begin{obs} \label{endtoend}
Given a piece containing a set of guillotine separable rectangles, there must exist an end-to-end guillotine cut in the piece. In other words, the first level of guillotine cuts in the piece is end-to-end.
\end{obs}
We follow some terminologies in the remainder of the section. We define subpiece $P$ completely containing corridor $C$ as \textit{smallest} if the piece $P$ which is obtained from the sequence of guillotine cuts has no previous cut that passed through the corridor $C$ and the next end to end cut in $P$ passes through $C$. We also define \textit{box $B$ bounding} a set of rectangles as a subpiece which is guillotine separable from the rest of the piece. In other ways $B$ if considered as a pseudo-rectangle, forms a guillotine separable arrangement with the rest of the items of knapsack. In the rest of the section, by \emph{freezing} a rectangle, we mean that the rectangle is not moved while shifting other rectangles. A subcorridor $S_{1}$ is said to be \emph{exhausted} if there is no rectangle from $S_{1}$ in the smaller subpiece on which we would running our recursive procedure in the following section. A box $B$ is said to be \emph{bounding} a corridor with atleast one bend if the outermost corners at the bends of the corridor coincides with the corners of the box.
	
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Explaination of Algorithm \ref{sepalgo}}
 Let $C$ have $k$ subcorridors $\{ S_{1},S_{2},S_{3},...,S_{k}\}$ such that $\forall i \in [k-1]$, $S_{i}$ and $S_{i+1}$ share a region $S_{i,i+1}$ with each other. Suppose that we are asked to separate out a smaller spiral corridor $C'$ with atmost 3 bends (number of bends in $C'$ is denoted by $b(C')$) from a corridor $C$ with $C'$. $\forall c\in[b(C')]$, subcorridor $S_{i'+c}$  contributes items to the subcorridor $S_{c}'$ of $C'$ . Consider a sequence of guillotine cuts through subcorridors $S_{i'},..S_{i'+c}$ such that these cuts are parallel to the orientation of the subcorridor and these occured before the halting condition was satisfied. Consider the set of cuts which occured last in their respective subcorridors. These cuts clearly divide separates $C'$ from $C$. This process clearly depicted in Figure \ref{ringproc} where we want to seperate out $U'$ from the original corridor.

Still work left to be done in this subsection.
\begin{algorithm}
\caption{Algo-separate($C,List,Halting Conditions$)}\label{sepalgo}
\begin{algorithmic}[1]
\STATE $k \gets 1$
\WHILE {(No Halting Condition is satisfied)}
\STATE Do Guillotine cuts of Stage-$k$
\ENDWHILE
\STATE Consider the set of cuts parallel to the orientation of Subcorridors in $List$ which occured last in their respective subcorridors.
\STATE Use the cuts in the previous step to separate out the spiral corridor $C'$ (contains from the items in $List$, some corridors can be degenerate too which when not considered may lead to $O(1)$ spiral corridors) from $C$
\STATE Return the Halting Condition which got satisfied in While Loop along with the $C'$
\end{algorithmic}
\end{algorithm}
\begin{algorithm}
\caption{Algo-Box-Creation($C$)}\label{boxalgo}
\begin{algorithmic}[1]
\STATE Separate out rectangles into corridor $C'$ until you get one rectangle from each subcorridor of $C$
 \IF {(Halting Condition == One rectangle obtained from each subcorridor in $C$)}
\STATE			Create a bounding box using the edges of the subpiece which contains the portion excluding $C'$ when atleast one rectangle from each corridor of $C$ was separated out into $C'$.
\STATE Let $S_{i}$ be the last corridor from which a rectangle was separated. Make $S_{i}'$ (\ama{Please define what you mean by $S_{i}'$, i guess $S_{i}'=S_{i}\cap C'$}) as a $B-Corridor$ . Let the corridor formed due to $S_{1}',..,S_{i-1}'$ (\ama{same here please define whats S'}) be $C_{1}$ if $i>1$. Let the corridor formed due to $S_{i+1}',..,S_{c}'$ be $C_{2}$ if $i<c$.
\IF{$i >2$} 
\STATE Algo-Box-Creation($C_{1}$)
\ENDIF 
\IF{$i<c-1$}
\STATE Algo-Box-Creation($C_{2}$)
\ENDIF
\ENDIF
\IF{(Halting Condition == Presence of Cut $l$ perpendicular to the orientation of a subcorridor (doesn't pass through interior of shared region) in $C$)}
\STATE Partition the existing corridors into smaller corridors using the cut $l$
\STATE Call the function Algo-Box-Creation($C''$) for all corridor $C''$ created from $C$ after cut $l$ except the $B-Corridor$.   
\ENDIF		 
\end{algorithmic}
\end{algorithm}
\begin{algorithm}
\caption{Algo-Boundary-L($Box,C$)}\label{Lalgo}
\begin{algorithmic}[1]
\STATE Consider a sequence of guillotine cuts to separate the rectangles in $C$ where $C$ is a boundary corridor.
\STATE While doing Step 1, consider consider each strip separated due to cut as a pseudo item. Consiser the subpiece left after all the  guillotines in Step 1 as a pseudoitem $B$. 
\STATE Remove $B$ and rearrange the remaining pseudoitems to get a boundary-$\Lc$ as done in Section \ref{glp}.
\STATE Place $B$ in the empty region left.   
\end{algorithmic}
\end{algorithm}
\begin{algorithm}
\caption{Algo-Spiral($C$)}\label{spialgo}
\begin{algorithmic}[1]
\STATE Let $List$ be the set of subcorridors containing the leftmost, bottommost, rightmost and topmost subcorridor
\STATE Algo-separate($C,List$,Presence of Cut $l$ perpendicular to the orientation of a subcorridor (doesn't pass through interior of shared region) in $C$)\label{spi2}
\STATE Partition the existing corridors after the previous step into smaller corridors using the cut $l$\label{spi1}
\STATE Call the function Algo-Spiral($C''$) for all corridor $C''$ created from $C$ after Step \ref{spi1} and Step \ref{spi2}  iff $b(C'')>3$.
\end {algorithmic}
\end{algorithm}
\subsection{Obtaining corridors of types $\Bc, \Lc, \Uc, \Gc$} 
\label{subsec:blug}

\begin{comment}
		\begin{figure}
			\captionsetup[subfigure]{justification=centering}
			\hspace{-15pt}
			
				\centering
				\resizebox{!}{4cm}{
					\begin{tikzpicture}					
					\draw[solid] (0,6) rectangle (2,10);
					\draw[solid, fill=lightgray] (0,4) rectangle (2,6);
					\draw[solid] (2,4) rectangle (8,6);
					\draw[solid, fill=lightgray] (8,4) rectangle (10,6);
					\draw[solid] (8,0) rectangle (10,4);
		
					\draw (1,8) node {\large \textbf{$S_{1}$}};
					\draw (1,5) node {\large \textbf{$S_{12}$}};
					\draw (6,5) node {\large \textbf{$S_{2}$}};
					\draw (9,5) node {\large \textbf{$S_{23}$}};
					\draw (9,2) node {\large \textbf{$S_{3}$}};
		
					\end{tikzpicture}}
				\caption{Corridor C consisting of subcorridors $S_{1},S_{2},S_{3}$ and overlapping regions of the subcorridors $S_{12}$  and  $S_{23}$.}
				\label{zstructure}
		\end{figure}
		
\end{comment}	
	
\subsubsection{Obtaining spiral corridors}
\begin{comment}
First, we show how to process $\Zc$-bends. 

\begin{lem}
\label{theorem1}
Any $\Zc$-corridor $C$ can be decomposed into $O(\frac{1}{\epsl})$. corridors of type $\Bc$ or $\Lc$. 
\end{lem}
\begin{proof}
W.l.o.g.~assume the center-sc of $C$ to be horizontal (See Figure \ref{zstructure}). 
%Region $S_{12}$ is shared by subcorridors $S_{1}$ and $S_{2}$ and similar convention holds for $S_{23}$. 
Consider the guillotine cutting sequence of all rectangles in the knapsack. 
Let $P$ be the smallest piece containing $C$, i.e., the next guillotine cut in $P$ passes through $C$. 
Now we will consider the guillotine cutting  sequence of rectangles in $P$ to iteratively decompose the $\Zc$-corridor into one of the three subcases: ($i$) into two $\Lc$-corridors, or ($ii$) a $\Bc$-corridor and an  $\Lc$-corridor, or ($iii$) a $\Bc$-corridor and a smaller $\Zc$-corridor.  
We stop when we reach subcases ($i$) or ($ii$). Otherwise in subcase ($iii$), we continue iteratively. 
This sequence can have five types of cuts:
\begin{itemize}
\item {\em HS}: horizontal guillotine cut which passes through a side-sc but doesn't pass through center-sc,
%\item Cut 2: horizontal guillotine cut which passes through $S_{3}$ and doesn't pass through $S_{23}$,
\item {\em VS}: vertical guillotine cut which passes through a side-sc,
%\item Cut 4: vertical guillotine cut which passes through $S_{3}$,
\item  {\em VC}: vertical guillotine cut which passes through center-sc but doesn't pass through any side-sc,
\item {\em HC}: horizontal guillotine cut which passes through center-sc,
\item {\em NC}: cut which doesn't pass through $\Zc$-corridor.
\end{itemize}
Now, if we get cuts of type  {\em VC} (or {\em HC}) at any subpiece, we are in case $(i)$ as we obtain 2 $\Lc$-corridors. 
On the other hand, if we get {\em NC}-type cut we just focus on the subpiece containing the  $\Zc$-corridor of the present iteration.
If we have either cuts of type {\em VS} (or {\em HS}) passing through a side-sc then we are dividing the $\Zc$-bend into a rectangular region and a smaller $\Zc$-corridor. 
If there are no rectangle left in one of the side-sc of the smaller $\Zc$-corridor, we call the subcorridor to be {\em exhausted}. In case of exhaustion of a subcorridor, we reach case $(ii)$ as the smaller $\Zc$-corridor can be considered as an $\Lc$-corridor by ignoring the exhausted side-sc.
Otherwise, we are in case $(iii)$. 
The rectangles in side-sc have height $\ge \epsl N$, so the consecutive cuts of {\em HS} creating $\Bc$-corridor have to be at a distance of atleast $\epsl N$. This ensures that the number of such corridors is $O(\frac{1}{\epsl})$. 
Note that we can merge all the adjacent rectangular regions obtained due to successive cuts of {\em VS} into a $\Bc$-corridor of same height till we arrive at a cut of different type (excluding {\em NC}). And since the number of cuts excluding {\em VS} and {\em NC} is $O(\frac{1}{\epsl})$, therefore number of such $\Bc$-corridors created due to successive cuts of {\em VS} is $O(\frac{1}{\epsl})$. 
\end{proof}
\end{comment}
\arir{need to add a figure. }


\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,6)--(2,6)--(2,5.5)--(4,5.5)--(4,6)--(6,6)--(6,4)--(5,4)--(5,3)--(4.5,3)--(4.5,4.5)--(5.5,4.5)--(5.5,5.5)--(4.5,5.5)--(4.5,5)--(1.5,5)--(1.5,5.5)--(.5,5.5)--(.5,4)--(2,4)--(2,3)--(4,3)--(4,2.5)--(1.5,2.5)--(1.5,3.5)--(0,3.5)--(0,6);		
						
						\draw[dotted] (6,4)--(5.5,4.5);
						\draw[dotted] (5,4)--(4.5,4.5);
						\draw[dotted] (6,6)--(5.5,5.5);
						\draw[dotted] (4,6)--(4.5,5.5);
						\draw[dotted] (2,6)--(1.5,5.5);
						\draw[dotted] (0,6)--(.5,5.5);
						\draw[dotted] (0.25,3.6)--(.5,4);
						\draw[dotted] (1.5,2.5)--(2,3);
						\draw[dotted] (1.5, 3.5)--(2,4);
						\draw[dotted] (1.5, 5)--(2,5.5);
						\draw[dotted] (4.5 , 5)--(4,5.5);

						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.4,3.5);	\draw (-.75,3.5) node {\textbf{$l_{i'+2}$}};
						\draw[->] (1,5.75) edge[out=90,in=0,->] (.8,6.5);	\draw (.5,6.5) node {\textbf{$l_{i'+1}$}};
						%\draw (1.75,5.25) node {\textbf{$l_{1}$}};
						%\draw (4.25, 5.25) node {\textbf{$l_{2}$}{spialgo}};
						%\draw[->] (5,5.75) edge[out=180,in=0,->] (4.75,6.5);	\draw (4.5,6.5) node {\textbf{$l$}};%
%						\draw[->] (5.75,5) edge[out=180,in=0,->] (6.5,5);	\draw (6.5,5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
						\fill [lightgray] (0,3.5) rectangle (0.5,4);
						\draw[->] (.2,3.75) edge[out=180,in=0,->] (-.4,2.5);	\draw (-.75,2.5) node {\textbf{$S_{i'+2,i'+3}$}};
						\draw[dashed] (4.75,3) -- ( 4.75 ,4.25) -- ( 5.75, 4.25) -- ( 5.75, 5.75) -- ( 4.25, 5.75) -- ( 4.25, 5.25) -- ( 1.75, 5.25) -- ( 1.75, 5.75) -- (.25, 5.75) -- (.25, 3.5) ;	
						%\draw (4,1.25) node {\large \textbf{$U'$}};
						%\draw (5,4.75) node {\large \textbf{$C$}};
						%\draw (4,3) node {\large \textbf{$B$}};
		
		\end{tikzpicture}}
		\caption{k-bend Corridor Processing}
		\label{fig:kbend}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,7)--(2,7)--(2,4)--(7,4)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw  (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7) --(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
					
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};


						\draw[dashed] (5.6,.5)--(5.6,4);
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend}
	\end{subfigure}
	\caption{}
\end{figure}



%\begin{figure}
%			\captionsetup[subfigure]{justification=centering}
%			\hspace{-15pt}
%			
%				\centering
%				\resizebox{!}{6cm}{
%					\begin{tikzpicture}					
%						\draw[thick] (0,6)--(2,6)--(2,5.5)--(4,5.5)--(4,6)--(6,6)--(6,4)--(5,4)--(5,3)--(4.5,3)--(4.5,4.5)--(5.5,4.5)--(5.5,5.5)--(4.5,5.5)--(4.5,5)--(1.5,5)--(1.5,5.5)--(.5,5.5)--(.5,4)--(2,4)--(2,3)--(4,3)--(4,2.5)--(1.5,2.5)--(1.5,3.5)--(0,3.5)--(0,6);		
%						
%						\draw[dotted] (6,4)--(5.5,4.5);
%						\draw[dotted] (5,4)--(4.5,4.5);
%						\draw[dotted] (6,6)--(5.5,5.5);
%						\draw[dotted] (4,6)--(4.5,5.5);
%						\draw[dotted] (2,6)--(1.5,5.5);
%						\draw[dotted] (0,6)--(.5,5.5);
%						\draw[dotted] (0.25,3.6)--(.5,4);
%						\draw[dotted] (1.5,2.5)--(2,3);
%						\draw[dotted] (1.5, 3.5)--(2,4);
%						\draw[dotted] (1.5, 5)--(2,5.5);
%						\draw[dotted] (4.5 , 5)--(4,5.5);
%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.4,3.5);	\draw (-.75,3.5) node {\textbf{$l_{i'+1}$}};
%						\draw[->] (1,5.75) edge[out=90,in=0,->] (.8,6.5);	\draw (.5,6.5) node {\textbf{$l_{i'+2}$}};
%						%\draw (1.75,5.25) node {\textbf{$l_{1}$}};
%						%\draw (4.25, 5.25) node {\textbf{$l_{2}$}};
%						%\draw[->] (5,5.75) edge[out=180,in=0,->] (4.75,6.5);	\draw (4.5,6.5) node {\textbf{$l$}};%
%%						\draw[->] (5.75,5) edge[out=180,in=0,->] (6.5,5);	\draw (6.5,5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%						\fill [lightgray] (0,3.5) rectangle (0.5,4);
%						\draw[->] (.2,3.75) edge[out=180,in=0,->] (-.4,2.5);	\draw (-.75,2.5) node {\textbf{$S_{i'+2,i'+3}$}};
%						\draw[dashed] (4.75,3) -- ( 4.75 ,4.25) -- ( 5.75, 4.25) -- ( 5.75, 5.75) -- ( 4.25, 5.75) -- ( 4.25, 5.25) -- ( 1.75, 5.25) -- ( 1.75, 5.75) -- (.25, 5.75) -- (.25, 3.5) ;	
%						%\draw (4,1.25) node {\large \textbf{$U'$}};
%						%\draw (5,4.75) node {\large \textbf{$C$}};
%						%\draw (4,3) node {\large \textbf{$B$}};
%					\end{tikzpicture}}
%				\caption{k-bend Corridor Processing}
%				\label{fig:kbend}
%		\end{figure}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,7)--(7,7)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw  (.75,6.25)--(6.25,6.25)--(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,0.5)--(5,0.5)--(5,0)--(7,0)--(7,7)--(0,7)--(0,3);
						
					
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};

						
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend1}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw  (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[pattern=north west lines, pattern color=gray] (5,.75)--(6.25,.75)--(6.25,0)--(5,0)--(5,.75);
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};
						

						
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend2}
	\end{subfigure}
	
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,7)--(7,7)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw  (.75,6.25)--(6.25,6.25)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,2)--(7,2)--(7,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
					
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};

						
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend3}
	\end{subfigure}
\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
						\draw[thick] (0,5)--(0.75,5)--(0.75,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,5);
						\draw  (.75,4.5)--(1.25,4.5)--(1.25,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,4.5); 	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,5)--(0,5)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (0.75,6.5)--(2,6.5)--(2,7)--(0.75,7)--(0.75,6.5);
						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
						\draw (.3,4.75) node {\large \textbf{$S_{1}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{4}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{3}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{2}$}};
						

						
	
		\end{tikzpicture}}
		\caption{Bounding Box of $S$ and Corridors with lesser number of bends}
		\label{fig:zbend4}
	\end{subfigure} 
	\caption{}\label{closedcor2}	
\end{figure}

\begin{lem}\label{noz}
%A non-spiral corridor $C$ can be decomposed  into $O_{\eps}(1)$ spiral corridors and $O_{\eps}(1)$ $\Zc$-corridors by dropping atmost $O_{\eps,\epsl}(1)$ rectangles. 
A corridor with one or more $\Zc$ bends can be partitioned into $O_{\eps}(1)$ spiral corridors  by removing $O_{\eps,\epsl}(1)$ items, maintaining guillotine separability.
\end{lem}
\arir{write this proof and figure appropriately.}
\begin{proof}
There are two cases. 

\noindent \textit{Case 1: $C$ is open corridor with at least one $\Zc$-bend.} Let $C$ have $k$ subcorridors $\{ S_{1},S_{2},S_{3},...,S_{k}\}$ such that $\forall i \in [k-1]$, $S_{i}$ and $S_{i+1}$ share a region $S_{i,i+1}$ with each other. Assume there are 5 subcorridors ( if there are less than 5 subcorridors the following proof would still hold \ama{Please explain a bit, why?} ) $S_{i'+1}, S_{i'+2}, S_{i'+3}, S_{i'+4} $ and $S_{i'+5}$ such that $\{S_{i'+2},S_{i'+3},S_{i'+4}\}$ form a $\Zc$ bend. Let $S_{i'+3}$ be a horizontal subcorridor and $S_{i'+2}$ be situated to the top left of $S_{i'+3}$. Let us consider a sequence of guillotine cuts through the five subcorridors  $S_{i'+1}, S_{i'+2}, S_{i'+3}, S_{i'+4} $ and $S_{i'+5}$.\\
After a sequence of guillotine cuts through corridor $C$ (including those which is coincident with the edges of $C$) , we get our first cut $l'$ which passes through the unshared region of $S_{i'+3}$ ( \amar{cut should be along the orientation of $S_{i'+3}$, else we already get smaller corridors}). Now consider the guillotine cuts which occured before the cut $l'$. Let $l_{i'+2}$ be the rightmost vertical cut (including those which pass through the boundary of $S_{i'+2,i'+3}$ if any) through $S_{i'+2,i'+3}$. Extend the cut $l_{i'+2}$ so that it touches the boundary curve between $S_{i'+1}$ and $S_{i'+2}$ at point $P$. Now draw a line $l_{i'+1}$ from point $P$ parallel to the orientation of $S_{i'+1}$ till it touches the boundary curve between $S_{i'+1}$ and $S_{i'}$. Continue the same process by drawing lines $l_{j}$ through corridors $S_{j}$ where $1 \leq j \leq i'$ in similar fashion. Stop drawing these lines when we draw a line $l_{1}$ through $S_{1}$ parallel to the orientation of $S_{1}$ and reach its boundary edge.   Lines $\{l_{1},l_{2},..,l_{i'+2}\}$ partitions the corridor $C$ into atmost 2 smaller corridors $C_{1},C_{2}$ as shown in Figure \ref{fig:kbend}\amar{seems like the figure's missing some notations}. $C_{1}$ contains rectangles from the subcorridors $S_{1},..,S_{i'+2}$ only. $C_{2}$ contains rectangles from the subcorridors $S_{1},...,S_{k}$ (maynot contain rectangles from every subcorridor). In a similar way we can partition $C_{2}$ into atmost 2 corridors $C_{3}$ and $C_{4}$ where $C_{3}$ contains rectangles from the subcorridors $S_{i'+4},..,S_{k}$ only \amar{we can have items from $S_{i'+3}$ here} and $C_{4}$ contains rectangles from the subcorridors $S_{1},...,S_{k}$ (maynot contain rectangles from every subcorridor). During this process of partitioning we drop atmost $O_{\eps,\epsl}(1)$ rectangles. Now suppose that the first cut through $S_{3}$ \amar{$S_{3} or S_{i'+3}$?} only is a horizontal cut. This divides the $C_{4}$ into 2 corridors containing atleast one lesser $\Zc$ bend when compared to $C$. Note that the reason for choosing $l_{i'+2}$ and extending it to partition the corridor $C$ is that $l_{i'+2}$ is the cut which intercepts the horizontal cut $l'$ in the shared region $S_{i'+2,i'+3}$ and hence it enables us to partition $C_{4}$ into 2 corridors using $l'$. Similarly if the first cut through $S_{3}$ only was vertical, then we can partition $C_{4}$ using the vertical cut into 2 corridors, each containing atleast one lesser $\Zc$ bend when compared to $C$.\\
Doing the above procedure for all $\Zc$ bends concludes the proof for case 1.

%Now let us consider the second subcase where we dont have any cut in the guillotine cutting sequence which passes through the region of $S_{3}$ which is not part of any other subcorridor and neither $S_{i'+2}$ nor $S_{i'+4}$ has a horizontal cut passing through the unshared regions of these subcorridors. If $S_{i'+2}$ gets exhausted during the guillotine cutting sequence then we simply divide the corridor $C$ into 2 corridors $C_{1'}$ and $C_{2'}$ such that $C_{1'}$ contains rectangles from  the subcorridors $S_{1},..,S_{i'+2}$ only and $C_{2'}$ contains rectangles from the subcorridors $S_{i'+3},...,S_{k}$ only. Similar partitioning can be done if $S_{i'+4}$ gets exhausted. Otherwise eventually due to the sequence of guillotine cuts $S_{i'+1}$ and $S_{i'+5}$ will be exhausted. Then we can partition $C$ into 3 corridors $C_{1''}$,$C_{2''}$ and $C_{3''}$ in similar fashion as we did in the previous subcase (which was done previously using the lines $\{l_{1},l_{2},..,l_{i'+2}\}$). $C_{1''}$ contains rectangles from the subcorridors $S_{1},..,S_{i'+2}$, $C_{2''}$ contains rectangles from the subcorridors $S_{i'+4},..,S_{k}$, $C_{3''}$ contains rectangles from the subcorridors $S_{i'+2},S_{i'+3},S_{i'+4}$.\\

%Now let us consider the last case where we dont have any cut in the guillotine cutting sequence which passes through the region of $S_{3}$ which is not part of any other subcorridor and either $S_{i'+2}$ or $S_{i'+4}$ has a horizontal cut passing through the unshared regions of these subcorridors.Let us assume that we have a horizontal cut through the unshared region of $S_{i'+2}$. Let $l_{v'}$ be the last vertical cut through $S_{i'+2,i'+3}$ before the first horizontal cut $l_{h}$ through $S_{i'+2}$ only. Let $l_{h'}$ be the part of $l_{h}$ which is inside $S_{i'+2}$. Extend $l_{v'}$ to meet the boundary curve between $S_{i'+2}$ and $S_{i'+1}$. Then continue making lines parallel to the orientation to the subcorridors $S_{i'+1},S_{i'},...,S_{1}$ as done in the previous subcase. Then using the lines created and $l_{h'}$ we can divide $C$ into 3 corridors $C_{1'''},C_{2'''},C_{3'''}$. $C_{1'''}$ and $C_{2'''}$ contains rectangles from the subcorridors $S_{1},..,S_{i'+2}$ only. $C_{3'''}$ contains rectangles from the subcorridor $S_{i'+2},...,S_{k}$. If there is a horizontal cut through the unshared region of $S_{i'+4}$ then we can partition $C_{3'''}$ into $C_{4'''}, C_{5'''},C_{6'''}$ where $C_{4'''}$ and $C_{5'''}$ contains rectangles from the subcorridors $S_{i'+4},..,S_{k}$,  $C_{6'''}$ contains rectangles from the subcorridors $S_{i'+2},S_{i'+3},S_{i'+4}$. Otherwise $C_{3'''}$ is handled appropriately in subcase 2.\\


\noindent \textit{Case 2: $C$ is a closed corridor with at least one $\Zc$-bend.}  Let $S_{1}$ be the leftmost vertical subcorridor in $C$, $S_{2}$ be the bottommost horizontal subcorridor in $C$, $S_{3}$ be the rightmost vertical subcorridor in $C$, $S_{4}$ be the topmost subcorridor in $C$.  Depending on the arrangement of these four subcorridors $\{S_{1},S_{2},S_{3},S_{4}\}$ we separate out the rectangles from these 4 subcorridors during guillotine cutting sequence into atmost 4 spiral corridors with atmost 4 bends as shown in Figure \ref{fig:zbend} and Figure  \ref{closedcor2}. Items are packed into $\Gc$ corridor if the 4 subcorridors  $\{S_{1},S_{2},S_{3},S_{4}\}$ form a $\Gc$ corridor among themselves. Similarly items are packed into a $\Uc$ corridor or $\Lc$ corridors or $\Bc$-corridors depending upon the arrangement of corridors among themselves. During the sequence of guillotine cuts if there is a cut which passes through the unshared region of subcorridor perpendicular to it's orientation then it clearly divides the subcorridor into $O_{\eps}(1)$ open corridors with atmost $O_{\eps}(1)$ which is handled in Case 1 as shown in Figure \ref{fig:zbend}. Otherwise if we don't have such cut then eventually one of the subcorridors  $\{S_{1},S_{2},S_{3},S_{4}\}$ is exhausted as the items are being added continuously to the $O(1)$ spiral corridors with atmost 4 bends. So, we are left with $O(1)$ open corridors as shown in Figure \ref{fig:zbend2} which is again dealt in Case 1. This concludes our proof.    
\end{proof}

\begin{comment}
\begin{lem}\label{no_z}
A corridor with one or more $\Zc$ bends can be partitioned into $O_{\eps}(1)$ spiral corridors  by removing $O_{\eps,\epsl}(1)$ items, maintaining guillotine separability. 
\end{lem}
\begin{proof}
Follows from Lemma \ref{noz} and Theorem \ref{thm:ldecom}.  
\end{proof}
\end{comment}
		
%		
%\begin{figure}[t]
%			\captionsetup[subfigure]{justification=centering}
%			\hspace{-15pt}
%
%				\centering
%				\resizebox{!}{5cm}{
%					\begin{tikzpicture}
%		
%					\draw[thick] (0,6) -- (0,0) -- (12,0) -- (12,10) -- (4,10) -- (4,4) -- (6,4) -- (6,8) -- ( 10,8) -- (10,2) -- (2,2) -- (2,6) -- (0,6); 
%		
%					\draw (1,3) node {\large \textbf{$S_{1}$}};
%					\draw (6,1) node {\large \textbf{$S_{2}$}};
%					\draw (11,5) node {\large \textbf{$S_{3}$}};
%					\draw (8,9) node {\large \textbf{$S_{4}$}};
%					\draw (5,7) node {\large \textbf{$S_{5}$}};
%		
%					\end{tikzpicture}}
%				\caption{Corridors with more than 3 bends is not possible}
%				\label{bends}
%
%		\end{figure}
%\begin{figure}[t]
%			\captionsetup[subfigure]{justification=centering}
%			\hspace{-15pt}
%
%				\centering
%				\resizebox{!}{5cm}{
%					\begin{tikzpicture}
%		
%					\draw[thick](0,0) rectangle (12,12);
%					\draw[thick](2,2) rectangle (10,10);
%					\draw (1,6) node { \large \textbf{$S_{1}$}};
%					\draw (11,6) node { \large \textbf{$S_{3}$}};
%					\draw (6,1) node { \large \textbf{$S_{2}$}};	
%					\draw (6,11) node { \large \textbf{$S_{4}$}};
%					\end{tikzpicture}}
%				\caption{Ring can be converted into corridors without any $\Zc$ bend and consisting of atmost 3 bends.}
%				\label{rings}
%		\end{figure}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.5cm}{
			\begin{tikzpicture}
		
					\draw[thick] (0,6) -- (0,0) -- (12,0) -- (12,10) -- (4,10) -- (4,4) -- (6,4) -- (6,8) -- ( 10,8) -- (10,2) -- (2,2) -- (2,6) -- (0,6); 
		
					\draw (1,3) node {\large \textbf{$S_{1}$}};
					\draw (6,1) node {\large \textbf{$S_{2}$}};
					\draw (11,5) node {\large \textbf{$S_{3}$}};
					\draw (8,9) node {\large \textbf{$S_{4}$}};
					\draw (5,7) node {\large \textbf{$S_{5}$}};
		
					\end{tikzpicture}}
				\caption{Corridors with more than 3 bends is not possible}
				\label{bends}

	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.5cm}{
		\begin{tikzpicture}		
					\draw[thick](0,0) rectangle (12,12);
					\draw[thick](2,2) rectangle (10,10);
					\draw (1,6) node { \large \textbf{$S_{1}$}};
					\draw (11,6) node { \large \textbf{$S_{3}$}};
					\draw (6,1) node { \large \textbf{$S_{1}$}};	
					\draw (6,11) node { \large \textbf{$S_{1}$}};
					\end{tikzpicture}}
				\caption{Ring can be converted into corridors without any z bend and consisting of atmost 3 bends.}
				\label{rings}
	\end{subfigure}
	\caption{}
\end{figure}


\begin{cor}
Every closed corridor $C$ in corridor decomposition of guillotine separable set of items, obtained after the processing done Lemma \ref{noz}, is a ring.
\end{cor}
%\begin{proof} It follows from Corollary \ref{no_z} as there exists no corridor with $\Zc$ bend.
%\end{proof}


%%%%%%%%%%%%%%%%%
\subsubsection{Obtaining corridors with at most three bends}

\begin{lem}
\label{ringlem}
Every ring $R$ obtained after the previous corridor decomposition, can be converted into $O(1)$ number of open corridors with at most 3 bends and possibly a box which is guillotine separable and the box contains a smaller ring. All items in this decomposition remain guillotine separable. 
\end{lem}
\begin{proof}
\begin{comment} 
Consider the guillotine cuts sequence on the knapsack. Let $P$ be the smallest subpiece such that ring $R$ lies completely inside $P$ and the next guillotine cut in $P$ is the first cut which passes through $R$.  As in Figure \ref{rings}, we call the left vertical, bottom horizontal, right vertical, top horizontal subcorridors of $R$ as $S_{1}$, $S_{2}$, $S_{3}$ and $S_{4}$ respectively. 
If any cut in $P$ cuts the smaller vertical (resp. horizontal) edges of $S_{1}$ and $S_{3}$ (resp. $S_{2}$ and $S_{4}$), then  we are done as $R$ gets divided into 2 $\Uc$-corridors.  Thus we can assume that first cut passes through a subcorridor and is parallel to its longer edges. 
We now define four types of end-to-end cuts possible in $P$ or in any of the subpieces formed by a sequence of cuts in $P$. The rightmost (resp. leftmost) end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$ ($S_{3}$) is termed as Type $1$ (resp. Type $3$). The topmost (resp. bottommost) end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{2}$ ($S_{4}$) is termed as Type $2$ (resp. Type $4$).  These  cuts may pass through the edges of the ring too.

The basic idea is to bound all the items of a ring to a bounding box $B$ and $O(1)$ number of open corridors with at most 3 bends such that the box is itself guillotine separable from the rest of the knapsack with guillotine cuts along the edges of $B$. We follow an iterative approach to define bounding box $B$. Clearly obtaining all four type of cuts will result in a box  bounded by these cuts which contains a smaller boundary ring. Thus our iterative algorithms halts when either ($i$) all four type of cuts are obtained, or ($ii$) when one of the subcorridors $S_{1}$, $S_{2}$, $S_{3}$, $S_{4}$ is exhausted (as previously, by exhausted we mean that there is no rectangle left in that subcorridor after a step of our iterative procedure in the new smaller subpiece),  or ($iii$) the corridor is divided into smaller open corridors by different type of cut other than the four types defined above.\\
We now formally define the iterative approach to find the bounding box. During the iterative procedure we will be adding rectangles to a 3 bend corridor $U'$(can be degenerate too) which we assume w.l.o.g.~to be coming from $S_{1},S_{2},S_{3}$, as in Figure \ref{ringproc}. That is w.l.o.g.~we assume that Type 4 cut doesn't come before other type of cuts. Considering the type of end-to-end guillotine cut in the subpiece do the following processing:
\begin{enumerate}
\item Case $1$: (Type $1$ cut) Add the items on left subpiece that are part of the ring, to the left-vertical subcorridor of the 3-bend corridor $U'$. Consider the new-subpiece to be the right-subpiece. Stop the iterative procedure if $S_{1}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new-subpiece. 
\item Case $2$: (Type $2$ cut) Add the items on bottom subpiece that are part of the ring,  to the horizontal subcorridor of $U'$. Consider the new-subpiece to be the top-subpiece. Stop the iterative procedure if $S_{2}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new-subpiece.
\item Case $3$: (Type $3$ cut) Add the items on the right subpiece that are part of the ring, to the right-vertical subcorridor of $U'$. Consider the new-subpiece to be the left-subpiece. Stop the iterative procedure if $S_{3}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new-subpiece.
\item  Case $4$: (Type $4$ cut) Pack the items of top subpiece in a new horizontal container $C$. Stop the iterative procedure. In this case we have $O(1)$ corridors and a box bounding the smaller ring whose edges are formed due to type cuts.
\item Case $5$: (Cuts perpendicular to the orientation of the subcorridors) Ring in the current subpiece is divided into 2 $\Uc$-corridors. Stop the iterative procedure.
\item Case $6$: (Cuts which don't pass through the ring) Continue only on the newly created subpiece that contains the ring,  ignore the other subpiece.
\end{enumerate}
\end{comment}
Call the function Algo-Box-Creation($R$) in the Algorithm \ref{boxalgo}.
Each of the halting conditions in Algo-Box-Creation($R$) results into $O(1)$ (\ama{$O_{\eps,\epsl}(1)$}) number of spiral corridors which are with atmost 3 bends bounded by a box and possibly a box bounding a ring. 

\arir{I guess, in case 5 we get 2-$\Uc$, case 4 we get 1 $\Uc$, 1 $\Bc$ and a Box, Other cases 1 $\Uc$, 1 $\Bc$ but no box.}
%Hence we prove Lemma \ref{ringlem}.		
\end{proof}




\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,4) -- (0,0) -- (6,0) -- (6,4) --( 0,4);
			\draw[thick] (1,3)--(5,3) -- (5,1) -- (1,1) -- (1,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,1.25) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};
			\draw (2.5,3.7) node {\large \textbf{$S_{4}$}};


			\draw (1,4.7) node {\large \textbf{Type 1}};
			\draw (6.9,.45) node {\large \textbf{Type 2}};
			\draw (6,4.7) node {\large \textbf{Type 3}};
			\draw (6.9,3.2) node {\large \textbf{Type 4}};

			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,4.5) -- ( .5,0) ;
			\draw[dotted] (.25,4.5) -- ( .25,0) ;
			
			\draw[dotted] (0,.5) -- ( 6.5,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0) ;
			\draw[dotted] (5.25,4) -- ( 5.25,0) ;

			\draw[dotted] (0,3.5) -- ( 6,3.5) ;
			\draw[dotted] (0,3.25) -- ( 6.5,3.25) ;
				
		
		\end{tikzpicture}}
		\caption{Types of cuts}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,5) -- (1,1) -- (7,1) -- (7,5) --(1,5);
			\draw[thick] (2,4)--(6,4)-- (6,2) -- (2,2) -- (2,4) ;
			\draw[thick]  (1.5,1.5) -- (1.5,6) ;% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[thick] (6.5,4.5)--(1.5,4.5);
			\draw[pattern=north east lines, pattern color=black] (6.5,4.5)--(6.5,5)--(1.5,5)--(1.5,4.5)--(6.5,4.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,5) -- (1.5,5) -- (1.5,1.5) -- (6.5,1.5) -- (6.5,5) --(7,5) -- (7,1)--(1,1)--(1,5);		

			\draw (4,1.25) node {\large \textbf{$U'$}};
			\draw (5,4.75) node {\large \textbf{$C$}};
			\draw (4,3) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Final Bounding Box of $S$}
	\end{subfigure}
	\caption{Processing 3-bend corridor}
	\label{ringproc}
\end{figure}



		\begin{thm}
		\label{3max}
		Any  corridor $C$ can be converted into $O_{\eps}(1)$ corridors of type $\Bc, \Lc, \Uc, \Gc$, maintaining guillotine separability.
		\end{thm}
		\begin{proof}W.l.o.g. assume $C$ has no $\Zc$-bends (else apply Lemma \ref{noz}) and more than 3 bends. There are 2 cases. 
		
\noindent {\em Case 1. } $C$ is an open corridor with more than \amar{incomplete}.  Call the function Algo-Spiral($C$) in the Algorithm \ref{spialgo}. The function Algo-Spiral($C$) results into $O_{\eps,\epsl}(1)$ spiral corridors with atmost 3 bends.
\begin{comment}
W.l.o.g~assume $C$ has 4 bends.  \ari{Similar argument holds for other corridors with greater than 4 bends.} We also assume $S_{1}$ to be longer in length than $S_{3}$ (see Figure \ref{bends}).  We follow an iterative approach to partition the corridor $C$  into $O_{\epsl}(1)$ open corridors with at most 3 bends. During the iterative procedure we will be adding rectangles to a $\Gc$-corridor $G'$ (can be degenerate too) which we assume to be coming from $S_{1},S_{2},S_{3},S_{4}$. Considering the type of end-to-end guillotine cut through the corridor $C$ do the following processing:
\begin{enumerate}
\item Case $1$: Cut passes through a subcorridor perpendicular to the orientation of that subcorridor. 
We get two corridors with smaller number of bends. If they have at most 3 bends, we stop. Otherwise, we continue iteratively with the smaller corridors.
%Portion of the corridor $C$ which isn't part of corridor $G'$ gets divided into at most 4 open corridors with at most 3 bends. Stop the iterative procedure.
\item Case $2$ : $V_{S_1}$ cut (Vertical guillotine cut through $S_{1}$). Add the items left of $V_{S_1}$ cut which are part of the corridor $C$ to the leftmost-vertical subcorridor of the 4-bend corridor $G'$.  Stop the iterative procedure if $S_{1}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise continue the iterative procedure on the remaining portion of the corridor $C$ which is not part of $G'$.
\item Case $3$ : $H_{S_2}$ cut (Horizontal guillotine cut through $S_{2}$). Add the items below $H_{S_2}$ cut to the bottommost-horizontal subcorridor of $G'$. Stop the iterative procedure if $S_{2}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise continue the iterative procedure on the remaining portion of the corridor $C$ which is not part of $G'$.
\item Case $4$ : $V_{S_3}$ cut (Vertical guillotine cut through $S_{3}$). Add the items right of $V_{S_3}$ cut  to the rightmost-vertical subcorridor of $G'$.  Stop the iterative procedure if $S_{3}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new subpieces.
\item  Case $5$ : $H_{S_4}$ cut (Horizontal guillotine cut through $S_{4}$). Add the items above $H_{S_4}$ cut  to the topmost-horizontal subcorridor of $G'$. Stop the iterative procedure if $S_{4}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise continue the iterative procedure on the remaining portion of the corridor $C$ which is not part of $G'$.
\end{enumerate}
Thus our iterative algorithms halts when one of the subcorridors $S_{1}$, $S_{2}$, $S_{3}$, $S_{4}$ is exhausted (by exhausted we mean that there is all rectangles of that subcorridor is packed in $G'$ after a step of our iterative procedure)  or when the portion of corridor $C$ which isn't part of $G'$ is divided into at most 4 open corridors with at most 3 bends as in Case 1. This iterative algorithm halts otherwise one of the type cuts will eventually exhaust a subcorridor as the number of cuts in the guillotine cutting sequence is finite. Each of the halting conditions results into $O(1)$ open corridors. 
\end{comment}\\

\noindent {\em Case 2.} $C$ is a ring (see Figure \ref{rings}). Then consider the bounding box $\mathcal{B}$ (if any) which contains a smaller ring as shown in Lemma \ref{ringlem}. 
If the width of the ring inside the bounding box $\mathcal{B}$ divide it into $O_{\epsl}(1)$ smaller rings such that the width of every ring is atmost $\frac{\epsl N}{2}$. Call the function Algo-Boundary-L($\mathcal{B'},C'$) in the Algorithm \ref{Lalgo} for all the smaller rings $C'$ created from $C$ along with their bounding box $\mathcal{B'}$. For inner rings the outermost edges is itself the bounding box. After this we get $O_{\epsl}(1)$ boundary-$\Lc$.

\begin{comment}
For the remainder of the proof by {\em freezing} a rectangle we mean that the rectangle is not moved while rearranging other rectangles. 
If there is any end to end cut which passes through only two subcorridors of same orientation then we can divide the corridor into 2 corridors each having 3 bends. So we now assume that there is no such end to end cut in $\mathcal{B}$. 
Now consider the sequence of guillotine cuts which separate the rectangles in the ring. If we are cutting through leftmost vertical subcorridor or bottom most horizontal subcorridors then we freeze these rectangles. Now in the remaining portion of the box if there is a cut $l_{1}$ through rightmost vertical subcorridor and the distance between $l_{1}$ and edge of the boundary to the right of it be $d$ then we remove the strip $S$ to the right of $l_{1}$. Then we shift the rest of items of box to the right which isn't frozen by a distance of $d$. Now in the empty region created near the left edge of the box we place the strip $S$ which we removed. Now freeze the rectangles in the strip $S$. Do the same process if there is a cut through the upper most horizontal corridor and now instead of shifting  the strip situated above the cut to the left we shift it down by appropriating shifting the remaining portion of the box upwards which isn't still frozen. Note that guillotine separability remains preserved by this rearrangement.
Continue this process till we convert these into single boundary-$\Lc$. We stop when we exhaust all rectangles or we find a cut that divides the ring into two corridors with 3 bends at most. Then we have a box with boundary-$\Lc$ and possibly 2 smaller boxes each containing corridors with at most 3 bends. This completes our proof.
\end{comment}
\end{proof}


==> 5_Non_Rotated_Cardinality.tex <==
%%%%%%%%%%%%%%%% Main Algorithm %%%%%%%%%%%%%%%

\section{$(\frac{4}{3}+\eps)$-approximation \tggkc}\label{sec:tggkcfull}
%\subsection{Item Classification}
%For two given constants $1\geq\epsl\geq\epss$ we classify item i as:
%\begin{itemize}
%\item $small$ if $\width_{i}\leq\epss$ and $\height{i}\leq\epss$;
%\item $horizontal$ if $\height_{i}\leq\epss$ and $\width_{i}>\epsl$;
%\item $vertical$ if $\width_{i}\leq\epss$ and $\height_{i}>\epsl$;
%\item $large$ if $\width_{i}>\epsl$ and $\height{i}>\epsl$;
%\item $intermediate$ otherwise.
%\end{itemize}
%\begin{lem}\cite{GalvezGHI0W17}\label{class}
%Let $\eps >0$ and let $f(.)$ be any positive increasing function such that $f(x)<x$ for all x between 0 and 1. Then, there exist positive constant values $\epsl,\epss \in \Omega_{\eps}(1)$, with $f(\eps)\geq\epsl$ and $f(\epsl)\geq\epss$ such that the total profit of intermediate rectangles is bounded by $\eps \profit(\opt)$. The pair ($\epsl,\epss$) is one pair from a set of $O_{\eps}(1)$  pairs and this set can be computed in polynomial time.
%\end{lem}

\subsection{Simplification of Input}\label{sec:inputsimplification}
For \tggkc, due to the following lemma, we will assume that remove $O(1)$ number of items without losing too much profit.

\begin{lem}\cite{adamaszek2015knapsack} 
\label{lem:drop}
If there is an algorithm for \tgkc~which outputs a solution with at least $(1-\eps)\opt-\beta^{O_\eps(1)}$ items in time $O(f(n))$,
then there is also a $(1+\eps)$-approximation algorithm with running time $O(f(n)+n^{{\beta}^{O_\eps(1)}})$.
\end{lem}

Thus for \tggkc, large items can be dropped as there are at most $O(\frac{1}{\epsl^{2}})$ large rectangles in any given packing. 
In fact, for now we assume that there are only skewed items in the packing. At the end of the section, we show how to repack the small items. 

\subsection{Processing of subcorridors from $\Bc\Lc$-arrangement}
From Lemma \ref{thm:ldecom}, we obtain $O_{\eps,\epsl}(1)$ number of corridors of type $\Bc$ or $\Lc$.
$\Lc$-corridors are  boundary-$\Lc$ of a guillotine separable box. 
Now we {\em process} the $\Lc$-corridors in 2 different ways (see Section \ref{prosec} and for processing of corridors) to obtain $L\&C$-packing, as in \cite{GalvezGHI0W17}. 
As they are part of boundary-$\Lc$ of a guillotine separable box, the processing preserves guillotine separability. 
For now we briefly define processing vertical subcorridor (see Figure \ref{fig:lproc}). We first divide the subcorridor with $\frac{1}{\eps_{box}}$ strips of equal width. Items intersected by these lines are termed as \emph{kill}, items in the leftmost strip are termed as \emph{thin} and the remaining set of items in the subcorridor as \emph{fat}. We then remove \emph{thin} and \emph{kill} items from the subcorridor and form boxes with maximal rectangular subregions formed between the boundary curve and the subcorridor. We then shift the remaining items in the boxes from other subregions to left to fill in the empty subregion formed by the removal of thin items. The projections from intersection of boxes and boundary curve are used to divide the horizontal subcorridor into similar strips. We again classify the items in this corridor as \emph{kill} for the items being intersected by the lines used to form strips and remove these items. Remaining items are packed as it is in the subregions.
Intuitively, one can view the creation of boxes in {\em processing of a subcorridor} as a series of guillotine cuts. 
The rearrangement of boxes can be viewed as movement of subpieces without violating guillotine separability. These movements do not disturb other parts of the bounding box as these cuts do not pass through the rest of the boxes.
After {\em processing} of all vertical subcorridors, we get a partition of $\optco \setminus \optco^{cross}$ (i.e., items contained inside the initial corridor decomposition) into three sets: $\optth$, $\optki$ and $\optfa$. 
Now we can use resource augmentation (see Lemma \ref{tool:container}) to get $\optfa^{cont} \subseteq \optfa$ such that all items in $\optfa^{cont}$ are packed into containers and $\profit(\optfa^{cont}) \ge (1-\eps)\profit(\optfa)$.


In second way, we process the horizontal subcorridors (analogous to the vertical corridor processing) of $\Lc$-corridors, where we only remove {\em thin} items from horizontal subcorridors. 

Each of these two different processing gives different sets $\optth$, $\optki$ and $\optfa^{cont}$. Based on these sets we classify the rectangles as follows:
%\arir{Need to explain processing in more details.}
\begin{itemize}
\item $\opt_{T}$ is the set of items which are in $\optth$ in one of the cases.
\item $\opt_{K}$ is the set of items which are in $\optki$ in one of the cases.
\item $\opt_{F}$ is the set of items which are in $\optfa^{cont}$ in both cases.
\end{itemize}
\begin{lem}\cite{GalvezGHI0W17}
\label{ering}
If we take any one of the cases of processing the following properties hold:
\begin{enumerate}
\item $|OPT_{kill}|=O_{\eps,\epsl,\epsb}(1)$;
\item For any given constant $\epsr>0$ there is a sufficiently small $\epsb>0$ such that the total height(resp.,width)of items in $\optth\cap\Rho$ (resp. $\optth\cap\Rve$) is at most $\epsr N$.
\end{enumerate}
\end{lem}

Now we classify items in the optimal packing into four sets: $\opt_{LT}, \opt_{ST}$ (long and short items in $\opt_T$, resp.),  $\opt_{LF}, \opt_{SF}$ (long and short items in $\opt_F$, resp.). \footnote{This notation is different from \cite{GalvezGHI0W17}, e.g., in our notation $|\opt_{LT}|$ can even be the same as $|\opt_{L}|$.} 	

%\subsection{Profitable Structure Packing}\label{profitstruc}
%\begin{lem}\cite{GalvezGHI0W17}\label{sumprofit}
%$\profit(\opt_{F}\cap\opt_{T})+\profit(\opt_{k})+\profit(\opt_{large})+\profit(\opt_{corr}^{cross})\geq(1-O(\eps))\profit(\opt)$.
%\end{lem}

\begin{lem}[restatement of Lemma \ref{algo1}]
$\profit(\opt_{L\&C})\geq\profit(\opt_{F})+\profit(\opt_{T})/2$.
\end{lem}


Now we show the detailed proof of Lemma \ref{algo3}.
\begin{lem}[restatement of Lemma \ref{algo3}]
$\profit(\opt_{L\&C})\geq\profit(\opt_{T})+(1-O_{\eps}(1))\profit(\opt_{F})/2$.
\end{lem}
%\arir{Check this proof. I plan to keep only case 1 in main body to convey the main idea and the whole proof in Appendix.}
\begin{proof}
Let $w_L N$ (resp. $w_{LT} N$) be the total width of vertical items in $\optln$ (resp. $\opt_{LT}$) and 
$h_L N$ (resp. $h_{LT} N$) be the total height of horizontal items in $\optln$ (resp. $\opt_{LT}$).
Then  $w_L, h_L \le 1$, $w_{LT},h_{LT}   \le \epsr$, and  all long items can be packed in a boundary-$\Lc$ of width $w_L N$ and height $h_L N$.  W.l.o.g.~assume $w_L \le h_L$ (the other case is analogous). 
Consider some small positive constant $\tilde{\eps}\le \frac12$ that we will choose later. 
Now if $w_L \ge \epsr/\tilde{\eps}$, then from vertical arm of  boundary-$\Lc$, we
choose  a random vertical strip $[\tilde{x}, \tilde{x}+\frac{w_L N}{2}+w_{LT} N] \times [0,N]$ (if $\tilde{x}+\frac{w_L}{2} N+w_{LT} N\le w_L N$) or two random strips $([\tilde{x}, w_L N]  \times [0,N]) \cup ([0, \tilde{x}+\frac{w_L N}{2}+w_{LT} N -w_L N] \times [0,N]$ (if $\tilde{x}+\frac{w_L N}{2}+w_{LT} N> w_L N$), where $\tilde{x}$ is chosen uniformly at random from $[w_L]$. We remove all fat items intersecting with this strip.
If $w_L <\epsr/\tilde{\eps}$, we do not remove any items.
Similarly, if $h_L \ge \epsr/\tilde{\eps}$,  we do similar operation on horizontal arm and remove all fat items intersecting random horizontal strip(s) of total width $\frac{h_L}{2} N+h_{LT} N$, and if $h_L < \epsr/\tilde{\eps}$, we do not remove any items.
Now we analyze these three cases separately. \\

\noindent {\em Case 1:} $w_L \ge \frac{\epsr}{\tilde{\eps}}$ and $h_L \ge \frac{\epsr}{\tilde{\eps}}$.
By averaging argument, the remaining items have profit $\frac{\big(1-O_{\epsl, \epsr, \tilde{\eps}}(1)\big)}{2}\cdot \opt_{LF}+\opt_{LT}$ and packed in boundary-$\Lc$ of width $\le w_L N/2$ and height $\le h_L N/2$ ( as shown in figure \ref{fig:c6}a).
In the remaining rectangular region of the box, we will place containers. 
Now we place items in $\opt_{ST}$ in two containers next to boundary-$\Lc$.
First, we place a container of height $N/2$ and width $\epsr N$, with its bottom-left corner at  $(\frac{w_L N}{2}, \frac{N}{2})$,  containing items in $\opt_{ST}$  coming from vertical subcorridors in the processing and then we place a container of width $N/2$ and height $\epsr N$, with its bottom-left corner at  $(\frac{N}{2}, \frac{h_L N}{2})$, containing items in $\opt_{ST}$  coming from horizontal  subcorridors in the processing.
As $w_L\le 1/2$, i.e., $1-w_L/2\ge 3/4$,  these two containers do not overlap. 
Now we are left with a rectangular region of width  $N\big(1-\frac{w_L}{2}-O_{\epsr}(1)\big)$ and height $N\big(1-\frac{h_L}{2}-O_{\epsr}(1)\big)$. We will use of slightly smaller region of width $N\big(1-\frac{w_L}{2}-O_{\epsr}(1)-\eps\big)$ and height $N\big(1-\frac{h_L}{2}-O_{\epsr}(1)-\eps\big)$ to show existence of a guillotine packing by Steinberg's Algorithm (Lemma \ref{lem:steinbeg}). However, Steinberg's algorithm may not give a container-based packing. Hence, we use resource augmentation (Lemma \ref{lemma1}) using the extra $\eps$-strips to obtain a container-based guillotine packing. This along with boundary-$\Lc$ will give a $L\&C$-packing.
Using Steinberg's algorithm, we can pack any subset of items  in $\opt_{SF}$ of total area at most 
$\Big(\big(1-\frac{w_L}{2}-O_{\epsr}(1)-\eps\big)\big(1-\frac{h_L}{2}-O_{\epsr}(1)-\eps\big)-\big(\frac{w_L}{2}+O_{\epsr}(1)+\eps\big)\big(\frac{h_L}{2}+O_{\epsr}(1)+\eps\big)\Big)N^2/2 \le \frac{N^2}{2}\big(1-\frac{(w_L+h_L)}{2}-O_{\epsr,\eps}(1)\big)$.
On the other hand, the total area of rectangles in $\opt_{SF}$ is at most $N^2\big(1-\frac{w_L+h_L}{2}-O_{\epsr}(1)\big)$.
So, consider rectangles in $\opt_{SF}$ in non-decreasing order of area till they reach $N^2\big(1-\frac{(w_L+h_L)}{2}-O_{\epsr}(1)\big)$.
These items can be packed in the remaining region and have total profit $\ge  \profit(\opt_{SF}) \Big(\frac{N^2}{2}\big(1-\frac{w_L+h_L}{2}-O_{\epsr, \eps}(1)\big)\Big) / \Big(N^2\big(1-\frac{w_L+h_L}{2}-O_{\epsr}(1)\big)\Big) \ge ( \profit({\opt_{SF}}) \cdot \big(1-O_{\epsr,\eps}(1)\big)/2$.
Thus we have $L\&C$-packing with profit  $\profit(\opt_{LT})+\profit(\opt_{ST})+\profit(\opt_{LF}) \cdot  \frac{\big(1-O_{\epsr}(1)\big)}{2}+\profit(\opt_{SF}) \cdot \frac{\big(1-O_{\epsr,\eps}(1)\big)}{2}$ ( as shown in figure \ref{fig:c6}b).\\

\noindent {\em Case 2:} $w_L < \frac{\epsr}{\tilde{\eps}}$ and $h_L \ge \frac{\epsr}{\tilde{\eps}}$.
The remaining items have profit at least $\frac{\big(1-O_{\epsl, \epsr}(1)\big)}{2}\cdot \opt_{LF}+\opt_{LT}$ and packed in boundary-$\Lc$ of width $\le w_L N$ and height $\le h_L N/2$.
In the remaining rectangular region of the box, we will place containers. 
Now we place items in $\opt_{ST}$ in two containers next to boundary-$\Lc$.
First, we place a container of height $N/2$ and width $\epsr N$, with its bottom-left corner at  $({w_L N}, \frac{N}{2})$,  containing items in $\opt_{ST}$  coming from vertical subcorridors in the processing and then we place a container of width $N/2$ and height $\epsr N$, with its bottom-left corner at  $( \frac{N}{2}, \frac{h_L N}{2})$, containing items in $\opt_{ST}$  coming from horizontal  subcorridors in the processing.
As in this case $w_L=O_{\epsr}(1)$, we are left with a rectangular region of width  $N \big(1-O_{\epsr}(1) \big)$ and height $N \big(1-\frac{h_L}{2}-O_{\epsr}(1) \big)$. We will use a region of width $N \big(1-O_{\epsr}(1)-\eps \big)$ and height $N \big(1-\frac{h_L}{2}-O_{\epsr}(1)-\eps \big)$ to  pack items from $\opt_{SF}$.
Using Steinberg's algorithm, we can pack any subset of items  in $\opt_{SF}$ of total area at most 
$\Big((1-O_{\epsr}(1)-\eps)(1-\frac{h_L}{2}-O_{\epsr}(1)-\eps)-(O_{\epsr}(1)+\eps)(\frac{h_L}{2}+O_{\epsr}(1)+\eps)\Big)N^2/2 \le \frac{N^2}{2}(1-\frac{h_L}{2}-O_{\epsr,\eps}(1))$.
On the other hand, the total area of rectangles in $\opt_{SF}$ is at most $N^2 \big(1-\frac{h_L}{2}-O_{\epsr}(1) \big)$.
So, consider rectangles in $\opt_{SF}$ in non-decreasing order of area till they reach $N^2 \big(1-\frac{(h_L)}{2}-O_{\epsr}(1) \big)$. These items can be packed in the remaining region and have total profit $\ge  \profit(\opt_{SF}) \Big(\frac{N^2}{2} \big(1-\frac{h_L}{2}-O_{\epsr, \eps}(1) \big)\Big) / \Big(N^2 \big(1-\frac{h_L}{2}-O_{\epsr}(1) \big)\Big) \ge ( \profit({\opt_{SF}}) \cdot  \big(1-O_{\epsr,\eps}(1) \big)/2$.
Thus we have $L\&C$-packing with profit  $\profit(\opt_{LT})+\profit(\opt_{ST})+\profit(\opt_{LF}) \cdot  \frac{(1-O_{\epsr}(1))}{2}+\profit(\opt_{SF}) \cdot \frac{ \big(1-O_{\epsr,\eps}(1) \big)}{2}$.
\\

\noindent {\em Case 3:} $w_L < \frac{\epsr}{\tilde{\eps}}$ and $h_L < \frac{\epsr}{\tilde{\eps}}$.
We do not remove any items from $\opt_L$.  We place a container of height $N/2$ and width $\epsr N$, with its bottom-left corner at  $( w_L N, \frac{N}{2})$,  containing items in $\opt_{ST}$  coming from vertical subcorridors in the processing and then we place a container of width $N/2$ and height $\epsr N$, with its bottom-left corner at  $( \frac{N}{2}, h_L N)$, containing items in $\opt_{ST}$  coming from horizontal  subcorridors in the processing. Then as above we will use remaining area to obtain a container-based guillotine packing. 
Now $w_L, h_L=O_{\epsr}$ and thus we can use a region of width $N \big(1-O_{\epsr}(1)-\eps \big)$ and height $N \big(1-O_{\epsr}(1)-\eps \big)$ to pack items from $\opt_{SF}$.
Using Steinberg's algorithm, we can pack any subset of items  in $\opt_{SF}$ of total area at most 
$\Big( \big(1-O_{\epsr}(1)-\eps \big) \big(1-O_{\epsr}(1)-\eps \big)- \big(O_{\epsr}(1)+\eps \big) \big(O_{\epsr}(1)+\eps \big)\Big)N^2/2 \le \frac{N^2}{2} \big(1-O_{\epsr,\eps}(1) \big)$.On the other hand, the total area of rectangles in $\opt_{SF}$ is at most $N^2 \big(1-O_{\epsr}(1) \big)$.
So, consider rectangles in $\opt_{SF}$ in nondecreasing order of area till they reach $N^2 \big(1-O_{\epsr}(1) \big)$.
These items can be packed in the remaining region and have total profit $\ge  \profit(\opt_{SF}) \Big(\frac{N^2}{2} \big(1-O_{\epsr, \eps}(1) \big)\Big) / \Big(N^2 \big(1-O_{\epsr}(1) \big)\Big) \ge ( \profit{\opt_{SF}}  \big(1-O_{\epsr,\eps}(1) \big)/2$.
Thus we have $L\&C$-packing with profit  $\profit(\opt_{LT})+\profit(\opt_{ST})+\profit(\opt_{LF}) +\profit(\opt_{SF}) \cdot \frac{ \big(1-O_{\epsr,\eps}(1) \big)}{2}$. \end{proof}



From Lemma \ref{algo1} and \ref{algo3}, we get $\profit(OPT_{L\&C})\geq(\frac{3}{4}-O(\eps))\profit(\opt)$.
The worst case is obtained when $\profit(\opt_{T})=\profit(\opt_{F})$. The resulting packing is guillotine separable as both the packings from Lemma \ref{algo1} and \ref{algo3} are guillotine separable. Lemma \ref{algo1} follows deletion of items from corridors obtained from $\Bc \Lc$-arrangement which preserves guillotine property. Lemma \ref{algo3} packs a subset of long items in a boundary-$\Lc$ and remaining items in the rest of the subpiece using Steinberg's algorithm, followed by a resource augmentation to obtain a container-based packing. It follows by a simple inductive argument that $\Lc$-packing can be guillotine separated from the rest of the subpiece. From Lemma \ref{lem:steinbeg} and Lemma \ref{lemma1}, it follows that Steinberg's algorithm and resource augmentation respectively maintain guillotine separability. This concludes that the resulting packing is guillotine separable. 
\begin{thm}
\label{LC}
Let $OPT_{L\&C}$ be the most profitable solution that is packed by a guillotine separable $L\&C$ packing and $\opt$ be optimal  packing for \tggkc. Then $\profit(OPT_{L\&C})\geq(\frac{3}{4}-O(\eps))\profit(\opt)$. 
\end{thm}

%%%5 previous results commented out begin
\begin{comment}
\subsubsection {Previous part, might be removed if above is true.}
\begin{lem}
\label{algo2}
$\profit(\opt_{L\&C})\geq\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{SF})$.
\end{lem}
\begin{proof}
From the optimal packing we remove all the items except the items in $\opt_{SF}$. Now in this new packing consider a horizontal (resp., vertical) random strip of height (resp., width) $3\eps N$. Remove the items which overlap with these vertical and horizontal strips. Let the items which remain be $\opt_{SF}'$. Due to horizontal strip, a horizontal item gets removed with probability at most $7\eps$ and a vertical item gets removed with probability at most $\frac{1}{2}+6\eps$. Similarly, due to vertical strip, a vertical item gets removed with probability at most $7\eps$ and a horizontal item gets removed with probability at most $\frac{1}{2}+6\eps$. From linearity of expectation we get that $\profit(\opt_{SF}' )\geq (\frac{1}{2}-13\eps)\profit(\opt_{SF})$. \\
\\Also clearly $\opt_{SF}'$ can be packed in a square of side length $(1-3\eps)N$. So by doing one sided resource augmentation we can get a packing with profit $(1-O(\eps))\profit(\opt_{SF}')$ in a square with side length $(1-2\eps)N$. In $N \times N$ knapsack we can pack all items in $\opt_{LT}$ in a boundary-$\Lc$ with width $\epsr N$. Two containers of dimensions $\epsr N \times \frac{N}{2}$ and $\frac{N}{2} \times \epsr N$ are created and kept just beside the subcorridors of boundary-$\Lc$ in such a way that the 2 created subcorridors don't overlap with each other. We pack all the items in $\opt_{ST}$ in these two containers. In the remaining square region which doesn't have items from $\opt_{T}$ we can pack the items from $\opt_{SF'}$ with profit $(1-O(\eps))\profit(\opt_{SF}')$ as the square region has side length at least $(1-2\eps)N$. This concludes the proof of this Lemma. 
\end{proof}

\begin{lem}
\label{idea}
$\profit(\opt_{L\&C})\geq\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{LF})$.
\end{lem}
\begin{proof}


%\begin{figure}[t]
%\centering
%\includegraphics[scale=1]{pic7}
%\caption{Case1}
%\label{prop1}
%\end{figure}
\begin{figure}[t]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\resizebox{!}{3cm}{
		\begin{tikzpicture}
		
				%box
			\draw [thick] (0,0) rectangle ( 20,20);
			\draw[solid , fill = lightgray] (0,0) -- (20,0) -- ( 20,16) -- ( 6,16) -- ( 6, 20) -- ( 0, 20) -- ( 0,0) ;


			\draw[solid, fill = darkgray] (9,7) rectangle (20,9);
			\draw[solid, fill = lightgray] (22,8) rectangle (26,8.5);
		\end{tikzpicture}}
		\caption{case1}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\resizebox{!}{3cm}{
		\begin{tikzpicture}
			\draw[thick] (0,0) rectangle (20,20);
			\draw[solid , fill = lightgray] (0,0) -- ( 20,0) -- ( 20, 12) -- ( 4, 12) -- ( 4,20 ) -- ( 0 , 20 ) -- ( 0,0) ;
			\draw ( 0, 10 ) -- ( 20 , 10) ;
			\draw ( 1, 0) -- ( 1, 6) -- ( 2, 6) -- ( 2, 8 ) -- ( 4, 8) -- ( 4, 12) ;
		\end{tikzpicture}}
		\caption{case2}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\resizebox{!}{3cm}{
		\begin{tikzpicture}
			\draw[thick] (0,0) rectangle (20,20);
			\draw[solid , fill = lightgray] (0,0) -- ( 20,0) -- ( 20, 10) -- ( 4, 10) -- ( 4,20 ) -- ( 0 , 20 ) -- ( 0,0) ;
			\draw[solid , fill = darkgray] ( 5, 11 ) rectangle ( 6 , 19) ;
			\draw[solid , fill = darkgray] ( 7, 10.5 ) rectangle ( 19 , 12) ;

		\end{tikzpicture}}
		\caption{case2}
		\label{case2}
	\end{subfigure}
	%\caption{Different types of subcorridors.Subcorridor as shown in (c) is not possible as z bend doesn't occur as shown in Theorem \ref{theorem1}}
	%\label{subcorridor}
	\caption{}\label{prop1}
\end{figure}

$Case$ $1$: In this case, total width of items in $\optve \cap \R_{long}$ is greater than or equal to $(\frac{1}{2}+\epsr)N$ and less than $\frac{N}{2}$ and total height of  items in $\optho \cap \R_{long}$ is more than $\frac{N}{2}$. Since we have excluded large items in this section, the L packing of long items doesn't have large items. Now by averaging argument we can identify a strip of height $\eps N$ and loose profit of at most $O(\eps)\profit(\opt_{LF})$  in the L-packing by removing only the items of $\opt_{LF} \cap \Rho$ which overlaps with this strip. If there are any items of $\opt_{LT}$ in the strip then we push it down. In the remaining space we identify a rectangular region which is doesn't cross the boundary curve (as shown in Figure \ref{prop1}(a)) to pack all the items in $\opt_{ST} \cap \Rho$ on top of each other. In a similar fashion we can pack all the rectangles in $\opt_{ST} \cap \Rve$
\\
\\$Case$ $2$: In this case, total width of items in $\optve \cap \R_{long}$ is less than $(\frac{1}{2}-\epsr)N$ and total height of items in $\optho \cap \R_{long}$ is more than $\frac{N}{2}$. We now cannot pack the items of $\opt_{ST} \cap \Rve$ in a vertical strip of width $\eps N$ in the vertical subcorridor as the strip may contain huge profit irrespective of the way it is being chosen. Now consider a horizontal line $l$ at the height of $\frac{N}{2}$ in the knapsack. Let the rectangles in $\optho \cap \R_{long}$ above $l$ be $\R_{1}$ and the rectangles below $l$ be $\R_{2}$. Now, if $\profit(\opt_{LF}) \cap \R_{2} > \profit(\opt_{LF}) \cap \R_{1}$  then we remove the items in $\R_{1}$ and pack the items of $\opt_{LT} \cap \R_{1}$  by removing the least profitable strip of height $\eps N$ of $\R_{2}$ in the similar way as done in Case 1. Otherwise if $\profit(\opt_{LF}) \cap \R_{1} > \profit(\opt_{LF}) \cap \R_{2}$, then remove the items in $\R_{2}$ and remove the least profitable strip of height $\eps N$ from $\R_{1}$ by assuming the rectangles of $\R_{1}$ to be part of a container of dimension $\frac{N}{2} \times \frac{N}{2}$. Then we place the items in $\opt_{LT} \cap \Rho$ at bottom right of the knapsack on top of each other in the decreasing order of width. Then place the remaining items of $\R_{1}$ on top of the items in  $\opt_{LT} \cap \Rho$ . Now we have a new L packing and an empty square region with height at least $\frac{N}{2}$ and width at least $(\frac{1}{2} + \epsr)N$. Therefore we can pack every item belonging to $\opt_{ST}$ in 2 separate containers as shown in Figure \ref{prop1}(b) and (c) .
\\We ignore other cases as they are symmetric to the above two cases. 
\\
\\ The profit we can pack is at least $\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{LF})$  
\end{proof}
Now combining Lemma \ref{idea} with Lemmas  \ref{algo1} and \ref{algo2} we get  $\profit(OPT_{L\&C})\geq(\frac{7}{10}-O(\eps))\profit(OPT)$.The worst case is obtained when $\profit(\opt_{T})=3\profit(\opt_{LF})=3\profit(\opt_{SF})$.
\end{comment}

%%%%%%%%%%%%5 comment ends

\subsection{Adding small rectangles}\label{smallrec}
\begin{lem}\cite{GalvezGHI0W17}\label{dead}
In the packings mentioned in Lemma \ref{algo1} (and Lemma \ref{algo2}), if we build a grid of width $\eps'N=\frac{\epss}{\eps}\cdot N$ and delete any cell of the grid that overlaps with the container or boundary-$\Lc$ then total area of the deleted (also called {\em dead}) grid cells is min$\{ (1-\eps) N^{2},a(\opt_{corr})+3\eps^{2}N^{2}\}$ where $a(\opt_{corr})$ denotes the  total area of  items in $\opt_{corr}$.
\end{lem}
 We denote the cells which are not dead as free cells. Now take the knapsack and find the regions which are guillotine separable and do not overlap with any container or boundary-$\Lc$. Let us denote these regions as guillotine free region. By appropriate choosing $\eps,\epsl,\epss,\eps_{box},\epsau$ (as shown in subsection \ref{cnt}) we can ensure that the total area of guillotine free regions which don't have both the dimensions greater than or equal to $\eps' N$ is $O_{\eps,\epsl,\eps_{box},\epsau}(1)\cdot \frac{\epss}{\eps}\cdot N^{2}$ which is at most $O(\eps^{2} N^{2})$. Now the total area of guillotine free region is greater than or equal to the total area of free cells. So the total area of guillotine free regions with both dimensions greater than or equal to  $\eps' N$ is at least $\max \{ (\eps N^{2},a(\opt_{small})\}-O(\eps^{2}N^{2}$)). We have sufficient area to pack small rectangles of the packings in Lemma \ref{algo1} (and Lemma \ref{algo2}). 
\begin{lem}\label{bigL}
In the packing mentioned in Lemma \ref{algo3}, consider a similar grid as created in Lemma \ref{dead}. Then the total area of deleted grid cells is at most $a(\opt_{L})+a(\opt_{ST})+5\eps'\cdot N^{2}$+min$\{(1-\eps)a(R'),a(\opt_{corr})+3\eps^{2}N^{2}\}$ where $R'$ is the maximal rectangular region in the knapsack which doesn't contain items from $\opt_{L}$ and $\opt_{ST}$. Grid cells are considered to be dead if they overlap with any rectangle.%\amar{Need to re-write}
\end{lem}
\begin{proof}Remove the containers in $R'$. Consider a boundary-$\Lc$ in the packing (the region not containing $R'$) under consideration such that the vertical subcorridor $S_{1}$ is top-left  of horizontal subcorridor $S_{2}$. In the packing of Lemma \ref{algo3}, we can ensure that width of the boundary-$\Lc$ is at most $\frac{N}{2}$. Now consider the first column of grid cells from left. The area of dead cells in first column is at most $\eps'N^{2}$. In the second column of grid cells from left if there are $x$ grids cells which are dead then the length of all the long  rectangles in the first column is at least $(x-1)\cdot \eps' N$ due to Lemma \ref{lpackinglem}. So the area of dead cells in second column is at most area of rectangles in the first column plus $\eps'^{2}N^{2}$. Adding up the area of all the dead cells in this manner and repeating the same for horizontal rectangles we get total area of deleted grid cells to be at most $a(\opt_{L})+a(\opt_{ST})+3\eps'\cdot N^{2}$. Now restore the containers which were removed from $R'$ to their original position. Applying Lemma \ref{dead} to $R'$, we get that the area of dead cells 
inside $R'$ is at most $\min \{(1-\eps)a(R'),a(\opt_{corr})+3\eps^{2}N^{2}\}$. Additional $2\eps' N^{2}$ can be lost if the gridcell intersects with the boundary of $R'$.
\\A box is said to be $\eps'$-large if both dimensions are greater than or equal to $\eps' N$. Now there are {\em $\eps'$-large} guillotine free regions in the rectangular region $R'$ which has total area of at least area(free cells in $R'$)-$O(\eps^{2}N^{2}$)).\\
 Now we describe a procedure to obtain $(1-\eps)\eps'$ large boxes (to pack the small rectangles) from the free cells in the region excluding $R'$ which is the boundary-$\Lc$. Note that these $(1-\eps)\eps'$ large boxes when considered as pseudorectangles are guillotine separable. Consider the first column of grid cells from the left and assume that we have free cells in this column. Separate the horizontal rectangle, if any (using a horizontal guillotine cut), which overlaps with this first column. Now consider the rightmost vertical cut which passes through this column. The distance of this cut from the right-hand side of this column is at most $\epss N$. So we obtain $(1-\eps)\eps'$ large boxes in the first column which are guillotine separable.  Continue the same process for other columns which overlap with the vertical subcorridor of the boundary-$\Lc$. Free cells which are in the horizontal subcorridor at the end of this process are guillotine separable.
 \end{proof}
Area of guillotine separable boxes obtained from free cells is at least\\ $(1-\eps)(\max\{ (\frac{\eps N^{2}}{4},a(\opt_{small})\}-O(\eps^{2}N^{2}))$. So if $a(\opt_{small})\geq \frac{\eps N^{2}}{4}$ we can pack almost all the small rectangles using NFDH in the guillotine separable  $(1-\eps)\eps'$-large boxes created and the guillotine free regions present in the region which doesn't contain boundary-$\Lc$. If $a(\opt_{small})$<$\frac{\eps N^{2}}{4}$, we can pack all the small rectangles as area of guillotine separable regions and boxes is at least $\frac{(1-\eps)\eps N^{2}}{4}$.
This ensures a packing of profit $(1-O(\eps))\profit(\opt_{small})$ from small items. 

%\arir{Did minor changes. go over small rectangles packing carefully.}

\subsection{Relationship between different constants}\label{cnt}
 We set $\epsau$ to be $\eps^{2}$ and $\epsau'=\epsau/2$. By choosing a big enough constant $\lambda$ such that number of corridors obtained is far less than $\frac{1}{\eps} \cdot (1/\epsl')^{\lambda}$ given that at least one of the dimension of the rectangles while corridor decomposition is greater than $\epsl' N$, we set function $f(x)$ in the lemma \ref{class} to be $\frac{x^{3\lambda}}{(2K'(\epsau'^{\lambda^{1/\eps}})+\frac{1}{\epsau'})^{2}}$. Note than $\lambda$ doesn't depend on $\epsl'$. Here $K'(x)=(\frac{2}{x^{10}}+(\frac{3}{x^{2}}(M(x))^{2}2^{2M(x)})^{\epsau'})$ $\lceil \log_{1+\epsau'}(1/x)\rceil/\eps^{2}$ where $M(x)=\frac{1+2x}{x^{2}}$. We set $\eps_{box}$ to be $\eps^{3}\epsl^{\lambda}$. This ensures that  sum of the heights of the rectangles in $\opt_{thin} \cap \R_{hor}$ is less than $\eps^{2} N$. Now we show that all our constraints are satisfied. By lemma \ref{class} we get a pair $(\epss,\epsl)$ such that $\epss \leq \frac{\epsl^{3\lambda}}{(2K'(\eps^{\lambda^{1/\epsau'}})+1/\epsau')^{2}}$.  Let the total area of guillotine free regions with at least one of the dimensions less than $\eps' N$ be $A_{< \eps'}$. Then $A_{< \eps'} < \frac{1}{\eps_{box}}\cdot(2K'(\delta)+1/\epsau')^{2}\cdot\frac{1}{\eps}\cdot(\frac{1}{\epsl})^{\lambda}\cdot\frac{\epss}{\eps}N^{2}<\eps^{2}N^{2}$. Here $\delta > \epsau'^{\lambda^{1/\eps}}$. Loose upper bound for $A_{< \eps'}$ is found by multiplying the total number of containers by maximum area of guillotine free region which isn't $\eps'$ large. Here as we said before $\lambda$ is a very large constant such that it satisfies all the inequalities which can be found by finding largest constant $c_{1}$ which arises in our equation which we can safely assume to be say greater than 5 and keeping $\lambda=c_{1}^{\frac{1}{\eps}\cdot 10^{10}}$.
 
\subsection{Finding the packing in polynomial time} \label{sec:findpack}%\arir{write more details.}
%Using GAP(as mentioned in \cite{GalvezGHI0W17}) and brute forcing among polynomial number of options we can find the packing which gives the desired approximation factor in polynomial time.
%\amar{both rotated and non-rotated cases are similar, can do in one section}
From Theorem \ref{LC}, we establish that there is a guillotine separable $L\&C$-packing with profit at least $(\frac{3}{4}-O(\eps))\profit(\opt)$. Now we describe how to guess similar profit  packing in polynomial time.  From Lemma \ref{class}, we can have $O_{\eps}(1)$ number of guesses for the values of $\epsl$ and $\epss$. We fix all other constants with the values as specified in Section \ref{cnt}. 
Now we consider two packings as from Lemma \ref{algo1} and \ref{algo3}. 

For the former case, we have a corridor decomposition with $O_{\eps,\epsl}(1)$ number of containers. Intuitively, we will first guess the containers from all possible sets of containers, then we will be reducing the problem instance to \emph{Generalized Assignment Problem (GAP)} to assign rectangles to the set of containers and then pack the rectangles assigned in respective containers. Thus we state the following lemma:
\begin{lem}\label{lem:findPacking}
[adapted from \cite{GalvezGHI0W17}]
Given a set $C$ of $O(1)$ containers and a set $\R$ of rectangles, there is a PTAS to pack a subset $\R' \subseteq \R$ into $C$ maintaining guillotine property, whether rotations are allowed or not.
\end{lem}
\begin{proof}
Note that we can  can check whether a given packing of items in a knapsack is guillotine separable or not (see Lemma \ref{polygil}).
So we enumerate all the possible choices of container packing and only consider those  that are guillotine separable. 
 This takes polynomial time as the number of corridors is $O_{\eps,\epsl}(1)$ and possible size set for containers has cardinality $n^{O_{\eps,\epsl}(1)}$. Once we get the containers we assign rectangles to individual containers by reducing to GAP. For every container there is a corresponding bin and for every rectangle there is a corresponding item with profits and sizes assigned w.r.t the type of the containers. After reduction we use PTAS from Lemma \ref{lem:GAP} to assign item to the bins. This gives a corresponding assignment of rectangles to containers. For placing the rectangles in assigned containers we use Lemma \ref{lem:NFDH} to pack them using \emph{Next Fit Decreasing Height (NFDH)} in a guillotine separable arrangement. We claim that in the end of packing guillotine property is maintained as containers are chosen to be guillotine separable and items packed inside them are packed using NFDH which is $2$-stage packing.
\end{proof}
In the latter case, we have packing of a boundary-$\Lc$ containing only long rectangles and in the remaining sub-piece we have a container packing with $O(1)$ containers. We obtain the $\Lc$-packing of rectangles in the boundary-$\Lc$ using PTAS from Lemma \ref{lem:PTASL}. For the remaining sub-piece we proceed with the same arguments as in first case for finding the packing for a constant number of containers and use lemma \ref{lem:findPacking} for packing them in polynomial time along with maintaining the guillotine separability.\\
Thus considering the best packing of above two, we can find a packing of a subset of given items in the given knapsack in time $n^{O_{\eps,\epsl}(1)}$ such that the items have profit at least $(\frac{3}{4}-O(\eps))\profit(\opt)$.




==> 6_Resource_Augmentation.tex <==
	\section{One Sided Resource Augmentation}
	In this section we show that the proof techniques used in \cite{GalvezGHI0W17} for packing rectangles with resource augmentation maintain the guillotine separability of the rectangles.
	\begin{lem}
	\label{lemma1}
	(Resource Augmentation Packing Lemma\cite{GalvezGHI0W17}) Let $\R'$ be a collection of rectangles that can be packed into a box of size $a\times b$, and $\epsau$>0 be a given constant. Here $a$ denotes the height of the box and $b$ denotes the width. Then there exists a container packing of $\R''\subseteq \R'$ inside a box of size $a\times(1+\epsau)b$(resp. $(1+\epsau)a\times b$)such that:
	\begin{enumerate}
	\item $\profit(\R'')\geq (1-O(\epsau))\profit(\R')$
	\item the number of containers is $O_{\epsau}(1)$ and their sizes belong to a set of cardinality $n^{O_{\epsau}(1)}$ that can be computed in polynomial time;
	\item the total area of the the containers is atmost $\area(\R')+\epsau ab$;  
	\end{enumerate}
	\end{lem}
	In the following subsections we show how to extend the above lemma using the same proof techniques and show at the end of each proof technique that the set of rectangles is still guillotine separable. Also we consider a=1 and b=1.
	\begin{lem}\cite{GalvezGHI0W17}
	Let $\eps$>0 and let $f(\cdot)$ be any positive increasing function such that $f(x)<x$ for all x. Then, $\exists \delta,\mu \in \Omega_{\eps}(1)$,with $f(\eps)\geq\mu$ such that the total profit of all rectangles whose width or height lies in $(\mu,\delta]$ is atmost $\eps\cdot \profit(\R')$.
	\end{lem}
	For now we use the value of $\eps$ required in this lemma as $\eps'_{ra}$ and later on define the function $f$ used. By choosing appropriate $\mu,\delta$ we classify the rectangles for this section as follows
	\begin{itemize}
%	\item small if $\height \leq \mu$ and $\width \leq \mu$;
%	\item horizontal if $\height \leq \mu$ and $\width > \delta$;
%	\item vertical if $\height >\delta$ and $\width \leq \mu$;
%	\item large if $\height >\delta$ and $\width>\delta$;
%	\item wide if the item is either horizontal or vertical.
	\item short if $\width \leq \mu$;
	\item narrow if $\height \leq \mu$;
	\item wide if $\width > \delta$;
	\item high if $\height >\delta$;
	\item Vertical is the item which is short as well as high i.e. $\height >\delta$ and $\width \leq \mu$;
	\item Horizontal is the item which is wide as well as narrow i.e. $\height \leq \mu$ and $\width > \delta$.
	\end{itemize}

	\subsection{Shifting Argument\cite{GalvezGHI0W17}}
	The procedure defined in this subsection is used as a tool at various steps of our proof of Resource Augmentation Lemma. Thus we define the processing and establish that it maintains guillotine property with losing no more than a small profit fraction as follows:
	\label{shifting1}
	\subsubsection{Process}
	%\begin{figure}[t]
	%\centering
	%\includegraphics[scale=1]{pic2}
	%\caption{For each vertical box,we can remove a low profit subset of rectangles(red in the picture),to make space for short-high rectangles that cross the right edge of the box(blue)\cite{GalvezGHI0W17}}
	%\label{shifting}
	%\end{figure}
	\begin{figure}[!tbh]
		%\centering
		\captionsetup[subfigure]{justification=centering}
		\hspace{-10pt}
		\begin{subfigure}[b]{.5\textwidth}
			\centering
			\resizebox{!}{4.5cm}{
			\begin{tikzpicture}
				%box		
				\draw[thick] (0,0) rectangle (6.08,6.08);
				\draw[solid, fill = gray] (-.12,.33) rectangle (.12,2.03);
				\draw[solid, fill = gray] (-.15,2.49) rectangle (.15,3.89);
				\draw[solid, fill = gray] (-.09, 4.3) rectangle (.09,5.93);
				\draw[solid, fill = lightgray] (.45,.45) rectangle (1.465,.75);
				\draw[solid, fill = lightgray] (.99, 4.47) rectangle (1.89,5.67);
				\draw[solid, fill = lightgray] (1.29, 1.07) rectangle (2.09,3.67);
				\draw[solid, fill = lightgray] (1.99, 4.97) rectangle (2.19,5.67);
	
	
				\draw[solid, fill = darkgray] (3.04,.75) rectangle (3.34,2.15);
				\draw[solid, fill = darkgray] (2.68,2.34) rectangle (2.98,3.74);
				\draw[solid, fill = darkgray] (2.3,3.92) rectangle (2.6,5.32);
	
				\draw[dashed] (2.45,0) -- ( 2.45, 6.08);
				\draw[dashed] (3.19, 0) -- ( 3.19, 6.08);
				
				\draw[solid, fill = lightgray] (3.92,.75) rectangle (4.56,3.04);
				\draw[solid, fill = lightgray] (5.39,2.29) rectangle (5.81,4.29);
				\draw[solid, fill = lightgray] (4.71,3.89) rectangle (5.13,5.89);
	
			\end{tikzpicture}}
			\caption{}
			\label{figure2}
		\end{subfigure}
		\begin{subfigure}[b]{.5\textwidth}
			\centering
			\resizebox{!}{4.5cm}{
			\begin{tikzpicture}
				%box			
				\draw[thick] (0,0) rectangle (6.08,6.08);
				
				\draw[solid, fill = lightgray] (.45,.45) rectangle (1.465,.75);
				\draw[solid, fill = lightgray] (.99, 4.47) rectangle (1.89,5.67);
				\draw[solid, fill = lightgray] (1.29, 1.07) rectangle (2.09,3.67);
				\draw[solid, fill = lightgray] (1.99, 4.97) rectangle (2.19,5.67);
	
	
		
	
				\draw[solid, fill = gray] (2.48,.33) rectangle (2.72,2.03);
				\draw[solid, fill = gray] (2.45,2.49) rectangle (2.75,3.89);
				\draw[solid, fill = gray] (2.51, 4.3) rectangle (2.69,5.93);
	
				\draw[dashed] (2.45,0) -- ( 2.45, 6.08);
				\draw[dashed] (3.19, 0) -- ( 3.19, 6.08);
				
				\draw[solid, fill = lightgray] (3.92,.75) rectangle (4.56,3.04);
				\draw[solid, fill = lightgray] (5.39,2.29) rectangle (5.81,4.29);
				\draw[solid, fill = lightgray] (4.71,3.89) rectangle (5.13,5.89);
			\end{tikzpicture}}
			\caption{}
			\label{figure1}
		\end{subfigure}
		\caption{For each packing originally arranged as in (a), we can remove a low profit subset of rectangles (darkgray in the picture), to make space for short-high rectangles that cross the left edge of the box (mediumgray)}
	\label{shifting}
	\end{figure}
	
	Consider a box $B$ with width $\delta^{2}$ consisting of vertical items only and leftmost edge intersecting some vertical items as shown in Figure \ref{figure2}. Also assume that the items in the box are guillotine separable Divide the box in vertical strips of width $\mu$. Using averaging argument, there must exist a strip where the weight of items which overlaps with it is atmost 2$\mu \profit(B)$ $\leq \epsau'\profit(B)$ where $\profit(B)$ denotes the total profit inside the box $B$. Now remove this low profit strip and place the items intersected by the leftmost edge of the box in the space created by the strip on top of one another. 
		\subsubsection{Guillotine Separability}
		The new set of items completely belonging to the strip processed in Section 6.1.1,  can be separated with guillotine cuts along the boundary of the strip. Since we delete all the rectangles lying either partially or completely on the strip, there is no rectangle which intercepts  the  cuts along the boundary of strip. Thus the strip can be guillotine separated from the rest of the knapsack. Given that the rest of the plane is already guillotine separable, it follows that the process of shifting maintains the guillotine structure.
	\subsection{Rounding wide rectangles}\label{roundwiderects}
We descirbe a procedure for rounding width and cordinates of wide items to nearest integral multiples of $\delta^{2}$ in this subsection. In the subsequent subsection \ref{box} we descirbe the procedure for packing vertical items as done in \cite{GalvezGHI0W17} thereby maintaining the guillotine property in the processing. We thus will be proving the following lemma in:
	% Proposition 59 of \cite{GalvezGHI0W17}}
\begin{lem}\label{verticalandbox}
Let $\R'$ be the set of guillotine separable items that can be packed into a $1\times1$ box. Then there exists a guillotine separable packing of a profitable subset $\R^{+}$ $\subset$ $\R'$ with profit of $\R^{+}$ is atleast $(1-O(\epsau')$$.\profit(\R')$ in a $1\times(1+2\delta)$ box such that:
\begin{itemize}
	\item Every wide item in $\R^{+}$ has width rounded up to the nearest multiple of $\delta^{2}$ and is shifted such that its leftmost ordinate is also an integral multiple of $\delta^{2}$.
	\item Every box in $B$ has width $\delta^{2}$ and stores atleast one vertical item packed in at most $1/\delta^{7}$ containers. 
\end{itemize}
\end{lem}
We prove the second point of Lemma \ref{verticalandbox} in the next subsection \ref{box}. For now we will be defining the processing done and prove the first point of the lemma. 
	\subsubsection{Process}
	%\begin{figure}[t]
	%\centering
	%\includegraphics[scale=1]{pic3}
	%\caption{Strips which share boundary with vertical cuts are shifted by $2\delta^{2}$}
	%\label{rounding}
	%\end{figure}
	
	\begin{figure}[b]
		%\centering
		\captionsetup[subfigure]{justification=centering}
		\hspace{-10pt}
		\begin{subfigure}[b]{.5\textwidth}
			\centering
			\resizebox{!}{4.5cm}{
			\begin{tikzpicture}
				%box		
				\draw[thick] (0,0) rectangle (26,18);
				\draw[solid, fill = lightgray] (0,6) rectangle (10,14);
				\draw[solid, fill = lightgray] (10,8) rectangle (18,16);
				\draw[solid, fill = lightgray] (18,4) rectangle (26,10);
				\draw[solid, fill = lightgray] (18,12) rectangle (26,18);
				\draw[dashed] (0,2) -- ( 26,2);
				\draw[dashed] ( 10,2) -- (10,18);
				\draw[dashed] ( 18,2) -- ( 18,18);	
			\end{tikzpicture}}
			%\caption{Cut 6: Compression of vertical item to vertical leg of L}
			\label{fig h}
		\end{subfigure}
		\begin{subfigure}[b]{.5\textwidth}
			\centering
			\resizebox{!}{4.5cm}{
			\begin{tikzpicture}
				%box			
				\draw[thick] (0,0) rectangle (30,18);
				\draw[solid, fill = lightgray] (0,6) rectangle (10,14);
				\draw[solid, fill = lightgray] (14,8) rectangle (22,16);
				\draw[solid, fill = lightgray] (22,4) rectangle (30,10);
				\draw[solid, fill = lightgray] (22,12) rectangle (30,18);
				\draw[dashed] (10,11) -- ( 14,11);
				\draw(12,12) node {\Huge \textbf{$2\delta^{2}$}};
			\end{tikzpicture}}
			%\caption{Cut 6: Compression of vertical item to vertical leg of L}
			\label{fig h}
		\end{subfigure}
		\caption{Strips which share boundary with vertical cuts are shifted by $2\delta^{2}$}
		\label{rounding}
	\end{figure}
	
	
	We start with optimal packing of rectangles belonging to $R'$. For now we remove the vertical rectangles in $R'$ which will be repacked later.
%We call the group of large and horizontal rectangles as wide rectangles.
Partition the wide rectangles into the groups $\{ $$R_{0}$,$R_{1}$,....,$R_{k-1}$$\}$ where $k=1/\delta$. Let $g(R)$ denote the distance between the leftmost edge of the knapsack and the leftmost vertical cut in the guillotine cutting sequence which separates the rectangles $R$ from the items left to it. Rectangles $R\in R_{i}$ have $\lfloor g(R)\rfloor=i\delta$. Now we describe a procedure on how to round the wide rectangles to the nearest integer multiple of $\delta^{2}$ and shift them horizontally so that the starting and ending coordinates is an integral multiple of $\delta^{2}$. Now consider rectangles in group $R_{0}$ from top to bottom and let these be $\{ R_{0_{1}},R_{0_{2}},...,R_{0_{m}}\}$ where $R_{0_{1}}$ is the topmost and $R_{0_{m}}$ is the bottom-most rectangle. Now consider the first vertical cut which separates $R_{0_{1}}$ from the rectangles right to it.
Now take the strips obtained after the guillotine cutting sequence which share a boundary with the previous vertical cut and shift these strips together to the right by $2\delta^{2}$ and repeat the procedure by considering each strip as pseudo rectangle and by considering the vertical strips in the same manner as before, shift the new strips which share boundary with these new strips as done in Figure \ref{rounding}. This process eventually terminates and the total increase in width is $2\delta^{2}$. Now we show that if we repeat the same procedure for the rest of the rectangles in $R_{0}$ there won't be any increase in the width of the knapsack. If the subsequent rectangle $R_{0_{2}}$ shares a vertical cut in the original $1\times1$ knapsack then we already have $2$$\delta^{2}$ space for the rectangles in the new $1\times(1+2\delta^{2})$ knapsack. Otherwise we continue with the same shifting process as done in case of the rectangle $R_{0_{1}}$. If there is any vertical cut which is shared with the vertical cuts obtained in the case of $R_{0_{1}}$ then there is no need to shift the strips which shared the boundary in the original $1\times1$ knapsack as they have been already shifted and there is $2\delta^{2}$ space left. Otherwise we continue and eventually reach the right most boundary where we have $2\delta^{2}$ space left. So there is no increase in the width. Now repeat the same procedure for the rest of the group of wide rectangles in the increasing order of the group numbers.   
	\begin{remark}\label{rem1}
	When we apply the above procedure to the group $R_{i}$ the groups $\{R_{0},R_{1},.....R_{i-1}\}$ remain unaffected.
	\end{remark}
	\begin{remark}
	Rectangles in group $R_{i}$ is shifted atmost $i$ times. So maximum number of times a rectangle is shifted is atmost $1/\delta$ and hence the extra width required is $1/\delta\cdot2\delta^{2}=2\delta$. So we can round the wide rectangles to the nearest integer multiple of $\delta^{2}$ and shift them horizontally so that the starting and ending coordinates are integral multiples of $\delta^{2}$.  
	\end{remark}
	\subsubsection{ Guillotine Separability }
		Basic idea considers the fact that we consider the strip of rectangles immediately right adjacent to $R$ as a pseudo item. The shifting of this pseudo item is done horizontally right to the nearest integral multiple of $2$$\delta^{2}$. Shifting horizontally doesn't disturb the guillotine separability as the guillotine cuts are always along the boundary of pseudo rectangle. We shift the entire guillotine partition (strip) to the immediate right of given rectangle. It follows from Remark \ref{rem1} that in every iteration the rectangles to the left of rectangle being processed remain unaffected. Since every iteration involves same shifting of pseudo rectangles horizontally to the right, the resulting rectangles in extended knapsack maintains guillotine structure.
	\subsection{Containers for vertical rectangles\cite{GalvezGHI0W17}}
	\label{box}
	Now we will descirbe the procedure for packing vertical items as done in \cite{GalvezGHI0W17} and thus establishing the safety of guillotine property in the processing. We will thus be establishing the proof of second point of lemma \ref{verticalandbox} thereby completing the proof of same as follows:
	\subsubsection{ Process }
	 Draw vertical lines spaced equally by $\delta^{2}$. In each vertical strip consider the maximal region which doesn't contain or overlap with any wide rectangle. We define a box for each such region which consists at least one vertical rectangle and denote such a set of boxes by $B$. Also consider $M:=(1+2\delta)/\delta^{2}$. A vertical rectangle can overlap with atmost $2$ vertical boxes and by considering these rectangles to be part of right of the two boxes and by the shifting argument as explained in subsection \ref{shifting1} we can have vertical boxes with no rectangle intersecting the boundary. By using the strip packing mentioned in \cite{kenyon2000near} we repack vertical items in a vertical box into atmost $1/\delta^{7}$ containers. 
	\subsubsection{ Guillotine Separability }
	The argument follows similarly as in subsection \ref{shifting1}. Consider each of these box as a pseudo-item. It can be separated by a sequence of guillotine cuts as there are no items intersecting the boundary after processing by shifting argument. So on a whole the knapsack is still guillotine separable. The repacking of vertical items maintains guillotine property as mentioned in \cite{kenyon2000near}. A pseudo-item can either be a single wide rectangle which is already guillotine separable or it can be strip packing of vertical rectangle which also follows guillotine property or it can be a set of items which follows guillotine property from original knapsack. Thus the new arrangement obtained maintains guillotine separability property. 
	\subsection{Packing wide rectangles into O(1) containers }
	\begin{lem}\cite{GalvezGHI0W17}
	Given rectangles at the end of subsection \ref{box} and considering the vertical boxes as pseudo-item there exists a packing of wide rectangles with profit $(1-O(\epsau')\profit(OPT)$ into $(K+3/\delta^{3})M2^{M}$ containers where $K\leq O_{\epsau',\delta}(1)$
	\end{lem}
	Intuitively the proof involves obtaining a fractional packing with $O(1)$ containers and then showing an existence of an integral packing with a profitable set of items.
	\subsubsection{Fractional Packing}\label{fracpack} 
	We follow the same procedure of fractionally packing the items as done in \cite{GalvezGHI0W17}. Following the processing in section \ref{box}, we obtain a set of guillotine separable items packed in boxes and a set of wide rectangles. Since the items inside the boxes are guillotine separable, we can consider a box as a single pseudo item and process it along with wide rectangles. Let us denote set of pseudo-items as $B$ and the set of wide items as $W$. The algorithm $Alg_{frac}$ takes in input a subset $K$ of $B$ and returns their fractional packing as follows. We have $R_{slice}$ as the set $K$ $\bigcup$ $W$. Draw end to end horizontal lines along horizontal edges of all the items $\R$ $\in$ $R_{slice}$ slicing the rest of the rectangles of knapsack. Each such end to end horizontal slice so formed is termed as a slice. We then define $configuration$ as the set of intercepts of vertical edges of items with the horizontal line at the given $y$-coordinate. We slice the rectangles suitably to arrange stripe with same configuration together. We then pack sliced rectangles into $M:=(1+2\delta)/\delta^{2}$ number of containers. Each stripe can have atmost $2^{M-1}$ configurations, which implies each stripe can contain at most $M2^{M-1}$ containers. Thus the total number of containers is atmost $2\times(|R_{slice}|+1)$$\times$$M2^{M-1}$. Since $|W|$$\leq$$\frac{1}{\delta^{2}}$ which follows from subsection \ref{box}, we get $|R_{slice}| \leq |K| + \frac{1}{\delta^{2}} $. Thus total number of containers cannot exceed $ (|K| + \frac{3}{\delta^{3}}) $$\times$$M2^{M}$.
	\begin{remark}
	Guillotine Separability : While slicing and rearranging of rectangles during the fractional packing, the slided rectangles  remains within the initial stripe created by extending the top and bottom edges of pseudoitems and some wide items and therefore vertical boxes as pseudoitems and some wide items which are never sliced are guillotine separable. Also the containers obtained at the end of this stage are guillotine separable as the container's height is equal to the height of the configuration\cite{GalvezGHI0W17} and no container is part of 2 different configuration.
	\end{remark}
	\subsubsection { Integral Packing } 
	We follow a greedy - recursive approach to convert the fraction packing obtained in section \ref{fracpack} to an integral packing without loosing much profit from optimal packing same as in \cite{GalvezGHI0W17}. The greedy algorithm $Alg_{G}$ run at each iteration proceeds as follows. Given a set of items obtained after fractional packing, pick items with same widths and try packing them in the same container. Either all items can be packed or single item can be left outside, we just discard the item ,close our current container and start packing in the other containers. We now propose the recursive formulation for integral packing. Consider set of items $S_{0}$ s.t. $S_{0}= \phi$. Run $Alg_{frac}$ on $S_{0}$, followed by $Alg_{G}$ on the output of fractional packing. Analyze the profit of set of items discarded say $S_{1}$ in greedy algorithm and it is clear that the number is bounded by the number of corridors. Thus the number of items $S_{1}$ i.e. $|(S_{1})|$ $\leq$$ (|S_{0}| + \frac{3}{\delta^{3}}) $$\times$$M2^{M}$. Check if $\profit(S_{1})$ $\leq$ $\eps'_{ra}$$\profit(OPT)$. If yes we have our set $S$$=$$S_{0}$ and an integral packing with the set $S_{0}\bigcup W$$\backslash$$S_{1}$. If not we recursively run $Alg_{frac}$ on $S$$=$$S_{0}\bigcup S_{1}$, followed by $Alg_{G}$ on the output of fractional packing. Same as before we consider the set of discarded items as $S_{3}$ which is bounded by number corridors ( $\leq $$ (|S| + \frac{3}{\delta^{3}}) $$\times$$M2^{M}$). Proceeding recursively every set $S_{k}$ is bounded by $|S_{k}|$ $\leq$ $ (|S_{0}+S_{1}+S_{2}+...+S_{k-2}+S_{k-1}|$ + $\frac{3}{\delta^{3}}) $$\times$$M2^{M}$ which implies $|S_{k}|$ $\leq$ ($\frac{3}{\delta^{3}} $$M2^{M}$ $\times$$M2^{M}$$)^{k}$. Thus k can at most be $\frac{1}{\eps'_{ra}} - 1$. Therefore number of containers is atmost $|S_{\frac{1}{\eps'_{ra}} - 1}|$ = $O_{\epsau',\delta}(1)$. Thus we are packing subset $I'$ of given set of items $I$ in $O_{\epsau',\delta}(1)$ containers without losing no more than constant fraction of profit i.e. $\profit(I')$ $\leq$ $\eps'_{ra}$$\profit(I)$
	
	 \begin{remark}
	Guillotine Separability : During integral packing, the rectangles of same width are packed on top of each other in the guillotine separable containers. So after the integral packing the rectangles are still guillotine separable. 
	\end{remark}
	\subsection{Rounding down horizontal and vertical containers}
	\begin{lem}\cite{GalvezGHI0W17}
	Let $C$ be a horizontal (resp. vertical) container defined above, and let $\R_{C}$ be the set of rectangles packed in $C$. Then, it is possible to pack a set $\R_{C}'\subseteq \R_{C}$ of profit at least $(1-3\epsau')\profit(\R_{C})$ in a set of at most $\lceil \log_{1+\epsau'}(1/\delta) \rceil /\epsau'^{2}$ horizontal (resp. vertical) containers that can be packed inside $C$ and such that their total area is at most $\area(I_{C})$.
	\end{lem}
	We begin with processing horizontal rectangles first (similar proof holds for vertical rectangles). Define a group of horizontal rectangles $\R_{1},\R_{2},...,$ in a single horizontal container $C$ where the width of the widest rectangle $\R_{j}$ is bigger than the smallest one by a factor of 1+$\epsau'$ and define container $C_{j}$ for each such group. Then in each such new container $C_{j}$  the operations done are either removing a set of low profit rectangles or making one container for a certain set of rectangles and shrinking the container with remaining rectangles. 
\begin{remark}
Guillotine Separability : Operations performed in the processing in this section involve deleting of items and shrinking of containers. It is trivial that deleting items doesn't disturb the guillotine property of remaining set of items. All containers when considered as pseudo-rectangles can be separated by guillotine cuts. Shrinking of any such pseudo-rectangle doesn't disturb this guillotine structure. In fact guillotine separability inside such a pseudo item isn't affected as shrinking of plane (shrinking along axis parallel directions doesn't affect the existing guillotine cuts inside it). Therefore the packing obtained after the whole processing follows guillotine separability.
	\end{remark}
	\subsection{Packing small rectangles}
	\begin{lem}\cite{GalvezGHI0W17}
	In a $1\times(1+\epsau')$  knapsack, there exists a packing of small rectangles into atmost $O_{\epsau'}(1)$ area containers such that the property (3) of Lemma \ref{lemma1} is satisfied.
	\end{lem}
	We process the knapsack by creating a non-uniform grid by extending each side of the containers until they hit the boundary or the other containers. Plus a uniform grid is created by adding vertical and horizontal rectangles which are spaced by a distance of $\epsau'$. Now cells  which do not overlap with any other container are defined to be free cell. Then the small rectangles are packed into free cells with both dimensions at least $8\mu/\epsau'$ and possibly an extra container $C_{S}$ with height and width $\epsau'/2$ using NFDH. Then items $R'_{D}\subseteq R_{D}$ in an area container $D$ is taken and repacked into a container $D'$ such that $\profit(R'_{D})\geq(1-4\epsau')\profit(R_{D})$ and width of $D'$ is $\width(D)$ and height is $(1-\epsau')\height(D)$. The previous procedure is not applied to $C_{S}$.
	\begin{remark}
	Guillotine Separability : During construction only we get the sequence of guillotine cuts along the grid which separated out the containers individually. Since the grid is formed by extending the boundaries of the containers, we can claim that they form guillotine cuts because containers so obtained from previous subsection were guillotine separable. Moreover the packing of small rectangles inside the grid cells can be isolated from same sequence of cuts. Since items within such a packing are packed using NFDH the arrangement is guillotine separable. Thus we conclude that the arrangement so obtained follows guillotine property.
	\end{remark}
	\subsection{Rounding containers to a polynomial set of sizes}
	\begin{definition}
	For a set $\R$ of rectangles, we define $WIDTHS(\R)=\{\width_{j}|R_{j}\in \R\}$ and $HEIGHTS(\R)=\{\height_{j}|R_{j}\in \R\}$.
	\end{definition}
	\begin{definition}
	Given a finite set $P$ of real numbers and a fixed natural number $k$, we define the set $P^{(k)}=\{(p_{1}+p_{2}+...+p_{l}\}+ip_{l+1}|p_{j}\in P \forall j,l\leq k,0\leq i\leq n, i  \in I \}$.
	\end{definition}
	\begin{lem}
	\label{lemma2}\cite{GalvezGHI0W17}
	Let $\eps$>0, and let $\R$ be set of rectangles packed in a horizontal or vertical container $C$. Then for any $k\geq 1/\eps$, there is a set $\R' \subseteq \R$ with profit $\profit(\R')\geq(1-\eps)\profit(\R)$ that can be packed in a container $C'$ smaller than $C$ such that $\width(C)\in WIDTHS(\R)^{(K)}$ and $\height(C)\in HEIGHTS(\R)^{(K)}$. 
	\end{lem} 
	\begin{proof} We prove the argument for vertical containers and the similar construction follows for horizontal case. The basic sketch revolves around linear grouping of items according to widths and further rounding to a given set of choices. Consider set of items $R$ in the container in sorted order of widths. If $|R|$ is sufficiently small, i.e., $\leq$ $\frac{1}{\eps}$ then we already meet the condition $\sum_{r \in R}w_{r}$ $\in$ $WIDTHS(\R)^{(K)}$. If not, we consider the set of items, say $R'$, with largest width from the set of sorted items such that $|R'|$ $\leq$ $\frac{1}{\eps}$. Using averaging argument, there must exist an item $r$ $\in$ $R'$ such that $\profit(r)$$\leq$$\eps\profit(R')$. We can safely discard $r$ without losing no more than constant $O(\eps)$ profit. Consider the set $R\backslash R'$, every item in the set has width almost $\width(r)$, sum of widths of all items in $R\backslash {r}$ is at most $(n - \frac{1}{\eps})\width(r)$. Thus we can pack all the items in $R \backslash {r}  $ in a new container. The sum of widths of items in the container is $\width( R \backslash {r})$ $=$ $\width(R') + (\lceil \frac{\width(R\backslash R')}{\width(r)} \rceil ) \width(r) $ $\leq$ $\width(R') + n$$\width(r) $. Thus width of the new container belongs to the set $WIDTHS(R)^{(K)}$. The given choice of factor $(\lceil \frac{\width(R\backslash R')}{\width(r)} \rceil )$ $\leq$ $n$ implies that the width of new container formed is at most width of original container considered.
	\end{proof}
	\begin{remark}
	Guillotine Separability : Applying processing done in Lemma \ref{lemma2} to a vertical container maintains guillotine separability as items are stacked beside each other, i.e., items are packed side by side sharing at most one common vertical edge and can thus be separated by single stage vertical guillotine cuts. Similar argument follows for proving guillotine separability of horizontal containers. Thus Lemma \ref{lemma2} maintains guillotine separability.
	\end{remark}
	\begin{lem}
	\label{lemma3}\cite{GalvezGHI0W17}
	Let $\eps$>0, and let $\R$ be a set of rectangles that are assigned to an area container $C$. Then there exists a subset $\R'\subseteq\R$ with profit $\profit(\R')\geq(1-3\eps)\profit(\R')$ and a container $C'$ smaller $C$ such that: $\area(\R')\leq\area(C)$,$\width(C')\in WIDTHS(\R)^{(0)}$,$\height(C')\in HEIGHTS(\R)^{(0)}$,and each $R_{j}\in\R'$ is $\frac{\eps}{1-\eps}$-small for $C'$.
	\end{lem}
	\begin{proof}
It follows from the initial assumption that items in any container $C$ are $\eps$-small for $C$, i.e., $\forall R \in \R$ which are packed inside $C$ $\width(R)$ $\leq$ $\eps\width(C)$ and $\height(R)$ $\leq$ $\eps\height(C)$. Thus $a(R) \leq \eps^{2} a(C)$. We first shrink the container C such that boundaries of C coincide with extreme edges of items in the set of packed items $\R$. Let $\width_{max}(\R)$ and $\height_{max}(\R)$ be respectively be the maximum height and width of items in $\R$. We further reduce the dimension of C by rounding off to maximum multiple of maximum item width ( resp. height ) less than the original dimension. The new container $C_{1-\eps}$ formed is such that the $\width(C_{1-\eps})$ $=$ $\width_{max}(I)$ $ \lfloor \frac{\width(C)}{\width_{max}(I)} \rfloor$ and  $\height(C_{1-\eps})$ $=$ $\height_{max}(I)$ $ \lfloor \frac{\height(C)}{\height_{max}(I)} \rfloor$.
We then follow a greedy approach to pack a subset $\R'$ $\subset $ $\R$ in container $C_{1-\eps}$. Pack the item in order of non-increasing area-density ( profit/area ) using NFDH. 
	Now we analyze the process followed above and prove the bounds. We get $a(C') = ( 1 - \eps )^{2} a(C)$ $\geq$ $a(C)$. Since we pack as many items as possible in the area and the area of each item in $\R$ is at most $\eps^{2}$, the area of items $I'$ packed in $C'$  is $a(\R')$ $\geq$ $(1-\eps - \eps^{2} ) a(C) $. Thus we get $\profit(\R') \geq (1 - 3$$\eps) \profit(\R)$. The items in $\R'$ are $\frac{\eps}{1-\eps}$-small for the new container. Also by rounding the dimensions of container to integral multiple of maximum dimensions of items packed inside, we get $\width(C')$ $\in$ $WIDTHS(I)^{(0)}$ and $\height(C')$ $\in$ $HEIGHTS(I)^{(0)}$. This concludes the proof of lemma.
	\end{proof}
	\begin{remark}
	Guillotine Separability : All containers when considered as pseudo-rectangles can be separated by guillotine cuts. Shrinking of any such pseudo-rectangle doesn't disturb this guillotine structure. In fact guillotine inside such a pseudo item isn't affected as shrinking of plane ( shrinking along axis parallel directions doesn't affect the existing guillotine cuts inside it ). Since items within such a packing are packed using NFDH the arrangement is guillotine separable. Thus we conclude that the arrangement so obtained follows guillotine property.
	\end{remark}
	By considering $\eps=\epsau'$ and applying Lemma \ref{lemma2} and Lemma \ref{lemma3} to all containers, we have completed the proof of Lemma \ref{lemma1} as $\frac{\epsau'}{1-\epsau'}\leq\epsau$. Also we have proved that Lemma \ref{lemma1} can be extended to the case of guillotine separable rectangle and hence we get one sided resource augmentation for guillotine separable rectangles. 


==> 6_Rotated_Cardinality.tex <==
	
\section{$(\frac{5}{4}+\eps)$-approximation \tggkcr}\label{sec:tggkcrfull}
We will continue to assume that we have only skewed items and we can remove $O(1)$ number of items, we use the same notations as the previous section.
Let $APX$ be the best container-based packing. 
As in Lemma \ref{algo1}, the processing of subcorridors give:
	\begin{lem}
	$|APX|\geq |\opt_{F}|+|\opt_{T}|/2$.
	\label{rlem1}  
	\end{lem}
	
	\begin{lem}\cite{GalvezGHI0W17}
	$|APX|\geq \frac{2|\opt_{F}|}{3}+|\opt_{T}|$.
	\label{rlem2}  
	\end{lem}
	\begin{proof}
	
	Lemma \ref{rlem2} holds even in the case of guillotine setup as the proof techniques used in \cite{GalvezGHI0W17} don't disturb the guillotine property. Only processing done during the proof include deletion of items and replacement (rotating sub-pieces and \emph{mirroring}) of sub-pieces containing items completely inside it. The deletion of items from optimal guillotine packing cannot disturb the guillotine property. Replacement of sub-pieces with items completely inside it, can be considered as rotation or mirroring of a pseudoitem which is guillotine separable. Removing this pseudoitem from packing leaves another guillotine separable sub-piece and then augmenting it back to the already guillotine separable plane maintains guillotine property. Thus summing up, guillotine separability is maintained after the processing.
	\end{proof}
	%\begin{figure}[!htb]
	%\centering
	%\includegraphics[scale=.7]{T+34SF}
	%\caption{Case: T+3/4SF processing}
	%\label{T+3/4SF-}
	%\end{figure}
	
	%%% added by Arindm
From Lemmas \ref{rlem1}, \ref{rlem2}, we get $\profit(APX)\geq(\frac{4}{5}-O(\eps))\profit(\opt)$.
The worst case is obtained when $\profit(\opt_{T}):\profit(\opt_{F})=2:3$.
\begin{thm}
\label{LCR}
Let $APX$ be the most profitable solution that is packed by a guillotine separable container packing and $\opt$ be optimal  packing for \tggkc. Then $\profit(APX)\geq(\frac{4}{5}-O(\eps))\profit(\opt)$.
\end{thm}
%
%\subsection{Part below is not required}
%
%	
%	
%	%\begin{figure}[!htb]
%	%\centering
%	%\includegraphics[scale=.7]{L+ST}
%	%\caption{Case : L+ST processing}
%	%\label{L+ST Processing}
%	%\end{figure}
%	
%		\begin{figure}[!htb]
%		%\centering
%		\captionsetup[subfigure]{justification=centering}
%		\hspace{-10pt}
%		\begin{subfigure}[b]{.32\textwidth}
%			\centering
%			\resizebox{!}{4.5cm}{
%			\begin{tikzpicture}
%				%box		
%				\draw[thick] (0,0) rectangle (8.0,8.0);
%				\draw[solid , fill = lightgray] (0,0)-- ( 8.0, 0) -- ( 8.0 , 6.2 ) -- ( 6.2, 6.2 ) -- ( 6.2, 8.0 ) -- ( 0 , 8.0 ) -- ( 0,0 ) ;
%				
%				\draw [dashed] ( .2,8.0) -- (.2 ,.2 ) -- ( 8.0, .2) ;
%				\draw [dashed] ( .6,8.0) -- ( .6, .6) -- ( 8.0, .6) ;
%				\draw [dashed] ( 1.4,8.0) -- ( 1.4, 1.4) -- ( 8.0,1.4 ) ;
%				\draw [dashed] ( 3.0,8.0) -- ( 3.0, 3.0) -- ( 8.0,3.0 ) ;
%				\draw [dashed] ( 6.2,8.0) -- (6.2 ,6.2 ) -- ( 8.0, 6.2) ;	
%	
%				\draw [dashed] ( 6.2,6.2) -- ( 6.2, 5.0) -- ( 5.0,5.0) -- ( 5.0, 4.0 ) -- ( 4.0 , 4.0 ) --( 4.0, 3.5) -- ( 3.5, 3.5) --( 3.0, 3.5)  -- ( 3.0 , 3.0) ;
%				\draw [dashed] ( 3.0 , 3.0 ) -- ( 3.0 , 2.0 ) -- ( 2.0 , 2.0 ) -- ( 2.0 , 1.4) -- ( 1.4, 1.4) ;
%				\draw [dashed] ( 1.4, 1.4) -- ( 1.0 , 1.4) -- ( 1.0 , 1.0 ) -- ( .6, 1.0 ) --( .6, .6) ;
%				\draw [dashed] ( .6,.6) -- ( .6 , .4) -- ( .4, .4) -- ( .4, .2) -- ( .2, .2);
%				\draw [dashed] ( .2, .2) -- ( .1 ,.2 ) -- ( .1, .1) -- ( 0 , .1) -- ( 0,0);	
%	
%				%labeling 
%				\draw (0,8.3) node {   \textbf{$2\eps'$}};
%				\draw (.5,8.3) node {  \textbf{$6\eps'$}};
%				\draw (1.0,8.3) node {   \textbf{$12\eps'$}};
%				\draw (2.2,8.3) node {   \textbf{$24\eps'$}};
%				\draw (4.6,8.3) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
%	
%				\draw (8.5,.1) node {   \textbf{$\leq 2\eps'$}};
%				\draw (8.5,.4) node {  \textbf{$\leq 6\eps'$}};
%				\draw (8.5,1) node {   \textbf{$\leq 12\eps'$}};
%				\draw (8.5,2.2) node {   \textbf{$\leq 24\eps'$}};
%				%\draw (9.1,4.6) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
%	
%			\end{tikzpicture}}
%			\caption{}
%		\end{subfigure}
%		\begin{subfigure}[b]{.32\textwidth}
%			\centering
%			\resizebox{!}{4.5cm}{
%			\begin{tikzpicture}
%				%box					
%				\draw[thick] (0,0) rectangle (8.0,8.0);
%				\draw[solid , fill = lightgray] (0,0)-- ( 8.0, 0) -- ( 8.0 , .6 ) --( .6,.6) -- ( .6, 8.0 ) -- ( 0, 8.0 ) -- ( 0,0);
%				\draw[solid , fill = lightgray] ( 8.0, 1.4) -- ( 1.4, 1.4) -- ( 1.4, 8.0 ) -- ( 6.2 , 8.0) -- ( 6.2, 6.2) -- ( 8.0 , 6.2) ;
%	
%				% dashed line 
%				\draw[dashed] ( 1.2, .6) --( 1.2, 8.0) ;
%				
%				\draw [dashed] ( .2,8.0) -- (.2 ,.2 ) -- ( 8.0, .2) ;
%				\draw [dashed] ( .6,8.0) -- ( .6, .6) -- ( 8.0, .6) ;
%				\draw [dashed] ( 1.4,8.0) -- ( 1.4, 1.4) -- ( 8.0,1.4 ) ;
%				\draw [dashed] ( 3.0,8.0) -- ( 3.0, 3.0) -- ( 8.0,3.0 ) ;
%				\draw [dashed] ( 6.2,8.0) -- (6.2 ,6.2 ) -- ( 8.0, 6.2) ;	
%	
%				\draw [dashed] ( 6.2,6.2) -- ( 6.2, 5.0) -- ( 5.0,5.0) -- ( 5.0, 4.0 ) -- ( 4.0 , 4.0 ) --( 4.0, 3.5) -- ( 3.5, 3.5) --( 3.0, 3.5)  -- ( 3.0 , 3.0) ;
%				\draw [dashed] ( 3.0 , 3.0 ) -- ( 3.0 , 2.0 ) -- ( 2.0 , 2.0 ) -- ( 2.0 , 1.4) -- ( 1.4, 1.4) ;
%				%\draw [dashed] ( 14, 14) -- ( 10 , 14) -- ( 10 , 10 ) -- ( 6, 10 ) --( 6, 6) ;
%				\draw [dashed] ( .6,.6) -- ( .6 , .4) -- ( .4, .4) -- ( .4, .2) -- ( .2, .2);
%				\draw [dashed] ( .2, .2) -- ( .1 ,.2 ) -- ( .1, .1) -- ( 0 , .1) -- ( 0,0);
%	
%	
%					%labeling 
%				\draw (0,8.3) node {   \textbf{$2\eps'$}};
%				\draw (.5,8.3) node {  \textbf{$6\eps'$}};
%				\draw (1.0,8.3) node {   \textbf{$12\eps'$}};
%				\draw (2.2,8.3) node {   \textbf{$24\eps'$}};
%				\draw (4.6,8.3) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
%	
%				\draw (8.5,.1) node {   \textbf{$\leq 2\eps'$}};
%				\draw (8.5,.4) node {  \textbf{$\leq 6\eps'$}};
%				\draw (8.5,1) node {   \textbf{$\leq 12\eps'$}};
%				\draw (8.5,2.2) node {   \textbf{$\leq 24\eps'$}};
%				%\draw (9.1,4.6) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
%	
%			\end{tikzpicture}}
%			\caption{}
%		\end{subfigure}
%			\begin{subfigure}[b]{.32\textwidth}
%			\centering
%			\resizebox{!}{4.5cm}{
%			\begin{tikzpicture}
%				%box					
%				\draw[thick] (0,0) rectangle (8.0,8.0);
%				%\draw[solid , fill = lightgray] (0,0)-- ( 80, 0) -- ( 80 , 6 ) --( 6,6) -- ( 6, 80 ) -- ( 0, 80 ) -- ( 0,0);
%				\draw[solid , fill = lightgray] ( 8.0, 1.4) -- ( 1.4, 1.4) -- ( 1.4, 8.0 ) -- ( 6.2 , 8.0) -- ( 6.2, 6.2) -- ( 8.0 , 6.2) ;
%	
%				% dashed line 
%				%\draw[dashed] ( 12, 6) --( 12, 80) ;
%				
%				\draw [dashed] ( .2,8.0) -- (.2 ,2 )  ;
%				\draw [dashed] ( .6,8.0) -- ( .6, 6) ;
%				\draw [dashed] ( 1.4,8.0) -- ( 1.4, 1.4)  ;
%				\draw [dashed] ( 3.0,8.0) -- ( 3.0, 3.0) -- ( 8.0,3.0 ) ;
%				\draw [dashed] ( 6.2,8.0) -- (6.2 ,6.2 ) -- ( 8.0, 6.2) ;	
%	
%				\draw [solid , fill = lightgray] ( 6.2,6.2) -- ( 6.2, 5.0) -- ( 5.0,5.0) -- ( 5.0, 4.0 ) -- ( 4.0 , 4.0 ) --( 4.0, 3.5) -- ( 3.5, 3.5) --( 3.0, 3.5)  -- ( 3.0 , 3.0) -- ( 3.0, 8.0) -- ( 6.2, 8.0 ) -- ( 6.2, 6.2)  ;
%				\draw [solid , fill = lightgray] ( 3.0 , 3.0 ) -- ( 3.0 , 2.0 ) -- ( 2.0 , 2.0 ) -- ( 2.0 , 1.4) -- ( 1.4, 1.4) -- ( 1.4, 8.0 ) -- ( 3.0, 8.0) -- ( 3.0, 3.0) ;
%				\draw [solid, fill = lightgray] ( 1.07, 8.0) -- ( 1.07, 1.0 ) -- ( 1.0 , 1.0) -- ( 1.0, .6) -- ( .6, .6) -- ( .6, 8.0) -- ( 1.07, 8.0);
%				\draw [solid , fill = lightgray] ( .6,.6) -- ( .6 , .4) -- ( .4, .4) -- ( .4, .2) -- ( .2, .2) -- ( .2, 8.0) -- ( .6, 8.0 ) -- ( .6, .6) ;
%				\draw [solid , fill = lightgray] ( .2, 8.0) -- ( .2, .2) -- ( .1 ,.2 ) -- ( .1, .1) -- ( 0 , .1) -- ( 0,0) -- ( 0 , 8.0) -- ( .2, 8.0) ;
%	
%	
%			% items 
%				\draw[ solid , fill = darkgray] (1.1,5.0) rectangle (1.2,7.5); 
%				\draw[ solid , fill = darkgray] (1.15,1.4) rectangle (1.24,3.0); 
%				\draw[ solid , fill = darkgray] (1.25,2.0) rectangle (1.3,6.0); 
%	
%			% dotted line
%				\draw [ dashed ] ( 1.3, 0 ) -- ( 1.3, 8.0) ;
%				\draw [ dashed ] ( 1.4, 0 ) -- ( 1.4, 8.0) ;
%	
%	
%				%labeling 
%				\draw (0,8.3) node {   \textbf{$2\eps'$}};
%				\draw (.5,8.3) node {  \textbf{$6\eps'$}};
%				\draw (1.0,8.3) node {   \textbf{$8\eps'$}};
%				\draw (2.2,8.3) node {   \textbf{$24\eps'$}};
%				\draw (4.6,8.3) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
%	
%				%\draw (8.5,.1) node {   \textbf{$\leq 2\eps$}};
%				%\draw (8.5,.4) node {  \textbf{$\leq 6\eps$}};
%				%\draw (8.5,1) node {   \textbf{$\leq 12\eps$}};
%				\draw (8.5,2.2) node {   \textbf{$\leq 24\eps'$}};
%				%\draw (9.1,4.6) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
%			\end{tikzpicture}}
%			\caption{}
%		\end{subfigure}
%	\caption{Case : L+ST processing [$\eps' = \epsr]$}
%	\label{L+ST Processing}
%	\end{figure}
%	
%	\begin{lem}
%	\label{rlem4}
%	$|\opt_{L\&C}|\geq (1-O(\eps))|\opt_{LF}|+|\opt_{ LT}|+|\opt_{ST}|$.
%	\end{lem}
%	\begin{proof}
%Consider the optimal packing and remove the items of $\opt_{SF}$. Now pack the items in $\opt_{LF}\cup \opt_{ LT}$ in the boundary $L$. Now partition the boundary L into $\frac{1}{2\eps_{rot}}$ smaller $L$ regions placed on top of each in the non-decreasing order of width of  $L$, where width of $L$ is the maximum of the height of the horizontal subcorridor and width of the vertical subcorridor. Here we assume that the sum of width of vertical subcorridor and height of horizontal subcorridor is more than $N$ otherwise we can rotate one of the subcorridor and place it to the side of the subcorridor and remove least profitable strip of width $\eps N$ and place all the items of $\opt_{ST}$. Let $\{L_{1},L_{2},...,L_{ \frac{1}{2\eps_{rot}}}\}$ be the set of smaller $L$ such that $L_{1}$ is the leftmost $L$ and $L_{ \frac{1}{2\eps_{rot}}}$ is the rightmost $L$. We now define the width of the smaller L regions and let us denote width by $w_{l}(.)$.  $w_{l}(L_{1})$ is $2\epsr$ and $w_{l}(L_{i})=\sum_{l=1}^{i-1}w_{l}(L_{l})+4\epsr$ for $2\leq i\leq \frac{1}{2\eps_{rot}}-1$. Note that $L_{\frac{1}{2\eps_{rot}}}$ automatically gets defined. If we choose $\eps_{rot}$ such that  $\eps_{rot}\geq \frac{1}{2(1+\frac{1}{log_{2}(\frac{1}{12\epsr})})} $ then we can ensure that $w_{l}(L_{\frac{1}{2\eps_{rot}}})\geq \sum_{l=1}^{i-1}w_{l}(L_{l})+4\epsr$. Now by averaging argument there exists a $L_{k}$ where $k \in [\frac{1}{2\eps_{rot}}]$ such that the number of rectangles intersecting $L_{k}$ is atmost $O(\eps_{rot})|\opt_{LF}\cup \opt_{ LT}|$. Now remove the rectangles intersecting this $L_{k}$. Without loss of generality we assume that the width of vertical subcorridor of $L_{k}$ is equal to $w_{l}(L_{k})$. Now rotate the horizontal subcorridors of $L_{i}$ where $1\leq i \leq k-1$ and place in the empty space created by removing $L_{k}$. Now there exists a vertical strip of width atleast $4\epsr N$. Now place the items of $\opt_{ST}$ and $\opt_{LT}$ in this strip. Now we are left with a strip of width atleast $2\epsr N$. Now we process the complete L region comprising of $L_{k+1},...,L_{\frac{1}{2\eps_{rot}}}$ as done in subsection \ref{prosec}. The least profitable strip which we remove as done in Lemma \ref{rlem1} can be packed in the vertical strip which is previously empty. This strip has width of atmost $2\epsr N$. Now we have a container packing. Hence our claim is proved.   
%\end{proof}
\subsection{Finding the packing in polynomial time}% \arir{write in more details}
%Using GAP(as mentioned in \cite{GalvezGHI0W17}) and brute forcing among polynomial number of options we can find the packing which gives the desired approximation factor in polynomial time.
This section is analogous to section \ref{sec:findpack}. We know that the there is a packing with $O_{\eps,\epsl}(1)$ number of containers of type $\Bc$ or $\Lc$. Also from Theorem \ref{LCR}, we establish that the given packing has a profit of at least $(\frac{4}{5}-O(\eps))\profit(\opt)$ which gives us an approximation factor of $\frac{5}{4}+O(\eps)$. We appropriately set all other constants as done in  \ref{sec:findpack} in $O_{\eps}(1)$ time. We take into account two packings as from \ref{rlem1} and \ref{rlem2} to pack the rectangles and consider the best of two. Since both the packings are container packing with constant number of containers and a possible size set for containers has cardinality $n^{O_{\eps,\epsl}(1)}$, we guess a near optimal  guillotine separable container packing. Then we use PTAS from Lemma \ref{lem:findPacking} since it is applicable to rotated case as well and conclude that we can find both the packings in polynomial time.

	


==> 7_Non_Rotated_Weighted.tex <==
\section{Weighted case}\label{w2dgk}
\subsection{Shifting Argumentation\cite{GalvezGHI0W17}}
\label{subsec:shifting}
%	We use similar process as used as in \cite{GalvezGHI0W17} and prove that if we begin with a guillotine separable solution, the process results in a final guillotine separable arrangement.
We aim to pack back the items dropped in all the previous steps of processing. Reconsidering the items dropped, i.e., $\opt_{kill}$, $\optla$, $\opt_{corr}^{cross}$, we give a similar processing as devised in \cite{GalvezGHI0W17} for packing these items with just losing a small fraction of profit. Intuitively we divide the knapsack into a grid iteratively and observe the profit of items dropped as a result of processing the items which are classified depending on the grid. Using standard averaging argument, we can claim that recursively doing the same procedure for $\frac{1}{\eps}$ times we get a set of items which can be dropped and have a profit of $O(\eps)$.

		\subsubsection{Grid and Corridor Partition}\label{gridpartition}
		We define $K(t)$ to be the set of items dropped in $i^{th}$ iteration and $\kappa(t)$ as the union of first $t$ sets $K(0),..., K(t)$. We initiate $K(0)$ to be the union of set of all items dropped in all the processing steps before (e.g., $\opt_{large}$, $\opt_{K}$, $\opt_{corr}^{cross}$). If the profit of items in $K(t)$ at any iteration $t$ is at most $\eps \profit(\opt)$ we get the desired set of items and halt.
Consider $t^{th}$ iteration, we denote $G(t)$ as the grid formed by extending the $x$, $y$ coordinates of the items in $\kappa(t)$. Consider $C_{t}$ to be the set of grid cells of $G(t)$. We classify items in the knapsack as small, large, horizontal, vertical as before depending on its intersection with the cells it overlaps. \\
An item $i$ having non-zero intersection with a cell $C$ $\in$ $C_{t}$ is classified inside $C$ as follows:
\begin{enumerate}
\item $\opt^{t}_{ver}(C)$, if  $\height(i \cap C)$ $>$ $\eps_{large}$ $\height(C)$ and $\width(i \cap C)$ $\leq$ $\eps_{small}$ $\width(C)$, 

\item $\opt^{t}_{hor}(C)$, if $\height(i \cap C)$ $\leq$ $\eps_{small}$ $\height(C)$ and $\width(i \cap C)$ $>$ $\eps_{large}$ $\width(C)$, 

\item $\opt^{t}_{large}(C)$, if $\height(i \cap C)$ $>$ $\eps_{large}$ $\height(C)$ and $\width(i \cap C)$ $>$ $\eps_{large}$ $\width(C)$, 

\item $\opt^{t}_{small}(C)$, if $\height(i \cap C)$ $\leq$ $\eps_{small}$ $\height(C)$ and $\width(i \cap C)$ $\leq$ $\eps_{small}$ $\width(C)$, 


\item $\opt^{t}_{intermediate}(C)$, if $\height(i \cap C)$ $\in$ $(\eps_{small}$ $\height(C)$,  $(\eps_{large}$ $\height(C)]$ or  $\width(i \cap C)$ $\in$ $(\eps_{small}$ $\width(C)$,  $(\eps_{large}$ $\width(C)]$ 

\item $\opt^{t}_{skew}(C)$ $=$  $\opt^{t}_{hor}(C) \cup \opt^{t}_{ver}(C)$.
\end{enumerate}

As done in previous sections, we can fix $\eps_{small}$ and $\eps_{large}$ such that the profit of items classified as intermediate for any cell is at  most $\eps \profit(\opt)$. $\eps$ $\geq$ $\eps_{large}$ $\geq$ $f(\eps_{small})$ $\geq$ $\omega_{\eps}(1)$, for some positive increasing function $f(.)$ .\\
We add items not contained in $\kappa(t)$ in $\opt_{large}(C)$ to $K(t+1)$ for all $C$ not fully covered by any item in $\kappa(t)$. We do corridor decomposition as in section \ref{sec:bldecom}, considering only skew items in all the cells.\\%put the reference
 Although this corridor decomposition might kill some of the items in $\kappa(t)$ which we want to save. Thus we apply Lemma \ref{focsagain}  and \ref{againfocs} which uses further decomposition of corridors with constant number of line segments dropping a $ \eps$ fraction from optimal.
%Old-------------------------\\
%		In this section we try to recursively divide the knapsack into a non-uniform grid, stretch it to make it a uniform grid. We then sacrifice a 
%		small fraction of intercepted items and perform corridor partition to the remaining set of items. The corridor partition follows similar to 						section \ref{subcorr}. Consider the set of items $\kappa(t)$ at $t^{th}$ iteration as the items forming the grid. The grid at any such level of iteration is formed by extending the edges of all the items in $\kappa(t)$. We initiate $\kappa(0)$ with the items in $\opt_{large}$ $\cup$ $\opt_{corr}^{cross}$ $\cup$  $\opt_{kill}$ as defined in section \ref{profitstruc}. We recursively augment items packed at each iteration to $\kappa(t)$.  We also define a set $K(t+1)$ which contains all the items killed at $t^{th}$ iteration during the process. \\
%Consider the set $C_{t}$ of all grid cells at $t^{th}$ iteration. Same as in lemma \ref{class} we classify the items in cells as $\opt_{small}(C)$, $\opt_{large}(C)$, $\opt_{hor}(C)$, $\opt_{ver}(C)$, $\opt_{intermediate}(C)$. The lemma lets us drop $\eps$ fraction profit $\opt_{intermediate}(C)$ items in every cell. We then kill all the $\opt_{large}(C)$ in every cell $C$ $\in$ $C_{t}$. The killed rectangles are added to $K(t+1)$. We then stretch the grid to a uniform grid throughout the knapsack. Using processes in section \ref{subcorr} we obtain the corridor decomposition of the knapsack with the set of all skew items with $O_{\eps,\eps_{large},\kappa(t)}(1)$ corridors. The decomposition is equivalent to the decomposition of the original knapsack and we get the same set of killed items in both the cases. Since only a $O_{\eps}(1)$ items $\opt_{cross}$ are killed in the corridor decomposition. We add items in $\opt_{cross}$ and items not in $\kappa(t)$ to the set $K(t+1)$. Next we state the following lemma.
%\\
%old end-----------\\
\begin{lem}\cite{GalvezGHI0W17}\label{focsagain}
	Let $S$ be an open corridor with $b(S)$ bends. Let $\R' \subseteq \opt$ be a collection of items which intersect the boundary of $S$ with $\R' \cap \opt_{skew}(C_{t}) = \phi$. Then there is a collection of $|\R'| \cdot b(S)$ line segments $L$ within $S$ which partition $S$ into sub-corridor with at most $b(S)$ bends each such that no item from $\R'$ is intersected by $L$ and there are at most $O_{\eps}(|\R'| \cdot b(S))$ items of $\opt_{skew}(C_{t})$ intersected by line segments in $L$.
\end{lem}
\begin{lem}\cite{GalvezGHI0W17}\label{againfocs}
Let $S$ be a closed corridor with $b(S)$ bends. Let $\opt_{skew}(S)$ denote the items in $\opt_{skew}(C_{t})$ that are contained in $S$. Let $\R'$ $\subseteq$ $\opt$ be a collection of items which intersect the boundary of $S$ with  $\R' \cap \opt_{skew}(C_{t}) = \phi$. Then there is a collection of $O_{\eps}(\frac{|\R'|^{2}}{\eps})$ line segments $L$ within $S$ which partition $S$ into a collection of closed corridors with at most $\frac{1}{\eps}$ bends each and possibly an open corridor with $b(S)$ bends such that no item from $\R'$ is intersected by $L$ and there is a set of items $\opt'_{skew}(S) \subseteq \opt_{skew}(S)$ with $|\opt'_{skew}(S)|\leq O_{\eps}(|\R'|^{2})$ such that the items in $\opt_{skew}(S) \setminus \opt'_{skew}(S)$ intersected by the line segments in $L$ have a total profit of at most $O(\eps) \cdot \profit(\opt_{skew}(C_{t}))$.
\end{lem}
Using Lemmas \ref{focsagain} and \ref{againfocs} we partition the piece in $O_{\eps}(1)$ corridors (open and closed) packing all the items in $\opt_{skew}(S)$ $\backslash$ $\opt'_{skew}(S)$. We augment the remaining set of items $\opt'_{skew}(S)$ with small profit to $K(t+1)$.
\begin{remark}
Guillotine Separability : All the processes used to obtain the bends and corridor decomposition follow deletion of items only. Thus the remaining subset of items should be guillotine separable given that the initial packing was guillotine separable.
\end{remark}
		\subsubsection{Box Partition}\label{boxpart}
			We follow the same process as in original corridor decomposition section \ref{prosec} on all the items completely lying inside the strips formed from the subcorridor processing in the previous section. The difference from previous section \ref{prosec} is the set $\opt_{fat}$ being considered for packing i.e. we don't drop large items while forming the set $\opt_{ fat}$ in this section section. Then by using similar shifting procedure as in section \ref{prosec} we shift items from one subcorridor to other to pack all but $\opt_{kill}$ of them. For now let us ignore the items in $\opt_{small}$ that cross a subcorridor (handled in section \ref{smallitems}). We add all the items in $\opt_{kill}$ into $K(t+1)$ which actually refers to the items killed in the $t^{th}$ iteration. From section \ref{prosec} it follows that only $O_{\eps,\eps_{large},\eps_{box}}(1)$ of items are killed in partition of subcorridors to boxes. Also the killed items  do not belong to the set $\kappa(t)$.
%We divide the subcorridor into strips and then classify the items as $fat$ lying completely inside these strips. We call the set of items in this optimal packing as $\opt_{fat}$. Then by simple shifting argument, we pack the items in the strips killing $\opt_{kill}$ items in the process. We add all the items in $\opt_{kill}$ into $K(t+1)$ which actually refers to the items killed in the $t^{th}$ iteration. From section \ref{prosec} it follows that only $O_{\eps,\eps_{large},\eps_{box}}(1)$ of items are killed in partition of subcorridors to boxes. Also the items killed do not belong to the set $\kappa(t)$.
			\begin{remark} 
			Guillotine Separability: The division of subcorridors into boxes involves partition of subcorridor with $1/\eps_{box}$ lines. We remove all the items killed by these lines and pack the rest completely into the strips formed. The strips can be themselves separated by the same set of lines. Also since we begin from a guillotine separable arrangement, shifting the horizontal (resp. vertical) items vertically (resp. horizontally) doesn't disturb the guillotine property. Thus guillotine separability is maintained after the processing of subcorridors into boxes. 
			\end{remark}
		\subsubsection{Container Partition}
		\label{containerweighted}
		We follow resource augmentation from Lemma \ref{lemma1}. The process borrows technique from partitioning box into containers as done in section \ref{prosec} with the only difference that we also include $\opt_{small}$ this time while processing. We classify an item as $\opt_{small}(C_{t}))$ if for every cell $C$ in $C_{t}$ intersecting with the item,  the item is classified as $\opt_{small}(C)$. In other words any item which is small in all the cells intersecting it, is classified as $\opt_{small}(C_{t})$. Now consider a horizontal box, using averaging argument there exits a strip with width $3\eps$ such that it intersects with items with total profit less than or equal to $O(\eps)\profit(\opt_{box})$. We neglect the small items intercepted by the strip for now and pack them later as mentioned in section \ref{smallitems}. Let the items killed be $\opt_{kill,box}$. We add items in $\opt_{kill,box}$ to the set of items dropped in the $t^{th}$ iteration, i.e., $K(t+1)$. We then apply resource augmentation to the set of remaining small items say $\opt'_{small}(C_{t})$ and pack subset $\opt''_{small}(C_{t})$.
This gives us an $L\&C$ packing of a profitable subset $\opt'_{skew}(C_{t})$ $\subseteq$ $\opt_{skew}(C_{t})$ and a subset of small items not intersected by the $3\eps$ strip, i.e., $\opt''_{small}(C_{t})$ $\subseteq$ $\opt'_{small}(C_{t})$. Total profit of items, i.e., $\profit(\opt'_{skew}(C_{t}))$ $+$ $\profit(\opt''_{small}(C_{t}))$ $+$ $\profit(K(t+1))$ $\geq$ ($1-O(\eps)$) $($ $\profit(\opt_{skew}(C_{t}))$ $+$ $\profit(\opt'_{small}(C_{t}))$ $)$.
%The subsets are such that only $O(\eps)$ factor of profit is lost. 
			\begin{remark}
			Guillotine Separability: The only process we do in this section is deleting some items intersecting a strip. Since deleting items doesn't affect guillotine separability the remaining items are guillotine separable given the original arrangement is guillotine separable. Thus we get a guillotine separable arrangement after doing the processing as given in this section.
			\end{remark}
		\subsubsection{Packing Small Items}\label{smallitems}

 %We denote the cells which are not dead as free cells. Now take the knapsack and and find the regions which are guillotine separable and doesn't overlap with any container or boundary-$\Lc$. Let us denote these regions as guillotine free region. By appropriate choosing $\eps,\epsl,\epss,\eps_{box},\epsau$ as shown in subsection \ref{cnt} we can ensure that the total area of guillotine free regions which don't have both the dimensions greater than or equal to $\eps' N$ is $O_{\eps,\epsl,\eps_{box},\epsau}(1)\cdot \frac{\epss}{\eps}\cdot N^{2}$ which is at most $O(\eps^{2})N^{2}$. Now total area of guillotine free region is greater than or equal to the total area of free cells. So the total area of gullotine free regions with both dimensions greater than or equal to  $\eps' N$ is at least (max$\{ (\eps N^{2},a(\opt_{small})\}-O(\eps^{2}N^{2}$)). We have sufficient area to pack small rectangles of the packings in Lemma \ref{algo1} and Lemma \ref{algo2}. 
%\amar{Arnab, verify if this goes with new small packing proof}
Now we repack the small items killed by lines of corridor decomposition in section \ref{boxpart}. Consider the set $\opt_{small,killed}(C_{t})$ as the given set of items. We assign each item in $\opt_{small,killed}(C_{t})$ to the cell it was contained maximally in the original packing. Consider a cell $C$ and the items assigned to $C$ as $\opt_{small,killed}(C)$. By appropriately choosing the factor $\eps_{small}$, we can force area of small items assigned to $C$, i.e.,  $a(\opt_{small,killed}(C))$ to be at most $\eps a(C)$. This follows from the fact that number of boxes intersecting $C$ would be $O_{\eps,\eps_{large}}(1)$. Next we claim that the free area in cell $C$, i.e. total area not-occupied by containers in the cell is at most $(1-2\eps)a(C)$ (Lemma \ref{areafocs}). Thus following the same argument as in Lemma \ref{dead}, the total area of guillotine free region is greater than or equal to the total area of free cells, and thus we have sufficient area to pack small rectangles using NFDH. Thus we can pack a profitable fraction of items  $\opt'_{small,killed}(C)$ $\subseteq$  $\opt_{small,killed}(C)$ such that $\profit(\opt_{small,killed}(C)) \geq (1-O(\eps)) \profit(\opt_{small,killed}(C))$.
			\begin{lem}\cite{GalvezGHI0W17}\label{areafocs}
				Let $C$ be a cell. The total area of $C$ occupied 	by containers is at most $(1-2\eps)a(C)$.
			\end{lem}
			\begin{remark}
				Guillotine Separability: The processing in the section involves deleting a subset of rectangles which doesn't affect the guillotine separability of items. We use NFDH to pack the items in the cells. Since NFDH is 2-stage guillotine separable packing, inside each cell items are guillotine separable. If we consider each cell as a pseudoitem, we claim that the whole knapsack is guillotine separable. The claim follows from the fact that cells are formed from extending the edges in $\kappa(t)$. The guillotine cuts will always follow the corresponding edges of the items. Thus the arrangement in whole after the processing is guillotine separable. 
			\end{remark}
		\subsubsection{L$\&$C Packing}\label{lc}
			Following the same iterative process we get $k$ subsets; $K(1), K(2), \cdots, K(k-1), K(k)$ such that $k\leq\frac{1}{\eps}$ and $\profit(K(k))$ $\leq$ $\eps \opt$. Now consider the grid $G_{k}$ corresponding to the set $\kappa(k)$ with the set of cells $C_{k}$. We do the corridor, subcorridor, box processing subroutines as defined in previous sections. We now apply routines of Lemma \ref{algo1} and prove the same result for weighted version of the problem. We keep the notations same as used in the unweighted version, thus we have the sets $\opt_{ST}$, $\opt_{SF}$, $\opt_{LF}$, $\opt_{LT}$. We augment items in $\kappa(k-1)$ to the set $\opt_{LF}$. We also define set $\opt_{small}$ to be $\opt_{small}(C(k))$ which is the set of items classified as small in each non-zero intersection cell of $C_k$.\\
Since we have followed the modified corridor decomposition from previous sections for packing $\opt_{small}$ which $O(\eps)$ loss in the profit, we can extend lemma \ref{algo1} to the weighted case.\\

Now to improve bounds further let us show another $L\&C$ packing. 
First we show the following lemma for the unweighted case. Then we will extend it to the weighted case. 

\begin{lem}
\label{algo2}
$\profit(\opt_{L\&C})\geq\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{SF})$.
\end{lem}
\begin{proof}
From the optimal packing we remove all the items except the items in $\opt_{SF}$. Now in this new packing consider a horizontal (resp., vertical) random strip of height (resp., width) $3\eps N$. Remove the items which overlap with these vertical and horizontal strips. Let the items which remain be $\opt_{SF}'$. Due to horizontal strip, a horizontal item gets removed with probability at most $7\eps$ and a vertical item gets removed with probability at most $\frac{1}{2}+6\eps$. Similarly, due to vertical strip, a vertical item gets removed with probability at most $7\eps$ and a horizontal item gets removed with probability at most $\frac{1}{2}+6\eps$. From linearity of expectation we get that $\profit(\opt_{SF}')\geq (\frac{1}{2}-13\eps)\profit(\opt_{SF})$. \\
\\Also clearly $\opt_{SF}'$ can be packed in a square of side length $(1-3\eps)N$. So by doing one sided resource augmentation we can get a packing with profit $(1-O(\eps))\profit(\opt_{SF}')$ in a square with side length $(1-2\eps)N$. In $N \times N$ knapsack we can pack all items in $\opt_{LT}$ in a boundary-$\Lc$ with width $\epsr N$. Two containers of dimensions $\epsr N \times \frac{N}{2}$ and $\frac{N}{2} \times \epsr N$ are created and kept just beside the subcorridors of boundary-$\Lc$ in such a way that the 2 created subcorridors don't overlap with each other. We pack all the items in $\opt_{ST}$ in these two containers. In the remaining square region which doesn't have items from $\opt_{T}$ we can pack the items from $\opt_{SF'}$ with profit $(1-O(\eps))\profit(\opt_{SF}')$ as the square region has side length at least $(1-2\eps)N$. This concludes the proof of this Lemma. 
\end{proof}
% extension of algo2 to weighted case
For extending the weighted argument to lemma \ref{algo2} (non-degenerate-$\Lc$ case), intuitively we follow the same striping argument to remove items and make space for items to be packed by resource augmentation. Thus we remove all the items from $\kappa(k-1)$, because any item in $\kappa(k-1)$ can be large in both dimensions and has a high probability of being cut by a strip. We further add small items as in previous sections without losing more than a constant profit. We then remove a $3\eps N$ strip as done in section \ref{containerweighted}. Any item in $\opt_{small}$ is cut by the strip with a probability $3\eps$ and any other item is cut with probability $\frac{1}{2} + O(\eps)$. We construct the $\Lc$ as done in unweighted case. Thus we get the following result:
\begin{lem}
\label{weightall}
Let $\opt_{L\&C}$ be the most profitable guillotine packing solution that is packed by an $L\&C$ packing and $\opt$ be the optimal  solution of $\tggk$. Then following lemmas hold:
	\begin{enumerate}
		\item $\profit(\opt_{L\&C})\geq\profit(\opt_{F})+\profit(\opt_{T})/2$ + $\profit(\opt_{small})$,
		\item $\profit(\opt_{L\&C})\geq\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{SF})$ + $\profit(\optsm)$.
		%\item $\profit(\opt_{L\&C})\geq\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{LF})$ + $\profit(\optsm)$		
		%\arir{3 is not established and removed T+F/2}
	\end{enumerate}
\end{lem}
\begin{proof}
All the inequalities follows from the processing done above. We also claim that the solution follows guillotine property as we use results and lemmas from previous sections which are already established to maintain guillotine separability. Another processing done is deleting of items intersecting with the strip, since deleting items doesn't disturb guillotine cuts we have a guillotine separable packing as a result.
\end{proof}
\begin{lem}
Let $\opt_{L\&C}$ be the most profitable solution that is packed by an $L\&C$ packing which is guillotine separable and $\opt$ be optimal guillotine packing. Then $\profit(\opt_{L\&C})\geq(\frac{2}{3}-O(\eps))\profit(\opt)$.
\end{lem}
\begin{proof}
The result follows from Lemma \ref{weightall}, we thus get a factor of $3/2$, i.e., $\profit(\opt_{L\&C})$ $\geq$ $ (2/3 - O(\eps))\profit(\opt)$ for weighted case.
\end{proof}

\subsection{ $(\frac{4}{3}+\eps)$-approximation \tggkr}
\label{subs:tggkr}
%%\arir{Use $N \times N$ knapsack instead of $1\times 1$ -- Done}

% Massive items defintion
%Large items which we drop out initially in the cardinality case analysis, cannot be removed in the weighed case as they might carry all the profit of the knapsack. Thus intuitively we define such a large item as {\em massive} item. Formally a
An item is called {\em massive} if $\width_{i} \geq (1-\eps)N$ and $\height_{i} \geq (1-\eps)N$, given the dimensions of original knapsack as $N \times N$. Chose $\eps > \epsr$ and $\eps < \frac{1}{10}$. Idea is to devise two packings; one when such a massive item is present and other when it is absent; and analyze the worst bound from both of them to get a bound for the weighted rotated case.

	\begin{lem}
		Given $\opt$ is the set of guillotine separable items that can be optimally packed in a $N \times N$ knapsack with associated profit $\profit(\opt)$, if rotations are allowed. Then there exits a guillotine separable packing of items $APX \subseteq \opt$ in $O_{\eps}(1)$ containers such that the profit of items $\profit(APX)\geq (\frac{3}{4}-O(\eps))\profit(\opt)$.
	\end{lem}
%\arnr{Mention in the lemma that the final packing which you are getting is also guillotine separable}
	\begin{proof}
		We prove the result by a case analysis. We subdivide the problem in two cases as discussed above on the basis of presence or absence of a massive item.	The result follows from Lemma \ref{lem:present} (packing when massive item is present) and Lemma \ref{lem:absent} (case when there exits no massive item). The worst case packing from among two gives us a factor of $4/3$, i.e., $\profit(APX)$ $\geq$ $ (3/4 - O(\eps))\profit(\opt)$ for weighted case given rotations are allowed.
	\end{proof}

%%%%%%%5 massive item present
	\begin{lem} \label{lem:present}
		Given $\opt$ be the set of items in the optimal guillotine separable packing into a $N\times N$ knapsack and there is a massive item $m \in \opt$. Then, there exists a set $\apx$ $\subseteq$ $\opt$ with $\profit(\apx) \geq (\frac{3}{4} - O(\eps)) \profit(\opt) $ which can be packed with rotations allowed in a container packing with $O_{\eps}(1)$ containers.
	\end{lem}%	\amar{tight case : (T,F,m) = (  .4, .4, .2)}
	\begin{proof}
	Consider the optimal packing of items in $\opt$. Irrespective of the initial arrangement inductively we can show that it is possible to place $m$ on the top-right corner of the knapsack with the remaining items forming a  boundary-$\Lc$ in the remaining region $\big(([0,N]\times[0,\height_{L}]) \cup ([0,\width_{L}] \times[0,N])\big)$, where $\height_{L} = N-\height(m)$ and $\width_{L} = N-\width(m)$. The proof follows constructively by considering the sequence of guillotine cuts on the knapsack and following similar {\em mirroring} arguments as done in section \ref{glp}. 
%\amar{do we need a rigorous proof show existence of an L}. \\
	We propose three different packings and consider the maximum profit packing from the three of them. Process the $\Lc$-corridor as done Section \ref{prosec} and then use shifting argumentation \ref{subsec:shifting} to get a corridor decomposition. We define items to be thin ($T$), and fat ($F$) (excluding $m$) as defined previously. Items completely lying in the horizontal arm of $L$ defined by the region  $([0,N]\times[0,\height_{L}])$ are defined as $\opt_{H}$. Similarly items completely lying the in vertical arm of $L$ defined by the region $([0,\width_{L}] \times[0,N])$ are defined as $\opt_{V}$. Thus we get $\opt_{HF}$, $\opt_{HT}$, $\opt_{VF}$, $\opt_{VT} $ as the fat-horizontal, thin-horizontal, fat-vertical, thin-vertical items respectively. W.l.o.g.~we can assume that $\width_{L} \geq \height_{L}$. \\
	
\noindent {\em Packing 1:}
We remove the lesser profit set among $\opt_{VT}$ and $\opt_{HT}$, and process the $\Lc$-corridor to obtain a container packing of the remaining items of $\opt_{T}$ and all items from $\opt_{F}$ as done in Section \ref{prosec}. Since $\opt_{VT} \cup \opt_{HT} = \opt_{T}$, from averaging principle we get the profit of thin items packed as at least $\profit(\opt_{T})/2$. This gives us a packing of a set of items $P_{1}$ with $\profit(P_{1})$ $\geq$ $(1-O(\eps))(\profit(m) + \profit(\opt_{T})/2 + \profit(\opt_{F}))$.\\
%\arnr{First line in Packing is not clear. How is total width atmost $\epsl w_{L}$}
%\arnr{Please write packing 2 properly. Plus the Packing 1 and 2 are giving the same profit according to the equations which you wrote}
%\amar{Bug (Packing 2): Rewrtten}

\noindent {\em Packing 2:}
From corridor decomposition it follows that the total width (resp. height) of thin items in vertical (resp. horizontal) subcorridor of the $\Lc$-corridor is at most $\epsr \width_{L}$ (resp. $\epsr \height_{L} $) which on the other hand is upper bounded by $\eps \width_{L}$ (resp. $\eps \height_{L} $) .We now rotate the items in $\opt_{HT}$ and pack the items in $\opt_{VT} \cup \opt_{HT}$ in region $([0,\eps(\height_{L}+\width_{L})]\times[0,N])$. 
%Items in $\opt_{HF}$ are rotated and then packed besides $\opt_{VF}$ so as to obtain a packing of $\opt_{F} = \opt_{VF} \cup \opt_{HF}$ in the plane of height $N$ and width at least $(1-\eps)(\width_{L} + \height_{L})$. We remove a random vertical strip of width $\height_{L}$ from this plane which can cut at most all the items from $\opt_{F}$. . 
We then remove all the items in $\opt_{F}$. Thus the remaining set of items $\R'$ have a width $\width(\R') \leq$ $\eps (\height_{L} + \width_{L})$ and a profit $\profit(\R') =$ $\profit(\opt_{T})$. Using resource augmentation (Lemma \ref{lemma1}) we obtain a packing of these items  $\R'' \subseteq \R'$ in a region $([0,\width_{L}]\times[0,N])$%, i.e. by using an additional vertical strip of width $\width_{L}-\eps (\height_{L} + \width_{L})$ and height $N$,
 such that $\profit(\R'') \geq (1-O(\eps)) \profit(\R')$. Thus we get a packing of $\R'' \cup \{ m\}$ such that $\profit(P_{2}) \geq (1-O(\eps)) \profit(\R') + \profit(m) = (1-O(\eps))(\profit(\opt_{T})) + \profit(m)$.\\
%From averaging principle any item of $\opt_{F}$ is saved by the random strip with probability atleast $\frac{(1-\eps)(\width_{L}) - \eps \height_{L}}{(1-\eps)(\width_{L} + \height_{L})} = \frac{\width_{L}}{\width_{L} + \height_{L}} - \frac{\eps}{1-\eps}.\frac{\height_{L}}{\width_{L} + \height_{L}} \geq \frac{1}{2} - \frac{\eps}{2(1-\eps)} = \frac{1}{2} - O(\eps)$. Thus the remaining set of items $\R'$ after removal of vertical strip have a width $\width(\R') \leq$ $\width_{L} - \eps (\height_{L} + \width_{L})$ and a profit $\profit(\R') \geq$ $\profit(\opt_{T}) + \profit(\opt_{F})/2$. Using resource augmentation (Lemma \ref{lemma1}) we obtain a packing of these items  $\R'' \subseteq \R'$ in a region $([0,\width_{L}]\times[0,N])$, i.e. by using an additional vertical strip of width $\eps (\height_{L} + \width_{L})$ and height $N$, such that $\profit(\R'') \geq (1-O(\eps)) \profit(\R')$. Thus we get a packing of $\R'' \cup \{ m\}$ such that $\profit(P_{2}) \geq (1-O(\eps)) \profit(\R') + \profit(m) = (1-O(\eps))( \profit(\opt_{F})/2 + \profit(\opt_{T})) + \profit(m)$.\\

\noindent {\em Packing 3:}
We consider the packing without $m$. Next we rotate $\opt_{H}$, to obtain a packing of $\opt_{H} \cup \opt_{V}$ in region $R'=$ $([0,\height_{L}+\width_{L}]\times[0,N])$. Clearly $R'$ $\subseteq$ $([0,2\eps]\times[0,1])$. Using resource augmentation lemma \ref{lemma1} we can pack a set of items $P_{3} \subseteq (\opt_{H} \cup \opt_{V})$ such that $\profit(P_{3}) \geq (1-O(\eps))(\profit(\opt_{H}) + \profit(\opt_{V})) = (1-O(\eps))(\profit(\opt_{F}) + \profit(\opt_{T}))$.\\

Considering the maximum profit packing from $P_1, P_2, P_3$, we obtain a packing of set of items $\apx$ $\subseteq$ $\opt$ with $\profit(\apx) \geq (\frac{3}{4} - O(\eps)) \profit(\opt) $ in $O_{\eps}(1) $ containers. The worst case corresponds the packing where profits are $\profit(\opt_{T}):\profit(\opt_{F}):\profit(m)=2:1:1$.
	\end{proof}

%%%%%% no massive item
	\begin{lem}[Lemma \ref{weightall}]
		\label{lem:wr1}
		$\profit(APX)\geq\profit(\opt \backslash \opt_{T})+\profit(\opt_{T})/2$.
	\end{lem}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5

	

	
%	
%	\begin{lem}
%		\label{lem:wr2}
%		$\profit(\opt_{L\&C})\geq(1-O(\eps)) \profit(\opt_{T})+\frac{3\profit( \opt_{SF})}{4} + \frac{\profit(\opt_{LF})}{2}+\profit(\opt_{small})$.
%	%\label{strip_improvement_with_cardinality}
%	%$|\opt_{L\&C}|\geq |\opt_{T}|+3|\opt_{SF}|/4+\opt_{LF}|/2$.
%	\end{lem}
%\begin{proof}
%% Consider the optimal packing of $\R_{SF}$ in the $N \times N$ knapsack. Chose a random horizontal strip $H$ of width $3\eps N$ at a random offset $r$ from the left boundary of knapsack where $r \in [0, (1-3\eps)N]$. The region is defined by $ H = [0 , N ] \times [ r, r +  \eps N ]$. Delete all items intersecting strip $H$. Since each item in $\opt_{SF} \cap \Rve$ is of height at most $\height_{ver} \leq .5 $, it is removed with probability at most $.5 + 6\eps$.  Each item of $\opt_{SF} \cap \Rho$ is of height at most $\height_{ver} \leq \epss N \leq \eps N $, it is removed with probability at most $7\eps$. Thus the items remaining after removal of strip $H$ have profit atleast $(.5 - 6\eps)(\profit(\opt_{SF})\cap\profit(\opt{ver})) + ( 1- 7\eps) (\profit(\opt_{SF})\cap\profit(\opt{hor}))$ .\\
%%	\\Similarly considering a vertical strip $V$ = $[ r, r + 3 \eps N  ] \times  [0 , N ]$ . Following arguments similar to horizontal case. Each item in $\opt_{SF} \cap \Rho$ is removed with probability at most $.5 + 6\eps$.  Each item of $\opt_{SF} \cap \Rve$ is removed with probability at most $7\eps$. Thus the items remaining after removal of strip $V$ have profit at-least $(.5 - 6\eps)(\profit(\opt_{SF})\cap\profit(\opt{hor}) )+ ( 1- 7\eps) (\profit(\opt_{SF})\cap\profit(\opt{ver}))$ .\\
%%	\\We obtain a packing of atleast  $(\frac{3}{4} - \frac{13}{2}\eps)(\profit(\opt_{SF}))$ items  by considering the best of above two cases in a region $[0 , N- 2\eps N] \times [0,N] $ after doing resource augmentation(assuming that the vertical strip removes less items in expectation).\\
%%	The total width ( resp., height)  of items in $\opt_{T} \cap \R_{hor}$ (resp., $\opt_{T} \cap \R_{ver}$) is at most $\epsr N $.
%%	It is also given that $\epsr \leq \eps$.  We then rotate every item in $\opt_{T} \cap \R_{hor}$ to make it vertical . The set of item $\opt_{T}$ is now of total width at most  $2\epsr N $. Now we place every item in $\opt_{T}$ beside each other in the rectangular region  $  [ N- 2\eps N ,N] \times [0,N] $ obtained from removing the vertical strip from $\opt_{SF}$ packing as shown in Figure \ref{T+3/4SF-}. It is worth mentioning that the proof indeed applies to a general weighted case also as every equation is in terms of profit of items. For our cardinality proof however we consider profit of each item to be 1 which concludes the proof.
%\arnr{where is the packing of $LF/2$}
%We first consider packing of items in $\opt_{SF}$ and add small items as in section \ref{smallitems} without losing more than a constant profit in the $N \times N$ knapsack. Chose a random horizontal strip $H$ of width $3\eps N$ at a random offset $r$ from the left boundary of knapsack where $r \in [0, (1-3\eps)N]$. The region is defined by $ H = [0 , N ] \times [ r, r +  \eps N ]$. Delete all items intersecting strip $H$. Since each item in $\opt_{SF} \cap \Rve$ is of height at most $\height_{ver} \leq .5 $, it is removed with probability at most $.5 + 6\eps$. Each item of $\opt_{SF} \cap \Rho$ is of height at most $\height_{ver} \leq \epss N \leq \eps N $, it is removed with probability at most $7\eps$. Any item in $\opt_{small}$ is cut by the strip with a probability $7\eps$. Thus the items remaining after removal of strip $H$ have profit atleast $(.5 - 6\eps)(\profit(\opt_{SF})\cap\profit(\opt{ver})) + ( 1- 7\eps) (\profit(\opt_{SF})\cap\profit(\opt{hor}))$ .\\
%	\\Similarly considering a vertical strip $V$ = $[ r, r + 3 \eps N  ] \times  [0 , N ]$ . Following arguments similar to horizontal case. Each item in $\opt_{SF} \cap \Rho$ is removed with probability at most $.5 + 6\eps$.  Any item in $\opt_{small}$ is cut by the strip with a probability $7\eps$. Each item of $\opt_{SF} \cap \Rve$ is removed with probability at most $7\eps$. Thus the items remaining after removal of strip $V$ have profit at-least $(.5 - 6\eps)(\profit(\opt_{SF})\cap\profit(\opt{hor}) )+ ( 1- 7\eps) (\profit(\opt_{SF})\cap\profit(\opt{ver}))$ .\\
%	\\We obtain a packing of atleast  $(\frac{3}{4} - \frac{13}{2}\eps)(\profit(\opt_{SF}) + (1-O(\eps))\profit(\opt_{small}))$ items  by considering the best of above two cases in a region $[0 , N- 2\eps N] \times [0,N] $ after doing resource augmentation(assuming that the vertical strip removes less items in expectation).\\
%	The total width ( resp., height)  of items in $\opt_{T} \cap \R_{hor}$ (resp., $\opt_{T} \cap \R_{ver}$) is at most $\epsr N $.
%	It is also given that $\epsr \leq \eps$.  We then rotate every item in $\opt_{T} \cap \R_{hor}$ to make it vertical . The set of item $\opt_{T}$ is now of total width at most  $2\epsr N $. Now we place every item in $\opt_{T}$ beside each other in the rectangular region  $  [ N- 2\eps N ,N] \times [0,N] $ obtained from removing the vertical strip from $\opt_{SF} \cup \opt_{small}$ packing as shown in Figure \ref{T+3/4SF-}. %It is worth mentioning that the proof indeed applies to a general weighted case also as every equation is in terms of profit of items. For our cardinality proof however we consider profit of each item to be 1 which concludes the proof.
%\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%6
%	\begin{lem}
%		\label{lem:wr2}
%		$\profit(\opt_{L\&C})\geq \profit(\opt_{T})+\frac{3 \opt_{SF}}{4} + \frac{\opt_{LF}}{2}+\profit(\opt_{small})$.
%	\end{lem}
%	\begin{proof}
%		We extend the weighted argument to Lemma \ref{strip_improvement_with_cardinality}. We first consider packing of items in $\opt_{SF}$ and add small items as in section \ref{smallitems} without losing more than a constant profit. 
%%We then remove a $3\eps N$ strip as done in Lemma \ref{strip_improvement_with_cardinality} which can be either horizontal or vertical. 
%We follow the same striping argument to remove the least profitable $3\eps N$ strip ( either horizontal or vertical ) and make space for items in $T$ to be packed in a $\eps N$ strip and then pack the items by resource augmentation. Any item in $\opt_{small}$ is cut by the strip with a probability $3\eps$.
%%Thus we remove all the items from $\kappa(k-1)$, because any item in $\kappa(k-1)$ can be large in both dimensions and has a high probability of being cut by a strip. 
%% Taking the best of horizontal and vertical strips we can ensure that any item in $\opt_{SF}$ is cut with probability $\frac{3}{4} + O(\eps)$ as done in Lemma \ref{strip_improvement_with_cardinality}.
%This gives us a packing with profit atleast  $\profit(\opt_{L\&C})\geq \profit(\opt_{T})+3(\opt_{SF}/4) + \profit(\optsm)$.
%	\end{proof}

	\begin{lem} \label{lem:absent}
		Given $\opt$ be the set of items in the optimal guillotine separable packing into a $N \times N$ knapsack and there exists no massive item in $ \opt$. Then, there exists a set $\apx$ $\subseteq$ $\opt$ with $\profit(\apx) \geq (\frac{3}{4} - O(\eps)) \profit(\opt)$ which can be packed with rotations allowed in a container packing with $O_{\eps}(1)$ containers.
	\end{lem}

	\begin{proof}
		We consider $2$ different packings and consider the most profitable of them for final packing. We first perform the basic corridor decomposition and classify items as $LT$, $ST$ and $LF$, $SF$. We define three different packings as follows:\\
		
\noindent{\em Packing 1:} Consider items in $\opt \backslash \opt_{T}$. Using resource contraction (Lemma \ref{lem:rsrccontraction}), we can pack items with profit at least $\profit(\opt \backslash \opt_{T})/2$ in a $(N\times(1-\eps/2)N)$ piece. We then pack $\opt_{T}$ in the remaining $(N \times \eps N/4)$ region and then apply resource augmentation Lemma \ref{lemma1} to get the packing without losing more then $O_{\eps}(1)$ profit of total items in a $N \times N$ piece. Thus we get a packing of a set of items $P_1$ with profit $\profit(P_1)\geq \profit(\opt \backslash \opt_{T})/2 + \profit(\opt_{T})$.\\

%\noindent{\em Packing 2:} Using Lemma \ref{lem:wr2} we get a packing of set of items $P2$ such that $\profit(P2)\geq \profit(\opt_{T})+3(\opt_{SF}/4) + (\opt_{LF}/2) +\profit(\opt_{small})$.

\noindent{\em Packing 2:} Using Lemma \ref{lem:wr1} we get a packing of set of items $P_2$ such that $\profit(P_2)\geq\profit(\opt \backslash \opt_{T})+\profit(\opt_{T})/2$.
\\
Considering the maximum profit packing from $P_1, P_2$, we obtain a packing of set of items $\apx$ $\subseteq$ $\opt$ with $\profit(\apx) \geq (\frac{3}{4} - O(\eps)) \profit(\opt) $ in $O_{\eps}(1) $ containers.  The worst case corresponds the packing where profits are $\profit(\opt_{T})=\profit(\opt \backslash \opt_{T})$.
	\end{proof}

	\begin{lem}\cite{GalvezGHI0W17} % lemma 51 \cite{GalvezGHI0W17}
		\label{lem:rsrccontraction}
		 (Resource Contraction Lemma) If a set of guillotine separable items $M$ contains no massive item and can be packed into a $1\times1$ bin, then it is possible to pack a set $M'$ of profit at least $\profit(M)/2$ into a $N \times (1 - \eps/2)N$ bin (or a $(1- \eps /2)N\times N $ bin), maintaining guillotine property, given rotations are allowed.
	\end{lem}
	\begin{proof}
		We proceed along the same proof as in Lemma 51 of \cite{GalvezGHI0W17} and prove that the processing done maintains guillotine property of items.\\
Intuitively we consider two disjoint subsets of $M$, say $M'$ and $M \backslash M'$, and pack them individually in a $N \times (1- \eps/2)N$ bin. The best of two packings will give us a packing of profit at least half the profit of $M$. We define set of items completely to the right, left, top, bottom of a given item $i$ as $Right(i)$, $Left(i)$, $Top(i)$, $Bottom(i)$ respectively. Formally, given item $i$ with bottom left coordinates as $(x_{i}, y_{i})$, we define $Right(i) = \{ i' \in M | x_{i'} \geq (x_{i}+\width(i))\}$, $Left(i) = \{ i' \in M | x_{i'} \leq x_{i}\}$,  $Top(i) = \{ i' \in M | y_{i'} \geq (y_{i}+\height(i))\}$, $Bottom(i) = \{ i' \in M | y_{i'} \leq y_{i}\}$. We consider $4$ boundary strips $S_{T,\frac{3}{2}\eps} := [0,N] \times [(1-\frac{3}{2}\eps)N, N]$, $S_{B,\frac{1}{2}\eps} := [0,N] \times [0,\frac{1}{2}\eps N]$, $S_{L,\frac{1}{2}\eps} := [0,\frac{1}{2}\eps N] \times [0,N]$, $S_{R,\frac{1}{2}\eps} := [1-\frac{1}{2}\eps N, N] \times [0,N]$. The set of items fully contained in and intersected by the strip $S_{X,Y}$ are denoted by $C_{X,Y}$ and $E_{X,Y}$ respectively. Also define $D_{X,Y} = E_{X,Y} \backslash C_{X,Y}$. We now consider following cases :
\\

\noindent{\em Case 1:} $D_{B,\frac{1}{2}\eps} \cap D_{T,\frac{3}{2}\eps} = \phi$. \\
Define $M'=E_{T,\frac{3}{2}\eps}$, which can be packed in a $[0,N] \times [0,(1-\frac{1}{2}\eps)N]$ region. This gives us our first packing which is guillotine separable as the operation performed here is just deletion of items in an already guillotine separable arrangement. For second packing we consider the items in $M\backslash (M' \cup C_{L,\frac{1}{2}\eps} \cup C_{R,\frac{1}{2}\eps} $. Pack $C_{L,\frac{1}{2}\eps}$ and $C_{R,\frac{1}{2}\eps}$ by rotating and packing them on the top of $M\backslash (M' \cup C_{L,\frac{1}{2}\eps} \cup C_{R,\frac{1}{2}\eps} $ in two horizontal strips of  width $\frac{1}{2}\eps N$ each. This adds up to a packing of $M\backslash M'$ in the region $[0,N] \times [0, (1- \frac{1}{2}\eps)N]$. The processing involves mirroring and rearrangement of {\em disjoint} sub-pieces which doesn't disturb the guillotine property.\\ 
\noindent{\em Case 2:} $D_{B,\frac{1}{2}\eps} \cap D_{T,\frac{1}{2}\eps} \neq \phi$.\\
\noindent{\em Case 2.1:}  There exists item $i$ intersecting none of $S_{L, \frac{1}{2}\eps}$ and $S_{R, \frac{1}{2}\eps}$. \\
W.l.o.g.~ assume $x_{i} \leq 1/2 N$. We consider completely disjoint partitions of items created by $i$, i.e., $Left(i)$, $Right(i)$, $\{i\}$, $C_{T, \frac{3}{2}\eps}$ and $C_{B, \frac{1}{2}\eps}$. Let $M'$ = $C_{T, \frac{3}{2}\eps}$  $\cup$ $C_{B, \frac{1}{2}\eps}$ $\cup Left(i)$. Consider optimal packing with just $Left(i)$, we pack  the items in $C_{T, \frac{3}{2}\eps}$ and $C_{B, \frac{1}{2}\eps}$ to the right of it by rotating them. This gives us a packing of $M'$ in a $(N \times (1-\frac{1}{2}\eps)N)$ plane. Now we show a packing for $M\backslash M' = Right(i) \cup {i}$. From the assumption that $i$ doesn't intersect $S_{L,\frac{1}{2}\eps}$, we trivially get a packing of $M \backslash M'$ in a $(N\times (1-\frac{1}{2}\eps)N)$ piece. Since only operations to obtain both the packings are deletion of items from optimal guillotine packing and replacement of disjoint subpieces, we can claim that guillotine property is maintained.\\
\noindent{\em Case 2.2:}  There exists item $i$ intersecting both $S_{L, \frac{1}{2}\eps}$ and $S_{R, \frac{1}{2}\eps}$.\\
We define $M' = (C_{R, \frac{1}{2}\eps} \cup C_{L, \frac{1}{2}\eps} \cup Top(i))$. 
For packing $M'$, consider $Top(i)$ in optimal packing and rotate and pack $C_{L, \frac{1}{2}\eps}$ and $C_{R, \frac{1}{2}\eps}$ on the top of it.Total height of the packing is $(N-y_{i}-\height(i)+\eps N) \leq (1-\eps)N$ since $\eps \leq .1$. For packing in the second case, i.e., for packing $M\backslash M'$, since there is no massive item it follows trivially that it can packed in a $(N \times (1-\frac{1}{2}\eps)N)$ piece. Thus we get both the packing and following the same argument as before the packings are guillotine separable.\\
\noindent{\em Case 2.3:}  There exists item $i$ intersecting both $S_{B, \frac{1}{2}\eps}$ and $S_{T,\frac{3}{2}\eps}$.\\
\noindent {\em Case 2.3.1:} There exists item $i$ $\in (D_{B, \frac{1}{2}\eps} \cap D_{T,\frac{3}{2}\eps} \cap D_{L,\frac{1}{2}\eps})$ and $x_{i}+\width(i) \leq \frac{1}{2}N $ (similar argument holds for $D_{R,\frac{1}{2}\eps}$) ] Since there is no massive item, $i$ can intersect at most one of $S_{L, \frac{1}{2}\eps} and S_{R, \frac{1}{2}\eps}$. We define $M'= Right(i)$. By rotating $M'$ we get a packing in $(N\times (1-\frac{1}{2}\eps)N)$  piece. Now we devise a packing for second set $M\backslash M'$. Consider packing of $M \backslash (C_{T, \frac{3}{2}\eps}$  $\cup$ $C_{B, \frac{1}{2}\eps}$ $\cup Right(i)$ as in optimal packing and pack $C_{T, \frac{3}{2}\eps}$ and $C_{B, \frac{1}{2}\eps}$ to the right of it by rotating them and packing in two vertical strips of $\frac{3}{2}\eps$ and $\frac{1}{2}\eps N$ widths respectively. This gives us the total width of the packing as less than or equal to $(1/2 + 2\eps)N \leq (1-\frac{1}{2}\eps)N$ since $\eps \leq .1$ from our initial assumption. Again the only operations during entire processing of both the packings are deletion of items from optimal guillotine packing and replacement of disjoint sub-pieces.\\
\noindent{\em Case 2.3.2:}  There exists item $i$ $\in (D_{B, \frac{1}{2}\eps} \cap D_{T,\frac{3}{2}\eps} \cap D_{L,\frac{1}{2}\eps})$ and $x_{i}+\width(i) > \frac{1}{2}N $ (similar argument holds for $D_{R,\frac{1}{2}\eps}$). \\
Define $M'= Left(i) \cup {i}$. Consider the packing of $M'$ in optimal packing, which clearly gives us a packing in a $(N\times (1-\frac{1}{2}\eps)N)$. Now we define second packing for items in $M\backslash M'$. Consider the packing of  $M \backslash (C_{T, \frac{3}{2}\eps}$  $\cup$ $C_{B, \frac{1}{2}\eps}$ $\cup M'$ as in optimal packing and pack $C_{T, \frac{3}{2}\eps}$ and $C_{B, \frac{1}{2}\eps}$ to the left of it by rotating them and packing in two vertical strips of $\frac{3}{2}\eps N$ and $\frac{1}{2}\eps N$ widths respectively. This gives us the total width of the packing as less than or equal to $(1/2 + 2\eps)N \leq (1-\frac{1}{2}\eps)N$ since $\eps \leq \frac{1}{10}$. Sole operations involved are deletion of items from already guillotine separable packing and replacement of disjoint pieces. thus maintaining guillotine separability.\\
\noindent{\em Case 2.3.3:} There exists no item $i$ $\in (D_{B, \frac{1}{2}\eps} \cap D_{T,\frac{3}{2}\eps} \cap (D_{L,\frac{1}{2}\eps} \cup D_{R,\frac{1}{2}\eps}))$.\\
W.l.o.g.~let $i \in C_{L,\frac{1}{2}\eps}$. We define $M'=E_{T,\frac{3}{2}\eps} \backslash (C_{L,\frac{1}{2}\eps} \cup C_{R,\frac{1}{2}\eps})$, which clearly gives us a packing in a $(N\times (1-\frac{1}{2}\eps)N)$. Consider $M \backslash (M' \cup  C_{L, \frac{1}{2}\eps} \cup C_{R, \frac{1}{2}\eps}$ in optimal packing and rotate and pack $C_{L, \frac{1}{2}\eps}$ and $C_{R, \frac{1}{2}\eps}$ on the top of it. Total height of the packing is at most $ (1-\eps)$. Operations involved in are deletion of items from already guillotine separable packing and replacement of disjoint pieces. thus maintaining guillotine separability.
\end{proof}

%
%We the use the corridor partitioning as in section \ref{prosec}. Consider the set of small items $\opt_{small}$ as the set of small items in $C(k)$ i.e. $\opt_{small}(C(k))$. We class items in the same fashion as in section \ref{profitstruc}.
 %Hence we prove that Lemmas \ref{sumprofit}, \ref{algo1}, \ref{idea} are also applicable in the weighted case. We extend Lemma \ref{algo2} to weighted case by considering items in $OPT_{small}$ while processing. Since every small item is cut by the vertical ( or horizontal ) strip with probability $O(\eps)$, we can follow the same processing as in \ref{algo2}. Combining results in Lemmas \ref{algo2}, \ref{sumprofit}, \ref{algo1}, \ref{idea}, we get the same factor of
% $10/7$ i.e.
% $\profit(OPT_{L\&C})$
% $\geq$ $ (10/7+O(\eps))\profit(OPT)$ for wieghted case.
%\section{Weighted Non-Rotated case}\label{w2dgk}
%	\subsection{Shifting Argumentation\cite{GalvezGHI0W17}}\label{shifting}
%	We use similar process as used as in \cite{GalvezGHI0W17} and prove that if we begin with a guillotine separable solution, the process results in a final guillotine separable arrangement.
%		\subsubsection{Grid and Corridor Partition}\label{gridpartition}
%		In this section we try to recursively divide the knapsack into a non-uniform grid, stretch it to make it a uniform grid. We then sacrifice a 
%		small fraction of intercepted items and perform corridor partition to the remaining set of items. The corridor partition follows similar to 						section \ref{prosec}. Consider the set of items $\kappa(t)$ at $t^{th}$ iteration as the items forming the grid. The grid at any such level of iteration is formed by extending the edges of all the items in $\kappa(t)$. We initiate $\kappa(0)$ with the items in $OPT_{large}$ $\cup$ $OPT_{corr}^{cross}$ $\cup$  $OPT_{kill}$ as defined in section \ref{profitstruc}. We recursively augment items packed at each iteration to $\kappa(t)$.  We also define a set $K(t+1)$ which contains all the items killed at $t^{th}$ iteration during the process. \\
%Consider the set $C_{t}$ of all grid cells at $t^{th}$ iteration. Same as in lemma \ref{class} we classify the items in cells as $OPT_{small}(C)$, $OPT_{large}(C)$, $OPT_{hor}(C)$, $OPT_{ver}(C)$, $OPT_{intermediate}(C)$. The lemma lets us drop $\eps$ fraction profit $OPT_{intermediate}(C)$ items in every cell. We then kill all the $OPT_{large}(C)$ in every cell $C$ $\in$ $C_{t}$. The killed rectangles are added to $K(t+1)$. We then stretch the grid to a uniform grid throughout the knapsack. Using processes in section \ref{prosec} we obtain the corridor decomposition of the knapsack with the set of all skew items with $O_{\eps,\eps_{large},\kappa(t)}(1)$ corridors. The decomposition is equivalent to the decomposition of the original knapsack and we get the same set of killed items in both the cases. Since only a $O_{\eps}(1)$ items $OPT_{cross}$ are killed in the corridor decomposition. We add items in $OPT_{cross}$ and items not in $\kappa(t)$ to the set $K(t+1)$. Next we state the following lemma.
%\begin{lem}\cite{GalvezGHI0W17}\label{focsagain}
%	Let $S$ be an open corridor with $b(S)$ bends. Let $I'$ $\subseteq$ $OPT$be a collection of items which intersect the boundary of $S$ with $I'\bigcap OPT_{skew}(C_{t}) = \phi$. Then there is a collection of $|I'|.b(S)$ line segments $L$ within $S$ which partition $S$ into subcorridor with at most $b(S)$ bends each such that no item from $I'$ is intersected by $L$ and there are at most $O_{\eps}(|I'|.b(S))$ items of $OPT_{skew}(C_{t})$ intersected by line segments in $L$.
%\end{lem}
%\begin{lem}\cite{GalvezGHI0W17}\label{againfocs}
%Let $S$ be a closed corridor with $b(S)$ bends. Let $OPT_{skew}(S)$ denote the items in $OPT_{skew}(C_{t})$ that are contained in $S$. Let $I'$ $\subseteq$ $OPT$ be a collection of items which intersect the boundary of $S$ with  $I'\bigcap OPT_{skew}(C_{t}) = \phi$. Then there is a collection of $O_{eps}(\frac{|I'|^{2}}{\eps})$ line segments $L$ within $S$ which partition $S$ into a collection of closed corridors with at most $\frac{1}{\eps}$ bends each and possibly an open corridor with $b(S)$ bends such that no item from $I'$ is intersected by $L$ and there is a set of items $OPT'_{skew}(S) \subset OPT_{skew}(S)$ with $|OPT'_{skew}(S)|\leq O_{\eps}(|I'|^{2})$ such that the items in $OPT_{skew}(S) \backslash OPT'_{skew}(S)$ intersected by the line segments in $L$ have a total profit of at most $O(\eps).\profit(OPT_{skew}(C_{t}))$.
%\end{lem}
%Using Lemmas \ref{focsagain} and \ref{againfocs} we partition the piece in $O_{\eps}(1)$ corridors (open and closed) packing all the items in $OPT_{skew}(S)$ $\backslash$ $OPT'_{skew}(S)$. We augment the remaining set of items $OPT'_{skew}(S)$ with small profit to $K(t+1)$.
%\begin{remark}
%Guillotine Separability : All the processes used to obtain the bends and corridor decomposition follow deleting of items only. Thus the remaining subset of items should be guillotine separable given that the initial packing was guillotine separable.
%\end{remark}
%		\subsubsection{Box Partition}\label{boxpart}
%			We follow the same process as in original corridor decomposition section \ref{prosec}. We divide the subcorridor into strips and then classify the items as $fat$ lying completely inside these strips. We call the set of items in this optimal packing as $OPT_{fat}$. Then by simple shifting argument, we pack the items in the strips killing $OPT_{kill}$ items in the process. We add all the items in $OPT_{kill}$ into $K(t+1)$ which actually refers to the items killed in the $t^{th}$ iteration. From section \ref{prosec} it follows that only $O_{\eps,\eps_{large},\eps_{box}}(1)$ of items are killed in partition of subcorridors to boxes. Also the items killed do not belong to the set $\kappa(t)$.
%			\begin{remark} 
%			Guillotine Separability : Since items the division of subcorridors into boxes involves partition of subcorridor with lines. We remove all the items killed by these lines and pack the rest completely into the strips formed. The strips can be themselves separated by the same set of lines. Also since we begin from a guillotine separable arrangement, shifting the horizontal ( resp. vertical) items vertically ( resp. horizontally ) doesn't disturb the guillotine property. Thus guillotine separability is maintained after the processing of subcorridors into boxes. 
%			\end{remark}
%		\subsubsection{Container Partition}
%		We follow resource augmentation from Lemma \ref{lemma1}. The process borrows technique from process of partitioning box into containers from section \ref{prosec}. We classify an item as $OPT_{small}(C_{t}))$ if for every cell $C$ in $C_{t}$ intersecting with the item,  the item is classified as $OPT_{small}(C)$. In other words any item which is small in all the cells intersecting it, is classified as $OPT_{small}(C_{t})$. Now consider a horizontal box, using averaging argument there exits a strip with width $3\eps$ such that it intersects with items with total profit less than or equal to $O(\eps)\profit(OPT_{box})$. We neglect the small items intercepted by the strip for now and pack them pack in section \ref{smallitems}. Let the items killed be $OPT_{kill,box}$, We add items in $OPT_{kill,box}$ to the set of items killed in the $t^{th}$ iteration, i.e., $K(t+1)$. We then apply resource augmentation to the set of remaining small items say $OPT_{small}(C_{t})$ and pack subset $OPT'_{small}(C_{t})$. We then pack profitable subsets $OPT'_{skew}(C_{t})$ $\subset$ $OPT_{skew}(C_{t})$ and $OPT'_{small}(C_{t})$ $\subset$ $OPT_{small}(C_{t})$ of items using $L\&C$ packing as in section \ref{lc}. The subsets are such that only $O(\eps)$ factor of profit is lost. 
%			\begin{remark}
%			Guillotine Separability : The only process we do in this section is deleting some items intersecting a strip. Since deleting items doesn't affect guillotine separability as the remaining items need to guillotine separable if the original arrangement is guillotine separable. Thus we get a guillotine separable arrangement after doing the processing as given in this section.
%			\end{remark}
%		\subsubsection{Packing Small Items}\label{smallitems}
%			Now we repack the small items killed in lines by corridor decomposition in section \ref{boxpart}. Consider the set $OPT_{skew,killed}(C_{T})$ as the given set of items. We assign each item in $OPT_{skew,killed}(C_{T})$ to the cell it was contained maximally in the original packing. Consider a cell $C$ and the items assigned to $C$ as $OPT_{skew,killed}(C)$. By wisely choosing the factor $\eps_{small}$ we can force area of small items assigned to $C$, i.e.,  $a(OPT_{skew,killed}(C))$ to be at most $\eps a(C)$. This follows from the fact that number of items intersecting $C$ would be $O_{\eps,\eps_{large}}(1)$. Thus by using %\ref{smallpacking} and 
%\ref{areafocs}
% we can pack a profitable fraction items  $OPT'_{skew,killed}(C)$ $\subset$  $OPT_{skew,killed}(C)$ such that $\profit(OPT_{skew,killed}(C)) \geq (1-O(\eps)) \profit(OPT_{skew,killed}(C))$.
%			\begin{lem}\cite{GalvezGHI0W17}\label{areafocs}
%				Let $C$ be a cell. The total area of $C$ occupied 	by containers is at most $(1-2\eps)a(C)$.
%			\end{lem}
%			\begin{remark}
%				Guillotine Separability : The processing in the section involves deleting a subset of rectangles which doesn't affect the guillotine separability of items. We use NFDH to pack the items in the cells. Since NFDH is 2-stage guillotine separable packing, inside each cell items are guillotine separable. If we consider each cell as a pseudoitem, we claim that the whole knapsack is guillotine separable. The claim follows from the fact that cells are formed from extending the edges in $\kappa(T)$. The guillotine cuts will always follow the corresponding edges of items. Thus the arrangement in whole after the processing is guillotine separable. 
%			\end{remark}
%		\subsubsection{L$\&$C Packing}\label{lc}
%			Following the same iterative process we get $k$ subsets; $K(1), K(2),... K(k-1), K(k)$ such that $k\leq\frac{1}{\eps}$ and $\profit(K(k))$ $\leq$ $\eps OPT$. We consider the cutting of piece, say $C(k)$, by extending the edges of items in $K(k-1)$. 
%We the use the corridor partitioning as in section \ref{subcorr}. Consider the set of small items $OPT_{small}$ as the set of small items in $C(k)$ i.e. $OPT_{small}(C(k))$. We class items in the same fashion as in section \ref{profitstruc}.
% Hence we prove that Lemmas \ref{sumprofit}, \ref{algo1}, \ref{idea} are also applicable in the weighted case. We extend Lemma \ref{algo2} to weighted case by considering items in $OPT_{small}$ while processing. Since every small item is cut by the vertical ( or horizontal ) strip with probability $O(\eps)$, we can follow the same processing as in \ref{algo2}. Combining results in Lemmas \ref{algo2}, \ref{sumprofit}, \ref{algo1}, \ref{idea}, we get the same factor of
% $10/7$ i.e.
% $\profit(OPT_{L\&C})$
% $\geq$ $ (10/7+O(\eps))\profit(OPT)$ for wieghted case.
%\begin{remark}
%Guillotine Separability : In the given section we use results and lemmas from previous sections which are already established to maintain guillotine separability. Another processing done is deleting of items intersecting with the strip, since deleting items doesn't disturb guillotine cuts we have a guillotine separable packing as a result.
%\end{remark}

==> 9_Comparison_To_General_Case.tex <==
	\section{Gap between Guillotine and Non-Guillotine Knapsack}
	

==> 9_QPTAS1.tex <==
\section{QPTAS for \tggkc}
\label{sec:qptas}
\subsection{Unweighted case}
\label{subsec:uqptas}
From Lemma \ref{structure} we get that there are corridors of at most 1 bend and if we move items in a corridor in such a way that locally within a corridor the items are guillotine separable then the packing in the entire knapsack is guillotine separable.
We will use couple of lemmas from \cite{adamaszek2015knapsack}.

\begin{lem}\label{qptas1}\cite{adamaszek2015knapsack}
For an optimal solution $\opt$ to \tggkc, there is a partition of the $N \times N$ knapsack into at most $(\frac{1}{\epsl})^{O(1)}(\frac{\log n}{\eps})^{O(\frac{1}{\eps})}$ rectangular boxes $\mathcal{B}$ with integral coordinates, a set of items $\R' \subseteq \opt \cap (V \cup H)$ with $|\R'| \geq (1-O(\eps))|\opt\cap(V\cup H)|-(\frac{1}{\epsl})^{O(1)}(\frac{\log n}{\eps})^{O(\frac{1}{\eps})}$, and an assignment $f:\R'\rightarrow \mathcal{B}$ such that for each box $B \in \mathcal{B}$ all items in $f^{-1}(B)$ fit into $B$. Moreover, each box $B \in \mathcal{B}$ has height or width at most $\epsl N$. Note a rectangle belongs to the set $V$ (resp. $H$) if it has height (resp. width) more than $\epsl N$.
\end{lem}

\begin{lem}\cite{adamaszek2015knapsack}\label{copylem}
If there is an algorithm for \tggkc~which outputs a solution with at least $(1-\eps)|\opt|-\log n)^{O_{\eps}(1)}$ items in time $O(f(n))$, then there is also a $(1+\eps)$-approximation algorithm with running time $O((f(n)+\log n)^{O_{\eps}(1)})$.
\end{lem} 

Lemma \ref{qptas1} can be extended to the guillotine case as the procedure used to create the boxes is similar to the process described in subsection \ref{prosec} and it is guillotine separable. Since the number of bends in any corridor is at most one, we have $(\frac{1}{\epsl})^{O(1)}O_{\eps}(\log n)$ rectangular boxes instead of $(\frac{1}{\epsl})^{O(1)}(\frac{\log n}{\eps})^{O(\frac{1}{\eps})}$. If we do resource augmentation on every box we have $(\frac{1}{\epsl})^{O(1)}O_{\eps,\epsau}(\log n)$  containers which can be guessed in $n^{(\frac{1}{\epsl})^{O(1)}O_{\eps,\epsau}(\log n)} $  time. So by Lemma \ref{copylem} and due to the maximum number of bends being one in any corridor, we have QPTAS with  running time $n^{(\frac{1}{\epsl})^{O(1)}O_{\eps,\epsau}(\log n)} $, improving the previous best QPTAS. Small rectangles can be added in the similar fashion as that of subsection \ref{smallrec} \amar{bug}. This gives us the following theorem:
\begin{thm}
Given $N$ is $O(n^{O(\log n)})$, we have a QPTAS for $\tggkc$ with running time $n^{(\frac{1}{\epsl})^{O(1)}O_{\eps,\epsau}(\log n)} $, whether rotations are allowed or not.
\end{thm}


\subsection{Weighted case}
\label{subsec:wqptas}
%\arir{add a comment why Abed et al. approach did not give weighted QPTAS. Also add two proper theorems summarizing the final result.}
\ama{Work by Abed et al \cite{AbedCCKPSW15} proves a QPTAS for $\tggkc$, although it cannot be extended to weighted case. Their procedure used to create boxes considers droppig $O(1)$ number of items, which cannot be extended to weighted case as the items dropped might carry a huge profit. Overcoming this, corridor decomposition from \ref{prosec} can repack those $O(1)$ items using the simple shifting argumentation without losing more than a subset of items with constant profit.} We use the same shifting argumentation techniques as mentioned in Section \ref{subsec:shifting} on the optimal packing. Suppose we are in the $k$th iteration of the shifting argument process. First we create grid cells and do corridor decomposition as mentioned in the Section \ref{gridpartition}. Then by Lemma \ref{structure} we get corridors with atmost 1 bend and any movement of rectangles within the corridor which ensures guillotine separability inside the corridor ensures guillotine separability in the entire knapsack. Then we create $O_{\eps,\epsl}(\log n)$ boxes according to  Lemma \ref{qptas1} and then we do resource augmentation to each box in the $k$th iteration where $k<1/\eps$ and in this process we get a set of items $K(k)$ which have profit atmost $\eps\cdot\profit(\opt)$ and we remove them. Then we pack the small items which were not packed earlier in the process in the same way as we do in Section \ref{smallitems}. The packing is guillotine separable as the  shifting argumentation techniques are guillotine separable. Now we have $O_{\eps,\epsl,\epsau}(\log n)$ containers which can be guessed in $n^{O_{\eps,\epsl,\epsau}(\log n)}$ time. Hence we have a QPTAS as stated:
\begin{thm}
Given $N$ is $O(n^{O(\log n)})$, we have a QPTAS for $\tggk$ with running time $n^{O_{\eps,\epsl,\epsau}(\log n)}$, whether rotations are allowed or not.
\end{thm}

==> Backup/4A_Structural_Property.tex <==
\subsection{Obtaining corridors with at most 2 bends}
\label{sub:bldec}

	
		\begin{figure}
			\captionsetup[subfigure]{justification=centering}
			\hspace{-15pt}
			
				\centering
				\resizebox{!}{6cm}{
					\begin{tikzpicture}					
						\draw[thick] (0,6)--(2,6)--(2,5.5)--(4,5.5)--(4,6)--(6,6)--(6,4)--(5,4)--(5,3)--(4.5,3)--(4.5,4.5)--(5.5,4.5)--(5.5,5.5)--(4.5,5.5)--(4.5,5)--(1.5,5)--(1.5,5.5)--(.5,5.5)--(.5,4)--(2,4)--(2,3)--(4,3)--(4,2.5)--(1.5,2.5)--(1.5,3.5)--(0,3.5)--(0,6);		
						
						\draw[dotted] (6,4)--(5.5,4.5);
						\draw[dotted] (5,4)--(4.5,4.5);
						\draw[dotted] (6,6)--(5.5,5.5);
						\draw[dotted] (4,6)--(4.5,5.5);
						\draw[dotted] (2,6)--(1.5,5.5);
						\draw[dotted] (0,6)--(.5,5.5);
						\draw[dotted] (0,3.5)--(.5,4);
						\draw[dotted] (1.5,2.5)--(2,3);
						\draw[dotted] (1.5, 3.5)--(2,4);
						\draw[dotted] (1.5, 5)--(2,5.5);
						\draw[dotted] (4.5 , 5)--(4,5.5);

						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};

						\draw[->] (1,5.75) edge[out=90,in=0,->] (.75,6.5);	\draw (.5,6.5) node {\textbf{$l$}};

						\draw (1.75,5.25) node {\textbf{$l_{1}$}};

						\draw (4.25, 5.25) node {\textbf{$l_{2}$}};

						\draw[->] (5,5.75) edge[out=180,in=0,->] (4.75,6.5);	\draw (4.5,6.5) node {\textbf{$l$}};
%
%						\draw[->] (5.75,5) edge[out=180,in=0,->] (6.5,5);	\draw (6.5,5) node {\textbf{$l_{V}$}};
%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};

						\draw[dashed] (4.75,3) -- ( 4.75 ,4.25) -- ( 5.75, 4.25) -- ( 5.75, 5.75) -- ( 4.25, 5.75) -- ( 4.25, 5.25) -- ( 1.75, 5.25) -- ( 1.75, 5.75) -- (.25, 5.75) -- (.25, 3.5) ;	
						%\draw (4,1.25) node {\large \textbf{$U'$}};
						%\draw (5,4.75) node {\large \textbf{$C$}};
						%\draw (4,3) node {\large \textbf{$B$}};
					\end{tikzpicture}}
				\caption{k-bend Corridor Processing}
				\label{fig:kbend}
		\end{figure}


	\begin{lem} \label{structure}
	Given an optimal guillotine packing of $\R$ rectangles and the rectangles are either horizontal or vertical, we can partition the knapsack into $O_{\eps}(1)$  L corridors and $O_{\eps}(1)$ corridors with 0 bends and place $\R' \subseteq \R$ rectangles in these corridors and corridors with 0 bends such that:
	\begin{enumerate}
	\item$\profit(\R') \geq (1-O(\eps))\profit(\R)$ provided we can drop $O_{\eps}(1)$ rectangles without loosing any profit
	\item Each corridor with 0 bends or subcorridor contains only one type of rectangle(i.e, either horizontal or vertical)
	\item Each rectangle is guillotine separable
	\item Each L corridor is a boundary $\Lc$ for a rectangular box.
         \item Rectangular boxes (which bound the items in $\Lc$ corridors ) when considered as a pseudo rectangle are guillotine separable and number of such boxes is $O_{\eps,\epsl}(1)$
         \item Each corridor with 0 bends when considered as a pseudo rectangles are guillotine separable and number of such corridors is $O_{\eps,\epsl}(1)$.
     	\end{enumerate}
	\end{lem}
\begin{proof}
	Given an optimal guillotine packing $\R$ (these rectangles are skewed) and using lemma \ref{lem:corridorPack} and Theorem \ref{3max} we  partition the knapsack into $O_{\eps}(1)$ corridors with no Z bends and the number of bends is atmost 3. Also the packing $\R'$ is guillotine separable and $\profit(\R') \geq (1-O(\eps))\profit(\R)$. We now a provide a construction of finding the rectangular box for each type of corridor with atleast one bend such that the corridor is at the boundary of the box and the box is guillotine separable. For the remainder of the section we assume that a given corridor $S$  can't be divided into smaller corridors with cuts perpendicular to the orientation of any subcorridor. If there were such corridors then we can divide our corridor into smaller corridor and $O(\frac{1}{\epsl})$ corridors with 0 bends which are obtained by these perpendicular cuts \end{proof}. In the following subsections we show a construction of boxes
\begin{obs} \label{endtoend}
Given a piece containing a set of guillotine separable rectangles, there must exist an end-to-end guillotine cut in the piece. In other words, the first level of guillotine cuts in the piece is end-to-end.
\end{obs}
We follow some terminologies in the remainder of the section. We define subpiece $P$ completely containing corridor $C$ as \textit{smallest} iff the piece $P$ which is obtained from the sequence of guillotine cuts has no previous cut that passed through the corridor $C$ and the next end to end cut in $P$ passes through $C$. We also define \textit{box $B$ bounding} a set of rectangles as a subpiece which is guillotine separable from the rest of the piece. In other ways $B$ if considered as a pseudo-rectangle, forms a guillotine separable arrangement with the rest of the items of knapsack. In the rest of the section, by freezing a rectangle, we mean that the rectangle is not moved while shifting other rectangles. A subcorridor $S_{1}$ is said to be exhausted if there is no rectangle from $S_{1}$ in the smaller subpiece on which we would running our recursive procedure in the following section. A box $B$ is said to be bounding a corridor with atleast one bend if the outermost corners at the bends of the corridor coincides with the corners of the box. Now in the following section we provide a construction of boxes and corridors with 0 bends which satisfy Lemma \ref{structure}.
	\subsubsection{$\Lc$ corridor}\label{L corridor}
	%Consider a L corridor $S$ with vertical subcorridor placed top left with respect to the horizontal subcorridor.W.l.o.g let us assume that the corridor $S$ can't be divided into smaller corridors with cuts perpendicular to subcorridor. Let us denote the line along the rightmost edge of horizontal subcorridor by $\Lc$. Consider the 2 left most vertical guillotine cuts in the vertical subcorridor of $S$ during the actual guillotine cutting sequence. If leftmost cut is intercepted by a rectangle $R_{1}$ which is above $S$ and the other cut is not intercepted by any rectangle which isn't completely above $R_{1}$ then there should exist a guillotine either top or bottom of the rectangle $R_{1}$ which crosses the line $\Lc$. Suppose there is no such cut and w.l.o.g let us assume that rectangle $R_{2}$ above $R_{1}$ which intercepts the second leftmost cut has a guillotine cut above it which crosses $\Lc$. But this situation is not possible as the set of rectangles in L corridor, rectangles which intercept the guillotine cuts of $R_{1}$ and $R_{2}$ form a non-guillotine structure as there is no end to end cuts be it horizontal or vertical  which spans the entire length of the subcorridor of $S$. So W.l.o.g let us assume that the two left most guillotine are intercepted by a single rectangle or by a rectangle which next to each other and above $S$. Consider the rectangle with upper most interception among the two. Let it be $R_{3}$. Now there must exist a guillotine cut between $R_{3}$ and the top most edge $e_{1}$ of vertical subcorridor of $S$ which crosses the line $\Lc$ and the leftmost guillotine cut. Suppose not then all the rectangles intercepting the guillotine cuts between $R_{3}$ and $e_{1}$, $R_{3}$ and the set of rectangles in the L corridor form a non-guillotine structure  as there is no end to end cuts be it horizontal or vertical which spans the entire length of the subcorridor of $S$. Now consider the lower most such guillotine cut which crosses line $\Lc$.Let this be $l_{1}$. Then by similar analogy we must have a guillotine cut to the right of horizontal subcorridor of $S$ which crosses $l_{1}$ and is parallel to $\Lc$. Hence we have constructed a box which is guillotine separable and has $S$ as it's boundary L.\\

Consider a $\Lc$ corridor $S$. W.l.o.g we can assume that vertical subcorridor $S_{1}$ of $S$ is placed to the top left w.r.t the horizontal subcorridor $S_{2}$. We consider the smallest subpiece $P$ containing $S$.
% Three cases might exist. Case 1: If left boundary of vertical subcorridor of S coincides with the left boundary of P, we have found the left boundary of bounding box. We then consider the sequence  If bottom boundary of horizontal subcorridor of S coincides with the bottom boundary of P, we have found the bottom boundary of bounding box. %
Next consider the first stage guillotine cuts in the $P$. W.l.o.g let the first stage cuts be vertical.
Then we have the following cuts which can occur to a $\Lc$ corridor during the recursive procedure to bound the $\Lc$ corridor which we are going to describe later:
\begin{itemize}
\item Cut 1:Rightmost vertical Guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$
\item Cut 2:Horizontal Guillotine cut passing through $S_{1}$ and not through the interior of $S_{12}$
\item Cut 3: Horizontal Guillotine cut passing through $S_{2}$
\item Cut 4:  Cut which doesn't pass through $\Lc$ corridor.
\end{itemize}
Now we describe the recursive procedure.According to our assumption we begin with Cut 1. If we have Cut 1 then make a corridor with 0 bends out of the rectangles separated from $\Lc$ corridor in our subpiece and consider the right subpiece to be the new subpiece. Merge all the corridors with 0 bends obtained due to Cut 1 provided that these cuts occured before the first cut 2.For the rest of cuts which are of type cut 1 make a corridor for rectangles separated by these cuts. If we have Cut 2 then make a corridor with 0 bends out of the rectangles separated from $\Lc$ corridor in our subpiece and consider the bottom subpiece to be the new subpiece.
We stop the recursive procedure if either $S_{1}$ has exhausted or we obtain cut 2. If we obtain a cut 2 then we clearly have a bounding box with the edges being cut 1,cut 2 and the top and the right edges of the smaller subpiece $P'$ we are in after the last step of the recursive procedure. In the whole procedure we obtain only $O(\frac{1}{\epsl})$ extra corridors with 0 bends. 
	\subsubsection{$\Uc$-corrdor}\label{twobends}
	%Consider a corridor $S$ with 2 bends such that 2 vertical subcorridors $S_{1},S_{3}$ placed on the top of the horizontal subcorridor $S_{2}$.W.l.o.g let us assume that the corridor $S$ can't be divided into smaller corridors with cuts perpendicular to subcorridor.Consider the 2 left most vertical guillotine cuts in the leftmost vertical subcorridor $S_{1}$ of $S$ during the actual guillotine cutting sequence. W.l.o.g let us assume that the two left most are intercepted by a single rectangle or by a rectangle which next to each other and above $S$. Consider the rectangle with upper most interception among the two. Let it be $R_{3}$. We denote the line along the rightmost edge of rightmost vertical subcorridor $S_{3}$ by $\Lc$. Now there must exist a guillotine cut between $R_{3}$ and the top most edge $e_{1}$ of vertical subcorridor of $S$ which crosses the line $\Lc$ and the leftmost guillotine cut. Suppose not then all the rectangles intercepting the guillotine cuts between $R_{3}$ and $e_{1}$, $R_{3}$ and the set of rectangles in the corridor $S$ form a non-guillotine structure as there is no end to end cuts be it horizontal or vertical  which spans the entire length of the subcorridor of $S$. Now consider the lower most such guillotine cut which crosses line $\Lc$.Let this be $l_{1}$. There is no rectangle between $l_{1}$ and topmost edge of the rightmost vertical subcorridor such that it intercepts line $\Lc$ otherwise the set of rectangle below line $l_{1}$ form a non-guillotine structure. Hence we have a box which is guillotine separable such that the corridor is along the boundary of the box. Now consider the corridor with 2 bends. By appropriate shifting of vertical rectangles we can convert it into a L corridor without disturbing the guillotine property. Exact details are available in subsubsection \ref{sss2}.\\
Let $S$ be a corridor with $2$ bends. Let the top left vertical, horizontal and top right vertical subcorridors of $S$ be $S_{1}$, $S_{2}$ and $S_{3}$ respectively as shown in Figure \ref{figtwobends}. Consider the smallest subpiece $P$ containing $S$. We define three types of end-to-end cuts possible in $P$ or in any of the subpieces formed by a sequence of cuts in $P$.The rightmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$ is termed as \textit{Type $1$}. The leftmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{3}$ is termed as \textit{Type $3$}. The topmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{2}$ is termed as \textit{Type $2$}. Figure \ref{figtwobends} shows all the three types of cuts defined. We then follow a recursive approach to define bounding box using the cuts in guillotine cutting sequence. Clearly obtaining all three type of cuts, i.e., type $1,2,3$ will result in a bounding box where the box is bounded by these cuts and upper boundary of subpiece $P'$ containing a subset of items of $S$. Subpiece $P'$ is that subpiece which contains smaller corridor with 2 bends after we obtain the last of the three type cut.  \\
\\Basic idea follows dividing $S$ into  $O(\frac{1}{\epsl})$ corridors $\{L_{1},L_{2},...,L_{k}\}$ (with atmost 1 bend) consisting of some items from $S_{1}$ ( w.l.og it can be $S_{3}$ but we assume for the remainder of the section that $S_{1}$ is the one contributing to $\Lc'$) and $S_{2}$,  $O(\frac{1}{\epsl})$ corridors with 0 bends $\{C_{1},C_{2},...,C_{l}\}$ from a subset of items of $S_{3}$ and a corridor (with at most 2 bends) with the remaining set of items. Note that $C_{i+1}$ is left of $C_{i}$ and $C_{i+1}$ has height less than $C_{i}$. Similarly $L_{i+1}$ is place to the top right of $L_{i}$ and $L_{i+1}$ is smaller in size than $L_{i}$   \\
\\We now formally define the algorithm for processing corridor $S$ with $2$ bends. From observation \ref{endtoend} we know that the first cut in any guillotine separable piece is end-to-end. In the remainder of the subsection by closing a corridor or corridor with 0 bends we mean that no more items will be packed in that corridor or corridor with 0 bends. And, by opening a corridor  or corridor with 0 bends we mean that we are allowed to pack rectangles in this corridor or corridor with 0 bends only. Initially corridor $L_{1}$ is open  and corridor with 0 bends $C_{1}$ is open. Depending on the type of this cut we do the following processing :
\begin{enumerate}
\item Scenario $1$:Let's assume that corridor $L_{i}$ and corridor with 0 bends $C_{j}$ is open right now. If we have a horizontal cut through $S_{1}$ or $S_{3}$ but not through $S_{2}$ then we pack the items of $S_{1}$ above the cut in one corridor with 0 bends and pack the items of $S_{3}$ above the cut in another corridor with 0 bends. Then we continue our recursive procedure for the smaller portion of our original corridor present in the subpiece below this cut. If the horizontal cut passes through $S_{1}$ then we close $L_{i}$ and open $L_{i+1}$. Similarly if the horizontal cut passes through $S_{3}$ then we close $C_{j}$ and open $C_{j+1}$.    Such kind of cuts can have $O(\frac{1}{\epsl})$ number of occurences as the larger dimension of any rectangle is atleast $\epsl N$. So when the recursive procedure halts scenario 1 would be contributing atmost $O(\frac{1}{\epsl})$ new corridors with 0 bends. 
\item Scenario $2$ : (Type $1$ cut) Add the items of $S_{1}$ which is left of cut 1 to the vertical subcorridor of $L'$. Consider the new-subpiece to be the subpiece which is right of cut 1. Run algorithm recursively on the new-subpiece.
\item Scenario $3$ : (Type $2$ cut) Add the items of $S_{2}$ below the cut 2 to the horizontal subcorridor of $L'$. Consider the new-subpiece to be the top-subpiece. Run algorithm recursively on the new-subpiece.
\item  Scenario $4$ : (Type $3$ cut) Pack the items of $S_{3}$ which is right of cut 3 in a new vertical corridor with 0 bends $C$. Consider the new-subpiece to be the subpiece which is right of cut 3. Run algorithm recursively on the new-subpiece.

\end{enumerate}
%The algorithm when run on subpiece $P$, considers one of the above three cases depending on the type of end-to-end cut, augments some items from $S_{1}$ or $S_{2}$ to $L'$ and runs again on the new subpiece. We halt at the iteration when at least one of each type of cut is obtained. The boundaries of subpiece at this step along with the cut considered define the bouding box for remaing set of items of $S$. Thus we get a box surrounded by $L'$ on two edges (left and bottom) and a corridor on the third (right). The fourth (top) edge of box is trivially defined by top edge of $P$\\It is clear that number of new corridors is 2, i.e., one L-corridor and one corridor with 0 bends. Since we follow the original sequence of guillotine cuts without moving any items, guillotine separability is not disturbed.

We halt if one of the following three cases happens. First case occurs if at some iteration at least one cut from each type of cut is obtained. The boundaries of subpiece at this step along with the cut considered define the bounding box for remaing set of items of $S$. Thus we get a box surrounded by corridors $\{L_{1},L_{2},...,L_{k}\}$ and corridors with 0 bends $\{C_{1},C_{2},...,C_{l}\}$ . Figure \ref{figtwobends} shows final bounding box $B$ formed after the algorithm alongwith $L_{1}$ formed after considering sequence of type $1$ and type $2$ cuts in subcorridors $S_{1}$, $S_{2}$ and the corridor with 0 bends $C_{1}$ formed from type $3$ cuts in $S_{3}$. Second case occurs if one or more subcorridors in the piece exhausts i.e. all the items of these subcorridors are already packed in corridors $\{L_{1},L_{2},...,L_{k}\}$ or in corridors with 0 bends $\{C_{1},C_{2},...,C_{l}\}$. In this case we are left with atmost 2 corridors with atmost 1 bend who rectangles are not part of the corridors with 0 bends or corridors created during the recursive procedure. We can use the previous section results to bound this corridor with the a box (Except for a corridor with 0 bends which will be dealt in the later subsections). Third Case occurs when the next guillotine cut in the sequence is vertical and passes through subcorridor $S_{2}$ only. This leaves us with 2 corridors of atmost 1 bend. So, we can use the previous section results to bound the corridors with the boxes (Except for a corridor with 0 bends which will be dealt in the later subsections).\\
\\Now we observe that using the algorithm defined above we add only a $O(\frac{1}{\epsl})$ number of new corridors and corridors with 0 bends. The proof follows from the fact that if it is the case that all algorithm halts when atleast one of each type of cuts is obtained then in the end we have corridors  $\{L_{1},L_{2},...,L_{k}\}$ (with atmost 1 bend) and corridors with 0 bends $\{C_{1},C_{2},...,C_{l}\}$. This accounts to $O(\frac{1}{\epsl})$ new corridors with 0 bends and corridors as new corridor with 0 bends or corridor is created only when we have scenario 1 and as we have shown there the number of times this scenario occurs is $O(\frac{1}{\epsl})$. Else if it is the case that algorithm halts when one or more of subcorridors is exhausted, then also we have either corridors $\{L_{1},L_{2},...,L_{k}\}$ (with atmost 1 bend) or we have corridors with 0 bends $\{C_{1},C_{2},...,C_{l}\}$ and we have already shown that the number of such corridors with 0 bends are $O(\frac{1}{\epsl})$. We then run the algorithm on remaining corridors which has lesser number of bends than $S$, i.e., atmost 1 bend(if there is any such corridor). As it follows from section \ref{L corridor}, we get $O(\frac{1}{\epsl})$ corridors from processing in this case. For  the third type of halting due to vertical cuts which passes through $S_{2}$ only, we have already shown in the previous paragraph that we obtain only $O(\frac{1}{\epsl})$ new corridors with 0 bends and corridors.


\begin{figure}[t]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,3) -- (0,0) -- (6,0) -- (6,4) -- ( 5,4) -- (5,1) -- (1,1) -- (1,3) -- (0,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,1.25) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};

			\draw (1,3.7) node {\large \textbf{Type 1}};
			\draw (6.7,.6) node {\large \textbf{Type 2}};
			\draw (6,4.7) node {\large \textbf{Type 3}};
		

			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,3.5) -- ( .5,0) ;
			\draw[dotted] (.25,3) -- ( .25,0) ;
			
			\draw[dotted] (0,.5) -- ( 6.2,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0) ;
			\draw[dotted] (5.25,4) -- ( 5.25,0) ;
				
		
		\end{tikzpicture}}
		\caption{Types of cuts}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,4) -- (1,1) -- (7,1) -- (7,5) -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick]  (1.5,6) -- (1.5,1.5) -- (7,1.5);% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[pattern=north east lines, pattern color=black] (6.5,1.5)--(6.5,5)--(7,5)--(7,1.5)--(6.5,1.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,4) -- (1.5,4) -- (1.5,1.5) -- (7,1.5) -- (7,1) --(1,1) -- (1,4);		

			\draw (1.25,1.25) node {\large \textbf{$L_{1}$}};
			\draw (6.75,2.5) node {\large \textbf{$C_{1}$}};
			\draw (4,4) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Final Bounding Box of $S$}
	\end{subfigure}
	\caption{Processing 2-bend corridor}
	\label{figtwobends}
\end{figure}
	\subsubsection{$\Gc$ Corridor}\label{threebends}
	%Consider a corridor $S$ with 3 bends.  W.l.o.g let us assume that the corridor $S$ can't be divided into smaller corridors with cuts perpendicular to subcorridor.Let us consider vertical subcorridors $S_{1}$ and $S_{3}$ which are on top of horizontal subcorridor $S_{2}$ and $S_{3}$ is right of $S_{1}$ and below horizontal subcorridor $S_{4}$. Now consider a corridor comprising of $S_{1},S_{2},S_{3}$ and assuming the w.l.o.g conditions of previous section we get a box for this triple. Similarly we get a box for the triple $S_{2},S_{3},S_{4}$ . Intersection of both the boxes gives us a box whose edges are the topmost,bottom most, leftmost and rightmost edges of the corridor $S$.  By appropriate shifting of vertical rectangles we can convert it into a L corridor without disturbing the guillotine property.Exact details are available in subsubsection \ref{sss3}.\\
The approach is similar to section \ref{twobends}. Let $S$ be a corridor with $3$ bends. Let the top left vertical, bottom horizontal, top right vertical subcorridors and top horizontal subcorridors of $S$ be $S_{1}$, $S_{2}$, $S_{3}$ and $S_{4}$ respectively as shown in Figure \ref{figthreebends}. Consider the smallest subpiece $P$ containing $S$. We define four types of end-to-end cuts possible in $P$ or in any of the subpieces formed by a sequence of cuts in $P$. The rightmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$ is termed as Type $1$. The leftmost end-to-end guillotine cut passing during a single stage of guillotine cutting sequence through $S_{3}$ is termed as Type $3$. The topmost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{2}$ is termed as Type $2$. The bottommost end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{4}$ is termed as Type $4$. Figure \ref{figthreebends} shows all the four types of cuts defined.
\\Basic idea follows divinding $S$ into a corridor $U'$ (with atmost $2$ bends) consisting of some items from $S_{1}$, $S_{2}$, $S_{3}$ ( w.l.og it can be $S_{2}$, $S_{3}$, $S_{4}$ but for the rest of the proof we assume that it's the former case not the latter), a corridor with 0 bends $C$ from a subset of items of $S_{4}$ and a corridor (with at most 3 bends) with the remaining set of items. We follow a recursive approach to define bounding box $B$. Clearly obtaining all four type of cuts will result in a box  bounded by these cuts. \\
We now formally define the algorithm for processing corridor $S$ with $3$ bends. From observation \ref{endtoend} we know that the first cut in any guillotine separable piece is end-to-end. Depending on the type of this cut we do the following processing :
\begin{enumerate}
\item Scenario $1$ : (Type $1$ cut) Add the items of $S_{1}$ which is left of Cut 1 to the left-vertical subcorridor of the 3-bend corridor $U'$. Consider the new-subpiece to be the subpiece which is right of Cut 1. Run algorithm recursively on the new-subpiece.
\item Scenario $2$ : (Type $2$ cut) Add the items of $S_{2}$ which is below Cut 2 to the horizontal subcorridor of $U'$. Consider the new-subpiece to be subpiece which is above Cut 2. Run algorithm recursively on the new-subpiece.
\item Scenario $3$ : (Type $3$ cut) Add the items of $S_{3}$ which is right of Cut 3  to the right-vertical subcorridor of $U'$. Consider the new-subpiece to be the subpiece which is left of Cut 3. Run algorithm recursively on the new-subpiece.
\item  Scenario $4$ : (Type $4$ cut) Pack the items of $S_{4}$ which is above Cut 4 in a new horizontal corridor with 0 bends $C$. Consider the new-subpiece to be the subpiece which is below Cut 4. Run algorithm recursively on the new-subpiece.
\end{enumerate}
 We halt if one of the following three cases happens. First case occurs if at some iteration at least one cut from each type of cut is obtained. The boundaries of subpiece at this step along with the cut considered define the bouding box for remaing set of items of $S$. Thus we get the box $B$ surrounded by $U'$ on three edges and a corridor with 0 bends $C$ on the fourth. Figure \ref{figthreebends} shows final bounding box $B$ formed after the algorithm alongwith $U'$ formed after considering sequence of type $1$ ,type $2$ and type $3$ cuts in subcorridors $S_{1}$, $S_{2}$, $S_{3}$ and the corridor with 0 bends formed from type $4$ cuts in $S_{4}$. Second case occurs if one or more of the subcorridors in the piece exhausts, i.e., all the items of subcorridor are already packed in $U'$ or in $C$. In this case we are left with atmost 2 corridors with at most 2 bends whose items are not part of either $U'$ or $C$. Using the previous section we get that the corridor with atmost two bends is bounded by a box (Except for a corridor with 0 bends which will be dealt in the later subsections) . Third Case occurs when the next guillotine cut in the guillotine cutting sequence passes completely through any subcorridor perpendicular to its longer sides. This divides $S$ into atmost three corridors with atmost 2 bends each. Using the previous section results each corridor with atmost two bends is bounded by a box (Except for a corridor with 0 bends which will be dealt in the later subsections) .\\
\\Now we observe that using the algorithm defined above we add only a $O(\frac{1}{\epsl})$ number of new corridors and corridors with 0 bends. The proof follows from the fact that if it the case that all algorithm halts when atleast one cut from each type of cuts is obtained then in the end we have a corridor ( with atmost 3 bends) , a corridor with 0 bends and a bounding box. This accounts to $O(1)$ new corridors with 0 bends and corridors. Else if it is the case that algorithm halts when one or more of subcorridors is exhausted, i.e., packed in either $U'$ or $C$, then we have a new corridor (with atmost 2 bends) or one new corridor with 0 bends $C$. We then run the algorithm on remaining corridors which has lesser number of bends than $S$ i.e. atmost 2 bends (Except for a corridor with 0 bends which will be dealt in the later subsections) . As it follows from subsections \ref{twobends} and \ref{L corridor}, we get $O(\frac{1}{\epsl})$ corridors from processing in both the cases. In the third case of halting, $O(\frac{1}{\epsl})$ extra corridors with 0 bends follows from the results of subsections \ref{twobends} and \ref{L corridor}.


\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,3) -- (0,0) -- (6,0) -- (6,4) --( 2,4)--(2,3)--(5,3) -- (5,1) -- (1,1) -- (1,3) -- (0,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,0.75) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};
                           \draw (3,3.5) node {\large \textbf{$S_{4}$}};

			\draw (1,3.7) node {\large \textbf{Type 1}};
			\draw (6.9,.45) node {\large \textbf{Type 2}};
			\draw (6,4.7) node {\large \textbf{Type 3}};
			\draw (6.9,3.2) node {\large \textbf{Type 4}};

			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,3.5) -- ( .5,0) ;
			\draw[dotted] (.25,3) -- ( .25,0) ;
			
			\draw[dotted] (0,.5) -- ( 6.5,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0) ;
			\draw[dotted] (5.25,4) -- ( 5.25,0) ;

			\draw[dotted] (2,3.5) -- ( 6,3.5) ;
			\draw[dotted] (2,3.25) -- ( 6.5,3.25) ;
				
		
		\end{tikzpicture}}
		\caption{Types of cuts}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,4) -- (1,1) -- (7,1) -- (7,5) -- ( 6,5) --(3,5)--(3,4)--(6,4)-- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick]  (1.5,1.5) -- (1.5,6) ;% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[thick] (6.5,4.5)--(1.5,4.5);
			\draw[pattern=north east lines, pattern color=black] (6.5,4.5)--(6.5,5)--(3,5)--(3,4.5)--(6.5,4.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,4) -- (1.5,4) -- (1.5,1.5) -- (6.5,1.5) -- (6.5,5) --(7,5) -- (7,1)--(1,1)--(1,4);		

			\draw (4,1.25) node {\large \textbf{$U'$}};
			\draw (5,4.75) node {\large \textbf{$C$}};
			\draw (4,3) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Final Bounding Box of $S$}
	\end{subfigure}
	\caption{Processing 3-bend corridor}
	\label{figthreebends}
\end{figure}
	\subsubsection{$\Bc$-Corridor}
	In this subsection we deal with the items inside a corridor with 0 bends in 2 ways. In first way, the corridors with 0 bends can be either divided into $O_{\eps,\epsl}(1)$ corridors with 0 bends and the corridors with 0 bends as a pseudo rectangle are guillotine separable. In second way, the items in corridors with 0 bends is merged with a corridor and later become a part of boundary $\Lc$ . Given a knapsack, first we construct the boxes as mentioned in the previous subsections. Note that one box may lie completely inside another box. Now consider the set of outermost boxes which are not part of any other box in the original Knapsack. Note that the boundaries of outermost boxes may divide the corridors with zero bends into smaller parts. The number of such smaller parts is $O(\frac{1}{\epsl})$ as the guillotine cuts which are part of the boundary of a single box can divide a corridor with 0 bends into atmost 6 parts and number of such boxes is $O(\frac{1}{\epsl})$. Now we have to deal with 2 cases.\\
\\ In the first case, a corridor with 0 bends say $S$ lies inside a box and if a part or the complete corridor with 0 bends $S$ lies between the lines along the two longer edges of a subcorridor say $S_{1}$ of a boundary $\Lc$ and the orientation of the corridor is same as that of the subcorridor $S_{1}$. This case is approriately handled in the subsubsection \ref{sssl} and we satisfy all the properties of the lemma \ref{structure}. Suppose instead that the longer edges of the rectangles in the corridor with 0 bends $S$ was perpendicular to the longer edges of subcorridor $S_{1}$ of boundary $\Lc$ then this case is approriately handled in the subsubsection \ref{sssl} and we satisfy all the properties of the lemma \ref{structure}. Similar argument holds for corridors with 2 or 3 bends instead of $\Lc$ corridor and after all the similar processing as done in subsubsection \ref{sssl}  we convert them into a $\Lc$ corridor by appropriate shifting as mentioned in the subsubsections \ref{sss2} and \ref{sss3}.\\
\\Now in the second case the corridors with 0 bends lies outside any box in the original knapsack. Now consider the set of guillotine cuts which separates the corridors with 0 bends and the boxes. Note that the way we have constructed the outermost boxes the guillotine cuts don't pass through the boxes except it's edges. Consider one corridor with 0 bends $S_{1}$ and let it's orientation be horizontal. Then we can divide into the following subcases based on the type of cut through $S_{1}$ and the interaction of the cuts with other cuts or rectangles:
\begin{itemize}
\item Subcase 1:  Now consider the horizontal cuts (which are not entirely inside the corridor with 0 bends $S_{1}$) through $S_{1}$. If 3 or more horizontal cuts are intercepted by the same vertical cut in the guillotine cutting sequence then consider the topmost and the bottom cut as the cuts and ignore the rest. This subcase is depicted in Figure \ref{C01b}.
\item Subcase 2: Now consider set of vertical cuts which intercept the horizontal cuts through $S_{1}$. If these vertical cuts are edges of an outermost box which we created then there can be atmost $O(\frac{1}{\epsl})$ of them. Now if these vertical cuts are edges of vertical rectangle which belonged to different corridors then these can be atmost $O_{\eps}(1)$ of them. Both of the scenarios are depicted together in Figure \ref{C01c}.
\item Subcase 3:Supposed the rectangles which intercept the horizontal cuts through $S_{1}$ belonged to the same corridor $S_{2}$. Now assume 2 or more than 2 consecutive horizontal cuts dont have space more than $\epsl N$ between them (otherwise the cuts are intercepted by atmost $O_{\epsl}(1)$ rectangles) . Then we take that cut $l$ among the consecutive cuts such that $|l\bigcap S_{2}|$ is maximum and shift vertically those rectangles which intercepted these consecutive cuts other than $l$ and make them touch $l$. Hence we consider $l$ as valid guillotine cut and deal with the rest of the consecutive cuts using the Subcase 1. Subcase 3 is depicted in Figure \ref{C02a} and Figure \ref{C02b}.  
\item Subcase 4: Using the same techniques of Subcase 1 and 3 and applying it to the vertical cuts which pass through some vertical corridor $S_{3}$ with zero bends (repeat the same for other set of cuts which pass through the same vertical corridor with 0 bends)  and are intercepted by the rectangles in $S_{2}$ we get that there can be atmost $O(\frac{1}{\epsl})$ vertical cuts  (which are not entirely inside the corridor with 0 bends $S_{1}$) passing through $S_{1}$ since width of each rectangle is atleast $\epsl N$. This subcase is depicted in Figure \ref{C01a}.
\end{itemize}
Now we argue that atmost $O(\frac{1}{\epsl})$ horizontal cuts (which are not entirely inside the corridor with 0 bends $S_{1}$) pass through the corridor with 0 bends $S_{1}$. Subcase 2 and Subcase 3 ensure that the number of vertical cuts which intercept the horizontal cuts passing through $S_{1}$ is $O_{\eps,\epsl}(1)$. And for each such vertical cut we end up keeping atmost 2 horizontal cuts which pass through $S_{1}$ as explained in Subcase 1. Now these horizontal cuts along with the vertical cuts of Subcase 4 and vertical edges of $S_{1}$ results into partition of $S_{1}$ into $O_{\eps,\epsl}$ corridors with 0 bends and these corridors when considered as a pseudo rectangle is guillotine separable
\\
\\ Now the procedure mentioned above is recursively applied to those portion of the outermost boxes which doesn't have items from its boundary $L$.  This process stops when there is no corridor with atleast one bend which is not bounded by any box or there is no corridor with 0 bends which when considered as a pseudo item isn't guillotine separable. Number of such boxes bounding the $\Lc$ corridor or items of a corridor with 0 bends is $O_{\eps,\epsl}(1)$. This follows from constructive procedures in subsection \ref{ssss} and the fact that we started the section with $O_{\eps,\epsl}(1)$ corridors with 0 bends and corridors.

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,8);
			\draw (1,4) rectangle (5,5);
			\draw[dotted] (0,4.3) -- ( 8,4.3) ;
			\draw[dotted] (0,4.6)--(8,4.6);
			\draw [dotted] (3,4.6)--(3,8);
			\draw [dotted] (2.3,4.3)--(2.3,0);
			\draw [dotted] (2,4)--(2,0);
			\draw[dotted] (2.5,4)--(2.5,0);
			\draw[dotted] (2.6,4)--(2.6,0);
			\draw[dotted] (2.7,4)--(2.7,0);			
			\draw[dotted](3.6,4.3)--(3.6,0);	
			\draw [dotted] (1,0)--(1,8);
			\draw [dotted] (5,0)--(5,8);
			
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Constant number of vertical cuts through a corridor $C$ which has horizontal orientation}\label{C01a}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			
			\draw (1,4) rectangle (5,6);
			\draw[solid,fill=lightgray] (7,3) rectangle (10,7);	
			\draw[dashed] (0,4.3) -- ( 7,4.3) ;
			\draw[dotted] (0,4.6)--(7,4.6);
			\draw[dotted] (0,4.9)--(7,4.9);
			\draw[dotted] (0,5.2)--(7,5.2);
			\draw[dotted] (0,5.5)--(7,5.5);
			\draw[dashed] (0,5.8)--(7,5.8);
			\draw[dotted](7,0)--(7,10);
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			\draw (8,5) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{We choose the topmost and bottommost horizontal cuts(shown as dashed lines in this figure ) if more than 3 horizontal cuts are intercepted by the same vertical cut as shown in this figure. Then these chosen cuts along with the portion of the boundary vertical edges of $C$ form the edges of a corridor with 0 bends which is guillotine separable.Rest of the cuts which were not chosen is divided into 2 parts and pass through rectangles which are outside $C$ }\label{C01b}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			\draw (1,4) rectangle (5,6);
			\draw[solid,fill=lightgray] (6,5) rectangle (8,7);
			\draw[solid,fill=lightgray] (8.3,1) rectangle (9,5);	
			\draw[dotted] (0,4.6)--(8.3,4.6);
			\draw[dotted] (0,5.8)--(6,5.8);
			
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			\draw (8.6,3) node {\large \textbf{$C_{1}$}};
			\draw (7,6) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Horizontal cuts intercepted by different boxes or corridors with 0 bends}\label{C01c}
	\end{subfigure}
	
	\caption{Handling Corridors with 0 bends Part-1}

\end{figure}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			
			\draw (1,4) rectangle (5,6);
			\draw[solid] (7,3) rectangle (10,7);	
			\draw[dotted] (0,4.3) -- ( 7.3,4.3) ;
			\draw[dotted] (0,4.6)--(7.6,4.6);
			
			\draw[dashed] (0,5.2)--(7.9,5.2);
			\draw[dotted] (0,5.5)--(7.6,5.5);
			\draw[dotted] (0,5.8)--(7.3,5.8);
			\draw[solid,fill=lightgray] (7.3,5.7) rectangle (7.5,6.8);
			\draw[solid,fill=lightgray] (7.6,5.4) rectangle (7.8,6.5);
			\draw[solid,fill=lightgray] (7.9,4) rectangle (8.1,6.2);
			\draw[solid,fill=lightgray] (7.5,4.8) rectangle (7.7,3.7);
			\draw[solid,fill=lightgray] (7.2,4.5) rectangle (7.4,3.4);
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			\draw (9,5) node {\large \textbf{$C_{1}$}};
			\draw (6,5) node {\large \textbf{$l$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Horizontal cuts are intercepted by vertical rectangles belonging to same corridor with 0 bends. Identify the horizontal cut $l$ (dashed line in this figure)which has maximum intrusion into corridor $C_{1}$. }\label{C02a}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			
			\draw (1,4) rectangle (5,6);
			\draw[solid] (7,3) rectangle (10,7);	
			\draw[dotted] (0,4.3) -- ( 7.3,4.3) ;
			\draw[dotted] (0,4.6)--(7.3,4.6);
			
			\draw[dashed] (0,5.2)--(7.9,5.2);
			\draw[dotted] (0,5.5)--(7.3,5.5);
			\draw[dotted] (0,5.8)--(7.3,5.8);
			\draw[solid,fill=lightgray] (7.3,5.2) rectangle (7.5,6.3);
			\draw[solid,fill=lightgray] (7.6,5.2) rectangle (7.8,6.3);
			\draw[solid,fill=lightgray] (7.9,4) rectangle (8.1,6.2);
			\draw[solid,fill=lightgray] (7.5,5.2) rectangle (7.7,4.1);
			\draw[solid,fill=lightgray] (7.2,5.2) rectangle (7.4,4.1);
			\draw (4.5,4.75) node {\large \textbf{$C$}};
			\draw (9,5) node {\large \textbf{$C_{1}$}};
			\draw (6,5) node {\large \textbf{$l$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Then shift all the rectangles which are intercepting other cuts which are under consideration so that it touches cut $l$. Cuts other than $l$ are bow divided into 2 group and are now dealt in the same way as we dealt the cuts intercepted by same vertical cut}\label{C02b}
	\end{subfigure}

	\caption{Handling Corridors with 0 bends Part-2}

\end{figure}

	\subsection{Shifting Procedure}\label{ssss}
	In this subsection by boundary corridor we mean that the corridor is bounded by a box which is obtained by the recursive procedure in the subsection  \ref{L corridor}, \ref{twobends}, \ref{threebends}. Also we assume that the cuts which we are considering in a box $B$ don't pass through the smaller boxes inside $B$ except through it's edges.
\subsubsection{Handling rectangles or corridors with 0 bends interacting with a boundary $\Lc$ corridor}\label{sssl}
	Consider a boundary $\Lc$ corridor $S$ with vertical subcorridor $S_{1}$ placed top left with respect to the horizontal subcorridor $S_{2}$. Now consider a sequence of guillotine cuts (cut is parallel to the orientation of the subcorridor and the rectangles which are being separated in that subcorridor) which separates the rectangles in the boundary $\Lc$. Continue this process till there doesn't exist any such cut. Either we have separated all the rectangles of a subcorridor of boundary $\Lc$ or still we have a portion of the boundary $\Lc$ left. In the former case we fix the rectangles which got separated due to guillotine cuts as the boundary $\Lc$ of the original box. In the later case w.l.o.g let the next stage of cuts be horizontal and these cuts passes though $S_{1}$ only . Now consider the lowermost cut among these horizontal cut. Let it be $l$. Let $l$ be at a distance of $h$ from the top of the box. If $h \leq \epsl N$,we remove the items in the strip above $l$, then we shift upwards the rectangles below the cut $l$ except those rectangles which got separated due to previous guillotine cuts by a distance of $h$ and then place the rectangles from the strip which we removed initially in the empty region created due to shifting. Otherwise if $h > \epsl N$ then we consider the items separated due to cuts before $l$ as the boundary $\Lc$ of the original box and we divide rest of region of the box into 2 smaller boxes with cut $l$ being the common edge between both the smaller boxes. Now that an original boundary $\Lc$ along with some corridors with 0 bends gets divided into $O(\frac{1}{\epsl})$ smaller boundary $\Lc$. The reason being that a boundary $\Lc$ and some corridors with 0 bends get divided into smaller boundary $\Lc$ only if the height of the new box which we are about to create is greater than $\epsl  N$ and therefore number of such boxes is $O(\frac{1}{\epsl})$. Similar processes can be done to corridors with 2 or 3 bends.
	\subsubsection{Converting boundary corridor with $2$ bends to a single Boundary $\Lc$ in a box}\label{sss2}
	Let us consider a boundary corridor with $2$ bends with two vertical subcorridors $S_{1}, S_{3}$ on top of the horizontal subcorridor $S_{2}$ with $S_{3}$ being placed to the right of $S_{1}$. W.l.o.g let us assume that the first stage cuts in the guillotine cutting sequence in the box is vertical. Now consider the cut $l$ through $S_{3}$. Let the distance between $l$ and edge of the boundary be $d$. Now remove the strip to the right of $l$ and shift the rest of items of box to the right by a distance of $d$. Now in the empty region created near the left edge of the box we place the strip which we removed. Now consider the rectangles in this strip, rectangles to the left of cut through $S_{1}$ before the shifting procedure and set of horizontal rectangles whose guillotine cut is intercepted by the former rectangles mentioned in this sentence. We now freeze these rectangles after shifting and consider the rest of the box as a new box and recursively apply the process to remaining part of the corridor till we don't have any vertical guillotine cuts left. If we have exhausted the corridor then we are done and we have a single boundary $\Lc$. Otherwise we must have horizontal cut through the remaining portion of the box to separate the rectangles because there no end to end vertical cut. We handle this in sub-subsection \ref{sssl}. The boundary $\Lc$ achieved due to the sequence of guillotine cuts forms the boundary $\Lc$ of the box. Also this boundary $\Lc$ can be converted into $O_{\epsl}$ smaller boundary $L$ with width atmost $\epsl N$ by  dropping atmost $O_{\eps,\epsl}(1)$ items as shown in Figure \ref{divL}. 
	\subsubsection{Converting boundary corridor with 3 bends to a single Boundary $\Lc$}\label{sss3}
	Consider a boundary corridor $S$ with 3 bends. Let us consider vertical subcorridors $S_{1}$ and $S_{3}$ which are on top of horizontal subcorridor $S_{2}$. $S_{3}$ is right of $S_{1}$ and below horizontal subcorridor $S_{4}$. Consider the horizontal guillotine cut through $S_{4}$ and remove the rectangles above this cut and place it  below corridor $S_{2}$ by shifting rectangles below the cut upwards. Now freeze this set of rectangles from $S_{4}$ which were moved down. Now in the remaining portion of the box take the vertical guillotine cut through $S_{3}$ and remove the rectangles to the right of this cut and place it to the left of $S_{1}$. Now freeze the rectangles in the similar fashion as done in the Sub-subsection \ref {sss2} and recursively repeat the process for the rectangles in subcorridors $S_{3}, S_{4}$ which aren't freezed yet till we exhaust these both the corridors. Note that we stop if there is no vertical cut through $S_{3}$ or a horizontal cut through $S_{4}$ then there must exist which divides the remaining portion of the box into 2 parts each containing corridors with atmost 2 bends. If any one of them has a corridors of 2 bends then we can use the results of sub-subsection \ref{sss2} to get a box with boundary $\Lc$. Otherwise, we are done  and the rectangles which got freezed before this step form the boundary $\Lc$ of our original box with which we started initially. Also this boundary $\Lc$ can be converted into $O_{\epsl}$ smaller boundary $L$ with width atmost $\epsl N$ by  dropping atmost $O_{\eps,\epsl}(1)$ items  as shown in Figure \ref{divL}.

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}

		\centering
		\resizebox{!}{3.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (10,10);
			
			\draw [solid,fill=lightgray] (0,0)--(0,10)--(3,10)--(3,3)--(10,3)--(10,0)--(0,0);
			
			\draw [dashed] (1,10)--(1,1)--(10,1);
			\draw [dashed] (2,10)--(2,2)--(10,2);
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}



	\caption{Dividing a boundary $L$ (shaded region) into smaller boundary using dashed lines as shown in this figure. Vertical and horizontal dashed lines meet at the boundary curve. Dashed lines also form the edges of the smaller boxes which bound the new $L$ corridors being created}\label{divL}

\end{figure}
	           
	%\subsubsection{Merging 2 boundary $\Lc$ into a single boundary $\Lc$}\label{sss2l}
	%Now consider that we have 2 boundary $\Lc$ for the same box. If there is any end to end cut possible in the box which doesn't pass through any of the 2 boundary $\Lc$ or it passes through one or more than one subcorridors of 2 boundary $\Lc$ but it is perpendicular to the orientation of these subcorridors, then we divide the box into 2 boxes. We repeat the same procedure on the smaller box which contains both the boundary $\Lc$. If at any stage we find a cut which places both the boundary $\Lc$ in 2 different smaller boxes then we are done. So we now assume that there is no such end to end cut in the box we are considering which has 2 boundary $\Lc$. If the 2 boundary $\Lc$  are placed diagonally opposite to each other then consider the 2 boundary $\Lc$ as a corridor with 3 bends and convert into a single boundary $\Lc$ as mentioned in the subsubsection  \ref{sss3}. If the process in subsection \ref{sss3} can't covert it into a single boundary $\Lc$ it means in the remaining portion of the box which hasn't formed a part of the boundary $\Lc$ we have an end to end cut which separates the 2 remaining portions of the 2 boundary $\Lc$. If the boundary $\Lc$ are placed at the adjacent corners of the box then consider the 2 boundary $\Lc$ as a corridor with 2 bends and convert it into a single boundary $\Lc$ as mentioned in the subsubsection \ref{sss2}. If the process in subsection \ref{sss2} can't covert it into a single boundary $\Lc$ it means in the remaining portion of the box which hasn't formed a part of the boundary $\Lc$ we have an end to end cut which separates the 2 remaining portions of the 2 boundary $\Lc$.
	%\subsubsection{Merging 3 boundary $\Lc$ into a single boundary $\Lc$}\label{sss3l}
	%Now consider that we have 3 boundary $\Lc$ for the same box. If there is any end to end cut possible in the box which doesn't pass through any of the 3 boundary $\Lc$ or it passes through one or more than one subcorridors of 3 boundary $\Lc$ but it is perpendicular to the orientation of these subcorridors, then we divide the box into 2 boxes. One of the box contains 2 boundary $\Lc$ and other box contains 1 boundary $\Lc$. Boxes with 2 boundary $\Lc$ is handled in subsubsection \ref{sss2l}. So we now assume that there is no such end to end cut in the box we are considering which has 3 boundary $\Lc$. Now consider the 3 boundary $\Lc$ as a corridor with 3 bends and convert into a single boundary $\Lc$ as mentioned in the subsubsection  \ref{sss3}. If the process in subsection \ref{sss3} can't covert it into a single boundary $\Lc$ it means in the remaining portion of the box which hasn't formed a part of the boundary $\Lc$ we have an end to end cut which separates the 3 remaining portions of the 3 boundary $\Lc$ into smaller boxes with one box containing 2 boundary $\Lc$ and other box containing 1 boundary $\Lc$. Boxes with 2 boundary $\Lc$ is handled in subsubsection \ref{sss2l}.
	 %\subsubsection{Merging 4 boundary $\Lc$ into a single boundary $\Lc$}\label{sss4l}
	%Now consider that we have 4 boundary $\Lc$ for the same box. If there is any end to end cut possible in the box which doesn't pass through any of the 4 boundary $\Lc$ or it passes through one or more than one subcorridors of 4 boundary $\Lc$ but it is perpendicular to the orientation of these subcorridors. Each box has now 2 boundary $\Lc$. Boxes with 2 boundary $\Lc$ is handled in subsubsection \ref{sss2l}. So we now assume that there is no end to end cut in the box we are considering which has 4 boundary $\Lc$. Let's combine these to form a ring. Now consider the sequence of gullotine cuts which separate the rectangles in the ring. If we are cutting (cut is parallel to the orientation of the subcorridor and the rectangles which are being separated in that subcorridor) through leftmost vertical subcorridor or bottom most horizontal subcorridors then we freeze these rectangles as we freezed rectangles in subsubsection \ref{sss2l} and \ref{sss3l}. Now in the remaining portion of the box if there is a cut $l_{1}$ (cut is parallel to the orientation of the subcorridor) through rightmost vertical subcorridor and the distance between $l_{1}$ and edge of the boundary to the right of it be $d$ then we remove the strip to the right of $l_{1}$ and shift the rest of items of box which are not freezed to the right by a distance of $d$. Now in the empty region created near the left edge of the box we place the strip which we removed. Now freeze the rectangles in the strip which we moved. Do the same process if there is a cut (cut is parallel to the orientation of the subcorridor the rectangles which are being separated in that subcorridor) through the upper most horizontal corridor and now instead of shifting the strip above the cut to the left we shift it down by appropriately shifting the remaining portion of the box upwards which isn't still freezed. Continue this process till we convert these in to single boundary $\Lc$. If at some we can no longer find any cut parallel to the orientation of the subcorridors in the remaing portion of the ring it implies that there should exist an end to end cut in the remaining portion of the box which divides the remaining portion of the box into 2 boxes each containing 2 boundary $\Lc$ atmost and this case is dealt in subsubsection \ref{sss2l}. So now have a box with boundary $\Lc$ and possibly 2 smaller boxes each containing 2 boundary $\Lc$.

	\subsection{Guillotine property}
	The construction of boxes and shifting of rectangle doesn't disturb the guillotine property. Now we show that the processing which we do in Subsection \ref{prosec} doesn't disturb the guillotine property if it is done to the boundary $\Lc$ which we obtain in the previous section. Now consider w.l.o.g that we are processing (as done in Subsection \ref{prosec}) a vertical subcorridor of the boundary $\Lc$ which is placed top-left with respect to horizontal subcorridor. Note that this processing does not create any conflict in terms of guillotine separability with elements in boxes and corridors with 0 bends outside the box bounding this boundary $\Lc$ since by construction the boxes and corridors with 0 bends are guillotine separable when considered as a pseudorectangle. Also the way in which we have constructed the boundary $\Lc$, we always have a sequence of vertical (resp., horiztonal) cuts through the vertical (resp., horiztonal) subcorridor of boundary $\Lc$ which separates the rectangles in the vertical (resp., horiztonal) subcorridor. This ensures that as long we can separate out the items in the boundary $L$ from the rest of box using cuts which doesn't pass through the rest of the box, then the items in the rest of box can be separated as we have not changed their orientation. Now we need to focus on the boundary curve of the $\Lc$ corridor. Consider the strip containing the thin items. Let the length of the shorter vertical edge be $l$. Now the vertical strip which replaces this strip has rectangles of length atmost $l$. So the horizontal rectangles which interacted with the thin items can be directly separated as there is no vertical rectangle intercepting the cut. Similar analogy for other strips shows that there is no conflict with horizontal rectangles. So we can conclude that the processing in Subsection \ref{prosec} doesn't disturb guillotine property.
	


==> Backup/4_Corridor_Decomposition.tex <==
\section{$\Bc \Lc$-decomposition for guillotine packing} \label{sec:bl}
In this section we will show that we can have a better decomposition of the optimal guillotine packing.
We will show the existence of a corridor-decomposition where all corridors are either $\Bc$ or $\Lc$s.	
We will prove the main strcutural result as follows:	
\begin{thm}
\label{thm:ldecom}
There exists a corridor partition (we call it $\Bc \Lc$-decomposition) and $\optco \subseteq \optsk$ such that:
\begin{enumerate}\itemsep0pt
\item there is a subset $\optco^{cross} \subseteq \optco$ with  $|\optco^{cross}| \le O_\eps(1)$ such that  each $i\in \optco \setminus \optco^{cross}$ is fully contained in some corridor,
\item $\profit(\optco) \ge (1-O(\eps))\profit(\optsk)$,
\item the number of corridors is $O_{\eps,\epsl}(1)$ and each corridor is either $\Bc$ or $\Lc$ corridor with width at most $\epsl N$.
\end{enumerate}
\end{thm}		
	
To prove the theorem, first we will start with the corridor decomposition from Lemma \ref{lem:corridorPack}. Then process the $\Zc$-bends in the corridors to obtain only spiral corridors. Thereafter, we will further process to obtain spiral corridors with bends at most 4. Finally we will process $\Uc$ and $\Gc$ corridors to obtain only $\Lc$ or $\Bc$ corridors. 	
%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Obtaining corridors of types $\Bc, \Lc, \Uc, \Gc$} 
\label{subsec:blug}


		\begin{figure}
			\captionsetup[subfigure]{justification=centering}
			\hspace{-15pt}
			
				\centering
				\resizebox{!}{4cm}{
					\begin{tikzpicture}					
					\draw[solid] (0,6) rectangle (2,10);
					\draw[solid, fill=lightgray] (0,4) rectangle (2,6);
					\draw[solid] (2,4) rectangle (8,6);
					\draw[solid, fill=lightgray] (8,4) rectangle (10,6);
					\draw[solid] (8,0) rectangle (10,4);
		
					\draw (1,8) node {\large \textbf{$S_{1}$}};
					\draw (1,5) node {\large \textbf{$S_{12}$}};
					\draw (6,5) node {\large \textbf{$S_{2}$}};
					\draw (9,5) node {\large \textbf{$S_{23}$}};
					\draw (9,2) node {\large \textbf{$S_{3}$}};
		
					\end{tikzpicture}}
				\caption{Corridor C consisting of subcorridors $S_{1},S_{2},S_{3}$ and overlapping regions of the subcorridors $S_{12}$  and  $S_{23}$.}
				\label{zstructure}
		\end{figure}
		
	
	
\subsubsection{Obtaining spiral corridors}
First, we show how to process $\Zc$-bends. 

\begin{lem}
\label{theorem1}
Any $\Zc$-corridor $C$ can be decomposed into $O(\frac{1}{\epsl})$. corridors of type $\Bc$ or $\Lc$. 
\end{lem}
\begin{proof}
W.l.o.g.~assume the center-sc of $C$ to be horizontal (See Figure \ref{zstructure}). 
%Region $S_{12}$ is shared by subcorridors $S_{1}$ and $S_{2}$ and similar convention holds for $S_{23}$. 
Consider the guillotine cutting sequence of all rectangles in the knapsack. 
Let $P$ be the smallest piece containing $C$, i.e., the next guillotine cut in $P$ passes through $C$. 
Now we will consider the guillotine cutting  sequence of rectangles in $P$ to iteratively decompose the $\Zc$-corridor into one of the three subcases: ($i$) into two $\Lc$-corridors, or ($ii$) a $\Bc$-corridor and an  $\Lc$-corridor, or ($iii$) a $\Bc$-corridor and a smaller $\Zc$-corridor.  
We stop when we reach subcases ($i$) or ($ii$). Otherwise in subcase ($iii$), we continue iteratively. 
This sequence can have five types of cuts:
\begin{itemize}
\item {\em HS}: horizontal guillotine cut which passes through a side-sc but doesn't pass through center-sc,
%\item Cut 2: horizontal guillotine cut which passes through $S_{3}$ and doesn't pass through $S_{23}$,
\item {\em VS}: vertical guillotine cut which passes through a side-sc,
%\item Cut 4: vertical guillotine cut which passes through $S_{3}$,
\item  {\em VC}: vertical guillotine cut which passes through center-sc but doesn't pass through any side-sc,
\item {\em HC}: horizontal guillotine cut which passes through center-sc,
\item {\em NC}: cut which doesn't pass through $\Zc$-corridor.
\end{itemize}
Now, if we get cuts of type  {\em VC} (or {\em HC}) at any subpiece, we are in case $(i)$ as we obtain 2 $\Lc$-corridors. 
On the other hand, if we get {\em NC}-type cut we just focus on the subpiece containing the  $\Zc$-corridor of the present iteration.
If we have either cuts of type {\em VS} (or {\em HS}) passing through a side-sc then we are dividing the $\Zc$-bend into a rectangular region and a smaller $\Zc$-corridor. 
If there are no rectangle left in one of the side-sc of the smaller $\Zc$-corridor, we call the subcorridor to be {\em exhausted}. In case of exhaustion of a subcorridor, we reach case $(ii)$ as the smaller $\Zc$-corridor can be considered as an $\Lc$-corridor by ignoring the exhausted side-sc.
Otherwise, we are in case $(iii)$. 
The rectangles in side-sc have height $\ge \epsl N$, so the consecutive cuts of {\em HS} creating $\Bc$-corridor have to be at a distance of atleast $\epsl N$. This ensures that the number of such corridors is $O(\frac{1}{\epsl})$. 
Note that we can merge all the adjacent rectangular regions obtained due to successive cuts of {\em VS} into a $\Bc$-corridor of same height till we arrive at a cut of different type (excluding {\em NC}). And since the number of cuts excluding {\em VS} and {\em NC} is $O(\frac{1}{\epsl})$, therefore number of such $\Bc$-corridors created due to successive cuts of {\em VS} is $O(\frac{1}{\epsl})$. 
\end{proof}

\arir{need to add a figure. }

\begin{figure}
			\captionsetup[subfigure]{justification=centering}
			\hspace{-15pt}
			
				\centering
				\resizebox{!}{10cm}{
					\begin{tikzpicture}					
					
					\draw[solid,fill=lightgray] (0,4)--(0,10)--(7.5,10)--(7.5,4)--(6.5,4)--(6.5,8)--(2,8)--(2,6)--(6,6)--(6,2)--(8,2)--(8,6)--(10,6)--(10,0)--(4,0)--(4,4)--(0,4);
					\draw (1.5,7) node {\large \textbf{$S_{2}$}};
					\draw (4,8.5) node {\large \textbf{$S_{1}$}};
					\draw (7.3,5) node {\large \textbf{$S_{0}$}};
					\draw (2,4.5) node {\large \textbf{$S_{3}$}};
					\draw (5,3) node {\large \textbf{$S_{4}$}};
					\draw (7,1.5) node {\large \textbf{$S_{5}$}};
					\draw (9.6,3) node {\large \textbf{$S_{6}$}};
					\draw [dashed] (0,9.8)--(7.4,9.8);
					\draw [dashed] (0.2,9.8)--(0.2,4);
					\draw [dashed] (0.2,9.6)--(7.3,9.6);
					\draw [dashed] (0.4,9.6)--(0.4,4);
					\draw [dashed] (0.4,9.4)--(7.2,9.4);
					\draw [dashed] (0.6,9.4)--(0.6,4);
					\draw [dotted] (6.5,8)--(7.5,10);
					\draw [solid] (0.6,4)--(0.6,9.4)--(7.1,9.4)--(7.1,4);
					\draw[solid](4.5,6)--(4.5,0.6);
					\draw [dashed] (4,0.2)--(9.8,0.2);
					\draw[dashed] (4,0.4)--(9.6,0.4);
					\draw[solid](4,0.6)--(9.4,0.6)--(9.4,6);
					\draw[dotted](10,0)--(8,2);
						
					\end{tikzpicture}}
				\caption{Shaded region is corridor $C$. Dashed lines are sequence of guillotine cuts. Boundary curve is depicted by dotted lines. Solid line inside the corridor $C$ divides it into O(1) corridors. Except atmost 1 corridor, rest of the $O(1)$ corridors have lesser number of $\Zc$ bends than $C$ } 
				
		\end{figure}

\begin{lem}\label{noz}
A non-spiral corridor $C$ can be decomposed  into $O_{\eps}(1)$ spiral corridors and $O_{\eps}(1)$ $\Zc$-corridors by dropping atmost $O_{\eps,\epsl}(1)$ rectangles. 
\end{lem}
\arir{write this proof and figure appropriately.}
\begin{proof}
There are two cases. 

\noindent \textit{Case 1: $C$ is open corridor with at least one $\Zc$-bend.} Let $C$ have $k$ subcorridors $\{ S_{1},S_{2},S_{3},...,S_{k}\}$ such that $\forall i \in [k-1]$, $S_{i}$ and $S_{i+1}$ share a region $S_{i,i+1}$ with each other. Assume there are 5 subcorridors (If there are less than 5 subcorridors the following proof would still hold) $S_{i'+1}, S_{i'+2}, S_{i'+3}, S_{i'+4} $ and $S_{i'+5}$ such that $\{S_{i'+2},S_{i'+3},S_{i'+4}\}$ form a $\Zc$ bend. Let $S_{i'+3}$ be a horizontal subcorridor and $S_{i'+2}$ be situated to the top left of $S_{i'+3}$. Let us consider a sequence of guillotine cuts through the five subcorridors  $S_{i'+1}, S_{i'+2}, S_{i'+3}, S_{i'+4} $ and $S_{i'+5}$. We now have 3 subcases.\\

In the first subcase, after a sequence of guillotine cuts through corridor $C$ (including those which is coincident with the edges of $C$) , we get our first cut $l'$ which passes through $S_{i'+3}$ only. Now consider the guillotine cuts which occured before the cut $l'$. Let $l_{i'+2}$ be the rightmost vertical cut through $S_{i'+2,i'+3}$. Extend the cut $l_{i'+2}$ so that it touches the boundary curve between $S_{i'+1}$ and $S_{i'+2}$ at point $P$. Now draw a line $l_{i'+1}$ from point $P$ parallel to the orientation of $S_{i'+1}$ till it touches the boundary curve between $S_{i'+1}$ and $S_{i'}$. Continue the same process by drawing lines $l_{j}$ through corridors $S_{j}$ where $1 \leq j \leq i'$ in similar fashion. Stop drawing these lines when we draw a line $l_{1}$ through $S_{1}$ parallel to the orientation of $S_{1}$ and reach its boundary edge.   Lines $\{l_{1},l_{2},..,l_{i'+2}\}$ partitions the corridor $C$ into atmost 2 smaller corridors $C_{1},C_{2}$. $C_{1}$ contains rectangles from the subcorridors $S_{1},..,S_{i'+2}$ only. $C_{2}$ contains rectangles from the subcorridors $S_{1},...,S_{k}$ (maynot contain rectangles from every subcorridor). In a similar way we can partition $C_{2}$ into atmost 2 corridors $C_{3}$ and $C_{4}$ where $C_{3}$ contains rectangles from the subcorridors $S_{i'+4},..,S_{k}$ only and $C_{4}$ contains rectangles from the subcorridors $S_{1},...,S_{k}$ (maynot contain rectangles from every subcorridor). During this process of partitioning we drop atmost $O_{\eps,\epsl}(1)$ rectangles. Now suppose that the first cut through $S_{3}$ only is a horizontal cut. This divides the $C_{4}$ into 2 corridors containing atleast one lesser $\Zc$ bend when compared to $C$. Similarly if the first cut through $S_{3}$ only was vertical, then we can partition $C_{4}$ into 2 corridors containing atleast one lesser $\Zc$ bend when compared to $C$.\\

Now let us consider the second subcase where we dont have any cut in the guillotine cutting sequence which passes through the region of $S_{3}$ which is not part of any other subcorridor and neither $S_{i'+2}$ nor $S_{i'+4}$ has a horizontal cut passing through the unshared regions of these subcorridors. If $S_{i'+2}$ gets exhausted during the guillotine cutting sequence then we simply divide the corridor $C$ into 2 corridors $C_{1'}$ and $C_{2'}$ such that $C_{1'}$ contains rectangles from  the subcorridors $S_{1},..,S_{i'+2}$ only and $C_{2'}$ contains rectangles from the subcorridors $S_{i'+3},...,S_{k}$ only. Similar partitioning can be done if $S_{i'+4}$ gets exhausted. Otherwise eventually due to the sequence of guillotine cuts $S_{i'+1}$ and $S_{i'+5}$ will be exhausted. Then we can partition $C$ into 3 corridors $C_{1''}$,$C_{2''}$ and $C_{3''}$ in similar fashion as we did in the previous subcase (which was done previously using the lines $\{l_{1},l_{2},..,l_{i'+2}\}$). $C_{1''}$ contains rectangles from the subcorridors $S_{1},..,S_{i'+2}$, $C_{2''}$ contains rectangles from the subcorridors $S_{i'+4},..,S_{k}$, $C_{3''}$ contains rectangles from the subcorridors $S_{i'+2},S_{i'+3},S_{i'+4}$.\\

Now let us consider the last case where we dont have any cut in the guillotine cutting sequence which passes through the region of $S_{3}$ which is not part of any other subcorridor and either $S_{i'+2}$ or $S_{i'+4}$ has a horizontal cut passing through the unshared regions of these subcorridors.Let us assume that we have a horizontal cut through the unshared region of $S_{i'+2}$. Let $l_{v'}$ be the last vertical cut through $S_{i'+2,i'+3}$ before the first horizontal cut $l_{h}$ through $S_{i'+2}$ only. Let $l_{h'}$ be the part of $l_{h}$ which is inside $S_{i'+2}$. Extend $l_{v'}$ to meet the boundary curve between $S_{i'+2}$ and $S_{i'+1}$. Then continue making lines parallel to the orientation to the subcorridors $S_{i'+1},S_{i'},...,S_{1}$ as done in the previous subcase. Then using the lines created and $l_{h'}$ we can divide $C$ into 3 corridors $C_{1'''},C_{2'''},C_{3'''}$. $C_{1'''}$ and $C_{2'''}$ contains rectangles from the subcorridors $S_{1},..,S_{i'+2}$ only. $C_{3'''}$ contains rectangles from the subcorridor $S_{i'+2},...,S_{k}$. If there is a horizontal cut through the unshared region of $S_{i'+4}$ then we can partition $C_{3'''}$ into $C_{4'''}, C_{5'''},C_{6'''}$ where $C_{4'''}$ and $C_{5'''}$ contains rectangles from the subcorridors $S_{i'+4},..,S_{k}$,  $C_{6'''}$ contains rectangles from the subcorridors $S_{i'+2},S_{i'+3},S_{i'+4}$. Otherwise $C_{3'''}$ is handled appropriately in subcase 2.\\

This concludes the proof  for Case 1.\\

\noindent \textit{Case 2: $C$ is a closed corridor with at least one $\Zc$-bend.}  Let $S_{1}$ be the leftmost vertical subcorridor in $C$, $S_{2}$ be the bottommost horizontal subcorridor in $C$, $S_{3}$ be the rightmost vertical subcorridor in $C$, $S_{4}$ be the topmost subcorridor in $C$.  Depending on the arrangement of these four subcorridors $\{S_{1},S_{2},S_{3},S_{4}\}$ we separate out the rectangles from these 4 subcorridors during guillotine cutting sequence into atmost 4 spiral corridors with atmost 4 bends. Items are packed into $\Gc$ corridor if the 4 subcorridors  $\{S_{1},S_{2},S_{3},S_{4}\}$ form a $\Gc$ corridor among themselves. Similarlary items are packed into a $\Uc$ corridor or $\Lc$ corridors or corridor with 0 bends depending upon the arrangement of corridors among themselves. During the sequence of guillotine cuts if there cut which passes through the unshared region of subcorridor perpendicular to it's orientation then it clearly divides the subcorridor into $O_{\eps}(1)$ open corridors with atmost $O_{\eps}(1)$ which is handled in Case 1. Otherwise if we don't have such cut then eventually one of the subcorridors  $\{S_{1},S_{2},S_{3},S_{4}\}$ as the items are being added to the $O(1)$ spiral corridors with atmost 4 bends. So, we are left with $O(1)$ open corridors which is again dealt in Case 1. This concludes our proof.    
\end{proof}


\begin{lem}\label{no_z}
A corridor with one or more $\Zc$ bends can be partitioned into $O_{\eps}(1)$ spiral corridors  by removing $O_{\eps,\epsl}(1)$ items, maintaining guillotine separability. 
\end{lem}
\begin{proof}
Follows from Lemma \ref{noz} and Theorem \ref{thm:ldecom}.  
\end{proof}

		
		
		\begin{figure}[t]
			\captionsetup[subfigure]{justification=centering}
			\hspace{-15pt}

				\centering
				\resizebox{!}{5cm}{
					\begin{tikzpicture}
		
					\draw[thick] (0,6) -- (0,0) -- (12,0) -- (12,10) -- (4,10) -- (4,4) -- (6,4) -- (6,8) -- ( 10,8) -- (10,2) -- (2,2) -- (2,6) -- (0,6); 
		
					\draw (1,3) node {\large \textbf{$S_{1}$}};
					\draw (6,1) node {\large \textbf{$S_{2}$}};
					\draw (11,5) node {\large \textbf{$S_{3}$}};
					\draw (8,9) node {\large \textbf{$S_{4}$}};
					\draw (5,7) node {\large \textbf{$S_{5}$}};
		
					\end{tikzpicture}}
				\caption{Corridors with more than 3 bends is not possible}
				\label{bends}

		\end{figure}
\begin{figure}[t]
			\captionsetup[subfigure]{justification=centering}
			\hspace{-15pt}

				\centering
				\resizebox{!}{5cm}{
					\begin{tikzpicture}
		
					\draw[thick](0,0) rectangle (12,12);
					\draw[thick](2,2) rectangle (10,10);
					\draw (1,6) node { \large \textbf{$S_{1}$}};
					\draw (11,6) node { \large \textbf{$S_{3}$}};
					\draw (6,1) node { \large \textbf{$S_{2}$}};	
					\draw (6,11) node { \large \textbf{$S_{4}$}};
					\end{tikzpicture}}
				\caption{Ring can be converted into corridors without any $\Zc$ bend and consisting of atmost 3 bends.}
				\label{rings}

		\end{figure}
		

\begin{cor}
Every closed corridor $C$ in corridor decomposition of guillotine separable set of items, obtained after the processing done in Theorem \ref{theorem1} and Lemma \ref{noz}, is a ring.
\end{cor}
%\begin{proof} It follows from Corollary \ref{no_z} as there exists no corridor with $\Zc$ bend.
%\end{proof}


%%%%%%%%%%%%%%%%%
\subsubsection{Obtaining corridors with at most three bends}

\begin{lem}
\label{ringlem}
Every ring $R$ obtained after the previous corridor decomposition, can be converted into $O(1)$ number of open corridors with at most 3 bends and possibly a box which is guillotine separable and the box contains a smaller ring. All items in this decomposition remain guillotine separable. 
\end{lem}
\begin{proof} Consider the guillotine cuts sequence on the knapsack. Let $P$ be the smallest subpiece such that ring $R$ lies completely inside $P$ and the next guillotine cut in $P$ is the first cut which passes through $R$.  As in Figure \ref{rings}, we call the left vertical, bottom horizontal, right vertical, top horizontal subcorridors of $R$ as $S_{1}$, $S_{2}$, $S_{3}$ and $S_{4}$ respectively. 
If any cut in $P$ cuts the smaller vertical (resp. horizontal) edges of $S_{1}$ and $S_{3}$ (resp. $S_{2}$ and $S_{4}$), then  we are done as $R$ gets divided into 2 $\Uc$-corridors.  Thus we can assume that first cut passes through a subcorridor and is parallel to its longer edges. 
We now define four types of end-to-end cuts possible in $P$ or in any of the subpieces formed by a sequence of cuts in $P$. The rightmost (resp. leftmost) end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{1}$ ($S_{3}$) is termed as Type $1$ (resp. Type $3$). The topmost (resp. bottommost) end-to-end guillotine cut during a single stage of guillotine cutting sequence passing through $S_{2}$ ($S_{4}$) is termed as Type $2$ (resp. Type $4$).  These  cuts may pass through the edges of the ring too.

The basic idea is to bound all the items of a ring to a bounding box $B$ and $O(1)$ number of open corridors with at most 3 bends such that the box is itself guillotine separable from the rest of the knapsack with guillotine cuts along the edges of $B$. We follow an iterative approach to define bounding box $B$. Clearly obtaining all four type of cuts will result in a box  bounded by these cuts which contains a smaller boundary ring. Thus our iterative algorithms halts when either ($i$) all four type of cuts are obtained, or ($ii$) when one of the subcorridors $S_{1}$, $S_{2}$, $S_{3}$, $S_{4}$ is exhausted (as previously, by exhausted we mean that there is no rectangle left in that subcorridor after a step of our iterative procedure in the new smaller subpiece),  or ($iii$) the corridor is divided into smaller open corridors by different type of cut other than the four types defined above.\\
We now formally define the iterative approach to find the bounding box. During the iterative procedure we will be adding rectangles to a 3 bend corridor $U'$(can be degenerate too) which we assume w.l.o.g.~to be coming from $S_{1},S_{2},S_{3}$, as in Figure \ref{ringproc}. That is w.l.o.g.~we assume that Type 4 cut doesn't come before other type of cuts. Considering the type of end-to-end guillotine cut in the subpiece do the following processing:
\begin{enumerate}
\item Case $1$: (Type $1$ cut) Add the items on left subpiece that are part of the ring, to the left-vertical subcorridor of the 3-bend corridor $U'$. Consider the new-subpiece to be the right-subpiece. Stop the iterative procedure if $S_{1}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new-subpiece. 
\item Case $2$: (Type $2$ cut) Add the items on bottom subpiece that are part of the ring,  to the horizontal subcorridor of $U'$. Consider the new-subpiece to be the top-subpiece. Stop the iterative procedure if $S_{2}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new-subpiece.
\item Case $3$: (Type $3$ cut) Add the items on the right subpiece that are part of the ring, to the right-vertical subcorridor of $U'$. Consider the new-subpiece to be the left-subpiece. Stop the iterative procedure if $S_{3}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new-subpiece.
\item  Case $4$: (Type $4$ cut) Pack the items of top subpiece in a new horizontal container $C$. Stop the iterative procedure. In this case we have $O(1)$ corridors and a box bounding the smaller ring whose edges are formed due to type cuts.
\item Case $5$: (Cuts perpendicular to the orientation of the subcorridors) Ring in the current subpiece is divided into 2 $\Uc$-corridors. Stop the iterative procedure.
\item Case $6$: (Cuts which don't pass through the ring) Continue only on the newly created subpiece that contains the ring,  ignore the other subpiece.
\end{enumerate}
The iterative algorithm stops in Case 5 or Case 4 or when one of the subcorridors get eventually exhausted by a type of cut. 
Each of the halting conditions results into $O(1)$ number of open corridors and possibly a box bounding a ring. 

\arir{I guess, in case 5 we get 2-$\Uc$, case 4 we get 1 $\Uc$, 1 $\Bc$ and a Box, Other cases 1 $\Uc$, 1 $\Bc$ but no box.}
%Hence we prove Lemma \ref{ringlem}.		
\end{proof}




\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				
			%box

			\draw[thick] (0,4) -- (0,0) -- (6,0) -- (6,4) --( 0,4);
			\draw[thick] (1,3)--(5,3) -- (5,1) -- (1,1) -- (1,3); 

			\draw (.5,1.5) node {\large \textbf{$S_{1}$}};
			\draw (3,1.25) node {\large \textbf{$S_{2}$}};
			\draw (5.5,2.5) node {\large \textbf{$S_{3}$}};
			\draw (2.5,3.7) node {\large \textbf{$S_{4}$}};


			\draw (1,4.7) node {\large \textbf{Type 1}};
			\draw (6.9,.45) node {\large \textbf{Type 2}};
			\draw (6,4.7) node {\large \textbf{Type 3}};
			\draw (6.9,3.2) node {\large \textbf{Type 4}};

			%\draw[solid, fill = lightgray] (0.1,0) rectangle (11.7,.5);
			%\draw[solid, fill = lightgray] (.3,.5) rectangle (11.1,1);
			%\draw[solid, fill = lightgray] (.5,1) rectangle (10.9,1.5);
			%\draw[solid, fill = lightgray] (.7,1.5) rectangle (10.5,2);

			\draw[dotted] (.5,4.5) -- ( .5,0) ;
			\draw[dotted] (.25,4.5) -- ( .25,0) ;
			
			\draw[dotted] (0,.5) -- ( 6.5,0.5) ;
			\draw[dotted] (0,.25) -- ( 6,0.25) ;
			
			
			\draw[dotted] (5.5,4.5) -- ( 5.5,0) ;
			\draw[dotted] (5.25,4) -- ( 5.25,0) ;

			\draw[dotted] (0,3.5) -- ( 6,3.5) ;
			\draw[dotted] (0,3.25) -- ( 6.5,3.25) ;
				
		
		\end{tikzpicture}}
		\caption{Types of cuts}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4.5cm}{
		\begin{tikzpicture}
				%box	
			\draw  (0,0) rectangle (8,6);
			\draw[thick] (1,5) -- (1,1) -- (7,1) -- (7,5) --(1,5);
			\draw[thick] (2,4)--(6,4)-- (6,2) -- (2,2) -- (2,4) ;
			\draw[thick]  (1.5,1.5) -- (1.5,6) ;% -- ( 6,5) -- (6,2) -- (2,2) -- (2,4) -- (1,4); 
			\draw[thick] (6.5,1.5)-- (6.5,6); 
			\draw[thick] (6.5,4.5)--(1.5,4.5);
			\draw[pattern=north east lines, pattern color=black] (6.5,4.5)--(6.5,5)--(1.5,5)--(1.5,4.5)--(6.5,4.5);
	
			\draw[pattern=north west lines, pattern color=gray] (1,5) -- (1.5,5) -- (1.5,1.5) -- (6.5,1.5) -- (6.5,5) --(7,5) -- (7,1)--(1,1)--(1,5);		

			\draw (4,1.25) node {\large \textbf{$U'$}};
			\draw (5,4.75) node {\large \textbf{$C$}};
			\draw (4,3) node {\large \textbf{$B$}};
			%\draw (1.5,2.5) node {\large \textbf{$S_{1}$}};
			%\draw (4,2.25) node {\large \textbf{$S_{2}$}};
			%\draw (6.5,3.5) node {\large \textbf{$S_{3}$}};	
							

		\end{tikzpicture}}
		\caption{Final Bounding Box of $S$}
	\end{subfigure}
	\caption{Processing 3-bend corridor}
	\label{ringproc}
\end{figure}



		\begin{thm}
		\label{3max}
		Any  corridor $C$ can be converted into $O_{\eps}(1)$ corridors of type $\Bc, \Lc, \Uc, \Gc$, maintaining guillotine separability.
		\end{thm}
		\begin{proof}W.l.o.g. assume $C$ has no $\Zc$-bends (else apply Lemma \ref{}) and more than 3 bends. There are 2 cases. 
		
\noindent {\em Case 1. } $C$ is an open corridor.  W.l.o.g~assume $C$ has 4 bends.  \ari{Similar argument holds for other corridors with greater than 4 bends.} We also assume $S_{1}$ to be longer in length than $S_{3}$ (see Figure \ref{bends}).  We follow an iterative approach to partition the corridor $C$  into $O_{\epsl}(1)$ open corridors with at most 3 bends. During the iterative procedure we will be adding rectangles to a $\Gc$-corridor $G'$ (can be degenerate too) which we assume to be coming from $S_{1},S_{2},S_{3},S_{4}$. Considering the type of end-to-end guillotine cut through the corridor $C$ do the following processing:
\begin{enumerate}
\item Case $1$: Cut passes through a subcorridor perpendicular to the orientation of that subcorridor. 
We get two corridors with smaller number of bends. If they have at most 3 bends, we stop. Otherwise, we continue iteratively with the smaller corridors.
%Portion of the corridor $C$ which isn't part of corridor $G'$ gets divided into at most 4 open corridors with at most 3 bends. Stop the iterative procedure.
\item Case $2$ : $V_{S_1}$ cut (Vertical guillotine cut through $S_{1}$). Add the items left of $V_{S_1}$ cut which are part of the corridor $C$ to the leftmost-vertical subcorridor of the 4-bend corridor $G'$.  Stop the iterative procedure if $S_{1}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise continue the iterative procedure on the remaining portion of the corridor $C$ which is not part of $G'$.
\item Case $3$ : $H_{S_2}$ cut (Horizontal guillotine cut through $S_{2}$). Add the items below $H_{S_2}$ cut to the bottommost-horizontal subcorridor of $G'$. Stop the iterative procedure if $S_{2}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise continue the iterative procedure on the remaining portion of the corridor $C$ which is not part of $G'$.
\item Case $4$ : $V_{S_3}$ cut (Vertical guillotine cut through $S_{3}$). Add the items right of $V_{S_3}$ cut  to the rightmost-vertical subcorridor of $G'$.  Stop the iterative procedure if $S_{3}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise run the algorithm iteratively on the new subpieces.
\item  Case $5$ : $H_{S_4}$ cut (Horizontal guillotine cut through $S_{4}$). Add the items above $H_{S_4}$ cut  to the topmost-horizontal subcorridor of $G'$. Stop the iterative procedure if $S_{4}$ has exhausted and in this case we have $O(1)$ corridors. Otherwise continue the iterative procedure on the remaining portion of the corridor $C$ which is not part of $G'$.
\end{enumerate}
Thus our iterative algorithms halts when one of the subcorridors $S_{1}$, $S_{2}$, $S_{3}$, $S_{4}$ is exhausted (by exhausted we mean that there is all rectangles of that subcorridor is packed in $G'$ after a step of our iterative procedure)  or when the portion of corridor $C$ which isn't part of $G'$ is divided into at most 4 open corridors with at most 3 bends as in Case 1. This iterative algorithm halts otherwise one of the type cuts will eventually exhaust a subcorridor as the number of cuts in the guillotine cutting sequence is finite. Each of the halting conditions results into $O(1)$ open corridors. 

\noindent {\em Case 2.} $C$ is a ring (see Figure \ref{rings}). Then consider the bounding box $\mathcal{B}$ (if any) which contains a smaller ring as shown in Lemma \ref{ringlem}. For the remainder of the proof by {\em freezing} a rectangle we mean that the rectangle is not moved while rearranging other rectangles. 
If there is any end to end cut which passes through only two subcorridors of same orientation then we can divide the corridor into 2 corridors each having 3 bends. So we now assume that there is no such end to end cut in $\mathcal{B}$. 
Now consider the sequence of guillotine cuts which separate the rectangles in the ring. If we are cutting through leftmost vertical subcorridor or bottom most horizontal subcorridors then we freeze these rectangles. Now in the remaining portion of the box if there is a cut $l_{1}$ through rightmost vertical subcorridor and the distance between $l_{1}$ and edge of the boundary to the right of it be $d$ then we remove the strip $S$ to the right of $l_{1}$. Then we shift the rest of items of box to the right which isn't frozen by a distance of $d$. Now in the empty region created near the left edge of the box we place the strip $S$ which we removed. Now freeze the rectangles in the strip $S$. Do the same process if there is a cut through the upper most horizontal corridor and now instead of shifting  the strip situated above the cut to the left we shift it down by appropriating shifting the remaining portion of the box upwards which isn't still frozen. Note that guillotine separability remains preserved by this rearrangement.
Continue this process till we convert these into single boundary-$\Lc$. We stop when we exhaust all rectangles or we find a cut that divides the ring into two corridors with 3 bends at most. Then we have a box with boundary-$\Lc$ and possibly 2 smaller boxes each containing corridors with at most 3 bends. This completes our proof.
\end{proof}


==> Backup/5_L_Packing.tex <==
\section{Guillotine $\lpack$}
\label{glp}
	In this section we show that given an existential guillotine separable packing of only tall and wide items we can obtain a $\lpack$ arrangement of all the items. It is worth to notice that using simple mathematical induction we can prove that every $\lpack$ arrangement is guillotine separable.
	We follow the same classification convention and definition of $\lpack$ arrangement as in section \ref{lpackingfocs}.
	
	\begin{lem}\label{lpackinglem}
	Given set $\optln$ of all tall and wide item (with height and width greater than $\frac{N}{2}$ respectively) as subsets of some feasible solution of guillotine knapsack. There exists an $\lpack$ of $\optln$ without loosing any profit into a $\Lp$ region defined by area  $\Lp$  =   ([0,N] $\times$ [0,$\height_{wide}$]) $\cup$ ([0,$\width_{tall}$] $\times$ [0,N]) where $\height_{wide}$ is the total height of all wide items and $\width_{tall}$ is the total width of all tall items.
	
	\end{lem}
	
	
	$\textit{Proof:}$ The proof follows from a constructive argument (iterative algorithm) to pack rectangles in $\optln$ into $\Lp$
	 - region defined in \ref{lpackingfocs}. Basic idea is rearranging optimal packing of items into an L-packing which consequently can be guessed in polynomial time as done in  \cite{GalvezGHI0W17}. \\
	 Let $\optln  \subseteq \opt$ be a set of guillotine separable tall and wide items. It follows from the classification \ref{lpackingfocs} each item $\R$ height and width strictly greater than $\frac{N}{2}$. Consider the guillotine cut sequence of the original arrangement of $\optln$. Every horizontal (resp. vertical) cut divides the $N\times N$ knapsack plane $P$ into two sub-planes. The sub-planes are of same width (reps.height) but heights (resp. vertical) smaller than the original plane, we annotate the sub-planes as $P_{h1}$ and $P_{h1}$ (resp.  $P_{w1}$ and $P_{w2}$). The nomenclature is such that $P_{h1}$ (resp. $P_{w1}$) is smaller (consider any if both are equal) among the two horizontal sub-planes $P_{h1}$ and $P_{h2} $(resp. $P_{w1}$ and $P_{w2}$) . We can claim that every $P_{h1}$ (resp. $P_{w1}$) consists of only wide (resp. tall) rectangles. [ The proof follows from the fact that width (resp. height) of horizontal (resp. vertical) is strictly greater than $\frac{N}{2}$ ]. For the proof we use some basic rearrangement techniques which maintain the guillotine separability of the given configuration of items : 
	\begin{enumerate}
	\item Compression
	\\We define compression as a process of reordering the set of items in planes obtained after a guillotine cut (either horizontal or vertical).
	 The horizontal (resp. vertical items) are piled such that they share a common vertical (resp. horizontal) edge .
	\item Sorting
	\\Given a set of compressed items, i.e, horizontal items(resp. vertical items) sharing a common vertical (resp. horizontal) edge . For sorting the rearrangement follows as below:
	\begin{itemize}
	\item Decreasing height from left to right with every item having topmost edge at the same horizontal level  : In case of vertical items.
	\item Decreasing width from bottom to top with every item having rightmost edge at same vertical level :  In case of horizontal items.
	\end{itemize}
	
	\item Plane Flipping 
	\\ Given two planes $P_{h1}$ and $P_{h1}$ (resp.  $P_{w1}$ and $P_{w2}$), we change relative configuration of the two planes with respect to horizontal (resp. vertical) orientation i.e bring the top plane to bottom and bottom plane to top (resp. right plane to left and left plane to right).
	
	
	\end{enumerate}
	
	\begin{lem}
	\label{arr_techniques}
	Resulting arrangement using techniques of Compression  and flipping follows guillotine separability globally as well as locally if items inside the plane being processed are only horizontal or vertical. In other words the resulting plane following the given rearrangement techniques is guillotine separable  from the rest of the knapsack (global separability) with the same number of guillotine cuts as required to separate the original plane before arrangement. Also each item inside the plane is also guillotine separable (local separability) with the same number of guillotine cuts as inside original plane.
	\end{lem}
	
	\begin{cor}
	\label{cor_arr}
	It follows immediately from Lemma \ref{arr_techniques} we can always consider that in a horizontal (resp. vertical) cut, the bottom (resp. left) sub-plane is the shorter one among the two resulting sub-planes [if it is not we can use flipping  and rearrange the relative configuration of two planes, making them follow the given property] .
	\end{cor}
	
	\begin{cor}
	It follows  from Lemma \ref{arr_techniques} that compression of a sub-plane results in a sub-plane smaller in width (or height) if every item inside is vertical (resp. horizontal).
	\end{cor}
	
	We now define the main rearrangement algorithm to form the $\lpack$ from given initial optimal packing. Consider the sequence of guillotine cuts of optimal configuration and rearrange as follows:
	\begin{itemize}
	\item Case: Horizontal cut : From Corollary  \ref{cor_arr} we can claim that out of the two sub-planes $P_{h1}$ and $P_{h2}$ obtained from the cut, $P_{h1}$ i.e. the bottom sub-plane is shorter. It is clear that $P_{h1}$ contains only horizontal items [ height of $P_{h1}$ is smaller than $\frac{N}{2}$ since it is the smaller sub-plane ]. We then use compression on sub-plane $P_{h1}$.  The rearranged $P_{h1}$ shares bottom edge with the horizontal leg of L obtained so far (except the first one which shares bottom-edge with bottom boundary of knapsack ).  We merge $P_{h1}$ into the horizontal leg of L and apply compression on the leg.
	\item Case: Vertical cut : Following similar process as done in previous case. From corollary \ref{cor_arr} we can claim that out of the two sub-planes $P_{w1}$ and $P_{w2}$ obtained from the cut, $P_{w1}$ i.e. the left sub-plane is shorter. It is clear that $P_{w1}$ contains only vertical items [ width of $P_{w1}$ is smaller than $\frac{N}{2}$ since it is the smaller sub-plane ]. We then use compression on sub-plane $P_{w1}$. The rearranged $P_{w1}$ shares left edge with the vertical leg of L obtained so far(except the first one which shares left-edge with left boundary of knapsack). We merge $P_{w1}$ into the vertical leg of L and apply compression on the leg.
	\end{itemize}
	Following the same flipping and compression procedures we constructively form the $\Lp$ - shaped region from $\optln$ following properties as defined in Lemma \ref{lpackinglem}.
	
	%\begin{figure}[!htb]
	%\centering
	%\includegraphics[scale=.75]{lpack}
	%\caption{An illustration of $\lpack$. Here we are doing compression after every stage. Flipping the red and yellow planes to bring smaller %plane to the horizontal leg of $\Lp$}
	%\label{$\lpack$}
	%\end{figure}
	
	\begin{figure}[!tbh]
		%\centering
		\captionsetup[subfigure]{justification=centering}
		\hspace{-10pt}
		\begin{subfigure}[t]{.25\textwidth}
			\centering
			\resizebox{!}{3.5cm}{
			\begin{tikzpicture}\node[rotate = 90, yscale  =-1] at (0,0){\begin{tikzpicture}
				%box			
				\draw[thick] (0,0) rectangle (70,70);
				% items
				\draw[solid, fill = lightgray] (2.4,4.2) rectangle (5.5,55.7);
				\draw[solid, fill = lightgray] (7.4,15) rectangle (8.2,61.7);
				\draw[solid, fill = lightgray] (12.4,5) rectangle (14.5,24.5);
				\draw[solid, fill = lightgray] (18.3,15.8) rectangle (26.6,44.1);
				\draw[solid, fill = lightgray] (28.3, .2) rectangle (28.31,70);
				\draw[dashed] (28.3,0) -- ( 28.3, 70);
				\draw[solid, fill = lightgray] (31.6,2.7) rectangle (33.3,40.2);
				\draw[solid, fill = lightgray] (35.8,6.9) rectangle (37.88,24.4);
				\draw[solid, fill = lightgray] (40.8,5.2) rectangle (69.2,6.9);
				\draw[solid, fill = lightgray] (39.9,14.4) rectangle (66.6,16.9);
				\draw[solid, fill = lightgray] (58.5,18.7) rectangle (61.4,32.7);
				\draw[solid, fill = lightgray] (39.5,35.8) rectangle (68.7,38.3);
				\draw[solid, fill = lightgray] (31.6,44.4) rectangle (69.1,46.9);
				\draw[solid, fill = lightgray] (38,49.4) rectangle (66.3,51.1);
				\draw[solid, fill = lightgray] (28.4,53.5) rectangle (55.9,58.1);
				\draw[solid, fill = lightgray] (33.3,60.2) rectangle (50,61.9);
	
				%\draw (50, 72) node {\large \textbf{$1$}};
			\end{tikzpicture}};\end{tikzpicture}}
		\caption{Horizontal cut separating horizontal only items on bottom sub-plane.}
		\label{fig a}
		\end{subfigure}
		\begin{subfigure}[t]{.25\textwidth}
			\centering
			\resizebox{!}{3.5cm}{
			\begin{tikzpicture}\node[rotate = 90, yscale  =-1] at (0,0){\begin{tikzpicture}
				%box			
				\draw[thick] (0,0) rectangle (70,70);
				% items
				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
				\draw[solid, fill = lightgray] (4.1,50) rectangle (6.6,70);
				\draw[solid, fill = lightgray] (6.6,41.7) rectangle (14.9,70);
				\draw[dotted] (15,0) -- (15,70);
				%first guillotine cut
				\draw[solid, fill = lightgray] (31.6,2.7) rectangle (33.3,40.2);
				\draw[solid, fill = lightgray] (35.8,6.9) rectangle (37.88,24.4);
				\draw[solid, fill = lightgray] (40.8,5.2) rectangle (69.2,6.9);
				\draw[solid, fill = lightgray] (39.9,14.4) rectangle (66.6,16.9);
				\draw[solid, fill = lightgray] (58.5,18.7) rectangle (61.4,32.7);
				\draw[solid, fill = lightgray] (39.5,35.8) rectangle (68.7,38.3);
				\draw[dotted] (15, 42) -- ( 70, 42);
				\draw[solid, fill = lightgray] (31.6,44.4) rectangle (69.1,46.9);
				\draw[solid, fill = lightgray] (38,49.4) rectangle (66.3,51.1);
				\draw[solid, fill = lightgray] (28.4,53.5) rectangle (55.9,58.1);
				\draw[solid, fill = lightgray] (33.3,60.2) rectangle (50,61.9);
			\end{tikzpicture}};\end{tikzpicture}}
			\caption{Compression of items on bottom subplane}
			\label{fig b}
		\end{subfigure}
		\begin{subfigure}[t]{.25\textwidth}
			\centering
			\resizebox{!}{3.5cm}{
			\begin{tikzpicture}\node[rotate = 90, yscale = -1] at (0,0){\begin{tikzpicture}
				%box			
				\draw[thick] (0,0) rectangle (70,70);
				% items
				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
				\draw[solid, fill = lightgray] (4.1,41.7) rectangle (12.4,70);
				\draw[solid, fill = lightgray] (12.4,50) rectangle (14.9,70);
				\draw[solid, fill = lightgray] (14.9,0) rectangle (15,70);
				%first guillotine cut
				\draw[solid, fill = lightgray] (31.6,2.7) rectangle (33.3,40.2);
				\draw[solid, fill = lightgray] (35.8,6.9) rectangle (37.88,24.4);
				\draw[solid, fill = lightgray] (40.8,5.2) rectangle (69.2,6.9);
				\draw[solid, fill = lightgray] (39.9,14.4) rectangle (66.6,16.9);
				\draw[solid, fill = lightgray] (58.5,18.7) rectangle (61.4,32.7);
				\draw[solid, fill = lightgray] (39.5,35.8) rectangle (68.7,38.3);
				% second cut
				\draw[solid, fill = lightgray] (22.5,67.5) rectangle (70,70);
				\draw[solid, fill = lightgray] (41.7,65.8) rectangle (70,67.5);
				\draw[solid, fill = lightgray] (42.5,61.4) rectangle (70,65.8);
				\draw[solid, fill = lightgray] (43.3,59.5) rectangle (70,61.4);
				\draw[solid, fill = lightgray] (15,59.4) rectangle (70,59.5);
			\end{tikzpicture}};\end{tikzpicture}}
			\caption{Vertical cut compressing and sorting rectangles in left subplane}
			\label{fig c}
		\end{subfigure}
		\begin{subfigure}[t]{.25\textwidth}
			\centering
			\resizebox{!}{3.5cm}{
			\begin{tikzpicture}\node[rotate = 90, yscale  =-1] at (0,0){\begin{tikzpicture}
				%box			
				\draw[thick] (0,0) rectangle (70,70);
				% items
				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
				\draw[solid, fill = lightgray] (4.1,41.7) rectangle (12.4,70);
				\draw[solid, fill = lightgray] (12.4,50) rectangle (14.9,70);
				\draw[solid, fill = lightgray] (14.9,0) rectangle (15,70);
				%first guillotine cut
				\draw[solid, fill = lightgray] (31.6,13.3) rectangle (33.3,50.8);
				\draw[solid, fill = lightgray] (35.8,17.5) rectangle (37.88,35);
				
				\draw[dashed] (39,10.6) -- (39,70);
				\draw[solid, fill = lightgray] (40.8,15.8) rectangle (69.2,17.5);
				\draw[solid, fill = lightgray] (39.9,25) rectangle (66.6,27.5);
				\draw[solid, fill = lightgray] (58.5,29.3) rectangle (61.4,43.3);
				\draw[solid, fill = lightgray] (39.5,46.4) rectangle (68.7,48.9);
				% second cut
				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
				\draw[solid, fill = lightgray] (41.7,2.5) rectangle (70,4.2);
				\draw[solid, fill = lightgray] (42.5,4.2) rectangle (70,8.8);
				\draw[solid, fill = lightgray] (43.3,8.8) rectangle (70,10.5);
				\draw[solid, fill = lightgray] (15,10.5) rectangle ( 70, 10.6);
			\end{tikzpicture}};\end{tikzpicture}}
			\caption{Flipping to form vertical leg of L, followed by compression and sorting to form Horizontal leg of L-structure}
			\label{fig d}
		\end{subfigure} 
		%\hspace{-20pt}
		\begin{subfigure}[t]{.25\textwidth}
			\centering
			\resizebox{!}{3.5cm}{
			\begin{tikzpicture}\node[rotate = 90 ,yscale = -1] at (0,0){\begin{tikzpicture}
				%box			
				\draw[thick] (0,0) rectangle (70,70);
				% items
				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
				\draw[solid, fill = lightgray] (4.1,32.5) rectangle (5.8,70);
				\draw[solid, fill = lightgray] (5.8,41.7) rectangle (14.1,70);
				\draw[solid, fill = lightgray] (14.1,50) rectangle (16.6,70);
				\draw[solid, fill = lightgray] (16.6,52.5) rectangle (19.4,70);
				\draw[dotted] (19.5,0) -- (19.5,70);
				
				%first guillotine cut
				
				
				%third cut
				
				\draw[solid, fill = lightgray] (40.8,15.8) rectangle (69.2,17.5);
				\draw[solid, fill = lightgray] (39.9,25) rectangle (66.6,27.5);
				\draw[dashed] (19.5, 28) -- ( 70, 28);
				\draw[solid, fill = lightgray] (58.5,29.3) rectangle (61.4,43.3);
				\draw[solid, fill = lightgray] (39.5,46.4) rectangle (68.7,48.9);
				% second cut
				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
				\draw[solid, fill = lightgray] (41.7,2.5) rectangle (70,4.2);
				\draw[solid, fill = lightgray] (42.5,4.2) rectangle (70,8.8);
				\draw[solid, fill = lightgray] (43.3,8.8) rectangle (70,10.5);
				\draw[solid, fill = lightgray] (19.5,10.5) rectangle ( 70, 10.6);
			\end{tikzpicture}};\end{tikzpicture}}
			\caption{Compression of items obtained by horizontal cut and sorting all items of horizontal leg of L-structure}
		\end{subfigure}	
		\begin{subfigure}[t]{.25\textwidth}
			\centering
			\resizebox{!}{3.5cm}{
			\begin{tikzpicture}\node[rotate = 90, yscale = -1] at (0,0){\begin{tikzpicture}
				%box
				
				\draw[thick] (0,0) rectangle (70,70);
				% items
				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
				\draw[solid, fill = lightgray] (4.1,32.5) rectangle (5.8,70);
				\draw[solid, fill = lightgray] (5.8,41.7) rectangle (14.1,70);
				\draw[solid, fill = lightgray] (14.1,50) rectangle (16.6,70);
				\draw[solid, fill = lightgray] (16.6,52.5) rectangle (19.4,70);
				\draw[dotted] (19.5,0) -- (19.5,70);
				
				%first guillotine cut
				
				
				%third cut
				\draw[solid, fill = lightgray] (58.5,29.3) rectangle (61.4,43.3);
				\draw[dotted] (19.5,45) -- (70,45);
				\draw[solid, fill = lightgray] (39.5,46.4) rectangle (68.7,48.9);
				% second cut
				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
				\draw[solid, fill = lightgray] (40.8,2.5) rectangle (70,4.2);
				\draw[solid, fill = lightgray] (41.7,4.2) rectangle (70,5.9);
				\draw[solid, fill = lightgray] (42.5,5.9) rectangle (70,10.5);
				\draw[solid, fill = lightgray] (43.3,10.5) rectangle (70,12.2);
				\draw[solid, fill = lightgray] (43.3,12.2) rectangle (70,14.7);
				\draw[dotted] (19.5,14.7) -- ( 70, 14.7);
			\end{tikzpicture}};\end{tikzpicture}}
			\caption{Compression of items obtained by vertical cut followed by sorting all items of vertical leg of L-structure}
			\label{fig f}
		\end{subfigure}
		%\hspace{5cm}
		\begin{subfigure}[t]{.25\textwidth}
			\centering
			\resizebox{!}{3.5cm}{
			\begin{tikzpicture}\node[rotate = 90, yscale = -1] at (0,0){\begin{tikzpicture}
				%box
				
				\draw[thick] (0,0) rectangle (70,70);
				% items
				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
				\draw[solid, fill = lightgray] (4.1,32.5) rectangle (5.8,70);
				\draw[solid, fill = lightgray] (5.8,41.7) rectangle (14.1,70);
				\draw[solid, fill = lightgray] (14.1,50) rectangle (16.6,70);
				\draw[solid, fill = lightgray] (16.6,52.5) rectangle (19.4,70);
				\draw[dotted] (19.5,0) -- (19.5,70);
				
				%first guillotine cut
				
				
				%third cut
				\draw[solid, fill = lightgray] (58.5,29.3) rectangle (61.4,43.3);
				\draw[dotted] (19.5,45) -- (70,45);
				
				% second cut
				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
				\draw[solid, fill = lightgray] (40.8,2.5) rectangle (70,5);
				\draw[solid, fill = lightgray] (40.8,5) rectangle (70,6.7);
				\draw[solid, fill = lightgray] (41.7,6.7) rectangle (70,8.4);
				\draw[solid, fill = lightgray] (42.5,8.4) rectangle (70,12.7);
				\draw[solid, fill = lightgray] (43.3,12.7) rectangle (70,14.7);
				\draw[solid, fill = lightgray] (43.3,14.7) rectangle (70,17.2);
				\draw[dotted] (19.5,17.2) -- ( 70, 17.2);
			\end{tikzpicture}};\end{tikzpicture}}
			\caption{Compression of items obtained by vertical cut followed by sorting all items of vertical leg of L-structure}
			\label{fig g}
		\end{subfigure}
		\begin{subfigure}[t]{.23\textwidth}
			\centering
			\resizebox{!}{3.5cm}{
			\begin{tikzpicture}\node[rotate = 90, yscale = -1] at (0,0){\begin{tikzpicture}
				%box
				
				\draw[thick] (0,0) rectangle (70,70);
				% items
				\draw[solid, fill = lightgray] (0,16.7) rectangle (3.3,70);
				\draw[solid, fill = lightgray] (3.3,23.3) rectangle (4.1,70);
				\draw[solid, fill = lightgray] (4.1,32.5) rectangle (5.8,70);
				\draw[solid, fill = lightgray] (5.8,41.7) rectangle (14.1,70);
				\draw[solid, fill = lightgray] (14.1,50) rectangle (16.6,70);
				\draw[solid, fill = lightgray] (16.6,52.5) rectangle (19.4,70);
				\draw[solid, fill = lightgray] (19.4,56) rectangle (22.3,70);
				\draw[dotted] (22.3,0) -- (22.3,70);
				
				%first guillotine cut
				
				
				%third cut
				
				
				% second cut
				\draw[solid, fill = lightgray] (22.5,0) rectangle (70,2.5);
				\draw[solid, fill = lightgray] (40.8,2.5) rectangle (70,5);
				\draw[solid, fill = lightgray] (40.8,5) rectangle (70,6.7);
				\draw[solid, fill = lightgray] (41.7,6.7) rectangle (70,8.4);
				\draw[solid, fill = lightgray] (42.5,8.4) rectangle (70,12.7);
				\draw[solid, fill = lightgray] (43.3,12.7) rectangle (70,14.7);
				\draw[solid, fill = lightgray] (43.3,14.7) rectangle (70,17.2);
				\draw[dotted] (22.3,17.2) -- ( 70, 17.2);
			\end{tikzpicture}};\end{tikzpicture}}
			\caption{Compression of item obtained by horizontal cut followed by sorting all items of horizontal leg of L-structure}
			\label{fig h}
		\end{subfigure}
		\caption{Step wise construction of L from guillotine separable optimal packing. }
%(a) Compression of item obtained by horizontal cut followed by sorting all items of horizontal leg of L-structure. (b)Compression of items obtained by vertical cut followed by sorting all items of vertical leg of L-structure. (c) Compression of items obtained by vertical cut followed by sorting all items of vertical leg of L-structure. (d) Compression of items obtained by horizontal cut and sorting all items of horizontal leg of L-structure. (e) Flipping to form vertical leg of L, followed by compression and sorting to form Horizontal leg of L-structure. (f) Vertical cut compressing and sorting rectangles in left subplane. (g) Compression of items on bottom subplane. (h) Horizontal cut separating horizontal only items on bottom sub-plane.}
		\label{$\lpack$}
	\end{figure}
	
	\begin{lem}
	Given a set of items $\R$, there is a PTAS for L-packing with profit $(1-O(\eps))\profit(\optln)$, where $\optln$ is the profit of long items in optimal packing.
	\end{lem}
	\textit{Proof: }
	Using the Lemma \ref{lpackinglem} of our paper and PTAS for L-packing from \cite{GalvezGHI0W17} on the input set $\R$ of all long items $\R_{long}$ (with width or height $\> \frac{N}{2}$),we get the packing (in polynomial time) with profit $(1-O(\eps))\profit(\optln)$ for 2-D guillotine knapsack case.
	

==> Backup/5_Non_Rotated_Cardinality.tex <==

%%%%%%%%%%%%%%%% Main Algorithm %%%%%%%%%%%%%%%

\section{$(\frac{4}{3}+\eps)$-approximation \tggkc}
%\subsection{Item Classification}
%For two given constants $1\geq\epsl\geq\epss$ we classify item i as:
%\begin{itemize}
%\item $small$ if $\width_{i}\leq\epss$ and $\height{i}\leq\epss$;
%\item $horizontal$ if $\height_{i}\leq\epss$ and $\width_{i}>\epsl$;
%\item $vertical$ if $\width_{i}\leq\epss$ and $\height_{i}>\epsl$;
%\item $large$ if $\width_{i}>\epsl$ and $\height{i}>\epsl$;
%\item $intermediate$ otherwise.
%\end{itemize}
%\begin{lem}\cite{GalvezGHI0W17}\label{class}
%Let $\eps >0$ and let $f(.)$ be any positive increasing function such that $f(x)<x$ for all x between 0 and 1. Then, there exist positive constant values $\epsl,\epss \in \Omega_{\eps}(1)$, with $f(\eps)\geq\epsl$ and $f(\epsl)\geq\epss$ such that the total profit of intermediate rectangles is bounded by $\eps \profit(\opt)$. The pair ($\epsl,\epss$) is one pair from a set of $O_{\eps}(1)$  pairs and this set can be computed in polynomial time.
%\end{lem}

For \tggkc, due to the following lemma we will assume that remove $O(1)$ number of items, without loosing too much profit.

\begin{lem}\cite{adamaszek2015knapsack} 
\label{lem:drop}
If there is an algorithm for \tgkc~which outputs a solution with at least $(1-\eps)\opt-\beta^{O_\eps(1)}$ items in time $O(f(n))$,
then there is also a $(1+\eps)$-approximation algorithm with running time $O(f(n)+n^{{\beta}^{O_\eps(1)}})$.
\end{lem}

Thus for \tggkc, large items can dropped as there are at most $O(\frac{1}{\epsl^{2}})$ large rectangles in any given packing. 
In fact, for now we assume that there is only skewed items in the packing. At the end of the section, we show how to repack the small items. 

\subsection{Processing of subcorridors from $\Bc\Lc$-decomposition}
From Lemma \ref{structure}, we obtain O(1) number of corridors of type $\Bc$ or $\Lc$, where they are in a boundary-$\Lc$ of a guillotine separable box as obtained. Now we process the $\Lc$-corridors in 2 different ways (see Figure \ref{process} for processing of corridors). As they are part of boundry-$\Lc$ of a guillotine separable box, the processing preserves guillotine separability. 
In first way, we process the vertical subcorridors as done in subsection \ref{prosec}. In second way, we process the horizontal subcorridors. Each of these different processing gives different sets $\optth$, $\optki$ and $\optfa^{corr}$. Based on these sets we classify the rectangles as follows:
\begin{itemize}
\item $\opt_{T}$ is the set of items which are in $\optth$ in one of the case.
\item $\opt_{K}$ is the set of items which are in $\optki$ in one of the case.
\item $\opt_{F}$ is the set of items which are in $\optfa^{corr}$ in both cases.
\end{itemize}
\begin{lem}\cite{GalvezGHI0W17}
\label{ering}
If we take any one of the cases of processing the following properties hold:
\begin{enumerate}
\item $|OPT_{kill}|=O_{\eps,\epsl,\epsb}(1)$;
\item For any given constant $\epsr>0$ there is a sufficiently small $\epsb>0$ such that the total height(resp.,width)of items in $\optth\cap\Rho$ (resp. $\optth\cap\Rve$) is at most $\epsr N$.
\end{enumerate}
\end{lem}

Now we classify items in the optimal packing into four sets: $\opt_{LT}, \opt_{ST}$ (long and short items in $\opt_T$, resp.),  $\opt_{LF}, \opt_{SF}$ (long and short items in $\opt_F$, resp.). 	

%\subsection{Profitable Structure Packing}\label{profitstruc}
%\begin{lem}\cite{GalvezGHI0W17}\label{sumprofit}
%$\profit(\opt_{F}\cap\opt_{T})+\profit(\opt_{k})+\profit(\opt_{large})+\profit(\opt_{corr}^{cross})\geq(1-O(\eps))\profit(\opt)$.
%\end{lem}

\begin{lem}
\label{algo1}
$\profit(\opt_{L\&C})\geq\profit(\opt_{F})+\profit(\opt_{T})/2$.
\end{lem}
\begin{proof} Consider the sum of profit in both the ways of processing a subcorridor of $\Lc$-corridor as mentioned above. By definition every item in $\opt_{F}$ is included in both the cases. Items belonging to $\opt_{T}$ is saved in at least one of the cases. The lemma follows as a result of averaging argument.
\end{proof}

Now we show a more involved $L\&C$-packing that packs almost $|T|+|F|/2$ items.
\begin{lem}
\label{algo2}
$\profit(\opt_{L\&C})\geq\profit(\opt_{T})+(1-O_{\eps}(1))\profit(\opt_{F})/2$.
\end{lem}
\begin{proof}
Let $w_L N$ (resp. $w_{LT} N$) be the total width of vertical items in $\optln$ (resp. $\opt_{LT}$) and 
$h_L N$ (resp. $h_{LT} N$) be the total height of horizontal items in $\optln$ (resp. $\opt_{LT}$).
Then  $w_L, h_L \le 1$, $w_{LT},h_{LT}   \le \epsr$, and  all long items can be packed in a boundary-$\Lc$ of width $w_L N$ and height $h_L N$.  
Now from vertical arm of  boundary-$\Lc$, we
choose  a random vertical strip $[\tilde{x}, \tilde{x}+\frac{w_L N}{2}+w_{LT} N] \times [0,N]$ (if $\tilde{x}+\frac{w_L}{2} N+w_{LT} N\le w_L N$) or two random strips $([\tilde{x}, w_L N]  \times [0,N]) \cup ([0, \tilde{x}+\frac{w_L N}{2}+w_{LT} N -w_L N] \times [0,N]$ (if $\tilde{x}+\frac{w_L N}{2}+w_{LT} N> w_L N$), where $\tilde{x}$ is chosen uniformly at random from $[w_L]$. We remove all short items intersecting with this strip.
We do similar operation on horizontal arm and remove all short items intersecting random horizontal strip(s) of total width $\frac{h_L}{2} N+h_{LT} N$. 
By averaging argument, the remaining items have profit $\frac{(1-O_{\epsl, \epsr}(1))}{2}\cdot \opt_{LF}+ST$ and packed in boundary-$\Lc$ of width $\le w_L/2$ and height $\le h_L/2$.
In the remaining rectangular region of the box, we will place containers. 
W.l.o.g. assume $w_L \le h_L$ (the other case is analogous). 
Now we place items in $\opt_{ST}$ in two containers next to boundary-$\Lc$.
First, we place a container of height 1/2 and width $\epsr$, touching top boundary and $x= w_L N/2$,  containing items in $\opt_{ST}$  coming from vertical subcorridors in the processing and then we place a container of width 1/2 and height $\epsr$, touching right  boundary and $y=h_L N/2$, containing items in $\opt_{ST}$  coming from horizontal  subcorridors in the processing.
As $w_L\le 1/2$, i.e., $1-w_L/2\ge 3/4$,  these two containers do not overlap. 
Now we are left with a rectangular region of width  $N(1-\frac{w_L}{2}-O_{\epsr}(1))$ and height $N(1-\frac{h_L}{2}-O_{\epsr}(1))$.
So, using Steinberg's algorithm \cite{??} (which is a guillotine packing, see Section \ref{??}), we can pack any subset of items  in $\opt_{SF}$ of total area at most 
$\Big((1-\frac{w_L}{2}-O_{\epsr}(1))(1-\frac{h_L}{2}-O_{\epsr}(1))-(\frac{w_L}{2}+O_{\epsr}(1))(\frac{h_L}{2}+O_{\epsr}(1))\Big)N^2/2 \le \frac{N^2}{2}(1-\frac{(w_L+h_L)}{2}-O_{\epsr}(1))$.
On the other hand, the total area of rectangles in $\opt_{SF}$ is at most $N^2(1-\frac{w_L+h_L}{2}-O_{\epsr}(1))$.
So, consider rectangles in $\opt_{SF}$ in nondecreasing order of area till they reach $N^2(1-\frac{(w_L+h_L)}{2}-O_{\epsr}(1))$.
These items can be packed in the remaining region and have total profit $\ge  \profit(\opt_{SF}) \Big(\frac{N^2}{2}(1-\frac{w_L+h_L}{2}-O_{\epsr}(1))\Big) / \Big(N^2(1-\frac{w_L+h_L}{2}-O_{\epsr}(1))\Big) \ge ( \profit{\opt_{SF}} (1-O_{\epsr}(1))/2$.
Thus we have $L\&C$-packing with profit  $\profit(\opt_{LT})+\profit(\opt_{ST})+\profit(\opt_{LF}) \cdot  \frac{(1-O_{\epsr}(1))}{2}+\profit(\opt_{SF}) \cdot \frac{(1-O_{\epsr}(1))}{2}$, concluding our proof.
%of width $\frac{w_L}{2}+w_{LT}$, choosing the starting x- starting at $x = \tilde\in [w_L N]$ and ending at 
\end{proof}

From Lemma \ref{algo1} and \ref{algo2}, we get $\profit(OPT_{L\&C})\geq(\frac{3}{4}-O(\eps))\profit(\opt)$.
The worst case is obtained when $\profit(\opt_{T})=\profit(\opt_{F})$.
\begin{thm}
\label{LC}
Let $OPT_{L\&C}$ be the most profitable solution that is packed by a guillotine separable $L\&C$ packing and $\opt$ be optimal  packing for \tggkc. Then $\profit(OPT_{L\&C})\geq(\frac{3}{4}-O(\eps))\profit(\opt)$.
\end{thm}

\subsubsection {Previous part, might be removed if above is true.}
\begin{lem}
\label{algo2}
$\profit(\opt_{L\&C})\geq\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{SF})$.
\end{lem}
\begin{proof}
From the optimal packing we remove all the items except the items in $\opt_{SF}$. Now in this new packing consider a horizontal (resp., vertical) random strip of height (resp., width) $3\eps N$. Remove the items which overlap with these vertical and horizontal strips. Let the items which remain be $\opt_{SF}'$. Due to horizontal strip, a horizontal item gets removed with probability at most $7\eps$ and a vertical item gets removed with probability at most $\frac{1}{2}+6\eps$. Similarly, due to vertical strip, a vertical item gets removed with probability at most $7\eps$ and a horizontal item gets removed with probability at most $\frac{1}{2}+6\eps$. From linearity of expectation we get that $\profit(\opt_{SF}' )\geq (\frac{1}{2}-13\eps)\profit(\opt_{SF})$. \\
\\Also clearly $\opt_{SF}'$ can be packed in a square of side length $(1-3\eps)N$. So by doing one sided resource augmentation we can get a packing with profit $(1-O(\eps))\profit(\opt_{SF}')$ in a square with side length $(1-2\eps)N$. In $N \times N$ knapsack we can pack all items in $\opt_{LT}$ in a boundary-$\Lc$ with width $\epsr N$. Two containers of dimensions $\epsr N \times \frac{N}{2}$ and $\frac{N}{2} \times \epsr N$ are created and kept just beside the subcorridors of boundary-$\Lc$ in such a way that the 2 created subcorridors don't overlap with each other. We pack all the items in $\opt_{ST}$ in these two containers. In the remaining square region which doesn't have items from $\opt_{T}$ we can pack the items from $\opt_{SF'}$ with profit $(1-O(\eps))\profit(\opt_{SF}')$ as the square region has side length at least $(1-2\eps)N$. This concludes the proof of this Lemma. 
\end{proof}

\begin{lem}
\label{idea}
$\profit(\opt_{L\&C})\geq\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{LF})$.
\end{lem}
\begin{proof}


%\begin{figure}[t]
%\centering
%\includegraphics[scale=1]{pic7}
%\caption{Case1}
%\label{prop1}
%\end{figure}
\begin{figure}[t]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\resizebox{!}{3cm}{
		\begin{tikzpicture}
		
				%box
			\draw [thick] (0,0) rectangle ( 20,20);
			\draw[solid , fill = lightgray] (0,0) -- (20,0) -- ( 20,16) -- ( 6,16) -- ( 6, 20) -- ( 0, 20) -- ( 0,0) ;


			\draw[solid, fill = darkgray] (9,7) rectangle (20,9);
			\draw[solid, fill = lightgray] (22,8) rectangle (26,8.5);
		\end{tikzpicture}}
		\caption{case1}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\resizebox{!}{3cm}{
		\begin{tikzpicture}
			\draw[thick] (0,0) rectangle (20,20);
			\draw[solid , fill = lightgray] (0,0) -- ( 20,0) -- ( 20, 12) -- ( 4, 12) -- ( 4,20 ) -- ( 0 , 20 ) -- ( 0,0) ;
			\draw ( 0, 10 ) -- ( 20 , 10) ;
			\draw ( 1, 0) -- ( 1, 6) -- ( 2, 6) -- ( 2, 8 ) -- ( 4, 8) -- ( 4, 12) ;
		\end{tikzpicture}}
		\caption{case2}
	\end{subfigure}
	\begin{subfigure}[b]{.3\textwidth}
		\centering
		\resizebox{!}{3cm}{
		\begin{tikzpicture}
			\draw[thick] (0,0) rectangle (20,20);
			\draw[solid , fill = lightgray] (0,0) -- ( 20,0) -- ( 20, 10) -- ( 4, 10) -- ( 4,20 ) -- ( 0 , 20 ) -- ( 0,0) ;
			\draw[solid , fill = darkgray] ( 5, 11 ) rectangle ( 6 , 19) ;
			\draw[solid , fill = darkgray] ( 7, 10.5 ) rectangle ( 19 , 12) ;

		\end{tikzpicture}}
		\caption{case2}
		\label{case2}
	\end{subfigure}
	%\caption{Different types of subcorridors.Subcorridor as shown in (c) is not possible as z bend doesn't occur as shown in Theorem \ref{theorem1}}
	%\label{subcorridor}
	\caption{}\label{prop1}
\end{figure}

$Case$ $1$: In this case, total width of items in $\optve \cap \R_{long}$ is greater than or equal to $(\frac{1}{2}+\epsr)N$ and less than $\frac{N}{2}$ and total height of  items in $\optho \cap \R_{long}$ is more than $\frac{N}{2}$. Since we have excluded large items in this section, the L packing of long items doesn't have large items. Now by averaging argument we can identify a strip of height $\eps N$ and loose profit of at most $O(\eps)\profit(\opt_{LF})$  in the L-packing by removing only the items of $\opt_{LF} \cap \Rho$ which overlaps with this strip. If there are any items of $\opt_{LT}$ in the strip then we push it down. In the remaining space we indentify a rectangular region which is doesn't cross the boundary curve (as shown in Figure \ref{prop1}(a)) to pack all the items in $\opt_{ST} \cap \Rho$ on top of each other. In a simlar fashion we can pack all the rectangles in $\opt_{ST} \cap \Rve$
\\
\\$Case$ $2$: In this case, total width of items in $\optve \cap \R_{long}$ is less than $(\frac{1}{2}-\epsr)N$ and total height of items in $\optho \cap \R_{long}$ is more than $\frac{N}{2}$. We now cannot pack the items of $\opt_{ST} \cap \Rve$ in a vertical strip of width $\eps N$ in the vertical subcorridor as the strip may contain huge profit irrespective of the way it is being chosen. Now consider a horizontal line $l$ at the height of $\frac{N}{2}$ in the knapsack. Let the rectangles in $\optho \cap \R_{long}$ above $l$ be $\R_{1}$ and the rectangles below $l$ be $\R_{2}$. Now, if $\profit(\opt_{LF}) \cap \R_{2} > \profit(\opt_{LF}) \cap \R_{1}$  then we remove the items in $\R_{1}$ and pack the items of $\opt_{LT} \cap \R_{1}$  by removing the least profitable strip of height $\eps N$ of $\R_{2}$ in the similar way as done in Case 1. Otherwise if $\profit(\opt_{LF}) \cap \R_{1} > \profit(\opt_{LF}) \cap \R_{2}$, then remove the items in $\R_{2}$ and remove the least profitable strip of height $\eps N$ from $\R_{1}$ by assuming the rectangles of $\R_{1}$ to be part of a container of dimension $\frac{N}{2} \times \frac{N}{2}$. Then we place the items in $\opt_{LT} \cap \Rho$ at bottom right of the knapsack on top of each other in the decreasing order of width. Then place the remaining items of $\R_{1}$ on top of the items in  $\opt_{LT} \cap \Rho$ . Now we have a new L packing and an empty square region with height at least $\frac{N}{2}$ and width at least $(\frac{1}{2} + \epsr)N$. Therefore we can pack every item belonging to $\opt_{ST}$ in 2 separate containers as shown in Figure \ref{prop1}(b) and (c) .
\\We ignore other cases as they are symmetric to the above two cases. 
\\
\\ The profit we can pack is at least $\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{LF})$  
\end{proof}
Now combining Lemma \ref{idea} with Lemmas  \ref{algo1} and \ref{algo2} we get  $\profit(OPT_{L\&C})\geq(\frac{7}{10}-O(\eps))\profit(OPT)$.The worst case is obtained when $\profit(\opt_{T})=3\profit(\opt_{LF})=3\profit(\opt_{SF})$.


\subsection{Adding small rectangles}\label{smallrec}
\begin{lem}\cite{GalvezGHI0W17}\label{dead}
In the packings mentioned in Lemma \ref{algo1} and Lemma \ref{algo2}, if we build a grid of width $\eps'N=\frac{\epss}{\eps}\cdot N$ and delete any cell of the grid that overlaps with the container or boundary-$\Lc$ then total area of the deleted grid cells is min$\{ (1-\eps) N^{2},a(\opt_{corr})+3\eps^{2}N^{2}\}$ where $a(\opt_{corr})$ denotes total area of corridors.
\end{lem}
 We denote the cells which are not dead as free cells. Now take the knapsack and and find the regions which are guillotine separable and doesn't overlap with any container or boundary-$\Lc$. Let us denote these regions as guillotine free region. By appropriate choosing $\eps,\epsl,\epss,\eps_{box},\epsau$ as shown in subsection \ref{cnt} we can ensure that the total area of guillotine free regions which don't have both the dimensions greater than or equal to $\eps' N$ is $O_{\eps,\epsl,\eps_{box},\epsau}(1)\cdot \frac{\epss}{\eps}\cdot N^{2}$ which is at most $O(\eps^{2})N^{2}$. Now total area of guillotine free region is greater than or equal to the total area of free cells. So the total area of gullotine free regions with both dimensions greater than or equal to  $\eps' N$ is at least (max$\{ (\eps N^{2},a(\opt_{small})-3\eps^{2}N^{2}\}-O(\eps^{2}N^{2}$)). We have sufficient area to pack small rectangles of the packings in Lemma \ref{algo1} and Lemma \ref{algo2}. 
\\ 
\begin{lem}\label{bigL}
In the packing mentioned in Lemma \ref{idea} and consider the grid created in Lemma \ref{dead}, total area of deleted grid cells is at most $a(\opt_{L})+a(\opt_{ST})+3\eps'\cdot N$. Grid cells are considered to be dead if they overlap with any rectangle.
\end{lem}
\begin{proof}Consider a boundary-$\Lc$ such that the vertical subcorridor $S_{1}$ is top-left  of horizontal subcorridor $S_{2}$.In the packing of Lemma \ref{idea} we can ensure that width of the boundary-$\Lc$ is at most $\frac{N}{2}$ (using similar techniques as used in Case  2 of Lemma \ref{idea}) and still satisfy Lemma \ref{idea}. Now consider the first column of grid cells from left. Area of dead cells in first column is at most $\eps'N^{2}$. In the second column of grid cells from left if there are $x$ grids cells which are dead then length of \ari{all the $L$ rectangles }in the first column is at least $(x-1)\cdot \eps' N$ due to Lemma \ref{lpackinglem}. So area of dead cells in second column is at most area of rectangles in first column plus $\eps'^{2}N^{2}$. Adding up the area of all the dead cells in this manner and repeating the same for horizontal rectangles we get total area of deleted grid cells to be at most $a(\opt_{L})+a(\opt_{ST})+3\eps'\cdot N^{2}$.
\\
\\A box is said to be $\eps'$ large if both dimensions are greater than or equal to $\eps' N$. Now the free grid cells in the rectangular region which doesn't contain boundary-$\Lc$ are guillotine separable. Now we describe a procedure to obtain $(1-\eps)\eps'$ large boxes (to pack the small rectangles) from the free cells in the boundary-$\Lc$. Note that these $(1-\eps)\eps'$ large boxes when considered as pseudorectangles are guillotine separable. Consider the first column of grid cells from the left and assume that we have free cells in this column. Separate the horizontal rectangle if any (using a horizontal guillotine cut) which overlaps with this first column. Now consider the rightmost vertical cut which passes through this column. Distance of this cut from the right-hand side of this column is at most $\epss N$. So we obtain $(1-\eps)\eps'$ large boxes in the first column which are guillotine separable.  Continue the same process for other columns which overlap with the vertical subcorridor of the boundary-$\Lc$. Free cells which are in the horizontal subcorridor at the end of this process are guillotine separable. Area of guillotine separable boxes obtained from free cells is at least $(1-\eps)(a(\opt_{small})-3\eps'\cdot N^{2})$. So if $a(\opt_{small})\geq \frac{N^{2}}{4}-2\eps' \cdot N^{2}$ we can pack almost all the small rectangles using NFDH in the guillotine separable  $(1-\eps)\eps'$ large boxes created and the guillotine separable free cells present in the region which doesn't contain boundary-$\Lc$. If $a(\opt_{small})$<$\frac{N^{2}}{4}-2\eps' \cdot N^{2}$ we can pack all the small rectangles as area of guillotine separable free cells is at least $\frac{N^{2}}{4}-2\eps' \cdot N^{2}$.
\end{proof}

\subsection{Relationship between different constants}\label{cnt}
 We set $\epsau$ to be $\eps^{2}$ and $\epsau'=\epsau/2$. By choosing a big enough constant $\lambda$ such that number of corridors obtained is far less than $\frac{1}{\eps} \cdot (1/\epsl')^{\lambda}$ given that at least one of the dimension of the rectangles while corridor decomposition is greater than $\epsl' N$, we set function $f(x)$ in the lemma \ref{class} to be $\frac{x^{3\lambda}}{(2K'(\epsau'^{\lambda^{1/\eps}})+\frac{1}{\epsau'})^{2}}$. Note than $\lambda$ doesn't depend on $\epsl'$. Here $K'(x)=(\frac{2}{x^{10}}+(\frac{3}{x^{2}}(M(x))^{2}2^{2M(x)})^{\epsau'})$ $\lceil log_{1+\epsau'}(1/x)\rceil/\eps^{2}$ where $M(x)=\frac{1+2x}{x^{2}}$. We set $\eps_{box}$ to be $\eps^{3}\epsl^{\lambda}$. This ensures that  sum of the heights of the rectangles in $\opt_{thin} \cap \R_{hor}$ is less than $\eps^{2} N$. Now we show that all our constraints are satisfied. By lemma \ref{class} we get a pair $(\epss,\epsl)$ such that $\epss \leq \frac{\epsl^{3\lambda}}{(2K'(\eps^{\lambda^{1/\epsau'}})+1/\epsau')^{2}}$.  Let the total area of guillotine free regions with at least one of the dimensions less than $\eps' N$ be $A_{< \eps'}$. Then $A_{< \eps'} < \frac{1}{\eps_{box}}\cdot(2K'(\delta)+1/\epsau')^{2}\cdot\frac{1}{\eps}\cdot(\frac{1}{\epsl})^{\lambda}\cdot\frac{\epss}{\eps}N^{2}<\eps^{2}N^{2}$. Here $\delta > \epsau'^{\lambda^{1/\eps}}$. Loose upper bound for $A_{< \eps'}$ is found by multiplying the total number of containers by maximum area of guillotine free region which isn't $\eps'$ large. Here as we said before $\lambda$ is a very large constant such that it satisfies all the inequalities which can be found by finding largest constant $c_{1}$ which arises in our equation which we can safely assume to be say greater than 5 and keeping $\lambda=c_{1}^{\frac{1}{\eps}\cdot 10^{10}}$.
 
\subsection{Finding the packing in polynomial time} \arir{write more details.}
Using GAP(as mentioned in \cite{GalvezGHI0W17}) and brute forcing among polynomial number of options we can find the packing which gives the desired approximation factor in polynomial time.


==> Backup/6_Rotated_Cardinality.tex <==
	
\section{$(\frac{5}{4}+\eps)$-approximation \tggkcr}
	\begin{lem}
	$|\opt_{L\&C}|\geq |\opt_{F}|+|\opt_{T}|/2$.
	\label{rlem1}  
	\end{lem}
	\begin{proof}Lemma \ref{rlem1} follows from Lemma \ref{algo1} by considering profit of each item to be 1.\end{proof}
	\begin{lem}\cite{GalvezGHI0W17}
	$|\opt_{L\&C}|\geq \frac{2|\opt_{F}|}{3}+|\opt_{T}|$.
	\label{rlem2}  
	\end{lem}
	\begin{proof}	
	Lemma \ref{rlem2} holds even in the case of Guillotine setup as the proof techniques used in \cite{GalvezGHI0W17} don't disturb the guillotine property.
	\end{proof}
	%\begin{figure}[!htb]
	%\centering
	%\includegraphics[scale=.7]{T+34SF}
	%\caption{Case: T+3/4SF processing}
	%\label{T+3/4SF-}
	%\end{figure}
	
	
	
	\begin{figure}[!htb]
		%\centering
		\captionsetup[subfigure]{justification=centering}
		\hspace{-10pt}
		\begin{subfigure}[b]{.32\textwidth}
			\centering
			\resizebox{!}{4cm}{
			\begin{tikzpicture}
				%box		
				\draw[thick] (0,0) rectangle (6.0,6.0);
				\draw[solid, fill = lightgray] (.47,.25) rectangle (.97,3.25);
				\draw[solid, fill = lightgray] (.17,4.66) rectangle (1.59,5.41);
				\draw[solid, fill = lightgray] (2.13,.38) rectangle (4.01,1.45);
				\draw[solid, fill = lightgray] (2.33,2.81) rectangle (2.83,5.81);
				\draw[solid, fill = lightgray] (3.29,2.2) rectangle (4.47,3);
				\draw[solid, fill = lightgray] (3.21,4.17) rectangle (5.66,4.67);
				\draw[solid, fill = lightgray] (3.5,5.16) rectangle (5.5,5.80);
				\draw[solid, fill = lightgray] (4.83,.5) rectangle (5.66,3.4);
				
	
				\draw[dashed] (1.75,0) -- ( 1.75, 6.0);
				\draw[dashed] (2.50, 0) -- ( 2.50, 6.0);
	
				\draw (2.125,6.3) node {\large \textbf{$3\eps N$}};
			
			
			\end{tikzpicture}}
			\caption{}
			
		\end{subfigure}
		\begin{subfigure}[b]{.32\textwidth}
			\centering
			\resizebox{!}{4cm}{
			\begin{tikzpicture}
				%box			
				\draw[thick] (0,0) rectangle (6.0,6.0);
				\draw[solid, fill = lightgray] (.47,.25) rectangle (.97,3.25);
				\draw[solid, fill = lightgray] (.17,4.66) rectangle (1.59,5.41);
				%\draw[solid, fill = lightgray] (2.13,.38) rectangle (4.01,1.45);
				%\draw[solid, fill = lightgray] (2.33,2.81) rectangle (2.83,5.81);
				\draw[solid, fill = lightgray] (2.54,2.2) rectangle (3.72,3);
				\draw[solid, fill = lightgray] (2.31,4.17) rectangle (4.91,4.67);
				\draw[solid, fill = lightgray] (2.75,5.16) rectangle (4.75,5.80);
				\draw[solid, fill = lightgray] (4.08,.5) rectangle (4.91,3.4);
				
	
				\draw[dashed] (5.25,0) -- ( 5.25, 6.0);
				%\draw[dashed] (3.19, 0) -- ( 3.19, 6.08);
		
				\draw (5.625,6.3) node {\large \textbf{$2\eps N$}};
			
			\end{tikzpicture}}
			\caption{}
			
		\end{subfigure}
		\begin{subfigure}[b]{.32\textwidth}
			\centering
			\resizebox{!}{4cm}{
			\begin{tikzpicture}
				%box			
				\draw[thick] (0,0) rectangle (6.0,6.0);
				\draw[solid, fill = lightgray] (.47,.25) rectangle (.97,3.25);
				\draw[solid, fill = lightgray] (.17,4.66) rectangle (1.59,5.41);
				%\draw[solid, fill = lightgray] (2.13,.38) rectangle (4.01,1.45);
				%\draw[solid, fill = lightgray] (2.33,2.81) rectangle (2.83,5.81);
				\draw[solid, fill = lightgray] (2.54,2.2) rectangle (3.72,3);
				\draw[solid, fill = lightgray] (2.31,4.17) rectangle (4.91,4.67);
				\draw[solid, fill = lightgray] (2.75,5.16) rectangle (4.75,5.80);
				\draw[solid, fill = lightgray] (4.08,.5) rectangle (4.91,3.4);
				
	
				\draw[dashed] (5.25,0) -- ( 5.25, 6.0);
	
				\draw[solid, fill = gray] (5.95,1) rectangle (6,6);
				\draw[solid, fill = gray] (5.85,1.1) rectangle (5.95,6);
				\draw[solid, fill = gray] (5.80,1.2) rectangle (5.85,6);
				\draw[solid, fill = gray] (5.75,1.25) rectangle (5.8,6);
				\draw[solid, fill = gray] (5.65,1.3) rectangle (5.75,6);
				\draw[solid, fill = gray] (5.55,1.4) rectangle (5.65,6);
				\draw[solid, fill = gray] (5.45,1.9) rectangle (5.55,6);
				\draw[solid, fill = gray] (5.35,2.1) rectangle (5.45,6);
				\draw[solid, fill = gray] (5.30,2.4) rectangle (5.35,6);
	
				
				%\draw[dashed] (3.19, 0) -- ( 3.19, 6.08);
		
				\draw (5.625,6.3) node {\large \textbf{$2\eps N$}};
			\end{tikzpicture}}
			\caption{}
			
		\end{subfigure}
		\caption{Case: T+3/4SF processing}
		\label{T+3/4SF-}
	\end{figure}
	
	
	\begin{lem}
	\label{strip_improvement_with_cardinality}
	$|\opt_{L\&C}|\geq |\opt_{T}|+3|\opt_{SF}/4|$.
	\end{lem}
	\begin{proof} Consider the optimal packing of $\R_{SF}$ in the $N \times N$ knapsack. Chose a random horizontal strip $H$ of width $3\eps N$ at a random offset $r$ from the left boundary of knapsack where $r \in [0, (1-3\eps)N]$. The region is defined by $ H = [0 , N ] \times [ r, r +  \eps N ]$. Delete all items intersecting strip $H$. Since each item in $\opt_{SF} \cap \Rve$ is of height at most $\height_{ver} \leq \frac{1}{2} $, it is removed with probability at most $\frac{1}{2} + 6\eps$.  Each item of $\opt_{SF} \cap \Rho$ is of height at most $\height_{ver} \leq \epss N \leq \eps N $, it is removed with probability at most $7\eps$. Thus the items remaining after removal of strip $H$ have profit atleast $(\frac{1}{2} - 6\eps)(\profit(\opt_{SF})\cap\profit(\opt{ver})) + ( 1- 7\eps) (\profit(\opt_{SF})\cap\profit(\opt{hor}))$ .\\
	\\Similarly considering a vertical strip $V$ = $[ r, r + 3 \eps N  ] \times  [0 , N ]$ . Following arguments similar to horizontal case. Each item in $\opt_{SF} \cap \Rho$ is removed with probability at most $\frac{1}{2} + 6\eps$.  Each item of $\opt_{SF} \cap \Rve$ is removed with probability at most $7\eps$. Thus the items remaining after removal of strip $V$ have profit at-least $(\frac{1}{2} - 6\eps)(\profit(\opt_{SF})\cap\profit(\opt{hor}) )+ ( 1- 7\eps) (\profit(\opt_{SF})\cap\profit(\opt{ver}))$ .\\
	\\We obtain a packing of atleast  $(\frac{3}{4} - \frac{13}{2}\eps)(\profit(\opt_{SF}))$ items  by considering the best of above two cases in a region $[0 , N- 2\eps N] \times [0,N] $ after doing resource augmentation(assuming that the vertical strip removes less items in expectation).\\
	The total width ( resp., height)  of items in $\opt_{T} \cap \R_{hor}$ (resp., $\opt_{T} \cap \R_{ver}$) is at most $\epsr N $.
	It is also given that $\epsr \leq \eps$.  We then rotate every item in $\opt_{T} \cap \R_{hor}$ to make it vertical . The set of item $\opt_{T}$ is now of total width at most  $2\epsr N $. Now we place every item in $\opt_{T}$ beside each other in the rectangular region  $  [ N- 2\eps N ,N] \times [0,N] $ obtained from removing the vertical strip from $\opt_{SF}$ packing as shown in Figure \ref{T+3/4SF-}. It is worth mentioning that the proof indeed applies to a general weighted case also as every equation is in terms of profit of items. For our cardinality proof however we consider profit of each item to be 1 which concludes the proof.
\end{proof}
	
	
	%\begin{figure}[!htb]
	%\centering
	%\includegraphics[scale=.7]{L+ST}
	%\caption{Case : L+ST processing}
	%\label{L+ST Processing}
	%\end{figure}
	
		\begin{figure}[!htb]
		%\centering
		\captionsetup[subfigure]{justification=centering}
		\hspace{-10pt}
		\begin{subfigure}[b]{.32\textwidth}
			\centering
			\resizebox{!}{4.5cm}{
			\begin{tikzpicture}
				%box		
				\draw[thick] (0,0) rectangle (8.0,8.0);
				\draw[solid , fill = lightgray] (0,0)-- ( 8.0, 0) -- ( 8.0 , 6.2 ) -- ( 6.2, 6.2 ) -- ( 6.2, 8.0 ) -- ( 0 , 8.0 ) -- ( 0,0 ) ;
				
				\draw [dashed] ( .2,8.0) -- (.2 ,.2 ) -- ( 8.0, .2) ;
				\draw [dashed] ( .6,8.0) -- ( .6, .6) -- ( 8.0, .6) ;
				\draw [dashed] ( 1.4,8.0) -- ( 1.4, 1.4) -- ( 8.0,1.4 ) ;
				\draw [dashed] ( 3.0,8.0) -- ( 3.0, 3.0) -- ( 8.0,3.0 ) ;
				\draw [dashed] ( 6.2,8.0) -- (6.2 ,6.2 ) -- ( 8.0, 6.2) ;	
	
				\draw [dashed] ( 6.2,6.2) -- ( 6.2, 5.0) -- ( 5.0,5.0) -- ( 5.0, 4.0 ) -- ( 4.0 , 4.0 ) --( 4.0, 3.5) -- ( 3.5, 3.5) --( 3.0, 3.5)  -- ( 3.0 , 3.0) ;
				\draw [dashed] ( 3.0 , 3.0 ) -- ( 3.0 , 2.0 ) -- ( 2.0 , 2.0 ) -- ( 2.0 , 1.4) -- ( 1.4, 1.4) ;
				\draw [dashed] ( 1.4, 1.4) -- ( 1.0 , 1.4) -- ( 1.0 , 1.0 ) -- ( .6, 1.0 ) --( .6, .6) ;
				\draw [dashed] ( .6,.6) -- ( .6 , .4) -- ( .4, .4) -- ( .4, .2) -- ( .2, .2);
				\draw [dashed] ( .2, .2) -- ( .1 ,.2 ) -- ( .1, .1) -- ( 0 , .1) -- ( 0,0);	
	
				%labeling 
				\draw (0,8.3) node {   \textbf{$2\eps'$}};
				\draw (.5,8.3) node {  \textbf{$6\eps'$}};
				\draw (1.0,8.3) node {   \textbf{$12\eps'$}};
				\draw (2.2,8.3) node {   \textbf{$24\eps'$}};
				\draw (4.6,8.3) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
	
				\draw (8.5,.1) node {   \textbf{$\leq 2\eps'$}};
				\draw (8.5,.4) node {  \textbf{$\leq 6\eps'$}};
				\draw (8.5,1) node {   \textbf{$\leq 12\eps'$}};
				\draw (8.5,2.2) node {   \textbf{$\leq 24\eps'$}};
				%\draw (9.1,4.6) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
	
			\end{tikzpicture}}
			\caption{}
		\end{subfigure}
		\begin{subfigure}[b]{.32\textwidth}
			\centering
			\resizebox{!}{4.5cm}{
			\begin{tikzpicture}
				%box					
				\draw[thick] (0,0) rectangle (8.0,8.0);
				\draw[solid , fill = lightgray] (0,0)-- ( 8.0, 0) -- ( 8.0 , .6 ) --( .6,.6) -- ( .6, 8.0 ) -- ( 0, 8.0 ) -- ( 0,0);
				\draw[solid , fill = lightgray] ( 8.0, 1.4) -- ( 1.4, 1.4) -- ( 1.4, 8.0 ) -- ( 6.2 , 8.0) -- ( 6.2, 6.2) -- ( 8.0 , 6.2) ;
	
				% dashed line 
				\draw[dashed] ( 1.2, .6) --( 1.2, 8.0) ;
				
				\draw [dashed] ( .2,8.0) -- (.2 ,.2 ) -- ( 8.0, .2) ;
				\draw [dashed] ( .6,8.0) -- ( .6, .6) -- ( 8.0, .6) ;
				\draw [dashed] ( 1.4,8.0) -- ( 1.4, 1.4) -- ( 8.0,1.4 ) ;
				\draw [dashed] ( 3.0,8.0) -- ( 3.0, 3.0) -- ( 8.0,3.0 ) ;
				\draw [dashed] ( 6.2,8.0) -- (6.2 ,6.2 ) -- ( 8.0, 6.2) ;	
	
				\draw [dashed] ( 6.2,6.2) -- ( 6.2, 5.0) -- ( 5.0,5.0) -- ( 5.0, 4.0 ) -- ( 4.0 , 4.0 ) --( 4.0, 3.5) -- ( 3.5, 3.5) --( 3.0, 3.5)  -- ( 3.0 , 3.0) ;
				\draw [dashed] ( 3.0 , 3.0 ) -- ( 3.0 , 2.0 ) -- ( 2.0 , 2.0 ) -- ( 2.0 , 1.4) -- ( 1.4, 1.4) ;
				%\draw [dashed] ( 14, 14) -- ( 10 , 14) -- ( 10 , 10 ) -- ( 6, 10 ) --( 6, 6) ;
				\draw [dashed] ( .6,.6) -- ( .6 , .4) -- ( .4, .4) -- ( .4, .2) -- ( .2, .2);
				\draw [dashed] ( .2, .2) -- ( .1 ,.2 ) -- ( .1, .1) -- ( 0 , .1) -- ( 0,0);
	
	
					%labeling 
				\draw (0,8.3) node {   \textbf{$2\eps'$}};
				\draw (.5,8.3) node {  \textbf{$6\eps'$}};
				\draw (1.0,8.3) node {   \textbf{$12\eps'$}};
				\draw (2.2,8.3) node {   \textbf{$24\eps'$}};
				\draw (4.6,8.3) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
	
				\draw (8.5,.1) node {   \textbf{$\leq 2\eps'$}};
				\draw (8.5,.4) node {  \textbf{$\leq 6\eps'$}};
				\draw (8.5,1) node {   \textbf{$\leq 12\eps'$}};
				\draw (8.5,2.2) node {   \textbf{$\leq 24\eps'$}};
				%\draw (9.1,4.6) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
	
			\end{tikzpicture}}
			\caption{}
		\end{subfigure}
			\begin{subfigure}[b]{.32\textwidth}
			\centering
			\resizebox{!}{4.5cm}{
			\begin{tikzpicture}
				%box					
				\draw[thick] (0,0) rectangle (8.0,8.0);
				%\draw[solid , fill = lightgray] (0,0)-- ( 80, 0) -- ( 80 , 6 ) --( 6,6) -- ( 6, 80 ) -- ( 0, 80 ) -- ( 0,0);
				\draw[solid , fill = lightgray] ( 8.0, 1.4) -- ( 1.4, 1.4) -- ( 1.4, 8.0 ) -- ( 6.2 , 8.0) -- ( 6.2, 6.2) -- ( 8.0 , 6.2) ;
	
				% dashed line 
				%\draw[dashed] ( 12, 6) --( 12, 80) ;
				
				\draw [dashed] ( .2,8.0) -- (.2 ,2 )  ;
				\draw [dashed] ( .6,8.0) -- ( .6, 6) ;
				\draw [dashed] ( 1.4,8.0) -- ( 1.4, 1.4)  ;
				\draw [dashed] ( 3.0,8.0) -- ( 3.0, 3.0) -- ( 8.0,3.0 ) ;
				\draw [dashed] ( 6.2,8.0) -- (6.2 ,6.2 ) -- ( 8.0, 6.2) ;	
	
				\draw [solid , fill = lightgray] ( 6.2,6.2) -- ( 6.2, 5.0) -- ( 5.0,5.0) -- ( 5.0, 4.0 ) -- ( 4.0 , 4.0 ) --( 4.0, 3.5) -- ( 3.5, 3.5) --( 3.0, 3.5)  -- ( 3.0 , 3.0) -- ( 3.0, 8.0) -- ( 6.2, 8.0 ) -- ( 6.2, 6.2)  ;
				\draw [solid , fill = lightgray] ( 3.0 , 3.0 ) -- ( 3.0 , 2.0 ) -- ( 2.0 , 2.0 ) -- ( 2.0 , 1.4) -- ( 1.4, 1.4) -- ( 1.4, 8.0 ) -- ( 3.0, 8.0) -- ( 3.0, 3.0) ;
				\draw [solid, fill = lightgray] ( 1.07, 8.0) -- ( 1.07, 1.0 ) -- ( 1.0 , 1.0) -- ( 1.0, .6) -- ( .6, .6) -- ( .6, 8.0) -- ( 1.07, 8.0);
				\draw [solid , fill = lightgray] ( .6,.6) -- ( .6 , .4) -- ( .4, .4) -- ( .4, .2) -- ( .2, .2) -- ( .2, 8.0) -- ( .6, 8.0 ) -- ( .6, .6) ;
				\draw [solid , fill = lightgray] ( .2, 8.0) -- ( .2, .2) -- ( .1 ,.2 ) -- ( .1, .1) -- ( 0 , .1) -- ( 0,0) -- ( 0 , 8.0) -- ( .2, 8.0) ;
	
	
			% items 
				\draw[ solid , fill = darkgray] (1.1,5.0) rectangle (1.2,7.5); 
				\draw[ solid , fill = darkgray] (1.15,1.4) rectangle (1.24,3.0); 
				\draw[ solid , fill = darkgray] (1.25,2.0) rectangle (1.3,6.0); 
	
			% dotted line
				\draw [ dashed ] ( 1.3, 0 ) -- ( 1.3, 8.0) ;
				\draw [ dashed ] ( 1.4, 0 ) -- ( 1.4, 8.0) ;
	
	
				%labeling 
				\draw (0,8.3) node {   \textbf{$2\eps'$}};
				\draw (.5,8.3) node {  \textbf{$6\eps'$}};
				\draw (1.0,8.3) node {   \textbf{$8\eps'$}};
				\draw (2.2,8.3) node {   \textbf{$24\eps'$}};
				\draw (4.6,8.3) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
	
				%\draw (8.5,.1) node {   \textbf{$\leq 2\eps$}};
				%\draw (8.5,.4) node {  \textbf{$\leq 6\eps$}};
				%\draw (8.5,1) node {   \textbf{$\leq 12\eps$}};
				\draw (8.5,2.2) node {   \textbf{$\leq 24\eps'$}};
				%\draw (9.1,4.6) node {   \textbf{$\geq 3 \times 2^{\frac{1}{\eps_{rot}} - 1}$}};
			\end{tikzpicture}}
			\caption{}
		\end{subfigure}
	\caption{Case : L+ST processing [$\eps' = \epsr]$}
	\label{L+ST Processing}
	\end{figure}
	
	\begin{lem}
	$|\opt_{L\&C}|\geq (1-O(\eps))|\opt_{LF}|+|\opt_{ LT}|+|\opt_{ST}|$.
	\end{lem}
	\begin{proof}
Consider the optimal packing and remove the items of $\opt_{SF}$. Now pack the items in $\opt_{LF}\cup \opt_{ LT}$ in the boundary $L$. Now partition the boundary L into $\frac{1}{2\eps_{rot}}$ smaller $L$ regions placed on top of each in the non-decreasing order of width of  $L$, where width of $L$ is the maximum of the height of the horizontal subcorridor and width of the vertical subcorridor. Here we assume that the sum of width of vertical subcorridor and height of horizontal subcorridor is more than $N$ otherwise we can rotate one of the subcorridor and place it to the side of the subcorridor and remove least profitable strip of width $\eps N$ and place all the items of $\opt_{ST}$. Let $\{L_{1},L_{2},...,L_{ \frac{1}{2\eps_{rot}}}\}$ be the set of smaller $L$ such that $L_{1}$ is the leftmost $L$ and $L_{ \frac{1}{2\eps_{rot}}}$ is the rightmost $L$. We now define the width of the smaller L regions and let us denote width by $w_{l}(.)$.  $w_{l}(L_{1})$ is $2\epsr$ and $w_{l}(L_{i})=\sum_{l=1}^{i-1}w_{l}(L_{l})+4\epsr$ for $2\leq i\leq \frac{1}{2\eps_{rot}}-1$. Note that $L_{\frac{1}{2\eps_{rot}}}$ automatically gets defined. If we choose $\eps_{rot}$ such that  $\eps_{rot}\geq \frac{1}{2(1+\frac{1}{log_{2}(\frac{1}{12\epsr})})} $ then we can ensure that $w_{l}(L_{\frac{1}{2\eps_{rot}}})\geq \sum_{l=1}^{i-1}w_{l}(L_{l})+4\epsr$. Now by averaging argument there exists a $L_{k}$ where $k \in [\frac{1}{2\eps_{rot}}]$ such that the number of rectangles intersecting $L_{k}$ is atmost $O(\eps_{rot})|\opt_{LF}\cup \opt_{ LT}|$. Now remove the rectangles intersecting this $L_{k}$. Without loss of generality we assume that the width of vertical subcorridor of $L_{k}$ is equal to $w_{l}(L_{k})$. Now rotate the horizontal subcorridors of $L_{i}$ where $1\leq i \leq k-1$ and place in the empty space created by removing $L_{k}$. Now there exists a vertical strip of width atleast $4\epsr N$. Now place the items of $\opt_{ST}$ and $\opt_{LT}$ in this strip. Now we are left with a strip of width atleast $2\epsr N$. Now we process the complete L region comprising of $L_{k+1},...,L_{\frac{1}{2\eps_{rot}}}$ as done in subsection \ref{prosec}. The least profitable strip which we remove as done in Lemma \ref{rlem1} can be packed in the vertical strip which is previously empty. This strip has width of atmost $2\epsr N$. Now we have a container packing. Hence our claim is proved.   
\end{proof}
\subsection{Finding the packing in polynomial time}

Using GAP(as mentioned in \cite{GalvezGHI0W17}) and brute forcing among polynomial number of options we can find the packing which gives the desired approximation factor in polynomial time.
	


==> Backup/7_Non_Rotated_Weighted.tex <==
\section{Weighted case}\label{w2dgk}
	\subsection{Shifting Argumentation\cite{GalvezGHI0W17}}\label{shifting}
%	We use similar process as used as in \cite{GalvezGHI0W17} and prove that if we begin with a guillotine separable solution, the process results in a final guillotine separable arrangement.
We aim to pack back the items dropped in all the previous steps of processing. Reconsidering the items dropped, i.e., $\opt_{kill}$, $\opt_{Large}$, $\opt_{corr}^{cross}$, we give a similar processing as devised in \cite{GalvezGHI0W17} for packing these items with just losing a small fraction of profit. Intuitively we divide the knapsack into a grid iteratively and observe the profit of items dropped as a result of processing the items which are classified depending on the grid. Using standard shifting argument we can claim that recursively doing the same procedure for $\frac{1}{\eps}$ times we get a set of items which can be dropped and have a profit of $O(\eps)$.

		\subsubsection{Grid and Corridor Partition}\label{gridpartition}
		We initiate $k(0)$ to the union of set of all items dropped in all the processing steps before (e.g., $\opt_{large}$, $\opt_{K}$, $\opt_{corr}^{cross}$ ). If the profit of items in $k(t)$ at any iteration $t$ is at most $\eps \profit(\opt)$ we get the desired set of items and halt.
Consider $t^{th}$ iteration, we denote $G(t)$ as the grid formed by extending the $x$, $y$ coordinates of the items in $\kappa(t)$. Consider $C_{t}$ to be the set of grid cells of $G(t)$. We classify items in the knapsack as small, large, horizontal, vertical as before depending on its intersection with the cells it overlaps. \\
An item $i$ having non-zero intersection with a cell $C$ $\in$ $C_{t}$ is classified inside $C$ as follows:
\begin{enumerate}
\item $\opt^{t}_{ver}(C)$ if  $\height(i \cap C)$ $>$ $\eps_{large}$ $\height(C)$ and $\width(i \cap C)$ $\leq$ $\eps_{small}$ $\width(C)$, 

\item $\opt^{t}_{hor}(C)$ if $\height(i \cap C)$ $\leq$ $\eps_{small}$ $\height(C)$ and $\width(i \cap C)$ $>$ $\eps_{large}$ $\width(C)$, 

\item $\opt^{t}_{large}(C)$ if $\height(i \cap C)$ $>$ $\eps_{large}$ $\height(C)$ and $\width(i \cap C)$ $>$ $\eps_{large}$ $\width(C)$, 

\item $\opt^{t}_{small}(C)$ if $\height(i \cap C)$ $\leq$ $\eps_{small}$ $\height(C)$ and $\width(i \cap C)$ $\leq$ $\eps_{small}$ $\width(C)$, 


\item $\opt^{t}_{intermediate}(C)$ if $\height(i \cap C)$ $\in$ $(\eps_{small}$ $\height(C)$,  $(\eps_{large}$ $\height(C)]$ or  $\width(i \cap C)$ $\in$ $(\eps_{small}$ $\width(C)$,  $(\eps_{large}$ $\width(C)]$ 

\item $\opt^{t}_{skew}(C)$ $=$  $\opt^{t}_{hor}(C) \cup \opt^{t}_{ver}(C)$.
\end{enumerate}

As done in previous sections, we can fix $\eps_{small}$ and $\eps_{large}$ such that the profit of items classified as intermediate for any cell is at  most $\eps \profit(\opt)$. $\eps$ $\geq$ $\eps_{large}$ $\geq$ $f(\eps_{small})$ $\geq$ $\omega_{\eps}(1)$, for some positive increasing function $f(.)$ .\\
We add items not contained in $\kappa(t)$ in $\opt_{large}(C)$ to $k(t+1)$ for all $C$ not fully covered by any item in $\kappa(t)$. We do corridor decomposition as in section \ref{subcorr}, considering only skew items in all the cells.\\%put the reference
 Although this corridor decomposition might kill some of the items in $\kappa(t)$ which we want to save. Thus we apply Lemma \ref{focsagain}  and \ref{againfocs} which uses further decomposition of corridors with constant number of line segments dropping a $ \eps$ fraction from optimal.
%Old-------------------------\\
%		In this section we try to recursively divide the knapsack into a non-uniform grid, stretch it to make it a uniform grid. We then sacrifice a 
%		small fraction of intercepted items and perform corridor partition to the remaining set of items. The corridor partition follows similar to 						section \ref{subcorr}. Consider the set of items $\kappa(t)$ at $t^{th}$ iteration as the items forming the grid. The grid at any such level of iteration is formed by extending the edges of all the items in $\kappa(t)$. We initiate $\kappa(0)$ with the items in $\opt_{large}$ $\cup$ $\opt_{corr}^{cross}$ $\cup$  $\opt_{kill}$ as defined in section \ref{profitstruc}. We recursively augment items packed at each iteration to $\kappa(t)$.  We also define a set $K(t+1)$ which contains all the items killed at $t^{th}$ iteration during the process. \\
%Consider the set $C_{t}$ of all grid cells at $t^{th}$ iteration. Same as in lemma \ref{class} we classify the items in cells as $\opt_{small}(C)$, $\opt_{large}(C)$, $\opt_{hor}(C)$, $\opt_{ver}(C)$, $\opt_{intermediate}(C)$. The lemma lets us drop $\eps$ fraction profit $\opt_{intermediate}(C)$ items in every cell. We then kill all the $\opt_{large}(C)$ in every cell $C$ $\in$ $C_{t}$. The killed rectangles are added to $K(t+1)$. We then stretch the grid to a uniform grid throughout the knapsack. Using processes in section \ref{subcorr} we obtain the corridor decomposition of the knapsack with the set of all skew items with $O_{\eps,\eps_{large},\kappa(t)}(1)$ corridors. The decomposition is equivalent to the decomposition of the original knapsack and we get the same set of killed items in both the cases. Since only a $O_{\eps}(1)$ items $\opt_{cross}$ are killed in the corridor decomposition. We add items in $\opt_{cross}$ and items not in $\kappa(t)$ to the set $K(t+1)$. Next we state the following lemma.
%\\
%old end-----------\\
\begin{lem}\cite{GalvezGHI0W17}\label{focsagain}
	Let $S$ be an open corridor with $b(S)$ bends. Let $\R'$ $\subseteq$ $\opt$ be a collection of items which intersect the boundary of $S$ with $\R'\bigcap \opt_{skew}(C_{t}) = \phi$. Then there is a collection of $|\R'|.b(S)$ line segments $L$ within $S$ which partition $S$ into sub-corridor with at most $b(S)$ bends each such that no item from $\R'$ is intersected by $L$ and there are at most $O_{\eps}(|\R'|.b(S))$ items of $\opt_{skew}(C_{t})$ intersected by line segments in $L$.
\end{lem}
\begin{lem}\cite{GalvezGHI0W17}\label{againfocs}
Let $S$ be a closed corridor with $b(S)$ bends. Let $\opt_{skew}(S)$ denote the items in $\opt_{skew}(C_{t})$ that are contained in $S$. Let $\R'$ $\subseteq$ $\opt$ be a collection of items which intersect the boundary of $S$ with  $\R'\bigcap \opt_{skew}(C_{t}) = \phi$. Then there is a collection of $O_{\eps}(\frac{|\R'|^{2}}{\eps})$ line segments $L$ within $S$ which partition $S$ into a collection of closed corridors with at most $\frac{1}{\eps}$ bends each and possibly an open corridor with $b(S)$ bends such that no item from $\R'$ is intersected by $L$ and there is a set of items $\opt'_{skew}(S) \subseteq \opt_{skew}(S)$ with $|\opt'_{skew}(S)|\leq O_{\eps}(|\R'|^{2})$ such that the items in $\opt_{skew}(S) \backslash \opt'_{skew}(S)$ intersected by the line segments in $L$ have a total profit of at most $O(\eps).\profit(\opt_{skew}(C_{t}))$.
\end{lem}
Using Lemmas \ref{focsagain} and \ref{againfocs} we partition the piece in $O_{\eps}(1)$ corridors (open and closed) packing all the items in $\opt_{skew}(S)$ $\backslash$ $\opt'_{skew}(S)$. We augment the remaining set of items $\opt'_{skew}(S)$ with small profit to $K(t+1)$.
\begin{remark}
Guillotine Separability : All the processes used to obtain the bends and corridor decomposition follow deletion of items only. Thus the remaining subset of items should be guillotine separable given that the initial packing was guillotine separable.
\end{remark}
		\subsubsection{Box Partition}\label{boxpart}
			We follow the same process as in original corridor decomposition section \ref{subcorr} on all the items completely lying inside the strips formed from the subcorridor processing in the previous section. The difference from previous section \ref{subcorr} is the set $\opt_{fat}$ being considered for packing i.e. we don't drop large items while forming the set $\opt_{ fat}$ in this section section. Then by using similar shifting procedure as in section \ref{subcorr} we shift items from one subcorridor to other to pack all but $\opt_{kill}$ of them.For now let us ignore the items in $\opt_{small}$ that cross a subcorridor (handled in section \ref{smallitems}). We add all the items in $\opt_{kill}$ into $K(t+1)$ which actually refers to the items killed in the $t^{th}$ iteration. From section \ref{subcorr} it follows that only $O_{\eps,\eps_{large},\eps_{box}}(1)$ of items are killed in partition of subcorridors to boxes. Also the killed items  do not belong to the set $\kappa(t)$.
%We divide the subcorridor into strips and then classify the items as $fat$ lying completely inside these strips. We call the set of items in this optimal packing as $\opt_{fat}$. Then by simple shifting argument, we pack the items in the strips killing $\opt_{kill}$ items in the process. We add all the items in $\opt_{kill}$ into $K(t+1)$ which actually refers to the items killed in the $t^{th}$ iteration. From section \ref{subcorr} it follows that only $O_{\eps,\eps_{large},\eps_{box}}(1)$ of items are killed in partition of subcorridors to boxes. Also the items killed do not belong to the set $\kappa(t)$.
			\begin{remark} 
			Guillotine Separability : Since items the division of subcorridors into boxes involves partition of subcorridor with lines. We remove all the items killed by these lines and pack the rest completely into the strips formed. The strips can be themselves separated by the same set of lines. Also since we begin from a guillotine separable arrangement, shifting the horizontal ( resp. vertical) items vertically ( resp. horizontally ) doesn't disturb the guillotine property. Thus guillotine separability is maintained after the processing of subcorridors into boxes. 
			\end{remark}
		\subsubsection{Container Partition}
		\label{containerweighted}
		We follow resource augmentation from Lemma \ref{lemma1}. The process borrows technique from partitioning box into containers as done in section \ref{subcorr} with the only difference that we include $\opt_{small}$ this time while processing. We classify an item as $\opt_{small}(C_{t}))$ if for every cell $C$ in $C_{t}$ intersecting with the item,  the item is classified as $\opt_{small}(C)$. In other words any item which is small in all the cells intersecting it, is classified as $\opt_{small}(C_{t})$. Now consider a horizontal box, using averaging argument there exits a strip with width $3\eps$ such that it intersects with items with total profit less than or equal to $O(\eps)\profit(\opt_{box})$. We neglect the small items intercepted by the strip for now and pack them later as mentioned in section \ref{smallitems}. Let the items killed be $\opt_{kill,box}$. We add items in $\opt_{kill,box}$ to the set of items dropped in the $t^{th}$ iteration, i.e., $K(t+1)$. We then apply resource augmentation to the set of remaining small items say $\opt'_{small}(C_{t})$ and pack subset $\opt''_{small}(C_{t})$.
This gives us an $L\&C$ packing of a profitable subset $\opt'_{skew}(C_{t})$ $\subseteq$ $\opt_{skew}(C_{t})$ and a subset of small items not intersected by the $3\eps$ strip, i.e., $\opt''_{small}(C_{t})$ $\subseteq$ $\opt'_{small}(C_{t})$. Total profit of items, i.e., $\profit(\opt'_{skew}(C_{t}))$ $+$ $\profit(\opt''_{small}(C_{t}))$ $+$ $\profit(K(t+1))$ $\geq$ ($1-O(\eps)$) $($ $\profit(\opt_{skew}(C_{t}))$ $+$ $\profit(\opt'_{small}(C_{t}))$ $)$.
%The subsets are such that only $O(\eps)$ factor of profit is lost. 
			\begin{remark}
			Guillotine Separability : The only process we do in this section is deleting some items intersecting a strip. Since deleting items doesn't affect guillotine separability therefore the remaining items are guillotine separable if the original arrangement is guillotine separable. Thus we get a guillotine separable arrangement after doing the processing as given in this section.
			\end{remark}
		\subsubsection{Packing Small Items}\label{smallitems}
			Now we repack the small items killed by lines of corridor decomposition in section \ref{boxpart}. Consider the set $\opt_{skew,killed}(C_{T})$ as the given set of items. We assign each item in $\opt_{skew,killed}(C_{T})$ to the cell it was contained maximally in the original packing. Consider a cell $C$ and the items assigned to $C$ as $\opt_{skew,killed}(C)$. By wisely choosing the factor $\eps_{small}$ we can force area of small items assigned to $C$, i.e.,  $a(\opt_{skew,killed}(C))$ to be at most $\eps a(C)$. This follows from the fact that number of items intersecting $C$ would be $O_{\eps,\eps_{large}}(1)$. Thus by using Lemma %\ref{smallpacking} and 
\ref{areafocs}
 we can pack a profitable fraction of items  $\opt'_{skew,killed}(C)$ $\subseteq$  $\opt_{skew,killed}(C)$ such that $\profit(\opt_{skew,killed}(C)) \geq (1-O(\eps)) \profit(\opt_{skew,killed}(C))$.
			\begin{lem}\cite{GalvezGHI0W17}\label{areafocs}
				Let $C$ be a cell. The total area of $C$ occupied 	by containers is at most $(1-2\eps)a(C)$.
			\end{lem}
			\begin{remark}
				Guillotine Separability : The processing in the section involves deleting a subset of rectangles which doesn't affect the guillotine separability of items. We use NFDH to pack the items in the cells. Since NFDH is 2-stage guillotine separable packing, inside each cell items are guillotine separable. If we consider each cell as a pseudo-item, we claim that the whole knapsack is guillotine separable. The claim follows from the fact that cells are formed from extending the edges in $\kappa(T)$. The guillotine cuts will always follow the corresponding edges of items. Thus the arrangement in whole after the processing is guillotine separable. 
			\end{remark}
		\subsubsection{L$\&$C Packing}\label{lc}
			Following the same iterative process we get $k$ subsets; $K(1), K(2),... K(k-1), K(k)$ such that $k\leq\frac{1}{\eps}$ and $\profit(K(k))$ $\leq$ $\eps \opt$. Now consider the grid $G_{k}$ corresponding to the set $\kappa(k)$ with the set of cells $C_{k}$. We do the corridor, subcorridor, box processing subroutines as defined in previous sections. We now apply routines of theorem \ref{LC} and prove the same result for weighted version of the problem. We keep the notations same as used in unweighted version, thus we have sets $\opt_{ST}$, $\opt_{SF}$, $\opt_{LF}$, $\opt_{LT}$. We augment items in $\kappa(k-1)$ to the set $\opt_{LF}$. We also define set $\opt_{small}$ to be $\opt_{small}(C(k))$ which is the set of items classified as small in each non-zero intersection cell of $C_k$.\\
Since we have followed the modified corridor decomposition from previous sections for packing $\opt_{small}$ which $O(\eps)$ loss in the profit, we can extend lemmas \ref{sumprofit}, \ref{algo1}, \ref{idea} to the weighted cases.\\
For extending the weighted argument to lemma \ref{algo2} (non-degenerate-$\Lc$ case), intuitively we follow the same striping argument to remove items and make space for items to be packed by resource augmentation. Thus we remove all the items from $\kappa(k-1)$, because any item in $\kappa(k-1)$ can be large in both dimensions and has a high probability of being cut by a strip. We further add small items as in previous sections without losing more than a constant profit. We then remove a $3\eps N$ strip as done in section \ref{containerweighted}. Any item in $\opt_{small}$ is cut by the strip with a probability $3\eps$ and any other item is cut with probability $\frac{1}{2} + O(\eps)$. We construct the $\Lc$ as done in unweighted case. Thus we get the following result :
\begin{lem}
\label{weightall}
Let $\opt_{L\&C}$ be the most profitable guillotine packing solution that is packed by an $L\&C$ packing and $\opt$ be the optimal  solution of $\tggk$. Then following lemmas hold:
	\begin{enumerate}
		\item $\profit(\opt_{L\&C})\geq\profit(\opt_{F})+\profit(\opt_{T})/2$ + $\profit(\opt_{small})$
		\item $\profit(\opt_{L\&C})\geq\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{SF})$ + $\profit(\optsm)$
		%\item $\profit(\opt_{L\&C})\geq\profit(\opt_{T})+\frac{1-O(\eps)}{2}\profit(\opt_{LF})$ + $\profit(\optsm)$		
		\arir{3 is not established and removed T+F/2}
	\end{enumerate}
\end{lem}
\begin{proof}
All the inequalities follows from the processing done above. We also claim that the solution follows guillotine property as we use results and lemmas from previous sections which are already established to maintain guillotine separability. Another processing done is deleting of items intersecting with the strip, since deleting items doesn't disturb guillotine cuts we have a guillotine separable packing as a result.
\end{proof}
\begin{lem}
Let $\opt_{L\&C}$ be the most profitable solution that is packed by an $L\&C$ packing which is guillotine and $\opt$ be optimal guillotine packing. Then $\profit(\opt_{L\&C})\geq(\frac{2}{3}-O(\eps))\profit(\opt)$.
\end{lem}
\begin{proof}
The result follows from lemma \ref{weightall}, we thus get a factor of $3/2$, i.e., $\profit(\opt_{L\&C})$ $\geq$ $ (2/3 - O(\eps))\profit(\opt)$ for weighted case.
\end{proof}

\subsection{Weighted Rotated Case : \tggkr}
%%\arir{Use $N \times N$ knapsack instead of $1\times 1$ -- Done}

% Massive items defintion
%Large items which we drop out initially in the cardinality case analysis, cannot be removed in the weighed case as they might carry all the profit of the knapsack. Thus intuitively we define such a large item as {\em massive} item. Formally a
An item is called {\em massive} if $\width_{i} \geq (1-\eps)N$ and $\height_{i} \geq (1-\eps)N$, given the dimensions of original knapsack as $N \times N$. Chose $\eps > \epsr$ and $\eps < \frac{1}{10}$. Idea is to devise two packings; one when such a massive item is present and other when it is absent; and analyze the worst bound from both of them to get a bound for the weighted rotated case.

	\begin{lem}
		Given $\opt$ is the set of guillotine separable items that can be optimally packed in a $N \times N$ knapsack with associated profit $\profit(\opt)$, if rotations are allowed. Then there exits a packing of items $APX \subseteq \opt$ in $O_{\eps}(1)$ containers such that the profit of items $\profit(APX)\geq (\frac{3}{4}-O(\eps))\profit(\opt)$.
	\end{lem}
	\begin{proof}
		We prove the result by a case analysis. We subdivide the problem in two cases as discussed above on the basis of presence or absence of a massive item.	The result follows from Lemma \ref{lem:present} ( packing when massive item is present ) and Lemma \ref{lem:absent} ( case when there exits no massive item ). The worst case packing from among two gives us a factor of $4/3$, i.e., $\profit(APX)$ $\geq$ $ (3/4 - O(\eps))\profit(\opt)$ for weighted case given rotations are allowed.
	\end{proof}

%%%%%%%5 massive item present
	\begin{lem} \label{lem:present}
		Given $\opt$ be the set of items in the optimal guillotine separable packing into a $N\times N$ knapsack and there is a massive item $m \in \opt$. Then, there exists a set $\apx$ $\subseteq$ $\opt$ with $\profit(\apx) \geq (\frac{4}{5} - O(\eps)) \profit(\opt) $ which can be packed with rotations allowed in a container packing with $O_{\eps}(1)$ containers.
	\end{lem}	\amar{tight case : (T,F,m) = (  .4, .4, .2)}
	\begin{proof}
	Consider the optimal packing of items in $\opt$. Irrespective of the initial arrangement inductively we can show that it is possible to place $m$ on the top-right corner of the knapsack with the remaining items forming a  boundary-$\Lc$ in the remaining region $\big(([0,N]\times[0,\height_{L}]) \cup ([0,\width_{L}] \times[0,N])\big)$, where $\height_{L} = N-\height(m)$ and $\width_{L} = N-\width(m)$. The proof follows constructively by considering the sequence of guillotine cuts on the knapsack and following similar {\em mirroring} arguments as done in section \ref{glp}. \amar{do we need a rigorous proof show existence of an L}. \\
	We propose three different packings and consider the maximum profit packing from the three of them. Process the $\Lc$-corridor to get a corridor decomposition as done Section \ref{subcorr}. We define items to be thin ($T$), and fat ($F$) ( excluding $m$ ) as defined previously. Items completely lying in the horizontal arm of $L$ defined by the region  $([0,N]\times[0,\height_{L}])$ are defined as $\opt_{H}$. Similarly items completely lying the in vertical arm of $L$ defined by the region $([0,\width_{L}] \times[0,N])$ are defined as $\opt_{V}$. Thus we get $\opt_{HF}$, $\opt_{HT}$, $\opt_{VF}$, $\opt_{VT} $ as the fat-horizontal, thin-horizontal, fat-vertical, thin-vertical items respectively. W.l.o.g.~we can assume that $\width_{L} \geq \height_{L}$. \\
	
\noindent {\em Packing 1:}
We remove the lesser profit set among $\opt_{VT}$ and $\opt_{HT}$, and process the $\Lc$-corridor to obtain a container packing of the remaining items of $\opt_{T}$ and all items from $\opt_{F}$ as done in Section \ref{subcorr}. Since $\opt_{VT} \cup \opt_{HT} = \opt_{T}$, from averaging principle we get the profit of thin items packed as at least $\profit(\opt_{T})/2$. This gives us a packing of a set of items $P1$ with $\profit(P1)$ $\geq$ $(1-O(\eps))(\profit(m) + \profit(\opt_{T})/2 + \profit(\opt_{F}))$.\\

\noindent {\em Packing 2:}
From corridor decomposition it follows that the total width ( resp. height ) of items in vertical ( resp. horizontal ) subcorridor of the $\Lc$-corridor is atmost $\epsr \width_{L}$ ( resp. $\epsr \height_{L} $) which on the other hand is upper bounded by $\eps \width_{L}$ ( resp. $\eps \height_{L} $) .We now rotate the items in $\opt_{HT}$ and pack the items in $\opt_{VT} \cup \opt_{HT}$ in region $([0,\eps(\height_{L}+\width_{L})]\times[0,N])$. Items in $\opt_{HF}$ are rotated and then packed besides $\opt_{VF}$ so as to obtain a packing of $\opt_{F} = \opt_{VF} \cup \opt_{HF}$ in the plane of height $N$ and width $\width_{F}$ atleast $(1-\eps)(\width_{L} + \height_{L})$. We remove a random vertical strip of width $\height_{L}$ from this plane. From averaging principle any item of $\opt_{F}$ is saved by the random strip with probability atleast $\frac{(1-\eps)(\width_{L}) - \eps \height_{L}}{(1-\eps)(\width_{L} + \height_{L})} = \frac{\width_{L}}{\width_{L} + \height_{L}} - \frac{\eps}{1-\eps}.\frac{\height_{L}}{\width_{L} + \height_{L}} \geq \frac{1}{2} - \frac{\eps}{2(1-\eps)} = \frac{1}{2} - O(\eps)$. Thus the remaining set of items $\R'$ after removal of vertical strip have a $\width(\R') \leq$ $\width_{L} - \eps (\height_{L} + \width_{L})$ and a profit $\profit(\R') \geq$ $\profit(\opt_{T}) + \profit(\opt_{F})/2$. Using resource augmentation (Lemma \ref{lemma1}) we obtain a packing of these items  $\R'' \subseteq \R'$ in a region $([0,\width_{L}]\times[0,N])$ using $O_{\eps}(1)$, with  $\profit(\R'') \geq (1-O(\eps)) \profit(\R')$. Thus we get a packing of $\R'' \cup \{ m\}$ such that $\profit(P2) \geq (1-O(\eps)) \profit(\R') + \profit(m) = (1-O(\eps))( \profit(\opt_{T})/2 + \profit(\opt_{F})) + \profit(m)$.\\

\noindent {\em Packing 3:}
We consider the packing without $m$. Next we rotate $\opt_{H}$, to obtain a packing of $\opt_{H} \cup \opt_{V}$ in region $R'=$ $([0,\height_{L}+\width_{L}]\times[0,N])$. Clearly $R'$ $\subseteq$ $([0,2\eps]\times[0,1])$. Using resource augmentation lemma \ref{lemma1} we can pack a set of items $P3 \subseteq (\opt_{H} \cup \opt_{V})$ such that $\profit(P3) \geq (1-O(\eps))(\profit(\opt_{H}) + \profit(\opt_{V})) = (1-O(\eps))(\profit(\opt_{F}) + \profit(\opt_{T}))$.\\

Considering the maximum profit packing from $P1, P2, P3$, we obtain a packing of set of items $\apx$ $\subseteq$ $\opt$ with $\profit(\apx) \geq (\frac{4}{5} - O(\eps)) \profit(\opt) $ in $O_{\eps}(1) $ containers.	
	\end{proof}

%%%%%% no massive item
	\begin{lem}[Lemma \ref{weightall}]
		\label{lem:wr1}
		$\profit(\opt_{L\&C})\geq\profit(\opt \backslash \opt_{T})+\profit(\opt_{T})/2$.
	\end{lem}
	
	\begin{lem}
		\label{lem:wr2}
		$\profit(\opt_{L\&C})\geq \profit(\opt_{T})+\frac{3 \opt_{SF}}{4} + \frac{\opt_{LF}}{2}+\profit(\opt_{small})$.
	\end{lem}
	\begin{proof}
		We extend the weighted argument to Lemma \ref{strip_improvement_with_cardinality}. We first consider packing of items in $\opt_{SF}$ and add small items as in section \ref{smallitems} without losing more than a constant profit. 
%We then remove a $3\eps N$ strip as done in Lemma \ref{strip_improvement_with_cardinality} which can be either horizontal or vertical. 
We follow the same striping argument to remove the least profitable $3\eps N$ strip ( either horizontal or vertical ) and make space for items in $T$ to be packed in a $\eps N$ strip and then pack the items by resource augmentation. Any item in $\opt_{small}$ is cut by the strip with a probability $3\eps$.
%Thus we remove all the items from $\kappa(k-1)$, because any item in $\kappa(k-1)$ can be large in both dimensions and has a high probability of being cut by a strip. 
% Taking the best of horizontal and vertical strips we can ensure that any item in $\opt_{SF}$ is cut with probability $\frac{3}{4} + O(\eps)$ as done in Lemma \ref{strip_improvement_with_cardinality}.
This gives us a packing with profit atleast  $\profit(\opt_{L\&C})\geq \profit(\opt_{T})+3(\opt_{SF}/4) + \profit(\optsm)$.
	\end{proof}

	\begin{lem} \label{lem:absent}
		Given $\opt$ be the set of items in the optimal guillotine separable packing into a $N \times N$ knapsack and there exists no massive item in $ \opt$. Then, there exists a set $\apx$ $\subseteq$ $\opt$ with $\profit(\apx) \geq (\frac{3}{4} - O(\eps)) \profit(\opt) $ which can be packed with rotations allowed in a container packing with $O_{\eps}(1)$ containers.
	\end{lem}
	\begin{proof}
		We consider $3$ different packings and consider the most profitable of them for final packing. We first perform the basic corridor decomposition and classify items as $LT$, $ST$ and $LF$, $SF$. We define three different packings as follows:\\
		
\noindent{\em Packing 1:} Consider items in $\opt \backslash \opt_{T}$. Using resource contraction (Lemma \ref{lem:rsrccontraction}), we can pack items with profit atleast $\profit(\opt \backslash \opt_{T})/2$ in a $(N\times(1-\eps/2)N)$ piece. We then pack $\opt_{T}$ in the remaining $(N \times \eps N/4)$ region and then apply resource augmentation Lemma \ref{lemma1} to get the packing without losing more then $O_{\eps}(1)$ profit of total items in a $N \times N$ piece. Thus we get a packing of a set of items $P1$ with profit $\profit(P1)\geq \profit(\opt \backslash \opt_{T})/2 + \profit(\opt_{T})$.\\

\noindent{\em Packing 2:} Using Lemma \ref{lem:wr2} we get a packing of set of items $P2$ such that $\profit(P2)\geq \profit(\opt_{T})+3(\opt_{SF}/4) + (\opt_{LF}/2) +\profit(\opt_{small})$.

\noindent{\em Packing 3:} Using Lemma \ref{lem:wr1} we get a packing of set of items $P3$ such that $\profit(P3)\geq\profit(\opt \backslash \opt_{T})+\profit(\opt_{T})/2$.
\\
Considering the maximum profit packing from $P1, P2, P3$, we obtain a packing of set of items $\apx$ $\subseteq$ $\opt$ with $\profit(\apx) \geq (\frac{3}{4} - O(\eps)) \profit(\opt) $ in $O_{\eps}(1) $ containers. \amar{Tight case : F=.5, T=.5}
	\end{proof}

	\begin{lem}\cite{GalvezGHI0W17} % lemma 51 \cite{GalvezGHI0W17}
		\label{lem:rsrccontraction}
		 (Resource Contraction Lemma) If a set of guillotine separable items $M$ contains no massive item and can be packed into a $1\times1$ bin, then it is possible to pack a set $M'$ of profit at least $\profit(M)/2$ into a $N \times (1 - \eps/2)N$ bin (or a $(1- \eps /2)N\times N $ bin), maintaining guillotine property, given rotations are allowed.
	\end{lem}
	\begin{proof}
		We proceed along the same proof as in Lemma 51 of \cite{GalvezGHI0W17} and prove that the processing done maintains guillotine property of items.\\
Intuitively we consider two disjoint subsets of $M$, say $M'$ and $M \backslash M'$, and pack them individually in a $N \times (1- \eps/2)N$ bin. The best of two packings will give us a packing of profit atleast half the profit of $M$. We define set of items completely to the right, left, top, bottom of a given item $i$ as $Right(i)$, $Left(i)$, $Top(i)$, $Bottom(i)$ respectively. Formally, given item $i$ with bottom left coordinates as $(x_{i}, y_{i})$, we define $Right(i) = \{ i' \in M | x_{i'} \geq (x_{i}+\width(i))\}$, $Left(i) = \{ i' \in M | x_{i'} \leq x_{i}\}$,  $Top(i) = \{ i' \in M | y_{i'} \geq (y_{i}+\height(i))\}$, $Bottom(i) = \{ i' \in M | y_{i'} \leq y_{i}\}$. We consider $4$ boundary strips $S_{T,1.5\eps} := [0,N] \times [(1-1.5\eps)N, N]$, $S_{B,.5\eps} := [0,N] \times [0,.5\eps N]$, $S_{L,.5\eps} := [0,.5\eps N] \times [0,N]$, $S_{R,.5\eps} := [1-.5\eps N, N] \times [0,N]$. The set of items fully contained in and intersected by the strip $S_{X,Y}$ are denoted by $C_{X,Y}$ and $E_{X,Y}$ respectively. Also define $D_{X,Y} = E_{X,Y} \backslash C_{X,Y}$. We now consider following cases :
\\

\noindent{\em Case 1:} $D_{B,.5\eps} \cap D_{T,1.5\eps} = \phi$. \\
Define $M'=E_{T,1.5\eps}$, which can be packed in a $[0,N] \times [0,(1-.5\eps)N]$ region. This gives us our first packing which is guillotine separable as the operation performed here is just deletion of items in an already guillotine separable arrangement. For second packing we consider the items in $M\backslash (M' \cup C_{L,.5\eps} \cup C_{R,.5\eps} $. Pack $C_{L,.5\eps}$ and $C_{R,.5\eps}$ by rotating and packing them on the top of $M\backslash (M' \cup C_{L,.5\eps} \cup C_{R,.5\eps} $ in two horizontal strips of  width $.5\eps N$ each. This adds up to a packing of $M\backslash M'$ in the region $[0,N] \times [0, (1-.05\eps)N]$. The processing involves mirroring and rearrangement of {\em disjoint} sub-pieces which doesn't disturb the guillotine property.\\ 
	
\noindent{\em Case 2:} $D_{B,.5\eps} \cap D_{T,.5\eps} \neq \phi$.\\
\noindent{\em Case 2.1:}  There exists item $i$ intersecting none of $S_{L, .5\eps}$ and $S_{R, .5\eps}$. \\
W.l.o.g.~ assume $x_{i} \leq 1/2 N$. We consider completely disjoint partitions of items created by $i$, i.e., $Left(i)$, $Right(i)$, $\{i\}$, $C_{T, 1.5\eps}$ and $C_{B, .5\eps}$. Let $M'$ = $C_{T, 1.5\eps}$  $\cup$ $C_{B, .5\eps}$ $\cup Left(i)$. Consider optimal packing with just $Left(i)$, we pack  the items in $C_{T, 1.5\eps}$ and $C_{B, .5\eps}$ to the right of it by rotating them. This gives us a packing of $M'$ in a $(N \times (1-.5\eps)N)$ plane. Now we show a packing for $M\backslash M' = Right(i) \cup {i}$. From the assumption that $i$ doesn't intersect $S_{L,.5\eps}$, we trivially get a packing of $M \backslash M'$ in a $( N\times (1-.5\eps)N)$ piece. Since only operations to obtain both the packings are deletion of items from optimal guillotine packing and replacement of disjoint subpieces, we can claim that guillotine property is maintained.\\
\noindent{\em Case 2.2:}  There exists item $i$ intersecting both $S_{L, .5\eps}$ and $S_{R, .5\eps}$.\\
We define $M' = (C_{R, .5\eps} \cup C_{L, .5\eps} \cup Top(i))$. 
For packing $M'$, consider $Top(i)$ in optimal packing and rotate and pack $C_{L, .5\eps}$ and $C_{R, .5\eps}$ on the top of it.Total height of the packing is $(N-y_{i}-\height(i)+\eps N) \leq (1-\eps)N$ since $\eps \leq .1$. For packing in the second case, i.e., for packing $M\backslash M'$, since there is no massive item it follows trivially that it can packed in a $(N \times (1-.5\eps)N)$ piece. Thus we get both the packing and following the same argument as before the packings are guillotine separable.\\
\noindent{\em Case 2.3:}  There exists item $i$ intersecting both $S_{B, .5\eps}$ and $S_{T,1.5\eps}$.\\
\noindent {\em Case 2.3.1:} There exists item $i$ $\in (D_{B, .5\eps} \cap D_{T,1.5\eps} \cap D_{L,.5\eps})$ and $x_{i}+\width(i) \leq \frac{1}{2}N $ ( similar argument holds for $D_{R,.5\eps}$) ] Since there is no massive item, $i$ can intersect at most one of $S_{L, .5\eps} and S_{R, .5\eps}$. We define $M'= Right(i)$. By rotating $M'$ we get a packing in $(N\times ( 1-.5\eps)N)$  piece. Now we devise a packing for second set $M\backslash M'$. Consider packing of $M \backslash ( C_{T, 1.5\eps}$  $\cup$ $C_{B, .5\eps}$ $\cup Right(i)$ as in optimal packing and pack $C_{T, 1.5\eps}$ and $C_{B, .5\eps}$ to the right of it by rotating them and packing in two vertical strips of $1.5\eps$ and $.5\eps N$ widths respectively. This gives us the total width of the packing as less than or equal to $(1/2 + 2\eps)N \leq (1-.5\eps)N$ since $\eps \leq .1$ from our initial assumption. Again the only operations during entire processing of both the packings are deletion of items from optimal guillotine packing and replacement of disjoint sub-pieces.\\
\noindent{\em Case 2.3.2:}  There exists item $i$ $\in (D_{B, .5\eps} \cap D_{T,1.5\eps} \cap D_{L,.5\eps})$ and $x_{i}+\width(i) > \frac{1}{2}N $ ( similar argument holds for $D_{R,.5\eps}$ ). \\
Define $M'= Left(i) \cup {i}$. Consider the packing of $M'$ in optimal packing, which clearly gives us a packing in a $(N\times (1-.5\eps)N)$. Now we define second packing for items in $M\backslash M'$. Consider the packing of  $M \backslash ( C_{T, 1.5\eps}$  $\cup$ $C_{B, .5\eps}$ $\cup M'$ as in optimal packing and pack $C_{T, 1.5\eps}$ and $C_{B, .5\eps}$ to the left of it by rotating them and packing in two vertical strips of $1.5\eps N$ and $.5\eps N$ widths respectively. This gives us the total width of the packing as less than or equal to $(1/2 + 2\eps)N \leq (1-.5\eps)N$ since $\eps \leq .1$. Sole operations involved are deletion of items from already guillotine separable packing and replacement of disjoint pieces. thus maintaining guillotine separability.\\
\noindent{\em Case 2.3.3:} There exists no item $i$ $\in (D_{B, .5\eps} \cap D_{T,1.5\eps} \cap (D_{L,.5\eps} \cup D_{R,.5\eps}))$.\\
W.l.o.g.~let $i \in C_{L,.5\eps}$. We define $M'=E_{T,1.5\eps} \backslash (C_{L,.5\eps} \cup C_{R,.5\eps})$, which clearly gives us a packing in a $(N\times (1-.5\eps)N)$. Consider $M \backslash (M' \cup  C_{L, .5\eps} \cup C_{R, .5\eps}$ in optimal packing and rotate and pack $C_{L, .5\eps}$ and $C_{R, .5\eps}$ on the top of it. Total height of the packing is at most $ (1-\eps)$. Operations involved in are deletion of items from already guillotine separable packing and replacement of disjoint pieces. thus maintaining guillotine separability.
\end{proof}

%
%We the use the corridor partitioning as in section \ref{subcorr}. Consider the set of small items $\opt_{small}$ as the set of small items in $C(k)$ i.e. $\opt_{small}(C(k))$. We class items in the same fashion as in section \ref{profitstruc}.
 %Hence we prove that Lemmas \ref{sumprofit}, \ref{algo1}, \ref{idea} are also applicable in the weighted case. We extend Lemma \ref{algo2} to weighted case by considering items in $OPT_{small}$ while processing. Since every small item is cut by the vertical ( or horizontal ) strip with probability $O(\eps)$, we can follow the same processing as in \ref{algo2}. Combining results in Lemmas \ref{algo2}, \ref{sumprofit}, \ref{algo1}, \ref{idea}, we get the same factor of
% $10/7$ i.e.
% $\profit(OPT_{L\&C})$
% $\geq$ $ (10/7+O(\eps))\profit(OPT)$ for wieghted case.
%\section{Weighted Non-Rotated case}\label{w2dgk}
%	\subsection{Shifting Argumentation\cite{GalvezGHI0W17}}\label{shifting}
%	We use similar process as used as in \cite{GalvezGHI0W17} and prove that if we begin with a guillotine separable solution, the process results in a final guillotine separable arrangement.
%		\subsubsection{Grid and Corridor Partition}\label{gridpartition}
%		In this section we try to recursively divide the knapsack into a non-uniform grid, stretch it to make it a uniform grid. We then sacrifice a 
%		small fraction of intercepted items and perform corridor partition to the remaining set of items. The corridor partition follows similar to 						section \ref{subcorr}. Consider the set of items $\kappa(t)$ at $t^{th}$ iteration as the items forming the grid. The grid at any such level of iteration is formed by extending the edges of all the items in $\kappa(t)$. We initiate $\kappa(0)$ with the items in $OPT_{large}$ $\cup$ $OPT_{corr}^{cross}$ $\cup$  $OPT_{kill}$ as defined in section \ref{profitstruc}. We recursively augment items packed at each iteration to $\kappa(t)$.  We also define a set $K(t+1)$ which contains all the items killed at $t^{th}$ iteration during the process. \\
%Consider the set $C_{t}$ of all grid cells at $t^{th}$ iteration. Same as in lemma \ref{class} we classify the items in cells as $OPT_{small}(C)$, $OPT_{large}(C)$, $OPT_{hor}(C)$, $OPT_{ver}(C)$, $OPT_{intermediate}(C)$. The lemma lets us drop $\eps$ fraction profit $OPT_{intermediate}(C)$ items in every cell. We then kill all the $OPT_{large}(C)$ in every cell $C$ $\in$ $C_{t}$. The killed rectangles are added to $K(t+1)$. We then stretch the grid to a uniform grid throughout the knapsack. Using processes in section \ref{subcorr} we obtain the corridor decomposition of the knapsack with the set of all skew items with $O_{\eps,\eps_{large},\kappa(t)}(1)$ corridors. The decomposition is equivalent to the decomposition of the original knapsack and we get the same set of killed items in both the cases. Since only a $O_{\eps}(1)$ items $OPT_{cross}$ are killed in the corridor decomposition. We add items in $OPT_{cross}$ and items not in $\kappa(t)$ to the set $K(t+1)$. Next we state the following lemma.
%\begin{lem}\cite{GalvezGHI0W17}\label{focsagain}
%	Let $S$ be an open corridor with $b(S)$ bends. Let $I'$ $\subseteq$ $OPT$be a collection of items which intersect the boundary of $S$ with $I'\bigcap OPT_{skew}(C_{t}) = \phi$. Then there is a collection of $|I'|.b(S)$ line segments $L$ within $S$ which partition $S$ into subcorridor with at most $b(S)$ bends each such that no item from $I'$ is intersected by $L$ and there are at most $O_{\eps}(|I'|.b(S))$ items of $OPT_{skew}(C_{t})$ intersected by line segments in $L$.
%\end{lem}
%\begin{lem}\cite{GalvezGHI0W17}\label{againfocs}
%Let $S$ be a closed corridor with $b(S)$ bends. Let $OPT_{skew}(S)$ denote the items in $OPT_{skew}(C_{t})$ that are contained in $S$. Let $I'$ $\subseteq$ $OPT$ be a collection of items which intersect the boundary of $S$ with  $I'\bigcap OPT_{skew}(C_{t}) = \phi$. Then there is a collection of $O_{eps}(\frac{|I'|^{2}}{\eps})$ line segments $L$ within $S$ which partition $S$ into a collection of closed corridors with at most $\frac{1}{\eps}$ bends each and possibly an open corridor with $b(S)$ bends such that no item from $I'$ is intersected by $L$ and there is a set of items $OPT'_{skew}(S) \subset OPT_{skew}(S)$ with $|OPT'_{skew}(S)|\leq O_{\eps}(|I'|^{2})$ such that the items in $OPT_{skew}(S) \backslash OPT'_{skew}(S)$ intersected by the line segments in $L$ have a total profit of at most $O(\eps).\profit(OPT_{skew}(C_{t}))$.
%\end{lem}
%Using Lemmas \ref{focsagain} and \ref{againfocs} we partition the piece in $O_{\eps}(1)$ corridors (open and closed) packing all the items in $OPT_{skew}(S)$ $\backslash$ $OPT'_{skew}(S)$. We augment the remaining set of items $OPT'_{skew}(S)$ with small profit to $K(t+1)$.
%\begin{remark}
%Guillotine Separability : All the processes used to obtain the bends and corridor decomposition follow deleting of items only. Thus the remaining subset of items should be guillotine separable given that the initial packing was guillotine separable.
%\end{remark}
%		\subsubsection{Box Partition}\label{boxpart}
%			We follow the same process as in original corridor decomposition section \ref{subcorr}. We divide the subcorridor into strips and then classify the items as $fat$ lying completely inside these strips. We call the set of items in this optimal packing as $OPT_{fat}$. Then by simple shifting argument, we pack the items in the strips killing $OPT_{kill}$ items in the process. We add all the items in $OPT_{kill}$ into $K(t+1)$ which actually refers to the items killed in the $t^{th}$ iteration. From section \ref{subcorr} it follows that only $O_{\eps,\eps_{large},\eps_{box}}(1)$ of items are killed in partition of subcorridors to boxes. Also the items killed do not belong to the set $\kappa(t)$.
%			\begin{remark} 
%			Guillotine Separability : Since items the division of subcorridors into boxes involves partition of subcorridor with lines. We remove all the items killed by these lines and pack the rest completely into the strips formed. The strips can be themselves separated by the same set of lines. Also since we begin from a guillotine separable arrangement, shifting the horizontal ( resp. vertical) items vertically ( resp. horizontally ) doesn't disturb the guillotine property. Thus guillotine separability is maintained after the processing of subcorridors into boxes. 
%			\end{remark}
%		\subsubsection{Container Partition}
%		We follow resource augmentation from Lemma \ref{lemma1}. The process borrows technique from process of partitioning box into containers from section \ref{subcorr}. We classify an item as $OPT_{small}(C_{t}))$ if for every cell $C$ in $C_{t}$ intersecting with the item,  the item is classified as $OPT_{small}(C)$. In other words any item which is small in all the cells intersecting it, is classified as $OPT_{small}(C_{t})$. Now consider a horizontal box, using averaging argument there exits a strip with width $3\eps$ such that it intersects with items with total profit less than or equal to $O(\eps)\profit(OPT_{box})$. We neglect the small items intercepted by the strip for now and pack them pack in section \ref{smallitems}. Let the items killed be $OPT_{kill,box}$, We add items in $OPT_{kill,box}$ to the set of items killed in the $t^{th}$ iteration, i.e., $K(t+1)$. We then apply resource augmentation to the set of remaining small items say $OPT_{small}(C_{t})$ and pack subset $OPT'_{small}(C_{t})$. We then pack profitable subsets $OPT'_{skew}(C_{t})$ $\subset$ $OPT_{skew}(C_{t})$ and $OPT'_{small}(C_{t})$ $\subset$ $OPT_{small}(C_{t})$ of items using $L\&C$ packing as in section \ref{lc}. The subsets are such that only $O(\eps)$ factor of profit is lost. 
%			\begin{remark}
%			Guillotine Separability : The only process we do in this section is deleting some items intersecting a strip. Since deleting items doesn't affect guillotine separability as the remaining items need to guillotine separable if the original arrangement is guillotine separable. Thus we get a guillotine separable arrangement after doing the processing as given in this section.
%			\end{remark}
%		\subsubsection{Packing Small Items}\label{smallitems}
%			Now we repack the small items killed in lines by corridor decomposition in section \ref{boxpart}. Consider the set $OPT_{skew,killed}(C_{T})$ as the given set of items. We assign each item in $OPT_{skew,killed}(C_{T})$ to the cell it was contained maximally in the original packing. Consider a cell $C$ and the items assigned to $C$ as $OPT_{skew,killed}(C)$. By wisely choosing the factor $\eps_{small}$ we can force area of small items assigned to $C$, i.e.,  $a(OPT_{skew,killed}(C))$ to be at most $\eps a(C)$. This follows from the fact that number of items intersecting $C$ would be $O_{\eps,\eps_{large}}(1)$. Thus by using %\ref{smallpacking} and 
%\ref{areafocs}
% we can pack a profitable fraction items  $OPT'_{skew,killed}(C)$ $\subset$  $OPT_{skew,killed}(C)$ such that $\profit(OPT_{skew,killed}(C)) \geq (1-O(\eps)) \profit(OPT_{skew,killed}(C))$.
%			\begin{lem}\cite{GalvezGHI0W17}\label{areafocs}
%				Let $C$ be a cell. The total area of $C$ occupied 	by containers is at most $(1-2\eps)a(C)$.
%			\end{lem}
%			\begin{remark}
%				Guillotine Separability : The processing in the section involves deleting a subset of rectangles which doesn't affect the guillotine separability of items. We use NFDH to pack the items in the cells. Since NFDH is 2-stage guillotine separable packing, inside each cell items are guillotine separable. If we consider each cell as a pseudo-item, we claim that the whole knapsack is guillotine separable. The claim follows from the fact that cells are formed from extending the edges in $\kappa(T)$. The guillotine cuts will always follow the corresponding edges of items. Thus the arrangement in whole after the processing is guillotine separable. 
%			\end{remark}
%		\subsubsection{L$\&$C Packing}\label{lc}
%			Following the same iterative process we get $k$ subsets; $K(1), K(2),... K(k-1), K(k)$ such that $k\leq\frac{1}{\eps}$ and $\profit(K(k))$ $\leq$ $\eps OPT$. We consider the cutting of piece, say $C(k)$, by extending the edges of items in $K(k-1)$. 
%We the use the corridor partitioning as in section \ref{subcorr}. Consider the set of small items $OPT_{small}$ as the set of small items in $C(k)$ i.e. $OPT_{small}(C(k))$. We class items in the same fashion as in section \ref{profitstruc}.
% Hence we prove that Lemmas \ref{sumprofit}, \ref{algo1}, \ref{idea} are also applicable in the weighted case. We extend Lemma \ref{algo2} to weighted case by considering items in $OPT_{small}$ while processing. Since every small item is cut by the vertical ( or horizontal ) strip with probability $O(\eps)$, we can follow the same processing as in \ref{algo2}. Combining results in Lemmas \ref{algo2}, \ref{sumprofit}, \ref{algo1}, \ref{idea}, we get the same factor of
% $10/7$ i.e.
% $\profit(OPT_{L\&C})$
% $\geq$ $ (10/7+O(\eps))\profit(OPT)$ for wieghted case.
%\begin{remark}
%Guillotine Separability : In the given section we use results and lemmas from previous sections which are already established to maintain guillotine separability. Another processing done is deleting of items intersecting with the strip, since deleting items doesn't disturb guillotine cuts we have a guillotine separable packing as a result.
%\end{remark}

==> Body4-old.tex <==
\section{BL-arrangement for guillotine packing} 
\label{sec:bldecom}
Now we show the existence of a guillotine packing where all items are packed into $\Bc$ or $\Lc$ corridors.
\begin{thm}[$\Bc \Lc$-arrangement]
\label{thm:ldecom}
Given an optimal guillotine packing, there is a rearrangement of items into another guillotine packing and $\optco \subseteq \optsk$ such that:
\begin{enumerate}\itemsep0pt
\item there is a subset $\optco^{cross} \subseteq \optco$ with  $|\optco^{cross}| \le O_\eps(1)$ such that  each $i\in \optco \setminus \optco^{cross}$ is fully contained in some corridor,
\item $\profit(\optco) \ge (1-O(\eps))\profit(\optsk)$,
\item the number of corridors is $O_{\eps,\epsl}(1)$ and each corridor is either $\Bc$ or $\Lc$ corridor of width at most $\epsl N$. Every $\Lc$-corridor is a boundary-$\Lc$ for some bounding box and every $\Bc$-corridor is guillotine separable as a box. 
\end{enumerate}
\end{thm}		
	
To prove the theorem, first we will start with the corridor decomposition from Lemma \ref{lem:corridorPack} (see Figure \ref{fig:3a}). Then we remove $\Zc$-bends to obtain only spiral corridors  (see Figure \ref{fig:3b}). Thereafter, we will further rearrange to obtain only $\Bc, \Lc, \Uc, \Gc$ corridors (see Figure \ref{fig:3c}). Finally, we will rearrange further to obtain only {\em special} $\Lc$ or $\Bc$ corridors (see Figure \ref{fig:3f}). 

\begin{lem}\label{noz}
A corridor with one or more $\Zc$-bends can be partitioned into $O_{\eps}(1)$ spiral corridors  by removing $O_{\eps,\epsl}(1)$ items, maintaining guillotine separability.
\end{lem}
\begin{proof}
There are two cases. 

\noindent \textit{Case 1: $C$ is an open corridor with at least one $\Zc$-bend.} 
Assume  $C$ has 5 subcorridors (also works for fewer subcorridors) $S_{i'+1}, S_{i'+2}, S_{i'+3}, S_{i'+4}, S_{i'+5}$ such that $\{S_{i'+2},S_{i'+3},S_{i'+4}\}$ form a $\Zc$-bend. W.l.o.g.~assume $S_{i'+3}$ be a horizontal subcorridor and $S_{i'+2}$ be situated to the top left of $S_{i'+3}$ (see Figure \ref{fig:kbend}). Let us consider a sequence of guillotine cuts through these five subcorridors.
Consider the unshared region of $S_{i'+3}$: $\overline{S_{i'+3}}:= S_{i'+3}$ $\setminus \{S_{i'+2} \cup S_{i'+4}\}$. Then from Observation \ref{endtoend}, there exists an end-to-end cut $l'$ in $\overline{S_{i'+3}}$. 

If this cut $l'$ through $\overline{S_{i'+3}}$ is vertical, then we can partition $C$ along $l'$ into $2$ new corridors, each containing at least one lesser $\Zc$-bend, compared to $C$.
 
If the cut $l'$ is horizontal, then consider the guillotine cuts which occurred before the cut $l'$. Let $l_{i'+2}$ be the rightmost vertical cut (including those which pass through the vertical boundary of $S_{i'+2}$, if any) through $S_{i'+2,i'+3}$. 
Extend the cut $l_{i'+2}$ so that it touches the boundary curve between $S_{i'+1}$ and $S_{i'+2}$ at point $p$. Now draw a line $l_{i'+1}$ from point $p$ parallel to the orientation of $S_{i'+1}$ till it touches the boundary curve between $S_{i'+1}$ and $S_{i'}$. Continue the same process by drawing lines $l_{j}$ through corridors $S_{j}$, where $1 \leq j \leq i'$, in a similar fashion. 
Drop items that are cut by these lines.
Stop  when we obtain a line $l_{t}$ through $S_{t}$ parallel to the orientation of $S_{t}$, $t\ge 1$,  that reaches a boundary edge of $C$.   Lines $\{l_{t},l_{t+1}, \dots ,l_{i'+2}\}$ partition the corridor $C$ into at most 2 smaller corridors $C_{1},C_{2}$ as shown in Figure \ref{fig:kbend}. $C_{1}$ contains rectangles from the subcorridors $S_{t}, \dots,S_{i'+2}$ only. $C_{2}$ contains rectangles from the subcorridors $S_{1}, \dots,S_{k}$. In a similar way, we choose $l_{i'+4}$ be the leftmost vertical cut through $S_{i'+3,i'+4}$ and  we can partition $C_{2}$ into at most 2 corridors $C_{3}$ and $C_{4}$ where $C_{3}$ contains rectangles from the subcorridors $S_{i'+4}, \dots,S_{t'}$ for $t' \le k$ and $C_{4}$ contains rectangles from the subcorridors $S_{1}, \dots,S_{k}$. During this process of partitioning we drop at most $O_{\eps,\epsl}(1)$ rectangles (these are also included in $\optco^{cross}$), as at most $\frac{1}{\epsl}$ items are dropped in at most $\frac{1}{\eps}$ subcorridors. Note that $l'$ divides  $C_{4}$ into 2 new corridors containing at least one lesser $\Zc$-bend when compared to $C$. The reason for choosing $l_{i'+2}$ (resp.~$l_{i'+4}$) and extending it to partition the corridor $C$ is that $l_{i'+2}$ (resp.~$l_{i'+4}$)  is the cut which intercepts the horizontal cut $l'$ in  $S_{i'+2,i'+3}$ (resp.~$S_{i'+3,i'+4}$) . 

Repeating the above procedure for all $\Zc$-bends concludes the proof for this case.


\noindent \textit{Case 2: $C$ is a closed corridor with at least one $\Zc$-bend.}  Let $S_{L}$ (resp. $S_{B}$, $S_{R}$, $S_{T}$)  be the leftmost vertical (resp. bottom-most hor., rightmost vert., topmost hor.) subcorridor in $C$.  
These four subcorridors can form following types of corridors among themselves: (i) one $\Gc$ (Figure \ref{fig:zbend1}), (ii) two $\Lc$ (Figure \ref{fig:zbend}), (iii) one $\Uc$ and one $\Bc$ (Figure \ref{fig:zbend3}), (iii) one $\Lc$ and two $\Bc$ (Figure \ref{fig:zbend2}) and (v) four $\Bc$ (Figure \ref{fig:zbend4}). 
We  call a cut to be a {\em good cut} if it passes through the unshared region of subcorridor perpendicular to its orientation.
A good guillotine cut divides a corridor into $O_{\eps}(1)$ open corridors  which can then be handled as in Case 1 (see Figure \ref{fig:zbend}). 
Now, consider the sequence of guillotine cuts in the smallest piece containing $C$. If there is a good guillotine cut, we stop the sequence of guillotine cuts and we are done as we get $O_\eps(1)$ open corridors. Else from Observation 
\ref{endtoend}, we get an end-to-end cut passing through one of the subcorridors $\{S_{L}, S_{B}, S_{R}, S_{T}\}$, parallel to the orientation of the subcorridor. 
We continue separating items from these four subcorridors $\{S_{L},S_{B},S_{R},S_{T}\}$ according to these end-to-end cuts, till either (i) we get a good cut or (ii) all the rectangles from one of these four subcorridors get completely separated from the rest. We now create at most 4 spiral corridors containing items from subcorridors $\{S_{L}, S_{B}, S_{R}, S_{T}\}$ only by using the last cut (excluding the good cut) in each of the subcorridors $\{S_{L}, S_{B}, S_{R}, S_{T}\}$.
In the first case, we separate out the rectangles from these 4 subcorridors into the newly created $O(1)$ spiral corridors with at most three bends and then using the good cut we divide rest of the closed corridor into $O_\eps(1)$ open corridors as shown in Figure \ref{fig:zbend} and Figure  \ref{closedcor2}.
In the second case, if we don't have such a good cut then eventually all the items in one of the subcorridors  $\{S_{L},S_{B},S_{R},S_{T}\}$ will have been separated out (we say that the subcorridor is {\em exhausted}) into the newly created $O(1)$ spiral corridors with at most $4$ bends. W.l.o.g.~assume that the subcorridor $S_{B}$ gets exhausted. Then the last cut through $S_{B}$ leaves us with $O(1)$ open corridors (see Figure \ref{fig:zbend2}). The open corridors are again dealt using Case 1, finally giving $O_{\eps}(1)$ spiral corridors.
\end{proof}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{1\textwidth}
		\centering
		\resizebox{!}{4.3 cm}{
		\begin{tikzpicture}
						\draw[thick] (0,6)--(2,6)--(2,5.5)--(4,5.5)--(4,6)--(6,6)--(6,4)--(5,4)--(5,3)--(4.5,3)--(4.5,4.5)--(5.5,4.5)--(5.5,5.5)--(4.5,5.5)--(4.5,5)--(1.5,5)--(1.5,5.5)--(.5,5.5)--(.5,4)--(2,4)--(2,3)--(4,3)--(4,2.5)--(1.5,2.5)--(1.5,3.5)--(0,3.5)--(0,6);		
						
						\draw[dotted] (6,4)--(5.5,4.5);
						\draw[dotted] (5,4)--(4.5,4.5);
						\draw[red] (6,6)--(5.9,6)--(5.9,5.9)--(5.8,5.9)--(5.8,5.8)--(5.7,5.8)--(5.7,5.7)--(5.6,5.7)--(5.6,5.6)--(5.5,5.6)--(5.5,5.5);
						\draw[dotted] (4,6)--(4.5,5.5);
						\draw[dotted] (2,6)--(1.5,5.5);
						\draw[red] (0,6)--(.1,6)--(.1,5.9)--(.2,5.9)--(.2,5.75)--(.25,5.75)--(.3,5.75)--(.3,5.67)--(.5,5.67)--(.5,5.6)--(.5,5.5);
						\draw[dotted] (0.25,3.6)--(.5,4);
						\draw[dotted] (1.5,2.5)--(2,3);
						\draw[dotted] (1.5, 3.5)--(2,4);
						\draw[dotted] (1.5, 5)--(2,5.5);
						\draw[dotted] (4.5 , 5)--(4,5.5);


						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.4,3.5);	\draw (-.75,3.5) node {\textbf{$l_{i'+2}$}};
						\draw[->] (.25,5.75) edge[out=180,in=0,->] (-.4,5.4);	\draw (-.6,5.4) node {\textbf{$p$}};
						\draw[->] (1,5.75) edge[out=90,in=0,->] (.8,6.5);	\draw (.5,6.5) node {\textbf{$l_{i'+1}$}};
						%\draw (1.75,5.25) node {\textbf{$l_{1}$}};
						%\draw (4.25, 5.25) node {\textbf{$l_{2}$}{spialgo}};
						%\draw[->] (5,5.75) edge[out=180,in=0,->] (4.75,6.5);	\draw (4.5,6.5) node {\textbf{$l$}};%
%						\draw[->] (5.75,5) edge[out=180,in=0,->] (6.5,5);	\draw (6.5,5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
						\fill [lightgray] (0,3.5) rectangle (0.5,4);
						\draw[->] (.2,3.75) edge[out=180,in=0,->] (-.4,2.5);	\draw (-.75,2.5) node {\textbf{$S_{i'+2,i'+3}$}};
						\draw[dashed] (4.75,3) -- ( 4.75 ,4.25) -- ( 5.75, 4.25) -- ( 5.75, 5.75) -- ( 4.25, 5.75) -- ( 4.25, 5.25) -- ( 1.75, 5.25) -- ( 1.75, 5.75) -- (.25, 5.75) -- (.25, 3.5) ;	
						\draw(4.75,2.7) node {\large \textbf{$S_{1}$}};
						\draw(.75,3.8) node {\large \textbf{$l'_{H}$}};
						\draw(1.2,4.7) node {\large \textbf{$l'_{V}$}};
						%\draw (5,4.75) node {\large \textbf{$C$}};
						%\draw (4,3) node {\large \textbf{$B$}};

						\draw [thick, blue] (.25,3.5)--(.25,5.75);
						\draw [thick, blue] (1.75,4)--(1.75,2.5);
						\draw[thick, green] (.25,3.6)--(1.75,3.6);
						\draw[thick, brown] (1.2,4.5)--(1.2,3);
		
		\end{tikzpicture}}
		\caption{Removal of $\Zc$-bend in an open corridor. $l_{i'+2}$, $l_{i'+4}$ are shown in blue. Vertical (resp.~horizontal) (if any) $l'$ is shown as $l'_{V}$(resp.~$l'_{H}$), boundary curves are shown in red or dotted.
		$l'$ separates the corridors into two corridors with lesser $\Zc$-bends.}
		\label{fig:kbend}
	\end{subfigure}

	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.5cm}{
		\begin{tikzpicture}
						\draw[thick, fill =lightgray] (0,7)--(2,7)--(2,4)--(7,4)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw [solid, fill=white] (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7) --(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						%\draw[fill=white] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3)--(.5,3);
						%\draw[fill=white] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
						%\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						%\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
						
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};


						\draw[dashed] (5.6,.5)--(5.6,4);
						\draw[dashed] (5,.5)--(6.7,.5);
						\draw[dashed] (6.5,.5)--(6.5,4);
						\draw[dashed] (.5,3)--(.5,6.5);
						\draw[dashed] (.3,6.5)--(2,6.5);
						\draw[dashed] (5,.3)--(6.9,.3);
						\draw[dashed] (6.7,.3)--(6.7,4);
						\draw[dashed] (.3,3)--(.3,6.7);
						\draw[dashed] (.1,6.7)--(2,6.7);
						\draw[dashed] (5,.1)--(7,.1);
						\draw[dashed] (6.9,.1)--(6.9,4);
						\draw[dashed] (.1,3)--(.1,6.9);
						\draw[dashed] (0,6.9)--(2,6.9);
		\end{tikzpicture}}
		\caption{A sequence of guillotine cuts (shown as dashed lines) until we get a good cut}
		\label{fig:zbend-lines}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{3.5cm}{
		\begin{tikzpicture}
						\draw[thick, fill =lightgray] (0,7)--(2,7)--(2,4)--(7,4)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw [solid, fill=white] (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7) --(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[fill=white] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3)--(.5,3);
						\draw[fill=white] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
					
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};


						\draw[thick] (5.6,.5)--(5.6,4);
	
		\end{tikzpicture}}
		\caption{A good cut is shown by bold line. Shaded regions show two $\Lc$ corridors created before we obtained the good cut.}
		\label{fig:zbend}
	\end{subfigure}
	\caption{}
\end{figure}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.25\textwidth}
		\centering
		\resizebox{!}{3.3cm}{
		\begin{tikzpicture}
						\draw[thick] (0,7)--(7,7)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);

						\draw[fill=lightgray] (0,7)--(7,7)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);	
						\draw[fill=white] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,0.5)--(5,0.5)--(5,0)--(7,0)--(7,7)--(0,7)--(0,3)--(.5,3);
						\draw [fill=white]  (.75,6.25)--(6.25,6.25)--(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,0.5)--(5,0.5)--(5,0)--(7,0)--(7,7)--(0,7)--(0,3)--(.5,3);
						
					
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};
						\draw[thick] (5.6,.5)--(5.6,6.5);
						
	
		\end{tikzpicture}}
		\caption{One $\Gc$ corridor created before we obtain a good cut.}
		\label{fig:zbend1}
	\end{subfigure}
	\begin{subfigure}[b]{.25\textwidth}
		\centering
		\resizebox{!}{3.3cm}{
		\begin{tikzpicture}
						\draw[fill=lightgray] (0,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw[fill=white]  (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[fill=white] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[fill=white] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[fill=white] (5,.75)--(6.25,.75)--(6.25,0)--(5,0)--(5,.75);
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[pattern=north west lines, pattern color=gray] (5,.75)--(6.25,.75)--(6.25,0)--(5,0)--(5,.75);
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};
						

						
	
		\end{tikzpicture}}
		\caption{One $\Lc$, two $\Bc$ corridors created before corridor $S_B$ gets exhausted.}
		\label{fig:zbend2}
	\end{subfigure}
	\begin{subfigure}[b]{.25\textwidth}
		\centering
		\resizebox{!}{3.3cm}{
		\begin{tikzpicture}
						\draw[thick, fill= lightgray] (0,7)--(7,7)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw [fill=white]  (.75,6.25)--(6.25,6.25)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[fill=white] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,2)--(7,2)--(7,7)--(0,7)--(0,3);
						\draw[fill=white] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,2)--(7,2)--(7,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
					
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};
						\draw[thick] (5.6,.5)--(5.6,6.5);
						
	
		\end{tikzpicture}}
		\caption{One $\Uc$ and one $\Bc$ corridor created before we obtain a good cut.}
		\label{fig:zbend3}
	\end{subfigure}
\begin{subfigure}[b]{.25\textwidth}
		\centering
		\resizebox{!}{3.3cm}{
		\begin{tikzpicture}
						\draw[thick, fill=lightgray] (0,5)--(0.75,5)--(0.75,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,5);
						\draw[fill=white]  (.75,4.5)--(1.25,4.5)--(1.25,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,4.5); 
						\draw[fill=white] (.5,3)--(.5,5)--(0,5)--(0,3);
						\draw[fill=white] (0.75,6.5)--(2,6.5)--(2,7)--(0.75,7)--(0.75,6.5);
						\draw[fill=white] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[fill=white] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,5)--(0,5)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (0.75,6.5)--(2,6.5)--(2,7)--(0.75,7)--(0.75,6.5);
						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};
						\draw[thick] (5.6,.5)--(5.6,4);						

						
	
		\end{tikzpicture}}
		\caption{Four $\Bc$ corridors created before we obtain a good cut.}
		\label{fig:zbend4}
	\end{subfigure} 
	\caption{Good cuts are shown as bold lines.}\label{closedcor2}	
\end{figure}

\begin{cor}
Every closed corridor obtained after the processing in Lemma \ref{noz}, is a {\em ring}.
\end{cor}

%%%%%%%%%%%%%% Fig
%%%%%%%%%%%%%%

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
		\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{2.5cm}{
		\begin{tikzpicture}
			\draw[solid, fill=lightgray] (5.3,5.4) rectangle (5.4,5.5);
			\draw[solid, fill=lightgray] (5.5,5.1) rectangle (4.7,5.2);	
			\draw[solid, fill=lightgray] (.7,5.4) rectangle (0.6,5.5);
			\draw[solid, fill=lightgray] (.6,5.1) rectangle (1.4,5.2);
			\draw[solid, fill=lightgray] (5.2,.8) rectangle (5.8,0.7);
			\draw[solid, fill=lightgray] (5.7,.6) rectangle (5.5,.5);	
			\draw[solid, fill=lightgray] (.7,.6) rectangle (0.6,0.5);
			\draw[solid, fill=lightgray] (.8,.8) rectangle (0.2,0.7);

			\draw[solid, fill=lightgray] (0,6.8) rectangle (5.5,6.7);
			\draw[solid, fill=lightgray] (0,-0.7) rectangle (5.5,-0.8);
			\draw[solid, fill=lightgray] (-0.7,0) rectangle (-0.8,6);
			\draw[solid, fill=lightgray] (6.7,0) rectangle (6.8,6);	
			\draw[solid, fill=lightgray] (0,6.3) rectangle (5.5,6.2);
			\draw[solid, fill=lightgray] (0,-0.2) rectangle (5.5,-0.3);
			\draw[solid, fill=lightgray] (-0.2,0) rectangle (-0.3,6);
			\draw[solid, fill=lightgray] (6.2,0) rectangle (6.3,6);	
			\draw[solid, fill=lightgray] (3.5,1.5) rectangle (3,1);
			\draw[solid, fill=lightgray] (3.5,5) rectangle (3,4.5);
						


			\draw[solid, fill=lightgray] (1.8,5.35) rectangle (4.2,5.5);
			\draw[solid, fill=lightgray] (2,5.15) rectangle (4.2,5.3);
			\draw[solid, fill=lightgray] (1.67,4.45) rectangle (1.85,5.3);
			\draw[solid, fill=lightgray] (1.95,4.45) rectangle (2.1,5.1);
			\draw[solid, fill=lightgray] (3.97,4.45) rectangle (4.15,5.1);
			\draw[solid, fill=lightgray] (4.25,4.45) rectangle (4.35,5.5);

			\draw[solid, fill=lightgray] (1.8,.65) rectangle (4.2,.5);
			\draw[solid, fill=lightgray] (2,.85) rectangle (4.2,.7);
			\draw[solid, fill=lightgray] (1.67,1.55) rectangle (1.85,.7);
			\draw[solid, fill=lightgray] (1.95,1.55) rectangle (2.1,.9);
			\draw[solid, fill=lightgray] (3.97,1.55) rectangle (4.15,.9);
			\draw[solid, fill=lightgray] (4.25,1.55) rectangle (4.35,.5);

			\draw[solid, fill=lightgray] (1.5,3.65) rectangle (4.7,3.77);
			\draw[solid, fill=lightgray] (1.5,3.95) rectangle (4.9,4.2);
			\draw[solid, fill=lightgray] (1.5,4.1) rectangle (5.2,4.35);
			\draw[solid, fill=lightgray] (1.4,3.5) rectangle (4,3.4);
			\draw[solid, fill=lightgray] (1.6,3.4) rectangle (4,3.3);
			\draw[solid, fill=lightgray] (2.6,3.2) rectangle (4,3);
			\draw[solid, fill=lightgray] (4.1,3.2) rectangle (4.2,2.7);
			\draw[solid, fill=lightgray] (2.6,2.6) rectangle (4,2.7);
			\draw[solid, fill=lightgray] (2.6,2.5) rectangle (4,2.6);
			\draw[solid, fill=lightgray] (4.3,3.2) rectangle (4.4,2.7);
			\draw[solid, fill=lightgray] (4.6,3.2) rectangle (4.7,2.7);				
			\draw[solid, fill=lightgray] (1.7,3.2) rectangle (1.8,2.7);
			\draw[solid, fill=lightgray] (1.5,3.2) rectangle (1.6,2.7);
			\draw[solid, fill=lightgray] (1.2,3.2) rectangle (1.3,2.7);
			\draw[solid, fill=lightgray] (1.2,3.3) rectangle (1.3,3.4);		

			\draw[solid, fill=lightgray] (.5,3.1) rectangle (.7,3.6);
			\draw[solid, fill=lightgray] (.8,3.1) rectangle (1,3.6);
			\draw[solid, fill=lightgray] (5.5,4.2) rectangle (5.3,1.8);
			\draw[solid, fill=lightgray] (5.2,3.6) rectangle (5,2.4);
			\draw[solid, fill=lightgray] (1,1.7) rectangle (4,1.8);
			\draw[solid, fill=lightgray] (0.5,1.7) rectangle (0.6,2.7);
			\draw[solid, fill=lightgray] (1,0.25) rectangle (4,0.35);
			\draw[solid, fill=lightgray] (1,5.75) rectangle (4,5.85);
			\draw[solid, fill=lightgray] (0.25,2) rectangle (0.35,4);
			\draw[solid, fill=lightgray] (5.65,2) rectangle (5.75,4);
			\draw[ ultra thick](-1,-1) rectangle (7,7);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			\draw[ultra thick] (1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);
			
			%\draw[ultra thick,brown] (.5,5.6)--(.5,4.4);
			%\draw[ultra thick,brown] (5.5,5.6)--(5.5,4.4);
			%\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			%\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			%\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			%\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			%\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			%\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			%\draw[ultra thick,brown] (.2,.4)--(.8,.4);
			%\draw[ultra thick,blue] (.8,.4)--(1,.4);
			%\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);
			%\draw[ultra thick,brown](5,.2)--(5,0);
			%\draw[ultra thick,blue]( 5,1.2)--(5,1.6);
			%\draw[ultra thick,red] (-.5,-1)--(-.5,7);
			%\draw[ultra thick,red] (6.5,-1)--(6.5,7);
			%\draw[ultra thick,red] (-.5,6.5)--(6.5,6.5);
			%\draw[ultra thick,red] (-.5,-0.5)--(6.5,-0.5);

			%\draw[ultra thick,red] (1.6,3.2)--(2.4,3.2);
			%\draw[ultra thick,red] (1.2,3.6)--(1.2,4.4);
			%\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			%\draw[ultra thick,brown] (0,5.6)--(6,5.6);
			%\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			%\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			%\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			%\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			%\draw[ultra thick,brown] (1,1.6)--(1,0);
			%\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			%\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.4);
			

		\end{tikzpicture}}
		\caption{}
		\label{fig:3a}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{2.5cm}{
		\begin{tikzpicture}
			\draw[ultra thick](-1,-1)rectangle(7,7);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			\draw[ultra thick] (1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);

			\draw[ultra thick,blue] (.5,5.3)--(.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,blue] (5.2,.7)--(5.2,1.2);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);
		\draw[ultra thick,red] (-.5,-1)--(-.5,7);
			\draw[ultra thick,red] (6.5,-1)--(6.5,7);
			\draw[ultra thick,red] (-.5,6.5)--(6.5,6.5);
			\draw[ultra thick,red] (-.5,-0.5)--(6.5,-0.5);
			\draw[ultra thick,blue]( 5,1.2)--(5,1.6);
		\end{tikzpicture}}
		\caption{}
		\label{fig:3b}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{2.5cm}{
		\begin{tikzpicture}
			\draw[ ultra thick](-1.5,-1.5) rectangle (6.5,6.5);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			\draw[ultra thick] (1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);

			\draw[ultra thick,blue] (.5,5.3)--(.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,blue] (5.2,.7)--(5.2,1.2);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);

			\draw[ultra thick,red] (-1,-1.5)--(-1,6.5);
			\draw[ultra thick,red] (6,-1.5)--(6,6.5);
			\draw[ultra thick,red] (-1,6)--(6,6);
			\draw[ultra thick,red] (-1,-1)--(6,-1);
			\draw[ultra thick,red] (1.2,3.6)--(1.2,4.4);
			\draw[ultra thick,red] (1.6,3.2)--(2.4,3.2);
			\draw[ultra thick,blue]( 5,1.2)--(5,1.6);
		\end{tikzpicture}}
		\caption{}
		\label{fig:3c}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{2.5cm}{
		\begin{tikzpicture}
			\draw[ ultra thick](-1.5,-1.5) rectangle (6.5,6.5);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			\draw[ultra thick] (1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);

			\draw[ultra thick,brown] (.5,5.6)--(.5,4.4);
			\draw[ultra thick,brown] (5.5,5.6)--(5.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,brown] (.2,.4)--(.8,.4);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);
			\draw[ultra thick,brown](5,.2)--(5,0);
			\draw[ultra thick,blue]( 5,1.2)--(5,1.6);
			\draw[ultra thick,red] (-1,-1.5)--(-1,6.5);
			\draw[ultra thick,red] (6,-1.5)--(6,6.5);
			\draw[ultra thick,red] (-1,6)--(6,6);
			\draw[ultra thick,red] (-1,-1)--(6,-1);

			\draw[ultra thick,red] (1.6,3.2)--(2.4,3.2);
			\draw[ultra thick,red] (1.2,3.6)--(1.2,4.4);
			\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			\draw[ultra thick,brown] (0,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.4);


		\end{tikzpicture}}
		\caption{}
		\label{fig:3d}
	\end{subfigure}
\begin{subfigure}[b]{.33\textwidth}
		\centering
		\resizebox{!}{2.5cm}{
		\begin{tikzpicture}
			\draw[ultra thick,brown] (.5,5.6)--(.5,4.4);
			\draw[ultra thick,brown] (5.5,5.6)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,brown] (.2,.4)--(.8,.4);
			\draw[ultra thick,brown](5,.2)--(5,0);
			\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			\draw[ultra thick,brown] (0,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			
			\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.4);
			\draw[ ultra thick](-1.5,-1.5) rectangle (6.5,6.5);
			\draw[ultra thick] (0,0) rectangle (6,6);
			
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			
			\draw[ultra thick,brown] (.5,5.3)--(.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);
			\draw[ultra thick,red] (-1,-1.5)--(-1,6.5);
			\draw[ultra thick,red] (6,-1.5)--(6,6.5);
			\draw[ultra thick,red] (-1,6)--(6,6);
			\draw[ultra thick,red] (-1,-1)--(6,-1);	
			\draw[ultra thick,red] (1.6,3.2)--(2.4,3.2);
			\draw[ultra thick,red] (1.2,3.6)--(1.2,4.4);
			\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			\draw[ultra thick,brown] (,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.6);

			\draw[ultra thick,orange](-1,6)--(6,6)--(6,-1)--(-1,-1)--(-1,6);
			\draw[ultra thick,orange](0,4.4)--(.5,4.4)--(.5,5.3)--(0,5.3)--(0,4.4);
			\draw[ultra thick,orange](5.5,4.4)--(5.5,5.3)--(6,5.3)--(6,4.4)--(5.5,4.4);
			\draw[ultra thick,orange](.2,1.2)--(1,1.2)--(1,.4)--(.2,.4)--(.2,1.2);
			\draw[ultra thick,orange](1,1.6)--(1,.2)--(5,.2)--(5,1.6);
			
			\draw[ultra thick, orange] (1.6,4.4)--(1.6,5.6)--(4.4,5.6)--(4.4,4.4);
			\draw[ultra thick,orange] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(1.6,4.4);	
			\draw[ultra thick,orange] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick,orange] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick,orange](1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);
			%\draw[ultra thick,orange](1.4,3.6)--(1.4,2.4);
			\draw[ultra thick,orange](1.6,3.2)--(1.6,2.6)--(4.3,2.6)--(4.3,3.2)--(1.6,3.2);
			\draw[ultra thick,orange] (1.6,3.4) rectangle (4.6,2.6);

		\end{tikzpicture}}
		\caption{}
		\label{fig:3e}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{2.5cm}{
		\begin{tikzpicture}
			\draw[ultra thick,brown] (.5,5.6)--(.5,4.4);
			\draw[ultra thick,brown] (5.5,5.6)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,brown] (.2,.4)--(.8,.4);
			\draw[ultra thick,brown](5,.2)--(5,0);
			%\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			\draw[ultra thick,brown] (0,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			%\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			%\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.4);
			\draw[ ultra thick](-1.5,-1.5) rectangle (6.5,6.5);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (2,3.2) rectangle (5.6,4.4);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			%\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](2,3.2)--(5.6,3.2)--(5.6,4.4)--(2,4.4)--(2,4.2)--(5.4,4.2)--(5.4,3.4)--(2.2,3.4)--(2.2,4)--(2,4)--(2,3.2);

			\draw[ultra thick](3.5,3.6) rectangle (5.1,4);
			\draw[ultra thick](2.4,4.2)--(2.4,3.4);
			\draw[ultra thick](4.8,4)--(5.1,4)--(5.1,3.4);
			
			\draw[ultra thick] (1.6,4.4)--(2.8,4.4)--(2.8,5)--(4.4,5)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);


			\draw[ultra thick,brown] (.5,5.3)--(.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);

			\draw[ultra thick,brown] (2,4.4)--(1.2,4.4);
			\draw[ultra thick,brown] (,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			\draw[ultra thick,brown] (2.2,4.2)--(2.2,3.2);
			\draw[ultra thick,brown] (5.4,4)--(5.4,3.4);

			\draw[ultra thick,orange] (2.2,1.6)--(3.4,1.6)--(3.4,1)--(5,1)--(5,1.6)--(5,.4)--(2.2,.4)--(2.2,1.6);

			\draw[ultra thick,orange](-1,6)--(6,6)--(6,-1)--(-1,-1)--(-1,6);
			\draw[ultra thick,orange](0,4.4)--(.5,4.4)--(.5,5.3)--(0,5.3)--(0,4.4);
			\draw[ultra thick,orange](5.5,4.4)--(5.5,5.3)--(6,5.3)--(6,4.4)--(5.5,4.4);
			\draw[ultra thick,orange](.2,1.2)--(1,1.2)--(1,.4)--(.2,.4)--(.2,1.2);
			\draw[ultra thick,orange](1,1.6)--(1,.2)--(5,.2)--(5,1.6);
			%\draw[ultra thick,green](1.6,4.4)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(2.2,1.6);
			%\draw[ultra thick,green] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(1.6,4.4);	
			\draw[ultra thick,orange] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick,orange] (2,3.2) rectangle (5.6,4.4);
			%\draw[ultra thick,green](1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);
			%\draw[ultra thick,green](1.4,3.6)--(1.4,2.4);
			\draw[ultra thick,orange](2.4,4)--(2.4,3.4)--(5.1,3.4)--(5.1,4)--(2.4,4);
			\draw[ultra thick,red] (-1,-1.5)--(-1,6.5);
			\draw[ultra thick,red] (6,-1.5)--(6,6.5);
			\draw[ultra thick,red] (-1,6)--(6,6);
			\draw[ultra thick,red] (-1,-1)--(6,-1);
			\draw[ultra thick,orange] (1.6,4.4)--(1.6,5.6)--(4.4,5.6)--(4.4,4.4)--(1.6,4.4);
			\draw[ultra thick,orange](2,3.2)--(2,3.6);
			\draw[ultra thick, orange](2.8,4.4)--(2.8,5)--(4.4,5);
			\draw[ultra thick,orange] (2.4,4.2) rectangle (5.4,3.4);

		\end{tikzpicture}}
		\caption{}
		\label{fig:3f}
	\end{subfigure}
	\caption{(a): Corridor decomposition, (b): Blue lines convert corridors into open corridors with no $\Zc$-bends, red lines bound rings into boxes, (c): Red lines also divide spiral corridors into corridors with at most $3$ bends, we convert outermost ring to boundary-$\Lc$, (d): brown lines denote guillotine cuts dividing a $\Bc$-corridor into $O(1)$ $\Bc$-corridors which are guillotine separable, (e): Orange lines define the bounding boxes, (f): Final $\Bc \Lc$-decomposition. See Section \ref{sec:bl} for details.}
	\label{fig:cnew}
\end{figure}
%\arir{Should we remove red lines from fig 2.}
%%%%%%. Fig


In G{\'a}lvez et al.~\cite{GalvezGHI0W17}, it was noted that spiral corridors are easier to {\em process} to obtain container-based packing. However, the processing as done in \cite{GalvezGHI0W17}, rearranges items and may violate guillotine separability.
Hence, we carefully decompose and rearrange further so that we can {\em process} simpler substructures without violating the guillotine separability. 


First, we show that any spiral open corridor and ring can be rearranged into $O_{\eps, \epsl}(1)$ number of corridors of type $\Bc, \Lc, \Uc, \Gc$ only (see Figure \ref{fig:3a}, \ref{fig:3b},  \ref{fig:3c}). Then we show  guillotine separable bounding boxes for each of the corridors (Figure \ref{fig:3d}). However, these corridors may not be boundary-corridors. Thereafter, we convert all corridors into boundary-corridors with an additional property that the rectangles in the boundary corridor can be separated out using cuts parallel to the orientation of the subcorridors in the boundary corridor (Figure \ref{fig:3e}). Boundary-corridors are then converted so that finally all corridors are either $\Bc$-corridors  (which are also guillotine separable as a pseudoitem) or boundary-$\Lc$ corridors bounded by a guillotine separable box, giving us the final $\Bc\Lc$-arrangement (Figure \ref{fig:3f}). Final $\Bc\Lc$-arrangement is guillotine separable and now we can {\em process} the subcorridors of $\Lc$ to obtain a guillotine separable container-based packing, as described in the next section. 
%\arir{Add more details. You can write about $\Bc$-corridors.}






==> Body4.tex <==

\section{Existence of near-optimal structured solutions}

\label{sec:bldecom} In this section we prove Lemma~?? in the cardinality
case, i.e., assuming that $\profit_{i}=1$ for each item $i\in\R$,
we prove that that there exists a $(1+\epsilon)$-approximate solution
whose items can be placed nicely inside a set of compartments $\C$
that admit a pseudo-guillotine cutting sequence. We will give the
proof of the weighted case in Appendix~??. 

Our strategy is to start with a partition of the knapsack into thin
corridors as defined in \cite{AHW19}. Intuitively, a corridor
is a path or cycle of width at most $\epsl N$, see Figure~??.

\noindent \begin{definition}[Open corridor] An open corridor is
a subregion of knapsack bounded by simple rectilinear polygon with
$2b$ edges $e_{0},e_{1},\dots,e_{2b-1}$ for $b\ge2,b\in\mathbb{N}$,
so that for each pair of horizontal (resp. vertical) edges $e_{i},e_{2b-i},i\in[b-1]$
there exists a vertical (resp. horizontal) line segment $\ell_{i}$
\aw{of length at most $\epsl N$} such that both $e_{i}$ and $e_{2b-i}$
intersect $\ell_{i}$ but no other edges intersect $\ell_{i}$. \end{definition}

\begin{definition}[Closed corridor] A closed corridor (or {\em
cycle}) is a subregion of knapsack bounded by two simple rectilinear
polygon defined by edges $e_{0},e_{1},\dots,e_{b-1}$ and $e'_{0},e'_{1},\dots,e'_{b-1}$
for $b\ge2,b\in\mathbb{N}$, so that the second polygon is contained
within the first polygon and for each pair of horizontal (resp.~vertical)
edges $e_{i},e'_{i},i\in[b-1]$, there exists a vertical (resp.~horizontal)
line segment $\ell_{i}$ \aw{of length at most $\epsl N$} such
that $e_{i}$ and $e'_{i}$ intersect $\ell_{i}$ but no other edges
intersect $\ell_{i}$. \end{definition}
\begin{lem}
[\cite{AHW19,adamaszek2015knapsack}] \label{lem:corridor-partition}There exists a solution
$\overline{\opt}\subseteq\opt$ with $\left|\opt\right|\le(1+\epsilon)\left|\overline{\opt}\right|$
and a partition of $K$ into a set of corridors $\bar{\C}$ with $|\bar{\C}|\le O_{\epsilon}(1)$
where each corridor $C\in\bar{\C}$ has at most $1/\epsilon$ bends
each and such that each item $i\in\overline{\opt}$ is contained in
one corridor of $\bar{\C}$. 
\end{lem}
%
Our strategy is to partition the corridors in $\bar{\C}$ step by
step, while moving some of the items, until the resulting packing
satisfies the properties claimed in Lemma~??. In the process, we
might drop an $\epsilon$-fraction of the items in $\overline{\opt}$.
For this, we need some definitions for the parts of a corridor (which
we will call subcorridors) and its bends. Given an open (resp.~closed)
corridor $C$, we define that a {\em subcorridor} $S_{i}$ is the
maximally large rectangle contained in the corridor containing the
edges $e_{i},e_{2b-i}$ (resp.~$e_{i},e_{i'}$) on its boundary.
Hence, an open (resp.~closed) corridor is the union of $b-1$ (resp.~$b$)
such rectangular regions. %The length of $S_i$ is the \emph{length} of the shortest such edge. 
%\arir{do we use long and short subcorridor in our paper? where?}
%We say that a subcorridor is \emph{long} if its length is more than $N/2$, and \emph{short} otherwise.  
%We call a subcorridor \emph{horizontal} (resp., \emph{vertical}) if 
%its width (resp. height) is more than its height (resp. width).
%Note that each rectangle in $\optco$ is distinctly associated with the only subcorridor that fully contains it.  Let  $S_1,\ldots,S_{k'}$ be a sequence of consecutive subcorridors of an open (or closed) corridor. 
%Consider two consecutive corridors $S_i$ and $S_{j}$ with $j=i+1$ in the case of an open corridor and $j=(i+1)$(mod $k'$) otherwise.
 We say that the region $S_{i,j}$ is the shared rectangular region
between two consecutive subcorridors $S_{i}$ and $S_{j}$, \aw{i.e.,
$S_{i,j}=S_{i}\cap S_{j}$}. The {\em unshared region} of $S_{i}$
is the part of $S_{i}$ that \aw{is not contained in any other subcorridor}.
%There is a natural subdivision of each corridor into regions that 
 For two two consecutive subcorridors $S_{i}$ and $S_{j}$ we \aw{can
find a monotone axis-parallel curve in $S_{i,j}$ that separates the
parts of $S_{i,j}$ containing only vertical or only horizontal items;
we call this curve the {boundary curve} of $S_{i,j}$} (see Figure
\ref{fig:lproc}). %\arir{defined boundary curve}
We define $S_{j}$ to be \aw{on} the right (resp.~left, top, bottom)
of $S_{i}$ if there exists a point in $S_{i}$ to the left (resp.~right,
bottom, top) of every point in $S_{j}\setminus S_{i,j}$. A pair $(S_{i},S_{j})$
forms a {\em clockwise} bend if $S_{i}$ is horizontal and $S_{j}$
is to either bottom-right or top-left of $S_{i}$, and the complementary
cases if $S_{i}$ is vertical. Otherwise, they form a counter-clockwise
bend. A corridor with no bends (resp.~one bend), is called a box-
or $\Bc$-corridor (resp.~$\Lc$-corridor). \aw{Observe that they
are also box-compartments (resp. L-compartments).} %A corridor with only one bend, is called an $\Lc$-corridor. 
An open corridor whose bends are all clockwise (resp.~counter-clockwise)
is a \emph{spiral}. Spirals with $2,3$ bends are called $\Uc,\Gc$-corridors,
respectively. A closed corridor with $b=4$ is a \emph{ring}. %Note that in a ring all bends are either clockwise or counter-clockwise, thus intuitively it is the closed analogue of a spiral.
We call a triple $(S_{i},S_{i'},S_{i''})$ of consecutive subcorridors
a\emph{ $\Zc$-bend} if $S_{i},S_{i'}$ form a clockwise (resp.~counterclockwise)
bend and $S_{i'},S_{i''}$ form a counterclockwise (resp.~clockwise)
bend, and the subcorridors $S_{i},S_{i'},S_{i''}$ are called $\Zc$-subcorridors.
We call $S_{i'}$ the \emph{center-subcorridor} of the bend, and $S_{i},S_{i''}$
its \emph{side-subcorridors}. A spiral corridor can not have $\Zc$
bends. A subcorridor that is not a $\Zc$-subcorridor is called a
{\em spiral subcorridor}. A $\Zc$-corridor is a corridor formed
by the union of 3 $\Zc$-subcorridors. 

For transforming $\overline{\opt}$ and the corridors in $\bar{\C}$,
we first apply the following lemma to each corridor with a \emph{$\Zc$}-bend.
Note that Lemma~?? trivially holds if $\left|\overline{\opt}\right|\le O_{\epsilon}(1)$
and hence we assume for the remainder of this section that $\left|\overline{\opt}\right|$
is larger than any given constant (which in particular implies that
we can drop any set of $O_{\epsilon}(1)$ items from $\overline{\opt}$
while losing only a factor of $1+\epsilon$). 

\begin{lem}\label{lem:noz} Let $C\in\bar{\C}$ be a corridor with
at least one $\Zc$-bend and let $\overline{\opt}(C)$ denote the
items from $\overline{\opt}$ inside $C$. We can be partition $C$
into $O_{\eps}(1)$ spiral corridors into which we can place at least
$\overline{\opt}(C)-O_{\eps,\epsl}(1)$ items from $\overline{\opt}(C)$,
such that globally the resulting solution is guillotine separable
(including the items in $\overline{\opt}\setminus\overline{\opt}(C)$).
\end{lem} \begin{proof} There are two cases.

\noindent \textit{Case 1: $C$ is an open corridor with at least one
$\Zc$-bend.} Assume $C$ has 5 subcorridors (also works for fewer
subcorridors) $S_{i'+1},S_{i'+2},S_{i'+3},S_{i'+4},S_{i'+5}$ such
that $\{S_{i'+2},S_{i'+3},S_{i'+4}\}$ form a $\Zc$-bend. W.l.o.g.~assume
$S_{i'+3}$ be a horizontal subcorridor and $S_{i'+2}$ be situated
to the top left of $S_{i'+3}$ (see Figure \ref{fig:kbend}). Let
us consider a sequence of guillotine cuts through these five subcorridors.
Consider the unshared region of $S_{i'+3}$: $\overline{S_{i'+3}}:=S_{i'+3}$
$\setminus\{S_{i'+2}\cup S_{i'+4}\}$. Then from Observation \ref{endtoend},
there exists an end-to-end cut $l'$ in $\overline{S_{i'+3}}$.

If this cut $l'$ through $\overline{S_{i'+3}}$ is vertical, then
we can partition $C$ along $l'$ into $2$ new corridors, each containing
at least one lesser $\Zc$-bend, compared to $C$.

If the cut $l'$ is horizontal, then consider the guillotine cuts
which occurred before the cut $l'$. Let $l_{i'+2}$ be the rightmost
vertical cut (including those which pass through the vertical boundary
of $S_{i'+2}$, if any) through $S_{i'+2,i'+3}$. Extend the cut $l_{i'+2}$
so that it touches the boundary curve between $S_{i'+1}$ and $S_{i'+2}$
at point $p$. Now draw a line $l_{i'+1}$ from point $p$ parallel
to the orientation of $S_{i'+1}$ till it touches the boundary curve
between $S_{i'+1}$ and $S_{i'}$. Continue the same process by drawing
lines $l_{j}$ through corridors $S_{j}$, where $1\leq j\leq i'$,
in a similar fashion. Drop items that are cut by these lines. Stop
when we obtain a line $l_{t}$ through $S_{t}$ parallel to the orientation
of $S_{t}$, $t\ge1$, that reaches a boundary edge of $C$. Lines
$\{l_{t},l_{t+1},\dots,l_{i'+2}\}$ partition the corridor $C$ into
at most 2 smaller corridors $C_{1},C_{2}$ as shown in Figure \ref{fig:kbend}.
$C_{1}$ contains rectangles from the subcorridors $S_{t},\dots,S_{i'+2}$
only. $C_{2}$ contains rectangles from the subcorridors $S_{1},\dots,S_{k}$.
In a similar way, we choose $l_{i'+4}$ be the leftmost vertical cut
through $S_{i'+3,i'+4}$ and we can partition $C_{2}$ into at most
2 corridors $C_{3}$ and $C_{4}$ where $C_{3}$ contains rectangles
from the subcorridors $S_{i'+4},\dots,S_{t'}$ for $t'\le k$ and
$C_{4}$ contains rectangles from the subcorridors $S_{1},\dots,S_{k}$.
During this process of partitioning we drop at most $O_{\eps,\epsl}(1)$
rectangles (these are also included in $\optco^{cross}$), as at most
$\frac{1}{\epsl}$ items are dropped in at most $\frac{1}{\eps}$
subcorridors. Note that $l'$ divides $C_{4}$ into 2 new corridors
containing at least one lesser $\Zc$-bend when compared to $C$.
The reason for choosing $l_{i'+2}$ (resp.~$l_{i'+4}$) and extending
it to partition the corridor $C$ is that $l_{i'+2}$ (resp.~$l_{i'+4}$)
is the cut which intercepts the horizontal cut $l'$ in $S_{i'+2,i'+3}$
(resp.~$S_{i'+3,i'+4}$) .

Repeating the above procedure for all $\Zc$-bends concludes the proof
for this case.

\noindent \textit{Case 2: $C$ is a closed corridor with at least
one $\Zc$-bend.} Let $S_{L}$ (resp. $S_{B}$, $S_{R}$, $S_{T}$)
be the leftmost vertical (resp. bottom-most hor., rightmost vert.,
topmost hor.) subcorridor in $C$. These four subcorridors can form
following types of corridors among themselves: (i) one $\Gc$ (Figure
\ref{fig:zbend1}), (ii) two $\Lc$ (Figure \ref{fig:zbend}), (iii)
one $\Uc$ and one $\Bc$ (Figure \ref{fig:zbend3}), (iii) one $\Lc$
and two $\Bc$ (Figure \ref{fig:zbend2}) and (v) four $\Bc$ (Figure
\ref{fig:zbend4}). We call a cut to be a {\em good cut} if it
passes through the unshared region of subcorridor perpendicular to
its orientation. A good guillotine cut divides a corridor into $O_{\eps}(1)$
open corridors which can then be handled as in Case 1 (see Figure
\ref{fig:zbend}). Now, consider the sequence of guillotine cuts in
the smallest piece containing $C$. If there is a good guillotine
cut, we stop the sequence of guillotine cuts and we are done as we
get $O_{\eps}(1)$ open corridors. Else from Observation \ref{endtoend},
we get an end-to-end cut passing through one of the subcorridors $\{S_{L},S_{B},S_{R},S_{T}\}$,
parallel to the orientation of the subcorridor. We continue separating
items from these four subcorridors $\{S_{L},S_{B},S_{R},S_{T}\}$
according to these end-to-end cuts, till either (i) we get a good
cut or (ii) all the rectangles from one of these four subcorridors
get completely separated from the rest. We now create at most 4 spiral
corridors containing items from subcorridors $\{S_{L},S_{B},S_{R},S_{T}\}$
only by using the last cut (excluding the good cut) in each of the
subcorridors $\{S_{L},S_{B},S_{R},S_{T}\}$. In the first case, we
separate out the rectangles from these 4 subcorridors into the newly
created $O(1)$ spiral corridors with at most three bends and then
using the good cut we divide rest of the closed corridor into $O_{\eps}(1)$
open corridors as shown in Figure \ref{fig:zbend} and Figure \ref{closedcor2}.
In the second case, if we don't have such a good cut then eventually
all the items in one of the subcorridors $\{S_{L},S_{B},S_{R},S_{T}\}$
will have been separated out (we say that the subcorridor is {\em
exhausted}) into the newly created $O(1)$ spiral corridors with
at most $4$ bends. W.l.o.g.~assume that the subcorridor $S_{B}$
gets exhausted. Then the last cut through $S_{B}$ leaves us with
$O(1)$ open corridors (see Figure \ref{fig:zbend2}). The open corridors
are again dealt using Case 1, finally giving $O_{\eps}(1)$ spiral
corridors. \end{proof}

Let $\overline{\opt}'$ and $\bar{\C}'$ denote the resulting solution
after applying Lemma~\ref{lem:noz} to each corridor in $\bar{\C}$
with at least one $\Zc$-bend. Then $\bar{\C}'$ contains only rings
and spirals, since if a closed corridor is not a ring, it has at least
one $\Zc$-bend, and if an open corridor does not have a $\Zc$-bend
then it must be a spiral.
\begin{lem}
Every corridor in $\bar{\C}'$ is a ring or a spiral. 
\end{lem}
We process the corridors in $\bar{\C}'$ and their items further.
Consider a ring corridor $C\in\bar{\C}'$, let $\overline{\opt}'(C)$
denote the items of $\overline{\opt}'$ placed inside $C$, and let
$\overline{\opt}'_{in}(C)$ denote the items of $\overline{\opt}'$
that are placed in the area of $K$ that is surrounded by $C$. Also,
let $R(C)$ denote the smallest rectangle that contains $C$. We rearrange
the items in $\overline{\opt}'(C)$ and $\overline{\opt}'_{in}(C)$
such that we move the items in $\overline{\opt}'_{in}(C)$ uniformly
towards the top right of $R(C)$ and rearrange the items in $\overline{\opt}'(C)$
such that they fit into an $\Lc$-corridor at the boundary of within
$R(C)$.
\begin{lem}
Given a ring corridor $C\in\bar{\C}'$, we can rearrange the items
in $\overline{\opt}'(C)$ and $\overline{\opt}'_{in}(C)$ inside $R(C)$
such that the items in $\overline{\opt}'(C)$ are placed inside an
$\Lc$-corridor $L$ such that $R(C)\setminus L$ is a rectangle,
and the items in $\overline{\opt}'_{in}(C)$ are placed inside $R(C)\setminus L$.
Moreover, globally the resulting solution is guillotine separable
(including the items in $\overline{\opt}'\setminus\overline{\opt}'(C)$).
\end{lem}
Next, we partition every spiral corridor $C\in\bar{\C}'$ and rearrange
its items $\overline{\opt}'(C)$ of $\overline{\opt}'$ such that
each of the resulting corridors has at most three bends, which are
hence of type $\Bc,\Lc,\Uc,$ or $\Gc$.
\begin{lem}
Given a spiral corridor $C\in\bar{\C}'$, we can rearrange the items
in $\overline{\opt}'(C)$ inside $C$ and partition $C$ into $O_{\eps,\epsl}(1)$
open corridors with at most three bends each, such that each item
in $\overline{\opt}'(C)$ is contained in one of the resulting corridors.
Moreover, globally the resulting solution is guillotine separable
(including the items in $\overline{\opt}'\setminus\overline{\opt}'(C)$).
\end{lem}
Let $\bar{\C}''$ denote the resuling set of corridors, each of them
having at most three bends, and denote by $\overline{\opt}''$ the
corresponding solution (i.e., the items in $\overline{\opt}'$ in
their new placement). We want to show that for each corridor $C\in\bar{\C}''$
we can define a rectangle $R(C)$ with $C\subseteq R(C)$ such that
these rectangles $\left\{ R(C)\right\} _{C\in\bar{\C}''}$ form a
laminar family and for each $C\in\bar{\C}''$ it holds that $C$ is
a boundary corridor of $R(C)$ according to the following definition.
These rectangles $R(C)$ will help us later to define a pseudo-guillotine
cutting sequence.

\noindent \begin{definition}[Boundary corridors] Given a rectangle
$[l,r]\times[b,t]\subseteq K$. A {\em boundary-$\Lc$} of height
$N_{1}$ and width $N_{2}$ is the region $\big(([l,r]\times[b,b+N_{1}])\cup([l,l+N_{2}]\times[b,t])\big)$.
Similarly, a {\em boundary-$\Uc$} (resp.~{\em boundary-$\Gc$})
occupies the region $\big(([l,r]\times[b,b+N_{1}])\cup([l,l+N_{2}]\times[t,b])\cup([r-N_{3},r]\times[b,t])\big)$
(resp.~ $\big(([l,r]\times[b,b+N_{1}])\cup([l,l+N_{2}]\times[t,b])\cup([r-N_{3},r]\times[b,t])\cup([l,r]\times[t-N_{4},t])\big)$).
Such a {\em boundary-$\Lc$, boundary-$\Uc$, boundary-$\Gc$}
is also called a {\em boundary corridors} for $[l,r]\times[b,t]$. 

\noindent \end{definition}
\begin{lem}
There is a family of rectangles $\left\{ R(C)\right\} _{C\in\bar{\C}''}$
such that
\begin{itemize}
\item for each $C\in\bar{\C}''$, $C$ is a boundary corridor for $R(C)$
(and hence $C\subseteq R(C)$), and each item $i\in\overline{\opt}''$
is contained in $R(C)$ or in $K\setminus R(C)$,
\item for any $C,C'\in\bar{\C}''$ it holds that $R(C)\subseteq R(C')$,
or $R(C')\subseteq R(C)$, or $R(C)\cap R(C')=\emptyset$.
\end{itemize}
\end{lem}
Now we adjust the corridors in $\bar{\C}''$ and the items contained
in them further such that we obtain only corridors with at most one
bend each. To this end, we process the corridors in $\bar{\C}''$
in an order induced by the laminar family $\left\{ R(C)\right\} _{C\in\bar{\C}''}$
and move the items contained in the respective rectangles $R(C)$,
such that at the end we can replace each corridor $C\in\bar{\C}''$
by a boundary-$\Lc$ corridor for $R(C)$ that contains the same items
as $C$ previously. 
\begin{lem}
Let $C\in\bar{\C}''$. We can rearrange the items from $\overline{\opt}''$
inside $R(C)$ such that there exists a partition of $C$ into a boundary-$\Lc$
$L$ and a rectangle $R\setminus L$ such that $L$ contains all items
that were contained in $C$ previously and $R\setminus L$ contains
a uniform translation of the items that were contained in $R(C)\setminus C$
previously.
\end{lem}
Finally, we subdivide each $\Bc$-corridor into $O_{\epsilon}(1)$
box-compartments, while losing at most a factor of $1+\epsilon$ in
the profit of the contained items.
\begin{lem}
\label{lem:compartments-boxes}Given a $\Bc$-corridor $B$ containing
a set of items $\R(B)$. There exists a partition of $B$ into $O_{\epsilon}(1)$
box-compartments $\B(B)$ that are guillotine separable and a nice
placement of a set of items $\R'(B)\subseteq\R(B)$ with $\profit(\R'(B))\ge(1-\epsilon)\profit(\R'(B))$
inside $\B(B)$. 
\end{lem}
Similarly, we subdivide each $\Lc$-corridor into one L-compartment
and $O_{\epsilon}(1)$ box-compartments, while losing at most a factor
of $1+\epsilon$ in the profit of the contained items.
\begin{lem}
\label{lem:compartments-L}Given a $\Lc$-corridor $L$ containing
a set of items $\R(L)$. There exists a partition of $L$ into one
L-compartment $L'$ and $O_{\epsilon}(1)$ box-compartments $\B(L)$
such that 
\begin{itemize}
\item $L'$ is a boundary-$\Lc$ corridor for $R(L)$,
\item the box-compartments in $\B(L)$ are guillotine separable, and 
\item there is a nice placement of a set of items $\R'(L)\subseteq\R(L)$
with $\profit(\R'(L))\ge(1-\epsilon)\profit(\R'(L))$ inside $\B(L)$
and $L'$. 
\end{itemize}
\end{lem}
Let $\C$ denote the compartments constructed in Lemmas~\ref{lem:compartments-boxes}
and \ref{lem:compartments-L}. We can show that they admit a pseudo-guillotine
cutting sequence since the constructed box-compartments are guillotine
separable and each constructed L-compartment $L'$ for an $\Lc$-corridor
$L$ is a boundary-$\Lc$ corridor for $R(L)$.
\begin{lem}
There is a pseudo-guillotine cutting sequence for the compartments
in $\C$.
\end{lem}
This completes the proof of Lemma~?? in the cardinality case. We
will prove the weighted case in Appendix~??.

% \end{document}

%\centering
\begin{figure}[h]
\captionsetup[subfigure]{justification=centering} \hspace{-10pt}
\begin{subfigure}[b]{1\textwidth} \centering \resizebox{!}{4.3 cm}{
\begin{tikzpicture}
						\draw[thick] (0,6)--(2,6)--(2,5.5)--(4,5.5)--(4,6)--(6,6)--(6,4)--(5,4)--(5,3)--(4.5,3)--(4.5,4.5)--(5.5,4.5)--(5.5,5.5)--(4.5,5.5)--(4.5,5)--(1.5,5)--(1.5,5.5)--(.5,5.5)--(.5,4)--(2,4)--(2,3)--(4,3)--(4,2.5)--(1.5,2.5)--(1.5,3.5)--(0,3.5)--(0,6);		
						
						\draw[dotted] (6,4)--(5.5,4.5);
						\draw[dotted] (5,4)--(4.5,4.5);
						\draw[red] (6,6)--(5.9,6)--(5.9,5.9)--(5.8,5.9)--(5.8,5.8)--(5.7,5.8)--(5.7,5.7)--(5.6,5.7)--(5.6,5.6)--(5.5,5.6)--(5.5,5.5);
						\draw[dotted] (4,6)--(4.5,5.5);
						\draw[dotted] (2,6)--(1.5,5.5);
						\draw[red] (0,6)--(.1,6)--(.1,5.9)--(.2,5.9)--(.2,5.75)--(.25,5.75)--(.3,5.75)--(.3,5.67)--(.5,5.67)--(.5,5.6)--(.5,5.5);
						\draw[dotted] (0.25,3.6)--(.5,4);
						\draw[dotted] (1.5,2.5)--(2,3);
						\draw[dotted] (1.5, 3.5)--(2,4);
						\draw[dotted] (1.5, 5)--(2,5.5);
						\draw[dotted] (4.5 , 5)--(4,5.5);


						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.4,3.5);	\draw (-.75,3.5) node {\textbf{$l_{i'+2}$}};
						\draw[->] (.25,5.75) edge[out=180,in=0,->] (-.4,5.4);	\draw (-.6,5.4) node {\textbf{$p$}};
						\draw[->] (1,5.75) edge[out=90,in=0,->] (.8,6.5);	\draw (.5,6.5) node {\textbf{$l_{i'+1}$}};
						%\draw (1.75,5.25) node {\textbf{$l_{1}$}};
						%\draw (4.25, 5.25) node {\textbf{$l_{2}$}{spialgo}};
						%\draw[->] (5,5.75) edge[out=180,in=0,->] (4.75,6.5);	\draw (4.5,6.5) node {\textbf{$l$}};%
%						\draw[->] (5.75,5) edge[out=180,in=0,->] (6.5,5);	\draw (6.5,5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};%
%						\draw[->] (.25,4.5) edge[out=180,in=0,->] (-.5,3.5);	\draw (-.75,3.5) node {\textbf{$l_{V}$}};
						\fill [lightgray] (0,3.5) rectangle (0.5,4);
						\draw[->] (.2,3.75) edge[out=180,in=0,->] (-.4,2.5);	\draw (-.75,2.5) node {\textbf{$S_{i'+2,i'+3}$}};
						\draw[dashed] (4.75,3) -- ( 4.75 ,4.25) -- ( 5.75, 4.25) -- ( 5.75, 5.75) -- ( 4.25, 5.75) -- ( 4.25, 5.25) -- ( 1.75, 5.25) -- ( 1.75, 5.75) -- (.25, 5.75) -- (.25, 3.5) ;	
						\draw(4.75,2.7) node {\large \textbf{$S_{1}$}};
						\draw(.75,3.8) node {\large \textbf{$l'_{H}$}};
						\draw(1.2,4.7) node {\large \textbf{$l'_{V}$}};
						%\draw (5,4.75) node {\large \textbf{$C$}};
						%\draw (4,3) node {\large \textbf{$B$}};

						\draw [thick, blue] (.25,3.5)--(.25,5.75);
						\draw [thick, blue] (1.75,4)--(1.75,2.5);
						\draw[thick, green] (.25,3.6)--(1.75,3.6);
						\draw[thick, brown] (1.2,4.5)--(1.2,3);
		
		\end{tikzpicture}} \caption{Removal of $\Zc$-bend in an open corridor. $l_{i'+2}$, $l_{i'+4}$
are shown in blue. Vertical (resp.~horizontal) (if any) $l'$ is
shown as $l'_{V}$(resp.~$l'_{H}$), boundary curves are shown in
red or dotted. $l'$ separates the corridors into two corridors with
lesser $\Zc$-bends.}
\label{fig:kbend} \end{subfigure}

\begin{subfigure}[b]{.5\textwidth} \centering \resizebox{!}{3.5cm}{
\begin{tikzpicture}
						\draw[thick, fill =lightgray] (0,7)--(2,7)--(2,4)--(7,4)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw [solid, fill=white] (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7) --(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						%\draw[fill=white] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3)--(.5,3);
						%\draw[fill=white] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
						%\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						%\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
						
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};


						\draw[dashed] (5.6,.5)--(5.6,4);
						\draw[dashed] (5,.5)--(6.7,.5);
						\draw[dashed] (6.5,.5)--(6.5,4);
						\draw[dashed] (.5,3)--(.5,6.5);
						\draw[dashed] (.3,6.5)--(2,6.5);
						\draw[dashed] (5,.3)--(6.9,.3);
						\draw[dashed] (6.7,.3)--(6.7,4);
						\draw[dashed] (.3,3)--(.3,6.7);
						\draw[dashed] (.1,6.7)--(2,6.7);
						\draw[dashed] (5,.1)--(7,.1);
						\draw[dashed] (6.9,.1)--(6.9,4);
						\draw[dashed] (.1,3)--(.1,6.9);
						\draw[dashed] (0,6.9)--(2,6.9);
		\end{tikzpicture}} \caption{A sequence of guillotine cuts (shown as dashed lines) until we get
a good cut}
\label{fig:zbend-lines} \end{subfigure} \begin{subfigure}[b]{.5\textwidth}
\centering \resizebox{!}{3.5cm}{ \begin{tikzpicture}
						\draw[thick, fill =lightgray] (0,7)--(2,7)--(2,4)--(7,4)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw [solid, fill=white] (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7) --(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[fill=white] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3)--(.5,3);
						\draw[fill=white] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.5,.5)--(6.5,4)--(7,4)--(7,0)--(5,0)--(5,.5);
					
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};


						\draw[thick] (5.6,.5)--(5.6,4);
	
		\end{tikzpicture}} \caption{A good cut is shown by bold line. Shaded regions show two $\Lc$ corridors
created before we obtained the good cut.}
\label{fig:zbend} \end{subfigure} \caption{}
\end{figure}

%\centering
\begin{figure}[h]
\captionsetup[subfigure]{justification=centering} \hspace{-10pt}
\begin{subfigure}[b]{.25\textwidth} \centering \resizebox{!}{3.3cm}{
\begin{tikzpicture}
						\draw[thick] (0,7)--(7,7)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);

						\draw[fill=lightgray] (0,7)--(7,7)--(7,0)--(5,0)--(5,3)--(0,3)--(0,7);	
						\draw[fill=white] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,0.5)--(5,0.5)--(5,0)--(7,0)--(7,7)--(0,7)--(0,3)--(.5,3);
						\draw [fill=white]  (.75,6.25)--(6.25,6.25)--(6.25,.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,0.5)--(5,0.5)--(5,0)--(7,0)--(7,7)--(0,7)--(0,3)--(.5,3);
						
					
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};
						\draw[thick] (5.6,.5)--(5.6,6.5);
						
	
		\end{tikzpicture}} \caption{One $\Gc$ corridor created before we obtain a good cut.}
\label{fig:zbend1} \end{subfigure} \begin{subfigure}[b]{.25\textwidth}
\centering \resizebox{!}{3.3cm}{ \begin{tikzpicture}
						\draw[fill=lightgray] (0,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw[fill=white]  (.75,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[fill=white] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[fill=white] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[fill=white] (5,.75)--(6.25,.75)--(6.25,0)--(5,0)--(5,.75);
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(2,6.5)--(2,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[pattern=north west lines, pattern color=gray] (5,.75)--(6.25,.75)--(6.25,0)--(5,0)--(5,.75);
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};
						

						
	
		\end{tikzpicture}} \caption{One $\Lc$, two $\Bc$ corridors created before corridor $S_{B}$
gets exhausted.}
\label{fig:zbend2} \end{subfigure} \begin{subfigure}[b]{.25\textwidth}
\centering \resizebox{!}{3.3cm}{ \begin{tikzpicture}
						\draw[thick, fill= lightgray] (0,7)--(7,7)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,7);
						\draw [fill=white]  (.75,6.25)--(6.25,6.25)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,6.25); 	
						\draw[fill=white] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,2)--(7,2)--(7,7)--(0,7)--(0,3);
						\draw[fill=white] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,6.5)--(6.5,6.5)--(6.5,2)--(7,2)--(7,7)--(0,7)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
					
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};
						\draw[thick] (5.6,.5)--(5.6,6.5);
						
	
		\end{tikzpicture}} \caption{One $\Uc$ and one $\Bc$ corridor created before we obtain a good
cut.}
\label{fig:zbend3} \end{subfigure} \begin{subfigure}[b]{.25\textwidth}
\centering \resizebox{!}{3.3cm}{ \begin{tikzpicture}
						\draw[thick, fill=lightgray] (0,5)--(0.75,5)--(0.75,7)--(2,7)--(2,4)--(7,4)--(7,2)--(6.25,2)--(6.25,0)--(5,0)--(5,3)--(0,3)--(0,5);
						\draw[fill=white]  (.75,4.5)--(1.25,4.5)--(1.25,6.25)--(1.75,6.25)--(1.75, 3.7)--(6.25,3.7)--(6.25,2.5) --(5.75,2.5)--(5.75,0.75)-- ( 5.25,.75)--(5.25,3.25)--(.75,3.25)--(.75,4.5); 
						\draw[fill=white] (.5,3)--(.5,5)--(0,5)--(0,3);
						\draw[fill=white] (0.75,6.5)--(2,6.5)--(2,7)--(0.75,7)--(0.75,6.5);
						\draw[fill=white] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[fill=white] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);	
						\draw[pattern=north west lines, pattern color=gray] (.5,3)--(.5,5)--(0,5)--(0,3);
						\draw[pattern=north west lines, pattern color=gray] (0.75,6.5)--(2,6.5)--(2,7)--(0.75,7)--(0.75,6.5);
						\draw[pattern=north west lines, pattern color=gray] (7,4)--(7,2)--(6.5,2)--(6.5,4)--(7,4);
						\draw[pattern=north west lines, pattern color=gray] (5,.5)--(6.25,.5)--(6.25,0)--(5,0)--(5,.5);
						\draw (.3,4.75) node {\large \textbf{$S_{L}$}};
						\draw (1.25,6.75) node {\large \textbf{$S_{T}$}};
						\draw (6.75,2.25) node {\large \textbf{$S_{R}$}};
						\draw (5.75,.25) node {\large \textbf{$S_{B}$}};
						\draw[thick] (5.6,.5)--(5.6,4);						

						
	
		\end{tikzpicture}} \caption{Four $\Bc$ corridors created before we obtain a good cut.}
\label{fig:zbend4} \end{subfigure} \caption{Good cuts are shown as bold lines.}
\label{closedcor2} 
\end{figure}

%%%%%%%%%%%%%% Fig
%%%%%%%%%%%%%%

%\centering
\begin{figure}[h]
\captionsetup[subfigure]{justification=centering} \hspace{-10pt}
\begin{subfigure}[b]{.32\textwidth} \centering \resizebox{!}{2.5cm}{
\begin{tikzpicture}
			\draw[solid, fill=lightgray] (5.3,5.4) rectangle (5.4,5.5);
			\draw[solid, fill=lightgray] (5.5,5.1) rectangle (4.7,5.2);	
			\draw[solid, fill=lightgray] (.7,5.4) rectangle (0.6,5.5);
			\draw[solid, fill=lightgray] (.6,5.1) rectangle (1.4,5.2);
			\draw[solid, fill=lightgray] (5.2,.8) rectangle (5.8,0.7);
			\draw[solid, fill=lightgray] (5.7,.6) rectangle (5.5,.5);	
			\draw[solid, fill=lightgray] (.7,.6) rectangle (0.6,0.5);
			\draw[solid, fill=lightgray] (.8,.8) rectangle (0.2,0.7);

			\draw[solid, fill=lightgray] (0,6.8) rectangle (5.5,6.7);
			\draw[solid, fill=lightgray] (0,-0.7) rectangle (5.5,-0.8);
			\draw[solid, fill=lightgray] (-0.7,0) rectangle (-0.8,6);
			\draw[solid, fill=lightgray] (6.7,0) rectangle (6.8,6);	
			\draw[solid, fill=lightgray] (0,6.3) rectangle (5.5,6.2);
			\draw[solid, fill=lightgray] (0,-0.2) rectangle (5.5,-0.3);
			\draw[solid, fill=lightgray] (-0.2,0) rectangle (-0.3,6);
			\draw[solid, fill=lightgray] (6.2,0) rectangle (6.3,6);	
			\draw[solid, fill=lightgray] (3.5,1.5) rectangle (3,1);
			\draw[solid, fill=lightgray] (3.5,5) rectangle (3,4.5);
						


			\draw[solid, fill=lightgray] (1.8,5.35) rectangle (4.2,5.5);
			\draw[solid, fill=lightgray] (2,5.15) rectangle (4.2,5.3);
			\draw[solid, fill=lightgray] (1.67,4.45) rectangle (1.85,5.3);
			\draw[solid, fill=lightgray] (1.95,4.45) rectangle (2.1,5.1);
			\draw[solid, fill=lightgray] (3.97,4.45) rectangle (4.15,5.1);
			\draw[solid, fill=lightgray] (4.25,4.45) rectangle (4.35,5.5);

			\draw[solid, fill=lightgray] (1.8,.65) rectangle (4.2,.5);
			\draw[solid, fill=lightgray] (2,.85) rectangle (4.2,.7);
			\draw[solid, fill=lightgray] (1.67,1.55) rectangle (1.85,.7);
			\draw[solid, fill=lightgray] (1.95,1.55) rectangle (2.1,.9);
			\draw[solid, fill=lightgray] (3.97,1.55) rectangle (4.15,.9);
			\draw[solid, fill=lightgray] (4.25,1.55) rectangle (4.35,.5);

			\draw[solid, fill=lightgray] (1.5,3.65) rectangle (4.7,3.77);
			\draw[solid, fill=lightgray] (1.5,3.95) rectangle (4.9,4.2);
			\draw[solid, fill=lightgray] (1.5,4.1) rectangle (5.2,4.35);
			\draw[solid, fill=lightgray] (1.4,3.5) rectangle (4,3.4);
			\draw[solid, fill=lightgray] (1.6,3.4) rectangle (4,3.3);
			\draw[solid, fill=lightgray] (2.6,3.2) rectangle (4,3);
			\draw[solid, fill=lightgray] (4.1,3.2) rectangle (4.2,2.7);
			\draw[solid, fill=lightgray] (2.6,2.6) rectangle (4,2.7);
			\draw[solid, fill=lightgray] (2.6,2.5) rectangle (4,2.6);
			\draw[solid, fill=lightgray] (4.3,3.2) rectangle (4.4,2.7);
			\draw[solid, fill=lightgray] (4.6,3.2) rectangle (4.7,2.7);				
			\draw[solid, fill=lightgray] (1.7,3.2) rectangle (1.8,2.7);
			\draw[solid, fill=lightgray] (1.5,3.2) rectangle (1.6,2.7);
			\draw[solid, fill=lightgray] (1.2,3.2) rectangle (1.3,2.7);
			\draw[solid, fill=lightgray] (1.2,3.3) rectangle (1.3,3.4);		

			\draw[solid, fill=lightgray] (.5,3.1) rectangle (.7,3.6);
			\draw[solid, fill=lightgray] (.8,3.1) rectangle (1,3.6);
			\draw[solid, fill=lightgray] (5.5,4.2) rectangle (5.3,1.8);
			\draw[solid, fill=lightgray] (5.2,3.6) rectangle (5,2.4);
			\draw[solid, fill=lightgray] (1,1.7) rectangle (4,1.8);
			\draw[solid, fill=lightgray] (0.5,1.7) rectangle (0.6,2.7);
			\draw[solid, fill=lightgray] (1,0.25) rectangle (4,0.35);
			\draw[solid, fill=lightgray] (1,5.75) rectangle (4,5.85);
			\draw[solid, fill=lightgray] (0.25,2) rectangle (0.35,4);
			\draw[solid, fill=lightgray] (5.65,2) rectangle (5.75,4);
			\draw[ ultra thick](-1,-1) rectangle (7,7);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			\draw[ultra thick] (1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);
			
			%\draw[ultra thick,brown] (.5,5.6)--(.5,4.4);
			%\draw[ultra thick,brown] (5.5,5.6)--(5.5,4.4);
			%\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			%\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			%\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			%\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			%\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			%\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			%\draw[ultra thick,brown] (.2,.4)--(.8,.4);
			%\draw[ultra thick,blue] (.8,.4)--(1,.4);
			%\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);
			%\draw[ultra thick,brown](5,.2)--(5,0);
			%\draw[ultra thick,blue]( 5,1.2)--(5,1.6);
			%\draw[ultra thick,red] (-.5,-1)--(-.5,7);
			%\draw[ultra thick,red] (6.5,-1)--(6.5,7);
			%\draw[ultra thick,red] (-.5,6.5)--(6.5,6.5);
			%\draw[ultra thick,red] (-.5,-0.5)--(6.5,-0.5);

			%\draw[ultra thick,red] (1.6,3.2)--(2.4,3.2);
			%\draw[ultra thick,red] (1.2,3.6)--(1.2,4.4);
			%\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			%\draw[ultra thick,brown] (0,5.6)--(6,5.6);
			%\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			%\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			%\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			%\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			%\draw[ultra thick,brown] (1,1.6)--(1,0);
			%\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			%\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.4);
			

		\end{tikzpicture}} \caption{}
\label{fig:3a} \end{subfigure} \begin{subfigure}[b]{.32\textwidth}
\centering \resizebox{!}{2.5cm}{ \begin{tikzpicture}
			\draw[ultra thick](-1,-1)rectangle(7,7);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			\draw[ultra thick] (1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);

			\draw[ultra thick,blue] (.5,5.3)--(.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,blue] (5.2,.7)--(5.2,1.2);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);
		\draw[ultra thick,red] (-.5,-1)--(-.5,7);
			\draw[ultra thick,red] (6.5,-1)--(6.5,7);
			\draw[ultra thick,red] (-.5,6.5)--(6.5,6.5);
			\draw[ultra thick,red] (-.5,-0.5)--(6.5,-0.5);
			\draw[ultra thick,blue]( 5,1.2)--(5,1.6);
		\end{tikzpicture}} \caption{}
\label{fig:3b} \end{subfigure} \begin{subfigure}[b]{.32\textwidth}
\centering \resizebox{!}{2.5cm}{ \begin{tikzpicture}
			\draw[ ultra thick](-1.5,-1.5) rectangle (6.5,6.5);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			\draw[ultra thick] (1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);

			\draw[ultra thick,blue] (.5,5.3)--(.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,blue] (5.2,.7)--(5.2,1.2);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);

			\draw[ultra thick,red] (-1,-1.5)--(-1,6.5);
			\draw[ultra thick,red] (6,-1.5)--(6,6.5);
			\draw[ultra thick,red] (-1,6)--(6,6);
			\draw[ultra thick,red] (-1,-1)--(6,-1);
			\draw[ultra thick,red] (1.2,3.6)--(1.2,4.4);
			\draw[ultra thick,red] (1.6,3.2)--(2.4,3.2);
			\draw[ultra thick,blue]( 5,1.2)--(5,1.6);
		\end{tikzpicture}} \caption{}
\label{fig:3c} \end{subfigure} \begin{subfigure}[b]{.32\textwidth}
\centering \resizebox{!}{2.5cm}{ \begin{tikzpicture}
			\draw[ ultra thick](-1.5,-1.5) rectangle (6.5,6.5);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			\draw[ultra thick] (1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);

			\draw[ultra thick,brown] (.5,5.6)--(.5,4.4);
			\draw[ultra thick,brown] (5.5,5.6)--(5.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,brown] (.2,.4)--(.8,.4);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);
			\draw[ultra thick,brown](5,.2)--(5,0);
			\draw[ultra thick,blue]( 5,1.2)--(5,1.6);
			\draw[ultra thick,red] (-1,-1.5)--(-1,6.5);
			\draw[ultra thick,red] (6,-1.5)--(6,6.5);
			\draw[ultra thick,red] (-1,6)--(6,6);
			\draw[ultra thick,red] (-1,-1)--(6,-1);

			\draw[ultra thick,red] (1.6,3.2)--(2.4,3.2);
			\draw[ultra thick,red] (1.2,3.6)--(1.2,4.4);
			\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			\draw[ultra thick,brown] (0,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.4);


		\end{tikzpicture}} \caption{}
\label{fig:3d} \end{subfigure} \begin{subfigure}[b]{.33\textwidth}
\centering \resizebox{!}{2.5cm}{ \begin{tikzpicture}
			\draw[ultra thick,brown] (.5,5.6)--(.5,4.4);
			\draw[ultra thick,brown] (5.5,5.6)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,brown] (.2,.4)--(.8,.4);
			\draw[ultra thick,brown](5,.2)--(5,0);
			\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			\draw[ultra thick,brown] (0,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			
			\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.4);
			\draw[ ultra thick](-1.5,-1.5) rectangle (6.5,6.5);
			\draw[ultra thick] (0,0) rectangle (6,6);
			
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](1.2,2.4)--(4.8,2.4)--(4.8,3.6)--(1.2,3.6)--(1.2,3.4)--(4.6,3.4)--(4.6,2.6)--(1.4,2.6)--(1.4,3.2)--(1.2,3.2)--(1.2,2.4);

			\draw[ultra thick](2.4,2.8) rectangle (4,3.2);
			\draw[ultra thick](1.6,3.4)--(1.6,2.6);
			\draw[ultra thick](4,3.2)--(4.3,3.2)--(4.3,2.6);
			
			
			\draw[ultra thick] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);

			
			\draw[ultra thick,brown] (.5,5.3)--(.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);
			\draw[ultra thick,red] (-1,-1.5)--(-1,6.5);
			\draw[ultra thick,red] (6,-1.5)--(6,6.5);
			\draw[ultra thick,red] (-1,6)--(6,6);
			\draw[ultra thick,red] (-1,-1)--(6,-1);	
			\draw[ultra thick,red] (1.6,3.2)--(2.4,3.2);
			\draw[ultra thick,red] (1.2,3.6)--(1.2,4.4);
			\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			\draw[ultra thick,brown] (,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.6);

			\draw[ultra thick,orange](-1,6)--(6,6)--(6,-1)--(-1,-1)--(-1,6);
			\draw[ultra thick,orange](0,4.4)--(.5,4.4)--(.5,5.3)--(0,5.3)--(0,4.4);
			\draw[ultra thick,orange](5.5,4.4)--(5.5,5.3)--(6,5.3)--(6,4.4)--(5.5,4.4);
			\draw[ultra thick,orange](.2,1.2)--(1,1.2)--(1,.4)--(.2,.4)--(.2,1.2);
			\draw[ultra thick,orange](1,1.6)--(1,.2)--(5,.2)--(5,1.6);
			
			\draw[ultra thick, orange] (1.6,4.4)--(1.6,5.6)--(4.4,5.6)--(4.4,4.4);
			\draw[ultra thick,orange] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(1.6,4.4);	
			\draw[ultra thick,orange] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick,orange] (1.2,2.4) rectangle (4.8,3.6);
			\draw[ultra thick,orange](1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);
			%\draw[ultra thick,orange](1.4,3.6)--(1.4,2.4);
			\draw[ultra thick,orange](1.6,3.2)--(1.6,2.6)--(4.3,2.6)--(4.3,3.2)--(1.6,3.2);
			\draw[ultra thick,orange] (1.6,3.4) rectangle (4.6,2.6);

		\end{tikzpicture}} \caption{}
\label{fig:3e} \end{subfigure} \begin{subfigure}[b]{.32\textwidth}
\centering \resizebox{!}{2.5cm}{ \begin{tikzpicture}
			\draw[ultra thick,brown] (.5,5.6)--(.5,4.4);
			\draw[ultra thick,brown] (5.5,5.6)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,brown] (.2,.4)--(.8,.4);
			\draw[ultra thick,brown](5,.2)--(5,0);
			%\draw[ultra thick,brown] (1.2,3.6)--(0.4,3.6);
			\draw[ultra thick,brown] (0,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			%\draw[ultra thick,brown] (1.4,3.4)--(1.4,2.4);
			%\draw[ultra thick,brown] (4.6,3.2)--(4.6,2.4);
			\draw[ ultra thick](-1.5,-1.5) rectangle (6.5,6.5);
			\draw[ultra thick] (0,0) rectangle (6,6);
			\draw[ultra thick] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick] (2,3.2) rectangle (5.6,4.4);
			\draw[ultra thick] (5.2,5.3) rectangle (6,6);		
			\draw[ultra thick] (.8,5.3) rectangle (0,6);
			\draw[ultra thick] (5.2,.7) rectangle (6,0);
			\draw[ultra thick] (.8,.7) rectangle (0,0);
	
			%\draw[ultra thick](.4,3)--(1.2,3);	
			
			\draw[ultra thick](2,3.2)--(5.6,3.2)--(5.6,4.4)--(2,4.4)--(2,4.2)--(5.4,4.2)--(5.4,3.4)--(2.2,3.4)--(2.2,4)--(2,4)--(2,3.2);

			\draw[ultra thick](3.5,3.6) rectangle (5.1,4);
			\draw[ultra thick](2.4,4.2)--(2.4,3.4);
			\draw[ultra thick](4.8,4)--(5.1,4)--(5.1,3.4);
			
			\draw[ultra thick] (1.6,4.4)--(2.8,4.4)--(2.8,5)--(4.4,5)--(4.4,4.4)--(4.4,5.6)--(1.6,5.6)--(1.6,4.4);


			\draw[ultra thick,brown] (.5,5.3)--(.5,4.4);
			\draw[ultra thick,blue] (.8,5.6)--(5.2,5.6);
			\draw[ultra thick,blue] (5.5,5.3)--(5.5,4.4);
			\draw[ultra thick,brown] (5.2,.7)--(5.2,1.6);
			\draw[ultra thick,blue] (5.2,.5)--(5,.5);

			\draw[ultra thick,blue] (.5,5)--(.2,5)--(.2,.7);
			\draw[ultra thick,blue] (.2,1.2)--(1,1.2);
			\draw[ultra thick,blue] (.8,.4)--(1,.4);
			\draw[ultra thick,blue] (1,1.6)--(1,.2)--(5,.2)--(5,1.2)--(5.8,1.2)--(5.8,4.8)--(5.5,4.8);

			\draw[ultra thick,brown] (2,4.4)--(1.2,4.4);
			\draw[ultra thick,brown] (,5.6)--(6,5.6);
			\draw[ultra thick,brown] (0,4.4)--(6,4.4);
			\draw[ultra thick,brown] (.2,4.4)--(.2,0);
			\draw[ultra thick,brown] (5.8,4.4)--(5.8,0);
			\draw[ultra thick,brown] (5.8,1.6)--(.2,1.6);
			\draw[ultra thick,brown] (1,1.6)--(1,0);
			\draw[ultra thick,brown] (2.2,4.2)--(2.2,3.2);
			\draw[ultra thick,brown] (5.4,4)--(5.4,3.4);

			\draw[ultra thick,orange] (2.2,1.6)--(3.4,1.6)--(3.4,1)--(5,1)--(5,1.6)--(5,.4)--(2.2,.4)--(2.2,1.6);

			\draw[ultra thick,orange](-1,6)--(6,6)--(6,-1)--(-1,-1)--(-1,6);
			\draw[ultra thick,orange](0,4.4)--(.5,4.4)--(.5,5.3)--(0,5.3)--(0,4.4);
			\draw[ultra thick,orange](5.5,4.4)--(5.5,5.3)--(6,5.3)--(6,4.4)--(5.5,4.4);
			\draw[ultra thick,orange](.2,1.2)--(1,1.2)--(1,.4)--(.2,.4)--(.2,1.2);
			\draw[ultra thick,orange](1,1.6)--(1,.2)--(5,.2)--(5,1.6);
			%\draw[ultra thick,green](1.6,4.4)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(2.2,1.6);
			%\draw[ultra thick,green] (1.6,4.4)--(2.2,4.4)--(2.2,5)--(3.8,5)--(3.8,4.4)--(1.6,4.4);	
			\draw[ultra thick,orange] (.4,1.6) rectangle (5.6,4.4);
			\draw[ultra thick,orange] (2,3.2) rectangle (5.6,4.4);
			%\draw[ultra thick,green](1.6,1.6)--(2.2,1.6)--(2.2,1)--(3.8,1)--(3.8,1.6)--(4.4,1.6)--(4.4,.4)--(1.6,.4)--(1.6,1.6);
			%\draw[ultra thick,green](1.4,3.6)--(1.4,2.4);
			\draw[ultra thick,orange](2.4,4)--(2.4,3.4)--(5.1,3.4)--(5.1,4)--(2.4,4);
			\draw[ultra thick,red] (-1,-1.5)--(-1,6.5);
			\draw[ultra thick,red] (6,-1.5)--(6,6.5);
			\draw[ultra thick,red] (-1,6)--(6,6);
			\draw[ultra thick,red] (-1,-1)--(6,-1);
			\draw[ultra thick,orange] (1.6,4.4)--(1.6,5.6)--(4.4,5.6)--(4.4,4.4)--(1.6,4.4);
			\draw[ultra thick,orange](2,3.2)--(2,3.6);
			\draw[ultra thick, orange](2.8,4.4)--(2.8,5)--(4.4,5);
			\draw[ultra thick,orange] (2.4,4.2) rectangle (5.4,3.4);

		\end{tikzpicture}} \caption{}
\label{fig:3f} \end{subfigure} \caption{(a): Corridor decomposition, (b): Blue lines convert corridors into
open corridors with no $\Zc$-bends, red lines bound rings into boxes,
(c): Red lines also divide spiral corridors into corridors with at
most $3$ bends, we convert outermost ring to boundary-$\Lc$, (d):
brown lines denote guillotine cuts dividing a $\Bc$-corridor into
$O(1)$ $\Bc$-corridors which are guillotine separable, (e): Orange
lines define the bounding boxes, (f): Final $\Bc\Lc$-decomposition.
See Section \ref{sec:bl} for details.}
\label{fig:cnew} 
\end{figure}

%\arir{Should we remove red lines from fig 2.}
%%%%%%. Fig

\begin{comment}
In G{á}lvez et al.~\cite{GalvezGHI0W17}, it was noted that spiral
corridors are easier to {\em process} to obtain container-based
packing. However, the processing as done in \cite{GalvezGHI0W17},
rearranges items and may violate guillotine separability. Hence, we
carefully decompose and rearrange further so that we can {\em process}
simpler substructures without violating the guillotine separability.

First, we show that any spiral open corridor and ring can be rearranged
into $O_{\eps,\epsl}(1)$ number of corridors of type $\Bc,\Lc,\Uc,\Gc$
only (see Figure \ref{fig:3a}, \ref{fig:3b}, \ref{fig:3c}). Then
we show guillotine separable bounding boxes for each of the corridors
(Figure \ref{fig:3d}). However, these corridors may not be boundary-corridors.
Thereafter, we convert all corridors into boundary-corridors with
an additional property that the rectangles in the boundary corridor
can be separated out using cuts parallel to the orientation of the
subcorridors in the boundary corridor (Figure \ref{fig:3e}). Boundary-corridors
are then converted so that finally all corridors are either $\Bc$-corridors
(which are also guillotine separable as a pseudoitem) or boundary-$\Lc$
corridors bounded by a guillotine separable box, giving us the final
$\Bc\Lc$-arrangement (Figure \ref{fig:3f}). Final $\Bc\Lc$-arrangement
is guillotine separable and now we can {\em process} the subcorridors
of $\Lc$ to obtain a guillotine separable container-based packing,
as described in the next section. %\arir{Add more details. You can write about $\Bc$-corridors.}
\end{comment}


==> Body5.tex <==
\section{Improved Approximation}
\subsection{$(\frac{4}{3}+\eps)$-approximation \tggkc}
\label{sec:tggkcal}
In this section, we give an overview of our algorithm for \tggkc.  
Using standard assumptions (see Section \ref{sec:inputsimplification}), we will assume that we can drop a constant number of items, and we have only skewed rectangles. For the general case, see Section \ref{w2dgk}.

%\arir{need to add reference to appendix and restatement of lemmas.}
  
\subsection{Processing of subcorridors from $\Bc\Lc$-arrangement}
From Lemma \ref{thm:ldecom}, we obtain $O_{\eps,\epsl}(1)$ number of corridors of type $\Bc$ or $\Lc$.
$\Lc$-corridors are  boundary-$\Lc$ of a guillotine separable box, which will help us to preserve the guillotine separability. 
Now we {\em process} the $\Lc$-corridors in 2 different ways (see Section \ref{prosec} for processing of corridors) to obtain $L\&C$-packing, as in \cite{GalvezGHI0W17}. 
%As they are part of boundary-$\Lc$ of a guillotine separable box, the processing preserves guillotine separability. 
First, we briefly define the processing of vertical subcorridor (see Figure \ref{fig:lproc}). We divide the subcorridor into $\frac{1}{\eps_{box}}$ strips of equal width (Figure \ref{fig:lproc}a). Items intersected by these lines are termed as \emph{kill}, items completely contained in the leftmost strip are termed as \emph{thin} and the remaining set of items in the subcorridor as \emph{fat}. We then remove \emph{thin} and \emph{kill} items from the subcorridor and form boxes with maximal rectangular subregions formed between the boundary curve and the subcorridor (Figure \ref{fig:lproc}b). We then shift the remaining items in the boxes from other subregions to left to fill in the empty subregion formed by the removal of thin items (Figure \ref{fig:lproc}c). The projections from the intersection of boxes and boundary curve are used to divide the horizontal subcorridor into similar strips. We again classify the items in this subcorridor as \emph{kill} for the items being intersected by these horizontal lines and remove them. The remaining items remain packed as they were. Note that we only remove thin items in the vertical subcorridor. These rearrangements do not violate guillotine separability of any items in the bounding box. 
After {\em processing} of all vertical subcorridors, we get a partition of $\optco \setminus \optco^{cross}$ (i.e., items contained inside the $\Bc\Lc$-arrangement) into three sets: $\optth$, $\optki$ and $\optfa$. 
Now we can use resource augmentation (see Lemma \ref{tool:container}) to get container packing of $\optfa^{cont} \subseteq \optfa$ s.t. $\profit(\optfa^{cont}) \ge (1-\eps)\profit(\optfa)$.


In second way, we process the horizontal subcorridors (analogous to the vertical corridor processing) of $\Lc$-corridors, where we only remove {\em thin} items from horizontal subcorridors. 

Each of these two different processing gives different sets $\optth$, $\optki$ and $\optfa^{cont}$. Based on these sets we classify the rectangles as follows:
%\arir{Need to explain processing in more details.}
\begin{itemize}
\item $\opt_{T}$ is the set of items which are in $\optth$ in one of the cases.
\item $\opt_{K}$ is the set of items which are in $\optki$ in one of the cases.
\item $\opt_{F}$ is the set of items which are in $\optfa^{cont}$ in both cases.
\end{itemize}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{3.5cm}{
		\begin{tikzpicture}			
			%\draw[thick] (0,0) rectangle (6,6);
			%box
			\draw[ultra thick](2.5,6)--(2.5,2.5)--(6,2.5)--(6,0)--(0,0)--(0,6)--(2.5,6);
			%boundary curve
			%--(6,2.5)--(6,0)--(0,0);
		
			%strips
			\draw[ultra thick] (.5,0.24) -- (.5,6.2);
			\draw[ultra thick] (1,0.73) -- (1,6.2);
			\draw[ultra thick](1.5,0.98) -- (1.5,6.2);
			\draw[ultra thick](2,1.48) -- (2,6.2);
			\draw[ultra thick](2.5,1.98)--(2.5,6.2);


			\draw[thick](0,0)--(.25,0)--(.25,.06)--(.28,.06)--(.28,.12)--(.34,.12)--(.34,.18)--(.4,.18)--(.4,.24)--(.51,.24)--(.51,.35)--(.6,.35)--(.6,.43)--(.67,.43)--(.67,.49)--(.76,.49)--(.76,.63)--(.88,.63)--(.88,.73)--(1.01,.73)--(1.01,.87)--(1.25,.87)--(1.25,.98)--(1.51,.98)--(1.51,1.19)--(1.75,1.19)--(1.75,1.48)--(2.01,1.48)--(2.01,1.75)--(2.25,1.75)--(2.25,2.02)--(2.5,2.02)--(2.5,2.5)--(6,2.5)--(6,0)--(0,0);
			%horizontal items
			\draw[solid, fill=lightgray] (.26,0) rectangle (6,.06); \draw[solid, fill=lightgray] (.28,.06) rectangle (6,.12); \draw[solid, fill=lightgray] (.34,.12) rectangle (6,.18); \draw[solid, fill=lightgray] (.40,.18) rectangle (6,.24);
			\draw[solid, fill=lightgray] (.51,.26) rectangle (6,.35);\draw[solid, fill=lightgray] (.6,.35) rectangle (6,.43); \draw[solid, fill=lightgray] (.67,.43) rectangle (6,.49);
			\draw[solid, fill=lightgray] (.76,.51) rectangle (6,.63); \draw[solid, fill=lightgray] (.88,.63) rectangle (6,.73);
			\draw[solid, fill=lightgray] (1.01,.76) rectangle (6,.87); \draw[solid, fill=lightgray] (1.25,.87) rectangle (6,.98);
			\draw[solid, fill=lightgray] (1.51,1.01) rectangle (6,1.19); \draw[solid, fill=lightgray] (1.75,1.19) rectangle (6,1.4);
			\draw[solid, fill=lightgray] (2.01,1.43) rectangle (6,1.7);  \draw[solid, fill=lightgray] (2.25,1.75) rectangle (6,1.9);
			\draw[solid, fill=lightgray] (2.52,1.95) rectangle (6,2.3);
			
			%vertical items
			\draw[solid, pattern=north west lines] (0.05,0.15) rectangle (.15,6);
			\draw[solid, fill=darkgray, pattern=north west lines] (.2,.2) rectangle (.35,6);
			\draw [solid, pattern=north east lines] (.45,.6) rectangle (.65,6);
			%\draw[solid, fill=gray, pattern=north west lines] (.6,.52) rectangle (.7,6);
			\draw[solid, fill=darkgray] (.8,.8) rectangle (.95,6);
			\draw[solid, fill=darkgray] (1.1,1.12) rectangle (1.4,6);
			\draw[solid, fill=darkgray] (1.62,1.62) rectangle (1.9,6);
			\draw[solid, fill=darkgray] (2.22,2.12) rectangle (2.4,6);
\draw[ultra thick, red](0,0)--(.25,0)--(.25,.06)--(.28,.06)--(.28,.12)--(.34,.12)--(.34,.18)--(.4,.18)--(.4,.24)--(.51,.24)--(.51,.35)--(.6,.35)--(.6,.43)--(.67,.43)--(.67,.49)--(.76,.49)--(.76,.63)--(.88,.63)--(.88,.73)--(1.01,.73)--(1.01,.87)--(1.25,.87)--(1.25,.98)--(1.51,.98)--(1.51,1.19)--(1.75,1.19)--(1.75,1.48)--(2.01,1.48)--(2.01,1.75)--(2.25,1.75)--(2.25,2.02)--(2.5,2.02)--(2.5,2.5);
%			\draw[solid, fill=gray, pattern=north west lines] (.2,.2) rectangle (.35,6);
%			\draw [solid, fill=gray,pattern=north west lines] (.45,.6) rectangle (.65,6);
%			%\draw[solid, fill=gray, pattern=north west lines] (.6,.52) rectangle (.7,6);
%			\draw[solid, fill=gray, pattern=north west lines] (.8,.77) rectangle (.95,6);
%			\draw[solid, fill=gray, pattern=north west lines] (1.1,1.02) rectangle (1.4,6);
%			\draw[solid, fill=gray, pattern=north west lines] (1.62,1.52) rectangle (1.9,6);
%			\draw[solid, fill=gray, pattern=north west lines] (2.22,2.02) rectangle (2.48,6);
		 \node[below,scale=2] at (2,0) {(a)};
		\end{tikzpicture}}
		%\caption{}
		%\label{fig:lproc1}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{3.5cm}{
		\begin{tikzpicture}			
			%\draw[thick] (0,0) rectangle (6,6);
			%box
			\draw[ultra thick](2.5,6)--(2.5,2.5)--(6,2.5)--(6,0)--(0,0)--(0,6)--(2.5,6);
			%horizontal items
			\draw[solid, fill=lightgray] (.26,0) rectangle (6,.06); \draw[solid, fill=lightgray] (.28,.06) rectangle (6,.12); \draw[solid, fill=lightgray] (.34,.12) rectangle (6,.18); \draw[solid, fill=lightgray] (.40,.18) rectangle (6,.24);
			\draw[solid, fill=lightgray] (.51,.26) rectangle (6,.35);\draw[solid, fill=lightgray] (.6,.35) rectangle (6,.43); \draw[solid, fill=lightgray] (.67,.43) rectangle (6,.49);
			\draw[solid, fill=lightgray] (.76,.51) rectangle (6,.63); \draw[solid, fill=lightgray] (.88,.63) rectangle (6,.73);
			\draw[solid, fill=lightgray] (1.01,.76) rectangle (6,.87); \draw[solid, fill=lightgray] (1.25,.87) rectangle (6,.98);
			\draw[solid, fill=lightgray] (1.51,1.01) rectangle (6,1.19); \draw[solid, fill=lightgray] (1.75,1.19) rectangle (6,1.4);
			\draw[solid, fill=lightgray, pattern=north east lines] (2.01,1.43) rectangle (6,1.7); \draw[solid, fill=lightgray] (2.25,1.75) rectangle (6,1.9);
			\draw[solid, fill=lightgray, pattern=north east lines] (2.52,1.95) rectangle (6,2.3);

%strips
			\draw[ultra thick] (0,.24)--(.5,0.24) -- (.5,6);
			\draw[ultra thick] (0.5,.73)--(1,0.73) -- (1,6);
			\draw[ultra thick] (1,.98)--(1.5,0.98) -- (1.5,6);
			\draw[ultra thick] (1.5,1.48)--(2,1.48) -- (2,6);
			\draw[ultra thick] (2,1.98)--(2.5,1.98)--(2.5,6);
			
			%vertical items
%			\draw[solid, pattern=north west lines] (0.05,0.15) rectangle (.15,6);
%		\draw[solid, fill=gray] (.2,.2) rectangle (.35,6);
%			\draw [solid, pattern=north east lines] (.45,.6) rectangle (.65,6);
%			%\draw[solid, fill=gray, pattern=north west lines] (.6,.52) rectangle (.7,6);
			\draw[solid, fill=gray] (.8,.8) rectangle (.95,6);
			\draw[solid, fill=gray] (1.1,1.12) rectangle (1.4,6);
			\draw[solid, fill=gray] (1.62,1.62) rectangle (1.9,6);
			\draw[solid, fill=gray] (2.22,2.12) rectangle (2.4,6);


			\draw[ultra thick, blue] (6.2,.24)--(.5,0.24) ;
			\draw[ultra thick, blue] (6.2,.73)--(1,0.73);
			\draw[ultra thick, blue] (6.2,.98)--(1.5,0.98);
			\draw[ultra thick, blue] (6.2,1.48)--(2,1.48);
			\draw[ultra thick, blue] (6.2,1.98)--(2.5,1.98);
			
			\draw[ultra thick, red](0,0)--(0,.24)--(.5,0.24)-- (0.5,.73)--(1,0.73) --(1,.98)--(1.5,0.98)--(1.5,1.48)--(2,1.48)--(2,1.98)--(2.5,1.98)--(2.5,2.5);

%			\draw[solid, fill=gray, pattern=north west lines] (.2,.2) rectangle (.35,6);
%			\draw [solid, fill=gray,pattern=north west lines] (.45,.6) rectangle (.65,6);
%			%\draw[solid, fill=gray, pattern=north west lines] (.6,.52) rectangle (.7,6);
%			\draw[solid, fill=gray, pattern=north west lines] (.8,.77) rectangle (.95,6);
%			\draw[solid, fill=gray, pattern=north west lines] (1.1,1.02) rectangle (1.4,6);
%			\draw[solid, fill=gray, pattern=north west lines] (1.62,1.52) rectangle (1.9,6);
%			\draw[solid, fill=gray, pattern=north west lines] (2.22,2.02) rectangle (2.48,6);

		\node[below,scale=2] at (2,0) {(b)};
		\end{tikzpicture}}
		%\caption{}
		%\label{fig:lproc2}
	\end{subfigure}
	\begin{subfigure}[b]{.32\textwidth}
		\centering
		\resizebox{!}{3.5cm}{
		\begin{tikzpicture}			
			%\draw[thick] (0,0) rectangle (6,6);
			\draw[ultra thick](2.5,6)--(2.5,2.5)--(6,2.5)--(6,0)--(0,0)--(0,6)--(2.5,6);

			%horizontal items
			\draw[solid, fill=gray] (.26,0) rectangle (6,.06); \draw[solid, fill=gray] (.28,.06) rectangle (6,.12); \draw[solid, fill=gray] (.34,.12) rectangle (6,.18); \draw[solid, fill=gray] (.40,.18) rectangle (6,.24);
			\draw[solid, fill=gray] (.51,.26) rectangle (6,.35);\draw[solid, fill=gray] (.6,.35) rectangle (6,.43); \draw[solid, fill=gray] (.67,.43) rectangle (6,.49);
			\draw[solid, fill=gray] (.76,.51) rectangle (6,.63); \draw[solid, fill=gray] (.88,.63) rectangle (6,.73);
			\draw[solid, fill=gray] (1.01,.76) rectangle (6,.87); \draw[solid, fill=gray] (1.25,.87) rectangle (6,.98);
			\draw[solid, fill=gray] (1.51,1.01) rectangle (6,1.19); \draw[solid, fill=gray] (1.75,1.19) rectangle (6,1.4);
			%\draw[solid, fill=gray] (2.01,1.43) rectangle (6,1.7);
			 \draw[solid, fill=gray] (2.25,1.75) rectangle (6,1.9);
			%\draw[solid, fill=gray, pattern=north east lines] (2.52,1.95) rectangle (6,2.3);
%strips
			\draw[ultra thick] (0,.24)--(.5,0.24) -- (.5,6);
			\draw[ultra thick] (0.5,.73)--(1,0.73) -- (1,6);
			\draw[ultra thick] (1,.98)--(1.5,0.98) -- (1.5,6);
			\draw[ultra thick] (1.5,1.48)--(2,1.48) -- (2,6);
			\draw[ultra thick] (2,1.98)--(2.5,1.98)--(2.5,6);

			\draw[solid, fill=gray] (.0,.8) rectangle (.15,6);
			\draw[solid, fill=gray] (.5,1.12) rectangle (.8,6);
			\draw[solid, fill=gray] (1,1.62) rectangle (1.18,6);
			\draw[solid, fill=gray] (1.5,2.12) rectangle (1.68,6);


			\draw[ultra thick, blue] (6,.24)--(.5,0.24) ;
			\draw[ultra thick, blue] (6,.73)--(1,0.73);
			\draw[ultra thick, blue] (6,.98)--(1.5,0.98);
			\draw[ultra thick, blue] (6,1.48)--(2,1.48);
			\draw[ultra thick, blue] (6,1.98)--(2.5,1.98);

			\draw[ultra thick, red](0,0)--(0,.24)--(.5,0.24)-- (0.5,.73)--(1,0.73) --(1,.98)--(1.5,0.98)--(1.5,1.48)--(2,1.48)--(2,1.98)--(2.5,1.98)--(2.5,2.5);

		\node[below,scale=2] at (2,0) {(c)};		
		\end{tikzpicture}}
		%\caption{}
		%\label{fig:lproc3}
	\end{subfigure}
%	\begin{subfigure}[b]{.24\textwidth}
%		\centering
%		\resizebox{!}{3.2cm}{
%		\begin{tikzpicture}		
%			%\draw[thick] (0,0) rectangle (6,6);	
%			\draw[ultra thick](2.5,6)--(2.5,2.5)--(6,2.5)--(6,0)--(0,0)--(0,6)--(2.5,6);
%
%			%horizontal items
%			\draw[solid, fill=gray] (.51,0) rectangle (6,.11);\draw[solid, fill=gray] (.6,.11) rectangle (6,.19); \draw[solid, fill=gray] (.67,.24) rectangle (6,.3);
%			\draw[solid, fill=gray] (.76,.3) rectangle (6,.42); \draw[solid, fill=gray] (.88,.42) rectangle (6,.52);
%			\draw[solid, fill=gray] (1.01,.52) rectangle (6,.63); \draw[solid, fill=gray] (1.25,.73) rectangle (6,.84);
%			\draw[solid, fill=gray] (1.51,.98) rectangle (6,1.16); \draw[solid, fill=gray] (1.75,1.16) rectangle (6,1.45);
%			\draw[solid, fill=gray] (2.01,1.45) rectangle (6,1.69); \draw[solid, fill=gray] (2.25,1.69) rectangle (6,1.84);
%
%
%%strips
%			\draw[ultra thick] (0,.24)--(.5,0.24) -- (.5,6);
%			\draw[ultra thick] (0.5,.73)--(1,0.73) -- (1,6);
%			\draw[ultra thick] (1,.98)--(1.5,0.98) -- (1.5,6);
%			\draw[ultra thick] (1.5,1.48)--(2,1.48) -- (2,6);
%			\draw[ultra thick] (2,1.98)--(2.5,1.98)--(2.5,6);
%
%			\draw[solid, fill=gray] (.0,.8) rectangle (.15,6);
%			\draw[solid, fill=gray] (.5,1.12) rectangle (.8,6);
%			\draw[solid, fill=gray] (1,1.62) rectangle (1.18,6);
%			\draw[solid, fill=gray] (1.5,2.12) rectangle (1.68,6);
%
%
%			\draw[ultra thick] (6,.24)--(.5,0.24) ;
%			\draw[ultra thick] (6,.73)--(1,0.73);
%			\draw[ultra thick] (6,.98)--(1.5,0.98);
%			\draw[ultra thick] (6,1.48)--(2,1.48);
%			\draw[ultra thick] (6,1.98)--(2.5,1.98);
%		
%		\end{tikzpicture}}
%		\caption{}
%		\label{fig:lproc4}
%	\end{subfigure}
	\caption{Processing of $\Lc$-corridor.} %Figure (a): Divided Vertical Subcorridor with $\frac{1}{\eps_{box}}$ strips. Figure (b): Removed \emph{thin} and \emph{kill} items from vertical subcorridor, formed boxes and extended projections (shown in blue) from intersection of boxes and boundary curve to divide horizontal subcorridor. Figure (c):  Shifted remaining items in vertical subcorridor to empty subregions, removed \emph{kill} items from horizontal subcorridor. (fat items are shown as dark gray, thin items with north west hash, kill items with north east hash, 
	%unprocessed items are light gray, processed items are gray 
	%and the boundary curve is shown as red). }
	\label{fig:lproc}
\end{figure}

\begin{lem}\cite{GalvezGHI0W17}
\label{ering}
For any one of the cases of processing, the following properties hold:
\begin{enumerate}
\item $|OPT_{kill}|=O_{\eps,\epsl,\epsb}(1)$;
\item For any given constant $\epsr>0$, there is a sufficiently small $\epsb>0$ such that the total height (resp.~width)of items in $\optth\cap\Rho$ (resp. $\optth\cap\Rve$) is at most $\epsr N$.
\end{enumerate}
\end{lem}

Now we classify items in the optimal packing into four sets: $\opt_{LT}, \opt_{ST}$ (long and short items in $\opt_T$, resp.),  $\opt_{LF}, \opt_{SF}$ (long and short items in $\opt_F$, resp.). \footnote{This notation is different from \cite{GalvezGHI0W17}, e.g., in our notation $|\opt_{LT}|$ can even be the same as $|\opt_{L}|$.} 	

%\subsection{Profitable Structure Packing}\label{profitstruc}
%\begin{lem}\cite{GalvezGHI0W17}\label{sumprofit}
%$\profit(\opt_{F}\cap\opt_{T})+\profit(\opt_{k})+\profit(\opt_{large})+\profit(\opt_{corr}^{cross})\geq(1-O(\eps))\profit(\opt)$.
%\end{lem}

\begin{lem}
\label{algo1}
$\profit(\opt_{L\&C})\geq\profit(\opt_{F})+\profit(\opt_{T})/2$.
\end{lem}
\begin{proof} Consider the sum of profit in both the ways of processing a subcorridor of $\Lc$-corridor as mentioned above. By definition every item in $\opt_{F}$ is included in both the cases. Items belonging to $\opt_{T}$ is saved in at least one of the cases. 
\end{proof}

Now we show a more involved $L\&C$-packing that packs almost $|T|+|F|/2$ items. 
\begin{lem}
\label{algo3}
$\profit(\opt_{L\&C})\geq\profit(\opt_{T})+(1-O_{\eps}(1))\profit(\opt_{F})/2$.
\end{lem}
\begin{proof}[Proof sketch]
We give a proof sketch here, for the detailed proof, see Section \ref{sec:tggkcfull}.
Let $w_L N$ (resp. $w_{LT} N$) be the total width of vertical items in $\optln$ (resp. $\opt_{LT}$) and 
$h_L N$ (resp. $h_{LT} N$) be the total height of horizontal items in $\optln$ (resp. $\opt_{LT}$).
W.l.o.g.~assume $w_L \le h_L$ (the other case is analogous). 
Then  $w_L \le 1/2, h_L \le 1$, $w_{LT},h_{LT}   \le \epsr$ (from Lemma \ref{ering}), and  all long items can be packed in a boundary-$\Lc$  with width $w_L N$ and height $h_L N$ in $[0,N]\times [0,N]$ box (from Lemma \ref{lpackinglem}).  Consider some small positive constant $\tilde{\eps}\le \frac12$ that we will choose later. 
For simplicity, we assume $w_L \ge \frac{\epsr}{\tilde{\eps}}$ and $h_L \ge \frac{\epsr}{\tilde{\eps}}$.
 
Now from vertical arm of  boundary-$\Lc$, we
choose  a random vertical strip $[\tilde{x}, \tilde{x}+\frac{w_L N}{2}+w_{LT} N] \times [0,N]$ (if $\tilde{x}+\frac{w_L}{2} N+w_{LT} N\le w_L N$) or two strips $([\tilde{x}, w_L N]  \times [0,N]) \cup ([0, \tilde{x}+\frac{w_L N}{2}+w_{LT} N -w_L N] \times [0,N]$ (if $\tilde{x}+\frac{w_L N}{2}+w_{LT} N> w_L N$), where $\tilde{x}$ is chosen uniformly at random from $[w_L]$. We remove all fat items intersecting with this strip.
We do similar operation on horizontal arm and remove all fat items intersecting such random horizontal strip(s) of total width $\frac{h_L}{2} N+h_{LT} N$.

By averaging argument, the remaining items have profit $\frac{\big(1-O_{\epsl, \epsr, \tilde{\eps}}(1)\big)}{2}\cdot \opt_{LF}+\opt_{LT}$ and packed in boundary-$\Lc$ of width $\le w_L N/2$ and height $\le h_L N/2$ (as shown in figure \ref{fig:c6}a).
In the remaining rectangular region of the box, we will place containers. 
Now we place items in $\opt_{ST}$ in two containers next to boundary-$\Lc$.
First, we place a container of height $N/2$ and width $\epsr N$, with its bottom-left corner at  $(\frac{w_L N}{2}, \frac{N}{2})$,  containing items in $\opt_{ST}$  coming from vertical subcorridors in the processing and then we place a container of width $N/2$ and height $\epsr N$, with its bottom-left corner at  $(\frac{N}{2}, \frac{h_L N}{2})$, containing items in $\opt_{ST}$  coming from horizontal  subcorridors in the processing.
As $w_L\le 1/2$, i.e., $1-w_L/2\ge 3/4$,  these two containers do not overlap. 
Now we are left with a rectangular region of width  $N\big(1-\frac{w_L}{2}-O_{\epsr}(1)\big)$ and height $N\big(1-\frac{h_L}{2}-O_{\epsr}(1)\big)$. We will use slightly smaller region of width $N\big(1-\frac{w_L}{2}-O_{\epsr}(1)-\eps\big)$ and height $N\big(1-\frac{h_L}{2}-O_{\epsr}(1)-\eps\big)$ to show existence of a guillotine packing by Steinberg's Algorithm (Lemma \ref{lem:steinbeg}). However, Steinberg's algorithm may not give a container-based packing. Hence, we use resource augmentation (Lemma \ref{lemma1}) using the extra $\eps$-strips to obtain a container-based guillotine packing. This along with boundary-$\Lc$ will give an $L\&C$-packing.
Using Steinberg's algorithm, we can pack any subset of items  in $\opt_{SF}$ of total area at most 
 $\frac{N^2}{2}\big(1-\frac{(w_L+h_L)}{2}-O_{\epsr,\eps}(1)\big)$.
On the other hand, the total area of rectangles in $\opt_{SF}$ is at most $N^2\big(1-\frac{w_L+h_L}{2}-O_{\epsr}(1)\big)$.
So, consider rectangles in $\opt_{SF}$ in non-decreasing order of area till they reach $N^2\big(1-\frac{(w_L+h_L)}{2}-O_{\epsr}(1)\big)$.
These items can be packed in the remaining region and have total profit $\ge ( \profit({\opt_{SF}}) \cdot \big(1-O_{\epsr,\eps}(1)\big)/2$.
Thus we have an $L\&C$-packing (as shown in figure \ref{fig:c6}b) with profit  $\profit(\opt_{LT})+\profit(\opt_{ST})+(\profit(\opt_{LF}+\profit(\opt_{SF}))\cdot  \frac{\big(1-O_{\epsr, \eps}(1)\big)}{2}$.
\end{proof}

From Lemma \ref{algo1} and \ref{algo3}, we get $\profit(OPT_{L\&C})\geq(\frac{3}{4}-O(\eps))\profit(\opt)$.
\begin{thm}
%\label{LC}
Let $OPT_{L\&C}$ be the most profitable guillotine separable $L\&C$ packing  solution and $\opt$ be the optimal  packing for \tggkc. Then $\profit(OPT_{L\&C})\geq(\frac{3}{4}-O(\eps))\profit(\opt)$.
\end{thm}

\begin{figure}[h]
	%\centering
	\captionsetup[subfigure]{justification=centering}
	\hspace{-10pt}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}		

			\draw[thick] (0,0) rectangle (6,6);
			% L boundary
			\draw[solid, fill=lightgray] (0,0)--(0,6)--(2.5,6)--(2.5,2.5)--(6,2.5)--(6,0)--(0,0);
		
			% vertical items
			\draw[solid, fill=darkgray] (0,0)rectangle(.15,6);
			\draw[solid, fill=darkgray] (.15,.15)rectangle(.3,6);
			\draw[solid, fill=darkgray] (.3,.3)rectangle(.45,6);
			\draw[solid, fill=darkgray] (.45,.45)rectangle(.6,6);

			\draw[solid, fill=gray] (.61,.75)rectangle(1,6);
			\draw[solid, fill=gray] (1.1,1)rectangle(1.5,6);
			\draw[solid, fill=gray] (1.7,1.5)rectangle(2.1,6);
			\draw[solid, fill=gray] (2.1,2.13)rectangle(2.5,6);
		
			% horizontal items
			\draw[solid, fill=darkgray] (0.17,0)rectangle(6,.13);
			\draw[solid, fill=darkgray] (0.32,.17)rectangle(6,.28);
			\draw[solid, fill=darkgray] (0.47,0.32)rectangle(6,.43);
			\draw[solid, fill=darkgray] (0.62,0.47)rectangle(6,.58);

			\draw[solid, fill=gray] (1.03,.59)rectangle(6,1.09);
			\draw[solid, fill=gray] (1.53,1.1)rectangle(6,1.6);
			\draw[solid, fill=gray] (2.13,1.71)rectangle(6,2.11);
			\draw[solid, fill=gray] (2.53,2.12)rectangle(6, 2.5);

			% strips
			\draw [thick, pattern=north west lines] (.6,6)--(1.7,6)--(1.7, 1.61)--(1.5,1.61)--(1.5,1.09)--(1,1.09)--(1,.75)--(.6,.75)--(.6,6);
			\draw[thick, pattern = north west lines] (6,.59)--(6,1.71)--(2.13,1.71)--(2.13,1.61)--(1.53,1.6)--(1.53,1.1)--(1.03,1.1)--(1.03,.59)--(6,.59);

			\draw (7,1.3) node {\large \textbf{$h_{L}N$}};
			\draw (1.3,7.4) node {\large \textbf{$w_{L}N$}};
			

			
			\draw [thick,decorate,decoration={brace,amplitude=8pt}] (0,6.7) -- (2.5,6.7); 

			\draw [thick,decorate,decoration={brace,amplitude=8pt}] (6.3,2.5) -- (6.3,0); 


			\draw (7.2,4.2) node {\large \textbf{$h_{LT}N + \frac{h_{L}}{2}N$}};
			\draw [->](6.3,1.15)--(6.3,4);

			\draw (5.3,6.3) node {\large \textbf{$w_{LT}N + \frac{w_{L}}{2}N$}};
			\draw [->](1.15,6.3)--(4,6.3);
			
			\draw [thick,decorate,decoration={brace,amplitude=8pt}] (.6,6) -- (1.7,6); 

			\draw [thick,decorate,decoration={brace,amplitude=8pt}] (6,1.71) -- (6,0.59); 
			 \node[below,scale=2] at (2,0) {(a)};
			
		\end{tikzpicture}}
		%\caption{}
		%\label{fig:c61}
	\end{subfigure}
	\begin{subfigure}[b]{.5\textwidth}
		\centering
		\resizebox{!}{4cm}{
		\begin{tikzpicture}		
			\draw[thick] (0,0) rectangle (6,6);	
			% L boundary
			\draw[solid, fill=lightgray] (0,0)--(0,6)--(1.5,6)--(1.5,1.5)--(6,1.5)--(6,0)--(0,0);

			% vertical items
			\draw[solid, fill=gray] (0,0)rectangle(.15,6);
			\draw[solid, fill=gray] (.15,.15)rectangle(.3,6);
			\draw[solid, fill=gray] (.3,.3)rectangle(.45,6);
			\draw[solid, fill=gray] (.45,.45)rectangle(.6,6);

			%\draw[solid, fill=gray] (.61,.75)rectangle(1,6);
			%\draw[solid, fill=gray] (1.1,1)rectangle(1.5,6);
			\draw[solid, fill=gray] (.6,1.5)rectangle(1,6);
			\draw[solid, fill=gray] (1.1,2)rectangle(1.5,6);

			% horizontal items
			\draw[solid, fill=gray] (0.17,0)rectangle(6,.13);
			\draw[solid, fill=gray] (0.32,.17)rectangle(6,.28);
			\draw[solid, fill=gray] (0.47,0.32)rectangle(6,.43);
			\draw[solid, fill=gray] (0.62,0.47)rectangle(6,.58);

			%\draw[solid, fill=gray] (1.03,.59)rectangle(6,1.09);
			%\draw[solid, fill=gray] (1.53,1.1)rectangle(6,1.6);
			\draw[solid, fill=gray] (2.03,.61)rectangle(6,1.11);
			\draw[solid, fill=gray] (2.53,1.12)rectangle(6, 1.5);

			% strips
			%\draw [thick, pattern=north west lines] (.7,6)--(1.3,6)--(1.3, 1.2)--(1,1.2)--(1,.75)--(.7,.75)--(.7,6);
			%\draw[thick, pattern = north west lines] (6,.7)--(6,1.4)--(1.53,1.4)--(1.53,1.1)--(1.03,1.1)--(1.03,.7)--(6,.7);
			
			% steinberg
			\draw [solid, fill= lightgray] (6,6)rectangle(2.3,2.3);

			%ST
			\draw [solid, fill= lightgray] (1.6,6)rectangle(2.2,3.1);
			\draw [solid, fill= lightgray] (6,1.6)rectangle(3.1,2.2);

			%vertical items ST
			\draw[solid, fill=gray] (1.6,3.15)rectangle(1.75,6);
			\draw[solid, fill=gray] (1.75,3.25)rectangle(1.9,6);
			\draw[solid, fill=gray] (1.9,3.35)rectangle(2.05,6);
			\draw[solid, fill=gray] (2.05,3.45)rectangle(2.2,6);
			% horizontal ST
			\draw[solid, fill=gray] (3.15,1.6)rectangle(6,1.75);
			\draw[solid, fill=gray] (3.25,1.75)rectangle(6,1.9);
			\draw[solid, fill=gray] (3.35,1.9)rectangle(6,2.05);
			\draw[solid, fill=gray] (3.45,2.05)rectangle(6,2.2);

			% items in steinberg
			\draw (6,6)rectangle(4,4);
			\draw[solid, fill=gray] (5.9,5.9)rectangle(4.1,4.1);

			\draw(2.3,3.7) rectangle (3.7,6);
			\draw[solid, fill=gray] (2.3,3.7)rectangle(2.8,6);
			\draw[solid, fill=gray] (2.85,3.7)rectangle(3.2,5.5);
			\draw[solid, fill=gray] (3.25,3.7)rectangle(3.7,5);

			\draw(3.9,2.3) rectangle (6,3.7);
			\draw[solid, fill=gray] (3.95,2.3)rectangle(6,2.8);
			\draw[solid, fill=gray] (3.95,2.85)rectangle(5.5,3.2);
			\draw[solid, fill=gray] (3.95,3.25)rectangle(5,3.7);

			\draw (2.3,2.3) rectangle (3.5,3.5);
			\draw[solid, fill=gray] (2.3,2.3)rectangle(2.8,2.5);
			\draw[solid, fill=gray] (2.85,2.3)rectangle(3.2,2.65);
			\draw[solid, fill=gray] (3.25,2.3)rectangle(3.5,2.8);

			\draw[solid, fill=gray] (2.3,2.85)rectangle(2.5,3.1);
			\draw[solid, fill=gray] (2.55,2.85)rectangle(3,3.2);
			\draw[solid, fill=gray] (3.05,2.85)rectangle(3.2,3.3);
			\draw[solid, fill=gray] (3.25,2.85)rectangle(3.5,3.5);

			\draw [ultra thick, red] (1.6,6)rectangle(2.2,3.1);
			\draw [ultra thick, red] (6,1.6)rectangle(3.1,2.2);
			\draw [ultra thick, blue] (6,6)rectangle(2.3,2.3);
			\draw[ultra thick, green] (0,0)--(0,6)--(1.5,6)--(1.5,1.5)--(6,1.5)--(6,0)--(0,0);

			\draw (1.9,6.5) node {\large \textbf{$\epsr N$}};

			\draw (7,1.9) node {\large \textbf{$\epsr N$}};
			
			\draw [thick,decorate,decoration={brace,amplitude=8pt}] (1.6,6) -- (2.2,6); 

			\draw [thick,decorate,decoration={brace,amplitude=8pt}] (6,2.2) -- (6,1.6); 

		 \node[below,scale=2] at (2,0) {(b)};
		\end{tikzpicture}}
		%\caption{}
		%\label{fig:c62}
	\end{subfigure}
	\caption{Depiction of Case where $w_L \ge \frac{\epsr}{\tilde{\eps}}$ and $h_L \ge \frac{\epsr}{\tilde{\eps}}$ in Lemma \ref{algo3}. (a) Packing of long items. Strips with north west lines are dropped. (thin items are shown in darkgray and fat in gray) (b) Final Packing with $LF/2+LT$ in green, $ST$ in red, $SF$ in blue.}
	\label{fig:c6}
\end{figure}
Small items are handled using standard arguments  (see Section \ref{smallrec}). We find the best guillotine $L\&C$ packing using PTAS for Generalized Assignment Problem (see Section \ref{sec:findpack}).% \ref{sec:GAP}).

%\arir{Did we mention why containers obtained from guillotine separable boxes are guillotine separable?}

\subsection{$(\frac{5}{4}+\eps)$-approximation \tggkcr}
Using a similar approach as above and techniques based on resource contraction from \cite{GalvezGHI0W17}, we obtain the following theorem. 
See Section \ref{sec:tggkcrfull} for the proof. 
\begin{thm}
\label{LCR}
For any constant $\eps>0$, there exists a polynomial time $\frac54+\eps$-approximation algorithm for $\tggkcr$.
\end{thm}

\subsection{Weighted case}
In weighted case, we can no longer drop $O(1)$ number of items. So we use standard shifting argumentation \cite{GalvezGHI0W17} and  exploit guillotine cuts to obtain slightly weaker  improved approximation. See Section \ref{w2dgk} and \ref{subs:tggkr} for the proof for \tggk, \tggkr, respectively. 

\begin{lem}
For any constant $\eps>0$, there exists a polynomial time $\frac32+\eps$-approximation and $\frac43+\eps$-approximation  algorithm for $\tggk$, $\tggkr$, respectively.
\end{lem}

\subsection{Limitation of stage packing}
We show that for \tgk, unlike  2BP or 2SP, any guillotine packing can not be approximated arbitrarily well by $O(1)$-stage packing. See Section \ref{sec:smallstage} for the proof.
\begin{thm}
For any $\eps \in (0, \frac{1}{2})$, $k=O(\eps \log N)$, 
there exists a \tggk~instance $\R$ so that for any $\R' \subseteq \R$ with $|\R|\leq(2 - \eps)|\R'|$, $\R'$ can not have a $k$-stage packing into $N \times N$ knapsack.
\end{thm}


==> L-compart.tex <==
\section{Proof of Lemma \ref{lem:make-L-nice}}
In this section, we give a detailed proof of Lemma \ref{lem:make-L-nice}. 
First, we prove the following lemma, which will be useful in the proof.


\begin{lem}\label{lem:A}
	[9A] There exists a set $OPT'\subseteq \opt$, $p(\opt') > (1-\eps)p(\opt)$ and a partition of $K$ 
	into a set of $O_{\eps}(1)$ compartments such that for every $\Lc$-compartment $L$ it holds that
	for each item $i$ contained in the horizontal  $P_H$ (resp. vertical arm $P_V$) of $L$, $\height(i)\le \eps^{4} \cdot\height(P)$ 
	(resp. $\width(i)\le \eps^{4} \cdot\width(P)$).
\end{lem}
\begin{proof}
	For an $\Lc$ compartment $L$, we use $P_H$ (resp. $P_V$) to denote the horizontal (resp. vertical) arm of $L$.
	In the cardinality case, we simply drop all the items of $\height(i) > \eps^{4} \cdot\height(P_H)$. 
	Number of such items can be at most $\frac{1}{\eps^4 \eps_{large}}$ which is a constant.
	Thus we get the required packing of rest of the items $\opt'$ s.t. $|\opt'| \leq (1-O_{\eps \eps_{large}}(1))|\opt|$.
	
	For weighted case, we cannot drop these $\frac{1}{\eps^4 \eps_{large}}$ as they might actually carry most of the profit of knapsack. Thus, we now aim to pack back this constant number of items dropped. We do this by dividing the knapsack into a non-uniform grid along the boundary of these items and observing the profit of items dropped as a result of processing the items which are classified depending on the grid. Using standard averaging argument, we can claim that recursively doing the same procedure for $\frac{1}{\eps}$ times, we get a set of items which can be dropped and have a profit of at most $O(\eps).p(\opt)$.

Formally, we employ a shifting argumentation. We define a family of disjoint sets of items $\{ K(0), K(1), ... , K(t) \}$, $t < \frac{1}{\eps}$, each containing at most $O_{\eps \eps_{large}}(1)$ number of items. We also define $\kappa(t) = \cup_{i=0}^{t}K(i)$. Intuitively, $\kappa(t)$ will be the set of items which are not allowed to be dropped in the $t^{th}$ iteration. For base case, we begin by adding all the items $\{ i | \height(i) > \eps^{4} \cdot\height(P_H)~or~\width(i) > \eps^{4} \cdot\width(P_V)  \}$ to $K(0)$, which are at most $O_{\eps,\epsl}(1)$ in number. If $p(K(0)) \leq \eps.p(\opt)$, then we stop and drop all items of $K(0)$ as the rest of items will have profit at least  $(1-\eps)p(\opt)$. Otherwise, we perform the procedure recursively. Consider that we are at the $t^{th}$ iteration, denote $G(t)$ as the non-uniform grid formed by extending the $x$, $y$ coordinates of the items in $\kappa(t)$(which we obtained from previous $t-1$ iterations). Consider $C_{t}$ to be the set of grid cells of $G(t)$. We classify items in the knapsack as small, large, horizontal, vertical as before depending on its intersection with the cells it overlaps. Let $\opt(C)$ denote the set of items from $OPT$ intersecting with grid cell C. This gives us the following partition of items inside cell $C$:
\begin{enumerate}
\item $\opt_{ver}(C) = \{ i~|~ \forall i\in C$ s.t. $ \height(i \cap C)$ $>$ $\eps_{large}$ $\height(C)$ and $\width(i \cap C)$ $\leq$ $\eps_{small}$ $\width(C)$ $\}$, 

\item $\opt_{hor}(C)= \{ i~ | ~\forall i\in C$ s.t. $\height(i \cap C)$ $\leq$ $\eps_{small}$ $\height(C)$ and $\width(i \cap C)$ $>$ $\eps_{large}$ $\width(C)$ $\}$, 

\item $\opt_{large}(C)$ $= \{ i~ |~ \forall i\in C$ s.t. $\height(i \cap C)$ $>$ $\eps_{large}$ $\height(C)$ and $\width(i \cap C)$ $>$ $\eps_{large}$ $\width(C)$ $\}$, 

\item $\opt_{small}(C)$ $= \{ i ~| ~\forall i\in C$ s.t.  $\height(i \cap C)$ $\leq$ $\eps_{small}$ $\height(C)$ and $\width(i \cap C)$ $\leq$ $\eps_{small}$ $\width(C)$ $\}$, 

\item $\opt_{intermediate}(C)$ $= \{ i ~| ~\forall i\in C$ s.t. $\height(i \cap C)$ $\in$ $(\eps_{small}$ $\height(C)$,  $(\eps_{large}$ $\height(C)]$ or  $\width(i \cap C)$ $\in$ $(\eps_{small}$ $\width(C)$,  $(\eps_{large}$ $\width(C)]$ $\}$, 

\item $\opt_{skew}(C)$ $=$  $\opt_{hor}(C) \cup \opt_{ver}(C)$.
\end{enumerate}
%Consider $\opt(C)$ to be the set of items in $\opt$ having a non-empty intersection with grid cell $C$. We define $\opt_{hor}(C)$, $\opt_{ver}(C)$, $\opt_{large}(C)$, $\opt_{small}(C)$, $\opt_{intermediate}(C)$ and $\opt_{skew}(C)$ to be set of items in intersection of $\opt(C)$ with $\opt_{hor}(C)$, $I_{ver}(C)$, $I_{large}(C)$, $I_{small}(C)$, $I_{intermediate}(C)$ and $I_{skew}(C)$ respectively.

Using Lemma~\ref{class}, we can fix $\eps_{small}$ and $\eps_{large}$ according to our convenience ensuring that the 
profit of items classified as intermediate for any cell is at most 
$\eps. \profit(\opt)$ such that $\eps$ $\geq$ $\eps_{large}$ $\geq$ $f(\eps_{small})$ $\geq$ $\omega_{\eps}(1)$, 
for some positive increasing function $f(.)$ . We add items from $\opt_{large}(C_t)$ (not contained in $\kappa(t)$) to $K(t+1)$ for all $C$ 
not fully covered by any item in $\kappa(t)$. This adds a constant number of items to $K(t+1)$. For simplification, we can stretch this non-uniform
 grid to a uniform $1\times1$ grid where each cell is of same dimension. Clearly, we can map any decomposition done in this uniform grid back to original knapsack, mapping back any guillotine cuts in the uniform grid as well, thereby conserving guillotine separability of items. In this process, skew items may stretch by a factor of $\frac{1}{1+|2.\kappa(t)|}$ or more i.e. for each cell $C$, each item in $\opt_{skew}(C)\setminus \kappa(t)$ 
has its longer dimension (width for $\opt_{hor}$ and height for $\opt_{ver}$) at least $\eps_{large}.\frac{1}{1+2.|\kappa(t)|}$.

Now we can do a decomposition into box- and $\Lc$-compartments as done in previous sections, considering only skew items in the cells i.e. $\opt_{skew}(C_t) = \cup_{\forall C \in C_t}\opt_{skew}(C)$. We add the items dropped during the decomposition to $K(t+1)$, which is again a constant number of items. After obtaining the compartments, we may have a set of troublesome items (disjoint from $\kappa(t)$) containing every item $i$ inside $\Lc$-compartment $L$ such that $\height(i) > \eps^{4} \cdot\height(P_H)$ for horizontal arm $P_H$ of $L$ (analogous statement for vertical arms). We directly add these items to $K(t+1)$. As claimed in cardinality case, number of such items can be at most $O_{\eps, \epsl}(1)$.

This way we repeatedly perform the same process for at most ${1}/{\eps}$ iterations ensuring $\kappa(t)$ being untouchable set of items in $t^{th}$ iteration as before. Now, we exploit the fact that sets $K(0), K(1), ..., K(t)$ are pairwise disjoint and have constant number of items. If the profit of items in $K(t)$ at any iteration $t$ is at most $\eps \profit(\opt)$ we get the desired set of items and halt. Otherwise, using a averaging argument, we can claim that $p(K(t+1)) \leq \eps. p(\opt)$. This way we drop $K(t+1)$ obtaining the $\Lc$-compartments satisfying the given condition. Thus we obtain a packing of items $\opt'$ with profit at least $(1-O(\eps))p(\opt)$ in at most ${1}/{\eps}$ iterations.
\end{proof}

Hence, we assume now on that for every $\Lc$-compartment $L$ it holds that
	for each item $i$ contained in the horizontal  $P_H$ (resp. vertical arm $P_V$) of $L$, $\height(i)\le \eps^{4} \cdot\height(P)$ 
	(resp. $\width(i)\le \eps^{4} \cdot\width(P)$).


Let $P_H$ and $P_V$ be the horizontal and vertical arms $L$, respectively.
So $P_H$ is defined via two horizontal edges $e_{1}=\overline{p_{1}p'_{1}}$
and $e_{2}=\overline{p_{2}p'_{2}}$, and additionally one monotone
axis-parallel curves connecting $p_{1}=(x_{1},y_{1})$ with $p_{2}=(x_{2},y_{2})$. 
Assume w.l.o.g. that $x_{1}\le x_{2}$ and that $y_{1}<y_{2}$. 
Let $h(P_H)$ denote the the height of $P_H$ which we define as the distance
between $e_{1}$ and $e_{2}$. Intuitively, we place $1/\eps^{2}$
boxes inside $P_H$ of height $\eps^{2}h(P_H)$ each, stacked one
on top of the other, and of maximum width such that they are contained
inside $P_H$. Formally, we define $1/\eps^{2}$ boxes $B_{0},...,B_{1/\eps^{2}-1}$
such that for each  $j\in\{0,...,1/\eps^{2}-1\}$ the bottom
edge of box $B_{j}$ has the $y$-coordinate $y_{1}+j\cdot\eps^{2}h(P_H)$
and the top edge of $B_{j}$ has the $y$-coordinate $y_{1}+(j+1)\cdot\eps^{2}h(P_H)$. 
For each such $j$ we define
the $x$-coordinate of the left edge of $B_{j}$ maximally small 
such that $B_{j}\subseteq P_H$.

%\ari{For proving the lemma for the unweighted
%case, we drop all skewed (i.e., horizontal) items in $\opt'(P_H)$
%that intersect a horizontal edge of a box in $\left\{ B_{0},...,B_{1/\eps^{2}-1}\right\} $.
%Note that there can be at most $1/\eps^{2}\cdot1/\epsl$ many.
%Now consider the first $1/\eps$ boxes, i.e., $B_{0},...,B_{1/\eps-1}$.
%For each box $B_{j}\in\left\{ B_{0},...,B_{1/\eps-1}\right\} $
%consider the horizontal stripe $S_{j}:=[y_{1}+j\cdot\eps^{2}h(P_H),y_{1}+(j+1)\cdot\eps^{2}h(P)]\times[0,N]$
%(i.e., the horizontal stripe of height $\eps^{2}h(P_H)$ that contains
%$B_{j}$). In the unweighted case,  due to Lemma {\bf ?? (Lemma A)} \arir{(need to add such as lemma)}
%no small item in $\opt'$ intersects $P$ if $h(P)\le\epss N/\eps^{4}$.
%Therefore, either $h(P)\le\epss N/\eps^{2}$ in which case $P$
%does not intersect any small item in $\opt'$, or $h(P)>\epss N/\eps^{2}$
%and in this case each small item intersects with at most 2 stripes
%in $\left\{ S_{0},...,S_{1/\eps^{2}-1}\right\} $.}

In the weighted
case, from Lemma \ref{lem:A} each item $i$ contained in $P_H$ satisfies that $\height(i)\le \eps^{4} \cdot\height(P)$
and therefore each item $i$ contained in $P_H$ intersects at most
2 stripes in $\left\{ S_{0},...,S_{1/\eps^{2}-1}\right\} $.
Therefore, by the pigeon hole principle, the exists two boxes $B_{j^{*}}, B_{j^{*}+1} \in\left\{ B_{0},...,B_{1/\eps-1}\right\} $
have the property that the stripe $S'_{j^{*}}:=[0,N]\times[y_{1}+j^{*}\cdot\eps^{2}h(P_H),y_{1}+(j^{*}+2)\cdot\eps^{2}h(P_H)]$
(containing $B_{j^{*}}, B_{j^{*}+1}$) intersects at most $2\eps|\opt'(P_H)|$
of the remaining items in $\opt'(P_H)$. We drop all items in $\opt'(P_H)$
that are intersected by $S'_{j^{*}}$. Next, we move down all items
in $\opt'(P_H)$ that intersect the boxes $B_{j^{*}+1},...,B_{1/\eps^{2}-1}$
by $\eps^{2}h(P_H)$ units. Note that then they fit into the area
defined by the union of the boxes $B_{j^{*}},...,B_{1/\eps^{2}-2}$.
We assign to $B_{j^{*}}$ all items that intersect
a horizontal edge of a box in $\left\{ B_{j^{*}+1},...,B_{1/\eps^{2}-1}\right\} $.
This can be done since each such item has a height of at most $\eps^{4} \cdot\height(P_H)$
which implies that $\eps^{4} \cdot\height(P)/\eps^{2}\le\eps^{2}\cdot\height(P_H)$.

Let  $w(P_H)$ and  $w'(P_H)$  be  the length of $e_{1}$ and $e_{2}$, resp. 
Due to the definition of $\Lc$-compartment, $w(P_H)\ge \epsl N$ and $w'(P_H)\ge w(P_H)-\epsl N/2 \ge w(P_H)/2$.
Next, we would
like to ensure that below the box $B_{j^{*}}$ there is no item $i$
with $\width(i)<w'(P_H)$ (we want to achieve this since then we can
stack the items underneath $B_{j^{*}}$ on top of each other) and
no small item intersects the boundary of a box.

Therefore, consider the topmost $1/\eps^{2}-1/\eps$ boxes.
We group them into $1/6\eps-1$ groups with $6/\eps$ boxes
each, i.e., for each $k\in\{0,...,1/6\eps-2\}$ we define a group
$\B_{k}:=\{B_{j}|j\in\{1/\eps+6k/\eps,...,1/\eps+6(k+1)/\eps-1\}\}$.
Note that each group $\B_{k}$ contains exactly $6/\eps$ boxes
and below $B_{j^{*}}$ there are at most $1/\eps$ boxes. By the
pigeon hole principle, there is a value $k^{*}\in\{0,...,1/\eps-2\}$
such that the the boxes in the group $\B_{k^{*}}$ intersect with
items of total weight of $O(\eps)w(\opt'(P_H))$ where $w(\opt'(P_H))$
denotes the weight of the remaining items in $\opt'(P_H)$. Therefore,
we drop all items that intersect a box in $\B_{k^{*}}$.

Consider all items $i\in\opt'(P_H)\cap\Rsk$ that intersect at least
one of the stripes in $\left\{ S_{0},...,S_{j^{*}-1}\right\} $ and
that satisfy that $\width(i)\le w'(P_H)$. Due to Steinberg's algorithm~\cite{steinberg1997strip}
% (see Appendix~??) 
they fit into a box of height $3\eps\cdot h(P_H)$ and width $w'(P_H)$.
Therefore, all but $O(1/\epsl\cdot1/\eps)$ of them fit into $3/\eps$
boxes in $\B_{k^{*}}$. We assign them to these boxes $3/\eps$
boxes in $\B_{k^{*}}$.

%Now consider all items $i\in\opt'(P_H)\cap\Rsm$ that intersect the
%boundary of a box in $\left\{ B_{0},...,B_{1/\eps^{2}-1}\right\} $
%or that are contained in one of the stripes in $\left\{ S_{0},...,S_{j^{*}-1}\right\} $.

%\ari{In the unweighted case, if there are such items we know that $h(P_H)>\epss N/\eps^{4}$
%and hence their total area is at most $\eps\cdot h(P_H)\cdot w(P_H)+w(P_H)N\epss/\eps^{2}\le4\eps\cdot h(P_H)\cdot w'(P_H)$,
%using that $w'(P_H)\ge(1-2\eps)w(P_H)$. Also, note that for each
%item $i\in\opt'(P_H)\cap\Rsm$ we have that $\width(i)\le\epss N\le O(\eps^{2})w'(P_H)$
%and $\height(i)\le\epss N\le O(\eps^{2})w'(P_H)$. \arir{unweighted:
%needs that $\epss\le\eps^{2}\epsl$} Therefore, we can partition
%all these small items into 9 groups such that each group contains
%items with a total area of $\eps\cdot h(P_H)w'(P_H)/2$ and each group
%can be packed into a box in $\B_{k^{*}}$ using Steinberg's algorithm~\cite{steinberg1997strip}.}

In the weighted case, the total area of items $i$ that intersect
the boundary of a box in $\left\{ B_{0},...,B_{1/\eps^{2}-1}\right\} $
or that are contained in one of the stripes in $\left\{ S_{0},...,S_{j^{*}-1}\right\} $
with $\height(i)\le \eps^{4} \cdot\height(P_H)$ and $\width(i)\le\epss\cdot\width(P_H)$
is bounded by $\eps\cdot h(P_H)\cdot w(P_H)+O(w(P_H)h(P_H)\epss/\eps^{2})\le O(\eps)\cdot h(P_H)\cdot w'(P_H)$.
Hence, we can pack them into the boxes $\B_{k^{*}}$ like before using Steinberg's algorithm~\cite{steinberg1997strip}.

Now we define $P'_H$ as the acute piece induced by $e_{1}$, the bottom
edge of $B_{j^{*}}$, and the respective part of the two monotone
axis-parallel curves connecting $p_{1}=(x_{1},y_{1})$ with $p_{2}=(x_{2},y_{2})$
and the right boundary edge of $P_H$,
respectively. Each remaining item $i\in\opt'(P_H)$ intersecting $P'_H$
satisfies that $\width(i)\ge w'(P_H)$. Therefore, we can stack these
items on top of each other (using that $w'(P_H)>w(P_H)/2$).

We obtain that each remaining item from $\opt'(P_H)$ is assigned to
a box in $\left\{ B_{j^{*}},...,B_{1/\eps^{2}-1}\right\} $ or
lies in $P'_H$. We define $\opt'_{1}(P_H)$ to be the former set of items
and $\opt'_{2}(P_H)$ to be the latter set. Finally, we apply Lemma \ref{lem:make-boxes-nice} 
to each box $B\in\left\{ B_{j^{*}},...,B_{1/\eps^{2}-1}\right\} $
in order to partition $B$ further and such that the items assigned
to $B$ are nicely packed inside $B$.

We do a symmetric procedure for $P_{V}$, yielding a set of boxes
$\B_{ver}$. Intuitively, we want to define $L'$ as $P'_{H}\cup P'_{V}$.
However, $P'_{H}\cup P'_{V}$ might not have exactly the shape of
an $\Lc$-compartment. Nevertheless, one can show that we can subdivide
one of these polygons, say $P'_{H},$ along a horizontal line into
two subpolygons $P'_{H,\mathrm{top}},P'_{H,\mathrm{bottom}}$ (with
$P'_{H,\mathrm{top}}$ lying on the top of $P'_{H,\mathrm{bottom}}$)
such that 
\begin{itemize}
\item we can place the items in $P'_{H,\mathrm{top}}$ into another set
of $O_{\eps}(1)$ boxes $\B'_{hor}$ that are non-overlapping
with $\B_{hor}\cup\B_{ver}$ and 
\item $L':=P'_{H,\mathrm{bottom}}\cup P'_{V}$ forms an $\Lc$-compartment,
see Figure~??.
\end{itemize}
Then the items in $L'$ are nicely placed inside $L'$. To each of
the $O_{\eps}(1)$ boxes $B\in\B_{hor}\cup\B'_{hor}\cup\B_{ver}$
we apply a standard routine that removes some of the items inside
$B$ and partitions $B$ into smaller boxes, such that inside these
smaller boxes the remaining items are nicely placed.
It is easy to check that the resulting packing satisfy guillotine separability.


==> PPTAlgo-unweighted.tex <==
\section{Unweighted Case}
In this section we give detailed prove of Lemma~\ref{lem:algorithm}. Given a set
of compartments $\C$, let $OPT'\subseteq\R$ denote the largest subset
of $\R$ such that the items in $OPT'$ can be placed nicely in the
compartments in $\C$. Our goal is to compute a solution $ALG\subseteq\R$
with $|ALG|\ge(1-\eps)|OPT'|$ that can also be placed nicely
in $\C$. Our algorithm is an adaptation of an algorithm in \cite{GalSocg21}
for 2GK.

First, we guess for each box-compartment $B\in\C'$ whether $B$ contains
only large, only skewed, or only small items in $OPT'$ (see Definition~\ref{def:structured-boxes}).
Denote by $\C'_{large},\C'_{skew},\C'_{small}\subseteq\C'$ the respective
set of box-compartments. For the compartments in $\C'_{large}$, we
can compute the optimal way to assign items into them by an easy reduction
to bipartite matching.
\begin{lem}
(Restatement of Lemma \ref{lem:large-items})Given a set $\hat{\C}{}_{large}$ of box-compartments
such that a set of items $I_{large}^{*}\subseteq I_{large}$ can be
placed non-overlappingly inside the compartments $\hat{\C}{}_{large}$.
Then in time $n^{O(1)}$ we can we can compute a set of items $I'_{large}\subseteq I_{large}$
with $|I'_{large}|\ge|I{}_{large}^{*}|$ and a nice placement of the
items in $I'_{large}$ inside the compartments $\hat{\C}{}_{large}$.
\end{lem}
\begin{proof}
Given a set $\hat{\C}{}_{large}$ of box-compartments and set of items  $I_{large}$, we show how to pack maximum number of items in these compartments. Note that in each compartment we place exactly one large item. Now we reduce this problem to the problem of finding maximum matching in a bipartite graph. Let us create a bipartite graph $G$ in the following manner. For each compartment $C$, we create a node $X_C$ in $G$. Similarly for each large item $I$ we create a node $Y_I$ in $G$. If we can place an item in a compartment such that the item doesn't cross the boundary of the compartment, then we add between between their corresponding nodes in $G$. Clearly $G$ is a bipartite graph. Now we show that there is a feasible packing of $k$ items if and only if there is a matching of size $k$ in $G$.  

In one direction, let there be a feasible packing of $k$ items. Now consider the set of edges $E':=\{(X_C,Y_I)|\text{ $C$ contains $I$ in the feasible packing } \}$. This forms a matching of size $k$ as each compartment can contain at most $1$ item in a feasible solution and each item is in at most $1$ compartment.

In other direction, let there be a matching of size $k$. Let the set of edges in the matching be $E'$. For each edge $(X_C,Y_I)\in E'$, we add item $I$ to compartment $C$. This is a feasible solution as degree of every vertex in a matching is $1$. Also number of items which is packed is $k$. 

So in order to pack maximum number of items, it suffices to find the maximum matching in $G$. Since maximum matching in any bipartite graph can be found in time polynomial with respect to number of vertices and edges \cite{cormen2009introduction}, the statement in the Lemma follows. 
\end{proof}

For the small items, we  use a standard reduction to the generalized
assignment problem for selecting a near-optimal set of small items
and an assignment of these items into the mentioned boxes. Inside
of each box-compartment $B$ we place the items with the Next-Fit-Decreasing-Height
algorithm \cite{coffman1980performance} which results in a guillotine separable packing
for the items inside $B$. 



\begin{lem}
(Restatement of Lemma \ref{lem:small-items}) Suppose we are given a set of boxes $\B$ such that a set
of items $I_{small}^{*}\subseteq I_{small}$ can be placed non-overlappingly
inside the boxes $\B$. Then in time $n^{O_{\eps}(1)}$ 
we can compute a set of items $I'_{small}\subseteq I_{small}$ with
$|I'_{small}|\ge(1-6\eps)|I{}_{small}^{*}|$ and a nice placement
of the items in $I'_{small}$ inside the boxes $\B$.
\end{lem}
\begin{proof}
Let us first formulate an instance of generalized assignment problem (GAP).  For each compartment $C_j$ we create a bin $j$ in the GAP instance with capacity equal to its area. For each item $i\in I_{small}$, we create an item in the GAP instance with $p_{ij}=1$ and $s_{ij}$ equal to area of item $i$ if $w(i)\leq \eps w(C_j)$ and $h(i)\leq \eps h(C_j)$ and equal to some arbitrary large greater than area of $C_j$ otherwise.  Now by applying Lemma \ref{sec:GAP} on the GAP instance, we get a subset $I_{small}''\subseteq I_{small}$ to the boxes in $\B$ such that $|I_{small}''|\geq (1-3\eps)|I_{small}^{*}|$,  and sum of areas of items assigned to a box $B$ doesn't cross the area of $B$. Also for $\forall i \in I_{small}''$, $w(i)\leq \eps w(C)$ and $h(i)\leq \eps h(C)$ where $C$ is the box to which $i$ is assigned to. Let the items assigned to a box $B\in \B$ be $I_B$. In the non-increasing order of profit by area ratio we choose items from $I_B$ until the total area of chosen items crosses $(1-2\eps-\eps^2)\cdot w(B)\cdot h(B)$. Let the set of items which were chosen be $I_B'$. Clearly $|I_B'|\geq (1-2\eps-\eps^2)  |I_B|$. Now by applying Lemma \ref{lem:NFDH}, we can pack all the items of $I_B'$ in $B$ and the packing is a 2 stage packing which is guillotine separable. Applying this procedure to every box, we get a packing of set of items $I_{small}'$ into the boxes such that $|I_{small}'|\geq (1-2\eps-\eps^2)|I_{small}''| \geq (1-2\eps-\eps^2)(1-3\eps)|I_{small}^{*}|\geq (1-6\eps)|I_{small}^{*}|$    
\end{proof}

The harder part is the assignment of the skewed items. For this we
distinguish whether $|OPT'_{corr}|=O(\log N)$ or not. 

\subsection{Few items in optimal solution}

Assume first that $|OPT'_{corr}|\le c\cdot\log N$ for some constant $c$.
In this case we show that in time $(nN)^{O(c)}$ we can compute a
set of $|OPT'_{corr}\cap\Rsk|$ items from $I_{skew}$ and place them nicely
inside the compartments in $\C'_{skew}$. 
\begin{lem}
(Restatement of Lemma \ref{lem:color-coding}) In time $N^{O_{\eps}(c)}$ we can guess
a partition $\left\{ I_{skew}(C)\right\} _{C\in\C_{skew}'}$ of $I_{skew}$
such that for each $C\in\C'_{skew}$ the set $I_{skew}(C)$ contains all
items in $OPT'$ that are placed inside $C$.
\end{lem}
\begin{proof}
We employ the color coding technique \cite{alon1995color} where we seek to color the items in
$I_{skew}$ such that no two items in $OPT'_{corr}$ have the same color. Let us denote $k'=|OPT'_{corr}|$ 
If we color the items randomly with $k=c\cdot\log N$ colors, then the probability that no items in $OPT'_{corr}$ have the same color is ${k \choose k'}\frac{k'!k^{n-k'}}{k^n} \geq \big(\frac{k}{k'}\big)^{k'}\cdot \frac{k'!}{k^{k'}}\geq \frac{k'!}{k'^{k'}}\geq e^{-|OPT'_{corr}|}\ge\left(\frac{1}{N}\right)^{O(c)}$.
Using splitters \cite{cygan2015parameterized} we can derandomize this to guess such a coloring
deterministically in time $N^{O(c)}$. Once we have guessed the coloring in which item of $OPT'_{corr}$ is colored different, then, for each color $d\in\{1,...,c\cdot\log N\}$
we guess which of the $O_{\eps}(1)$ compartments in $\C'$ contains
an item of color $d$ so that the condition in the lemma is guaranteed to be achieved, which can be done deterministically in time $2^{O_{\eps}(c\cdot\log N)}=N^{O_{\eps}(c)}$ by exploring all possibilities. 
\end{proof}

In other words, the condition in Lemma~\ref{lem:color-coding} is guaranteed to be achieved in time $N^{O_{\eps}(c)}$ as we explore all the possibilities. Since we try to pack the items in all the possibilities which we mentioned previously and then choose the best packing,  we are guaranteed to get near optimal solution. 
Hence, Lemma~\ref{lem:color-coding} reduces the general case to
one independent subproblem for each compartment in $\C'_{skew}$. 
For each box-compartment $C\in\C'_{skew}$ the problem is simple: we
first guess whether horizontal or vertical items are placed inside
$C$ by $OPT'$. Then the remaining problem is equivalent to an instance
of knapsack in the cardinality case which can be solved by ordering
the items non-decreasingly by their heights/widths and selecting them
greedily in this order. For each $\Lc$-compartment $C\in\C'_{skew}$ we
 essentially invoke an algorithm from \cite{GalvezGHI0W17} as a black-box (after
some straight forward adjustments of the input items).
\begin{lem}
(Restatement of Lemma \ref{lem:pseudoL})
Given an $\Lc$-compartment $C$ and a set of items $I_{skew}(C)\subseteq I{}_{skew}$.
In time $(nN)^{O(1)}$ we can compute the subset $I_{skew}^{*}(C)\subseteq I{}_{skew}(C)$
of maximum cardinality that can be placed nicely inside $C$ and the
corresponding packing.
\end{lem}
\begin{proof}
Let us consider an $\Lc$-compartment $C$ and a set of items $I_{skew}(C)\subseteq I_{skew}$. Let the height and width of the vertical subcorridor of $C$ be $h_v$ and $w_v$ respectively. Similarly let the height and width of the vertical subcorridor of $C$ be $h_h$ and $w_h$ respectively. Now we redefine the height of a vertical item $i$ as max$( h(i), h_v-h_h)$.  If $h(i)< h_v-h_h$, then 
\begin{align*}
h_v&>h(i)+h_h\\
h_v&>2h_h \text{ (as $h(i)> h_h$ )}\\
h_v/2&>h_h\\
h_v-h_v/2&>h_h\\
h_v-h_h&>h_v/2
\end{align*}
Similarly if $h(i)\geq h_v-h_h$ then $h(i)> h_v-h(i)$ as $h(i)>h_h$. This implies that $h(i)>h_v/2$. Similarly we can redefine the width of a horizontal item  $j$ as max$( w(j), w_h-w_v)$ and we would get similar inequalities as we got for item $i$. In order to correctly apply the pseudo-polynomial time algorithm (\cite{GalvezGHI0W17}) of nice-packing the items in an $\Lc$-compartment $C$, the items have to be long (that is if the item is horizontal then the width is greater than $w_h/2$, similar analogy for the vertical items) with respect to the compartment which we are ensuring by redefining the dimensions and also we have ensure that the items whose dimension was increased after redefining it don't interact with the items in the other subcorridor. Now applying the pseudo-polynomial time algorithm of \cite{GalvezGHI0W17} on the items with redefined dimension concludes the proof of this lemma.
\end{proof}

Thus, we obtain the following lemma.
\begin{lem}
(Restatement of Lemma \ref{lem:OPT-small}) Let $c\in \mathbb{N}$. If $|OPT'|\le c\cdot\log N$
then in time $(nN)^{O(c)}$ we can compute a set of items of size
$\left|OPT'\cap I_{skew}\right|$ that can be placed nicely in the
box- and $\Lc$-compartments in $\C'_{skew}$.
\end{lem}
\begin{proof}
Using the color coding techinque Lemma \ref{lem:small-items}, we can explore all possibilities in pseudo-polynomial time. One of the possibilities has a near-optimal solution in it. This near-optimal solution contains $\left|OPT'\cap I_{skew}\right|$  items and we depicted how to pack items in $\Lc$-compartments(Lemma \ref{lem:pseudoL} ) and box-compartments (special case of knapsack) to get this near-optimal solution if we are in the possibility where the near-optimal solution exists. Since we don't know which possiblility contains the near-optimal, just considering the packing with maximum number of items serves our purpose. 
\end{proof}

\begin{figure}[]
\centering
\resizebox{!}{6cm}{
\begin{tikzpicture}
\draw[solid,fill=lightgray] (0,0) rectangle (2,2);
\draw[solid,fill=lightgray] (0,3) rectangle (2,5);
\draw[solid,fill=lightgray] (0,6) rectangle (2,8);
\draw[solid,fill=lightgray] (13,0) rectangle (15,2);
\draw[solid,fill=lightgray] (13,3) rectangle (15,5);
\draw[solid,fill=lightgray] (13,6) rectangle (15,8);
\draw[solid,fill=lightgray] (13,9) rectangle (15,11);
\draw[thick,color=blue] (2,7)--(13,10);
\draw[thick,color=blue] (2,4)--(13,7);
\draw[thick] (2,4)--(13,4);
\draw[thick] (2,4)--(13,1);
\draw[thick] (2,1)--(13,10);
\draw[thick,color=blue] (2,1)--(13,4);
\draw (1,1) node { \large\textbf{$C_3$}};
\draw (1,4) node { \large \textbf{$C_2$}};
\draw (1,7) node { \large \textbf{$C_1$}};
\draw (14,1) node { \large \textbf{$I_4$}};
\draw (14,4) node { \large \textbf{$I_3$}};
\draw (14,7) node { \large \textbf{$I_2$}};
\draw (14,10) node { \large \textbf{$I_1$}};

\end{tikzpicture}}
\caption{}
\label{bip:large}
\end{figure}

\begin{figure}[]
\centering
\resizebox{!}{2cm}{
\begin{tikzpicture}
\draw[ultra thick](6,1.5)--(6,0)--(0,0)--(0,1.5)--(6,1.5);
	
			
			\draw[solid, fill=lightgray] (.28,.06) rectangle (6,.12); 
			\draw[solid, fill=lightgray] (.34,.12) rectangle (6,.18); 
			\draw[solid, fill=lightgray] (.40,.18) rectangle (6,.24);
			\draw[solid, fill=lightgray] (.51,.26) rectangle (6,.35);
			\draw[solid, fill=lightgray] (.6,.35) rectangle (6,.43); 
			\draw[solid, fill=lightgray] (.67,.43) rectangle (6,.49);
			\draw[solid, fill=lightgray] (.76,.51) rectangle (6,.63); 
			\draw[solid, fill=lightgray] (.88,.63) rectangle (6,.73);
			\draw[solid, fill=lightgray] (1.01,.76) rectangle (6,.87); 
			\draw[solid, fill=lightgray] (1.25,.87) rectangle (6,.98);
			\draw[solid, fill=lightgray] (1.51,1.01) rectangle (6,1.19); 
			\draw[solid, fill=lightgray] (1.75,1.19) rectangle (6,1.4);
			%vertical items
			

			


\end{tikzpicture}}
\caption{}
\label{bip:large}
\end{figure}

\begin{figure}[]
\centering
\resizebox{!}{4cm}{
\begin{tikzpicture}
\draw[ultra thick](1.5,6)--(1.5,1.5)--(6,1.5)--(6,0)--(0,0)--(0,6)--(1.5,6);
	
			
			\draw[solid, fill=lightgray] (.28,.06) rectangle (6,.12); 
			\draw[solid, fill=lightgray] (.34,.12) rectangle (6,.18); 
			\draw[solid, fill=lightgray] (.40,.18) rectangle (6,.24);
			\draw[solid, fill=lightgray] (.51,.26) rectangle (6,.35);
			\draw[solid, fill=lightgray] (.6,.35) rectangle (6,.43); 
			\draw[solid, fill=lightgray] (.67,.43) rectangle (6,.49);
			\draw[solid, fill=lightgray] (.76,.51) rectangle (6,.63); 
			\draw[solid, fill=lightgray] (.88,.63) rectangle (6,.73);
			\draw[solid, fill=lightgray] (1.01,.76) rectangle (6,.87); 
			\draw[solid, fill=lightgray] (1.25,.87) rectangle (6,.98);
			\draw[solid, fill=lightgray] (1.51,1.01) rectangle (6,1.19); 
			\draw[solid, fill=lightgray] (1.75,1.19) rectangle (6,1.4);
			%vertical items
			\draw[solid, fill=lightgray] (.15,.6) rectangle (.35,6);
			\draw[solid, fill=lightgray] (.4,.8) rectangle (.60,6);
			\draw[solid, fill=lightgray] (.65,1) rectangle (.85,6);
			\draw[solid, fill=lightgray] (.9,1.2) rectangle (1.1,6);
			\draw[solid, fill=lightgray] (1.15,1.45) rectangle (1.35,6);


			


\end{tikzpicture}}
\caption{}
\label{bip:large}
\end{figure}


\begin{figure}[]
\centering
\resizebox{!}{4cm}{
\begin{tikzpicture}
\draw[ultra thick](1.5,6)--(1.5,1.5)--(6,1.5)--(6,0)--(0,0)--(0,6)--(1.5,6);
	
			\draw (0,0) rectangle (6,6);
			\draw[solid, fill=blue] (.28,.06) rectangle (6,.36); 
			 
			\draw[solid, fill=green] (2,.58) rectangle (6,1);
			
			
			%vertical items
			\draw[solid, fill=orange] (.15,.6) rectangle (.35,6);
			\draw[solid, fill=yellow] (1,.8) rectangle (1.2,6);
			
			\draw (1.5,5)--(6,5);
			\draw[solid, fill=red] (1.6,5.1) rectangle (5.8,5.9);

			\draw[solid, fill=violet] (2.15,1.6) rectangle (3.35,4.8);
			\draw[solid, fill=pink] (4,1.8) rectangle (5.2,4.7);


\end{tikzpicture}}
\caption{}
\label{bip:large}
\end{figure}

\noindent {\bf Lemma B:} A Box-compartment containing skewed items can be converted to $O_{\eps,\epsl}(1)$ nicely packed box compartments that are guillotine separable with $(1-O(\eps))$ fraction of profit.
\begin{proof}
Let us consider a box-compartment $B$ which contains only horizontal rectangles.  Now we remove the cheapest strip $S_1$ of height of $3\eps\cdot h(B)$. Note that the profit of a strip is calculated by adding the profits of the items lying completely inside the strip. So the profit of the strip $S_1$ is at most $O(\eps)\cdot \profit(B)$. Now remove the items in the strip $S_1$ and also the items which partially overlap with $S_1$. Note that the number of items which partially overlap with $S_1$ is $O_{\epsl}$. Now by using the techinque of resource augmentation, we can repack $(1-O(\eps))\profit(B)$ in a region of size $w(B)\times (1-2\eps)h(B)$ such that this region contains $O_{\eps,\epsl}(1)$ nicely packed box compartments that are guillotine separable. Now this works well in the unweighted case. But if we are dealing with a weighted case then we can't drop the $O_{\epsl}(1)$ items which we were dropping as it might contain a lot of profit. So instead we try to consider these $O_{\epsl}(1)$ as a single compartment and then divide the compartment $B$ into $O_{\epsl}(1)$ guillotine separable box compartments and repeat the process of removing strip on these compartments recursively until we find a set of items with low profit which partially overlap with the least profitable strips and this leads to the statement in the lemma as shown in the unweighted case. Now we formally describe this process. We define a pairwise disjoint set of items $K(t)$ where $0\leq t < 1/\eps$. Also for $0\leq t < 1/\eps$, let $\mathcal{K}(t):=\bigcup \limits  _{i=1}^t K(t)$. Note that we begin with $t=0$. Assume that we have computed $\mathcal{K}(t-1)$ and using it partitioned $B$ into $O_{\eps,\epsl}(1)$ guillotine separable box compartments (for $t=0$, assume that $\mathcal{K}(t-1)=\phi$ and the box $B$ itself is the partition about which we talked about). Now for each compartment not containing an item from  $\mathcal{K}(t-1)$, we consider the least profitable strip whose height is $3\eps$ times the height of the compartment. Now add all the items which partially overlap with these strips in the set $K(t)$. Let the top most and bottom most item  in $\mathcal{K}(t)$ be $I_1$ and $I_2$ respectively. Now consider minimal strip $S_t^1$ containing both $I_1$ and $I_2$. Now make the strips above and below $S_t^1$ as box compartments. Add the items which partially overlaps with this strip to $K(t+1)$. Let consider the minimal guillotine separable rectangular region $R_t^1$ inside $S_t^1$ which contains all the items of  $\mathcal{K}(t)$. Note that $R_t^1$ has same height as that of $S_t^1$. Now make the rectangular region to the left and right of $R_t^1$ as box compartments. Now consider a cut through the $R_t^1$ which divides it into 2 parts $R_t^2$ and $R_t^3$. Now recursively repeat the process done on $B$ on each of the parts $R_t^2$ and $R_t^3$ by considering the items of  $\mathcal{K}(t)$ in it until we obtain a region which contains only one item and that item belongs to $\mathcal{K}(t)$. The number of compartments created is  $O_{\eps,\epsl}(1)$ as in order to create $R_t^2$ and $R_t^3$ we added 4 extra compartments and number of items in $R_t^2$ (similarly for $R_t^3$) which are part of $\mathcal{K}(t)$ is less than that of $R_t^1$ (similarl stuff happens for each recursive call) and $|\mathcal{K}(t)|\leq O_{\eps.\epsl}(1)$. These set of compartments will be used in the timestep $t+1$. Now due to averaging argument, there will exist a timestep $t$ such that $\profit(K(t)\leq O(\eps)\profit(B)$. So the procedure of creating $O_{\eps,\epsl}(1)$ nicely packed box compartments in unweighted case can now be applied to the compartments created for the timestep $t$ and hence we will get $O_{\eps,\epsl}(1)$ nicely packed box compartments that are guillotine separable with $(1-O(\eps))$ fraction of profit.
\end{proof}



==> PPTAlgo.tex <==
\section{Assigning items into compartments\label{sec:algorithm}}

In this section we prove Lemma~\ref{lem:algorithm}. Given a set
of compartments $\C$, let $OPT'\subseteq\R$ denote the largest subset
of $\R$ such that the items in $OPT'$ can be placed nicely in the
compartments in $\C$. Our goal is to compute a solution $ALG\subseteq\R$
with $|ALG|\ge(1-\eps)|OPT'|$ that can also be placed nicely
in $\C$. Our algorithm is an adaptation of an algorithm in \cite{GalSocg21}
for 2GK.

First, we guess for each box-compartment $B\in\C'$ whether $B$ contains
only large, only skewed, or only small items in $OPT'$ (see Definition~\ref{def:structured-boxes}).
Denote by $\C'_{large},\C'_{skew},\C'_{small}\subseteq\C'$ the respective
set of box-compartments. For the compartments in $\C'_{large}$, we
can compute the optimal way to assign items into them by an easy reduction
to bipartite matching.
\begin{lem}
\label{lem:large-items}Given a set $\hat{\C}{}_{large}$ of box-compartments
such that a set of items $I_{large}^{*}\subseteq I_{large}$ can be
placed non-overlappingly inside the compartments $\hat{\C}{}_{large}$.
Then in time $n^{O(1)}$ we can we can compute a set of items $I'_{large}\subseteq I_{large}$
with $|I'_{large}|\ge|I{}_{large}^{*}|$ and a nice placement of the
items in $I'_{large}$ inside the compartments $\hat{\C}{}_{large}$.
\end{lem}
For the small items, we  use a standard reduction to the generalized
assignment problem for selecting a near-optimal set of small items
and an assignment of these items into the mentioned boxes. Inside
of each box-compartment $B$ we place the items with the Next-Fit-Decreasing-Height
algorithm \cite{coffman1980performance} which results in a guillotine separable packing
for the items inside $B$. 
\begin{lem}
\label{lem:small-items}Given a set of boxes $\B$ such that a set
of items $I_{small}^{*}\subseteq I_{small}$ can be placed non-overlappingly
inside the boxes $\B$. Then in time $n^{O_{\eps}(1)}$ we can
we can compute a set of items $I'_{small}\subseteq I_{small}$ with
$|I'_{small}|\ge(1-\eps)|I{}_{small}^{*}|$ and a nice placement
of the items in $I'_{small}$ inside the boxes $\B$.
\end{lem}
The harder part is the assignment of the skewed items. For this we
distinguish whether $|OPT'_{corr}|=O(\log N)$ or not. 

\subsection{Few items in optimal solution}

Assume first that $|OPT'|\le c\cdot\log N$ for some constant $c$.
In this case we show that in time $(nN)^{O(c)}$ we can compute a
set of $|OPT'\cap\Rsk|$ items from $I_{skew}$ and place them nicely
inside the compartments in $\C'_{skew}$. To this end, we employ the
color coding technique \cite{alon1995color} where we seek to color the items in
$I_{skew}$ such that no two items in $OPT'$ have the same color.
If we color the items randomly with $c\cdot\log N$ colors, one can
show that we obtain such a coloring with probability $e^{-|OPT'|}\ge\left(\frac{1}{N}\right)^{O(c)}$.
Using splitters \cite{cygan2015parameterized} we can derandomize this to guess such a coloring
deterministically in time $N^{O(c)}$. Then, for each color $d\in\{1,...,c\cdot\log N\}$
we guess which of the $O_{\eps}(1)$ compartments in $\C'$ contains
an item of color $d$, which can be done in time $2^{O_{\eps}(c\cdot\log N)}=N^{O_{\eps}(c)}$.
\begin{lem}
\label{lem:color-coding}In time $N^{O_{\eps}(c)}$ we can guess
a partition $\left\{ I_{skew}(C)\right\} _{C\in\C'}$ of $I_{skew}$
such that for each $C\in\C'$ the set $I_{skew}(C)$ contains all
items in $OPT'$ that are placed inside $C$.
\end{lem}
Hence, Lemma~\ref{lem:color-coding} reduces the general case to
one independent subproblem for each compartment in $\C'_{skew}$.
For each box-compartment $C\in\C'_{skew}$ the problem is simple: we
first guess whether horizontal or vertical items are placed inside
$C$ by $OPT'$. Then the remaining problem is equivalent to an instance
of knapsack in the cardinality case which can be solved by ordering
the items non-decreasingly by their heights/widths and selecting them
greedily in this order. For each $\Lc$-compartment $C\in\C'_{skew}$ we
 essentially invoke an algorithm from \cite{GalvezGHI0W17} as a black-box (after
some straight forward adjustments of the input items).
\begin{lem}\label{lem:pseudoL}
Given an $\Lc$-compartment $C$ and a set of items $I_{skew}(C)\subseteq I{}_{skew}$.
In time $(nN)^{O(1)}$ we can compute the subset $I_{skew}^{*}(C)\subseteq I{}_{skew}(C)$
of maximum cardinality that can be placed nicely inside $C$ and the
corresponding packing.
\end{lem}

Thus, we obtain the following lemma.
\begin{lem}
\label{lem:OPT-small}Let $c\in \mathbb{N}$. If $|OPT'|\le c\cdot\log N$
then in time $(nN)^{O(c)}$ we can compute a set of items of size
$\left|OPT'\cap I_{skew}\right|$ that can be placed nicely in the
box- and $\Lc$-compartments in $\C'_{skew}$.
\end{lem}

\subsection{Many items in optimal solution}

Assume now that for a constant $c_{\eps}$ to be defined later,
it holds that $|OPT'|>c_{\eps}\cdot\log N$. We group the items
in $\Rho$ into $O_{\eps}(\log N)$ groups each such that within
each group the items have essentially the same height. We do a similar
grouping with the items in $\Rve$. Formally, for each $\ell\in\{0,...,\left\lfloor \log_{1+\eps}N\right\rfloor \}$
we define $\Rho^{(\ell)}:=\{i\in\Rho|\height(i)\in[(1+\eps)^{\ell},(1+\eps)^{\ell+1})\}$
and $\Rve^{(\ell)}:=\{i\in\Rve|\width(i)\in[(1+\eps)^{\ell},(1+\eps)^{\ell+1})\}$.
For each $\ell\in\{0,...,\left\lfloor \log_{1+\eps}N\right\rfloor \}$
we round the heights of the items in $\Rho^{(\ell)}$ to $(1+\eps)^{\ell+1}$,
i.e., to the maximum height of the items in the group. Similarly,
for each $\ell\in\{0,...,\left\lfloor \log_{1+\eps}N\right\rfloor \}$
we round the widths of the items in $\Rve^{(\ell)}$ to $(1+\eps)^{\ell+1}$.
For each $\ell\in\{0,...,\left\lfloor \log_{1+\eps}N\right\rfloor \}$
we denote by $\Rbho^{(\ell)}$ and $\Rbve^{(\ell)}$ the resulting
set of items and we define $\Rbho:=\bigcup_{\ell}\Rbho^{(\ell)}$
and $\Rbve:=\bigcup_{\ell}\Rbve^{(\ell)}$. Since in the compartments
in $\C'_{skew}$ the items in $OPT'\cap\Rsk$ are packed in a very
simple way, we can show that we can find a solution $\overline{OPT}'_{skew}\subseteq\Rbho\cup\Rbve$
which contains almost as many items as $OPT'\cap\Rsk$. Do to the
rounding, the items from $OPT'_{corr}$ might not fit anymore. However,
we can repair this if for each compartment $C\in\C'$ and for each
set $\Rho^{(\ell)}$ or $\Rve^{(\ell)}$ we sacrifice an $O(\eps)$-fraction
of the items from that set placed in $C$; if between 1 and $1/\eps$
items of that set are placed inside $C$ then we still sacrifice one
item. 

\begin{lem}
There exists a solution $\overline{OPT}'_{skew}\subseteq\Rbho\cup\Rbve$
with $\left|\overline{OPT}'_{skew}\right|\ge(1-O(\eps))\left|OPT'\cap\Rsk\right|-|\C'|\left\lfloor \log_{1+\eps}N\right\rfloor $
that can be nicely placed into compartments in $\C'_{skew}$.
\end{lem}
By choosing $c_{\eps}$ sufficiently large, we will later ensure
that $|\C'|\left\lfloor \log_{1+\eps}N\right\rfloor \le\eps\left|OPT'\cap\Rsk\right|$
and hence $\left|\overline{OPT}'_{skew}\right|\ge(1-O(\eps))\left|OPT'\cap\Rsk\right|$.

We would like to guess for each group $\Rbho^{(\ell)}$ and $\Rbve^{(\ell)}$
the quantity $|\Rbho^{(\ell)}\cap\overline{OPT}'_{skew}|$ and $|\Rbve^{(\ell)}\cap\overline{OPT}'_{skew}|$,
respectively. However, there are too many options for this. Instead,
we guess estimates $\mathrm{opt}_{hor}^{(\ell)},\mathrm{opt}_{ver}^{(\ell)}$
for these values which we can guess in time $(nN)^{O_{\eps}(1)}$
for all groups in parallel, by adapting a technique from~\cite{chekuri2005polynomial}. 

\begin{lem}
\label{lem:estimate-sizes}In time $(nN)^{O_{\eps}(1)}$ we can
guess values $\mathrm{opt}_{hor}^{(\ell)},\mathrm{opt}_{ver}^{(\ell)}$
for each $\ell\in\{0,...,\left\lfloor \log_{1+\eps}N\right\rfloor \}$
such that 
\begin{itemize}
\item $\sum_{\ell}\mathrm{opt}_{hor}^{(\ell)}+\mathrm{opt}_{ver}^{(\ell)}\ge(1-\eps)|\overline{OPT}'_{skew}|$
and 
\item $\mathrm{opt}_{hor}^{(\ell)}\le|\overline{OPT}'_{skew}\cap\Rbho^{(\ell)}|$
and $\mathrm{opt}_{ver}^{(\ell)}\le|\overline{OPT}'_{skew}\cap\Rbve^{(\ell)}|$
for each $\ell\in\{0,...,\left\lfloor \log_{1+\eps}N\right\rfloor \}$. 
\end{itemize}
\end{lem}

Since in each group $\Rbho^{(\ell)}$ all items have the same height,
for each $\ell\in\{0,...,\left\lfloor \log_{1+\eps}N\right\rfloor \}$
we select the $\mathrm{opt}_{hor}^{(\ell)}$ items in $\Rbho^{(\ell)}$
of the smallest width, let $\hat{\R}_{hor}^{(\ell)}\subseteq\Rbho^{(\ell)}$
denote the resulting set. Similarly, we select the $\mathrm{opt}_{ver}^{(\ell)}$
shortest items from $\Rbve^{(\ell)}$ for each $\ell\in\{0,...,\left\lfloor \log_{1+\eps}N\right\rfloor \}$,
let $\hat{\R}_{ver}^{(\ell)}\subseteq\Rbve^{(\ell)}$ denote the resulting
set. 

Next, we do standard linear grouping \cite{vl81} with the items in the sets $\hat{\R}_{hor}^{(\ell)}/\hat{\R}_{ver}^{(\ell)}$
so that the resulting items have only $1/\eps$ different widths/heights
respectively. Formally, consider a group $\hat{\R}_{hor}^{(\ell)}$.
We sort the items in $\hat{\R}_{hor}^{(\ell)}$ non-increasingly by
width and then partition them into $1/\eps+1$ groups such that
each of the first $1/\eps$ groups contains $\left\lceil \frac{1}{1/\eps+1}|\hat{\R}_{hor}^{(\ell)}|\right\rceil $
items and the last group contains the remaining items (which might
be less than $\left\lceil \frac{1}{1/\eps+1}|\hat{\R}_{hor}^{(\ell)}|\right\rceil $
but not more). Let $\hat{\R}_{hor}^{(\ell)}=\hat{\R}_{hor,1}^{(\ell)}\dot{\cup}...\dot{\cup}\hat{\R}_{hor,1/\eps+1}^{(\ell)}$
denote the resulting partition. We drop the items in $\hat{\R}_{hor,1}^{(\ell)}$
(which are at most $\eps\cdot\left|\hat{\R}_{hor}^{(\ell)}\right|$
many). Then, for each $j\in\{2,...,1/\eps+1\}$ we increase the
width of the items in $\hat{\R}_{hor,j}^{(\ell)}$ to the width of
the widest item in $\hat{\R}_{hor,j}^{(\ell)}$. By construction,
the resulting items have $1/\eps$ different widths. Let $\tilde{\R}_{hor}^{(\ell)}$
denote the resulting set and let $\tilde{\R}_{hor}^{(\ell)}=\tilde{\R}_{hor,1}^{(\ell)}\dot{\cup}...\dot{\cup}\tilde{\R}_{hor,1/\eps}^{(\ell)}$
denote a partition of $\tilde{\R}_{hor}^{(\ell)}$ according to the
widths of the items, i.e., for each $j\in\{1,...,1/\eps\}$ the
set $\tilde{\R}_{hor,j}^{(\ell)}$ contains the rounded items from
$\hat{\R}_{hor,j+1}^{(\ell)}$. We do this procedure for each $\ell$
and a symmetric procedure for the group $\hat{\R}_{ver}^{(\ell)}$
for each $\ell$.

\begin{lem}
\label{lem:tilde-skew-solution}There exists a solution $\widetilde{OPT}'_{skew}\subseteq\bigcup_{\ell}\tilde{\R}_{hor}^{(\ell)}\cup\tilde{\R}_{ver}^{(\ell)}$
with $\left|\widetilde{OPT}'_{skew}\right|\ge(1-O(\eps))\left|\overline{OPT}'_{skew}\right|$
that can be nicely placed into the compartments in $\C'_{skew}$.
\end{lem}

Finally, for each set $\tilde{\R}_{hor,j}^{(\ell)}$ and each $C\in\C'_{skew}$
we denote by $\tilde{\R}_{hor,j}^{(\ell)}(C)$ the number of items
from $\tilde{\R}_{hor,j}^{(\ell)}$ that are assigned to $C$ in the
solution due to Lemma~\ref{lem:tilde-skew-solution}. We define $\tilde{\R}_{ver,j}^{(\ell)}(C)$
similarly for each set $\tilde{\R}_{ver,j}^{(\ell)}$ and each $C\in\C'_{skew}$.
If we could guess all the values $\left|\tilde{\R}_{hor,j}^{(\ell)}(C)\right|$
and $\left|\tilde{\R}_{ver,j}^{(\ell)}(C)\right|$ we would know exactly
which items need to be assigned into which compartment in $\C'_{skew}$,
since the items in each set $\tilde{\R}_{hor,j}^{(\ell)}(C)$ and
$\tilde{\R}_{ver,j}^{(\ell)}(C)$ are identical. It is not clear how
to guess these values $O(\log N)$ values exactly in polynomial time,
but we can guess them approximately in time $(nN)^{O_{\eps}(1)}$
while losing only a factor of $1+\eps$.

\begin{lem}
\label{lem:guess-slices}In time $(nN)^{O_{\eps}(1)}$ we can
guess values $\mathrm{opt}_{hor,j}^{(\ell)}(C),\mathrm{opt}_{ver,j}^{(\ell)}(C)$
for each $\ell\in\{0,...,\left\lfloor \log_{1+\eps}N\right\rfloor \}$,
$j\in\{1,...,1/\eps\}$, $C\in\C'_{skew}$ such that
\begin{itemize}
\item $\mathrm{opt}_{hor,j}^{(\ell)}(C)\le\left|\tilde{\R}_{hor,j}^{(\ell)}(C)\right|$
and $\mathrm{opt}_{ver,j}^{(\ell)}(C)\le\left|\tilde{\R}_{ver,j}^{(\ell)}(C)\right|$
for each $\ell,j,C$, and
\item $\sum_{C\in\C'_{skew}}\mathrm{opt}_{hor,j}^{(\ell)}(C)\ge(1-\eps)\sum_{C\in\C'_{skew}}\left|\tilde{\R}_{hor,j}^{(\ell)}(C)\right|$
for each $\ell,j$, and 
\item $\sum_{C\in\C'_{skew}}\mathrm{opt}_{ver,j}^{(\ell)}(C)\ge(1-\eps)\sum_{C\in\C'_{skew}}\left|\tilde{\R}_{ver,j}^{(\ell)}(C)\right|$
for each $\ell,j$.
\end{itemize}
\end{lem}

Consider a compartment $C\in\C'_{skew}$. From each set $\tilde{\R}_{hor,j}^{(\ell)}$
we assign exactly $\mathrm{opt}_{hor,j}^{(\ell)}(C)$ items to $C$
and from each set $\tilde{\R}_{ver,j}^{(\ell)}$ we assign exactly
$\mathrm{opt}_{ver,j}^{(\ell)}(C)$ items to $C$. If $C$ is a box-compartment then it is very simple to pack the items assinged to $C$:
if they are horizontal then we simply stack them on top of each other,
if they are vertical then we stack them side by side. If $C$ is an
$\Lc$-compartment the packing is also quite easy: assume w.l.o.g.~that
$e_{0}$ is adjacent to a vertical subcompartment and that $e_{3}$
is adjacent to a horizontal subcompartment, see Figure~??. We stack
the horizontal items on top of each other, ordered non-increasingly
by width starting at $e_{2}$, and pushed as far as possible towards
$e_{3}$. Similarly, we stack the vertical items side by side ordered
non-increasingly by by height, starting at $e_{1}$, and pushed as
far as possible towards $e_{0}$. One can show that this yields a
feasible packing (assuming that one such packing exists) and by construction
it yields a nice placement inside $C$.

\begin{lem}
Consider a compartment $C\in\C'_{skew}$. Given the values $\left\{ \mathrm{opt}_{hor,j}^{(\ell)}(C),\mathrm{opt}_{ver,j}^{(\ell)}(C)\right\} _{\ell,j}$,
in time $(nN)^{O(1)}$ we can pack items into $C$ such that they
are nicely placed inside $C$ and for each $\ell,j$ we place exactly
$\mathrm{opt}_{hor,j}^{(\ell)}(C)$ items from $\tilde{\R}_{hor,j}^{(\ell)}(C)$
and $\mathrm{opt}_{ver,j}^{(\ell)}(C)$ items from $\tilde{\R}_{ver,j}^{(\ell)}(C)$. 
\end{lem}
% \begin{figure}[t]
% \centering \includegraphics[width=0.9\linewidth]{../../../../SVN/GIT-me-github/2D-knapsack-rectangles-pseudopoly/SODA-version/Figures/LUZ}
% \caption{The three different types of LUZ-compartments and a cycle compartment}
% \label{fig:luz}
% \end{figure}

Finally, we take our packing for the items in $\tilde{\R}:=\bigcup_{\ell}\tilde{\R}_{hor}^{(\ell)}\cup\tilde{\R}_{ver}^{(\ell)}$
and replace these items by items from $\bigcup_{\ell}\R_{hor}^{(\ell)}\cup\R_{ver}^{(\ell)}$.
This is easily possible since we constructed the items in $\tilde{\R}$
by increasing the heights and widths of items in $\Rsk$.

\begin{lem}
\label{lem:OPT-large}There exists a constant $c_{\eps}\in \mathbb{N}$
such that if $|OPT'|>c_{\eps}\cdot\log N$ then in time $(nN)^{O_{\eps}(1)}$
we can compute a set of items of size $(1-\eps)\left|OPT'\cap I_{skew}\right|$
that can be placed nicely in the box- and $\Lc$-compartments in $\C'_{skew}$.
\end{lem}

Now Lemma~\ref{lem:algorithm} follows from Lemmas~\ref{lem:large-items},  \ref{lem:small-items},
\ref{lem:OPT-small}, and \ref{lem:OPT-large},
i.e., we guess if $|OPT'|\le c_{\eps}\cdot\log N$ and in this
case we invoke Lemma~\ref{lem:OPT-small} for the skewed items and
otherwise Lemma~\ref{lem:OPT-large}.


==> conclusion.tex <==

\section{Conclusion}
\label{sec:concl}
We conjecture that the worst-case ratio between the optimal profit of \tggk~and \tgk~is 4/3. Bansal et al.~\cite{bansal2014binpacking} conjectured that a similar ratio is $4/3$ for 2BP. 
If our conjecture is true, then any $\alpha$-approximation for \tggk~will imply a ${4 \alpha}/{3}$-approximation for \tgk. For example, our PPTAS will then imply a pseudo-polynomial time ${4}/{3}+\eps$-approximation for \tgk, matching the approximation guarantee in \cite{GalSocg21}. 


